Covariates-Adjusted Mixed-Membership Estimation: A Novel Network Model with Optimal Guarantees

This paper addresses the problem of mixed-membership estimation in networks, where the goal is to efficiently estimate the latent mixed-membership structure from the observed network. Recognizing the widespread availability and valuable information carried by node covariates, we propose a novel network model that incorporates both community information, as represented by the Degree-Corrected Mixed Membership (DCMM) model, and node covariate similarities to determine connections. We investigate the regularized maximum likelihood estimation (MLE) for this model and demonstrate that our approach achieves optimal estimation accuracy for both the similarity matrix and the mixed-membership, in terms of both the Frobenius norm and the entrywise loss. Since directly analyzing the original convex optimization problem is intractable, we employ nonconvex optimization to facilitate the analysis. A key contribution of our work is identifying a crucial assumption that bridges the gap between convex and nonconvex solutions, enabling the transfer of statistical guarantees from the nonconvex approach to its convex counterpart. Importantly, our analysis extends beyond the MLE loss and the mean squared error (MSE) used in matrix completion problems, generalizing to all the convex loss functions. Consequently, our analysis techniques extend to a broader set of applications, including ranking problems based on pairwise comparisons. Finally, simulation experiments validate our theoretical findings, and real-world data analyses confirm the practical relevance of our model.

==> Auxiliary.tex <==
\section{Auxiliary Results}

\begin{lemma}\label{ar:lem1}
For matrix $A\in \mathbb{R}^{n_1\times m}, B\in \mathbb{R}^{n_2\times m}$, we have
\begin{align*}
\max\{\|A\|,\|B\|\}\leq \left\|
\begin{bmatrix}
A\\
B
\end{bmatrix}
\right\|
\leq \|A\|+\|B\|.
\end{align*}
\end{lemma}

\begin{proof}[Proof of Lemma \ref{ar:lem1}]
Given $A\in \mathbb{R}^{n_1\times m}, B\in \mathbb{R}^{n_2\times m}$. We have
\begin{align*}
\left\|
\begin{bmatrix}
A\\
B
\end{bmatrix}
\right\| &= \sup_{v\in \mathbb{R}^{n_1+n_2},u\in \mathbb{R}^{m}, \|u\|_2,\|v\|_2\leq 1} v^\top \begin{bmatrix}
A\\
B
\end{bmatrix} u  \\
&= \sup_{v_1\in \mathbb{R}^{n_1},v_2\in \mathbb{R}^{n_2}, u\in \mathbb{R}^{m}, \|u\|_2 \leq 1, \sqrt{\|v_1\|_2^2+\|v_2\|_2^2} \leq 1} v_1^\top A u +v_2^\top B u \\
&\leq \sup_{v_1\in \mathbb{R}^{n_1},v_2\in \mathbb{R}^{n_2}, u\in \mathbb{R}^{m}, \|u\|_2 ,\|v_1\|_2, \|v_2\|_2\leq 1} v_1^\top A u +v_2^\top B u \\
&\leq \sup_{v_1\in \mathbb{R}^{n_1}, u\in \mathbb{R}^{m}, \|u\|_2 \|v_1\|_2\leq 1} v_1^\top A u+\sup_{v_2\in \mathbb{R}^{n_2}, u\in \mathbb{R}^{m}, \|u\|_2 ,\|v_2\|_2\leq 1} v_2^\top B u \\
&= \|A\|_2 + \|B\|_2.
\end{align*}

Given $A\in \mathbb{R}^{n_1\times m}, B\in \mathbb{R}^{n_2\times m}$. We have
\begin{align*}
\left\|
\begin{bmatrix}
A\\
B
\end{bmatrix}
\right\| &= \sup_{v\in \mathbb{R}^{n_1+n_2},u\in \mathbb{R}^{m}, \|u\|_2,\|v\|_2\leq 1} v^\top \begin{bmatrix}
A\\
B
\end{bmatrix} u  \\
&= \sup_{v_1\in \mathbb{R}^{n_1},v_2\in \mathbb{R}^{n_2}, u\in \mathbb{R}^{m}, \|u\|_2 \leq 1, \sqrt{\|v_1\|_2^2+\|v_2\|_2^2} \leq 1} v_1^\top A u +v_2^\top B u \\
&\geq \sup_{v_1\in \mathbb{R}^{n_1},v_2\in \mathbb{R}^{n_2}, u\in \mathbb{R}^{m}, \|u\|_2 \leq 1, \sqrt{\|v_1\|_2^2+\|v_2\|_2^2} \leq 1, v_2 = 0} v_1^\top A u +v_2^\top B u \\
&= \sup_{v_1\in \mathbb{R}^{n_1}, u\in \mathbb{R}^{m}, \|u\|_2 \leq 1, \|v_1\|_2 <= 1} v_1^\top A u = \|A\|_2.
\end{align*}

\end{proof}


\begin{lemma}\label{ar:lem3}
Suppose \( F_1, F_2, F_0 \in \mathbb{R}^{2n \times r} \) are three matrices such that
\[
\|F_1 - F_0\| \|F_0\| \leq \sigma_r^2(F_0)/2 \quad \text{and} \quad \|F_1 - F_2\| \|F_0\| \leq \sigma_r^2(F_0)/4,
\]
where \(\sigma_i(A)\) stands for the \(i\)-th largest singular value of \(A\). Denote
\[
\mathbf{R}_1 \triangleq \arg \min_{\mathbf{R} \in \cO^{r \times r}} \|F_1 \mathbf{R} - F_0\|_F \quad \text{and} \quad \mathbf{R}_2 \triangleq \arg \min_{\mathbf{R} \in \cO^{r \times r}} \|F_2 \mathbf{R} - F_0\|_F.
\]
Then the following two inequalities hold:
\[
\|F_1 \mathbf{R}_1 - F_2 \mathbf{R}_2\| \leq \frac{5 \sigma_1^2(F_0)}{\sigma_r^2(F_0)} \|F_1 - F_2\| \quad \text{and} \quad \|F_1 \mathbf{R}_1 - F_2 \mathbf{R}_2\|_F \leq \frac{5 \sigma_1^2(F_0)}{\sigma_r^2(F_0)} \|F_1 - F_2\|_F.
\]
\end{lemma}
\begin{proof}[Proof of Lemma \ref{ar:lem3}]
See Lemma 37 in \cite{ma2018implicit}.
\end{proof}


\begin{lemma}\label{ar:lem2}
Suppose Lemma \ref{lem:ncv1}-Lemma \ref{lem:ncv5} hold for the $t$-th iteration. We then have
\begin{align*}
\left\|F^{t,(m)}R^{t,(m)}-F^{t}R^t\right\|_F\leq 5\kappa  \left\|F^{t,(m)}O^{t,(m)}-F^{t}R^t\right\|_F.    
\end{align*}
\end{lemma}
\begin{proof}[Proof of Lemma \ref{ar:lem2}]
By Lemma \ref{lem:ncv1}, we have
\begin{align*}
\|F^tR^t-F^*\|\|F^*\|\leq \sigma_r^2(F^*)/2.
\end{align*}
Note that
\begin{align*}
  \|F^{t,(m)}R^{t,(m)}-F^{t}R^t\|_F
  &\leq \|F^{t,(m)}R^{t,(m)}-F^*\|_F+\|F^*-F^{t}R^t\|_F\\
  &\leq  \|F^{t,(m)}O^{t,(m)}-F^*\|_F+\|F^*-F^{t}R^t\|_F \tag{by the definition of $R^{t,(m)}$}\\
  &\leq   \|F^{t,(m)}O^{t,(m)}-F^{t}R^t\|_F+2\|F^*-F^{t}R^t\|_F\\
  &\leq c_{21}+2c_{11}\sqrt{n}.
\end{align*}
Thus, it holds that
\begin{align*}
\|F^{t,(m)}R^{t,(m)}-F^{t}R^t\|\|F^*\|
\leq \|F^{t,(m)}R^{t,(m)}-F^{t}R^t\|_F\|F^*\|
\leq \sigma_r^2(F^*)/4.
\end{align*}
Then by Lemma \ref{ar:lem3} with $F_0=F^*, F_1=F^tR^t, F_2=F^{t,(m)}O^{t,(m)}$, we have
\begin{align*}
\left\|F^{t,(m)}R^{t,(m)}-F^{t}R^t\right\|_F
&\leq  
\frac{5 \sigma_1^2(F^*)}{\sigma_r^2(F^*)} 
\left\|F^{t,(m)}O^{t,(m)}-F^{t}R^t\right\|_F\\
&=\frac{5 \sigma_{\max}}{\sigma_{\min}} 
\left\|F^{t,(m)}O^{t,(m)}-F^{t}R^t\right\|_F.
\end{align*}
\end{proof}



\begin{lemma}\label{ar:lem4}
Suppose Lemma \ref{lem:ncv1}-Lemma \ref{lem:ncv5} hold for the $t$-th iteration. We then have
\begin{align*}
\sigma_{\min}/2\leq \sigma_{\min}\left(\left(Y^{t,(m)}R^{t,(m)}\right)^TY^{t,(m)}R^{t,(m)}\right)\leq \sigma_{\max}\left(\left(Y^{t,(m)}R^{t,(m)}\right)^TY^{t,(m)}R^{t,(m)}\right)\leq 2\sigma_{\max}.
\end{align*}
\end{lemma}
\begin{proof}[Proof of Lemma \ref{ar:lem4}]
By Weyl's inequality, we have
\begin{align*}
&\left|\sigma_{\min}\left(\left(Y^{t,(m)}R^{t,(m)}\right)^TY^{t,(m)}R^{t,(m)}\right)-\sigma_{\min}\right|\\
    &=\left|\sigma_{\min}\left(\left(Y^{t,(m)}R^{t,(m)}\right)^TY^{t,(m)}R^{t,(m)}\right)-\sigma_{\min}\left(Y^{*T}Y^*\right)\right|\\
    &\leq \left\|\left(Y^{t,(m)}R^{t,(m)}\right)^TY^{t,(m)}R^{t,(m)}-Y^{*T}Y^*\right\|\\
    &\leq \left\|Y^{t,(m)}R^{t,(m)}-Y^*\right\|\left(\left\|Y^{t,(m)}R^{t,(m)}\right\|+\left\|Y^*\right\|\right)\\
    &\leq  \left\|Y^{t,(m)}R^{t,(m)}-Y^*\right\|\left(\left\|Y^{t,(m)}R^{t,(m)}-Y^*\right\|+2\left\|Y^*\right\|\right).
\end{align*}
Note that
\begin{align*}
\|Y^{t,(m)}R^{t,(m)}-Y^*\|
&\leq \|F^{t,(m)}R^{t,(m)}-F^*\|\\
&\leq \|F^{t,(m)}R^{t,(m)}-F^tR^t\|+\|F^tR^t-F^*\|\\
&\leq 5\kappa\|F^{t,(m)}O^{t,(m)}-F^tR^t\|_F+\|F^tR^t-F^*\|\tag{by Lemma \ref{ar:lem2}}\\
&\lesssim c_{11}\sqrt{n}
\end{align*}
and $\|Y^*\|=\sqrt{\sigma_{\max}}$.
We then have
\begin{align*}
 \left|\sigma_{\min}\left(\left(Y^{t,(m)}R^{t,(m)}\right)^TY^{t,(m)}R^{t,(m)}\right)-\sigma_{\min}\right|\lesssim c_{11}\sqrt{n\sigma_{\max}}\leq    \sigma_{\min}/2,
\end{align*}
which implies 
\begin{align*}
\sigma_{\min}\left(\left(Y^{t,(m)}R^{t,(m)}\right)^TY^{t,(m)}R^{t,(m)}\right)\geq  \sigma_{\min}/2.   
\end{align*}
Similarly, we can show that
\begin{align*}
\sigma_{\max}\left(\left(Y^{t,(m)}R^{t,(m)}\right)^TY^{t,(m)}R^{t,(m)}\right)\leq 2\sigma_{\max}.
\end{align*}
\end{proof}



\begin{lemma}\label{ar:lem5}
Let \( S \in \mathbb{R}^{r \times r} \) be a nonsingular matrix. Then for any matrix \( K \in \mathbb{R}^{r \times r} \) with \(\|K\| \leq \sigma_{\min}(S)\), one has
\[
\| \text{sgn}(S + K) - \text{sgn}(S) \| \leq \frac{2}{\sigma_{r-1}(S) + \sigma_r(S)} \|K\|,
\]
where \(\text{sgn}(\cdot)\) denotes the matrix sign function, i.e. \(\text{sgn}(A) = UV^\top\) for a matrix \( A \) with SVD \( U \Sigma V^\top \).
\end{lemma}
\begin{proof}
See Lemma 36 in \cite{ma2018implicit}. 
\end{proof}



\begin{lemma}\label{ar:lem6}
Let $U \Sigma V^\top$ be the SVD of a rank-$r$ matrix $XY^\top$ with $X, Y \in \mathbb{R}^{n \times r}$. Then there exists an invertible matrix ${Q} \in \mathbb{R}^{r \times r}$ such that $X = U \Sigma^{1/2} {Q}$ and $Y = V \Sigma^{1/2} {Q}^{-T}$. In addition, one has
\begin{align*}
    \| \Sigma_{Q} - \Sigma_{{Q}}^{-1} \|_F &\leq \frac{1}{\sigma_{\min} (\Sigma)} \| X^\top X - Y^\top Y \|_F, \tag{140}
\end{align*}
where $U_Q \Sigma_Q V_Q^\top$ is the SVD of ${Q}$. In particular, if $X$ and $Y$ have balanced scale, i.e., $X^\top X - Y^\top Y = 0$, then ${Q}$ must be a rotation matrix.
\end{lemma}
\begin{proof}
See Lemma 20 in \cite{ma2018implicit}. 
\end{proof}

==> convex-nonconvex.tex <==
\section{Bridge convex optimizer and approximate nonconvex optimizer}\label{sec:cv_ncv}
In Section \ref{sec:ncv_debias}, we obtain the distributional results for $(\hat{\theta}^d, \hat{H}^d, \hat{X}^d\hat{Y}^{dT})$, which is the debiased estimator based on the nonconvex optimization problem. However, the nonconvex optimizer $(\hat{\theta}, \hat{H}, \hat{X}, \hat{Y})$ is obtained by running GD starting from the ground truth $({\theta}^*, {H}^*, {X}^*, {Y}^*)$, which cannot be implemented in practice. Practically, to do inference: (1) first, we solve the convex optimization problem defined in \eqref{obj:cv} with the constraint that $\mathbf{1}^T\theta=0$ and obtain $(\hat{\theta}_c, \hat{H}_c, \hat{\Gamma}_c)$; (2) second, we obtain $(\hat{X}_c, \hat{Y}_c)$ based on the SVD of $\hat{\Gamma}_c$; (3) third, we obtain the debiased estimator $(\hat{\theta}^d_c, \hat{H}^d_c, \hat{X}^d_c, \hat{Y}^d_c)$ given by
\begin{align*}
 \begin{bmatrix}
\hat{\theta}^d_c-\hat{\theta}_c\\
\hat{H}^d_c-\hat{H}_c\\
\hat{X}^d_c-\hat{X}_c\\
\hat{Y}^d_c-\hat{Y}_c
\end{bmatrix}:=-(\cP \hat{D}_c \cP)^{\dagger}  \cP \nabla L(\hat{\theta}_c,\hat{H}_c,\hat{X}_c,\hat{Y}_c)
\text{ where }
\hat{D}_c:=
\sum_{i\neq j}\frac{e^{\hat{P_c}_{ij}}}{(1+e^{\hat{P_c}_{ij}})^2}
\begin{bmatrix}
\frac{1}{\sqrt{n}}(e_i+e_j)\\
z_iz_j^T\\
\frac1ne_ie_j^T\hat{Y}_c\\
\frac1ne_je_i^T\hat{X}_c
\end{bmatrix}^{\otimes 2}.
\end{align*}
It then satisfies:
\begin{align*}
\cP\left(
\nabla L(\hat{\theta}_c,\hat{H}_c,\hat{X}_c,\hat{Y}_c)+
\hat{D}_c
\begin{bmatrix}
\hat{\theta}^d_c-\hat{\theta}_c\\
\hat{H}^d_c-\hat{H}_c\\
\hat{X}^d_c-\hat{X}_c\\
\hat{Y}^d_c-\hat{Y}_c
\end{bmatrix}
\right)=0
\text{ and }
\cP\begin{bmatrix}
\hat{\theta}^d_c\\
\hat{H}^d_c\\
\hat{X}^d_c\\
\hat{Y}^d_c
\end{bmatrix}=\begin{bmatrix}
\hat{\theta}^d_c\\
\hat{H}^d_c\\
\hat{X}^d_c\\
\hat{Y}^d_c
\end{bmatrix}.
\end{align*}
(4) finally, we use the distributional results on $(\hat{\theta}^d_c, \hat{H}^d_c, \hat{X}^d_c\hat{Y}^{dT}_c)$ to do inference.

In the following, we show that the convex optimizer $(\hat{\theta}_c, \hat{H}_c, \hat{X}_c\hat{Y}^{T}_c)$ is close to the nonconvex optimizer $(\hat{\theta}, \hat{H}, \hat{X}\hat{Y}^{T})$ in Theorem \ref{thm:cv_ncv}. 

% In the following, we establish the distributional results for the convex debiased estimator $(\hat{\theta}^d_c, \hat{H}^d_c, \hat{X}^d_c\hat{Y}^{dT}_c)$. We first show that the convex and nonconvex optimizer $(\hat{\theta}_c, \hat{H}_c, \hat{X}_c\hat{Y}^{T}_c)$ is close to $(\hat{\theta}, \hat{H}, \hat{X}\hat{Y}^{T})$ in Theorem \ref{thm:cv_ncv}. 
% We then show that the debiased estimators $(\hat{\theta}^d_c, \hat{H}^d_c, \hat{X}^d_c\hat{Y}^{dT}_c)$ and $(\hat{\theta}^d, \hat{H}^d, \hat{X}^d\hat{Y}^{dT})$ are also close to each other in Theorem \ref{thm:cvd_ncvd}. Finally, based on the distributional results for $(\hat{\theta}^d, \hat{H}^d, \hat{X}^d\hat{Y}^{dT})$ obtained in Section \ref{sec:ncv_debias}, we obtain the distributional results for $(\hat{\theta}^d_c, \hat{H}^d_c, \hat{X}^d_c\hat{Y}^{dT}_c)$ in Theorem \ref{thm:cv_distribution}.



\begin{assumption}\label{assumption:r+1}
We define a matrix $M^{*}$ such that
\begin{align*}
M^{*}_{ij}=
\begin{cases}
    \frac{e^{P_{ij}^*}}{(1+e^{P_{ij}^*})^2} & i\neq j\\
    0 & i=j.
\end{cases}
\end{align*}
Let $D^*$ be defined as that in Section \ref{sec:ncv_debias} and $(\Delta_{\theta}, \Delta_{H}, \Delta_{X}, \Delta_{Y})$ given by
\begin{align*}
 \begin{bmatrix}
\Delta_{\theta}\\
\Delta_{H}\\
\Delta_{X}\\
\Delta_{Y}
\end{bmatrix}
=-(\cP D^*\cP)^{\dagger}\begin{bmatrix}
0\\
0\\
-X^{*}\\
-Y^{*}
\end{bmatrix}
\end{align*}
% \begin{align*}
% \begin{cases}
% \begin{bmatrix}
% 0\\
% 0\\
% -X^{*}\\
% -Y^{*}
% \end{bmatrix}
% +\cP D^*\cP
%  \begin{bmatrix}
% \Delta_{\theta}\\
% \Delta_{H}\\
% \Delta_{X}\\
% \Delta_{Y}
% \end{bmatrix}
% =0\\
% \cP_{\theta}(\Delta_{\theta})=\Delta_{\theta}
% \end{cases}.
% \end{align*}
We assume that there exists a constant $\epsilon > 0$ such that
\begin{align*}
    \sigma_{r+1}\left(\frac{1}{n}{M}^* \odot \left(\frac{(\Delta_{\theta})_i+(\Delta_{\theta})_j}{\sqrt{n}}+{z}_i^T\Delta_{H}{z}_j+\frac{(\Delta_{X}{Y}^{*T}+{X}^*{\Delta^T_{Y}})_{ij}}{n}\right)_{ij}\right) <1-\epsilon.
\end{align*}
\end{assumption}
This assumption may not seem intuitive at first glance, but we will demonstrate that it holds true for a wide range of cases.


\begin{proposition}\label{prop:assumption_example}
Assumption \ref{assumption:r+1} holds for the stochastic block model with two communities. More specifically, Assumption \ref{assumption:r+1} holds when $\theta^*=0,H^*=0$ and
\begin{align*}
\Gamma^*=
\begin{bmatrix}
p\mathbf{1}\mathbf{1}^T & q\mathbf{1}\mathbf{1}^T\\
q\mathbf{1}\mathbf{1}^T & p\mathbf{1}\mathbf{1}^T\\
\end{bmatrix},
\end{align*}
where $\mathbf{1}\in\bbR^{\frac{n}{2}\times 1}$ is an all one vector and $p>q$.
\end{proposition}
\begin{proof}
See Appendix \ref{pf:prop_assumption_example}.
\end{proof}

% \textcolor{red}{Add one more example: $\theta^*=0, \Gamma^*=0$, what condition should $\{z_i\}$ and $H^*$ satisfy so that Assumption \ref{assumption:r+1} holds?}


\begin{theorem}\label{thm:cv_ncv}
Suppose Assumption \ref{assumption:r+1} holds. We then have
\begin{align*}
\left\|
\begin{bmatrix}
\hat{\theta}_c-\hat{\theta}\\
\hat{H}_c-\hat{H}\\
\frac{1}{n}(\hat{\Gamma}_c-\hat{X}\hat{Y}^T)
\end{bmatrix}
\right\|_F
\lesssim \frac{(1+e^{c c_P})^2}{\sl e^{c c_P}}\left(1+\frac{ 72 \kappa n}{\sqrt{\sigma_{\min}}}\right)\|\cP(\nabla f(\hat{\theta},\hat{H},\hat{X},\hat{Y}))\|_F
\end{align*}
for some constant $c$.
\end{theorem}
\begin{proof}
See Appendix \ref{pf:thm_cv_ncv}. \ntc
\end{proof}


\begin{corollary}\label{cor:cv_ncv} We have
\begin{align*}
&\|\hat{\Gamma}_c-\Gamma^{*}\|\lesssim \sqrt{\sigma_{\max}n}c_{14}\\
&\|\hat{\Gamma}_c-\Gamma^{*}\|_{F}\lesssim \sqrt{\sigma_{\max}n}c_{11}\\
&\|\hat{\Gamma}_c-\Gamma^{*}\|_{\infty}\lesssim \sqrt{\mu\sX\sY r^2 n}c_{43}.
\end{align*}
\end{corollary}
\begin{proof}
See Appendix \ref{pf:cor_cv_ncv}.
\end{proof}


% \begin{theorem}\label{thm:cvd_ncvd}
% \ntd
% \end{theorem}
% \begin{proof}
% See Appendix \ref{pf:thm_cvd_ncvd}.
% \end{proof}




% \begin{theorem}\label{thm:cv_distribution}
% \ntd  
% \end{theorem}
% \begin{proof}
% See Appendix \ref{pf:thm_cv_distribution}.
% \end{proof}

==> convexity.tex <==
\section{Local geometry}
We define
\begin{align*}
f_{\aug}(\theta,H,X,Y):= f(\theta,H,X,Y)+\frac{c_{\aug}}{n^2}\|X^TX-Y^TY\|^2_{F},
\end{align*}
where $c_{\aug}=\frac{\sl e^{2c_P}}{8(1+e^{2c_P})^2}$.
\begin{lemma}[Local geometry]\label{lem:convexity}
Let $\Delta=\begin{bmatrix}
\Delta_{\theta}\\ \Delta_H\\ \Delta_X\\ \Delta_Y
\end{bmatrix}$. Under assumptions given in Section \ref{sec:assumptions}, with probability at least $1-n^{-10}$, we have
\begin{align*}
&\vec(\Delta)^T\nabla^2f_{\aug}(\theta,H,X,Y)\vec(\Delta)\\
&\geq  \sl\frac{e^{2c_P}}{(1+e^{2c_P})^2}\left(  \|\Delta_{\theta}\|^2_F+\|\Delta_{H}\|^2_F+ \frac{\sigma_{\min}}{8n^2}\left(\left\| \Delta_X \right\|_F^2 + \left\|  \Delta_Y \right\|_F^2 \right)\right)
\geq \sl\frac{e^{2c_P}}{(1+e^{2c_P})^2}\cdot\min\left\{1,\frac{\sigma_{\min}}{8n^2}\right\}\|\Delta\|^2_F,\\
&\max\left\{\left\|\nabla^2f_{\aug}(\theta,H,X,Y)\right\|,\left\|\nabla^2f(\theta,H,X,Y)\right\|\right\}\leq  \max\left\{\su,\frac{20\su\sigma_{\max}}{n^2}\right\}
\end{align*}
for $(\theta,H,X,Y)$ obeying $\mathbf{1}^T\theta=0$ and
\begin{align*}
\|\theta-\theta^{*}\|_{\infty}\leq c_1,\ \|H-H^{*}\|_{F}\leq c_2\sqrt{n},\ \left\|
\begin{bmatrix}
XR-X^*\\
YR-Y^*
\end{bmatrix}\right\|_{2,\infty}\leq c_3,
\end{align*}
$\Delta_{\theta}$ such that $\mathbf{1}^T\Delta_{\theta}=0$ and $\begin{bmatrix}\Delta_X\\\Delta_Y\end{bmatrix}$ lying in the set
\begin{align*}
\left\{
\begin{bmatrix}
X_1\\Y_1
\end{bmatrix}
\hat{R}-
\begin{bmatrix}
X_2\\Y_2
\end{bmatrix}\bigg|
\left\|\begin{bmatrix}
X_2-X^*\\Y_2-Y^*
\end{bmatrix}\right\|\leq c_4 \sqrt{n},
% \|X_2-X^*\|\lesssim \sqrt{n},\ \|Y_2-Y^*\|\lesssim \sqrt{n},
\ \hat{R}:=\argmin_{R\in\cO^{r\times r}}
\left\|\begin{bmatrix}
X_1\\Y_1
\end{bmatrix}
R-
\begin{bmatrix}
X_2\\Y_2
\end{bmatrix}\right\|_F
\right\}.
\end{align*}
\end{lemma}
\begin{proof}
See Appendix \ref{proof_convexity}.
\end{proof}

\begin{remark}

\textcolor{blue}{Here we only visualize the $n$ dependency and $c_1,c_2,c_3,c_4$ may involve $r,p, \sigma_{\max},\sigma_{\min}, \log n$, etc.}
For notation simplicity, we denote
\begin{align*}
\underline{C}:=\sl\frac{e^{2c_P}}{(1+e^{2c_P})^2}\cdot\min\left\{1,\frac{\sigma_{\min}}{8n^2}\right\},\quad
\overline{C}:= \max\left\{\su,\frac{20\su\sigma_{\max}}{n^2}\right\}.
\end{align*}
\end{remark}




% \begin{lemma}[Local convexity]\label{lem:convexity}
% Let $\Delta=\begin{bmatrix}
% \Delta_{\theta}\\ \Delta_H\\ \Delta_X\\ \Delta_Y
% \end{bmatrix}$. With probability at least $1-n^{-10}$, we have
% \begin{align*}
% \vec(\Delta)^T\nabla^2f_{\aug}(\theta,H,X,Y)\vec(\Delta)&\lesssim \|\Delta_{\theta}\|^2_F+\|\Delta_{H}\|^2_F+\left(\lambda+\frac{\sigma_{\max}}{n^2}\right)\left(\|\Delta_{X}\|^2_F+\|\Delta_{Y}\|^2_F\right),\\
% \vec(\Delta)^T\nabla^2f_{\aug}(\theta,H,X,Y)\vec(\Delta)&\gtrsim\|\Delta_{\theta}\|^2_F+\|\Delta_{H}\|^2_F+\left(\lambda+\frac{\sigma_{\min}}{n^2}\right)\left(\|\Delta_{X}\|^2_F+\|\Delta_{Y}\|^2_F\right),
% \end{align*}
% for $(\theta,H,X,Y)$ obeying $\mathbf{1}^T\theta=0$ and
% \begin{align*}
% \|\theta-\theta^{*}\|_{\infty}\lesssim 1,\ \|H-H^{*}\|_{F}\lesssim\sqrt{n},\ \left\|
% \begin{bmatrix}
% XR-X^*\\
% YR-Y^*
% \end{bmatrix}\right\|_{2,\infty}\lesssim 1,
% % \|XY^T-X^{*}Y^{*T}\|_{F}\lesssim n^{3/2},
% \end{align*}
% $\Delta_{\theta}$ such that $\mathbf{1}^T\Delta_{\theta}=0$ and $\begin{bmatrix}\Delta_X\\\Delta_Y\end{bmatrix}$ lying in the set
% \begin{align*}
% \left\{
% \begin{bmatrix}
% X_1\\Y_1
% \end{bmatrix}
% \hat{R}-
% \begin{bmatrix}
% X_2\\Y_2
% \end{bmatrix}\bigg|
% % \left\|\begin{bmatrix}
% % X_2-X^*\\Y_2-Y^*
% % \end{bmatrix}\right\|\lesssim \sqrt{n},
% \|X_2-X^*\|\lesssim \sqrt{n},\ \|Y_2-Y^*\|\lesssim \sqrt{n},
% \ \hat{R}:=\argmin_{R\in\cO^{r\times r}}
% \left\|\begin{bmatrix}
% X_1\\Y_1
% \end{bmatrix}
% R-
% \begin{bmatrix}
% X_2\\Y_2
% \end{bmatrix}\right\|_F
% \right\}.
% \end{align*}
% \end{lemma}
% \textcolor{red}{
% Need to be changed to the same statement as that in Lemma 17 in \cite{chen2020noisy}.
% }
% \begin{proof}
% See Appendix \ref{proof_convexity}.
% \end{proof}

% \begin{remark}
% Lemma \ref{lem:convexity} implies that
% \begin{align*}
%     \vec(\Delta)^T\nabla^2f(\theta,H,X,Y)\vec(\Delta)&\lesssim \|\Delta_{\theta}\|^2_F+\|\Delta_{H}\|^2_F+\left(\lambda+\frac{\sigma_{\max}}{n^2}\right)\left(\|\Delta_{X}\|^2_F+\|\Delta_{Y}\|^2_F\right).
% \end{align*}
% \end{remark}

==> inference.tex <==
\section{Inference}
next paper

==> membership_est.tex <==
\section{Membership Estimation}\label{sec:mem_est}
In the previous section, we obtain the estimator $\hat{\Gamma}_c$ by solving the convex optimization problem. In this section, we reconstruct the membership $\Pi^*$ based on $\hat{\Gamma}_c$.

Let $U^*\Sigma^* V^{*\top}$ be the SVD of $\Gamma^*=\Pi^* P \Pi^{*\top}$. There exists a unique non-singular matrix $B\in\bbR^{r\times r}$ 
such that $U^*=\Pi^* B$, i.e.,
\begin{align*}
\begin{bmatrix}
    {u}_1^{* \top}\\
    \vdots\\
    {u}_n^{* \top}
    \end{bmatrix}
=
\begin{bmatrix}
    {\pi}_1^{* \top}\\
    \vdots\\
    {\pi}_n^{* \top}
    \end{bmatrix}
\begin{bmatrix}
    {v}_1^{\top}\\
    \vdots\\
    {v}_r^{\top}
    \end{bmatrix}.
\end{align*}
Thus, we have ${u}_i^{* }=\sum^r_{\ell=1}{\pi}_{i}^{* }(\ell)v_{\ell}$ for all $i\in [n]$.

Inspired by the above observations, we consider the following three-step procedure:
\begin{enumerate}
    \item \textbf{Score step}: Obtain $\hat{U}_c=\begin{bmatrix}
    \hat{u}_1^{\top}\\
    \vdots\\
    \hat{u}_n^{\top}
    \end{bmatrix}\in\bbR^{n\times r}$ by SVD of $\hat{\Gamma}_c$ (i.e., $\hat{\Gamma}_c=\hat{U}_c\hat{\Sigma}_c\hat{V}_c^{\top}$).

    \item \textbf{Vertex Hunting step}: Run a convex hull algorithm on the rows of $\hat{U}_c$. Denote vertices of the obtained convex hull by $\{\hat{v}_{\ell}\}_{\ell = 1}^r$.


    \item \textbf{Membership Reconstruction step}:
    For each $i\in [n]$: solve $\hat{u}_i = \sum^r_{\ell=1}\pi_i(\ell)\hat{v}_{\ell}$ to obtain $\hat{\pi}_i$.

\end{enumerate}

Finally, we output
\begin{align*}
 \hat{\Pi}_c:=
 \begin{bmatrix}
\hat{\pi}_1^{\top}\\
    \vdots\\
    \hat{\pi}_n^{\top}
 \end{bmatrix}.
\end{align*}

\begin{definition}[Efficient Vertex Hunting]\label{def:eff_vh}
A Vertex Hunting algorithm is efficient if it satisfies
\begin{align*}
\max_{1\leq \ell\leq r}\|\hat{v}_{\ell}-v_{\ell}\|\leq C \max_{1\leq i\leq n}\|\hat{u}_{i}-u_{i}\|
\end{align*}
for some constant $C$.
\end{definition}

\begin{assumption}\label{assumption:mem_est}
Let $G=\frac{r}{n}(\Pi^{*\top}\Pi^{*})$. We assume $\|G\|\leq C$ and $\|G^{-1}\|\leq C$ for some constant $C$.  
\end{assumption}


\begin{theorem}
\label{thm:mem_est}
Let $\hat{\Pi}_c\in\bbR^{n\times r}$ be the membership estimation given by $\hat{\Gamma}_c$. Suppose there is an efficient Vertex Hunting algorithm available.
Under Assumption \ref{assumption:mem_est}, it holds that
\begin{align*}
\|\hat{\Pi}_c -\Pi^*\|_{2,\infty}\lesssim \sqrt{\frac{1}{nr}}\left(\frac{n}{\sqrt{\sigma_{\min}}}c_{43}+\frac{n^2}{\sigma_{\min}}\sqrt{\kappa\mu\sX\sY r^2 }c_{14}\right).
\end{align*}
\end{theorem}
\begin{proof}
See Appendix \ref{pf:thm_mem_est}.
\end{proof}

==> nonconvex_debias.tex <==
\section{Properties of debiased nonconvex estimator}\label{sec:ncv_debias}
Let 
\begin{align*}
&t^*:=\argmin_{0\leq t<t_0}\left\|
\nabla f(M^{t},F^{t})
-
\begin{bmatrix}
\mean\left(\nabla_{\theta}f(M^{t},F^{t})\right)\cdot\mathbf{1}\\
0
\end{bmatrix} 
\right\|_F.
\end{align*}
And we denote $(\hat{\theta},\hat{H},\hat{X},\hat{Y})=({\theta}^{t^{*}},{H}^{t^{*}},{X}^{t^{*}}R^{t^{*}},{Y}^{t^{*}}R^{t^{*}})$. It then holds that
\begin{align}\label{ncv:est}
&\|\hat{\theta}-\theta^{*}\|_{\infty}\leq c_{41},\ \|\hat{H}-H^{*}\|_F\leq c_{11}\sqrt{n},\ \|\hat{X}-X^{*}\|_{2,\infty}\leq c_{43},\
\|\hat{Y}-Y^{*}\|_{2,\infty}\leq c_{43},\\\label{ncv:grad}
&\left\|\nabla f(\hat{\theta},\hat{H},\hat{X},\hat{Y})-
\begin{bmatrix}
\mean\left(\nabla_{\theta}f(\hat{\theta},\hat{H},\hat{X},\hat{Y})\right)\cdot\mathbf{1}\\
0
\end{bmatrix}
\right\|_F\lesssim n^{-5}.
\end{align}


We define a projection matrix $\cP$ such that
\begin{align}\label{def:projection}
\cP:=
\begin{bmatrix}
\cP_{\theta} & \\
 & I
\end{bmatrix}
\text{ where }
\cP_{\theta}:=I_n-\frac1n \mathbf{1} \mathbf{1}^T
\text{ and }
I=
\begin{bmatrix}
I_H & & \\
 & I_X & \\
 & & I_Y
\end{bmatrix}.
\end{align}





Let
\begin{align*}
\hat{D}:=
\sum_{i\neq j}\frac{e^{\hat{P}_{ij}}}{(1+e^{\hat{P}_{ij}})^2}
\begin{bmatrix}
\frac{1}{\sqrt{n}}(e_i+e_j)\\
z_iz_j^T\\
\frac1ne_ie_j^T\hat{Y}\\
\frac1ne_je_i^T\hat{X}
\end{bmatrix}^{\otimes 2}.
\end{align*}
We define the debiased estimator $(\hat{\theta}^d,\hat{H}^d,\hat{X}^d,\hat{Y}^d)$ as
\begin{align}\label{def:debias}
\begin{bmatrix}
\hat{\theta}^d-\hat{\theta}\\
\hat{H}^d-\hat{H}\\
\hat{X}^d-\hat{X}\\
\hat{Y}^d-\hat{Y}
\end{bmatrix}:=-(\cP\hat{D}\cP)^{\dagger}\cP\nabla L(\hat{\theta},\hat{H},\hat{X},\hat{Y}),
\end{align}
which then satisfies:
\begin{align}\label{property:debias}
% \begin{cases}
\cP\left(\nabla L(\hat{\theta},\hat{H},\hat{X},\hat{Y})+\hat{D}
\begin{bmatrix}
\hat{\theta}^d-\hat{\theta}\\
\hat{H}^d-\hat{H}\\
\hat{X}^d-\hat{X}\\
\hat{Y}^d-\hat{Y}
\end{bmatrix}
\right)=0
\text{ and }
\cP
\begin{bmatrix}
\hat{\theta}^d\\
\hat{H}^d\\
\hat{X}^d\\
\hat{Y}^d
\end{bmatrix}=
\begin{bmatrix}
\hat{\theta}^d\\
\hat{H}^d\\
\hat{X}^d\\
\hat{Y}^d
\end{bmatrix}.
% \end{cases}.
\end{align}
Here the second condition leads to the fact that $\mathbf{1}^T \hat{\theta}^d=0$.

Similarly, let
\begin{align*}
{D}^*:=
\sum_{i\neq j}\frac{e^{{P}^*_{ij}}}{(1+e^{{P}^*_{ij}})^2}
\begin{bmatrix}
\frac{1}{\sqrt{n}}(e_i+e_j)\\
z_iz_j^T\\
\frac1ne_ie_j^T{Y}^*\\
\frac1ne_je_i^T{X}^*
\end{bmatrix}^{\otimes 2}.
\end{align*}
We define
\begin{align}\label{def:bar}
\begin{bmatrix}
\bar{\theta}-\theta^*\\
\bar{H}-H^*\\
\bar{X}-X^*\\
\bar{Y}-Y^*
\end{bmatrix}:=-(\cP D^*\cP)^{\dagger}\cP\nabla L(\theta^*,H^*,X^*,Y^*)
\end{align}
which then satisfies
\begin{align}\label{property:bar}
\cP\left(
\nabla L(\theta^*,H^*,X^*,Y^*)+D^*
\begin{bmatrix}
\bar{\theta}-\theta^*\\
\bar{H}-H^*\\
\bar{X}-X^*\\
\bar{Y}-Y^*
\end{bmatrix}
\right)=0
\text{ and }
\cP \begin{bmatrix}
\bar{\theta}\\
\bar{H}\\
\bar{X}\\
\bar{Y}
\end{bmatrix}
=
\begin{bmatrix}
\bar{\theta}\\
\bar{H}\\
\bar{X}\\
\bar{Y}
\end{bmatrix}.
\end{align}
Here the second condition leads to the fact that $\mathbf{1}^T\bar{\theta}=0$.


\begin{assumption}\label{assumption:D_eigen}
We assume
\begin{align*}
\slD\leq \lambda_{\min}(\cP D^* \cP)\leq \lambda_{\max}(\cP D^* \cP)\leq \suD
\end{align*}
for some $\slD$ and $\suD$.   
\end{assumption}


The distance between the debiased estimator and the original estimator can be captured by the following proposition.
\begin{proposition}\label{prop:debias_dist}
We have
\begin{align*}
 \left\|\begin{bmatrix}
\hat{\theta}^d-\hat{\theta}\\
\hat{H}^d-\hat{H}\\
\hat{X}^d-\hat{X}\\
\hat{Y}^d-\hat{Y}
\end{bmatrix}\right\|_F
\leq  c_a \sqrt{n},
\quad \text{where} \quad
c_a\asymp \frac{c_{\lambda}\sqrt{\mu \sX\sY r^2 \log n}}{\slD}.
\end{align*}
\end{proposition}
\begin{proof}
See Appendix \ref{pf:prop_debias_dist}.
\end{proof}







Similarly, we have the following proposition.
\begin{proposition}\label{prop:bar_dist}
We have
\begin{align*}
 \left\|\begin{bmatrix}
\bar{\theta}-{\theta^{*}}\\
\bar{H}-{H^{*}}\\
\bar{X}-{X^{*}}\\
\bar{Y}-{Y^{*}}
\end{bmatrix}\right\|_F
\leq  c'_a \sqrt{n},
\quad \text{where} \quad
c'_a\asymp \frac{\sqrt{\mu \sX\sY r^2 \log n}}{\slD}.
\end{align*}
Moreover, it holds that
\begin{align*}
 \left\|\begin{bmatrix}
\bar{\theta}-{\theta^{*}}\\
\bar{X}-{X^{*}}\\
\bar{Y}-{Y^{*}}
\end{bmatrix}\right\|_{\infty}
\leq  c_b ,
\quad \text{where} \quad
c_b\asymp  \sqrt{\frac{(1+e^{c_P})^2\log n}{\slD e^{c_P}}}.
\end{align*}
\end{proposition}
\begin{proof}
See Appendix \ref{pf:prop_bar_dist}. 
\end{proof}

\begin{assumption}\label{assumption:2_infty}
We assume
\begin{align*}
\|I-(\cP D^* \cP)^{\dagger}(\cP D^* \cP)\|_{2,\infty}\leq c_{2,\infty}\sqrt{\frac{r^2+1}{n}}
\end{align*}
for some $c_{2,\infty}$.
\end{assumption}

We can then establish the following theorem.
\begin{theorem}\label{thm:ncv_debias}
Under Assumption \ref{assumption:2_infty}, it holds that
\begin{align*}
\left\|
\begin{bmatrix}
\hat{\theta}^d-\bar{\theta}\\
\hat{H}^d-\bar{H}\\
\frac{1}{n}(\hat{X}^{d}(\hat{Y}^{d})^T-\bar{X}\bar{Y}^T)
\end{bmatrix}
\right\|_F
\lesssim c_{d} n^{1/4},
\end{align*}
where 
\begin{align*}
c_d\asymp \sqrt{\frac{(1+e^{c_P})^2}{\sl e^{c_P}}}(\su \mu\sX\sY r^2)^{1/4}(c_a+c_{11})^{3/2}.
\end{align*}
% \begin{align*}
% \left\|\hat{\theta}^d-\bar{\theta}\right\|_2=O\left(n^{1/4}\right),\ 
% \left\|\hat{H}^d-\bar{H}\right\|_F=O\left(n^{1/4}\right),\ 
% \left\|\hat{X}^{d}(\hat{Y}^{d})^T-\bar{X}\bar{Y}^T\right\|_F=O\left(n^{5/4}\right).
% \end{align*}
\end{theorem}
\begin{proof}
See Appendix \ref{pf:ncv_debias}. 
\end{proof}

% Regarding the distribution of $(\bar{\theta},\bar{H}, \bar{X}, \bar{Y})$, we have the following theorem.
% \begin{theorem}\label{thm:distribution}
% We have (\ntd).
% \end{theorem}
% \begin{proof}
% See Appendix \ref{pf:distribution}.
% \end{proof}

==> nonconvex_iterates.tex <==
\section{Properties of the nonconvex iterates}\label{sec:ncv_induction}
In this section, we study the gradient descent starting from the ground truth $(\theta^*,H^*,X^*,Y^*)$. Note that this algorithm cannot be implemented in practice because we do not have access to the ground truth parameters. More specifically, we consider the following algorithm:
\begin{algorithm}[H]
\caption{Gradient Descent}\label{GD}
\begin{algorithmic}[1]
\STATE {\bf Initialize:} $\theta^0=\theta^{*}$, $H^0=H^{*}$, $X^0=X^{*}$, and $Y^0=Y^{*}$
\FOR{$t=0,\ldots,T-1$}
\STATE Update
\begin{align}\label{alg:update_M}
&M^{t+1}:=
\begin{bmatrix}
\theta^{t+1}\\
H^{t+1}
\end{bmatrix}=
\begin{bmatrix}
\theta^{t}-\eta\left(\nabla_{\theta}f(M^t,F^t)-\mean\left(\nabla_{\theta}f(M^t,F^t)\right)\cdot\mathbf{1}\right)\\
H^{t}-\eta\nabla_{H}f(M^t,F^t)
\end{bmatrix}\\\label{alg:update_F}
&F^{t+1}:=
\begin{bmatrix}
X^{t+1}\\
Y^{t+1}
\end{bmatrix}=
\begin{bmatrix}
X^{t}-\eta\nabla_{X}f(M^t,F^t)\\
Y^{t}-\eta\nabla_{Y}f(M^t,F^t)
\end{bmatrix}
\end{align}
\ENDFOR
% \STATE {\bf Output:}
\end{algorithmic}
\end{algorithm}
Here $\eta$ is the step-size, and the update in \eqref{alg:update_M} is to guarantee that $\mathbf{1}^T\theta^{t+1}=0$ always holds on the trajectory.

\paragraph{Leave-one-out objective} For $1\leq m\leq n$, we define the following leave-one-out objective
\begin{align*}
L^{(m)}(\theta,H,X,Y)&=\sum_{\substack{
        i \neq j \\
        i, j \neq m
    }}\log(1+e^{P_{ij}})  - A_{ij}P_{ij}\\
    &+\quad \sum_{i\neq m}\left\{\log(1+e^{P_{im}})+\log(1+e^{P_{mi}})-\frac{e^{P^{*}_{im}}}{1+e^{P^{*}_{im}}}P_{im}-\frac{e^{P^{*}_{mi}}}{1+e^{P^{*}_{mi}}}P_{mi}\right\}
\end{align*}
and $f^{(m)}$, $f^{(m)}_{\aug}$, $M^{t+1,(m)}$, $F^{t+1,(m)}$ are defined correspondingly.

\paragraph{Properties}
Let
\begin{align*}
R^t&:=\argmin_{R\in\cO^{r\times r}}\|F^tR-F^*\|_F,\\
R^{t,(m)}&:=\argmin_{R\in\cO^{r\times r}}\|F^{t,(m)}R-F^*\|_F,\\
O^{t,(m)}&:=\argmin_{R\in\cO^{r\times r}}\|F^{t,(m)}R-F^tR^t\|_F.
\end{align*}
We will inductively prove the following lemmas.
\textcolor{blue}{Note that the following rates only show the dependency on $n$ (ignoring the $\log n$ dependency).
In other words, $\{c_{ij}\}$ in the lemmas are not absolute constants and may involve $r,p, \sigma_{\max},\sigma_{\min}, \log n$, etc.}






\begin{lemma}\label{lem:ncv1}
For all $0\leq t\leq t_0$, we have
\begin{align*}
\left\|
\begin{bmatrix}
\theta^t-\theta^{*}\\
H^t-H^{*}\\
F^tR^t-F^{*}
\end{bmatrix}
\right\|_F\leq c_{11}\sqrt{n},\quad 
 \|F^tR^t-F^{*}\|\leq c_{14}\sqrt{n}.
\end{align*}
\end{lemma}
% \begin{lemma}\label{lem:ncv1}
% For all $0\leq t\leq t_0$, we have
% \begin{align*}
% \|\theta^t-\theta^{*}\|_2\leq c_{11}\sqrt{n},\ \|H^t-H^{*}\|_F\leq c_{12}\sqrt{n},\ \|F^tR^t-F^{*}\|_F\leq c_{13}\sqrt{n},\ \|F^tR^t-F^{*}\|\leq c_{14}\sqrt{n}.
% \end{align*}
% \end{lemma}
\begin{proof}
See Appendix \ref{pf:lem_ncv1}.
\end{proof}








\begin{lemma}\label{lem:ncv2}
For all $0\leq t\leq t_0$, we have
\begin{align*}
\max_{1\leq m\leq n}
\left\|
\begin{bmatrix}
\theta^{t,(m)}-\theta^t\\
H^{t,(m)}-H^t\\
F^{t,(m)}O^{t,(m)}-F^tR^t
\end{bmatrix}
\right\|_F\leq c_{21}.
\end{align*}
\end{lemma}
% \begin{lemma}\label{lem:ncv2}
% For all $0\leq t\leq t_0$, we have
% \begin{align*}
% &\max_{1\leq m\leq n}\|\theta^{t,(m)}-\theta^t\|_2=O(1),\ 
% \max_{1\leq m\leq n}\|H^{t,(m)}-H^t\|_F=O(1),\\
% &\max_{1\leq m\leq n}\|F^tR^t-F^{t,(m)}O^{t,(m)}\|_F=O(1).
% \end{align*}
% \end{lemma}
\begin{proof}
See Appendix \ref{pf:lem_ncv2}.
\end{proof}







\begin{lemma}\label{lem:ncv3}
For all $0\leq t\leq t_0$, we have
\begin{align*}
\max_{1\leq m\leq n}
\left\|
\begin{bmatrix}
\theta^{t,(m)}_m-\theta^*_m\\
\left(F^{t,(m)}R^{t,(m)}-F^{*}\right)_{m,\cdot}\\
\left(F^{t,(m)}R^{t,(m)}-F^{*}\right)_{m+n,\cdot}
\end{bmatrix}
\right\|_2\leq c_{31}
\end{align*}
\end{lemma}
% \begin{lemma}\label{lem:ncv3}
% For all $0\leq t\leq t_0$, we have
% \begin{align*}
% &\max_{1\leq m\leq n}|\theta^{t,(m)}_m-\theta^*_m|=O(1),\\
% &\max_{1\leq m\leq n}\left\|\left(F^{t,(m)}R^{t,(m)}-F^{*}\right)_{m,\cdot}\right\|_2=O(1),\\
% &\max_{1\leq m\leq n}\left\|\left(F^{t,(m)}R^{t,(m)}-F^{*}\right)_{m+n,\cdot}\right\|_2=O(1).
% \end{align*}
% \end{lemma}
\begin{proof}
See Appendix \ref{pf:lem_ncv3}.
\end{proof}






\begin{lemma}\label{lem:ncv4}
For all $0\leq t\leq t_0$, we have
\begin{align*}
\|\theta^t-\theta^{*}\|_{\infty}\leq c_{41},\ \|H^t-H^{*}\|_F\leq c_{11}\sqrt{n},\ \|F^tR^t-F^{*}\|_{2,\infty}\leq c_{43},
\end{align*}
where $c_{41}=c_{21}+c_{31}$ and $c_{43}=5\kappa c_{21}+c_{31}$.
\end{lemma}
% \begin{lemma}\label{lem:ncv4}
% For all $0\leq t\leq t_0$, we have
% \begin{align*}
% \|\theta^t-\theta^{*}\|_{\infty}=O(1),\ \|H^t-H^{*}\|_F=O(\sqrt{n}),\ \|F^tR^t-F^{*}\|_{2,\infty}=O(1).
% \end{align*}
% \end{lemma}
\begin{proof}
See Appendix \ref{pf:lem_ncv4}.
\end{proof}











\begin{lemma}\label{lem:ncv5}
For all $0\leq t\leq t_0$, we have
\begin{align}
&X^tY^{tT}=Y^tX^{tT},\ X^{t,(m)}(Y^{t,(m)})^T= Y^{t,(m)}(X^{t,(m)})^T\notag\\
&\|X^{tT}X^t-Y^{tT}Y^t\|_F\leq c_{51}\eta n^2,\ \|(X^{t,(m)})^TX^{t,(m)}-(Y^{t,(m)})^TY^{t,(m)}\|_F\leq c_{51}\eta n^2\notag\\\label{ineq:gradient}
&f(M^t,F^t)\leq f(M^{t-1},F^{t-1})-\frac{\eta}{2}
\left\|
\nabla f(M^{t-1},F^{t-1})
-
\begin{bmatrix}
\mean\left(\nabla_{\theta}f(M^{t-1},F^{t-1})\right)\cdot\mathbf{1}\\
0
\end{bmatrix} 
\right\|_F^2.
\end{align}
\end{lemma}
% \begin{lemma}\label{lem:ncv5}
% For all $0\leq t\leq t_0$, we have
% \begin{align}
% &X^tY^{tT}=Y^tX^{tT},\ X^{t,(m)}(Y^{t,(m)})^T= Y^{t,(m)}(X^{t,(m)})^T\notag\\
% &\|X^{tT}X^t-Y^{tT}Y^t\|_F=O(\eta n^2),\ \|(X^{t,(m)})^TX^{t,(m)}-(Y^{t,(m)})^TY^{t,(m)}\|_F=O(\eta n^2)\notag\\
% &f(M^t,F^t)\leq f(M^{t-1},F^{t-1})-\frac{\eta}{2}\left\|\nabla_{\theta}f(M^{t-1},F^{t-1})-\mean\left(\nabla_{\theta}f(M^{t-1},F^{t-1})\right)\cdot\mathbf{1}\right\|^2_2\notag\\\label{ineq:gradient}
% &\qquad\qquad\qquad-\frac{\eta}{2}\left(\|\nabla_H f(M^{t-1},F^{t-1})\|_F^2+\|\nabla_F f(M^{t-1},F^{t-1})\|_F^2\right).
% \end{align}
% \end{lemma}
\begin{proof}
See Appendix \ref{pf:lem_ncv5}.
\end{proof}








\begin{lemma}\label{lem:ncv6}
If Lemma \ref{lem:ncv1}-Lemma \ref{lem:ncv4} hold for all $0\leq t\leq t_0$ and Lemma \ref{lem:ncv5} holds for all $1\leq t\leq t_0$, we then have
\begin{align*}
\min_{0\leq t< t_0}
\left\|
\nabla f(M^{t},F^{t})
-
\begin{bmatrix}
\mean\left(\nabla_{\theta}f(M^{t},F^{t})\right)\cdot\mathbf{1}\\
0
\end{bmatrix} 
\right\|_F
\lesssim n^{-5},
\end{align*}
% \begin{align*}
% &\min_{0\leq t< t_0}\left\|\nabla_{\theta}f(M^{t},F^{t})-\mean\left(\nabla_{\theta}f(M^{t},
% F^{t})\right)\cdot\mathbf{1}\right\|_2\lesssim n^{-5}, \\
% &\min_{0\leq t< t_0}\|\nabla_H f(M^{t},F^{t})\|_F\lesssim n^{-5}, \\
% &\min_{0\leq t< t_0}\|\nabla_F f(M^{t},F^{t})\|_F\lesssim n^{-5},
% \end{align*}
as long as $\eta t_0\geq n^{12}$.
\end{lemma}
\begin{proof}
See Appendix \ref{pf:lem_ncv6}.
\end{proof}






Here Lemma \ref{lem:ncv4} (approximation result) and Lemma \ref{lem:ncv6} (small gradient) are essential for us.

==> pf_geometry_v1.tex <==
\begin{proof}[Proof of Lemma \ref{lem:convexity}]
By the form of $\nabla^2 L(\theta,H,X,Y)$, we have
\begin{align*}
&\vec(\Delta)^T\nabla^2 L(\theta,H,X,Y)\vec(\Delta)\\
&=\sum_{i\neq j}\frac{e^{P_{ij}}}{(1+e^{P_{ij}})^2}\left(\frac{1}{\sqrt{n}}\langle\Delta_{\theta},e_i+e_j\rangle+\langle\Delta_{H},z_iz_j^T\rangle+\frac1n\langle\Delta_{X}Y^T+X\Delta_{Y}^T,e_i e_j^T\rangle\right)^2\\
&\quad +\frac2n\sum_{i\neq j}\left(\frac{e^{P_{ij}}}{1+e^{P_{ij}}}-A_{ij}\right)\langle\Delta_X,e_ie_j^T\Delta_Y\rangle.
\end{align*}
Thus, it holds that
\begin{align}\label{eq:convexity}
&\vec(\Delta)^T\nabla^2 f_{\aug}(\theta,H,X,Y)\vec(\Delta)\notag\\
&=\vec(\Delta)^T\nabla^2 L(\theta,H,X,Y)\vec(\Delta)
+\lambda\|\Delta_X\|_F^2+\lambda\|\Delta_Y\|_F^2+\frac{2c_{\aug}}{n^2}\|\Delta_X^T X+X^T\Delta_X-\Delta_Y^T Y-Y^T\Delta_Y\|_F^2\notag\\
&=\sum_{i\neq j}\frac{e^{P_{ij}}}{(1+e^{P_{ij}})^2}\left(\frac{1}{\sqrt{n}}\langle\Delta_{\theta},e_i+e_j\rangle+\langle\Delta_{H},z_iz_j^T\rangle+\frac1n\langle\Delta_{X}Y^T+X\Delta_{Y}^T,e_i e_j^T\rangle\right)^2\notag\\
&\quad+\lambda\|\Delta_X\|_F^2+\lambda\|\Delta_Y\|_F^2+\frac{2c_{\aug}}{n^2}\|\Delta_X^T X+X^T\Delta_X-\Delta_Y^T Y-Y^T\Delta_Y\|_F^2\notag\\
&\quad +\frac2n\sum_{i\neq j}\left(\frac{e^{P_{ij}}}{1+e^{P_{ij}}}-A_{ij}\right)\langle\Delta_X,e_ie_j^T\Delta_Y\rangle.   
\end{align}
We first deal with the last term, which is the only term that contains $A_{ij}$ thus has randomness. Note that
\begin{align*}
& \frac2n\sum_{i\neq j}\left(\frac{e^{P_{ij}}}{1+e^{P_{ij}}}-A_{ij}\right)\langle\Delta_X,e_ie_j^T\Delta_Y\rangle\\
& =\frac2n\sum_{i\neq j}\left(\frac{e^{P_{ij}}}{1+e^{P_{ij}}}-\frac{e^{P^{*}_{ij}}}{1+e^{P^{*}_{ij}}}\right)\langle\Delta_X,e_ie_j^T\Delta_Y\rangle+\frac2n\sum_{i\neq j}\left(\frac{e^{P^{*}_{ij}}}{1+e^{P^{*}_{ij}}}-A_{ij}\right)\langle\Delta_X,e_ie_j^T\Delta_Y\rangle.  
\end{align*}
For the first term, we have
\begin{align*}
&\left|\frac2n\sum_{i\neq j}\left(\frac{e^{P_{ij}}}{1+e^{P_{ij}}}-\frac{e^{P^{*}_{ij}}}{1+e^{P^{*}_{ij}}}\right)\langle\Delta_X,e_ie_j^T\Delta_Y\rangle\right|\\
&=\left|\frac2n\sum_{i\neq j}\left(\frac{e^{P_{ij}}}{1+e^{P_{ij}}}-\frac{e^{P^{*}_{ij}}}{1+e^{P^{*}_{ij}}}\right)(\Delta_X\Delta_Y^T)_{ij}\right|\\
&\leq \frac{1}{n}\sum_{i\neq j}|P_{ij}-P_{ij}^*||(\Delta_X\Delta_Y^T)_{ij}|\tag{\text{mean-value theorem}}\\
&\leq \frac{1}{n}\|\Delta_X\Delta_Y^T\|_F\cdot\sqrt{\sum_{i\neq j}(P_{ij}-P_{ij}^*)^2}\tag{\text{Cauchy}}.
\end{align*}
Note that
\begin{align*}
&\sum_{i\neq j}(P_{ij}-P_{ij}^*)^2\\
&=\sum_{i\neq j}\left(\frac{1}{\sqrt{n}}\langle\theta-\theta^*,e_i+e_j\rangle+\langle H-H^*,z_iz_j^T\rangle+\frac1n\langle XY^T-X^*Y^{*T},e_i e_j^T\rangle\right)^2\\
&=
\begin{bmatrix}
  \vec(\theta-\theta^*)\\
  \vec(H-H^*)\\
  \frac1n\vec(XY^T-X^*Y^{*T})
\end{bmatrix}^T
\left(\sum_{i\neq j}
  \begin{bmatrix}
  \frac{1}{\sqrt{n}}\vec(e_i+e_j)\\
  \vec(z_iz_j^T)\\
  \vec(e_ie_j^T)
  \end{bmatrix}
   \begin{bmatrix}
  \frac{1}{\sqrt{n}}\vec(e_i+e_j)\\
  \vec(z_iz_j^T)\\
  \vec(e_ie_j^T)
  \end{bmatrix}^T
\right)
\begin{bmatrix}
  \vec(\theta-\theta^*)\\
  \vec(H-H^*)\\
  \frac1n\vec(XY^T-X^*Y^{*T})
\end{bmatrix}\\
&\leq \su \left\|\begin{bmatrix}
  \vec(\theta-\theta^*)\\
  \vec(H-H^*)\\
  \frac1n\vec(XY^T-X^*Y^{*T})
\end{bmatrix}\right\|^2 \tag{By Assumption \ref{assumption:eigenvalues} and $\mathbf{1}^T(\theta-\theta^*)=0$}\\
& =\su\|\theta-\theta^{*}\|^2_{2}+\su\|H-H^{*}\|^2_{F}+\frac{\su}{n^2}\|XY^T-X^{*}Y^{*T}\|^2_{F}.
\end{align*}
Thus, we have
\begin{align*}
 &\left|\frac2n\sum_{i\neq j}\left(\frac{e^{P_{ij}}}{1+e^{P_{ij}}}-\frac{e^{P^{*}_{ij}}}{1+e^{P^{*}_{ij}}}\right)\langle\Delta_X,e_ie_j^T\Delta_Y\rangle\right|\\
 &\leq   \frac{\sqrt{\su}}{n}\|\Delta_X\Delta_Y^T\|_F\cdot\left(\|\theta-\theta^{*}\|_{2}+\|H-H^{*}\|_{F}+\frac{1}{n}\|XY^T-X^{*}Y^{*T}\|_{F}\right)\\
 &\leq   \sqrt{\frac{\su}{n}}\|\Delta_X\Delta_Y^T\|_F\cdot\left(c_1+c_2+\frac{3c_3\sqrt{\sigma_{\max}}}{n}\right)\tag{By the observations}\\
 &\leq c\frac{\sigma_{\min}}{n^{5/2}}\|\Delta_X\Delta_Y^T\|_F\tag{as long as $\sqrt{\su}\left(c_1+c_2+\frac{3c_3\sqrt{\sigma_{\max}}}{n}\right)\leq c\frac{\sigma_{\min}}{n^2}$ for some $c$}\\
 &\leq c\frac{\sigma_{\min}}{n^{5/2}}\left(\|\Delta_X\|_F^2+\|\Delta_Y\|_F^2\right)\tag{$ab\leq a^2+b^2$}
\end{align*}
For the second term, note that $(\frac{e^{P^{*}_{ij}}}{1+e^{P^{*}_{ij}}}-A_{ij})(\Delta_X\Delta_Y^T)_{ij}$ is mean-zero $|(\Delta_X\Delta_Y^T)_{ij}|^2$-subgaussian variable. By the independency, it holds that
\begin{align*}
\sum_{i\neq j}\left(\frac{e^{P^{*}_{ij}}}{1+e^{P^{*}_{ij}}}-A_{ij}\right)(\Delta_X\Delta_Y^T)_{ij}
\end{align*}
is mean-zero $\|\Delta_X\Delta_Y^T\|^2_F$-subgaussian variable. Thus, with probability at least $1-n^{-10}$, we have
\begin{align*}
  \left|\sum_{i\neq j}\left(\frac{e^{P^{*}_{ij}}}{1+e^{P^{*}_{ij}}}-A_{ij}\right)(\Delta_X\Delta_Y^T)_{ij}  \right|\lesssim \|\Delta_X\Delta_Y^T\|_F\sqrt{\log n}.
\end{align*}
As a result, with probability at least $1-n^{-10}$, we have
\begin{align*}
&\left|\frac2n\sum_{i\neq j}\left(\frac{e^{P^{*}_{ij}}}{1+e^{P^{*}_{ij}}}-A_{ij}\right)\langle\Delta_X,e_ie_j^T\Delta_Y\rangle\right|\\
&\lesssim \frac{\sqrt{\log n}}{n}\|\Delta_X\Delta_Y^T\|_F\\
 &\leq \frac{\sigma_{\min}}{n^{5/2}}\|\Delta_X\Delta_Y^T\|_F\tag{as long as $\sqrt{\frac{\log n}{n}}\ll \frac{\sigma_{\min}}{n^2}$ }\\
 &\leq \frac{\sigma_{\min}}{n^{5/2}}\left(\|\Delta_X\|_F^2+\|\Delta_Y\|_F^2\right)\tag{$ab\leq a^2+b^2$}.
\end{align*}
To summarize, we show that with probability at least $1-n^{-10}$,
\begin{align*}
    \left|\frac2n\sum_{i\neq j}\left(\frac{e^{P_{ij}}}{1+e^{P_{ij}}}-A_{ij}\right)\langle\Delta_X,e_ie_j^T\Delta_Y\rangle\right|\leq c\frac{\sigma_{\min}}{n^{5/2}}\left(\|\Delta_X\|_F^2+\|\Delta_Y\|_F^2\right).
\end{align*}


For the rest of the terms, note that
\begin{align}\label{ineq:convexity_upper}
&\sum_{i\neq j}\frac{e^{P_{ij}}}{(1+e^{P_{ij}})^2}\left(\frac{1}{\sqrt{n}}\langle\Delta_{\theta},e_i+e_j\rangle+\langle\Delta_{H},z_iz_j^T\rangle+\frac1n\langle\Delta_{X}Y^T+X\Delta_{Y}^T,e_i e_j^T\rangle\right)^2\notag\\
&\quad+\frac{2c_{\aug}}{n^2}\|\Delta_X^T X+X^T\Delta_X-\Delta_Y^T Y-Y^T\Delta_Y\|_F^2   \notag \\
&\leq \frac14
\begin{bmatrix}
  \vec(\Delta_{\theta})\\
  \vec(\Delta_{H})\\
  \frac1n\vec(\Delta_{X}Y^T+X\Delta_{Y}^T)
\end{bmatrix}^T
\left(\sum_{i\neq j}
  \begin{bmatrix}
  \frac{1}{\sqrt{n}}\vec(e_i+e_j)\\
  \vec(z_iz_j^T)\\
  \vec(e_ie_j^T)
  \end{bmatrix}
   \begin{bmatrix}
  \frac{1}{\sqrt{n}}\vec(e_i+e_j)\\
  \vec(z_iz_j^T)\\
  \vec(e_ie_j^T)
  \end{bmatrix}^T
\right)
\begin{bmatrix}
  \vec(\Delta_{\theta})\\
  \vec(\Delta_{H})\\
  \frac1n\vec(\Delta_{X}Y^T+X\Delta_{Y}^T)
\end{bmatrix}\notag\\
&\quad+\frac{2c_{\aug}}{n^2}\|\Delta_X^T X+X^T\Delta_X-\Delta_Y^T Y-Y^T\Delta_Y\|_F^2    \notag\\
&\leq \su\|\Delta_{\theta}\|^2_F+\su\|\Delta_{H}\|^2_F+\frac{\su}{n^2} \|\Delta_{X}Y^T+X\Delta_{Y}^T\|^2_F+\frac{2c_{\aug}}{n^2}\|\Delta_X^T X+X^T\Delta_X-\Delta_Y^T Y-Y^T\Delta_Y\|_F^2\notag\\
&\leq \su\|\Delta_{\theta}\|^2_F+\su\|\Delta_{H}\|^2_F+\frac{\su}{n^2} \|\Delta_{X}Y^T+X\Delta_{Y}^T\|^2_F+\frac{\su}{4n^2}\|\Delta_X^T X+X^T\Delta_X-\Delta_Y^T Y-Y^T\Delta_Y\|_F^2 ,
\end{align}
where the second inequality follows from Assumption \ref{assumption:eigenvalues} and the condition that $\mathbf{1}^T\Delta_{\theta}=0$, and the third inequality follows from the fact that $8c_{\aug}\leq \su$.
Moreover, we have
\begin{align*}
&\sum_{i\neq j}\frac{e^{P_{ij}}}{(1+e^{P_{ij}})^2}\left(\frac{1}{\sqrt{n}}\langle\Delta_{\theta},e_i+e_j\rangle+\langle\Delta_{H},z_iz_j^T\rangle+\frac1n\langle\Delta_{X}Y^T+X\Delta_{Y}^T,e_i e_j^T\rangle\right)^2\\
&\quad+\frac{2c_{\aug}}{n^2}\|\Delta_X^T X+X^T\Delta_X-\Delta_Y^T Y-Y^T\Delta_Y\|_F^2    \\
&\geq \frac{e^{2c_P}}{(1+e^{2c_P})^2}
\begin{bmatrix}
  \vec(\Delta_{\theta})\\
  \vec(\Delta_{H})\\
  \frac1n\vec(\Delta_{X}Y^T+X\Delta_{Y}^T)
\end{bmatrix}^T
\left(\sum_{i\neq j}
  \begin{bmatrix}
  \frac{1}{\sqrt{n}}\vec(e_i+e_j)\\
  \vec(z_iz_j^T)\\
  \vec(e_ie_j^T)
  \end{bmatrix}
   \begin{bmatrix}
  \frac{1}{\sqrt{n}}\vec(e_i+e_j)\\
  \vec(z_iz_j^T)\\
  \vec(e_ie_j^T)
  \end{bmatrix}^T
\right)
\begin{bmatrix}
  \vec(\Delta_{\theta})\\
  \vec(\Delta_{H})\\
  \frac1n\vec(\Delta_{X}Y^T+X\Delta_{Y}^T)
\end{bmatrix}\\
&\quad+\frac{2c_{\aug}}{n^2}\|\Delta_X^T X+X^T\Delta_X-\Delta_Y^T Y-Y^T\Delta_Y\|_F^2  
\end{align*}
since by observations, we know $|P_{ij}|\leq 2c_P$. Then, similarly, by Assumption \ref{assumption:eigenvalues} and the condition that $\mathbf{1}^T\Delta_{\theta}=0$, we have
\begin{align}\label{ineq:convexity_lower}
&\sum_{i\neq j}\frac{e^{P_{ij}}}{(1+e^{P_{ij}})^2}\left(\frac{1}{\sqrt{n}}\langle\Delta_{\theta},e_i+e_j\rangle+\langle\Delta_{H},z_iz_j^T\rangle+\frac1n\langle\Delta_{X}Y^T+X\Delta_{Y}^T,e_i e_j^T\rangle\right)^2\notag\\
&\quad+\frac{2c_{\aug}}{n^2}\|\Delta_X^T X+X^T\Delta_X-\Delta_Y^T Y-Y^T\Delta_Y\|_F^2   \notag \\
&\geq \sl\frac{e^{2c_P}}{(1+e^{2c_P})^2}\left(\|\Delta_{\theta}\|^2_F+\|\Delta_{H}\|^2_F+\frac{1}{n^2} \|\Delta_{X}Y^T+X\Delta_{Y}^T\|^2_F\right)+\frac{2c_{\aug}}{n^2}\|\Delta_X^T X+X^T\Delta_X-\Delta_Y^T Y-Y^T\Delta_Y\|_F^2\notag\\
&= \sl\frac{e^{2c_P}}{(1+e^{2c_P})^2}\left(\|\Delta_{\theta}\|^2_F+\|\Delta_{H}\|^2_F+\frac{1}{n^2} \|\Delta_{X}Y^T+X\Delta_{Y}^T\|^2_F\right)\notag\\
&\quad +\frac{\sl e^{2c_P}}{4(1+e^{2c_P})^2n^2}\|\Delta_X^T X+X^T\Delta_X-\Delta_Y^T Y-Y^T\Delta_Y\|_F^2
\end{align}
By \eqref{eq:convexity}, \eqref{ineq:convexity_upper} and \eqref{ineq:convexity_lower}, to obtain the local geometry results, we only need to bound:
\begin{align}\label{term1:lem_convexity}
\|\Delta_{X}Y^T+X\Delta_{Y}^T\|^2_F+\frac{1}{4}\|\Delta_X^T X+X^T\Delta_X-\Delta_Y^T Y-Y^T\Delta_Y\|_F^2 .  
\end{align}
For the upper bound of \eqref{term1:lem_convexity}, note that 
\begin{align*}
&\|\Delta_{X}Y^T+X\Delta_{Y}^T\|^2_F\leq \left(\|Y\|\|\Delta_X\|_F+\|X\|\|\Delta_Y\|_F\right)^2   \leq \left(\|X\|^2+\|Y\|^2\right)\left(\|\Delta_X\|_F^2+\|\Delta_Y\|_F^2\right),\\
 &\|\Delta_X^T X+X^T\Delta_X-\Delta_Y^T Y-Y^T\Delta_Y\|_F^2\leq 4\left(\|X\|^2+\|Y\|^2\right)\left(\|\Delta_X\|_F^2+\|\Delta_Y\|_F^2\right).
\end{align*}
Thus, it holds that
\begin{align*}
&\|\Delta_{X}Y^T+X\Delta_{Y}^T\|^2_F+\frac{1}{4}\|\Delta_X^T X+X^T\Delta_X-\Delta_Y^T Y-Y^T\Delta_Y\|_F^2\\
&\leq
2\left(\|X\|^2+\|Y\|^2\right)\left(\|\Delta_X\|_F^2+\|\Delta_Y\|_F^2\right).
\end{align*}
By Weyl's inequality, we have
\begin{align*}
|\sigma_{\max}(X)-\sigma_{\max}(X^{*})|\leq \|XR-X^{*}\|\leq c_3 \sqrt{n},\  |\sigma_{\max}(Y)-\sigma_{\max}(Y^{*})|\leq \|YR-Y^{*}\|\leq c_3 \sqrt{n}.
\end{align*}
As long as $c_3\sqrt{n}\ll \sqrt{\sigma_{\max}}$, we have 
\begin{align*}
\sigma_{\max}(X)\leq 2\sqrt{\sigma_{\max}},\ 
\sigma_{\max}(Y)\leq 2\sqrt{\sigma_{\max}},
\end{align*}
which implies
\begin{align*}
\|\Delta_{X}Y^T+X\Delta_{Y}^T\|^2_F+\frac{1}{4}\|\Delta_X^T X+X^T\Delta_X-\Delta_Y^T Y-Y^T\Delta_Y\|_F^2  \leq 16 \sigma_{\max} \left(\|\Delta_X\|_F^2+\|\Delta_Y\|_F^2\right).
\end{align*}

For the lower bound of \eqref{term1:lem_convexity}, note that 
\begin{align*}
&\left\| \Delta_X Y^{T} + X \Delta_Y^{T} \right\|_F^2 + \frac{1}{4} \left\| \Delta_X^{T} X + X^{T} \Delta_X -\Delta_Y^T Y-Y^T\Delta_Y\right\|_F^2 \\
&= \left\| \Delta_X Y^{T} \right\|_F^2 + \left\| X \Delta_Y^{T} \right\|_F^2 + \frac12\left\| \Delta_X^{T} X \right\|_F^2 + \frac{1}{2} \left\| \Delta_Y^{T} Y \right\|_F^2 - \left\langle \Delta_X^{T} X, \Delta_Y^{T} Y \right\rangle  \\
&\quad+\frac{1}{2} \left\langle X^{T} \Delta_X, \Delta_X^{T} X \right\rangle+ \frac{1}{2} \left\langle Y^{T} \Delta_Y, \Delta_Y^{T} Y \right\rangle+ \left\langle \Delta_X^T X, Y^{T} \Delta_Y \right\rangle \\
&= \left\| \Delta_X Y^{T} \right\|_F^2 + \left\| X \Delta_Y^{T} \right\|_F^2 + \frac12\left\| \Delta_X^{T} X - \Delta_Y^{T} Y \right\|_F^2 + \frac{1}{2} \left\langle X^{T} \Delta_X + Y^T\Delta_Y, \Delta_X^{T} X + \Delta_Y^{T} Y \right\rangle \\
&= \left\| \Delta_X Y^{T} \right\|_F^2 + \left\| X \Delta_Y^{T} \right\|_F^2 + \frac12\left\| \Delta_X^{T} X - \Delta_Y^{T} Y \right\|_F^2 \\
&\quad+ \frac{1}{2} \left\langle (XR)^{T} (\Delta_X R)+(YR)^T(\Delta_Y R), (\Delta_X R)^{T} (XR) + (\Delta_YR)^{T} (YR) \right\rangle \\
&= \left\| \Delta_X Y^{T} \right\|_F^2 + \left\| X \Delta_Y^{T} \right\|_F^2 + \frac12\left\| \Delta_X^{T} X - \Delta_Y^{T} Y \right\|_F^2 \\
&\quad+ \frac{1}{2} \left\langle X_2^{T} (\Delta_X R)+Y_2^T(\Delta_Y R), (\Delta_X R)^TX_2 + (\Delta_Y R)^T Y_2 \right\rangle + \mathcal{E}_1 \\
&=  \left\| \Delta_X Y^{T} \right\|_F^2 + \left\| X \Delta_Y^{T} \right\|_F^2 + \frac12\left\| \Delta_X^{T} X - \Delta_Y^{T} Y \right\|_F^2  + \frac12\left\| X_2^{T} \Delta_X +Y_2^T\Delta_Y  \right\|_F^2 + \mathcal{E}_1,
\end{align*}
where 
\begin{align*}
% \mathcal{E}_1 &:= \frac{1}{2} \left\langle (X - X_2)^{T} \Delta_X + (Y - Y_2)^{T} \Delta_Y, \Delta_X^{T} X_2 + \Delta_Y^{T} Y_2 \right\rangle \\
% & \quad+ \frac{1}{2} \left\langle X_2^{T} \Delta_X + Y_2^{T} \Delta_Y, \Delta_X^{T} (X - X_2) + \Delta_Y^{T} (Y - Y_2) \right\rangle \\
% & \quad+ \frac{1}{2} \left\langle (X - X_2)^{T} \Delta_X + (Y - Y_2)^{T} \Delta_Y, \Delta_X^{T} (X - X_2) + \Delta_Y^{T} (Y - Y_2) \right\rangle\\
\mathcal{E}_1 &:=  \left\langle (XR - X_2)^{T} \Delta_X R + (YR - Y_2)^{T} \Delta_Y R, (\Delta_X R)^{T} X_2 + (\Delta_Y R)^{T} Y_2 \right\rangle \\
& \quad+ \frac{1}{2} \left\langle (X R- X_2)^{T} \Delta_X R + (YR - Y_2)^{T} \Delta_Y R, (\Delta_X R)^{T} (XR - X_2) + (\Delta_Y R)^{T} (YR - Y_2) \right\rangle.
\end{align*}
Based on the fact that $|\langle A,B\rangle|\leq\|A\|_F\|B\|_F$ and $\|AB\|_F\leq \|A\|\|B\|_F$, we have
\begin{align*}
|\mathcal{E}_1|\leq 
\left((\|XR-X_2\|+\|YR-Y_2\|)(\|X_2\|+\|Y_2\|)+\frac12 (\|XR-X_2\|+\|YR-Y_2\|)^2\right)\left(\|\Delta_X\|^2_F+\|\Delta_Y\|^2_F\right).
\end{align*}
By the definition of $X_2,Y_2$, as long as $c_4\sqrt{n}\ll \sqrt{\sigma_{\max}}$, we have 
\begin{align*}
\|X_2\|\leq \|X_2-X^*\|+\|X^*\|\leq 2 \sqrt{\sigma_{\max}},\ \|Y_2\|\leq \|Y_2-X^*\|+\|Y^*\|\leq 2 \sqrt{\sigma_{\max}}.
\end{align*}
Moreover, by the observations, we have
\begin{align*}
&\|XR-X_2\|\leq \|XR-X^*\|+\|X_2-X^*\|\leq (c_3+c_4)\sqrt{n},\notag\\
&\|YR-Y_2\|\leq \|YR-Y^*\|+\|Y_2-Y^*\|\leq (c_3+c_4) \sqrt{n}.
\end{align*}
Thus, we have
\begin{align*}
 |\mathcal{E}_1|\leq 10(c_3+c_4) \sqrt{n\sigma_{\max}}  \left(\|\Delta_X\|^2_F+\|\Delta_Y\|^2_F\right).
\end{align*}
As a result, we have
\begin{align*}
 &\left\| \Delta_X Y^{T} + X \Delta_Y^{T} \right\|_F^2 + \frac{1}{4} \left\| \Delta_X^{T} X + X^{T} \Delta_X -\Delta_Y^T Y-Y^T\Delta_Y\right\|_F^2 \\
 &\geq  \left\| \Delta_X Y^{T} \right\|_F^2 + \left\| X \Delta_Y^{T} \right\|_F^2  - |\mathcal{E}_1|\\
 &\geq \frac{\sigma_{\min}}{4}\left(\left\| \Delta_X \right\|_F^2 + \left\|  \Delta_Y \right\|_F^2 \right)- |\mathcal{E}_1|\\
 &\geq \left(\frac{\sigma_{\min}}{4}-10(c_3+c_4) \sqrt{n\sigma_{\max}}  \right)\left(\left\| \Delta_X \right\|_F^2 + \left\|  \Delta_Y \right\|_F^2 \right).
\end{align*}
% and 
% \begin{align*}
%  &\left\| \Delta_X Y^{T} + X \Delta_Y^{T} \right\|_F^2 + \frac{1}{4} \left\| \Delta_X^{T} X + X^{T} \Delta_X -\Delta_Y^T Y-Y^T\Delta_Y\right\|_F^2 \\
%  &\lesssim \left(\|X\|^2+\|Y\|^2+\|X_2\|^2+\|Y_2\|^2\right) \left(\left\| \Delta_X \right\|_F^2 + \left\|  \Delta_Y \right\|_F^2 \right)  +|\mathcal{E}_1|\\
%  &\lesssim\sigma_{\max}\left(\left\| \Delta_X \right\|_F^2 + \left\|  \Delta_Y \right\|_F^2 \right)+ |\mathcal{E}_1|\\
%  &\lesssim (\sigma_{\max}+\lambda n^2)\left(\left\| \Delta_X \right\|_F^2 + \left\|  \Delta_Y \right\|_F^2 \right).
% \end{align*}
Here we use Weyl's inequality to obtain that
\begin{align*}
|\sigma_{\min}(X)-\sigma_{\min}(X^{*})|\leq \|XR-X^{*}\|\leq c_3 \sqrt{n},\  |\sigma_{\min}(Y)-\sigma_{\min}(Y^{*})|\leq \|YR-Y^{*}\|\leq c_3 \sqrt{n}.
\end{align*}
As long as $c_3\sqrt{n}\ll \sqrt{\sigma_{\min}}$, we have
\begin{align*}
  \sigma_{\min}(X)\geq \frac12\sqrt{\sigma_{\min}}, \ \sigma_{\min}(Y)\geq\frac12\sqrt{\sigma_{\min}}.
\end{align*}

Combine the upper and lower bound for \eqref{term1:lem_convexity} with \eqref{ineq:convexity_upper} and \eqref{ineq:convexity_lower}, we obtain that
\begin{align*}
&\sum_{i\neq j}\frac{e^{P_{ij}}}{(1+e^{P_{ij}})^2}\left(\frac{1}{\sqrt{n}}\langle\Delta_{\theta},e_i+e_j\rangle+\langle\Delta_{H},z_iz_j^T\rangle+\frac1n\langle\Delta_{X}Y^T+X\Delta_{Y}^T,e_i e_j^T\rangle\right)^2\notag\\
&\quad+\frac{2c_{\aug}}{n^2}\|\Delta_X^T X+X^T\Delta_X-\Delta_Y^T Y-Y^T\Delta_Y\|_F^2   \notag \\
&\leq\su\|\Delta_{\theta}\|^2_F+\su\|\Delta_{H}\|^2_F+ \frac{16\su\sigma_{\max}}{n^2}\left(\left\| \Delta_X \right\|_F^2 + \left\|  \Delta_Y \right\|_F^2 \right),
\end{align*}
and 
\begin{align*}
&\sum_{i\neq j}\frac{e^{P_{ij}}}{(1+e^{P_{ij}})^2}\left(\frac{1}{\sqrt{n}}\langle\Delta_{\theta},e_i+e_j\rangle+\langle\Delta_{H},z_iz_j^T\rangle+\frac1n\langle\Delta_{X}Y^T+X\Delta_{Y}^T,e_i e_j^T\rangle\right)^2\notag\\
&\quad+\frac{2c_{\aug}}{n^2}\|\Delta_X^T X+X^T\Delta_X-\Delta_Y^T Y-Y^T\Delta_Y\|_F^2   \notag \\
&\geq \sl\frac{e^{2c_P}}{(1+e^{2c_P})^2}\left(\|\Delta_{\theta}\|^2_F+\|\Delta_{H}\|^2_F+ \frac{1}{n^2}\left(\frac{\sigma_{\min}}{4}-10(c_3+c_4) \sqrt{n\sigma_{\max}}  \right)\left(\left\| \Delta_X \right\|_F^2 + \left\|  \Delta_Y \right\|_F^2 \right)\right).
\end{align*}

Combine the above results with \eqref{eq:convexity}, we final obtain that with probability at least $1-n^{-10}$, we have
\begin{align*}
 &\vec(\Delta)^T\nabla^2 f_{\aug}(\theta,H,X,Y)\vec(\Delta)\notag\\  
 &\leq \su\|\Delta_{\theta}\|^2_F+\su\|\Delta_{H}\|^2_F+ \left(\frac{16\su\sigma_{\max}}{n^2}+\lambda +c\frac{\sigma_{\min}}{n^{5/2}}\right)\left(\left\| \Delta_X \right\|_F^2 + \left\|  \Delta_Y \right\|_F^2 \right)\\
 &\leq \su|\Delta_{\theta}\|^2_F+\su\|\Delta_{H}\|^2_F+\frac{20\su\sigma_{\max}}{n^2}\left(\left\| \Delta_X \right\|_F^2 + \left\|  \Delta_Y \right\|_F^2 \right)
\end{align*}
as long as $\lambda, c\frac{\sigma_{\min}}{n^{5/2}}\ll \frac{\su\sigma_{\max}}{n^2}$,
and 
\begin{align*}
 &\vec(\Delta)^T\nabla^2 f_{\aug}(\theta,H,X,Y)\vec(\Delta)\notag\\  
 &\geq \sl\frac{e^{2c_P}}{(1+e^{2c_P})^2}\left(\|\Delta_{\theta}\|^2_F+\|\Delta_{H}\|^2_F\right)\notag\\
 &\quad+ \left(\sl\frac{e^{2c_P}}{(1+e^{2c_P})^2}\frac{1}{n^2}\left(\frac{\sigma_{\min}}{4}-10(c_3+c_4) \sqrt{n\sigma_{\max}}  \right)+\lambda -c\frac{\sigma_{\min}}{n^{5/2}}\right)\left(\left\| \Delta_X \right\|_F^2 + \left\|  \Delta_Y \right\|_F^2 \right)\\
 &\geq  \sl\frac{e^{2c_P}}{(1+e^{2c_P})^2}\left(  \|\Delta_{\theta}\|^2_F+\|\Delta_{H}\|^2_F+ \frac{\sigma_{\min}}{8n^2}\left(\left\| \Delta_X \right\|_F^2 + \left\|  \Delta_Y \right\|_F^2 \right)\right)
\end{align*}
as long as $\sigma_{\min}\gg 40(c_3+c_4)\sqrt{n\sigma_{\max}}$, $n\gg c^2$.
This further implies that 
\begin{align*}
\left\|\nabla^2f_{\aug}(\theta,H,X,Y)\right\|\leq \max\left\{\su,\frac{20\su\sigma_{\max}}{n^2}\right\}.
\end{align*}
We then finish the proofs.
\end{proof}


==> pf_main_result_v1.tex <==
\section{Proofs of Section \ref{sec:results}}\label{sec:pf_results}






\subsection{Proofs of Proposition \ref{prop:assumption_example}}\label{pf:prop_assumption_example}
In this example, we have
\begin{align*}
\Gamma^*=
\begin{bmatrix}
p\mathbf{1}\mathbf{1}^T & q\mathbf{1}\mathbf{1}^T\\
q\mathbf{1}\mathbf{1}^T & p\mathbf{1}\mathbf{1}^T\\
\end{bmatrix}
=\Pi
\begin{bmatrix}
p & q\\
q & p\\
\end{bmatrix}
\Pi^{T}
=\Pi
\begin{bmatrix}
1 & 1\\
1 & -1\\
\end{bmatrix}
\begin{bmatrix}
\frac{p+q}{2} & 0\\
0 & \frac{p-q}{2}\\
\end{bmatrix}
\begin{bmatrix}
1 & 1\\
1 & -1\\
\end{bmatrix}
\Pi^{T},
\end{align*}
where $\Pi\in\bbR^{n\times 2}$ with the first $n/2$ rows being $[1,0]$ and the last $n/2$ rows being $[0,1]$. It then holds that
\begin{align}\label{eq3:pf_example}
X^{*}=Y^{*}
=\Pi
\begin{bmatrix}
1 & 1\\
1 & -1\\
\end{bmatrix}
\begin{bmatrix}
\sqrt{\frac{p+q}{2}} & 0\\
0 & \sqrt{\frac{p-q}{2}}\\
\end{bmatrix}
=\begin{bmatrix}
\sqrt{\frac{p+q}{2}}\mathbf{1} & \sqrt{\frac{p-q}{2}} \mathbf{1}\\
\sqrt{\frac{p+q}{2}}\mathbf{1} & -\sqrt{\frac{p-q}{2}} \mathbf{1}
\end{bmatrix},
\end{align}
where $\mathbf{1}\in\bbR^{\frac{n}{2}\times 1}$.
We denote
\begin{align*}
&\cA_1:=\{(i,j)\mid 1\leq i,j\leq n/2, i\neq j\},\\
&\cA_2:=\{(i,j)\mid 1\leq i\leq n/2,n/2< j\leq n, i\neq j\},\\
&\cA_3:=\{(i,j)\mid n/2< i\leq n,1\leq j\leq n/2,i\neq j\},\\
&\cA_4:=\{(i,j)\mid n/2< i,j\leq n, i\neq j\}.
\end{align*}
Since $\theta^*=0, H^*=0$, we then have
\begin{align*}
D^{*}
&=
\sum_{(i,j)\in\cA_1}\frac{e^{\frac{p}{n}}}{(1+e^{\frac{p}{n}})^2}
\begin{bmatrix}
\frac1n e_i \left[\sqrt{\frac{p+q}{2}}, \sqrt{\frac{p-q}{2}}\right]\\[10pt]
\frac1n e_j \left[\sqrt{\frac{p+q}{2}}, \sqrt{\frac{p-q}{2}}\right]
\end{bmatrix}^{\otimes 2}
+\sum_{(i,j)\in\cA_2}\frac{e^{\frac{q}{n}}}{(1+e^{\frac{q}{n}})^2}
\begin{bmatrix}
\frac1n e_i \left[\sqrt{\frac{p+q}{2}}, -\sqrt{\frac{p-q}{2}}\right]\\[10pt]
\frac1n e_j \left[\sqrt{\frac{p+q}{2}}, \sqrt{\frac{p-q}{2}}\right]
\end{bmatrix}^{\otimes 2}\\
&\quad +\sum_{(i,j)\in\cA_3}\frac{e^{\frac{q}{n}}}{(1+e^{\frac{q}{n}})^2}
\begin{bmatrix}
\frac1n e_i \left[\sqrt{\frac{p+q}{2}}, \sqrt{\frac{p-q}{2}}\right]\\[10pt]
\frac1n e_j \left[\sqrt{\frac{p+q}{2}}, -\sqrt{\frac{p-q}{2}}\right]
\end{bmatrix}^{\otimes 2}
+\sum_{(i,j)\in\cA_4}\frac{e^{\frac{p}{n}}}{(1+e^{\frac{p}{n}})^2}
\begin{bmatrix}
\frac1n e_i \left[\sqrt{\frac{p+q}{2}}, -\sqrt{\frac{p-q}{2}}\right]\\[10pt]
\frac1n e_j \left[\sqrt{\frac{p+q}{2}}, -\sqrt{\frac{p-q}{2}}\right]
\end{bmatrix}^{\otimes 2}.
\end{align*}
In what follows, we view $D^*$ as a $4n\times 4n$ matrix and denote
\begin{align*}
D^*=
\begin{bmatrix}
D_{11}^* & D_{12}^* & D_{13}^* & D_{14}^*\\
D_{21}^* & D_{22}^* & D_{23}^* & D_{24}^*\\
D_{31}^* & D_{32}^* & D_{33}^* & D_{34}^*\\
D_{41}^* & D_{42}^* & D_{43}^* & D_{44}^*
\end{bmatrix},
\end{align*}
where $D_{ij}^*\in\bbR^{n\times n}$.
Recall that we have
\begin{align*}
D^*
\begin{bmatrix}
\Delta_X\\
\Delta_Y
\end{bmatrix}
=
\begin{bmatrix}
X^*\\
Y^*
\end{bmatrix},
\end{align*}
where we view $\Delta_X,\Delta_Y,X^*,Y^*$ as $2n\times 1$ vectors. Thus, we have
\begin{align}\label{eq1:pf_example}
\begin{bmatrix}
D_{11}^* & D_{12}^* \\
D_{21}^* & D_{22}^*    
\end{bmatrix}\Delta_X
+\begin{bmatrix}
D_{13}^* & D_{14}^*\\
D_{23}^* & D_{24}^*\\  
\end{bmatrix}\Delta_Y
=X^*.
\end{align}
Based on the specific form of $X^*$ and $Y^*$, it can be seen that the solutions must have the following form:\textcolor{red}{Why???}
\begin{align}\label{eq2:pf_example}
\Delta_X=\Delta_Y
=\vec 
\begin{bmatrix}
a & b\\
\vdots & \vdots\\
a & b\\
c & d\\
\vdots & \vdots\\
c & d\\
\end{bmatrix}.
\end{align}
The matrix on the RHS has its first $n$ rows being $[a,b]$ and last $n$ rows being $[c,d]$ for some $a,b,c,d$.
By \eqref{eq1:pf_example}, we have
\begin{align}\label{eq4:pf_example}
\begin{bmatrix}
D_{11}^* + D_{13}^* & D_{12}^* + D_{14}^* \\
D_{21}^* + D_{23}^* & D_{22}^* + D_{24}^*  
\end{bmatrix}\Delta_X
=X^*.
\end{align}
With a little abuse of notion, we denote $e_i,e_j\in\bbR^{\frac{n}{2}\times 1}$ the one-hot vector in the following. And we denote $s=\sqrt{\frac{p+q}{2}}, t=\sqrt{\frac{p-q}{2}}$. It then holds that
\begin{align}\label{eq5:pf_example}
&D_{11}^* + D_{13}^*
=\frac{1}{n^2}\sum_{\substack{
        i \neq j \\
        1\leq i, j \leq \frac{n}{2}
    }}\frac{e^{\frac{p}{n}}}{(1+e^{\frac{p}{n}})^2}
\begin{bmatrix}
e_i [s, t]
\end{bmatrix}^{\otimes 2}
+\frac{1}{n^2}\sum_{\substack{
        i \neq j \\
        1\leq i, j \leq \frac{n}{2}
    }}\frac{e^{\frac{p}{n}}}{(1+e^{\frac{p}{n}})^2}
\begin{bmatrix}
e_i [s, t]
\end{bmatrix}^{\otimes}
\begin{bmatrix}
e_j [s, t]
\end{bmatrix}\notag\\
&\qquad\qquad\qquad +
\frac{1}{n^2}\sum_{
        1\leq i, j \leq \frac{n}{2}}\frac{e^{\frac{q}{n}}}{(1+e^{\frac{q}{n}})^2}
\begin{bmatrix}
e_i [s, -t]
\end{bmatrix}^{\otimes 2}\notag\\
&D_{12}^* + D_{14}^*
=
\frac{1}{n^2}\sum_{
        1\leq i, j \leq \frac{n}{2}}\frac{e^{\frac{q}{n}}}{(1+e^{\frac{q}{n}})^2}
\begin{bmatrix}
e_i [s, -t]
\end{bmatrix}^{\otimes}
\begin{bmatrix}
e_j [s, t]
\end{bmatrix}\notag\\
&D_{21}^* + D_{23}^*
=
\frac{1}{n^2}\sum_{
        1\leq i, j \leq \frac{n}{2}}\frac{e^{\frac{q}{n}}}{(1+e^{\frac{q}{n}})^2}
\begin{bmatrix}
e_i [s, t]
\end{bmatrix}^{\otimes}
\begin{bmatrix}
e_j [s, -t]
\end{bmatrix}\notag\\
&D_{22}^* + D_{24}^*
=\frac{1}{n^2}\sum_{\substack{
        i \neq j \\
        1\leq i, j \leq \frac{n}{2}
    }}\frac{e^{\frac{p}{n}}}{(1+e^{\frac{p}{n}})^2}
\begin{bmatrix}
e_i [s, -t]
\end{bmatrix}^{\otimes 2}
+\frac{1}{n^2}\sum_{\substack{
        i \neq j \\
        1\leq i, j \leq \frac{n}{2}
    }}\frac{e^{\frac{p}{n}}}{(1+e^{\frac{p}{n}})^2}
\begin{bmatrix}
e_i [s, -t]
\end{bmatrix}^{\otimes}
\begin{bmatrix}
e_j [s, -t]
\end{bmatrix}\notag\\
&\qquad\qquad\qquad +
\frac{1}{n^2}\sum_{
        1\leq i, j \leq \frac{n}{2}}\frac{e^{\frac{q}{n}}}{(1+e^{\frac{q}{n}})^2}
\begin{bmatrix}
e_i [s, t]
\end{bmatrix}^{\otimes 2}.
\end{align}
Combine \eqref{eq3:pf_example}, \eqref{eq2:pf_example}, \eqref{eq4:pf_example}, \eqref{eq5:pf_example}, we have
\begin{align*}
&\mathbf{1}_{\frac{n}{2}}\cdot[s,t]
=(n-2)\frac{as+bt}{n^2}\frac{e^{\frac{p}{n}}}{(1+e^{\frac{p}{n}})^2}\cdot (\mathbf{1}_{\frac{n}{2}}\cdot[s,t])
+\frac{n}{2}\frac{as-bt}{n^2}\frac{e^{\frac{q}{n}}}{(1+e^{\frac{q}{n}})^2}\cdot (\mathbf{1}_{\frac{n}{2}}\cdot[s,-t])\\
&\qquad\qquad\qquad +\frac{n}{2}\frac{cs+dt}{n^2}\frac{e^{\frac{q}{n}}}{(1+e^{\frac{q}{n}})^2}\cdot (\mathbf{1}_{\frac{n}{2}}\cdot[s,-t])\\
&\mathbf{1}_{\frac{n}{2}}\cdot[s,-t]
=(n-2)\frac{cs-dt}{n^2}\frac{e^{\frac{p}{n}}}{(1+e^{\frac{p}{n}})^2}\cdot (\mathbf{1}_{\frac{n}{2}}\cdot[s,-t])
+\frac{n}{2}\frac{cs+dt}{n^2}\frac{e^{\frac{q}{n}}}{(1+e^{\frac{q}{n}})^2}\cdot (\mathbf{1}_{\frac{n}{2}}\cdot[s,t])\\
&\qquad\qquad\qquad +\frac{n}{2}\frac{as-bt}{n^2}\frac{e^{\frac{q}{n}}}{(1+e^{\frac{q}{n}})^2}\cdot (\mathbf{1}_{\frac{n}{2}}\cdot[s,t]),
\end{align*}
which implies
\begin{align*}
\begin{cases}
as-bt=-(cs+dt)\\
(n-2)\frac{as+bt}{n^2}\frac{e^{\frac{p}{n}}}{(1+e^{\frac{p}{n}})^2}=1\\
(n-2)\frac{cs-dt}{n^2}\frac{e^{\frac{p}{n}}}{(1+e^{\frac{p}{n}})^2}=1
\end{cases}.
\end{align*}
We denote
\begin{align*}
N:=\frac{n^2}{n-2}\frac{(1+e^{\frac{p}{n}})^2}{e^{\frac{p}{n}}}.
\end{align*}
It then holds that
\begin{align*}
a=c=\frac{N}{2s}, \quad b=-d=\frac{N}{2t}
\end{align*}
and 
\begin{align}\label{eq6:pf_example}
\Delta_X
=\begin{bmatrix}
\frac{N}{2s}\mathbf{1} & \frac{N}{2t}\mathbf{1}\\[10pt]
\frac{N}{2s}\mathbf{1} & -\frac{N}{2t}\mathbf{1}
\end{bmatrix}.
\end{align}
Combine with \eqref{eq3:pf_example}, we have
\begin{align*}
\Delta_X Y^{*\top}+X^{*}\Delta^{\top}_Y=\Delta_X X^{*\top}+X^{*}\Delta^{\top}_X
=\begin{bmatrix}
2N\mathbf{1}\mathbf{1}^{\top} & 0\\
0 & 2N\mathbf{1}\mathbf{1}^{\top}
\end{bmatrix}\in\bbR^{n\times n}.
\end{align*}
By the definition of $M^*$, we have
\begin{align*}
M^*=
\begin{bmatrix}
\frac{e^{\frac{p}{n}}}{(1+e^{\frac{p}{n}})^2}\mathbf{1}\mathbf{1}^{\top} & \frac{e^{\frac{q}{n}}}{(1+e^{\frac{q}{n}})^2}\mathbf{1}\mathbf{1}^{\top}\\
\frac{e^{\frac{q}{n}}}{(1+e^{\frac{q}{n}})^2}\mathbf{1}\mathbf{1}^{\top} & \frac{e^{\frac{p}{n}}}{(1+e^{\frac{p}{n}})^2}\mathbf{1}\mathbf{1}^{\top}
\end{bmatrix}
-
\begin{bmatrix}
\frac{e^{\frac{p}{n}}}{(1+e^{\frac{p}{n}})^2} & & \\
 & \ddots & \\
 & & \frac{e^{\frac{p}{n}}}{(1+e^{\frac{p}{n}})^2}
\end{bmatrix}.
\end{align*}
Thus, we have
\begin{align*}
\frac1n M^*\odot \left(\frac1n(\Delta_X Y^{*\top}+X^{*}\Delta^{\top}_Y) \right)
&=\begin{bmatrix}
\frac{2}{n-2}\mathbf{1}\mathbf{1}^{\top} & 0\\
0 & \frac{2}{n-2}\mathbf{1}\mathbf{1}^{\top}
\end{bmatrix}
-
\begin{bmatrix}
\frac{2}{n-2} & & \\
 & \ddots & \\
 & & \frac{2}{n-2}
\end{bmatrix}\\
&=\frac{2}{n-2}
\begin{bmatrix}
\mathbf{1}\mathbf{1}^{\top}-I_{\frac{n}{2}} & 0\\
0 & \mathbf{1}\mathbf{1}^{\top}-I_{\frac{n}{2}} 
\end{bmatrix}.
\end{align*}
Note that
\begin{align*}
  \begin{bmatrix}
\mathbf{1}\mathbf{1}^{\top}-I_{\frac{n}{2}} & 0\\
0 & \mathbf{1}\mathbf{1}^{\top}-I_{\frac{n}{2}} 
\end{bmatrix}  
\end{align*}
has $2$ singular values equal to $\frac{n}{2}-1$ and $n-2$ singular values equal to $1$. And in this example, we have $r=2$. Thus we verify
\begin{align*}
\sigma_{3}\left(\frac1n M^*\odot \left(\frac1n(\Delta_X Y^{*\top}+X^{*}\Delta^{\top}_Y) \right)\right)=\frac{2}{n-2}<\frac12.
\end{align*}
That is to say Assumption \ref{assumption:r+1} holds with $\eps = 1/2$. Thus, we finish the proofs.




















\subsection{Bridge convex optimizer and approximate nonconvex optimizer}\label{pf:thm_cv_ncv}

In this section, we prove the following theorem.
\begin{theorem}\label{thm:cv_ncv}
Suppose Assumption \ref{assumption:r+1} holds. We then have
\begin{align*}
\left\|
\begin{bmatrix}
\hat{\theta}_c-\hat{\theta}\\
\hat{H}_c-\hat{H}\\
\frac{1}{n}(\hat{\Gamma}_c-\hat{X}\hat{Y}^T)
\end{bmatrix}
\right\|_F
\lesssim \frac{(1+e^{c c_P})^2}{\sl e^{c c_P}}\left(1+\frac{ 72 \kappa n}{\sqrt{\sigma_{\min}}}\right)\|\cP(\nabla f(\hat{\theta},\hat{H},\hat{X},\hat{Y}))\|_F
\end{align*}
for some constant $c$.
\end{theorem}


For notation simplicity, we denote the solution given by gradient descent as $(\theta,H,X,Y)$ instead of $(\hat{\theta},\hat{H},\hat{X},\hat{Y})$. First of all, we have the following claim.
\begin{claim}\label{claim1:pf_cv_ncv}
Let $U\Sigma V^T$ be the SVD of $XY^T$. There exists an invertible matrix $Q\in\bbR^{r\times r}$ such that $X=U\Sigma^{1/2}Q$, $Y=V\Sigma^{1/2}Q^{-T}$ and
\begin{align}\label{ineq1:pf_cv_ncv}
\left\|\Sigma_Q-\Sigma_Q^{-1}\right\|_F\leq\frac{8 \sqrt{\kappa} }{\lambda \sqrt{\sigma_{\min}}} \|\cP(\nabla f(\theta,H,X,Y))\|_F.
\end{align}
Here $U_Q\Sigma_Q V_Q^T$ is the SVD of Q. 
% and $\cP$ is the projection onto the space where $\mathbf{1}^T\nabla_{\theta} f(\theta, H, X, Y)=0$.
\end{claim}
\begin{proof}[Proof of Claim \ref{claim1:pf_cv_ncv}]
Let
\begin{align*}
B_1:=\nabla_{\Gamma}L_c(\theta,H,XY^{\top})Y + \lambda X \quad \text{and} \quad B_2:=\nabla_{\Gamma}L_c(\theta,H,XY^{\top})X + \lambda Y.
\end{align*}
By the definition of $\nabla_X f(\theta,H,X,Y)$ and $\nabla_Y f(\theta,H,X,Y)$, we have
\begin{align*}
    \max\{\|{B}_1\|_F, \|{B}_2\|_F\} 
   & =\max\{\|\nabla_X f(\theta,H,X,Y)\|_F, \|\nabla_Y f(\theta,H,X,Y)\|_F\}\\
&\leq \|\cP(\nabla f(\theta,H,X,Y))\|_F.
\end{align*}
In addition, the definition of $B_1$ and $B_2$ allow us to obtain
\begin{align*}
    \|X^\top X - Y^\top Y\|_F &= \frac{1}{\lambda} \|X^\top ({B}_1 - \nabla_{\Gamma}L_c(\theta,H,XY^{\top}) Y) - ({B}_2 - \nabla_{\Gamma}L_c(\theta,H,XY^{\top})X)^{\top}Y\|_F \\
    &= \frac{1}{\lambda} \|X^\top {B}_1 - {B}_2^\top Y\|_F \\
    &\leq \frac{1}{\lambda} \|X\| \|{B}_1\|_F + \frac{1}{\lambda} \|{B}_2\|_F \|Y\| \\
    &\leq \frac{4}{\lambda} \sqrt{ \sigma_{\max}} \|\cP(\nabla f(\theta,H,X,Y))\|_F.
\end{align*}
Here, the last inequality follows from the fact that $\|X\|, \|Y\| \leq 2\sqrt{\sigma_{\max}}$. In view of Lemma \ref{ar:lem6}, one can find an invertible ${Q}$ such that $X = U \Sigma^{1/2} {Q}$, $Y = V \Sigma^{1/2} {Q}^{-T}$ and
\begin{align*}
    \|\Sigma_{Q} - \Sigma_{Q}^{-1}\|_F &\leq \frac{1}{\sigma_{\min} (\Sigma)} \|X^\top X - Y^\top Y\|_F \\
    &\leq \frac{2}{\sigma_{\min}} \cdot \frac{4}{\lambda} \sqrt{ \sigma_{\max}} \|\cP(\nabla f(\theta,H,X,Y))\|_F\\
    &= \frac{8 \sqrt{\kappa} }{\lambda \sqrt{\sigma_{\min}}} \|\cP(\nabla f(\theta,H,X,Y))\|_F,
\end{align*}
where $\Sigma_Q$ is a diagonal matrix consisting of all singular values of ${Q}$. Here the second inequality follows from 
\begin{align*}
\left|\sigma_{\min}(XY^{\top})-\sigma_{\min}(X^* Y^{*\top})\right|\leq \left\|XY^{\top}-X^* Y^{*\top}\right\|\lesssim \sqrt{\sigma_{\max}}\|X-X^*\|\lesssim c_{14}\sqrt{\sigma_{\max} n},
\end{align*}
which implies $\sigma_{\min}(XY^{\top})\geq \sigma_{\min}/2$ as long as $c_{14}\sqrt{\sigma_{\max} n}\ll \sigma_{\min}$.
This completes the proof.   
\end{proof}

With Claim \ref{claim1:pf_cv_ncv} in hand, we are ready to establish the following claim.
\begin{claim}\label{claim2:pf_cv_ncv}
Suppose that Assumption \ref{assumption:r+1} holds. Under the same notations in Claim \ref{claim1:pf_cv_ncv}, let $\nabla_{\Gamma}L_c(\theta, H, XY^{\top})=-\lambda UV^{\top}+R$.
% \begin{align*}
% \nabla_{\Gamma}L_c(\theta, H, XY^{\top})=-\lambda UV^{\top}+R,
% \end{align*}
Then $R$ satisfies:
\begin{align*}
\|\cP_{\cT}(R)\|_F\leq \frac{ 72 \kappa}{\sqrt{\sigma_{\min}}} \|\cP(\nabla f(\theta,H,X,Y))\|_F\quad\text{and}\quad \|\cP_{\cT^{\perp}}(R)\|<\left(1-\frac{\eps}{4}\right)\lambda
\end{align*}
for $\eps>0$ specified in Assumption \ref{assumption:r+1}. Here $\cT$ is the tangent space for $U\Sigma V^{\top}$ defined as 
\begin{align*}
\cT:=\{UA^{\top}+BV^{\top}\mid A,B\in\bbR^{n\times r}\},
\end{align*}
$\cT^{\perp}$ is the orthogonal complement of $\cT$, and $\cP_{\cT}$, $\cP_{\cT^{\perp}}$ are the orthogonal projection onto the subspace $\cT$, $\cT^{\perp}$, respectively.
\end{claim}
\begin{proof}[Proof of Claim \ref{claim2:pf_cv_ncv}]
Recall the notations in the proof of Claim \ref{claim1:pf_cv_ncv}, we have
\begin{align}\label{eq:B}
B_1=\nabla_{\Gamma}L_c(\theta,H,XY^{\top})Y + \lambda X \quad \text{and} \quad B_2=\nabla_{\Gamma}L_c(\theta,H,XY^{\top})X + \lambda Y.
\end{align}
By the definition of $R$, we have
\begin{align}\label{eq:R}
\nabla_{\Gamma}L_c(\theta, H, XY^{\top})=R-\lambda UV^{\top}.
\end{align}
From the definition of $\mathcal{P}_{\cT}$, we have
\begin{align}\label{eq4:pf_cv_ncv}
    \|\mathcal{P}_{\cT}({R})\|_F &= \|UU^\top {R} (I - VV^\top) + RVV^\top\|_F \notag\\
    &\leq \|U^\top {R} (I - VV^\top)\|_F + \|RVV^\top\|_F \notag\\
    &\leq \|U^\top {R}\|_F + \|RV\|_F.
\end{align}
In addition, by Claim \ref{claim1:pf_cv_ncv}, we have
\begin{align}\label{eq2:pf_cv_ncv}
    X &= U \Sigma^{1/2} {Q} \quad \text{and} \quad Y = V \Sigma^{1/2} {Q}^{-T} 
\end{align}
for some invertible matrix ${Q} \in \mathbb{R}^{r \times r}$, whose SVD $U_Q \Sigma_Q V_Q^\top$ obeys \eqref{ineq1:pf_cv_ncv}. Combine \eqref{eq:B} and \eqref{eq:R}, we have
\begin{align*}
    -\lambda UV^\top Y + RY &= -\lambda X + {B}_1,
\end{align*}
which together with \eqref{eq2:pf_cv_ncv} yields
\begin{align*}
    RV &= \lambda U \Sigma^{1/2} (I_r - {Q} {Q}^\top) \Sigma^{-1/2} + {B}_1 {Q}^\top \Sigma^{-1/2}.
\end{align*}
Apply the triangle inequality to get
\begin{align}\label{eq3:pf_cv_ncv}
    \|RV\|_F &\leq \|\lambda U \Sigma^{1/2} (I_r - {Q} {Q}^\top) \Sigma^{-1/2}\|_F + \|{B}_1 {Q}^\top \Sigma^{-1/2}\|_F \notag\\
    &\leq \lambda \|\Sigma^{1/2}\| \|\Sigma^{-1/2}\| \| {Q} {Q}^\top - I_r \|_F + \|{Q}\| \|\Sigma^{-1/2}\| \|{B}_1\|_F.
\end{align}
In order to further upper bound \eqref{eq3:pf_cv_ncv}, we first recognize the fact that as long as $c_{14}\sqrt{\sigma_{\max} n}\ll \sigma_{\min}$,
\begin{align*}
    \|\Sigma^{1/2}\| &\leq \sqrt{2 \sigma_{\max}}, \quad \text{and} \quad \|\Sigma^{-1/2}\| = 1 / \sqrt{\sigma_{\min} (\Sigma)} \leq \sqrt{2 / \sigma_{\min}},
\end{align*}
which holds since
\begin{align*}
\left|\sigma_{i}(XY^{\top})-\sigma_{i}(X^* Y^{*\top})\right|\leq \left\|XY^{\top}-X^* Y^{*\top}\right\|\lesssim \sqrt{\sigma_{\max}}\|X-X^*\|\lesssim c_{14}\sqrt{\sigma_{\max} n}.
\end{align*}
Second, Claim \ref{claim1:pf_cv_ncv} and \eqref{ncv:grad} yields
\begin{align*}
    \|\Sigma_{Q} - \Sigma_{Q}^{-1}\|_F &\leq \frac{8 \sqrt{\kappa} }{\lambda \sqrt{\sigma_{\min}}} \|\cP(\nabla f(\theta,H,X,Y))\|_F \ll 1 .
\end{align*}
This in turn implies that $\|{Q}\| = \|\Sigma_Q\| \leq 2$. Putting the above bounds together yields
\begin{align*}
    \|RV\|_F &\leq \lambda \sqrt{2 \sigma_{\max}} \sqrt{\frac{2}{\sigma_{\min}}} \|\Sigma_Q^2 - I_r\|_F + 2 \sqrt{\frac{2}{\sigma_{\min}}} \|\cP(\nabla f(\theta,H,X,Y))\|_F \\
    &\leq \lambda \sqrt{2 \sigma_{\max}} \sqrt{\frac{2}{\sigma_{\min}}} \|\Sigma_Q \| \|\Sigma_Q - \Sigma_Q^{-1}\|_F + 2 \sqrt{\frac{2}{\sigma_{\min}}}\|\cP(\nabla f(\theta,H,X,Y))\|_F \\
    &\leq 2 \lambda \sqrt{2 \sigma_{\max}} \sqrt{\frac{2}{\sigma_{\min}}}\frac{8 \sqrt{\kappa} }{\lambda \sqrt{\sigma_{\min}}} \|\cP(\nabla f(\theta,H,X,Y))\|_F + 2 \sqrt{\frac{2}{\sigma_{\min}}} \|\cP(\nabla f(\theta,H,X,Y))\|_F  \\
    &\leq \frac{ 36 \kappa}{\sqrt{\sigma_{\min}}} \|\cP(\nabla f(\theta,H,X,Y))\|_F .
\end{align*}
Similarly, we can show that
\begin{align*}
    \|U^\top {R}\|_F &\leq \frac{ 36 \kappa}{\sqrt{\sigma_{\min}}} \|\cP(\nabla f(\theta,H,X,Y))\|_F.
\end{align*}
These bounds together with \eqref{eq4:pf_cv_ncv} result in
\begin{align}\label{eq6:pf_cv_ncv}
    \|\mathcal{P}_{\cT}({R})\|_F &\leq \frac{ 72 \kappa}{\sqrt{\sigma_{\min}}} \|\cP(\nabla f(\theta,H,X,Y))\|_F.
\end{align}


In the following, we establish the bound for $\|\cP_{\cT^{\perp}}(R)\|$. Note that
\begin{align*}
\nabla_{\Gamma}L_c(\theta,H,XY^{\top})=-\lambda UV^{\top}+R=-\lambda UV^{\top}+\mathcal{P}_{\cT}({R})+\mathcal{P}_{\cT^{\perp}}({R}).
\end{align*}
Suppose for the moment that
\begin{align}\label{eq5:pf_cv_ncv}
  \|\mathcal{P}_{\cT}({R})\|_F \leq\frac{\eps}{4}\lambda \quad\text{and} \quad \sigma_{r+1}\left(\nabla_{\Gamma}L_c(\theta,H,XY^{\top})\right)<\left(1-\frac{\eps}{2}\right)\lambda.
\end{align}
Then, by Weyl's inequality, we have
\begin{align*}
\sigma_{r+1}\left(-\lambda UV^{\top}+\mathcal{P}_{\cT^{\perp}}({R})\right)
&\leq\sigma_{r+1}\left( -\lambda UV^{\top}+\mathcal{P}_{\cT}({R})+\mathcal{P}_{\cT^{\perp}}({R})\right)+\|\mathcal{P}_{\cT}({R})\|_F\\
&=\sigma_{r+1}\left(\nabla_{\Gamma}L_c(\theta,H,XY^{\top})\right)+\|\mathcal{P}_{\cT}({R})\|_F\\
&< \left(1-\frac{\eps}{2}\right)\lambda+\frac{\eps}{4}\lambda\\
&=\left(1-\frac{\eps}{4}\right)\lambda.
\end{align*}
Since $-\lambda UV^T\in\cT$ with $r$ singular values of $\lambda$, we conclude that 
\begin{align*}
\|\cP_{\cT^{\perp}}(R)\|<\left(1-\frac{\eps}{4}\right)\lambda.
\end{align*}
Thus, it remains to verify the two conditions listed in \eqref{eq5:pf_cv_ncv}. For the first condition, by \eqref{eq6:pf_cv_ncv}, we have
\begin{align*}
\|\mathcal{P}_{\cT}({R})\|_F \leq\frac{\eps}{4}\lambda\quad\text{as long as} \quad 
\|\cP(\nabla f(\theta,H,X,Y))\|_F\leq \frac{\eps\lambda}{288\kappa}\sqrt{\sigma_{\min}},
\end{align*}
which is guaranteed by \eqref{ncv:grad}. 
We then verify the second condition in the following. For notation simplicity, we denote
\begin{align*}
\ell_{ij}(x):=\log (1+e^x)-A_{ij}x.
\end{align*}
Then we have
\begin{align*}
&\left(\nabla_{\Gamma} L_c(\theta,H,XY^{\top})-\nabla_{\Gamma} L_c(\theta^{*},H^{*},{\Gamma}^{{*}})\right)_{ij}\\
&=
\begin{cases}
\int^1_{0}\ell''_{ij}\left(P^{*}_{ij}+\tau(P_{ij}-P^{*}_{ij})\right)d\tau\cdot \frac{P_{ij}-P^{*}_{ij}}{n} & i\neq j\\
0 & i=j
\end{cases}.
\end{align*}
We define a matrix $H\in\bbR^{n\times n}$ such that
\begin{align*}
H_{ij}=
\begin{cases}
\int^1_{0}\ell''_{ij}\left(P^{*}_{ij}+\tau(P_{ij}-P^{*}_{ij})\right)d\tau & i\neq j\\
0 & i=j
\end{cases}.
\end{align*}
It then holds that
\begin{align}\label{eq14:pr_cv_ncv}
&\nabla_{\Gamma} L_c(\theta,H,XY^{\top})\notag\\
&=\nabla_{\Gamma} L_c(\theta^{*},H^{*},{\Gamma}^{{*}})+\frac1n H\odot(P-P^*)\notag\\
&=\nabla_{\Gamma} L_c(\theta^{*},H^{*},{\Gamma}^{{*}})+\frac1n (H-M^*)\odot(P-P^*)+\frac1n M^*\odot(P-P^*).
\end{align}
Recall the definition of $M^*$ where 
\begin{align*}
M^{*}_{ij}=
\begin{cases}
    \frac{e^{P_{ij}^*}}{(1+e^{P_{ij}^*})^2} & i\neq j\\
    0 & i=j
\end{cases}
=\begin{cases}
    \ell''_{ij}(P^{*}_{ij}) & i\neq j\\
    0 & i=j
\end{cases}.
\end{align*}
We then have for $i\neq j$:
\begin{align*}
|M^{*}_{ij}-H_{ij}|\leq \int^1_{0}\left|\ell''_{ij}\left(P^{*}_{ij}+\tau(P_{ij}-P^{*}_{ij})\right)- \ell''_{ij}(P^{*}_{ij})\right|d\tau\leq \frac14 |P_{ij}-P^{*}_{ij}|,
\end{align*}
where the last inequality follows from the mean-value theorem and the fact that $|\ell'''_{ij}(x)|\leq \ell''_{ij}(x)\leq 1/4$ for any $x$.
This further implies that
\begin{align*}
&\left\|\frac1n (H-M^*)\odot(P-P^*)\right\|\notag\\
&\leq\left\|\frac1n (H-M^*)\odot(P-P^*)\right\|_F\notag\\
&\leq \frac1n \cdot n\|P-P^{*}\|_{\infty}^2\notag\\
&\leq \left(\frac{2}{\sqrt{n}}\|\theta-\theta^*\|_{\infty}+\frac{\sz}{n}\|H-H^*\|_F+\frac1n \|XY^{\top}-\Gamma^{*}\|_{\infty}\right)^2\\
&\lesssim \left(\frac{1}{\sqrt{n}}\|\theta-\theta^*\|_{\infty}+\frac{\sz}{n}\|H-H^*\|_F+\frac1n\|F^*\|_{2,\infty} \|F-F^*\|_{2,\infty}\right)^2\\
&\lesssim \frac1n \left(c_{41}^2+\sz^2 c_{11}^2+ \mu\sX\sY r^2 c_{43}^2\right),
\end{align*}
where the last inequality follows from \eqref{ncv:est} and Assumption \ref{assumption:incoherent}.
Thus, as long as $n$ large enough, we have
\begin{align}\label{eq12:pf_cv_ncv}
\left\|\frac1n (H-M^*)\odot(P-P^*)\right\|
\lesssim \frac1n \left(c_{41}^2+\sz^2 c_{11}^2+ \mu\sX\sY r^2 c_{43}^2\right)<\frac{\eps\lambda}{10}.
\end{align}
Moreover, as shown in the proofs of Lemma \ref{lem:gradient_norm}, we have
\begin{align}\label{eq13:pf_cv_ncv}
\left\|\nabla_{\Gamma}L_c(\theta^*,H^*,\Gamma^*)\right\|
\lesssim\sqrt{\frac{\log n}{n}}<\frac{\eps\lambda}{10}
\end{align}
as long as $\eps c_{\lambda}\gg 1$.
Thus, it remains to deal with $\frac1n M^*\odot(P-P^*)$.
Note that
\begin{align}\label{eq18:pf_cv_ncv}
\frac1n M^*\odot(P-P^*)=
\underbrace{\frac1n M^*\odot(\hat{P}^d-\bar{P})}_{(1)}
+\underbrace{\frac1n M^*\odot(\bar{P}-P^*)}_{(2)}
+\underbrace{\frac1n M^*\odot(P-\hat{P}^d)}_{(3)}.
\end{align}
In what follows, we will deal with (1),(2) and (3), respectively.
\begin{enumerate}
\item For (1), note that
\begin{align*}
\|(1)\|
&\leq \left\|\frac1n M^*\odot(\hat{P}^d-\bar{P})\right\|_F\\
&\leq \frac{1}{4n}\sqrt{\sum_{i\neq j}(\hat{P}^d_{ij}-\bar{P}_{ij})^2}\\
&\lesssim \frac{\sqrt{\su}}{n}\left(\|\hat{\theta}^d-\bar{\theta}\|_{2}+\|\hat{H}^d-\bar{H}\|_{F}+\frac{1}{n}\|\hat{X}^d\hat{Y}^{d\top}-\bar{X}\bar{Y}^{\top}\|_{F}\right),
\end{align*}
where the last inequality follows the same trick we used before and we omit the details here. By Theorem \ref{thm:ncv_debias}, we obtain
\begin{align}\label{eq14:pf_cv_ncv}
\|(1)\|\lesssim \frac{\sqrt{\su}c_d}{n^{3/4}}<\frac{\eps\lambda}{10}
\end{align}
as long as $n$ is large enough. 

\item 
For (2), note that
\begin{align*}
\|(2)\|
&\leq \left\|\frac1n M^*\odot(\bar{P}-P^*)\right\|_F\\
&\leq \frac{1}{4n}\sqrt{\sum_{i\neq j}(\bar{P}_{ij}-P^*_{ij})^2}\\
&\lesssim \frac{\sqrt{\su}}{n}\left(\|\bar{\theta}-\theta^*\|_{2}+\|\bar{H}-H^*\|_{F}+\frac{1}{n}\|\bar{X}\bar{Y}^{\top}-X^{*}Y^{*\top}\|_{F}\right).
\end{align*}
By Proposition \ref{prop:bar_dist}, we have
\begin{align}\label{eq15:pf_cv_ncv}
\|(2)\|\lesssim c'_a\sqrt{\frac{\su}{n}}<\frac{\eps\lambda}{10}
\end{align}
as long as $\eps c_{\lambda}\gg \sqrt{\su\mu\sX\sY r^2}/\slD$.

\item 
We denote $\hat\Delta$ such that
\begin{align*}
\begin{bmatrix}
\hat{\Delta}_{\theta}\\
\hat{\Delta}_{H}\\
\hat{\Delta}_{X}\\
\hat{\Delta}_{Y}
\end{bmatrix}
=
\begin{bmatrix}
\hat{\theta}^d-\theta\\
\hat{H}^d-H\\
\hat{X}^d-X\\
\hat{Y}^d-Y
\end{bmatrix}.
\end{align*}
With a little abuse of notation, we denote $(\Delta_{\theta}, \Delta_{H}, \Delta_{X}, \Delta_{Y})$ such that
\begin{align*}
\begin{bmatrix}
\Delta_{\theta}\\
\Delta_{H}\\
\Delta_{X}\\
\Delta_{Y}
\end{bmatrix} =-(\cP D^*\cP)^{\dagger}\begin{bmatrix}
0\\
0\\
-\lambda X^{*}\\
-\lambda Y^{*}
\end{bmatrix},
\end{align*}
% \begin{align*}
% \begin{cases}
% \begin{bmatrix}
% 0\\
% 0\\
% -\lambda X^{*}\\
% -\lambda Y^{*}
% \end{bmatrix}
% +\cP D^*\cP
%  \begin{bmatrix}
% \Delta_{\theta}\\
% \Delta_{H}\\
% \Delta_{X}\\
% \Delta_{Y}
% \end{bmatrix}
% =0\\
% \cP_{\theta}(\Delta_{\theta})=\Delta_{\theta}
% \end{cases}.
% \end{align*}
Then by Assumption \ref{assumption:r+1}, we have
\begin{align*}
    \sigma_{r+1}\left(\frac{1}{n}{M}^* \odot \left(\frac{(\Delta_{\theta})_i+(\Delta_{\theta})_j}{\sqrt{n}}+{z}_i^T\Delta_{H}{z}_j+\frac{(\Delta_{X}{Y}^{*T}+{X}^*{\Delta^T_{Y}})_{ij}}{n}\right)_{ij}\right) <(1-\epsilon)\lambda
\end{align*}
for some $\eps>0$.
We further have the following claim.
\begin{claim}\label{claim1:delta_diff}
It holds that
\begin{align*}
 \left\|\begin{bmatrix}
\hat{\Delta}_{\theta}-{\Delta}_{\theta}\\
\hat{\Delta}_{H}-{\Delta}_{H}\\
\hat{\Delta}_{X}-{\Delta}_{X}\\
\hat{\Delta}_{Y}-{\Delta}_{Y}
\end{bmatrix}
\right\|_F   \leq c_{\text{diff}},
\end{align*}
where 
\begin{align}
c_{\text{diff}}\asymp \frac{\hat{c}\sqrt{\mu\sX\sY r^2 }+c_{11}\slD}{\slD^2} c_{\lambda}\sqrt{\log n}.
\end{align}
\end{claim}
\begin{proof}[Proof of Claim \ref{claim1:delta_diff}]
By the definition of $(\Delta_{\theta}, \Delta_{H}, \Delta_{X}, \Delta_{Y})$, we have
\begin{align*}
\begin{bmatrix}
\Delta_{\theta}\\
\Delta_{H}\\
\Delta_{X}\\
\Delta_{Y}
\end{bmatrix} =-(\cP D^*\cP)^{\dagger}\begin{bmatrix}
0\\
0\\
-\lambda X^{*}\\
-\lambda Y^{*}
\end{bmatrix},
\end{align*}
where $(\cP D^*\cP)^{\dagger}$ represents the pseudo-inverse of $\cP D^*\cP$.
By the definition of the debiased estimator, we have
\begin{align*}
\begin{bmatrix}
\hat{\Delta}_{\theta}\\
\hat{\Delta}_{H}\\
\hat{\Delta}_{X}\\
\hat{\Delta}_{Y}
\end{bmatrix} 
=-(\cP\hat{D}\cP)^{\dagger}\left(\cP\nabla L(\hat{\theta},\hat{H},\hat{X},\hat{Y})\right),
\end{align*}
where $(\cP \hat{D}\cP)^{\dagger}$ represents the pseudo-inverse of $\cP \hat{D}\cP$.
For notation simplicity, we denote
\begin{align*}
& A_1:=(\cP D^*\cP)^{\dagger},\ 
b_1:=\begin{bmatrix}
0\\
0\\
-\lambda X^{*}\\
-\lambda Y^{*}
\end{bmatrix}\\
\text{and }
& A_2:=(\cP\hat{D}\cP)^{\dagger},\ 
b_2:=\cP\nabla L(\hat{\theta},\hat{H},\hat{X},\hat{Y}).
\end{align*}
It then holds that
\begin{align}\label{eq8:delta_diff}
\left\|\begin{bmatrix}
\hat{\Delta}_{\theta}-{\Delta}_{\theta}\\
\hat{\Delta}_{H}-{\Delta}_{H}\\
\hat{\Delta}_{X}-{\Delta}_{X}\\
\hat{\Delta}_{Y}-{\Delta}_{Y}
\end{bmatrix}
\right\|_F
&=\|A_1b_1-A_2b_2\|_2\notag\\
&\leq \|A_1-A_2\|\|b_2\|_2+\|A_1\|\|b_1-b_2\|_2.
\end{align}
In the following, we control $ \|A_1-A_2\|$, $\|b_1-b_2\|_2$, $\|A_1\|$, and $\|b_2\|_2$, respectively.
\begin{enumerate}
    
\item For $ \|A_1-A_2\|$, by Theorem 3.3 in \cite{stewart1977perturbation}, we have
\begin{align}\label{eq4:delta_diff}
\|A_1-A_2\|
&\leq \frac{1+\sqrt{5}}{2}\max\{\|(\cP\hat{D}\cP)^{\dagger}\|^2, \|(\cP D^*\cP)^{\dagger}\|^2\}\cdot \|\cP\hat{D}\cP-\cP D^*\cP\|.
\end{align}
By Lemma \ref{lem:D}, we have
\begin{align*}
\max\{\|(\cP\hat{D}\cP)^{\dagger}\|^2, \|(\cP D^*\cP)^{\dagger}\|^2\}\lesssim \frac{1}{\slD^2}, \quad
\|\cP\hat{D}\cP-\cP D^*\cP\|\lesssim  \frac{\hat{c}}{\sqrt{n}}.
\end{align*}
Finally, by \eqref{eq4:delta_diff}, we obtain
\begin{align}\label{eqA:delta_diff}
\|A_1-A_2\|\lesssim \frac{\hat{c}}{\slD^2\sqrt{n}}.
\end{align}

\item For $\|b_1-b_2\|_2$, we have
\begin{align}\label{eq5:delta_diff}
\|b_1-b_2\|_2
&=\left\|\begin{bmatrix}
0\\
0\\
-\lambda X^{*}\\
-\lambda Y^{*}
\end{bmatrix}-\cP\nabla L(\hat{\theta},\hat{H},\hat{X},\hat{Y})\right\|_2\notag\\
&\leq \left\|\begin{bmatrix}
0\\
0\\
\lambda X^{*}\\
\lambda Y^{*}
\end{bmatrix}-
\begin{bmatrix}
0\\
0\\
\lambda \hat{X}\\
\lambda \hat{Y}
\end{bmatrix}\right\|_2
+\left\|\cP\nabla L(\hat{\theta},\hat{H},\hat{X},\hat{Y})-\begin{bmatrix}
0\\
0\\
-\lambda \hat{X}\\
-\lambda \hat{Y}
\end{bmatrix}\right\|_2
\end{align}
For the first term, we have
\begin{align}\label{eq6:delta_diff}
 \left\|\begin{bmatrix}
0\\
0\\
\lambda X^{*}\\
\lambda Y^{*}
\end{bmatrix}-
\begin{bmatrix}
0\\
0\\
\lambda \hat{X}\\
\lambda \hat{Y}
\end{bmatrix}\right\|_2
\leq \lambda (\|X^*-\hat{X}\|_F+(\|Y^*-\hat{Y}\|_F)\leq 2 \lambda c_{11}\sqrt{n},
\end{align}
where the last inequality follows from Lemma \ref{lem:ncv1}.
For the second term, follow the same argument as in Appendix \ref{pf:prop_debias_dist}, we have
\begin{align}\label{eq7:delta_diff}
\left\|\cP\nabla L(\hat{\theta},\hat{H},\hat{X},\hat{Y})-\begin{bmatrix}
0\\
0\\
-\lambda \hat{X}\\
-\lambda \hat{Y}
\end{bmatrix}\right\|_2   \lesssim n^{-5}.
\end{align}
Combine \eqref{eq5:delta_diff}, \eqref{eq6:delta_diff} and \eqref{eq7:delta_diff}, we have
\begin{align*}
\|b_1-b_2\|_2\lesssim \lambda c_{11}\sqrt{n}.
\end{align*}

\item For $\|A_1\|$, by Lemma \ref{lem:D}, we have $\|A_1\|\leq 1/\slD$.


\item For $\|b_2\|_2$, we have
\begin{align*}
\|b_2\|_2
&\leq \|b_1-b_2\|_2+\|b_1\|_2\\
&\leq \|b_1-b_2\|_2+\lambda(\|X^*\|_F+\|Y^*\|_F)\\
&\lesssim \lambda \sqrt{\mu r\sigma_{\max}}
\end{align*}
as long as $ \sqrt{\mu r\sigma_{\max}}\gg c_{11}\sqrt{n}$.




\end{enumerate}

Combine the above results with \eqref{eq8:delta_diff}, we have
\begin{align*}
\left\|\begin{bmatrix}
\hat{\Delta}_{\theta}-{\Delta}_{\theta}\\
\hat{\Delta}_{H}-{\Delta}_{H}\\
\hat{\Delta}_{X}-{\Delta}_{X}\\
\hat{\Delta}_{Y}-{\Delta}_{Y}
\end{bmatrix}
\right\|_2 
&\lesssim \frac{\hat{c}}{\slD^2\sqrt{n}}\cdot \lambda \sqrt{\mu r\sigma_{\max}}+\frac{1}{\slD}\cdot\lambda c_{11}\sqrt{n}\\
&\leq \frac{\hat{c}}{\slD^2}\cdot \lambda \sqrt{\mu\sX\sY r^2 n}+\frac{1}{\slD}\cdot\lambda c_{11}\sqrt{n}\\
&=\frac{\hat{c}\sqrt{\mu\sX\sY r^2 }+c_{11}\slD}{\slD^2} c_{\lambda}\sqrt{\log n}.
\end{align*}
We then finish the proofs.

\end{proof}








By Weyl's inequality, we have
\begin{align*}
&\sigma_{r+1}\left(\frac{1}{n}{M}^* \odot \left((\hat{P}^d-P)-\frac1n(\hat{X}^d-X)(\hat{Y}^d-Y)^{\top}\right)\right)\\
&=\sigma_{r+1}\left(\frac{1}{n}{M}^* \odot \left(\frac{(\hat{\Delta}_{\theta})_i+(\hat{\Delta}_{\theta})_j}{\sqrt{n}}+{z}_i^T\hat{\Delta}_{H}{z}_j+\frac{(\hat{\Delta}_{X}{Y}^{T}+{X}{\hat{\Delta}^T_{Y}})_{ij}}{n}\right)_{ij}\right)\\
&\leq \sigma_{r+1}\left(\frac{1}{n}{M}^* \odot \left(\frac{(\Delta_{\theta})_i+(\Delta_{\theta})_j}{\sqrt{n}}+{z}_i^T\Delta_{H}{z}_j+\frac{(\Delta_{X}{Y}^{*T}+{X}^*{\Delta^T_{Y}})_{ij}}{n}\right)_{ij}\right)\\
&\quad +\frac1n \left\|{M}^* \odot\left(\frac{(\hat{\Delta}_{\theta}-{\Delta}_{\theta})_i+(\hat{\Delta}_{\theta}-{\Delta}_{\theta})_j}{\sqrt{n}}\right)_{ij} \right\|_F+\frac1n \left\|{M}^* \odot\left({z}_i^T(\hat{\Delta}_{H}-{\Delta}_{H}){z}_j\right)_{ij} \right\|_F\\
&\quad + \frac{1}{n^2} \left\|{M}^* \odot \left((\hat{\Delta}_{X}{Y}^{T}+{X}{\hat{\Delta}^T_{Y}})-(\Delta_{X}{Y}^{*T}+{X}^*{\Delta^T_{Y}})\right) \right\|_F\\
&\leq \sigma_{r+1}\left(\frac{1}{n}{M}^* \odot \left(\frac{(\Delta_{\theta})_i+(\Delta_{\theta})_j}{\sqrt{n}}+{z}_i^T\Delta_{H}{z}_j+\frac{(\Delta_{X}{Y}^{*T}+{X}^*{\Delta^T_{Y}})_{ij}}{n}\right)_{ij}\right)\\
&\quad +\frac{1}{4n} \left\|\left(\frac{(\hat{\Delta}_{\theta}-{\Delta}_{\theta})_i+(\hat{\Delta}_{\theta}-{\Delta}_{\theta})_j}{\sqrt{n}}\right)_{ij} \right\|_F+\frac{1}{4n}\left\|\left({z}_i^T(\hat{\Delta}_{H}-{\Delta}_{H}){z}_j\right)_{ij} \right\|_F\\
&\quad + \frac{1}{4n^2} \left\|(\hat{\Delta}_{X}{Y}^{T}+{X}{\hat{\Delta}^T_{Y}})-(\Delta_{X}{Y}^{*T}+{X}^*{\Delta^T_{Y}})\right\|_F.
\end{align*}
By Claim \ref{claim1:delta_diff}, we can bound the Frobenius norms on the RHS respectively.
\begin{enumerate}
    \item For the first Frobenius norm, we have
    \begin{align*}
      \left\|\left(\frac{(\hat{\Delta}_{\theta}-{\Delta}_{\theta})_i+(\hat{\Delta}_{\theta}-{\Delta}_{\theta})_j}{\sqrt{n}}\right)_{ij} \right\|_F  \leq 2 \|\hat{\Delta}_{\theta}-{\Delta}_{\theta}\|_2\lesssim c_{\text{diff}}.
    \end{align*}


    
      \item For the second Frobenius norm, we have
      \begin{align*}
      \left\|\left({z}_i^T(\hat{\Delta}_{H}-{\Delta}_{H}){z}_j\right)_{ij} \right\|_F
      &=\sqrt{\sum_{i,j}\left({z}_i^T(\hat{\Delta}_{H}-{\Delta}_{H}){z}_j\right)^2}    \\
      &\leq \|\hat{\Delta}_{H}-{\Delta}_{H}\|\sqrt{\sum_{i,j}\|z_i\|_2^2\|z_j\|_2^2} \\
      &\leq \sz \|\hat{\Delta}_{H}-{\Delta}_{H}\| \\
      &\leq \sz c_{\text{diff}}.
      \end{align*}


      \item For the third Frobenius norm, we have
      \begin{align*}
        &\left\|(\hat{\Delta}_{X}{Y}^{T}+{X}{\hat{\Delta}^T_{Y}})-(\Delta_{X}{Y}^{*T}+{X}^*{\Delta^T_{Y}})\right\|_F\\
        &\leq \|\hat{\Delta}_{X}{Y}^{T}-\Delta_{X}{Y}^{*T}\|_F
        + \|{X}{\hat{\Delta}^T_{Y}}-{X}^*{\Delta^T_{Y}}\|_F\\
        &\leq \|\hat{\Delta}_{X}\|_F \|Y-Y^*\|_F+ \|Y^*\|_F \|\hat{\Delta}_{X}-{\Delta}_{X}\|_F+\|\hat{\Delta}_{Y}\|_F \|X-X^*\|_F+ \|X^*\|_F \|\hat{\Delta}_{Y}-{\Delta}_{Y}\|_F\\
        &\lesssim c_a c_{11} n+\sqrt{\mu r \sigma_{\max}}c_{\text{diff}}\\
        &\lesssim ( c_a c_{11}+\sqrt{\mu\sX\sY r^2}c_{\text{diff}})n,
      \end{align*}
where the last inequality follows from Lemma \ref{lem:ncv1}, Proposition \ref{prop:debias_dist}, Claim \ref{claim1:delta_diff}, and Assumption \ref{assumption:incoherent}.


\end{enumerate}

Combine the above bounds, we have
\begin{align*}
&\sigma_{r+1}\left(\frac{1}{n}{M}^* \odot \left((\hat{P}^d-P)-\frac1n(\hat{X}^d-X)(\hat{Y}^d-Y)^{\top}\right)\right)\\
&\leq \sigma_{r+1}\left(\frac{1}{n}{M}^* \odot \left(\frac{(\Delta_{\theta})_i+(\Delta_{\theta})_j}{\sqrt{n}}+{z}_i^T\Delta_{H}{z}_j+\frac{(\Delta_{X}{Y}^{*T}+{X}^*{\Delta^T_{Y}})_{ij}}{n}\right)_{ij}\right)\\
&\quad+\frac{c}{n}( c_a c_{11}+\sqrt{\mu\sX\sY r^2}c_{\text{diff}})\\
&< (1-\eps)\lambda +\frac{\eps\lambda}{20}\\
&=\left(1-\frac{19\eps}{20}\right)\lambda
\end{align*}
as long as $ c_a c_{11}+\sqrt{\mu\sX\sY r^2}c_{\text{diff}}\ll \eps\lambda n$ ($n$ is large enough).
By Weyl's inequality, we have
\begin{align}
&\sigma_{r+1}\left(\frac{1}{n}{M}^* \odot (\hat{P}^d-P)\right)\notag\\
&\leq \sigma_{r+1}\left(\frac{1}{n}{M}^* \odot \left((\hat{P}^d-P)-\frac1n(\hat{X}^d-X)(\hat{Y}^d-Y)^{\top}\right)\right)+\frac{1}{n^2}\left\|{M}^* \odot(\hat{X}^d-X)(\hat{Y}^d-Y)^{\top}\right\|_F\notag\\
&\leq \sigma_{r+1}\left(\frac{1}{n}{M}^* \odot \left((\hat{P}^d-P)-\frac1n(\hat{X}^d-X)(\hat{Y}^d-Y)^{\top}\right)\right)+\frac{1}{4n^2}\|\hat{X}^d-X\|_F\|\hat{Y}^d-Y\|_F\notag\\
&\leq \sigma_{r+1}\left(\frac{1}{n}{M}^* \odot \left((\hat{P}^d-P)-\frac1n(\hat{X}^d-X)(\hat{Y}^d-Y)^{\top}\right)\right)+\frac{c_a^2}{4n}\tag{by Proposition \ref{prop:debias_dist}}\\
&<\left(1-\frac{19\eps}{20}\right)\lambda+\frac{\eps\lambda}{20}\notag\\\label{eq16:pf_cv_ncv}
&=\left(1-\frac{9\eps}{10}\right)\lambda
\end{align}
as long as $c_a^2\ll \eps\lambda n$ ($n$ is large enough).
\end{enumerate}

Combine \eqref{eq18:pf_cv_ncv}, \eqref{eq14:pf_cv_ncv}, \eqref{eq15:pf_cv_ncv}, \eqref{eq16:pf_cv_ncv} and apply Weyl's inequality, we have
\begin{align}\label{eq19:pf_cv_ncv}
\sigma_{r+1}\left(\frac{1}{n}{M}^* \odot (P-P^*)\right)
&\leq \sigma_{r+1}\left(\frac{1}{n}{M}^* \odot (P-\hat{P}^d)\right)+\|(1)\|+\|(2)\|\notag\\    
&<\left(1-\frac{9\eps}{10}\right)\lambda+\frac{\eps\lambda}{10}+\frac{\eps\lambda}{10}\notag\\
&=\left(1-\frac{7\eps}{10}\right)\lambda.
\end{align}

Finally, combine \eqref{eq14:pr_cv_ncv}, \eqref{eq12:pf_cv_ncv}, \eqref{eq13:pf_cv_ncv}, \eqref{eq19:pf_cv_ncv} and apply Weyl's inequality, we have
\begin{align*}
&\sigma_{r+1}\left(\nabla_{\Gamma} L_c(\theta,H,XY^{\top})\right)\notag\\
&\leq \sigma_{r+1}\left(\frac{1}{n}{M}^* \odot (P-P^*)\right)+\left\|\frac1n (H-M^*)\odot(P-P^*)\right\|+\left\|\nabla_{\Gamma}L_c(\theta^*,H^*,\Gamma^*)\right\|\notag\\
&<\left(1-\frac{7\eps}{10}\right)\lambda+\frac{\eps\lambda}{10}+\frac{\eps\lambda}{10}\notag\\
&=\left(1-\frac{\eps}{2}\right)\lambda.
\end{align*}
Thus, we finish the proof of Claim \ref{claim2:pf_cv_ncv}.



\end{proof}

The following claim shows that $\|\hat{\theta}_c-\theta^*\|_{\infty}$, $\|\hat{H}_c-H^*\|_F$, $\|\hat{\Gamma}_c-\Gamma^*\|_{\infty}$ is bounded even though the convex optimization problem is not constrained to do so.
\begin{claim}\label{claim:MLE_bound}
We have
\begin{align*}
\|\hat{\theta}_c-\theta^*\|_{\infty}\leq c_P \sqrt{n}, \ 
\|\hat{H}_c-H^*\|_{F}\leq c_P n, \ \|\hat{\Gamma}_c-\Gamma^*\|_{\infty}\leq c_P n.
\end{align*}
\end{claim}
\begin{proof}[Proof of Claim \ref{claim:MLE_bound}]
In the following, we fix a constant $c=c_P$. We define a constraint convex optimization problem as
\begin{align}\label{obj:con}
(\hat{\theta}^{con}, \hat{H}^{con}, \hat{\Gamma}^{con}) 
:=\argmin_{\substack{\mathbf{1}^{\top}\theta=0,\|{\theta}-\theta^*\|_{\infty}\leq c\sqrt{n},\\
\|{H}-H^*\|_{F}\leq c n, \ \|{\Gamma}-\Gamma^*\|_{\infty}\leq c n}} f_c(\theta,H,\Gamma),
\end{align}
where $f_c$ is the convex objective defined in \eqref{obj:cv}.
By \eqref{ncv:est}, $(\theta,H, \Gamma)$ is feasible for the constraint of \eqref{obj:con}. We then have
\begin{align}\label{eq7:MLE_bound}
L_c(\hat{\theta}^{con}, \hat{H}^{con}, \hat{\Gamma}^{con}) +\lambda\|\hat{\Gamma}^{con}\|_{*}\leq L_c({\theta}, {H}, {\Gamma})+\lambda\|\Gamma\|_{*}.
\end{align}
We denote 
\begin{align*}
\Delta_{\theta}^{con}:=\hat{\theta}^{con}-\theta,\ 
\Delta_{H}^{con}:=\hat{H}^{con}-H,\ 
\Delta_{\Gamma}^{con}:=\hat{\Gamma}^{con}-\Gamma.
\end{align*}
By Taylor expansion, we have
\begin{align}\label{eq30:MLE_bound}
&L_c(\hat{\theta}^{con}, \hat{H}^{con}, \hat{\Gamma}^{con}) -L_c({\theta}, {H}, {\Gamma})\notag\\
&=\nabla L_c({\theta}, {H}, {\Gamma})^{\top}
\begin{bmatrix}
\Delta_{\theta}^{con}\\
\Delta_{H}^{con}\\
\Delta_{\Gamma}^{con}
\end{bmatrix}
+\frac12 
\begin{bmatrix}
\Delta_{\theta}^{con}\\
\Delta_{H}^{con}\\
\Delta_{\Gamma}^{con}
\end{bmatrix}^{\top}
\nabla^2 L_c(\tilde{\theta}, \tilde{H}, \tilde{\Gamma})
\begin{bmatrix}
\Delta_{\theta}^{con}\\
\Delta_{H}^{con}\\
\Delta_{\Gamma}^{con}
\end{bmatrix}\notag\\
&=\nabla L_c({\theta}, {H}, {\Gamma})^{\top}
\begin{bmatrix}
\Delta_{\theta}^{con}\\
\Delta_{H}^{con}\\
\Delta_{\Gamma}^{con}
\end{bmatrix}
+\frac12 
\begin{bmatrix}
\Delta_{\theta}^{con}\\
\Delta_{H}^{con}\\
\Delta_{\Gamma}^{con}
\end{bmatrix}^{\top}
\left(\sum_{i\neq j}\frac{e^{ \tilde{P}_{ij}}}{(1+e^{ \tilde{P}_{ij}})^2} 
\begin{bmatrix}
\frac{{e}_i+{e}_j}{\sqrt{n}}\\
{z}_i{z}_j^T\\
\frac{{e}_i{e}_j^T}{n}
\end{bmatrix}^{\otimes 2}\right)
\begin{bmatrix}
\Delta_{\theta}^{con}\\
\Delta_{H}^{con}\\
\Delta_{\Gamma}^{con}
\end{bmatrix}.
\end{align}
Note that for some constant $c'$
\begin{align}\label{ineq30:MLE_bound}
 &\begin{bmatrix}
\Delta_{\theta}^{con}\\
\Delta_{H}^{con}\\
\Delta_{\Gamma}^{con}
\end{bmatrix}^{\top}
\left(\sum_{i\neq j}\frac{e^{ \tilde{P}_{ij}}}{(1+e^{ \tilde{P}_{ij}})^2} 
\begin{bmatrix}
\frac{{e}_i+{e}_j}{\sqrt{n}}\\
{z}_i{z}_j^T\\
\frac{{e}_i{e}_j^T}{n}
\end{bmatrix}^{\otimes 2}\right)
\begin{bmatrix}
\Delta_{\theta}^{con}\\
\Delta_{H}^{con}\\
\Delta_{\Gamma}^{con}
\end{bmatrix}\notag\\
&\geq_{(1)}  \frac{e^{c' c_P}}{(1+e^{c' c_P})^2}
\begin{bmatrix}
\Delta_{\theta}^{con}\\
\Delta_{H}^{con}\\
\Delta_{\Gamma}^{con}
\end{bmatrix}^{\top}
\left(\sum_{i\neq j}
\begin{bmatrix}
\frac{{e}_i+{e}_j}{\sqrt{n}}\\
{z}_i{z}_j^T\\
\frac{{e}_i{e}_j^T}{n}
\end{bmatrix}^{\otimes 2}\right)
\begin{bmatrix}
\Delta_{\theta}^{con}\\
\Delta_{H}^{con}\\
\Delta_{\Gamma}^{con}
\end{bmatrix}\notag\\
&=\frac{e^{c' c_P}}{(1+e^{c' c_P})^2}\begin{bmatrix}
\Delta_{\theta}^{con}\\
\Delta_{H}^{con}\\
\frac1n \Delta_{\Gamma}^{con}
\end{bmatrix}^{\top}
\left(\sum_{i\neq j}
\begin{bmatrix}
\frac{{e}_i+{e}_j}{\sqrt{n}}\\
{z}_i{z}_j^T\\
{{e}_i{e}_j^T}
\end{bmatrix}^{\otimes 2}\right)
\begin{bmatrix}
\Delta_{\theta}^{con}\\
\Delta_{H}^{con}\\
\frac1n \Delta_{\Gamma}^{con}
\end{bmatrix}\notag\\
&\geq \frac{\sl e^{c' c_P}}{(1+e^{c' c_P})^2} \left(\|\Delta_{\theta}^{con}\|_2^2+\|\Delta_{H}^{con}\|_F^2+\frac{1}{n^2}\|\Delta_{\Gamma}^{con}\|_F^2\right),
\end{align}
where the last inequality follows from Assumption \ref{assumption:eigenvalues}.
Here (1) follows from the following argument: note that
\begin{align*}
|P_{ij}|
&:=\left|\frac{\theta_i+\theta_j}{\sqrt{n}}+{z}_i^\top{H}{z}_j + \frac{(XY^{\top})_{ij}}{n}\right|\\
&\leq |P_{ij}^{*}|+\frac{2}{\sqrt{n}}\|\theta-\theta^*\|_{\infty}+\frac{\sz}{n}\|H-H^*\|_2+\frac{1}{n}\|XY^{\top}-\Gamma^*\|_{\infty}.
\end{align*}
Further, by \eqref{ncv:est}, we have
\begin{align*}
&\|XY^T-\Gamma^*\|_{\infty}\\
&=\|(X-X^*)Y^T+X^{*}(Y-Y^*)^T\|_{\infty}\\
&\leq \|X-X^*\|_{2,\infty}\|Y\|_{2,\infty}+\|X^{*}\|_{2,\infty}\|Y-Y^*\|_{2,\infty} \tag{Cauchy}\\
&\lesssim c_{43}\sqrt{\mu \sX\sY r^2 n}.
\end{align*}
Thus, by \eqref{ncv:est} and Assumption \ref{assumption:scales}, we have $|P_{ij}|\leq 2c_P$.
Similarly, we have
\begin{align*}
|(\hat{P}^{con})_{ij}|
&:=\left|\frac{(\hat{\theta}^{con})_i+(\hat{\theta}^{con})_j}{\sqrt{n}}+{z}_i^\top{\hat{H}^{con}}{z}_j + \frac{(\hat{\Gamma}^{con})_{ij}}{n}\right|\\
&\leq |P_{ij}^{*}|+\frac{2}{\sqrt{n}}\|\hat{\theta}^{con}-\theta^*\|_{\infty}+\frac{\sz}{n}\|\hat{H}^{con}-H^*\|_2+\frac{1}{n}\|\hat{\Gamma}^{con}-\Gamma^*\|_{\infty}\\
&\leq |P_{ij}^{*}|+\frac{2}{\sqrt{n}}\|\hat{\theta}^{con}-\theta^*\|_{\infty}+\frac{\sz}{n}\|\hat{H}^{con}-H^*\|_F+\frac{1}{n}\|\hat{\Gamma}^{con}-\Gamma^*\|_{\infty}.
\end{align*}
Further, by the constraints, we have $|(\hat{P}^{con})_{ij}|\lesssim c_P$. Since $\tilde{P}_{ij}$ lies between $P_{ij}$ and $(\hat{P}^{con})_{ij}$, we conclude that $|\tilde{P}_{ij}|\lesssim c_P$. Consequently, we have $\frac{e^{ \tilde{P}_{ij}}}{(1+e^{ \tilde{P}_{ij}})^2} \geq \frac{e^{c' c_P}}{(1+e^{c' c_P})^2}$ for some constant $c'$, which implies (1).

Combine \eqref{eq30:MLE_bound} and \eqref{ineq30:MLE_bound}, we have
\begin{align}\label{eq8:MLE_bound}
L_c(\hat{\theta}^{con}, \hat{H}^{con}, \hat{\Gamma}^{con}) -L_c({\theta}, {H}, {\Gamma})
\geq \nabla L_c({\theta}, {H}, {\Gamma})^{\top}
\begin{bmatrix}
\Delta_{\theta}^{con}\\
\Delta_{H}^{con}\\
\Delta_{\Gamma}^{con}
\end{bmatrix}
+C\left(\|\Delta_{\theta}^{con}\|_2^2+\|\Delta_{H}^{con}\|_F^2+\frac{1}{n^2}\|\Delta_{\Gamma}^{con}\|_F^2\right)
\end{align}
for $C:=\frac{\sl e^{c' c_P}}{2(1+e^{c' c_P})^2} $. By \eqref{eq7:MLE_bound} and \eqref{eq8:MLE_bound}, we obtain
\begin{align}\label{eq9:MLE_bound}
 C\left(\|\Delta_{\theta}^{con}\|_2^2+\|\Delta_{H}^{con}\|_F^2+\frac{1}{n^2}\|\Delta_{\Gamma}^{con}\|_F^2\right)
 \leq -\nabla L_c({\theta}, {H}, {\Gamma})^{\top}
\begin{bmatrix}
\Delta_{\theta}^{con}\\
\Delta_{H}^{con}\\
\Delta_{\Gamma}^{con}
\end{bmatrix}+\lambda\|\Gamma\|_{*}-\lambda\|\hat{\Gamma}^{con}\|_{*}.
\end{align}
In addition, by the convexity of $\|\cdot\|_{*}$, we have
\begin{align*}
\|\hat{\Gamma}^{con}\|_{*}-\|\Gamma\|_{*}=\|\Gamma+\Delta_{\Gamma}^{con}\|_{*}-\|\Gamma\|_{*}\geq \langle UV^{\top}+W,\Delta_{\Gamma}^{con}\rangle
\end{align*}
for any $W\in\cT^{\perp}$ obeying $\|W\|\leq 1$. In the following, we pick $W$ such that $\langle W, \Delta_{\Gamma}^{con}\rangle=\|\cP_{\cT^{\perp}}(\Delta_{\Gamma}^{con})\|_{*}$. We then obtain $\|\hat{\Gamma}^{con}\|_{*}-\|\Gamma\|_{*}\geq  \langle UV^{\top},\Delta_{\Gamma}^{con}\rangle+\|\cP_{\cT^{\perp}}(\Delta_{\Gamma}^{con})\|_{*}$, and consequently, by \eqref{eq9:MLE_bound}, we have
\begin{align*}
C\left(\|\Delta_{\theta}^{con}\|_2^2+\|\Delta_{H}^{con}\|_F^2+\frac{1}{n^2}\|\Delta_{\Gamma}^{con}\|_F^2\right)
 \leq -\nabla L_c({\theta}, {H}, {\Gamma})^{\top}
\begin{bmatrix}
\Delta_{\theta}^{con}\\
\Delta_{H}^{con}\\
\Delta_{\Gamma}^{con}
\end{bmatrix}-\lambda\langle UV^{\top},\Delta_{\Gamma}^{con}\rangle-\lambda\|\cP_{\cT^{\perp}}(\Delta_{\Gamma}^{con})\|_{*}.
\end{align*}
Recall the definition of $R$ in \eqref{eq:R}, we further have
\begin{align}\label{eq10:MLE_bound}
&C\left(\|\Delta_{\theta}^{con}\|_2^2+\|\Delta_{H}^{con}\|_F^2+\frac{1}{n^2}\|\Delta_{\Gamma}^{con}\|_F^2\right)\notag\\
& \leq  -\nabla_{\theta} L_c({\theta}, {H}, {\Gamma})^{\top} \Delta_{\theta}^{con} -\nabla_{H} L_c({\theta}, {H}, {\Gamma})^{\top} \Delta_{H}^{con}-\langle R,\Delta_{\Gamma}^{con}\rangle-\lambda\|\cP_{\cT^{\perp}}(\Delta_{\Gamma}^{con})\|_{*}\notag\\
&=  -\nabla_{\theta} L_c({\theta}, {H}, {\Gamma})^{\top} \Delta_{\theta}^{con} -\nabla_{H} L_c({\theta}, {H}, {\Gamma})^{\top} \Delta_{H}^{con}-\langle \cP_{\cT}(R),\Delta_{\Gamma}^{con}\rangle-\langle \cP_{\cT^{\perp}}(R),\Delta_{\Gamma}^{con}\rangle-\lambda\|\cP_{\cT^{\perp}}(\Delta_{\Gamma}^{con})\|_{*}\notag\\
&\leq  -\nabla_{\theta} L_c({\theta}, {H}, {\Gamma})^{\top} \Delta_{\theta}^{con} -\nabla_{H} L_c({\theta}, {H}, {\Gamma})^{\top} \Delta_{H}^{con}\notag\\
&\quad +\|\cP_{\cT}(R)\|_F\|\cP_{\cT}(\Delta_{\Gamma}^{con})\|_F-\langle \cP_{\cT^{\perp}}(R),\Delta_{\Gamma}^{con}\rangle-\lambda\|\cP_{\cT^{\perp}}(\Delta_{\Gamma}^{con})\|_{*}.
\end{align}
By Claim \ref{claim2:pf_cv_ncv}, we have
\begin{align}\label{eq11:MLE_bound}
 -\langle \cP_{\cT^{\perp}}(R),\Delta_{\Gamma}^{con}\rangle
 \leq  \| \cP_{\cT^{\perp}}(R)\|\|\cP_{\cT^{\perp}}(\Delta_{\Gamma}^{con})\|_{*}
 \leq\left(1-\frac{\eps}{4}\right)\lambda\cdot\|\cP_{\cT^{\perp}}(\Delta_{\Gamma}^{con})\|_{*}.
\end{align}
Combine \eqref{eq10:MLE_bound} and \eqref{eq11:MLE_bound}, we obtain
\begin{align*}
 &C\left(\|\Delta_{\theta}^{con}\|_2^2+\|\Delta_{H}^{con}\|_F^2+\frac{1}{n^2}\|\Delta_{\Gamma}^{con}\|_F^2\right)\notag\\ &\leq  -\nabla_{\theta} L_c({\theta}, {H}, {\Gamma})^{\top} \Delta_{\theta}^{con} -\nabla_{H} L_c({\theta}, {H}, {\Gamma})^{\top} \Delta_{H}^{con} +\|\cP_{\cT}(R)\|_F\|\cP_{\cT}(\Delta_{\Gamma}^{con})\|_F-\frac{\eps}{4}\lambda\|\cP_{\cT^{\perp}}(\Delta_{\Gamma}^{con})\|_{*}\notag\\
 &\leq  -\nabla_{\theta} L_c({\theta}, {H}, {\Gamma})^{\top} \Delta_{\theta}^{con} -\nabla_{H} L_c({\theta}, {H}, {\Gamma})^{\top} \Delta_{H}^{con} +\|\cP_{\cT}(R)\|_F\|\cP_{\cT}(\Delta_{\Gamma}^{con})\|_F\notag\\
  &\leq  -\nabla_{\theta} L_c({\theta}, {H}, {\Gamma})^{\top} \Delta_{\theta}^{con} -\nabla_{H} L_c({\theta}, {H}, {\Gamma})^{\top} \Delta_{H}^{con} +\frac{ 72 \kappa}{\sqrt{\sigma_{\min}}} \|\cP(\nabla f(\theta,H,X,Y))\|_F\|\Delta_{\Gamma}^{con}\|_F\tag{by Claim \ref{claim2:pf_cv_ncv}}\\
&= -\left(\nabla_{\theta} L_c({\theta}, {H}, {\Gamma})-\mean(\nabla_{\theta} L_c({\theta}, {H}, {\Gamma}))\cdot\mathbf{1}\right)^{\top} \Delta_{\theta}^{con} -\nabla_{H} L_c({\theta}, {H}, {\Gamma})^{\top} \Delta_{H}^{con} \notag\\
&\quad+\frac{ 72 \kappa}{\sqrt{\sigma_{\min}}} \|\cP(\nabla f(\theta,H,X,Y))\|_F\|\Delta_{\Gamma}^{con}\|_F\tag{since $\mathbf{1}^T\Delta_{\theta}^{con}=0$}\\
&\leq \|\cP(\nabla f(\theta,H,X,Y))\|_F\|\Delta_{\theta}^{con}\|_F+\|\cP(\nabla f(\theta,H,X,Y))\|_F\|\Delta_{H}^{con}\|_F\notag\\
&\quad+\frac{ 72 \kappa}{\sqrt{\sigma_{\min}}} \|\cP(\nabla f(\theta,H,X,Y))\|_F\|\Delta_{\Gamma}^{con}\|_F\notag\\
&\leq \left(1+\frac{ 72 \kappa n}{\sqrt{\sigma_{\min}}}\right)\|\cP(\nabla f(\theta,H,X,Y))\|_F\cdot\left(\|\Delta_{\theta}^{con}\|_2+\|\Delta_{H}^{con}\|_F+\frac{1}{n}\|\Delta_{\Gamma}^{con}\|_F\right).
\end{align*}
Note that
\begin{align*}
\|\Delta_{\theta}^{con}\|_2^2+\|\Delta_{H}^{con}\|_F^2+\frac{1}{n^2}\|\Delta_{\Gamma}^{con}\|_F^2\geq \frac13 \left(\|\Delta_{\theta}^{con}\|_2+\|\Delta_{H}^{con}\|_F+\frac{1}{n}\|\Delta_{\Gamma}^{con}\|_F\right)^2.
\end{align*}
Thus, we have
\begin{align*}
&\frac{C}{3}\left(\|\Delta_{\theta}^{con}\|_2+\|\Delta_{H}^{con}\|_F+\frac{1}{n}\|\Delta_{\Gamma}^{con}\|_F\right)^2\\
&\leq \left(1+\frac{ 72 \kappa n}{\sqrt{\sigma_{\min}}}\right)\|\cP(\nabla f(\theta,H,X,Y))\|_F\cdot\left(\|\Delta_{\theta}^{con}\|_2+\|\Delta_{H}^{con}\|_F+\frac{1}{n}\|\Delta_{\Gamma}^{con}\|_F\right),
\end{align*}
which implies
\begin{align*}
\|\Delta_{\theta}^{con}\|_2+\|\Delta_{H}^{con}\|_F+\frac{1}{n}\|\Delta_{\Gamma}^{con}\|_F   
\leq \frac{3}{C}\left(1+\frac{ 72 \kappa n}{\sqrt{\sigma_{\min}}}\right)\|\cP(\nabla f(\theta,H,X,Y))\|_F.
\end{align*}
Further by \eqref{ncv:grad}, we obtain
\begin{align*}
\|\Delta_{\theta}^{con}\|_2\lesssim n^{-5},\quad
\|\Delta_{H}^{con}\|_F \lesssim n^{-5},\quad
\|\Delta_{\Gamma}^{con}\|_F\lesssim n^{-4}.
\end{align*}
Consequently, we show that
\begin{align*}
&\|\hat{\theta}^{con}-\theta^*\|_{\infty}\leq \|\Delta_{\theta}^{con}\|_2+\|\theta-\theta^*\|_{\infty}\lesssim c_{41}<c\sqrt{n},\\
&\|\hat{H}^{con}-H^*\|_F\leq \|\Delta_{H}^{con}\|_F+\|H-H^*\|_F\lesssim c_{11}\sqrt{n}<cn,\\
&\|\hat{\Gamma}^{con}-\Gamma^*\|_{\infty}\leq \|\Delta_{\Gamma}^{con}\|_F+\|\Gamma-\Gamma^*\|_{\infty}\lesssim c_{43}\sqrt{\mu\sX\sY r^2 n}<cn
\end{align*}
as long as $n$ is large enough.
In other words, the minimizer of \eqref{obj:con} is in the interior of the constraint. By the convexity of \eqref{obj:con}, we have $(\hat{\theta}^{con}, \hat{H}^{con}, \hat{\Gamma}^{con}) =(\hat{\theta}_c, \hat{H}_c, \hat{\Gamma}_c)$. By the constraints, we finish the proofs.
\end{proof}


With Claim \ref{claim2:pf_cv_ncv} and Claim \ref{claim:MLE_bound} in hand, we are ready to prove Theorem \ref{thm:cv_ncv} in the following.

\begin{proof}[Proof of Theorem \ref{thm:cv_ncv}]
We denote 
\begin{align*}
\Delta_{\theta}:=\hat{\theta}_c-\theta,\ 
\Delta_{H}:=\hat{H}_c-H,\ 
\Delta_{\Gamma}:=\hat{\Gamma}_c-XY^{\top}.
\end{align*}
By the optimality of $(\hat{\theta}_c, \hat{H}_c, \hat{\Gamma}_c)$, we have
\begin{align}\label{eq7:pf_cv_ncv}
L_c(\hat{\theta}_c, \hat{H}_c, \hat{\Gamma}_c)+\lambda\|\hat{\Gamma}_c\|_{*}\leq L_c({\theta}, {H}, {\Gamma})+\lambda\|\Gamma\|_{*}.
\end{align}
By Taylor expansion, we have
\begin{align}\label{eq30:pf_cv_ncv}
&L_c(\hat{\theta}_c, \hat{H}_c, \hat{\Gamma}_c)-L_c({\theta}, {H}, {\Gamma})\notag\\
&=\nabla L_c({\theta}, {H}, {\Gamma})^{\top}
\begin{bmatrix}
\Delta_{\theta}\\
\Delta_{H}\\
\Delta_{\Gamma}
\end{bmatrix}
+\frac12 
\begin{bmatrix}
\Delta_{\theta}\\
\Delta_{H}\\
\Delta_{\Gamma}
\end{bmatrix}^{\top}
\nabla^2 L_c(\tilde{\theta}, \tilde{H}, \tilde{\Gamma})
\begin{bmatrix}
\Delta_{\theta}\\
\Delta_{H}\\
\Delta_{\Gamma}
\end{bmatrix}\notag\\
&=\nabla L_c({\theta}, {H}, {\Gamma})^{\top}
\begin{bmatrix}
\Delta_{\theta}\\
\Delta_{H}\\
\Delta_{\Gamma}
\end{bmatrix}
+\frac12 
\begin{bmatrix}
\Delta_{\theta}\\
\Delta_{H}\\
\Delta_{\Gamma}
\end{bmatrix}^{\top}
\left(\sum_{i\neq j}\frac{e^{ \tilde{P}_{ij}}}{(1+e^{ \tilde{P}_{ij}})^2} 
\begin{bmatrix}
\frac{{e}_i+{e}_j}{\sqrt{n}}\\
{z}_i{z}_j^T\\
\frac{{e}_i{e}_j^T}{n}
\end{bmatrix}^{\otimes 2}\right)
\begin{bmatrix}
\Delta_{\theta}\\
\Delta_{H}\\
\Delta_{\Gamma}
\end{bmatrix}.
\end{align}
Note that for some constant $c''$
\begin{align}\label{ineq30:pf_cv_ncv}
 &\begin{bmatrix}
\Delta_{\theta}\\
\Delta_{H}\\
\Delta_{\Gamma}
\end{bmatrix}^{\top}
\left(\sum_{i\neq j}\frac{e^{ \tilde{P}_{ij}}}{(1+e^{ \tilde{P}_{ij}})^2} 
\begin{bmatrix}
\frac{{e}_i+{e}_j}{\sqrt{n}}\\
{z}_i{z}_j^T\\
\frac{{e}_i{e}_j^T}{n}
\end{bmatrix}^{\otimes 2}\right)
\begin{bmatrix}
\Delta_{\theta}\\
\Delta_{H}\\
\Delta_{\Gamma}
\end{bmatrix}\notag\\
&\geq_{(1)}
 \frac{e^{c'' c_P}}{(1+e^{c'' c_P})^2}
\begin{bmatrix}
\Delta_{\theta}\\
\Delta_{H}\\
\Delta_{\Gamma}
\end{bmatrix}^{\top}
\left(\sum_{i\neq j}
\begin{bmatrix}
\frac{{e}_i+{e}_j}{\sqrt{n}}\\
{z}_i{z}_j^T\\
\frac{{e}_i{e}_j^T}{n}
\end{bmatrix}^{\otimes 2}\right)
\begin{bmatrix}
\Delta_{\theta}\\
\Delta_{H}\\
\Delta_{\Gamma}
\end{bmatrix}\notag\\
&= \frac{e^{c'' c_P}}{(1+e^{c'' c_P})^2}\begin{bmatrix}
\Delta_{\theta}\\
\Delta_{H}\\
\frac1n \Delta_{\Gamma}
\end{bmatrix}^{\top}
\left(\sum_{i\neq j}
\begin{bmatrix}
\frac{{e}_i+{e}_j}{\sqrt{n}}\\
{z}_i{z}_j^T\\
{{e}_i{e}_j^T}
\end{bmatrix}^{\otimes 2}\right)
\begin{bmatrix}
\Delta_{\theta}\\
\Delta_{H}\\
\frac1n \Delta_{\Gamma}
\end{bmatrix}\notag\\
&\geq  \frac{\sl e^{c'' c_P}}{(1+e^{c'' c_P})^2}\left( \|\Delta_{\theta}\|_2^2+\|\Delta_{H}\|_F^2+\frac{1}{n^2}\|\Delta_{\Gamma}\|_F^2\right),
\end{align}
where the last inequality follows Assumption \ref{assumption:eigenvalues}.
Here (1) follows from the following argument: note that
\begin{align*}
|P_{ij}|
&:=\left|\frac{\theta_i+\theta_j}{\sqrt{n}}+{z}_i^\top{H}{z}_j + \frac{(XY^{\top})_{ij}}{n}\right|\\
&\leq |P_{ij}^{*}|+\frac{2}{\sqrt{n}}\|\theta-\theta^*\|_{\infty}+\frac{\sz}{n}\|H-H^*\|_2+\frac{1}{n}\|XY^{\top}-\Gamma^*\|_{\infty}.
\end{align*}
Further, by \eqref{ncv:est}, we have
\begin{align*}
&\|XY^T-\Gamma^*\|_{\infty}\\
&=\|(X-X^*)Y^T+X^{*}(Y-Y^*)^T\|_{\infty}\\
&\leq \|X-X^*\|_{2,\infty}\|Y\|_{2,\infty}+\|X^{*}\|_{2,\infty}\|Y-Y^*\|_{2,\infty} \tag{Cauchy}\\
&\lesssim c_{43}\sqrt{\mu \sX\sY r^2 n}.
\end{align*}
Thus, by \eqref{ncv:est} and Assumption \ref{assumption:scales}, as long as $n$ is large enough, we have $|P_{ij}|\leq 2c_P$.
Similarly, we have
\begin{align*}
|(\hat{P}_c)_{ij}|
&:=\left|\frac{(\hat{\theta}_c)_i+(\hat{\theta}_c)_j}{\sqrt{n}}+{z}_i^\top{\hat{H}_c}{z}_j + \frac{(\hat{\Gamma}_c)_{ij}}{n}\right|\\
&\leq |P_{ij}^{*}|+\frac{2}{\sqrt{n}}\|\hat{\theta}_c-\theta^*\|_{\infty}+\frac{\sz}{n}\|\hat{H}_c-H^*\|_2+\frac{1}{n}\|\hat{\Gamma}_c-\Gamma^*\|_{\infty}\\
&\leq |P_{ij}^{*}|+\frac{2}{\sqrt{n}}\|\hat{\theta}_c-\theta^*\|_{\infty}+\frac{\sz}{n}\|\hat{H}_c-H^*\|_F+\frac{1}{n}\|\hat{\Gamma}_c-\Gamma^*\|_{\infty}.
\end{align*}
Further by Claim \ref{claim:MLE_bound}, we have $|(\hat{P}_c)_{ij}|\lesssim c_P$.
Since $\tilde{P}_{ij}$ lies between $P_{ij}$ and $(\hat{P}_c)_{ij}$, we conclude that $|\tilde{P}_{ij}|\lesssim c_P$. Consequently, we have $\frac{e^{ \tilde{P}_{ij}}}{(1+e^{ \tilde{P}_{ij}})^2} \geq  \frac{e^{c'' c_P}}{(1+e^{c'' c_P})^2}$ for some constant $c''$, which implies (1).

Combine \eqref{eq30:pf_cv_ncv} and \eqref{ineq30:pf_cv_ncv}, we have
\begin{align}\label{eq8:pf_cv_ncv}
L_c(\hat{\theta}_c, \hat{H}_c, \hat{\Gamma}_c)-L_c({\theta}, {H}, {\Gamma})
\geq \nabla L_c({\theta}, {H}, {\Gamma})^{\top}
\begin{bmatrix}
\Delta_{\theta}\\
\Delta_{H}\\
\Delta_{\Gamma}
\end{bmatrix}
+C'\left(\|\Delta_{\theta}\|_2^2+\|\Delta_{H}\|_F^2+\frac{1}{n^2}\|\Delta_{\Gamma}\|_F^2\right)
\end{align}
for $C':= \frac{\sl e^{c'' c_P}}{2(1+e^{c'' c_P})^2}$. By \eqref{eq7:pf_cv_ncv} and \eqref{eq8:pf_cv_ncv}, we obtain
\begin{align}\label{eq9:pf_cv_ncv}
 C'\left(\|\Delta_{\theta}\|_2^2+\|\Delta_{H}\|_F^2+\frac{1}{n^2}\|\Delta_{\Gamma}\|_F^2\right)
 \leq -\nabla L_c({\theta}, {H}, {\Gamma})^{\top}
\begin{bmatrix}
\Delta_{\theta}\\
\Delta_{H}\\
\Delta_{\Gamma}
\end{bmatrix}+\lambda\|\Gamma\|_{*}-\lambda\|\hat{\Gamma}_c\|_{*}.
\end{align}
In addition, by the convexity of $\|\cdot\|_{*}$, we have
\begin{align*}
\|\hat{\Gamma}_c\|_{*}-\|\Gamma\|_{*}=\|\Gamma+\Delta_{\Gamma}\|_{*}-\|\Gamma\|_{*}\geq \langle UV^{\top}+W,\Delta_{\Gamma}\rangle
\end{align*}
for any $W\in\cT^{\perp}$ obeying $\|W\|\leq 1$. In the following, we pick $W$ such that $\langle W, \Delta_{\Gamma}\rangle=\|\cP_{\cT^{\perp}}(\Delta_{\Gamma})\|_{*}$. We then obtain $\|\hat{\Gamma}_c\|_{*}-\|\Gamma\|_{*}\geq  \langle UV^{\top},\Delta_{\Gamma}\rangle+\|\cP_{\cT^{\perp}}(\Delta_{\Gamma})\|_{*}$, and consequently, by \eqref{eq9:pf_cv_ncv}, we have
\begin{align*}
C'\left(\|\Delta_{\theta}\|_2^2+\|\Delta_{H}\|_F^2+\frac{1}{n^2}\|\Delta_{\Gamma}\|_F^2\right)
 \leq -\nabla L_c({\theta}, {H}, {\Gamma})^{\top}
\begin{bmatrix}
\Delta_{\theta}\\
\Delta_{H}\\
\Delta_{\Gamma}
\end{bmatrix}-\lambda\langle UV^{\top},\Delta_{\Gamma}\rangle-\lambda\|\cP_{\cT^{\perp}}(\Delta_{\Gamma})\|_{*}.
\end{align*}
Recall the definition of $R$ in \eqref{eq:R}, we further have
\begin{align}\label{eq10:pf_cv_ncv}
&C'\left(\|\Delta_{\theta}\|_2^2+\|\Delta_{H}\|_F^2+\frac{1}{n^2}\|\Delta_{\Gamma}\|_F^2\right)\notag\\
& \leq  -\nabla_{\theta} L_c({\theta}, {H}, {\Gamma})^{\top} \Delta_{\theta} -\nabla_{H} L_c({\theta}, {H}, {\Gamma})^{\top} \Delta_{H}-\langle R,\Delta_{\Gamma}\rangle-\lambda\|\cP_{\cT^{\perp}}(\Delta_{\Gamma})\|_{*}\notag\\
&=  -\nabla_{\theta} L_c({\theta}, {H}, {\Gamma})^{\top} \Delta_{\theta} -\nabla_{H} L_c({\theta}, {H}, {\Gamma})^{\top} \Delta_{H}-\langle \cP_{\cT}(R),\Delta_{\Gamma}\rangle-\langle \cP_{\cT^{\perp}}(R),\Delta_{\Gamma}\rangle-\lambda\|\cP_{\cT^{\perp}}(\Delta_{\Gamma})\|_{*}\notag\\
&\leq  -\nabla_{\theta} L_c({\theta}, {H}, {\Gamma})^{\top} \Delta_{\theta} -\nabla_{H} L_c({\theta}, {H}, {\Gamma})^{\top} \Delta_{H}\notag\\
&\quad +\|\cP_{\cT}(R)\|_F\|\cP_{\cT}(\Delta_{\Gamma})\|_F-\langle \cP_{\cT^{\perp}}(R),\Delta_{\Gamma}\rangle-\lambda\|\cP_{\cT^{\perp}}(\Delta_{\Gamma})\|_{*}.
\end{align}
By Claim \ref{claim2:pf_cv_ncv}, we have
\begin{align}\label{eq11:pf_cv_ncv}
 -\langle \cP_{\cT^{\perp}}(R),\Delta_{\Gamma}\rangle
 \leq  \| \cP_{\cT^{\perp}}(R)\|\|\cP_{\cT^{\perp}}(\Delta_{\Gamma})\|_{*}
 \leq\left(1-\frac{\eps}{4}\right)\lambda\cdot\|\cP_{\cT^{\perp}}(\Delta_{\Gamma})\|_{*}
\end{align}
Combine \eqref{eq10:pf_cv_ncv} and \eqref{eq11:pf_cv_ncv}, we obtain
\begin{align*}
 &C'\left(\|\Delta_{\theta}\|_2^2+\|\Delta_{H}\|_F^2+\frac{1}{n^2}\|\Delta_{\Gamma}\|_F^2\right)\notag\\ &\leq  -\nabla_{\theta} L_c({\theta}, {H}, {\Gamma})^{\top} \Delta_{\theta} -\nabla_{H} L_c({\theta}, {H}, {\Gamma})^{\top} \Delta_{H} +\|\cP_{\cT}(R)\|_F\|\cP_{\cT}(\Delta_{\Gamma})\|_F-\frac{\eps}{4}\lambda\|\cP_{\cT^{\perp}}(\Delta_{\Gamma})\|_{*}\notag\\
 &\leq  -\nabla_{\theta} L_c({\theta}, {H}, {\Gamma})^{\top} \Delta_{\theta} -\nabla_{H} L_c({\theta}, {H}, {\Gamma})^{\top} \Delta_{H} +\|\cP_{\cT}(R)\|_F\|\cP_{\cT}(\Delta_{\Gamma})\|_F\notag\\
  &\leq  -\nabla_{\theta} L_c({\theta}, {H}, {\Gamma})^{\top} \Delta_{\theta} -\nabla_{H} L_c({\theta}, {H}, {\Gamma})^{\top} \Delta_{H} +\frac{ 72 \kappa}{\sqrt{\sigma_{\min}}} \|\cP(\nabla f(\theta,H,X,Y))\|_F\|\Delta_{\Gamma}\|_F\tag{by Claim \ref{claim2:pf_cv_ncv}}\\
&= -\left(\nabla_{\theta} L_c({\theta}, {H}, {\Gamma})-\mean(\nabla_{\theta} L_c({\theta}, {H}, {\Gamma}))\cdot\mathbf{1}\right)^{\top} \Delta_{\theta} -\nabla_{H} L_c({\theta}, {H}, {\Gamma})^{\top} \Delta_{H} \notag\\
&\quad+\frac{ 72 \kappa}{\sqrt{\sigma_{\min}}} \|\cP(\nabla f(\theta,H,X,Y))\|_F\|\Delta_{\Gamma}\|_F\tag{since $\mathbf{1}^T\Delta_{\theta}=0$}\\
&\leq \|\cP(\nabla f(\theta,H,X,Y))\|_F\|\Delta_{\theta}\|_F+\|\cP(\nabla f(\theta,H,X,Y))\|_F\|\Delta_{H}\|_F\notag\\
&\quad+\frac{ 72 \kappa}{\sqrt{\sigma_{\min}}} \|\cP(\nabla f(\theta,H,X,Y))\|_F\|\Delta_{\Gamma}\|_F\notag\\
&\leq \left(1+\frac{ 72 \kappa n}{\sqrt{\sigma_{\min}}}\right)\|\cP(\nabla f(\theta,H,X,Y))\|_F\cdot\left(\|\Delta_{\theta}\|_2+\|\Delta_{H}\|_F+\frac{1}{n}\|\Delta_{\Gamma}\|_F\right).
\end{align*}
Note that
\begin{align*}
\|\Delta_{\theta}\|_2^2+\|\Delta_{H}\|_F^2+\frac{1}{n^2}\|\Delta_{\Gamma}\|_F^2\geq \frac13 \left(\|\Delta_{\theta}\|_2+\|\Delta_{H}\|_F+\frac{1}{n}\|\Delta_{\Gamma}\|_F\right)^2.
\end{align*}
Thus, we have
\begin{align*}
&\frac{C'}{3}\left(\|\Delta_{\theta}\|_2+\|\Delta_{H}\|_F+\frac{1}{n}\|\Delta_{\Gamma}\|_F\right)^2\\
&\leq \left(1+\frac{ 72 \kappa n}{\sqrt{\sigma_{\min}}}\right)\|\cP(\nabla f(\theta,H,X,Y))\|_F\cdot\left(\|\Delta_{\theta}\|_2+\|\Delta_{H}\|_F+\frac{1}{n}\|\Delta_{\Gamma}\|_F\right),
\end{align*}
which implies
\begin{align*}
\|\Delta_{\theta}\|_2+\|\Delta_{H}\|_F+\frac{1}{n}\|\Delta_{\Gamma}\|_F   
\leq \frac{3}{C'}\left(1+\frac{ 72 \kappa n}{\sqrt{\sigma_{\min}}}\right)\|\cP(\nabla f(\theta,H,X,Y))\|_F.
\end{align*}


\end{proof}









\subsection{Proofs of Theorem \ref{thm:cv_est}}\label{pf:cor_cv_ncv}
Note that $\|\cP(\nabla f(\hat{\theta},\hat{H},\hat{X},\hat{Y}))\|_F\lesssim n^{-5}$.
By Theorem \ref{thm:cv_ncv}, Lemma \ref{lem:ncv1} and Lemma \ref{lem:ncv4}, we then have
\begin{align*}
&\|\hat{\theta}_c-\theta^*\|_2\lesssim \|\hat{\theta}-\theta^*\|_2\lesssim c_{11}\sqrt{n}\\
&\|\hat{\theta}_c-\theta^*\|_{\infty}\lesssim \|\hat{\theta}-\theta^*\|_{\infty}\lesssim c_{41}\\
&\|\hat{H}_c-H^*\|_F\lesssim \|\hat{H}-H^*\|_F\lesssim c_{11}\sqrt{n}.
\end{align*}
Note that by Lemma \ref{lem:ncv1}, we have
\begin{align*}
\|\hat{X}\hat{Y}^{\top}-\Gamma^{*}\|_F\leq 
\|\hat{X}-{X}^{*}\|_F\|\hat{Y}\|+\|\hat{Y}-{Y}^{*}\|_F\|{X}^{*}\|
\lesssim \sqrt{\sigma_{\max}n}c_{11}.
\end{align*}
By Lemma \ref{lem:ncv4}, we have
\begin{align*}
\|\hat{X}\hat{Y}^{\top}-\Gamma^{*}\|_{\infty}\leq 
\|\hat{X}-{X}^{*}\|_{2,\infty}\|\hat{Y}\|_{2,\infty}+\|\hat{Y}-{Y}^{*}\|_{2,\infty}\|{X}^{*}\|_{2,\infty}
\lesssim \sqrt{\frac{\mu r\sigma_{\max}}{n}}c_{43}.
\end{align*}
Further by Theorem \ref{thm:cv_ncv}, we have
\begin{align*}
&\|\hat{\Gamma}_c-\Gamma^{*}\|_{F}\lesssim \|\hat{X}\hat{Y}^{\top}-\Gamma^{*}\|_F\lesssim \sqrt{\sigma_{\max}n}c_{11}\\
&\|\hat{\Gamma}_c-\Gamma^{*}\|_{\infty}\lesssim \|\hat{X}\hat{Y}^{\top}-\Gamma^{*}\|_{\infty}\lesssim \sqrt{\frac{\mu r\sigma_{\max}}{n}}c_{43}.
\end{align*}





\subsection{Proofs of Theorem \ref{thm:mem_est}}\label{pf:thm_mem_est}

We first prove the following lemma.
\begin{lemma}\label{lem:U_2inf}
It holds that
\begin{align*}
    \min_{R\in\cO^{r\times r}}
    \|\hat{U}_c R-U^*\|_{2,\infty}\lesssim\frac{1}{\sqrt{\sigma_{\min}}}c_{43}+\frac{\sqrt{\kappa\mu\sX\sY r^2 }}{\sigma_{\min}}c_{14}n.
\end{align*}
\end{lemma}
\begin{proof}[Proof of Lemma \ref{lem:U_2inf}]
Let $\hat{U}\hat{\Sigma}\hat{V}^{\top}$ be the SVD of $\hat{X}\hat{Y}^{\top}$, where $\hat{X},\hat{Y}$ are the nonconvex estimators given in Section \ref{sec:nonconvex_debias}.
By Weyl’s inequality and the proof of Theorem \ref{thm:cv_est}, we have
\begin{align*}
|\sigma_{\min}(\hat{\Gamma})-\sigma_{\min}|\leq \|\hat{\Gamma}-{\Gamma}^*\|\lesssim \sqrt{\sigma_{\max}n}c_{14},
\end{align*}
which implies $\sigma_{\min}(\hat{\Gamma})\geq \sigma_{\min}/2$. By Davis-Kahan Theorem, we have
\begin{align*}
\min_{R\in\cO^{r\times r}}\|\hat{U}_c R-\hat{U}\|
&\leq \frac{2}{\sigma_{\min}(\hat{\Gamma})}\|\hat{\Gamma}_c -\hat{\Gamma}\|\\
&\leq \frac{4}{\sigma_{\min}}\|\hat{\Gamma}_c -\hat{\Gamma}\|_F\\
&\lesssim_{(1)}\frac{1}{\sigma_{\min}}\frac{(1+e^{c c_P})^2}{\sl e^{c c_P}}\left(1+\frac{ 72 \kappa n}{\sqrt{\sigma_{\min}}}\right)n^{-4}\\
&\lesssim n^{-5},
\end{align*}
where (1) follows from Theorem \ref{thm:cv_ncv} and \eqref{ncv:grad}.
We denote $\hat{R}_c:=\hat{O}_c\hat{R}$, where
\begin{align*}
\hat{O}_c:=\argmin_{R\in\cO^{r\times r}}\|\hat{U}_c R-\hat{U}\|,\quad
\hat{R}:=\argmin_{R\in\cO^{r\times r}}\|\hat{U} R-{U}^*\|.
\end{align*}
It then holds that
\begin{align}\label{ineq1:pf_mem}
&\min_{R\in\cO^{r\times r}}
\|\hat{U}_c R-U^*\|_{2,\infty}\notag\\
&\leq 
\|\hat{U}_c \hat{R}_c-U^*\|_{2,\infty}\notag\\
&\leq 
\|\hat{U}_c \hat{R}_c-\hat{U}\hat{R}\|_{2,\infty}+
\|\hat{U}\hat{R}-U^*\|_{2,\infty}\notag\\
&\leq \|\hat{U}_c \hat{O}_c\hat{R}-\hat{U}\hat{R}\|+
\|\hat{U}\hat{R}-U^*\|_{2,\infty}\notag\\
&\leq n^{-5}+\|\hat{U}\hat{R}-U^*\|_{2,\infty}.
\end{align}
Thus, it remains to bound $\|\hat{U}\hat{R}-U^*\|_{2,\infty}$ in the following.
By Claim \ref{claim1:pf_cv_ncv}, there exists an invertible matrix $Q$ such that $\hat{X}=\hat{U}\hat{\Sigma}^{\frac{1}{2}}Q$ and \eqref{ineq1:pf_cv_ncv} holds. By the definition of $X^{*}$, we have $X^*=U^*\Sigma^{* \frac{1}{2}}$. Thus, we have
\begin{align}\label{eq1:pf_mem}
&\hat{U}=  \hat{X}(\hat{\Sigma}^{\frac{1}{2}}Q)^{-1},\quad \hat{U}^{\top}\hat{X}=\hat{\Sigma}^{\frac{1}{2}}Q\notag\\
& U^*=X^*(\Sigma^{* \frac{1}{2}})^{-1},\quad U^{*\top}X^*=\Sigma^{* \frac{1}{2}}.
\end{align}
It then holds that
\begin{align}\label{ineq2:pf_mem}
&\|\hat{U}\hat{R}-U^*\|_{2,\infty}\notag\\
&=\|\hat{X}(\hat{\Sigma}^{\frac{1}{2}}Q)^{-1}\hat{R}-X^*(\Sigma^{* \frac{1}{2}})^{-1}\|_{2,\infty}\notag\\
&\leq \|(\hat{X}-X^*)(\Sigma^{* \frac{1}{2}})^{-1}\|_{2,\infty}+\|\hat{X}(Q^{-1}\hat{\Sigma}^{-\frac{1}{2}}\hat{R}-\Sigma^{* -\frac{1}{2}})\|_{2,\infty}\notag\\
&\leq \|\Sigma^{* -\frac{1}{2}}\|\|\hat{X}-X^*\|_{2,\infty}+\|Q^{-1}\hat{\Sigma}^{-\frac{1}{2}}\hat{R}-\Sigma^{* -\frac{1}{2}}\|\|\hat{X}\|_{2,\infty}\notag\\
&\leq \frac{1}{\sqrt{\sigma_{\min}}}c_{43}+2\|Q^{-1}\hat{\Sigma}^{-\frac{1}{2}}\hat{R}-\Sigma^{* -\frac{1}{2}}\|\sqrt{\mu\sX\sY r^2 n},
\end{align}
where the last inequality follows from \eqref{ncv:est} and the fact that
\begin{align*}
\|\hat{X}\|_{2,\infty}\leq \|\hat{X}-X^*\|_{2,\infty}+\|{X}^*\|_{2,\infty} \leq 2   \|{X}^*\|_{2,\infty}
\leq 2\sqrt{\mu\sX\sY r^2 n}.
\end{align*}
Note that
\begin{align*}
&\|Q^{-1}\hat{\Sigma}^{-\frac{1}{2}}\hat{R}-\Sigma^{* -\frac{1}{2}}\|\\
&=\|\Sigma^{* -\frac{1}{2}}(\hat{R}^{\top} \hat{\Sigma}^{\frac{1}{2}}Q-\Sigma^{* \frac{1}{2}})Q^{-1}\hat{\Sigma}^{-\frac{1}{2}}\hat{R}\|\\
&\leq \|\Sigma^{* -\frac{1}{2}}\| \|\hat{R}^{\top} \hat{\Sigma}^{\frac{1}{2}}Q-\Sigma^{* \frac{1}{2}}\| \|Q^{-1}\hat{\Sigma}^{-\frac{1}{2}}\hat{R}\|\\
&\leq \|\Sigma^{* -\frac{1}{2}}\| \|\hat{\Sigma}^{ -\frac{1}{2}}\|\|Q^{-1}\|\|\hat{R}^{\top} \hat{\Sigma}^{\frac{1}{2}}Q-\Sigma^{* \frac{1}{2}}\|.
\end{align*}
Since $Q$ satisfies \eqref{ineq1:pf_cv_ncv}, we have $\|Q^{-1}\|\leq 2$. Moreover, we have show that $\|\hat{\Sigma}^{-\frac{1}{2}}\|=\sqrt{1/\sigma_{\min}(\hat{\Gamma})}\leq \sqrt{2/\sigma_{\min}}$.
Thus, we obtain
\begin{align}\label{ineq3:pf_mem}
\|Q^{-1}\hat{\Sigma}^{-\frac{1}{2}}\hat{R}-\Sigma^{* -\frac{1}{2}}\|\leq \frac{4}{\sigma_{\min}}\|\hat{R}^{\top} \hat{\Sigma}^{\frac{1}{2}}Q-\Sigma^{* \frac{1}{2}}\|.
\end{align}
By \eqref{eq1:pf_mem}, we have
\begin{align*}
&\|\hat{R}^{\top} \hat{\Sigma}^{\frac{1}{2}}Q-\Sigma^{* \frac{1}{2}}\|\\
&=\|\hat{R}^{\top}\hat{U}^{\top}\hat{X}-{U}^{* \top}{X}^{*}\|\\
&\leq \|(\hat{R}^{\top}\hat{U}^{\top}-{U}^{* \top})\hat{X}\|+\|{U}^{* \top}(\hat{X}-{X}^{*})\|\\
&\leq \|\hat{X}\|\|\hat{U}\hat{R}-U^{*}\|+\|\hat{X}-{X}^{*}\|\\
&\leq 2\sqrt{\sigma_{\max}}\|\hat{U}\hat{R}-U^{*}\|+c_{14}\sqrt{n},
\end{align*}
where the last inequality follows from Lemma \ref{lem:ncv1} and the fact that
\begin{align*}
\|\hat{X}\|\leq \|\hat{X}-X^*\|+\|{X}^*\|\leq 2\|{X}^*\|=2\sqrt{\sigma_{\max}}.
\end{align*}
By Davis-Kahan Theorem and the definition of $\hat{R}$, we have
\begin{align*}
 \|\hat{U}\hat{R}-U^{*}\|=\min_{R\in\cO^{r\times r}}\|\hat{U}R-U^{*}\|  \leq \frac{2}{\sqrt{\sigma_{\min}} }\|\hat{X}-X^{*}\|
 \leq 2c_{14}\sqrt{\frac{n}{\sigma_{\min}}}.
\end{align*}
Thus, we have
\begin{align}\label{ineq4:pf_mem}
 \|\hat{R}^{\top} \hat{\Sigma}^{\frac{1}{2}}Q-\Sigma^{* \frac{1}{2}}\|\leq 4c_{14}\sqrt{\kappa n} +c_{14}\sqrt{n}\leq   5c_{14}\sqrt{\kappa n} .
\end{align}
Combine \eqref{ineq3:pf_mem} and \eqref{ineq4:pf_mem}, we have
\begin{align}\label{ineq5:pf_mem}
 \|Q^{-1}\hat{\Sigma}^{-\frac{1}{2}}\hat{R}-\Sigma^{* -\frac{1}{2}}\|\leq \frac{20}{\sigma_{\min}} c_{14}\sqrt{\kappa n} .  
\end{align}
Further by \eqref{ineq2:pf_mem}, we have
\begin{align*}
&\|\hat{U}\hat{R}-U^*\|_{2,\infty}\notag\\
&\leq \frac{1}{\sqrt{\sigma_{\min}}}c_{43}+\frac{40}{\sigma_{\min}}\sqrt{\kappa\mu\sX\sY r^2 }c_{14}n.
\end{align*}
Plug the above inequality into \eqref{ineq1:pf_mem}, we obtain
\begin{align*}
&\min_{R\in\cO^{r\times r}}
\|\hat{U}_c R-U^*\|_{2,\infty}\notag\\
&\leq n^{-5}+    \frac{1}{\sqrt{\sigma_{\min}}}c_{43}+\frac{40}{\sigma_{\min}}\sqrt{\kappa\mu\sX\sY r^2 }c_{14}n\notag\\
&\lesssim \frac{1}{\sqrt{\sigma_{\min}}}c_{43}+\frac{\sqrt{\kappa\mu\sX\sY r^2 }}{\sigma_{\min}}c_{14}n.
\end{align*}
We then finish the proof of Lemma \ref{lem:U_2inf}.
\end{proof}

Let
\begin{align*}
H:=\argmin_{R\in\cO^{r\times r}}\max_{1\leq i\leq n}\|R\hat{u}_i-u^{*}_i\|.
\end{align*}
By Lemma \ref{lem:U_2inf}, we have
\begin{align}\label{prop1:pf_mem}
  \max_{1\leq i\leq n}\|H\hat{u}_i-u^{*}_i\|  =\min_{R\in\cO^{r\times r}}
\|\hat{U}_c R-U^*\|_{2,\infty}\lesssim \frac{1}{\sqrt{\sigma_{\min}}}c_{43}+\frac{\sqrt{\kappa\mu\sX\sY r^2 }}{\sigma_{\min}}c_{14}n.
\end{align}
Recall the definition of efficient vertex-hunting algorithms, we have
\begin{align}\label{prop2:pf_mem}
 \max_{1\leq \ell \leq r}\|H\hat{v}_{\ell}-v_{\ell}\|\lesssim  \max_{1\leq i\leq n}\|H\hat{u}_i-u^{*}_i\| \lesssim \frac{1}{\sqrt{\sigma_{\min}}}c_{43}+\frac{\sqrt{\kappa\mu\sX\sY r^2 }}{\sigma_{\min}}c_{14}n.
\end{align}
We then prove Theorem \ref{thm:mem_est} in the following.
\begin{proof}[Proof of Theorem \ref{thm:mem_est}]
Note that
\begin{align*}
\underbrace{
\begin{bmatrix}
v_1,\ldots,v_r
\end{bmatrix}}_{=:Q}\pi^{*}_i=u^{*}_i,\quad
\underbrace{\begin{bmatrix}
H\hat{v}_1,\ldots,H\hat{v}_r
\end{bmatrix}}_{=:\hat{Q}}\hat{\pi}_i=H\hat{u}_i.
\end{align*}
We have the following claim.
\begin{claim}\label{claim1:pf_mem}
Under Assumption \ref{assumption:mem_est}, it holds that \begin{align*}
\|Q\|\lesssim \sqrt{\frac{r}{n}}\text{ and }
\|Q^{-1}\|\lesssim \sqrt{\frac{n}{r}}.
\end{align*}
\end{claim}
\begin{proof}[Proof of Claim \ref{claim1:pf_mem}]
Note that $U^*=\Pi^* B=\Pi^* Q^{\top}$. Thus, it holds that
\begin{align*}
I_r=U^{*\top}U^*=Q\Pi^{*\top}\Pi^*Q^{\top}=\frac{n}{r}QGQ^{\top}.
\end{align*}
This further implies that
\begin{align*}
Q^{\top}Q=\frac{n}{r}(Q^{\top}Q)G(Q^{\top}Q).
\end{align*}
Since $Q^{\top}Q$ is invertible, we have
\begin{align*}
Q^{\top}Q=\frac{r}{n}G^{-1}\text{ and }
Q^{-1}Q^{-\top}=(Q^{\top}Q)^{-1}=\frac{n}{r}G.
\end{align*}
By Assumption \ref{assumption:mem_est}, it then holds that
\begin{align*}
\|Q\|\leq \sqrt{\frac{r}{n}\|G^{-1}\|}\lesssim \sqrt{\frac{r}{n}}\text{ and }
\|Q^{-1}\|\leq \sqrt{\frac{n}{r}\|G\|}\lesssim \sqrt{\frac{n}{r}}.
\end{align*}
We then finish the proof of Claim \ref{claim1:pf_mem}.
\end{proof}
By Claim \ref{claim1:pf_mem}, we have $\sigma_{\min}(Q)\gtrsim \sqrt{r/n}$.
By Weyl's inequality, we have
\begin{align*}
|\sigma_{\min}(\hat{Q})-\sigma_{\min}(Q)|
&\leq \|\hat{Q}-Q\|\\
&\leq \|\hat{Q}-Q\|_F\\
&\leq \sqrt{r}\max_{1\leq \ell \leq r}\|H\hat{v}_{\ell}-v_{\ell}\|\\
&\lesssim \sqrt{r}\left(\frac{1}{\sqrt{\sigma_{\min}}}c_{43}+\frac{\sqrt{\kappa\mu\sX\sY r^2 }}{\sigma_{\min}}c_{14}n\right)\tag{by \eqref{prop2:pf_mem}}\\
&\ll \sqrt{\frac{r}{n}}.
\end{align*}
Thus, it holds that
\begin{align}\label{ineq6:pf_mem}
\|\hat{Q}^{-1}\|=\frac{1}{\sigma_{\min}(\hat{Q})}\leq \frac{2}{\sigma_{\min}({Q})}\lesssim \sqrt{\frac{n}{r}}.
\end{align}
Note that
\begin{align*}
\hat{\pi}_i-\pi^{*}_i
&=\hat{Q}^{-1}H\hat{u}_i-Q^{-1}u^{*}_i\\
&=\hat{Q}^{-1}(H\hat{u}_i-u^{*}_i)-\hat{Q}^{-1}(\hat{Q}-Q)Q^{-1}u^{*}_i\\
&=\hat{Q}^{-1}(H\hat{u}_i-u^{*}_i)-\hat{Q}^{-1}(\hat{Q}-Q)\pi^{*}_i.
\end{align*}
Consequently, we have
\begin{align*}
\|\hat{\pi}_i-\pi^{*}_i\|
&\leq \|\hat{Q}^{-1}\|\left(\|H\hat{u}_i-u^{*}_i\|+\|(\hat{Q}-Q)\pi^{*}_i\|\right)\\
&\lesssim \sqrt{\frac{n}{r}}\left(\|H\hat{u}_i-u^{*}_i\|+\|(\hat{Q}-Q)\pi^{*}_i\|\right),
\end{align*}
where the last inequality follows from \eqref{ineq6:pf_mem}.
Note that
\begin{align*}
\|(\hat{Q}-Q)\pi^{*}_i\|
&=\left\|\sum^r_{\ell=1}\pi^{*}_i(\ell)(H\hat{v}_{\ell}-v_{\ell})\right\|\\
&\leq \sum^r_{\ell=1}\pi^{*}_i(\ell)\|H\hat{v}_{\ell}-v_{\ell}\|\\
&\leq \max_{1\leq\ell r}\|H\hat{v}_{\ell}-v_{\ell}\|,
\end{align*}
where the last inequality follows from the fact that $\sum^r_{\ell=1}\pi^{*}_i(\ell)=1$. Thus, we obtain
\begin{align*}
\|\hat{\pi}_i-\pi^{*}_i\|\lesssim    \sqrt{\frac{n}{r}}\left(\|H\hat{u}_i-u^{*}_i\|+\max_{1\leq\ell r}\|H\hat{v}_{\ell}-v_{\ell}\|\right),
\end{align*}
which then gives
\begin{align*}
\max_{1\leq i\leq n}\|\hat{\pi}_i-\pi^{*}_i\|\lesssim    \sqrt{\frac{n}{r}}\left(\max_{1\leq i\leq n}\|H\hat{u}_i-u^{*}_i\|+\max_{1\leq\ell r}\|H\hat{v}_{\ell}-v_{\ell}\|\right).
\end{align*}
Further by \eqref{prop1:pf_mem} and \eqref{prop2:pf_mem}, we obtain
\begin{align*}
 \max_{1\leq i\leq n}\|\hat{\pi}_i-\pi^{*}_i\|
 &\lesssim    \sqrt{\frac{n}{r}}\left(\frac{1}{\sqrt{\sigma_{\min}}}c_{43}+\frac{\sqrt{\kappa\mu\sX\sY r^2 }}{\sigma_{\min}}c_{14}n\right) \\
 &= \sqrt{\frac{1}{nr}}\left(\frac{n}{\sqrt{\sigma_{\min}}}c_{43}+\frac{n^2}{\sigma_{\min}}\sqrt{\kappa\mu\sX\sY r^2 }c_{14}\right).
\end{align*}

\end{proof}



























==> pf_nonconvex_iterates_v1.tex <==

\section{Proofs of Section \ref{sec:nonconvex_iterates}}\label{sec:pf_nonconvex_iterates}



We define
\begin{align*}
f_{\diff}(X,Y):=\frac{c_{\aug}}{n^2}\|X^TX-Y^TY\|^2_{F}.
\end{align*}
Thus, we have $f_{\aug}(\theta,H,X,Y)=f(\theta,H,X,Y)+f_{\diff}(X,Y)$.
Note that for any $M$, $F$, and $R\in\cO^{r\times r}$, we have
\begin{align*}
f(M,FR)=f(M,F),\ \nabla_M f(M,FR)=\nabla_M f(M,F), \ \nabla_M f(M,F)R=\nabla_M f(M,FR), 
\end{align*}
which will be used in the following proofs.
We first present the following lemmas, which will be constantly used in the proofs.
\begin{lemma}\label{lem:gradient_norm}
Let $M^*, F^*$ be the ground truth parameters and $\lambda\gtrsim\sqrt{\frac{\log n}{n}}$. Under Assumption \ref{assumption:scales}, it holds with probability at least $1-n^{-10}$ that
\begin{align*}
&\|\nabla_{\theta} f(M^*,F^*)\|_2\lesssim\sqrt{n\log n},\quad
\|\nabla_{H} f(M^*,F^*)\|_F\lesssim\sz\sqrt{p\log n},\\
&\|\nabla_{F} f(M^*,F^*)\|_F\lesssim \lambda   \left(\|X^{*}\|_F+\|Y^{*}\|_F\right).
\end{align*}
\end{lemma}
\begin{proof}[Proof of Lemma \ref{lem:gradient_norm}]
In the following, we will bound $\|\nabla_{\theta} f(M^*,F^*)\|_2$, $\|\nabla_{H} f(M^*,F^*)\|_F$ and $\|\nabla_{F} f(M^*,F^*)\|_F$, respectively.
Note that
\begin{align*}
\nabla_{\theta} f(M^*,F^*)
&=\nabla_{\theta} L(M^*,F^*)\\
&= \frac{1}{\sqrt{n}}\sum_{i\neq j}\left(\frac{e^{P_{ij}^*}}{1+e^{P_{ij}^*}}-A_{ij}\right)(e_i+e_j)\\
&=\frac{2}{\sqrt{n}}\sum_{i\neq j}\left(\frac{e^{P_{ij}^*}}{1+e^{P_{ij}^*}}-A_{ij}\right)e_i\\
&=\frac{2}{\sqrt{n}}\sum_{i=1}^n\left(\sum_{j\neq i}\left(\frac{e^{P_{ij}^*}}{1+e^{P_{ij}^*}}-A_{ij}\right)\right)e_i.
\end{align*}
For any fixed $i$, we have
\begin{align*}
\sum_{j\neq i}\left(\frac{e^{P_{ij}^*}}{1+e^{P_{ij}^*}}-A_{ij}\right)  
\end{align*}
is the sum of $n-1$ independent $1$-subgaussian random variables. Thus, with probability at least $1-n^{-11}$, it holds that
\begin{align*}
    \left|\sum_{j\neq i}\left(\frac{e^{P_{ij}^*}}{1+e^{P_{ij}^*}}-A_{ij}\right) \right|\lesssim \sqrt{n\log n}.
\end{align*}
Take union bound, we have with probability at least $1-n^{-10}$, for all $i\in [n]$, it holds that 
\begin{align*}
    \left|\sum_{j\neq i}\left(\frac{e^{P_{ij}^*}}{1+e^{P_{ij}^*}}-A_{ij}\right) \right|\lesssim \sqrt{n\log n},
\end{align*}
which implies $\|\nabla_{\theta} f(M^*,F^*)\|_2\lesssim \sqrt{n\log n}$.

To bound $\|\nabla_{H} f(M^*,F^*)\|_F$, note that
\begin{align*}
 \nabla_{H} f(M^*,F^*)
=\nabla_{H} L(M^*,F^*)
=\sum_{i\neq j}\left(\frac{e^{P_{ij}^*}}{1+e^{P_{ij}^*}}-A_{ij}\right)z_iz_j^T.
\end{align*}
By Assumption \ref{assumption:scales}, we have
\begin{align*}
\left\|\sum_{i\neq j}\bbE\left[\left(\frac{e^{P_{ij}^*}}{1+e^{P_{ij}^*}}-A_{ij}\right)^2z_iz_j^Tz_jz_i^T\right]\right\|\lesssim \sum_{i\neq j}\|z_i\|_2^2\|z_j\|_2^2
\asymp \sz^2.
\end{align*}
Thus, by matrix Bernstein inequality, with probability at least $1-n^{-10}$, we have
\begin{align*}
    \left\|\sum_{i\neq j}\left(\frac{e^{P_{ij}^*}}{1+e^{P_{ij}^*}}-A_{ij}\right)z_iz_j^T\right\|\lesssim \sz\sqrt{\log n},
\end{align*}
which implies that $\|\nabla_{H} f(M^*,F^*)\|_F\leq \sqrt{p}\|\nabla_{H} f(M^*,F^*)\|\lesssim \sz\sqrt{p\log n}$.


Finally, we bound $\|\nabla_{F} f(M^*,F^*)\|_F$. Note that
\begin{align*}
\|\nabla_{F} f(M^*,F^*)\|_F&\leq \|\nabla_{X} f(M^*,F^*)\|_F+\|\nabla_{Y} f(M^*,F^*)\|_F\\
&\leq \|\nabla_{X} L(M^*,F^*)\|_F+\|\nabla_{Y} L(M^*,F^*)\|_F+\lambda\left(\|X^{*}\|_F+\|Y^{*}\|_F\right)\\
&\leq \|\nabla_{\Gamma}L_c(\theta^*,H^*,\Gamma^*)\|\left(\|X^{*}\|_F+\|Y^{*}\|_F\right)+\lambda\left(\|X^{*}\|_F+\|Y^{*}\|_F\right),
\end{align*}
where the last inequality follows from the fact that $\|AB\|_F\leq \|A\|\|B\|_F$. Here 
\begin{align*}
\nabla_{\Gamma}L_c(\theta^*,H^*,\Gamma^*)=\frac{1}{n}\sum_{i\neq j}\left(\frac{e^{P_{ij}^*}}{1+e^{P_{ij}^*}}-A_{ij}\right)e_ie_j^T.
\end{align*}
Note that
\begin{align*}
\left\|\sum_{i\neq j}\bbE\left[\left(\frac{e^{P_{ij}^*}}{1+e^{P_{ij}^*}}-A_{ij}\right)^2e_ie_j^Te_je_i^T\right]\right\|\lesssim n\left\|\sum^n_{i=1}e_ie_i^T\right\|=n.
\end{align*}
Thus, by matrix Bernstein inequality, with probability at least $1-n^{-10}$, we have $\|\nabla_{\Gamma}L_c(\theta^*,H^*,\Gamma^*)\|\lesssim\sqrt{\frac{\log n}{n}}\lesssim\lambda$. Consequently, it holds that
\begin{align*}
 \|\nabla_{F} f(M^*,F^*)\|_F\lesssim \lambda   \left(\|X^{*}\|_F+\|Y^{*}\|_F\right).
\end{align*}
\end{proof}


\begin{lemma}\label{lem:gradient_spectral}
Suppose Lemma \ref{lem:ncv1} holds for the $t$-th iteration. Under Assumption \ref{assumption:eigenvalues}, we have
\begin{align*}
&\left\|\frac1n\sum_{i\neq j}\left(\frac{e^{P_{ij}^t}}{1+e^{P_{ij}^t}}-A_{ij}\right)e_i e_j^T\right\|\\
&\lesssim   \frac{\sqrt{\su}}{n}\left(\|\theta^t-\theta^{*}\|_{2}+\|H^t-H^{*}\|_{F}+\frac{1}{n}\|X^*\|\|F^tR^t-F^{*}\|_{F}\right)+\sqrt{\frac{\log n}{n}}\\
&\lesssim \sqrt{\frac{c_{11}^2\overline{C}+\log n}{n}}.
\end{align*}
\end{lemma}
\begin{proof}[Proof of Lemma \ref{lem:gradient_spectral}]
We denote 
\begin{align*}
D^t:=\frac1n\sum_{i\neq j}\left(\frac{e^{P_{ij}^t}}{1+e^{P_{ij}^t}}-A_{ij}\right)e_i e_j^T.
\end{align*}   
Note that
\begin{align*}
\|D^t\|\leq \left\|\frac1n\sum_{i\neq j}\left(\frac{e^{P_{ij}^t}}{1+e^{P_{ij}^t}}-\frac{e^{P_{ij}^*}}{1+e^{P_{ij}^*}}\right)e_i e_j^T\right\|
+\left\|\frac1n\sum_{i\neq j}\left(\frac{e^{P_{ij}^*}}{1+e^{P_{ij}^*}}-A_{ij}\right)e_i e_j^T\right\|.
\end{align*}
For the first term, we have
\begin{align*}
&\left\|\frac1n\sum_{i\neq j}\left(\frac{e^{P_{ij}^t}}{1+e^{P_{ij}^t}}-\frac{e^{P_{ij}^*}}{1+e^{P_{ij}^*}}\right)e_i e_j^T\right\|\\
&\leq  \frac1n\left\|\sum_{i\neq j}\left(\frac{e^{P_{ij}^t}}{1+e^{P_{ij}^t}}-\frac{e^{P_{ij}^*}}{1+e^{P_{ij}^*}}\right)e_i e_j^T\right\|_F\\
&=\frac1n\sqrt{\sum_{i\neq j}\left(\frac{e^{P_{ij}^t}}{1+e^{P_{ij}^t}}-\frac{e^{P_{ij}^*}}{1+e^{P_{ij}^*}}\right)^2}\\
&\leq \frac{1}{4n}\sqrt{\sum_{i\neq j}\left(P^t_{ij}-P^*_{ij}\right)^2}\tag{by mean value theorem}\\
&\lesssim \frac{\sqrt{\su}}{n}\left(\|\theta^t-\theta^{*}\|_{2}+\|H^t-H^{*}\|_{F}+\frac{1}{n}\|X^*\|\|F^tR^t-F^{*}\|_{F}\right),
\end{align*}
where the last inequality follows from
\begin{align*}
&\sum_{i\neq j}(P_{ij}^{t}-P_{ij}^*)^2\\
&=\sum_{i\neq j}\left(\frac{1}{\sqrt{n}}\langle\theta^{t}-\theta^*,e_i+e_j\rangle+\langle H^{t}-H^*,z_iz_j^T\rangle+\frac1n\langle X^{t}Y^{tT}-X^*Y^{*T},e_i e_j^T\rangle\right)^2\\
&=
\begin{bmatrix}
  \vec(\theta^{t}-\theta^*)\\
  \vec(H^{t}-H^*)\\
  \frac1n\vec(X^{t}Y^{tT}-X^*Y^{*T})
\end{bmatrix}^T
\left(\sum_{i\neq j}
  \begin{bmatrix}
  \frac{1}{\sqrt{n}}\vec(e_i+e_j)\\
  \vec(z_iz_j^T)\\
  \vec(e_ie_j^T)
  \end{bmatrix}
   \begin{bmatrix}
  \frac{1}{\sqrt{n}}\vec(e_i+e_j)\\
  \vec(z_iz_j^T)\\
  \vec(e_ie_j^T)
  \end{bmatrix}^T
\right)
\begin{bmatrix}
  \vec(\theta^{t}-\theta^*)\\
  \vec(H^{t}-H^*)\\
  \frac1n\vec(X^{t}Y^{tT}-X^*Y^{*T})
\end{bmatrix}\\
&\leq\su \left\|\begin{bmatrix}
  \vec(\theta^{t}-\theta^*)\\
  \vec(H^{t}-H^*)\\
  \frac1n\vec(X^{t}Y^{tT}-X^*Y^{*T})
\end{bmatrix}\right\|^2 \tag{by Assumption \ref{assumption:eigenvalues} and $\mathbf{1}^T(\theta^t-\theta^*)=0$}\\
& =\su\left(\|\theta^t-\theta^{*}\|^2_{2}+\|H^t-H^{*}\|^2_{F}+\frac{1}{n^2}\|X^tY^{tT}-X^{*}Y^{*T}\|^2_{F}\right)
\end{align*} 
and 
\begin{align*}
&\|X^tY^{tT}-X^{*}Y^{*T}\|_{F}\\
&=\|(X^tR^t-X^*)(Y^tR^t)^T+X^{*}(Y^tR^t-Y^*)^T\|_F\\
&\leq \|X^tR^t-X^*\|_F\|Y^tR^t\|+\|X^{*}\|\|Y^tR^t-Y^*\|_F\\
&\leq \|X^tR^t-X^*\|_F\|Y^tR^t-Y^*\|+\|X^tR^t-X^*\|_F\|Y^*\|+\|X^{*}\|\|Y^tR^t-Y^*\|_F\\
&\leq 3 \|X^{*}\|\|F^tR^t-Y^*\|_F.
\end{align*}
For the second term, as bound $\|\nabla_{\Gamma}L_c(\theta^*,H^*,\Gamma^*)\|$ in the proof of Lemma \ref{lem:gradient_norm}, we have with probability at least $1-n^{-10}$ that
\begin{align*}
 \left\|\frac1n\sum_{i\neq j}\left(\frac{e^{P_{ij}^*}}{1+e^{P_{ij}^*}}-A_{ij}\right)e_i e_j^T\right\|\lesssim \sqrt{\frac{\log n}{n}}   .
\end{align*}
As a result, we have
\begin{align*}
 \|D^t\|
 &\lesssim   \frac{\sqrt{\su}}{n}\left(\|\theta^t-\theta^{*}\|_{2}+\|H^t-H^{*}\|_{F}+\frac{1}{n}\|X^*\|\|F^tR^t-F^{*}\|_{F}\right)+\sqrt{\frac{\log n}{n}}\\
 &\lesssim c_{11}\sqrt{\frac{\overline{C}}{n}}+\sqrt{\frac{\log n}{n}} \tag{recall the definition of $\overline{C}$}\\
 &\lesssim \sqrt{\frac{c_{11}^2\overline{C}+\log n}{n}}.
\end{align*}
We then finish the proof.
\end{proof}





\subsection{Proofs of Lemma \ref{lem:ncv1}}\label{pf:lem_ncv1}
Suppose Lemma \ref{lem:ncv1}-Lemma \ref{lem:ncv5} hold for the $t$-th iteration. In the following, we prove Lemma \ref{lem:ncv1} for the $(t+1)$-th iteration. 
By the gradient decent update, we have
\begin{align*}
M^{t+1}=M^t-\eta\cP\left(\nabla_{M}f(M^t,F^t)\right)=\cP\left(M^t-\eta\nabla_{M}f(M^t,F^t)\right).
\end{align*}
Thus, it holds that
\begin{align*}
\|M^{t+1}-M^*\|_F
=\left\|\cP\left(M^t-\eta\nabla_{M}f(M^t,F^t)-M^*\right)\right\|_F
\leq \left\|M^t-\eta\nabla_{M}f(M^t,F^t)-M^*\right\|_F,
\end{align*}
which then gives
\begin{align}\label{ineq30:pf_lem_ncv1}
\left\|\begin{bmatrix}
M^{t+1}-M^{*}\\
F^{t+1}R^t-F^{*}
\end{bmatrix}\right\|_F
\leq 
\left\|\begin{bmatrix}
M^t-\eta\nabla_{M}f(M^t,F^t)-M^*\\
F^{t+1}R^t-F^{*}
\end{bmatrix}\right\|_F.
\end{align}
Consequently, we only need to bound the RHS of \eqref{ineq30:pf_lem_ncv1}. Note that
\begin{align*}
&\begin{bmatrix}
M^t-\eta\nabla_{M}f(M^t,F^t)-M^*\\
F^{t+1}R^t-F^{*}
\end{bmatrix}\\
&=
\begin{bmatrix}
M^t-\eta\nabla_{M}f(M^t,F^t)-M^*\\
\left(F^t-\eta\nabla_F f(M^t,F^t)\right)R^t-F^*
\end{bmatrix}\\
&=\begin{bmatrix}
M^t-\eta\nabla_{M}f(M^t,F^tR^t)
-M^*\\
F^tR^t-\eta\nabla_F f(M^t,F^tR^t)-F^*
\end{bmatrix}\\
&=\begin{bmatrix}
M^t-M^{*}\\
F^tR^t-F^*
\end{bmatrix}-\eta\nabla f(M^t,F^tR^t)\\
&=\begin{bmatrix}
M^t-M^{*}\\
F^tR^t-F^*
\end{bmatrix}-\eta\left(\nabla f_{\aug}(M^t,F^tR^t)-\nabla f_{\aug}(M^*,F^*)\right)+\eta\nabla f_{\diff}(F^tR^t)-\eta\nabla f_{\aug}(M^*,F^*).
\end{align*}
% \begin{align*}
% &\begin{bmatrix}
% M^{t+1}-M^{*}\\
% F^{t+1}R^t-F^{*}
% \end{bmatrix}\\
% &=
% \begin{bmatrix}
% M^t-\eta\nabla_{M}f(M^t,F^t)+\eta
% \begin{bmatrix}
% \mean\left(\nabla_{\theta}f(M^t,F^t)\right)\cdot\mathbf{1}\\
% 0
% \end{bmatrix}-M^*\\
% \left(F^t-\eta\nabla_F f(M^t,F^t)\right)R^t-F^*
% \end{bmatrix}\\
% &=\begin{bmatrix}
% M^t-\eta\nabla_{M}f(M^t,F^tR^t)+\eta
% \begin{bmatrix}
% \mean\left(\nabla_{\theta}f(M^t,F^tR^t)\right)\cdot\mathbf{1}\\
% 0
% \end{bmatrix}-M^*\\
% F^tR^t-\eta\nabla_F f(M^t,F^tR^t)-F^*
% \end{bmatrix}\\
% &=\begin{bmatrix}
% M^t-M^{*}\\
% F^tR^t-F^*
% \end{bmatrix}-\eta\nabla f(M^t,F^tR^t)+\eta\begin{bmatrix}
% \mean\left(\nabla_{\theta}f(M^t,F^tR^t)\right)\cdot\mathbf{1}\\
% 0
% \end{bmatrix}\\
% &=\begin{bmatrix}
% M^t-M^{*}\\
% F^tR^t-F^*
% \end{bmatrix}-\eta\left(\nabla f_{\aug}(M^t,F^tR^t)-\nabla f_{\aug}(M^*,F^*)\right)+\eta\nabla f_{\diff}(F^tR^t)-\eta\nabla f_{\aug}(M^*,F^*)\\
% &\quad+\eta\begin{bmatrix}
% \mean\left(\nabla_{\theta}f(M^t,F^tR^t)\right)\cdot\mathbf{1}\\
% 0
% \end{bmatrix}.
% \end{align*}
Also, it holds that
\begin{align*}
\nabla f_{\aug}(M^t,F^tR^t)-\nabla f_{\aug}(M^*,F^*)=\int^1_0\nabla^2 f_{\aug}\left((M^*,F^*)+\tau(M^t-M^*,F^tR^t-F^*)\right)d \tau\cdot \begin{bmatrix}
M^t-M^{*}\\
F^tR^t-F^*
\end{bmatrix}.
\end{align*}
Thus, we have
\begin{align*}
&\begin{bmatrix}
M^t-\eta\nabla_{M}f(M^t,F^t)-M^*\\
F^{t+1}R^t-F^{*}
\end{bmatrix}\\
&=\left(I-\eta\int^1_0\nabla^2 f_{\aug}\left((M^*,F^*)+\tau(M^t-M^*,F^tR^t-F^*)\right)d \tau\right)\cdot \begin{bmatrix}
M^t-M^{*}\\
F^tR^t-F^*
\end{bmatrix}\\
&\quad +\eta\nabla f_{\diff}(F^tR^t)-\eta\nabla f_{\aug}(M^*,F^*).
\end{align*}
For notation simplicity, we denote 
\begin{align*}
A:=\int^1_0\nabla^2 f_{\aug}\left((M^*,F^*)+\tau(M^t-M^*,F^tR^t-F^*)\right)d \tau.
\end{align*}
Since Lemma \ref{lem:ncv4} holds for the $t$-th iteration, we know $A$ satisfies the local geometry properties as outlined in Lemma \ref{lem:convexity} as long as $c_{41}\leq c_1$, $c_{11}\leq c_2$, $c_{43}\leq c_3$.
By triangle inequality, we have
\begin{align*}
&\left\|\begin{bmatrix}
M^t-\eta\nabla_{M}f(M^t,F^t)-M^*\\
F^{t+1}R^t-F^{*}
\end{bmatrix}\right\|_F\\
&\leq \underbrace{\left\|(I-\eta A)\begin{bmatrix}
M^t-M^{*}\\
F^tR^t-F^*
\end{bmatrix}\right\|_F}_{(1)}+\eta\underbrace{\|\nabla f_{\diff}(F^tR^t)\|_F}_{(2)}+\eta\underbrace{\|\nabla f_{\aug}(M^*,F^*)\|_F}_{(3)}.
% +\eta\cdot\underbrace{\sqrt{n}\left|\mean\left(\nabla_{\theta}f(M^t,F^tR^t)\right)\right|}_{(4)}.
\end{align*}
In the following, we bound (1)-(3), respectively.
\begin{enumerate}
\item We first bound (1).
Note that
\begin{align*}
(1)^2&=\vec
\begin{bmatrix}
M^t-M^{*}\\
F^tR^t-F^{*}
\end{bmatrix}^T
(I-2\eta A+\eta^2 A^2)
\vec
\begin{bmatrix}
M^t-M^{*}\\
F^tR^t-F^{*}
\end{bmatrix}\\
&=\left\|
\begin{bmatrix}
M^t-M^{*}\\
F^tR^t-F^{*}
\end{bmatrix}
\right\|_F^2-2\eta\vec
\begin{bmatrix}
M^t-M^{*}\\
F^tR^t-F^{*}
\end{bmatrix}^T A \ 
\vec
\begin{bmatrix}
M^t-M^{*}\\
F^tR^t-F^{*}
\end{bmatrix}\\
&\quad+\eta^2\vec
\begin{bmatrix}
M^t-M^{*}\\
F^tR^t-F^{*}
\end{bmatrix}^TA^2\ \vec
\begin{bmatrix}
M^t-M^{*}\\
F^tR^t-F^{*}
\end{bmatrix}.
\end{align*}
By Lemma \ref{lem:convexity}, we have
\begin{align*}
% & \vec
% \begin{bmatrix}
% M^t-M^{*}\\
% F^tR^t-F^{*}
% \end{bmatrix}^T A \ 
% \vec
% \begin{bmatrix}
% M^t-M^{*}\\
% F^tR^t-F^{*}
% \end{bmatrix}\geq \underline{C}\left( \|\theta^t-\theta^{*}\|^2_2+\|H^t-H^{*}\|^2_F+\frac{\sigma_{\min}}{8n^2}\|F^tR^t-F^*\|_F^2\right),\\
& \vec
\begin{bmatrix}
M^t-M^{*}\\
F^tR^t-F^{*}
\end{bmatrix}^T A \ 
\vec
\begin{bmatrix}
M^t-M^{*}\\
F^tR^t-F^{*}
\end{bmatrix}\geq \underline{C}\left\|
\begin{bmatrix}
M^t-M^{*}\\
F^tR^t-F^{*}
\end{bmatrix}
\right\|_F^2,\\
&\vec
\begin{bmatrix}
M^t-M^{*}\\
F^tR^t-F^{*}
\end{bmatrix}^TA^2\ \vec
\begin{bmatrix}
M^t-M^{*}\\
F^tR^t-F^{*}
\end{bmatrix}\leq \overline{C}^2\left\|
\begin{bmatrix}
M^t-M^{*}\\
F^tR^t-F^{*}
\end{bmatrix}
\right\|_F^2,
\end{align*}
where the second inequality holds since by Lemma \ref{lem:convexity}, we know $\|A\|\leq  \overline{C}$. As a result, we have
% \begin{align*}
% (1)^2&\leq \left(1+\eta^2\left(\frac{20\su\sigma_{\max}}{n^2}\right)^2-2\underline{C}\eta\right)\left(\|\theta^t-\theta^{*}\|^2_2+\|H^t-H^{*}\|^2_F\right)\\
% &\quad +\left(1+\eta^2\left(\frac{20\su\sigma_{\max}}{n^2}\right)^2-\underline{C}\eta\frac{\sigma_{\min}}{4n^2}\right)\|F^tR^t-F^*\|_F^2\\
% &\leq  \left(1-\underline{C}\eta\right)\left(\|\theta^t-\theta^{*}\|^2_2+\|H^t-H^{*}\|^2_F\right)+\left(1-\frac{\underline{C}\sigma_{\min}}{8n^2}\eta\right)\|F^tR^t-F^*\|_F^2,
% \end{align*}
\begin{align*}
(1)^2&\leq \left(1+\eta^2\overline{C}^2-2\underline{C}\eta\right)
\left\|
\begin{bmatrix}
M^t-M^{*}\\
F^tR^t-F^{*}
\end{bmatrix}
\right\|_F^2\\
&\leq  \left(1-\underline{C}\eta\right)
\left\|
\begin{bmatrix}
M^t-M^{*}\\
F^tR^t-F^{*}
\end{bmatrix}
\right\|_F^2,
\end{align*}
where the second inequality holds as long as $\eta\overline{C}^2\leq \underline{C}$.
This implies 
\begin{align*}
(1)&\leq \left(1-\frac{\underline{C}}{2}\eta\right)
\left\|
\begin{bmatrix}
M^t-M^{*}\\
F^tR^t-F^{*}
\end{bmatrix}
\right\|_F,
\end{align*}
% \begin{align*}
% (1)&\leq \left(1-\frac{\underline{C}}{2}\eta\right)\left(\|\theta^t-\theta^{*}\|_2+\|H^t-H^{*}\|_F\right)+\left(1-\frac{\underline{C}\sigma_{\min}}{16n^2}\eta\right)\|F^tR^t-F^*\|_F,
% \end{align*}
which follows from the fact that $\sqrt{1-x}\leq 1-\frac{x}{2}$.



\item We then bound (2). Note that
\begin{align*}
&\nabla_X f_{\diff}(F^tR^t)=\frac{4c_{\aug}}{n^2}X^t(X^{tT}X^t-Y^{tT}Y^t)R^t,\\
&\nabla_Y f_{\diff}(F^tR^t)=\frac{4c_{\aug}}{n^2}Y^t(Y^{tT}Y^t-X^{tT}X^t)R^t.
\end{align*}
Thus, we have
\begin{align*}
\|\nabla f_{\diff}(F^tR^t)\|_F&\leq \frac{4c_{\aug}}{n^2}\left(\|X^t(X^{tT}X^t-Y^{tT}Y^t)R^t\|_F+\|Y^t(Y^{tT}Y^t-X^{tT}X^t)R^t\|_F\right)\\
&\leq \frac{4c_{\aug}}{n^2}\left(\|X^t\|+\|Y^t\|\right)\|X^{tT}X^t-Y^{tT}Y^t\|_F.
\end{align*}
Since Lemma \ref{lem:ncv1} holds for the $t$-th iteration, we have
\begin{align*}
\|F^t\|=\|F^tR^t\|\leq \|F^tR^t-F^*\|+\|F^*\|\leq 2\|F^*\|,
\end{align*}
where the last inequality holds because by Lemma \ref{lem:ncv1}, we have $\|F^tR^t-F^*\|\ll \|F^*\|$.
Consequently, we have
\begin{align*}
 (2)=\|\nabla f_{\diff}(F^tR^t)\|_F\leq \frac{16c_{\aug}}{n^2} \|F^*\|  \|X^{tT}X^t-Y^{tT}Y^t\|_F.
\end{align*}


\item We then bound (3).
Note that $X^{*T}X^{*}=Y^{*T}Y^{*}$. Thus, we have $\nabla f_{\diff}(F^*)=0$, which implies $\nabla f_{\aug}(M^*,F^*)=\nabla f(M^*,F^*)$.
By Lemma \ref{lem:gradient_norm}, we have 
\begin{align*}
(3)=\|\nabla f(M^*,F^*)\|_F\lesssim \sqrt{n \log n}+c_z\sqrt{p\log n}+c_{\lambda}\sqrt{\frac{\log n}{n}}\cdot \sqrt{\mu r \sigma_{\max}}\lesssim \frac{c_{\lambda}\sqrt{\mu r\sigma_{\max}}}{n}\sqrt{n \log n}
\end{align*}
as long as $\sz^2 p\lesssim n$ and $1\lesssim \frac{c_{\lambda}\sqrt{\mu r\sigma_{\max}}}{n}$.


% \item Finally, we bound (4).
% \textcolor{red}{
% Here 
% \begin{align*}
% (4):= \sqrt{n}\left|\mean\left(\nabla_{\theta}f(M^t,F^tR^t)\right)\right|.
% \end{align*}
% At the beginning of the proof, we already removed this term by considering the projection. Thus, the bound on this term is no longer needed. But we still keep it here in case other parts need this proof.
% }



% Note that
% \begin{align*}
% \nabla_{\theta}f(M^t,F^tR^t)
% &=\nabla_{\theta}L(M^t,F^tR^t)\\
% &=\nabla_{\theta}L(M^*,F^*)+\nabla_{\theta}L(M^t,F^tR^t)-\nabla_{\theta}L(M^*,F^*).
% \end{align*}
% For the first term, we have
% \begin{align*}
% n\cdot \mean\left(\nabla_{\theta}L(M^*,F^*)\right)&=\nabla_{\theta}L(M^*,F^*)^T\cdot\mathbf{1}\\
% &=\frac{2}{\sqrt{n}}\sum_{i\neq j}\left(\frac{e^{P_{ij}^{*}}}{1+e^{P_{ij}^{*}}}-A_{ij}\right)\\
% &=\frac{4}{\sqrt{n}}\sum_{i< j}\left(\frac{e^{P_{ij}^{*}}}{1+e^{P_{ij}^{*}}}-A_{ij}\right)
% \end{align*}
% Since $\sum_{i< j}\left(\frac{e^{P_{ij}^{*}}}{1+e^{P_{ij}^{*}}}-A_{ij}\right)$ is the sum of $n(n-1)/2$ i.i.d mean zero $1$-subgaussian random variables, we have with probability at least $1-n^{-10}$ that
% \begin{align*}
% \left| \sum_{i\neq j}\left(\frac{e^{P_{ij}^{*}}}{1+e^{P_{ij}^{*}}}-A_{ij}\right)\right|\lesssim n\sqrt{\log n},
% \end{align*}
% which implies that
% \begin{align*}
% \left|\mean\left(\nabla_{\theta}L(M^*,F^*)\right)\right|=O\left(\sqrt{\frac{\log n}{n}}\right).    
% \end{align*}
% For the rest of the terms, we have 
% \begin{align*}
% &n\cdot \mean\left(\nabla_{\theta}L(M^t,F^tR^t)-\nabla_{\theta}L(M^*,F^*)\right)\\
% &=\frac{2}{\sqrt{n}}\sum_{i\neq j}\left(\frac{e^{P_{ij}^{t}}}{1+e^{P_{ij}^{t}}}-\frac{e^{P_{ij}^{*}}}{1+e^{P_{ij}^{*}}}\right)\\
% &\leq \frac{1}{2\sqrt{n}}\sum_{i\neq j}\left|P^t_{ij}-P^{*}_{ij}\right| \tag{by mean-value theorem}\\
% &\leq \frac{\sqrt{n}}{2}\sqrt{\sum_{i\neq j}\left|P^t_{ij}-P^{*}_{ij}\right|^2}. \tag{by Cauchy-Schwarz}
% \end{align*}

% Note that
% \begin{align*}
% &\sum_{i\neq j}(P_{ij}^{t}-P_{ij}^*)^2\\
% &=\sum_{i\neq j}\left(\frac{1}{\sqrt{n}}\langle\theta^{t}-\theta^*,e_i+e_j\rangle+\langle H^{t}-H^*,z_iz_j^T\rangle+\frac1n\langle X^{t}Y^{tT}-X^*Y^{*T},e_i e_j^T\rangle\right)^2\\
% &=
% \begin{bmatrix}
%   \vec(\theta^{t}-\theta^*)\\
%   \vec(H^{t}-H^*)\\
%   \frac1n\vec(X^{t}Y^{tT}-X^*Y^{*T})
% \end{bmatrix}^T
% \left(\sum_{i\neq j}
%   \begin{bmatrix}
%   \frac{1}{\sqrt{n}}\vec(e_i+e_j)\\
%   \vec(z_iz_j^T)\\
%   \vec(e_ie_j^T)
%   \end{bmatrix}
%    \begin{bmatrix}
%   \frac{1}{\sqrt{n}}\vec(e_i+e_j)\\
%   \vec(z_iz_j^T)\\
%   \vec(e_ie_j^T)
%   \end{bmatrix}^T
% \right)
% \begin{bmatrix}
%   \vec(\theta^{t}-\theta^*)\\
%   \vec(H^{t}-H^*)\\
%   \frac1n\vec(X^{t}Y^{tT}-X^*Y^{*T})
% \end{bmatrix}\\
% &\lesssim \left\|\begin{bmatrix}
%   \vec(\theta^{t}-\theta^*)\\
%   \vec(H^{t}-H^*)\\
%   \frac1n\vec(X^{t}Y^{tT}-X^*Y^{*T})
% \end{bmatrix}\right\|^2 \tag{by balanced eigenvalues assumption and $\mathbf{1}^T(\theta^t-\theta^*)=0$}\\
% & =\|\theta^t-\theta^{*}\|^2_{2}+\|H^t-H^{*}\|^2_{F}+\frac{1}{n^2}\|X^tY^{tT}-X^{*}Y^{*T}\|^2_{F}.
% \end{align*}
% As a result, we have
% \begin{align*}
% \left|\mean\left(\nabla_{\theta}L(M^t,F^tR^t)-\nabla_{\theta}L(M^*,F^*)\right)\right|
% \lesssim \frac{1}{\sqrt{{n}}}\left(\|\theta^t-\theta^{*}\|_{2}+\|H^t-H^{*}\|_{F}+\frac{1}{n}\|X^tY^{tT}-X^{*}Y^{*T}\|_{F}\right).
% \end{align*}
% Combine the above results, we show that
% \begin{align*}
%  \left|\mean\left(\nabla_{\theta}f(M^t,F^tR^t)\right)\right| 
%  \lesssim O\left(\sqrt{\frac{\log n}{n}}\right)+\frac{1}{\sqrt{{n}}}\left(\|\theta^t-\theta^{*}\|_{2}+\|H^t-H^{*}\|_{F}+\frac{1}{n}\|X^tY^{tT}-X^{*}Y^{*T}\|_{F}\right),
% \end{align*}
% which implies
% \begin{align*}
%  (4)
%  \lesssim O\left(\sqrt{\log n}\right)+\|\theta^t-\theta^{*}\|_{2}+\|H^t-H^{*}\|_{F}+\frac{1}{n}\|X^tY^{tT}-X^{*}Y^{*T}\|_{F}.
% \end{align*}

\end{enumerate}




Consequently, we conclude that
\begin{align*}
&\left\|\begin{bmatrix}
M^t-\eta\nabla_{M}f(M^t,F^t)-M^*\\
F^{t+1}R^t-F^{*}
\end{bmatrix}\right\|_F\\
&\leq\left(1-\frac{\underline{C}}{2}\eta\right)
\left\|
\begin{bmatrix}
M^t-M^{*}\\
F^tR^t-F^{*}
\end{bmatrix}
\right\|_F+\frac{16 \eta c_{\aug}}{n^2} \|F^*\|  \|X^{tT}X^t-Y^{tT}Y^t\|_F+\frac{c_{\lambda}\eta \sqrt{\mu r\sigma_{\max}}}{n}\sqrt{n \log n}.
% &\quad +\eta\left(\|\theta^t-\theta^{*}\|_{2}+\|H^t-H^{*}\|_{F}+\frac{1}{n}\|X^tY^{tT}-X^{*}Y^{*T}\|_{F}\right).
\end{align*}
Recall \eqref{ineq30:pf_lem_ncv1}, we then have
\begin{align*}
 &\left\|\begin{bmatrix}
M^{t+1}-M^{*}\\
F^{t+1}R^t-F^{*}
\end{bmatrix}\right\|_F\\  
&\leq\left(1-\frac{\underline{C}}{2}\eta\right)
\left\|
\begin{bmatrix}
M^t-M^{*}\\
F^tR^t-F^{*}
\end{bmatrix}
\right\|_F+\frac{16 \eta c_{\aug}}{n^2} \|F^*\|  \|X^{tT}X^t-Y^{tT}Y^t\|_F+\frac{c_{\lambda}\eta \sqrt{\mu r\sigma_{\max}}}{n}\sqrt{n \log n}.
\end{align*}
By Lemma \ref{ar:lem1}, we know $\|F^*\|\leq 2\sqrt{\sigma_{\max}}$. By Lemma \ref{lem:ncv5}, we have $\|X^{tT}X^t-Y^{tT}Y^t\|_F\leq c_{51}\eta n^2$. 
We then obtain that
\begin{align*}
 &\left\|\begin{bmatrix}
M^{t+1}-M^{*}\\
F^{t+1}R^t-F^{*}
\end{bmatrix}\right\|_F\\   
&\leq\left(1-\frac{\underline{C}}{2}\eta\right)
\left\|
\begin{bmatrix}
M^t-M^{*}\\
F^tR^t-F^{*}
\end{bmatrix}
\right\|_F
+{32 c_{\aug}c_{51}\sqrt{\sigma_{\max}}\eta^2}+\frac{c_{\lambda}\eta \sqrt{\mu r\sigma_{\max}}}{n}\sqrt{n \log n}.
\end{align*}
Since Lemma \ref{lem:ncv1} holds for the $t$-th iteration, we have
\begin{align*}
 &\left\|\begin{bmatrix}
M^{t+1}-M^{*}\\
F^{t+1}R^t-F^{*}
\end{bmatrix}\right\|_F\\   
&\leq\left(1-\frac{\underline{C}}{2}\eta\right)c_{11}\sqrt{n}+{32 c_{\aug}c_{51}\sqrt{\sigma_{\max}}\eta^2}+\frac{c_{\lambda}\eta \sqrt{\mu r\sigma_{\max}}}{n}\sqrt{n \log n}\\
&\leq c_{11}\sqrt{n}
\end{align*}
as long as $\frac{8 c_{\lambda} \sqrt{\mu r\sigma_{\max}}}{n}\sqrt{ \log n}\leq c_{11} \underline{C} $ and $\frac{256 c_{\aug}c_{51}\sqrt{\sigma_{\max}}\eta}{\sqrt{n}}\leq c_{11} \underline{C} $.
Finally, by the definition of $R^{t+1}$, we have
\begin{align*}
 \|F^{t+1}R^{t+1}-F^{*}\|_F\leq  \|F^{t+1}R^{t}-F^{*}\|_F.   
\end{align*}
Consequently, we have
\begin{align*}
&\left\|\begin{bmatrix}
M^{t+1}-M^{*}\\
F^{t+1}R^{t+1}-F^{*}
\end{bmatrix}\right\|_F  \leq c_{11}\sqrt{n}.
\end{align*}



It remains to show that $\|F^{t+1}R^{t+1}-F^{*}\|\leq c_{14}\sqrt{n}$.
To facilitate analysis, we introduce an auxiliary point $\tilde{F}^{t+1}:=\begin{bmatrix}
\tilde{X}^{t+1}\\
\tilde{Y}^{t+1}
\end{bmatrix}$ where
\begin{align*}
&\tilde{X}^{t+1}={X}^{t}{R}^{t}-\frac{\eta}{n}\sum_{i\neq j}\left(\frac{e^{P_{ij}^{t}}}{1+e^{P_{ij}^{t}}}-A_{ij}\right)e_ie_j^TY^*-\eta\lambda X^*-\frac{4c_{\aug}\eta}{n^2}X^*{R}^{tT}\left({X}^{tT}{X}^{t}-{Y}^{tT}{Y}^{t}\right){R}^{t},\\
&\tilde{Y}^{t+1}={Y}^{t}{R}^{t}-\frac{\eta}{n}\sum_{i\neq j}\left(\frac{e^{P_{ij}^{t}}}{1+e^{P_{ij}^{t}}}-A_{ij}\right)e_je_i^TX^*-\eta\lambda Y^*-\frac{4c_{\aug}\eta}{n^2}Y^*{R}^{tT}\left({Y}^{tT}{Y}^{t}-{X}^{tT}{X}^{t}\right){R}^{t}.
\end{align*}
We then have
\begin{align*}
\|F^{t+1}R^{t+1}-F^{*}\|\leq \underbrace{\|\tilde{F}^{t+1}-F^{*}\|}_{(1)} + \underbrace{\|F^{t+1}R^{t+1}-\tilde{F}^{t+1}\|}_{(2)}.
\end{align*}
In the following, we bound (1) and (2), respectively.
\begin{enumerate}
\item We first bound (1).
Note that
\begin{align*}
&\left\|\tilde{F}^{t+1}-F^{*}\right\|\\
&\leq \left\| 
\begin{bmatrix}
X^t R^t - \frac{8c_{\aug}\eta}{n^2} \left[ (X^t Y^{t T} - \Gamma^{*}) Y^* + \frac{1}{2} X^* R^t (X^t X^t - Y^{t T} Y^t) R^t \right] - X^* \\
Y^t R^t -\frac{8c_{\aug}\eta}{n^2} \left[ (X^t Y^{t T} - \Gamma^{*}) X^* + \frac{1}{2} Y^* R^t (Y^{t T} Y^t - X^t X^t) R^t \right] - Y^* 
\end{bmatrix}\right\|\\
&\quad +\frac{\eta}{n} \left\| 
\begin{bmatrix}
\sum_{i\neq j}\left(\frac{e^{P_{ij}^{t}}}{1+e^{P_{ij}^{t}}}-\frac{e^{P_{ij}^{*}}}{1+e^{P_{ij}^{*}}}\right)e_ie_j^TY^*  \\
 \sum_{i\neq j}\left(\frac{e^{P_{ij}^{t}}}{1+e^{P_{ij}^{t}}}-\frac{e^{P_{ij}^{*}}}{1+e^{P_{ij}^{*}}}\right)e_je_i^TX^*
\end{bmatrix}-\frac{8c_{\aug}}{n}
\begin{bmatrix}
(X^t Y^{t T} - \Gamma^{*}) Y^{*}  \\
 (X^t Y^{t T} - \Gamma^{*}) X^* 
\end{bmatrix}\right\|\\
&\quad +\frac{\eta}{n}\left\| 
\begin{bmatrix}
\sum_{i\neq j}\left(\frac{e^{P_{ij}^{*}}}{1+e^{P_{ij}^{*}}}-A_{ij}\right)e_ie_j^TY^*  \\
 \sum_{i\neq j}\left(\frac{e^{P_{ij}^{*}}}{1+e^{P_{ij}^{*}}}-A_{ij}\right)e_je_i^TX^*
\end{bmatrix}\right\|+\eta\lambda \|F^{*}\|\\
&\leq \left\| 
\begin{bmatrix}
X^t R^t - \frac{8c_{\aug}\eta}{n^2} \left[ (X^t Y^{t T} - \Gamma^{*}) Y^* + \frac{1}{2} X^* R^t (X^t X^t - Y^{t T} Y^t) R^t \right] - X^* \\
Y^t R^t -\frac{8c_{\aug}\eta}{n^2} \left[ (X^t Y^{t T} - \Gamma^{*}) X^* + \frac{1}{2} Y^* R^t (Y^{t T} Y^t - X^t X^t) R^t \right] - Y^* 
\end{bmatrix}\right\|\\
&\quad +\frac{\eta}{n} \left\| 
\sum_{i\neq j}\left(\frac{e^{P_{ij}^{t}}}{1+e^{P_{ij}^{t}}}-\frac{e^{P_{ij}^{*}}}{1+e^{P_{ij}^{*}}}\right)e_ie_j^T- \frac{8c_{\aug}}{n}(X^t Y^{t T} - \Gamma^{*})
\right\| \|F^{*}\|\\
&\quad +\frac{\eta}{n}\left\| 
\sum_{i\neq j}\left(\frac{e^{P_{ij}^{*}}}{1+e^{P_{ij}^{*}}}-A_{ij}\right)e_ie_j^T \right\|\|F^{*}\|+\eta\lambda \|F^{*}\|.
\end{align*}
For the first term, as bounding $\beta_1$ in the proof of Lemma 11 in \cite{chen2020noisy}, we have
\begin{align*}
 &\left\| 
\begin{bmatrix}
X^t R^t - \frac{8c_{\aug}\eta}{n^2} \left[ (X^t Y^{t T} - \Gamma^{*}) Y^* + \frac{1}{2} X^* R^t (X^t X^t - Y^{t T} Y^t) R^t \right] - X^* \\
Y^t R^t -\frac{8c_{\aug}\eta}{n^2} \left[ (X^t Y^{t T} - \Gamma^{*}) X^* + \frac{1}{2} Y^* R^t (Y^{t T} Y^t - X^t X^t) R^t \right] - Y^* 
\end{bmatrix}\right\|\\
&\leq \left(1-\eta\frac{8c_{\aug}\sigma_{\min}}{n^2}\right)\|F^tR^t-F^{*}\|   + \frac{32c_{\aug}\eta}{n^2}\|F^tR^t-F^{*}\|^2\|F^*\|
\end{align*}
For the second term, we have 
\begin{align*}
&\frac{1}{n} \left\| 
\sum_{i\neq j}\left(\frac{e^{P_{ij}^{t}}}{1+e^{P_{ij}^{t}}}-\frac{e^{P_{ij}^{*}}}{1+e^{P_{ij}^{*}}}\right)e_ie_j^T- \frac{8c_{\aug}}{n}(X^t Y^{t T} - \Gamma^{*})
\right\|\\
&\leq \frac{1}{n} \left\| 
\sum_{i\neq j}\left(\frac{e^{P_{ij}^{t}}}{1+e^{P_{ij}^{t}}}-\frac{e^{P_{ij}^{*}}}{1+e^{P_{ij}^{*}}}\right)e_ie_j^T- \frac{8c_{\aug}}{n}(X^t Y^{t T} - \Gamma^{*})
\right\|_F.
\end{align*}
By the mean-value theorem, there exists $\{c_{ij}\}$ such that
\begin{align*}
\frac{e^{P_{ij}^{t}}}{1+e^{P_{ij}^{t}}}-\frac{e^{P_{ij}^{*}}}{1+e^{P_{ij}^{*}}}
=\frac{e^{c_{ij}}}{(1+e^{c_{ij}})^2}\left(P_{ij}^{t}-P_{ij}^{*}\right).
\end{align*}
Note that $\frac{e^{c_{ij}}}{(1+e^{c_{ij}})^2}\leq \frac14$ and $\left|\frac{e^{c_{ij}}}{(1+e^{c_{ij}})^2}-8c_{\aug}\right|\lesssim 1$, Thus, we have
\begin{align*}
&\left\| 
\sum_{i\neq j}\left(\frac{e^{P_{ij}^{t}}}{1+e^{P_{ij}^{t}}}-\frac{e^{P_{ij}^{*}}}{1+e^{P_{ij}^{*}}}\right)e_ie_j^T- \frac{8c_{\aug}}{n}(X^t Y^{t T} - \Gamma^{*})
\right\|_F\\
&=\left\| 
\sum_{i\neq j}\frac{e^{c_{ij}}}{(1+e^{c_{ij}})^2}\left(P_{ij}^{t}-P_{ij}^{*}\right)e_ie_j^T- \frac{8c_{\aug}}{n}(X^t Y^{t T} - \Gamma^{*})
\right\|_F\\
&\lesssim \|\theta^t-\theta^{*}\|_{2}+\|H^t-H^{*}\|_{F}+\frac{1}{n}\|X^tY^{tT}-X^{*}Y^{*T}\|_{F}\\
& \lesssim\|\theta^t-\theta^{*}\|_{2}+\|H^t-H^{*}\|_{F}+\frac{1}{n}\|X^*\|\|F^tR^t-F^{*}\|_{F}\\
& \lesssim \frac{\sqrt{\sigma_{\max}}}{n} c_{11}\sqrt{n},
\end{align*}
where the last inequality follows from Lemma \ref{lem:ncv1}.
Consequently, we obtain
\begin{align*}
\frac{1}{n} \left\| 
\sum_{i\neq j}\left(\frac{e^{P_{ij}^{t}}}{1+e^{P_{ij}^{t}}}-\frac{e^{P_{ij}^{*}}}{1+e^{P_{ij}^{*}}}\right)e_ie_j^T- \frac{8c_{\aug}}{n}(X^t Y^{t T} - \Gamma^{*})
\right\|\lesssim \frac{\sqrt{\sigma_{\max}}}{n^{3/2}} c_{11}.
\end{align*}
For the third term, as bound $\|\nabla_{\Gamma}L_c(\theta^*,H^*,\Gamma^*)\|$ in the proof of Lemma \ref{lem:gradient_norm}, we have
\begin{align*}
 \left\|\frac1n\sum_{i\neq j}\left(\frac{e^{P_{ij}^*}}{1+e^{P_{ij}^*}}-A_{ij}\right)e_i e_j^T\right\|\lesssim \sqrt{\frac{\log n}{n}}   .
\end{align*}
Consequently, we have
\begin{align*}
&\left\|\tilde{F}^{t+1}-F^{*}\right\|\\
&\leq  \left(1-\eta\frac{8c_{\aug}\sigma_{\min}}{n^2}\right)\|F^tR^t-F^{*}\|   + \frac{32c_{\aug}\eta}{n^2}\|F^tR^t-F^{*}\|^2\|F^*\|\\
&\quad+c\eta\frac{{\sigma_{\max}}}{n^{3/2}} c_{11}+c{\eta}\|F^*\|\sqrt{\frac{\log n}{n}}+\eta\lambda \|F^{*}\| \\
&\leq  \left(1-\eta\frac{8c_{\aug}\sigma_{\min}}{n^2}\right)\|F^tR^t-F^{*}\|   + \eta\frac{64c_{\aug}\sqrt{\sigma_{\max}}}{n^2}\|F^tR^t-F^{*}\|^2\\
&\quad+c\eta\frac{{\sigma_{\max}}}{n^{3/2}} c_{11}+c{\eta}\sqrt{\frac{\sigma_{\max}\log n}{n}}+2\eta\lambda\sqrt{\sigma_{\max}} \\
&\leq  \left(1-\eta\frac{8c_{\aug}\sigma_{\min}}{n^2}\right)c_{14}\sqrt{n}  + \eta\frac{64c_{\aug}\sqrt{\sigma_{\max}}}{n}c_{14}^2\\
&\quad+c\eta\frac{{\sigma_{\max}}}{n^{3/2}} c_{11}+c{\eta}\sqrt{\frac{\sigma_{\max}\log n}{n}}+2\eta\lambda\sqrt{\sigma_{\max}} \\
&\leq \left(1-\eta\frac{c_{\aug}\sigma_{\min}}{n^2}\right)c_{14}\sqrt{n}
\end{align*}
as long as $\sigma_{\min}\gtrsim \sqrt{n\sigma_{\max}}c_{14}$ and $\lambda+\sqrt{\frac{\log n}{n}}+\frac{\sqrt{\sigma_{\max}}}{n^{3/2}}c_{11}\lesssim \frac{c_{\aug}\sigma_{\min}}{n^{3/2}\sqrt{\sigma_{\max}}}c_{14}$.

\textcolor{red}{
Question:
The above condition implies $c_{14}\gtrsim \kappa c_{11}$. However, since the spectral norm is smaller than the Frobenius norm, we need $c_{14}\leq c_{11}$.
}



\item We then bound (2).
Note that by the above arguments, we have
\begin{align*}
\|F^{* T}\tilde{F}^{t+1}-F^{* T}F^{*}\|\leq \|F^*\|\|\tilde{F}^{t+1}-F^{*}\|\leq 2c_{14}\sqrt{n\sigma_{\max}}\leq \sigma_{\min},
\end{align*}
which then implies the following claim.
\begin{claim}\label{claim1:lem_ncv1}
We have
\begin{align*}
I_r = \argmin_{R\in\cO^{r\times r}}\left\|\tilde{F}^{t+1}R-F^*\right\|_F.
\end{align*}
\end{claim}
\begin{proof}
See Claim 4 in \cite{chen2020noisy}.
\end{proof}

We intend to apply Lemma \ref{ar:lem3} with $F_0=F^*, F_1=\tilde{F}^{t+1}, F_2=F^{t+1}R^t$, for which we need to check the two conditions therein.
First, we already have
\begin{align*}
\|F_1-F_0\|\|F_0\|=\|\tilde{F}^{t+1}-F^*\|\|F^*\|\leq \sigma_{\min}=\frac12 \sigma_r^2(F_0).
\end{align*}
Second, note that $\|F_1-F_2\|\|F_0\|=\|\tilde{F}^{t+1}-F^{t+1}R^t\|\|F^*\|$, thus we control $\|\tilde{F}^{t+1}-F^{t+1}R^t\|$ in the following.
Note that
\begin{align*}
    &F^{t+1} R^{t} - \tilde{F}^{t+1} = -\eta \begin{bmatrix} B & 0 \\ 0 & B^\top \end{bmatrix} \begin{bmatrix} Y^{t}R^{t}-Y^*  \\ X^{t}R^{t}-X^* \end{bmatrix} + \frac{4c_{\aug}\eta}{n^2} \begin{bmatrix} X^\star \\ -Y^\star \end{bmatrix} R^{t \top} C R^{t} - \eta \lambda\begin{bmatrix}   X^{t}R^{t}-X^*\\ Y^{t}R^{t}-Y^* \end{bmatrix} ,
\end{align*}
where we denote
\begin{align*}
 &B := \frac1n\sum_{i\neq j}\left(\frac{e^{P_{ij}^{t}}}{1+e^{P_{ij}^{t}}}-A_{ij}\right)e_ie_j^T,\\ 
 &C := X^{t \top} X^{t} - Y^{t \top} Y^{t}.
\end{align*}
This enables us to obtain
\begin{align*}
 &\left\|F^{t+1} R^{t} - \tilde{F}^{t+1}\right\|  \leq \eta \left\| B \right\| \left\| F^{t}R^{t}-F^*\right\| + \frac{4c_{\aug}\eta}{n^2} \left\| F^* \right\| \left\| C \right\|_F +\eta \lambda\left\| F^{t}R^{t}-F^*\right\|.   
\end{align*}
By Lemma \ref{lem:gradient_spectral}, we have
\begin{align*}
\|B\|\lesssim \sqrt{\frac{c_{11}^2\overline{C}+\log n}{n}},
\end{align*}
which implies 
\begin{align*}
 &\left\|F^{t+1} R^{t} - \tilde{F}^{t+1}\right\|    \\
 &\leq c{\eta}\left\| F^{t}R^{t}-F^*\right\|\sqrt{\frac{c_{11}^2\overline{C}+\log n}{n}}+ \frac{4c_{\aug}\eta}{n^2} \left\| F^* \right\| \left\|X^{t \top} X^{t} - Y^{t \top} Y^{t}\right\|_F +\eta \lambda\left\| F^{t}R^{t}-F^*\right\|\\
 &\lesssim \eta\left(c_{14}\sqrt{c_{11}^2\overline{C}+\log n}+c_{\aug}c_{51}\eta\sqrt{\sigma_{\max}}+\lambda c_{14}\sqrt{n}\right).
\end{align*}
An immediate consequence is that
\begin{align*}
 \|F_1-F_2\|\|F_0\|=\|\tilde{F}^{t+1}-F^{t+1}R^t\|\|F^*\|\leq    \frac{\sigma_{\min}}{2}=\frac14 \sigma_r^2(F_0)
\end{align*}
as long as $\eta\ll \frac{\sigma_{\min}}{\sqrt{n\sigma_{\max}}}$.

Since the two conditions in Lemma \ref{ar:lem3} holds with $F_0=F^*, F_1=\tilde{F}^{t+1}, F_2=F^{t+1}R^t$, we have
\begin{align*}
(2)&=\left\|\tilde{F}^{t+1}-F^{t+1}R^{t+1}\right\|\\
&\leq 5\kappa\left\|\tilde{F}^{t+1}-F^{t+1}R^{t}\right\|\\
& \lesssim \eta\kappa\left(c_{14}\sqrt{c_{11}^2\overline{C}+\log n}+c_{\aug}c_{51}\eta\sqrt{\sigma_{\max}}+\lambda c_{14}\sqrt{n}\right).
\end{align*}

\end{enumerate}

Combine the results for (1) and (2), we have
\begin{align*}
&\|F^{t+1}R^{t+1}-F^{*}\|\\
&\leq \left(1-\eta\frac{c_{\aug}\sigma_{\min}}{n^2}\right)c_{14}\sqrt{n}+c\eta\kappa\left(c_{14}\sqrt{c_{11}^2\overline{C}+\log n}+c_{\aug}c_{51}\eta\sqrt{\sigma_{\max}}+\lambda c_{14}\sqrt{n}\right)\\
&\leq c_{14}\sqrt{n}
\end{align*}
as long as $n$ large enough.
We then finish the proofs.



\subsection{Proofs of Lemma \ref{lem:ncv2}}\label{pf:lem_ncv2}
Suppose Lemma \ref{lem:ncv1}-Lemma \ref{lem:ncv5} hold for the $t$-th iteration. In the following, we prove Lemma \ref{lem:ncv2} for the $(t+1)$-th iteration.
More specifically, we fix $m$ and aim to bound
\begin{align*}
\left\|
\begin{bmatrix}
M^{t+1,(m)}-M^{t+1}\\
F^{t+1,(m)}O^{t+1,(m)}-F^{t+1}R^{t+1}
\end{bmatrix}
\right\|_F.
\end{align*}
\begin{claim}\label{claim:lem_ncv2}
It holds that
\begin{align*}
\|F^{t+1}R^{t+1}-F^{t+1,(m)}O^{t+1,(m)}\|_F\leq \|F^{t+1}R^{t}-F^{t+1,(m)}O^{t,(m)}\|_F.
\end{align*}
\end{claim}
\begin{proof}[Proof of Claim]
By the definition of $O^{t+1,(m)}$, for any $O\in\cO^{r\times r}$, we have
\begin{align*}
\|F^{t+1}R^{t+1}-F^{t+1,(m)}O^{t+1,(m)}\|_F\leq \|F^{t+1}R^{t+1}-F^{t+1,(m)}O\|_F.
\end{align*}
Choosing $O=O^{t,(m)}(R^t)^{-1}R^{t+1}$, we then have
\begin{align*}
\|F^{t+1}R^{t+1}-F^{t+1,(m)}O\|_F&=\|F^{t+1}R^{t+1}-F^{t+1,(m)}O^{t,(m)}(R^t)^{-1}R^{t+1}\|_F\\
&=\|F^{t+1}-F^{t+1,(m)}O^{t,(m)}(R^t)^{-1}\|_F\\
&=\|F^{t+1}R^t-F^{t+1,(m)}O^{t,(m)}\|_F,
\end{align*}
which then finishes the proofs.
\end{proof}

By Claim \ref{claim:lem_ncv2}, we only need to bound $\|F^{t+1}R^{t}-F^{t+1,(m)}O^{t,(m)}\|_F$.

Moreover, by the gradient decent update and the fact that $\nabla_M f(M,F)=\nabla_M f_{\aug}(M,F)$, we have
\begin{align*}
&M^{t+1}
=M^t-\eta\cP\left(\nabla_{M}f_{\aug}(M^t,F^t)\right)
=\cP\left(M^t-\eta\nabla_{M}f_{\aug}(M^t,F^t)\right)\\
&M^{t+1,(m)}
=M^{t,(m)}-\eta\cP\left(\nabla_{M}f^{(m)}_{\aug}(M^{t,(m)},F^{t,(m)})\right)
=\cP\left(M^{t,(m)}-\eta\nabla_{M}f^{(m)}_{\aug}(M^{t,(m)},F^{t,(m)})\right).
\end{align*}
It then holds that
\begin{align}\label{ineq30:pr_lem_ncv2}
&\left\|M^{t+1}-M^{t+1,(m)}\right\|_F\notag\\
&\leq \left\|\left(M^t-\eta\nabla_{M}f_{\aug}(M^t,F^t)\right)-\left(M^{t,(m)}-\eta\nabla_{M}f^{(m)}_{\aug}(M^{t,(m)},F^{t,(m)})\right)\right\|_F.
\end{align}
Thus, we only need to control the RHS of \eqref{ineq30:pr_lem_ncv2}.


Note that
\begin{align*}
&M^t-\eta\nabla_{M}f_{\aug}(M^t,F^t)
-
\left(
M^{t,(m)}-\eta\nabla_{M}f^{(m)}_{\aug}(M^{t,(m)},F^{t,(m)})
\right)\\
&=M^t-M^{t,(m)}-\eta\left(\nabla_{M}f_{\aug}(M^t,F^t)-\nabla_{M}f_{\aug}(M^{t,(m)},F^{t,(m)})\right)\\
&\quad +\eta\left(\nabla_{M}f^{(m)}_{\aug}(M^{t,(m)},F^{t,(m)})-\nabla_{M}f_{\aug}(M^{t,(m)},F^{t,(m)})\right)\\
&=M^t-M^{t,(m)}-\eta\left(\nabla_{M}f_{\aug}(M^t,F^tR^t)-\nabla_{M}f_{\aug}(M^{t,(m)},F^{t,(m)}O^{t,(m)})\right)\\
&\quad +\eta\left(\nabla_{M}f^{(m)}(M^{t,(m)},F^{t,(m)}O^{t,(m)})-\nabla_{M}f(M^{t,(m)},F^{t,(m)}O^{t,(m)})\right),
\end{align*}
% \begin{align*}
% &M^{t+1}-M^{t+1,(m)}\\
% &=M^t-\eta\nabla_{M}f_{\aug}(M^t,F^t)+\eta
% \begin{bmatrix}
% \mean\left(\nabla_{\theta}f(M^t,F^t)\right)\cdot\mathbf{1}\\
% 0
% \end{bmatrix}\\
% &\quad-
% \left(
% M^{t,(m)}-\eta\nabla_{M}f^{(m)}_{\aug}(M^{t,(m)},F^{t,(m)})+\eta
% \begin{bmatrix}
% \mean\left(\nabla_{\theta}f^{(m)}(M^{t,(m)},F^{t,(m)})\right)\cdot\mathbf{1}\\
% 0
% \end{bmatrix}
% \right)\\
% &=M^t-M^{t,(m)}-\eta\left(\nabla_{M}f_{\aug}(M^t,F^t)-\nabla_{M}f_{\aug}(M^{t,(m)},F^{t,(m)})\right)\\
% &\quad +\eta\left(\nabla_{M}f^{(m)}_{\aug}(M^{t,(m)},F^{t,(m)})-\nabla_{M}f_{\aug}(M^{t,(m)},F^{t,(m)})\right)\\
% &\quad+\eta
% \begin{bmatrix}
% \mean\left(\nabla_{\theta}f(M^t,F^t)-\nabla_{\theta}f^{(m)}(M^{t,(m)},F^{t,(m)})\right)\cdot\mathbf{1}\\
% 0
% \end{bmatrix}\\
% &=M^t-M^{t,(m)}-\eta\left(\nabla_{M}f_{\aug}(M^t,F^tR^t)-\nabla_{M}f_{\aug}(M^{t,(m)},F^{t,(m)}O^{t,(m)})\right)\\
% &\quad +\eta\left(\nabla_{M}f^{(m)}(M^{t,(m)},F^{t,(m)}O^{t,(m)})-\nabla_{M}f(M^{t,(m)},F^{t,(m)}O^{t,(m)})\right)\\
% &\quad+\eta
% \begin{bmatrix}
% \mean\left(\nabla_{\theta}f(M^t,F^tR^t)-\nabla_{\theta}f^{(m)}(M^{t,(m)},F^{t,(m)}O^{t,(m)})\right)\cdot\mathbf{1}\\
% 0
% \end{bmatrix},
% \end{align*}
and 
\begin{align*}
&F^{t+1}R^t-F^{t+1,(m)}O^{t,(m)}\\
&=F^{t}R^t-F^{t,(m)}O^{t,(m)}-\eta\left(\nabla_F f_{\aug}(M^t,F^tR^t)-\nabla_F f_{\aug}(M^{t,(m)},F^{t,(m)}O^{t,(m)})\right)\\
&\quad+\eta\left(\nabla_F f^{(m)}(M^{t,(m)},F^{t,(m)}O^{t,(m)})-\nabla_F f(M^{t,(m)},F^{t,(m)}O^{t,(m)})\right)\\
&\quad+\eta\left(\nabla_F f_{\diff}(M^t,F^tR^t)-\nabla_F f_{\diff}(M^{t,(m)},F^{t,(m)}O^{t,(m)})\right).
\end{align*}
As a result, we have
\begin{align*}
&\begin{bmatrix}
M^t-\eta\nabla_{M}f_{\aug}(M^t,F^t)
-
\left(
M^{t,(m)}-\eta\nabla_{M}f^{(m)}_{\aug}(M^{t,(m)},F^{t,(m)})
\right)\\
F^{t+1}R^t-F^{t+1,(m)}O^{t,(m)}
\end{bmatrix}\\
&=\underbrace{\left(I-\eta A\right)
\begin{bmatrix}
M^{t}-M^{t,(m)}\\
F^{t}R^t-F^{t,(m)}O^{t,(m)}
\end{bmatrix}}_{(1)}\\
&\quad +\eta\underbrace{\left(\nabla f^{(m)}(M^{t,(m)},F^{t,(m)}O^{t,(m)})-\nabla f(M^{t,(m)},F^{t,(m)}O^{t,(m)})\right)}_{(2)}\\
% &\quad+\eta
% \underbrace{\begin{bmatrix}
% \mean\left(\nabla_{\theta}f(M^t,F^tR^t)-\nabla_{\theta}f^{(m)}(M^{t,(m)},F^{t,(m)}O^{t,(m)})\right)\cdot\mathbf{1}\\
% 0
% \end{bmatrix}}_{(3)}\\
&\quad+\eta\underbrace{\left(\nabla_F f_{\diff}(M^t,F^tR^t)-\nabla_F f_{\diff}(M^{t,(m)},F^{t,(m)}O^{t,(m)})\right)}_{(3)}
\end{align*}
where
\begin{align*}
A=\int^1_0\nabla^2 f_{\aug}\left((M^{t,(m)},F^{t,(m)}O^{t,(m)})+\tau (M^t-M^{t,(m)},F^tR^t-F^{t,(m)}O^{t,(m)})\right)d\tau.
\end{align*}
In the following, we bound the Frobenius norm of (1)-(3), respectively.
\begin{enumerate}
\item  We first bound (1).
Since Lemma \ref{lem:ncv2} and Lemma \ref{lem:ncv4} hold for the $t$-th iteration, we have
\begin{align*}
&\left\|\theta^{t,(m)}+\tau\left(\theta^t-\theta^{t,(m)}\right)-\theta^*\right\|_{\infty}
\leq \|\theta^t-\theta^*\|_{\infty}+(1-\tau)\|\theta^{t,(m)}-\theta^t\|_{\infty}\leq c_{41}+c_{21}\leq c_1\\
&\left\|H^{t,(m)}+\tau\left(H^t-H^{t,(m)}\right)-H^*\right\|_{F}   \leq \|H^t-H^*\|_{F}+(1-\tau)\|H^{t,(m)}-H^t\|_{F}\leq c_{11}\sqrt{n}+c_{21}\leq c_2\sqrt{n}\\
&\left\|F^{t,(m)}O^{t,(m)}+\tau\left(F^tR^t-F^{t,(m)}O^{t,(m)}\right)-F^*\right\|_{2,\infty}   \\
&\quad\leq \|F^tR^t-F^*\|_{2,\infty}+(1-\tau)\|F^{t,(m)}O^{t,(m)}-F^tR^t\|_{2,\infty}\\
&\quad\leq \|F^tR^t-F^*\|_{2,\infty}+\|F^{t,(m)}O^{t,(m)}-F^tR^t\|_{F}\leq c_{43}+c_{21}\leq c_3.
\end{align*}
Moreover, we have $\mathbf{1}^T(\theta^t-\theta^{t,(m)})=0$ by the GD update and $\|F^{t}R^t-F^*\|\leq c_{14}\sqrt{n}\leq c_4\sqrt{n}$ by Lemma \ref{lem:ncv1} for the $t$-th iteration. Thus Lemma \ref{lem:convexity} can be applied to bound the Frobenius norm of (1). Follow the same argument as bounding term (1) in Appendix \ref{pf:lem_ncv1}, we have
\begin{align*}
\|(1)\|_F\leq \left(1-\frac{\underline{C}}{2}\eta\right)
\left\|
\begin{bmatrix}
M^{t}-M^{t,(m)}\\
F^{t}R^t-F^{t,(m)}O^{t,(m)}
\end{bmatrix}
\right\|_F
\end{align*}





\item  We then bound (2).
Note that
\begin{align*}
(2)&=\nabla L^{(m)}(M^{t,(m)},F^{t,(m)}O^{t,(m)})-\nabla L(M^{t,(m)},F^{t,(m)}O^{t,(m)})\\
&=\sum_{i\neq m}\left(\frac{e^{P_{im}^*}}{1+e^{P_{im}^*}}-A_{im}\right)
\begin{bmatrix}
\frac{1}{\sqrt{n}}(e_i+e_m)\\
z_iz_m^T\\
\frac1n e_ie_m^T Y^{t,(m)}O^{t,(m)}\\
\frac1n e_me_i^T X^{t,(m)}O^{t,(m)}
\end{bmatrix}
+
\sum_{i\neq m}\left(\frac{e^{P_{mi}^*}}{1+e^{P_{mi}^*}}-A_{mi}\right)
\begin{bmatrix}
\frac{1}{\sqrt{n}}(e_i+e_m)\\
z_mz_i^T\\
\frac1n e_me_i^T Y^{t,(m)}O^{t,(m)}\\
\frac1n e_ie_m^T X^{t,(m)}O^{t,(m)}
\end{bmatrix}.
\end{align*}
Since the first and second terms are similar, we only focus on bounding the Frobenius norm of the first term in the following.
It can be seen that
\begin{align*}
\left(\frac{1}{\sqrt{n}}\sum_{i\neq m}\left(\frac{e^{P_{im}^*}}{1+e^{P_{im}^*}}-A_{im}\right)(e_i+e_m)\right)_j=
\begin{cases} 
      \frac{1}{\sqrt{n}}\left(\frac{e^{P_{jm}^*}}{1+e^{P_{jm}^*}}-A_{jm}\right) & j\neq m \\
      \frac{1}{\sqrt{n}}\sum_{i\neq m}\left(\frac{e^{P_{im}^*}}{1+e^{P_{im}^*}}-A_{im}\right) & j=m 
   \end{cases}.
\end{align*}
Since $\sum_{i\neq m}\left(\frac{e^{P_{im}^*}}{1+e^{P_{im}^*}}-A_{im}\right) $ is the sum of $n-1$ i.i.d mean zero $1$-subgaussian random variables, we have with probability at least $1-n^{-10}$ that $|\sum_{i\neq m}\left(\frac{e^{P_{im}^*}}{1+e^{P_{im}^*}}-A_{im}\right)|\lesssim \sqrt{n\log n}$. This implies with probability at least $1-n^{-10}$ that
\begin{align}\label{ineq1:lem_ncv2}
\left\|\frac{1}{\sqrt{n}}\sum_{i\neq m}\left(\frac{e^{P_{im}^*}}{1+e^{P_{im}^*}}-A_{im}\right)(e_i+e_m)\right\|_2\lesssim \sqrt{\frac{n-1}{n}+\log n}\lesssim\sqrt{\log n}.
\end{align}
In the following, we apply matrix Berstein's inequality to bound the Frobenius norms of the rest of the terms.
Notice that
\begin{align*}
    &\max\Bigg\{\left\|\sum_{i\neq m}\bbE\left[\left(\frac{e^{P_{im}^*}}{1+e^{P_{im}^*}}-A_{im}\right)^2\vec(z_iz_m^T)\vec(z_iz_m^T)^T\right]\right\|,\\
    &\qquad\qquad\left\|\sum_{i\neq m}\bbE\left[\left(\frac{e^{P_{im}^*}}{1+e^{P_{im}^*}}-A_{im}\right)^2\vec(z_iz_m^T)^T\vec(z_iz_m^T)\right]\right\|\Bigg\}\\
    &\quad\leq \sum_{i\neq m}\|\vec(z_iz_m^T)\|_2^2=\sum_{i\neq m}\|z_iz_m^T\|_F^2=\sum_{i\neq m}\|z_i\|^2_2\|z_m\|_2^2\lesssim \frac{\sz^2}{n}.
\end{align*}
Thus by matrix Berstein's inequality, we have with probability at least $1-n^{-10}$ that
\begin{align}\label{ineq2:lem_ncv2}
  \left\|\sum_{i\neq m}\left(\frac{e^{P_{im}^*}}{1+e^{P_{im}^*}}-A_{im}\right)z_iz_m^T\right\|_F=\left\|\sum_{i\neq m}\left(\frac{e^{P_{im}^*}}{1+e^{P_{im}^*}}-A_{im}\right)\vec(z_iz_m^T)\right\|_2 \lesssim \sz\sqrt{\frac{\log n}{n}}.
\end{align}
Notice that
\begin{align*}
    &\max\Bigg\{\left\|\sum_{i\neq m}\bbE\left[\left(\frac{e^{P_{im}^*}}{1+e^{P_{im}^*}}-A_{im}\right)^2\vec(e_me_i^T Y^{t,(m)}O^{t,(m)})\vec(e_me_i^T Y^{t,(m)}O^{t,(m)})^T\right]\right\|,\\
    &\qquad\qquad\left\|\sum_{i\neq m}\bbE\left[\left(\frac{e^{P_{im}^*}}{1+e^{P_{im}^*}}-A_{im}\right)^2\vec(e_me_i^T Y^{t,(m)}O^{t,(m)})^T\vec(e_me_i^T Y^{t,(m)}O^{t,(m)})\right]\right\|\Bigg\}\\
    &\quad\leq \sum_{i\neq m}\|\vec(e_me_i^T Y^{t,(m)}O^{t,(m)})\|_2^2\\
    &\quad=\sum_{i\neq m}\|e_me_i^T Y^{t,(m)}O^{t,(m)}\|_F^2\\
    &\quad=\sum_{i\neq m}\Tr\left(e_me_i^T Y^{t,(m)}(Y^{t,(m)})^{T}e_i e_m^T\right)\\
    &\quad = \sum_{i\neq m}\left( Y^{t,(m)}(Y^{t,(m)})^{T}\right)_{ii}\\
    &\quad \leq \|Y^{t,(m)}\|_F^2\\
    &\quad\leq (\|Y^{t,(m)}O^{t,(m)}-Y^{t}R^t\|_F+\|Y^{t}R^t-Y^*\|_F+\|Y^*\|_F)^2\lesssim \mu r\sigma_{\max},
\end{align*}
where the last equation follows from Assumption \ref{assumption:incoherent} and the fact that Lemma \ref{lem:ncv1} and Lemma \ref{lem:ncv2} hold for the $t$-th iteration.
Thus by matrix Berstein's inequality, we have with probability at least $1-n^{-10}$ that
\begin{align}\label{ineq3:lem_ncv2}
  \left\|\frac1n\sum_{i\neq m}\left(\frac{e^{P_{im}^*}}{1+e^{P_{im}^*}}-A_{im}\right)e_me_i^T Y^{t,(m)}O^{t,(m)}\right\|_F&=\left\|\frac1n\sum_{i\neq m}\left(\frac{e^{P_{im}^*}}{1+e^{P_{im}^*}}-A_{im}\right)\vec(e_me_i^T Y^{t,(m)}O^{t,(m)})\right\|_2  \notag\\
  &\lesssim \frac{\sqrt{\mu r \sigma_{\max}\log n}}{n}.
\end{align}
Similarly, we have with probability at least $1-n^{-10}$ that
\begin{align}\label{ineq4:lem_ncv2}
  \left\|\frac1n\sum_{i\neq m}\left(\frac{e^{P_{im}^*}}{1+e^{P_{im}^*}}-A_{im}\right)e_ie_m^T X^{t,(m)}O^{t,(m)}\right\|_F\lesssim \frac{\sqrt{\mu r \sigma_{\max}\log n}}{n}.
\end{align}
Combine \eqref{ineq1:lem_ncv2}, \eqref{ineq2:lem_ncv2}, \eqref{ineq3:lem_ncv2} and \eqref{ineq4:lem_ncv2}, we conclude that $ \|(2)\|_F\lesssim \frac{\sqrt{\mu r \sigma_{\max}\log n}}{n}$.
% \begin{align*}
%     \|(2)\|_F\leq O(\sqrt{\log n}).
% \end{align*}
\item  We then bound (3). 
Notice that
\begin{align*}
\|F^{t,(m)}\|=\|F^{t,(m)}O^{t,(m)}\|\leq \|F^{t,(m)}O^{t,(m)}-F^tR^t\|+\|F^tR^t-F^*\|+\|F^*\|\leq 2\|F^*\|.
\end{align*}
Then following the same argument as bounding term (2) in Appendix \ref{pf:lem_ncv1}, we have
\begin{align*}
&\|\nabla_F f_{\diff}(M^t,F^tR^t)\|_F\lesssim\frac{c_{\aug}}{n^2}\|F^*\|\|X^{tT}X^t-Y^{tT}Y^t\|_F,\\
&\|\nabla_F f_{\diff}(M^{t,(m)},F^{t,(m)}O^{t,(m)})\|_F\lesssim\frac{c_{\aug}}{n^2}\|F^*\|\|X^{t,(m)T}X^{t,(m)}-Y^{t,(m)T}Y^{t,(m)}\|_F.
\end{align*}
Thus, it holds that
\begin{align*}
\|(3)\|_F&\lesssim \frac{c_{\aug}}{n^2}\|F^*\|\left(\|X^{tT}X^t-Y^{tT}Y^t\|_F+\|X^{t,(m)T}X^{t,(m)}-Y^{t,(m)T}Y^{t,(m)}\|_F\right)\\
&\lesssim \eta c_{51} c_{\aug}\sqrt{\sigma_{\max}}.
\end{align*}

% \item  Finally, we bound (4).
% \textcolor{red}{
% Here 
% \begin{align*}
% (4):= 
% \begin{bmatrix}
% \mean\left(\nabla_{\theta}f(M^t,F^tR^t)-\nabla_{\theta}f^{(m)}(M^{t,(m)},F^{t,(m)}O^{t,(m)})\right)\cdot\mathbf{1}\\
% 0
% \end{bmatrix}.
% \end{align*}
% At the beginning of the proof, we already removed this term by considering the projection. Thus, the bound on this term is no longer needed. But we still keep it here in case other parts need this proof.
% }

% Note that
% \begin{align*}
% \|(4)\|_F
% &=\sqrt{n}\left|\mean\left(\nabla_{\theta}f(M^t,F^tR^t)-\nabla_{\theta}f^{(m)}(M^{t,(m)},F^{t,(m)}O^{t,(m)})\right)\right|\\
% &=\sqrt{n}\left|\mean\left(\nabla_{\theta}L(M^t,F^tR^t)-\nabla_{\theta}L^{(m)}(M^{t,(m)},F^{t,(m)}O^{t,(m)})\right)\right|\\
% &\leq \sqrt{n}\left|\mean\left(\nabla_{\theta}L(M^t,F^tR^t)-\nabla_{\theta}L(M^{t,(m)},F^{t,(m)}O^{t,(m)})\right)\right|\\
% &\quad+\sqrt{n}\left|\mean\left(\nabla_{\theta}L(M^{t,(m)},F^{t,(m)}O^{t,(m)})-\nabla_{\theta}L^{(m)}(M^{t,(m)},F^{t,(m)}O^{t,(m)})\right)\right|\\
% \end{align*}
% For the first term, follow the same argument as bounding term (4) in Appendix \ref{pf:lem_ncv1}, we have
% \begin{align*}
% & \sqrt{n}\left|\mean\left(\nabla_{\theta}L(M^t,F^tR^t)-\nabla_{\theta}L(M^{t,(m)},F^{t,(m)}O^{t,(m)})\right)\right|\\
% &\lesssim \|\theta^t-\theta^{t,(m)}\|_2+\|H^t-H^{t,(m)}\|_F+\frac{1}{n}\|X^*\|\|F^tR^t-F^{t,(m)}O^{t,(m)}\|_F.
% \end{align*}
% For the second term, note that
% \begin{align*}
%  &\nabla_{\theta}L(M^{t,(m)},F^{t,(m)}O^{t,(m)})-\nabla_{\theta}L^{(m)}(M^{t,(m)},F^{t,(m)}O^{t,(m)})\\
%  &=\frac{2}{\sqrt{n}}\sum_{i\neq m}\left(\frac{e^{P_{im}^*}}{1+e^{P_{im}^*}}-A_{im}\right)(e_i+e_m).
% \end{align*}
% Using the argument as bounding term (2) in this proof, we have
% \begin{align*}
% &\sqrt{n}\left|\mean\left(\nabla_{\theta}L(M^{t,(m)},F^{t,(m)}O^{t,(m)})-\nabla_{\theta}L^{(m)}(M^{t,(m)},F^{t,(m)}O^{t,(m)})\right)\right|\\
% &\lesssim \frac{1}{\sqrt{n}}\left(\frac{n-1}{\sqrt{n}}+\sqrt{\log n}\right)=O(1).
% \end{align*}
% As a result, we conclude that 
% \begin{align*}
% \|(4)\|_F\lesssim \|\theta^t-\theta^{t,(m)}\|_2+\|H^t-H^{t,(m)}\|_F+\frac{1}{n}\|X^*\|\|F^tR^t-F^{t,(m)}O^{t,(m)}\|_F+O(1).
% \end{align*}
\end{enumerate}

Combine the bounds of Frobenius norm of (1)-(3), we conclude that
\begin{align*}
&\left\|\begin{bmatrix}
M^t-\eta\nabla_{M}f_{\aug}(M^t,F^t)
-
\left(
M^{t,(m)}-\eta\nabla_{M}f^{(m)}_{\aug}(M^{t,(m)},F^{t,(m)})
\right)\\
F^{t+1}R^t-F^{t+1,(m)}O^{t,(m)}
\end{bmatrix}\right\|_F\\
&\leq \left(1-\frac{\underline{C}}{2}\eta\right)
\left\|
\begin{bmatrix}
M^{t}-M^{t,(m)}\\
F^{t}R^t-F^{t,(m)}O^{t,(m)}
\end{bmatrix}
\right\|_F
+c\eta\frac{\sqrt{\mu r \sigma_{\max}\log n}}{n}+c\eta^2 c_{51} c_{\aug}\sqrt{\sigma_{\max}}\\
&\leq \left(1-\frac{\underline{C}}{2}\eta\right)
c_{21}
+c\eta\frac{\sqrt{\mu r \sigma_{\max}\log n}}{n}+c\eta^2 c_{51} c_{\aug}\sqrt{\sigma_{\max}}\\
&\leq c_{21}
\end{align*}
as long as $\frac{\sqrt{\mu r \sigma_{\max}\log n}}{\underline{C}n}\lesssim c_{21}$ and $\eta\ll \frac{\underline{C}c_{21}}{c_{51} c_{\aug}\sqrt{\sigma_{\max}}}$.
By \eqref{ineq30:pr_lem_ncv2} and Claim \ref{claim:lem_ncv2}, we further have
\begin{align*}
\left\|
\begin{bmatrix}
M^{t+1}-M^{t+1,(m)}\\
F^{t+1}R^{t+1}-F^{t+1,(m)}O^{t+1,(m)}
\end{bmatrix}
\right\|_F \leq c_{21}.
\end{align*}
Finally, by the arbitrariness of $m$, we finish the proofs.









\subsection{Proofs of Lemma \ref{lem:ncv3}}\label{pf:lem_ncv3}
Suppose Lemma \ref{lem:ncv1}-Lemma \ref{lem:ncv5} hold for the $t$-th iteration. In the following, we prove Lemma \ref{lem:ncv3} for the $(t+1)$-th iteration. 
Note that by the gradient descent update, we have
\begin{align*}
&\theta^{t+1,(m)}_m-\theta^*_m\\
&=\theta^{t,(m)}_m-\theta^*_m
-\frac{2\eta}{\sqrt{n}}\sum_{i\neq m}\left(\frac{e^{P^{t,(m)}_{im}}}{1+e^{P^{t,(m)}_{im}}}-\frac{e^{P^{*}_{im}}}{1+e^{P^{*}_{im}}}\right)+\eta\cdot\mean\left(\nabla_{\theta}L^{(m)}(M^{t,(m)}, F^{t,(m)})\right),
\end{align*}
where we use the symmetry of $X^{t,(m)}(Y^{t,(m)})^T$ obtained via Lemma \ref{lem:ncv5}.
By the mean value theorem, we have for some $\{c_i\}$ that
\begin{align*}
& \sum_{i\neq m}\left(\frac{e^{P^{t,(m)}_{im}}}{1+e^{P^{t,(m)}_{im}}}-\frac{e^{P^{*}_{im}}}{1+e^{P^{*}_{im}}}\right)\\
&= \sum_{i\neq m}\frac{e^{c_i}}{(1+e^{c_i})^2}\left(P^{t,(m)}_{im}-P^{*}_{im}\right)\\
& = \sum_{i\neq m}\frac{e^{c_i}}{(1+e^{c_i})^2}\left(\frac{1}{\sqrt{n}}\left(\theta^{t,(m)}_i-\theta^{*}_i+\theta^{t,(m)}_m-\theta^{*}_m\right)+\langle H^{t,(m)}-H^*,z_iz_m^T\rangle+\frac1n \left(X^{t,(m)}(Y^{t,(m)})^T-X^{*}Y^{*T}\right)_{im}\right)\\
& = \left(\frac{1}{\sqrt{n}}\sum_{i\neq m}\frac{e^{c_i}}{(1+e^{c_i})^2}\right)\left(\theta^{t,(m)}_m-\theta^{*}_m\right)\\
&\quad+\sum_{i\neq m}\frac{e^{c_i}}{(1+e^{c_i})^2}\left(\frac{1}{\sqrt{n}}\left(\theta^{t,(m)}_i-\theta^{*}_i\right)+\langle H^{t,(m)}-H^*,z_iz_m^T\rangle+\frac1n \left(X^{t,(m)}(Y^{t,(m)})^T-X^{*}Y^{*T}\right)_{im}\right).
\end{align*}
Thus, it holds that
\begin{align}\label{eq1:lem_ncv3}
 &\theta^{t+1,(m)}_m-\theta^*_m\notag\\
 &=\left(1-\frac{2\eta}{n}\sum_{i\neq m}\frac{e^{c_i}}{(1+e^{c_i})^2}\right)\left(\theta^{t,(m)}_m-\theta^*_m\right)
+\eta\cdot\mean\left(\nabla_{\theta}L^{(m)}(M^{t,(m)}, F^{t,(m)})\right)\notag\\
&\quad -\frac{2\eta}{\sqrt{n}}\sum_{i\neq m}\frac{e^{c_i}}{(1+e^{c_i})^2}\left(\frac{1}{\sqrt{n}}\left(\theta^{t,(m)}_i-\theta^{*}_i\right)+\langle H^{t,(m)}-H^*,z_iz_m^T\rangle+\frac1n \left(X^{t,(m)}(Y^{t,(m)})^T-X^{*}Y^{*T}\right)_{im}\right)\notag\\
&=\left(1-\frac{2\eta}{n}\sum_{i\neq m}\frac{e^{c_i}}{(1+e^{c_i})^2}\right)\left(\theta^{t,(m)}_m-\theta^*_m\right)
+\eta\cdot\mean\left(\nabla_{\theta}L^{(m)}(M^{t,(m)}, F^{t,(m)})\right)\notag\\
&\quad -\frac{2\eta}{\sqrt{n}}\sum_{i\neq m}\frac{e^{c_i}}{(1+e^{c_i})^2}\left(\frac{1}{\sqrt{n}}\left(\theta^{t,(m)}_i-\theta^{*}_i\right)+\langle H^{t,(m)}-H^*,z_iz_m^T\rangle\right)\notag\\
&\quad -\frac{\eta}{n^{3/2}}\sum_{i\neq m}\frac{e^{c_i}}{(1+e^{c_i})^2}\left(X^{t,(m)}(Y^{t,(m)})^T-X^{*}Y^{*T}\right)_{im}\notag\\
&\quad -\frac{\eta}{n^{3/2}}\sum_{i\neq m}\frac{e^{c_i}}{(1+e^{c_i})^2}\left(X^{t,(m)}(Y^{t,(m)})^T-X^{*}Y^{*T}\right)_{mi},
\end{align}
where the last equation follows from the symmetry property.
Notice that
\begin{align*}
& X^{t,(m)}(Y^{t,(m)})^T-X^{*}Y^{*T}\notag\\
&=\left(X^{t,(m)}R^{t,(m)}-X^{*}\right)\left(Y^{t,(m)}R^{t,(m)}\right)^T+X^*\left(Y^{t,(m)}R^{t,(m)}-Y^{*}\right)^T\notag\\
&=\left(X^{t,(m)}R^{t,(m)}\right)\left(Y^{t,(m)}R^{t,(m)}-Y^{*}\right)^T+\left(X^{t,(m)}R^{t,(m)}-X^{*}\right)\left(Y^{*}\right)^T.
\end{align*}
Thus, we have
\begin{align*}
&\left(X^{t,(m)}(Y^{t,(m)})^T-X^{*}Y^{*T}\right)_{im}\\
&=\left(X^{t,(m)}R^{t,(m)}-X^{*}\right)_{i,\cdot}^{\top}\left(Y^{t,(m)}R^{t,(m)}\right)_{m,\cdot}+(X^*_{i,\cdot})^{\top}\left(Y^{t,(m)}R^{t,(m)}-Y^{*}\right)_{m,\cdot},
\end{align*}
and
\begin{align*}
&\left(X^{t,(m)}(Y^{t,(m)})^T-X^{*}Y^{*T}\right)_{mi}\\
&=\left(Y^{t,(m)}R^{t,(m)}-Y^{*}\right)_{i,\cdot}^{\top}\left(X^{t,(m)}R^{t,(m)}\right)_{m,\cdot}+\left(Y^{*}_{i,\cdot}\right)^T\left(X^{t,(m)}R^{t,(m)}-X^{*}\right)_{m,\cdot}.
\end{align*}
By \eqref{eq1:lem_ncv3}, we obtain
\begin{align}\label{eq11:lem_ncv3}
 &\theta^{t+1,(m)}_m-\theta^*_m\notag\\
&=\left(1-\frac{2\eta}{n}\sum_{i\neq m}\frac{e^{c_i}}{(1+e^{c_i})^2}\right)\left(\theta^{t,(m)}_m-\theta^*_m\right)\notag\\
&
-\frac{\eta}{n^{3/2}}\sum_{i\neq m}\frac{e^{c_i}}{(1+e^{c_i})^2}\left(Y^{*}_{i,\cdot}\right)^T\left(X^{t,(m)}R^{t,(m)}-X^{*}\right)_{m,\cdot}
-\frac{\eta}{n^{3/2}}\sum_{i\neq m}\frac{e^{c_i}}{(1+e^{c_i})^2}(X^*_{i,\cdot})^{\top}\left(Y^{t,(m)}R^{t,(m)}-Y^{*}\right)_{m,\cdot}\notag\\
&\quad+\eta\cdot\mean\left(\nabla_{\theta}L^{(m)}(M^{t,(m)}, F^{t,(m)})\right)-\frac{2\eta}{\sqrt{n}}\sum_{i\neq m}\frac{e^{c_i}}{(1+e^{c_i})^2}\left(\frac{1}{\sqrt{n}}\left(\theta^{t,(m)}_i-\theta^{*}_i\right)+\langle H^{t,(m)}-H^*,z_iz_m^T\rangle\right)\notag\\
&\quad -\frac{\eta}{n^{3/2}}\sum_{i\neq m}\frac{e^{c_i}}{(1+e^{c_i})^2}\left(X^{t,(m)}R^{t,(m)}-X^{*}\right)_{i,\cdot}^{\top}\left(Y^{t,(m)}R^{t,(m)}\right)_{m,\cdot}
\notag\\
&\quad -\frac{\eta}{n^{3/2}}\sum_{i\neq m}\frac{e^{c_i}}{(1+e^{c_i})^2}\left(Y^{t,(m)}R^{t,(m)}-Y^{*}\right)_{i,\cdot}^{\top}\left(X^{t,(m)}R^{t,(m)}\right)_{m,\cdot}\notag\\
&=\left(1-\frac{2\eta}{n}\sum_{i\neq m}\frac{e^{c_i}}{(1+e^{c_i})^2}\right)\left(\theta^{t,(m)}_m-\theta^*_m\right)
-\frac{\eta}{n^{3/2}}\sum_{i\neq m}\frac{e^{c_i}}{(1+e^{c_i})^2}\left(Y^{*}_{i,\cdot}\right)^T\left(X^{t,(m)}R^{t,(m)}-X^{*}\right)_{m,\cdot}\notag\\
&\quad-\frac{\eta}{n^{3/2}}\sum_{i\neq m}\frac{e^{c_i}}{(1+e^{c_i})^2}(X^*_{i,\cdot})^{\top}\left(Y^{t,(m)}R^{t,(m)}-Y^{*}\right)_{m,\cdot}+r_1,
\end{align}
where 
\begin{align*}
r_1&:=\eta\cdot\mean\left(\nabla_{\theta}L^{(m)}(M^{t,(m)}, F^{t,(m)})\right)-\frac{2\eta}{\sqrt{n}}\sum_{i\neq m}\frac{e^{c_i}}{(1+e^{c_i})^2}\left(\frac{1}{\sqrt{n}}\left(\theta^{t,(m)}_i-\theta^{*}_i\right)+\langle H^{t,(m)}-H^*,z_iz_m^T\rangle\right)\notag\\
&\quad -\frac{\eta}{n^{3/2}}\sum_{i\neq m}\frac{e^{c_i}}{(1+e^{c_i})^2}\left(X^{t,(m)}R^{t,(m)}-X^{*}\right)_{i,\cdot}^{\top}\left(Y^{t,(m)}R^{t,(m)}\right)_{m,\cdot}
\notag\\
&\quad -\frac{\eta}{n^{3/2}}\sum_{i\neq m}\frac{e^{c_i}}{(1+e^{c_i})^2}\left(Y^{t,(m)}R^{t,(m)}-Y^{*}\right)_{i,\cdot}^{\top}\left(X^{t,(m)}R^{t,(m)}\right)_{m,\cdot}
\end{align*}
In the following, we bound $|r_1|$.
\begin{enumerate}
\item  For the first term, note that
\begin{align*}
&\left|\mean\left(\nabla_{\theta}L^{(m)}(M^{t,(m)}, F^{t,(m)})\right)\right|\\
&=\left|\mean\left(\nabla_{\theta}L^{(m)}(M^{t,(m)}, F^{t,(m)}O^{t,(m)})\right)\right|\\
&\leq \left|\mean\left(\nabla_{\theta}L^{(m)}(M^{t,(m)}, F^{t,(m)}O^{t,(m)})-\nabla_{\theta}L(M^{t}, F^{t}R^{t})\right)\right|+ \left|\mean\left(\nabla_{\theta}L(M^{t}, F^{t}R^{t})\right)\right|.
\end{align*}
For the first part, we have the following claim.
\begin{claim}\label{claim1:gradient_mean}
It holds that
\begin{align*}
 & \left|\mean\left(\nabla_{\theta}L^{(m)}(M^{t,(m)}, F^{t,(m)}O^{t,(m)})-\nabla_{\theta}L(M^{t}, F^{t}R^{t})\right)\right|\\
 & \lesssim   \sqrt{\frac{\su}{n}}\left(\|\theta^t-\theta^{t,(m)}\|_2+\|H^t-H^{t,(m)}\|_F+\frac{1}{n}\|X^*\|\|F^tR^t-F^{t,(m)}O^{t,(m)}\|_F\right)+\sqrt{\frac{\log n}{n}}.
\end{align*}
\end{claim}
\begin{proof}[Proof of Claim \ref{claim1:gradient_mean}]
 Note that
\begin{align*}
&\left|\mean\left(\nabla_{\theta}L(M^t,F^tR^t)-\nabla_{\theta}L^{(m)}(M^{t,(m)},F^{t,(m)}O^{t,(m)})\right)\right|\\
&\leq\left|\mean\left(\nabla_{\theta}L(M^t,F^tR^t)-\nabla_{\theta}L(M^{t,(m)},F^{t,(m)}O^{t,(m)})\right)\right|\\
&\quad+\left|\mean\left(\nabla_{\theta}L(M^{t,(m)},F^{t,(m)}O^{t,(m)})-\nabla_{\theta}L^{(m)}(M^{t,(m)},F^{t,(m)}O^{t,(m)})\right)\right|\\
\end{align*}
For the first term, we have
\begin{align*}
&\mean\left(\nabla_{\theta}L(M^t,F^tR^t)-\nabla_{\theta}L(M^{t,(m)},F^{t,(m)}O^{t,(m)})\right)\\
&=\frac{2}{n^{3/2}}\sum_{i\neq j}\left(\frac{e^{P_{ij}^{t}}}{1+e^{P_{ij}^{t}}}-\frac{e^{P_{ij}^{t,(m)}}}{1+e^{P_{ij}^{t,(m)}}}\right)\\
&\leq \frac{1}{2n^{3/2}}\sum_{i\neq j}\left|P^t_{ij}-P^{t,(m)}_{ij}\right| \tag{by mean-value theorem}\\
&\leq \frac{1}{2\sqrt{n}}\sqrt{\sum_{i\neq j}\left|P^t_{ij}-P^{t,(m)}_{ij}\right|^2}. \tag{by Cauchy-Schwarz}
\end{align*}

Note that
\begin{align*}
&\sum_{i\neq j}(P_{ij}^{t}-P_{ij}^{t,(m)})^2\\
&=\sum_{i\neq j}\left(\frac{1}{\sqrt{n}}\langle\theta^{t}-\theta^{t,(m)},e_i+e_j\rangle+\langle H^{t}-H^{t,(m)},z_iz_j^T\rangle+\frac1n\langle X^{t}Y^{tT}-X^{t,(m)}Y^{t,(m) T},e_i e_j^T\rangle\right)^2\\
&=
\begin{bmatrix}
  \vec(\theta^{t}-\theta^{t,(m)})\\
  \vec(H^{t}-H^{t,(m)})\\
  \frac1n\vec(X^{t}Y^{tT}-X^{t,(m)}Y^{t,(m) T})
\end{bmatrix}^T
\left(\sum_{i\neq j}
  \begin{bmatrix}
  \frac{1}{\sqrt{n}}\vec(e_i+e_j)\\
  \vec(z_iz_j^T)\\
  \vec(e_ie_j^T)
  \end{bmatrix}
   \begin{bmatrix}
  \frac{1}{\sqrt{n}}\vec(e_i+e_j)\\
  \vec(z_iz_j^T)\\
  \vec(e_ie_j^T)
  \end{bmatrix}^T
\right)
\begin{bmatrix}
  \vec(\theta^{t}-\theta^{t,(m)})\\
  \vec(H^{t}-H^{t,(m)})\\
  \frac1n\vec(X^{t}Y^{tT}-X^{t,(m)}Y^{t,(m) T})
\end{bmatrix}\\
&\leq \su \left\|\begin{bmatrix}
  \vec(\theta^{t}-\theta^{t,(m)})\\
  \vec(H^{t}-H^{t,(m)})\\
  \frac1n\vec(X^{t}Y^{tT}-X^{t,(m)}Y^{t,(m) T})
\end{bmatrix}\right\|^2 \tag{by Assumption \ref{assumption:eigenvalues} and $\mathbf{1}^T(\theta^t-\theta^{t,(m)})=0$}\\
& =\su\left(\|\theta^t-\theta^{t,(m)}\|^2_{2}+\|H^t-H^{t,(m)}\|^2_{F}+\frac{1}{n^2}\|X^tY^{tT}-X^{t,(m)}Y^{t,(m) T}\|^2_{F}\right).
\end{align*}
As a result, we have
\begin{align*}
&\left|\mean\left(\nabla_{\theta}L(M^t,F^tR^t)-\nabla_{\theta}L(M^{t,(m)},F^{t,(m)}O^{t,(m)})\right)\right|\\
&\lesssim \sqrt{\frac{\su}{n}}\left(\|\theta^t-\theta^{t,(m)}\|_{2}+\|H^t-H^{t,(m)}\|_{F}+\frac{1}{n}\|X^tY^{tT}-X^{t,(m)}Y^{t,(m) T}\|_{F}\right)\\
&\lesssim \sqrt{\frac{\su}{n}}\left(\|\theta^t-\theta^{t,(m)}\|_2+\|H^t-H^{t,(m)}\|_F+\frac{1}{n}\|X^*\|\|F^tR^t-F^{t,(m)}O^{t,(m)}\|_F\right).
\end{align*}

For the second term, note that
\begin{align*}
 &\nabla_{\theta}L(M^{t,(m)},F^{t,(m)}O^{t,(m)})-\nabla_{\theta}L^{(m)}(M^{t,(m)},F^{t,(m)}O^{t,(m)})\\
 &=\frac{2}{\sqrt{n}}\sum_{i\neq m}\left(\frac{e^{P_{im}^*}}{1+e^{P_{im}^*}}-A_{im}\right)(e_i+e_m).
\end{align*}
Thus, we have
\begin{align*}
&\left|\mean\left(\nabla_{\theta}L(M^{t,(m)},F^{t,(m)}O^{t,(m)})-\nabla_{\theta}L^{(m)}(M^{t,(m)},F^{t,(m)}O^{t,(m)})\right)\right|\\
&\leq \frac1n \left\|\frac{2}{\sqrt{n}}\sum_{i\neq m}\left(\frac{e^{P_{im}^*}}{1+e^{P_{im}^*}}-A_{im}\right)(e_i+e_m)\right\|_1\\
&\leq \frac{1}{\sqrt{n}}\left\|\frac{2}{\sqrt{n}}\sum_{i\neq m}\left(\frac{e^{P_{im}^*}}{1+e^{P_{im}^*}}-A_{im}\right)(e_i+e_m)\right\|_2\\
&\lesssim \sqrt{\frac{\log n}{n}} \tag{by \eqref{ineq1:lem_ncv2}}.
\end{align*}
Combining the above two terms, we then finish the proof.  
\end{proof}

For the second part, we have the following claim.
\begin{claim}\label{claim2:gradient_mean}
It holds that
\begin{align*}
 & \left|\mean\left(\nabla_{\theta}L(M^{t}, F^{t}R^{t})\right)\right|\\
 & \lesssim  \sqrt{\frac{\su}{n}}\left(\|\theta^t-\theta^{*}\|_{2}+\|H^t-H^{*}\|_{F}+\frac{1}{n}\|X^*\|\|F^tR^t-F^{*}\|_{F}\right)+\sqrt{\frac{\log n}{n}}.
\end{align*}
\end{claim}
\begin{proof}[Proof of Claim \ref{claim2:gradient_mean}]
Note that
\begin{align*}
\nabla_{\theta}L(M^t,F^tR^t)=\nabla_{\theta}L(M^*,F^*)+\nabla_{\theta}L(M^t,F^tR^t)-\nabla_{\theta}L(M^*,F^*).
\end{align*}
For the first term, by Lemma \ref{lem:gradient_norm}, we have
\begin{align*}
\left| \mean\left(\nabla_{\theta}L(M^*,F^*)\right)\right|\leq \frac{1}{\sqrt{n}}\left\|\nabla_{\theta}L(M^*,F^*)\right\|_2\lesssim \sqrt{\frac{\log n}{n}}.
\end{align*}
For the rest of the terms, same as the proof of Claim \ref{claim1:gradient_mean}, we have
\begin{align*}
\left|\mean\left(\nabla_{\theta}L(M^t,F^tR^t)-\nabla_{\theta}L(M^*,F^*)\right)\right|
\lesssim \sqrt{\frac{\su}{n}}\left(\|\theta^t-\theta^{*}\|_{2}+\|H^t-H^{*}\|_{F}+\frac{1}{n}\|X^*\|\|F^tR^t-F^{*}\|_{F}\right).
\end{align*}
Combining the above two terms, we then finish the proof.


% For the rest of the terms, we have 
% \begin{align*}
% &n\cdot \mean\left(\nabla_{\theta}L(M^t,F^tR^t)-\nabla_{\theta}L(M^*,F^*)\right)\\
% &=\frac{2}{\sqrt{n}}\sum_{i\neq j}\left(\frac{e^{P_{ij}^{t}}}{1+e^{P_{ij}^{t}}}-\frac{e^{P_{ij}^{*}}}{1+e^{P_{ij}^{*}}}\right)\\
% &\leq \frac{1}{2\sqrt{n}}\sum_{i\neq j}\left|P^t_{ij}-P^{*}_{ij}\right| \tag{by mean-value theorem}\\
% &\leq \frac{\sqrt{n}}{2}\sqrt{\sum_{i\neq j}\left|P^t_{ij}-P^{*}_{ij}\right|^2}. \tag{by Cauchy-Schwarz}
% \end{align*}
% Note that
% \begin{align*}
% &\sum_{i\neq j}(P_{ij}^{t}-P_{ij}^*)^2\\
% &=\sum_{i\neq j}\left(\frac{1}{\sqrt{n}}\langle\theta^{t}-\theta^*,e_i+e_j\rangle+\langle H^{t}-H^*,z_iz_j^T\rangle+\frac1n\langle X^{t}Y^{tT}-X^*Y^{*T},e_i e_j^T\rangle\right)^2\\
% &=
% \begin{bmatrix}
%   \vec(\theta^{t}-\theta^*)\\
%   \vec(H^{t}-H^*)\\
%   \frac1n\vec(X^{t}Y^{tT}-X^*Y^{*T})
% \end{bmatrix}^T
% \left(\sum_{i\neq j}
%   \begin{bmatrix}
%   \frac{1}{\sqrt{n}}\vec(e_i+e_j)\\
%   \vec(z_iz_j^T)\\
%   \vec(e_ie_j^T)
%   \end{bmatrix}
%    \begin{bmatrix}
%   \frac{1}{\sqrt{n}}\vec(e_i+e_j)\\
%   \vec(z_iz_j^T)\\
%   \vec(e_ie_j^T)
%   \end{bmatrix}^T
% \right)
% \begin{bmatrix}
%   \vec(\theta^{t}-\theta^*)\\
%   \vec(H^{t}-H^*)\\
%   \frac1n\vec(X^{t}Y^{tT}-X^*Y^{*T})
% \end{bmatrix}\\
% &\lesssim \left\|\begin{bmatrix}
%   \vec(\theta^{t}-\theta^*)\\
%   \vec(H^{t}-H^*)\\
%   \frac1n\vec(X^{t}Y^{tT}-X^*Y^{*T})
% \end{bmatrix}\right\|^2 \tag{by balanced eigenvalues assumption and $\mathbf{1}^T(\theta^t-\theta^*)=0$}\\
% & =\|\theta^t-\theta^{*}\|^2_{2}+\|H^t-H^{*}\|^2_{F}+\frac{1}{n^2}\|X^tY^{tT}-X^{*}Y^{*T}\|^2_{F}.
% \end{align*}
% As a result, we have
% \begin{align*}
% \left|\mean\left(\nabla_{\theta}L(M^t,F^tR^t)-\nabla_{\theta}L(M^*,F^*)\right)\right|
% \lesssim \frac{1}{\sqrt{{n}}}\left(\|\theta^t-\theta^{*}\|_{2}+\|H^t-H^{*}\|_{F}+\frac{1}{n}\|X^tY^{tT}-X^{*}Y^{*T}\|_{F}\right).
% \end{align*}
% Combine the above results, we show that
% \begin{align*}
%  \left|\mean\left(\nabla_{\theta}f(M^t,F^tR^t)\right)\right| 
%  \lesssim O\left(\sqrt{\frac{\log n}{n}}\right)+\frac{1}{\sqrt{{n}}}\left(\|\theta^t-\theta^{*}\|_{2}+\|H^t-H^{*}\|_{F}+\frac{1}{n}\|X^tY^{tT}-X^{*}Y^{*T}\|_{F}\right),
% \end{align*}
% which implies
% \begin{align*}
%  (4)
%  \lesssim O\left(\sqrt{\log n}\right)+\|\theta^t-\theta^{*}\|_{2}+\|H^t-H^{*}\|_{F}+\frac{1}{n}\|X^tY^{tT}-X^{*}Y^{*T}\|_{F}.
% \end{align*}
\end{proof}

By Claim \ref{claim1:gradient_mean} and \ref{claim2:gradient_mean}, we have
\begin{align}\label{ineq1:lem_ncv3}
&\left|\mean\left(\nabla_{\theta}L^{(m)}(M^{t,(m)}, F^{t,(m)})\right)\right|\notag\\
&\lesssim \sqrt{\frac{\su}{n}}\left(\|\theta^t-\theta^{t,(m)}\|_2+\|H^t-H^{t,(m)}\|_F+\frac{1}{n}\|X^*\|\|F^tR^t-F^{t,(m)}O^{t,(m)}\|_F\right)\notag\\
&\quad + \sqrt{\frac{\su}{n}}\left(\|\theta^t-\theta^{*}\|_{2}+\|H^t-H^{*}\|_{F}+\frac{1}{n}\|X^*\|\|F^tR^t-F^*\|_F\right)+O\left(\sqrt{\frac{\log n}{n}}\right).
\end{align}


\item For the second term, we have
\begin{align}\label{ineq12:lem_ncv3}
&\left|\sum_{i\neq m}\frac{e^{c_i}}{(1+e^{c_i})^2}\left(\frac{1}{\sqrt{n}}\left(\theta^{t,(m)}_i-\theta^{*}_i\right)+\langle H^{t,(m)}-H^*,z_iz_m\rangle\right)\right|\notag\\
&\leq \frac14\sum_{i\neq m}\frac{1}{\sqrt{n}}\left|\theta^{t,(m)}_i-\theta^{*}_i\right|+\left|\langle H^{t,(m)}-H^*,z_iz_m^T\rangle\right|\notag\\
&\leq \|\theta^{t,(m)}-\theta^{*}\|_2+\| H^{t,(m)}-H^*\|\sum_{i\neq m}\|z_i\|\|z_m\|\notag\\
&\leq \|\theta^{t,(m)}-\theta^{*}\|_2+\sz\| H^{t,(m)}-H^*\|.
\end{align}

\item For the third and fourth terms, note that
\begin{align*}
&\left|\frac{1}{n^{3/2}}\sum_{i\neq m}\frac{e^{c_i}}{(1+e^{c_i})^2}\left(X^{t,(m)}R^{t,(m)}-X^{*}\right)_{i,\cdot}^{\top}\left(Y^{t,(m)}R^{t,(m)}\right)_{m,\cdot}\right|\notag\\
&\leq \frac{1}{n^{3/2}}\sum_{i\neq m}\left|\left(X^{t,(m)}R^{t,(m)}-X^{*}\right)_{i,\cdot}^{\top}\left(Y^{t,(m)}R^{t,(m)}\right)_{m,\cdot}\right|\notag\\
&=\frac{1}{n^{3/2}}\left\|\left(X^{t,(m)}R^{t,(m)}-X^{*}\right)\left(Y^{t,(m)}R^{t,(m)}\right)_{m,\cdot}\right\|_1\notag\\
&\leq \frac{1}{n}\left\|\left(X^{t,(m)}R^{t,(m)}-X^{*}\right)\left(Y^{t,(m)}R^{t,(m)}\right)_{m,\cdot}\right\|_2\notag\\
&\leq \frac{1}{n}\left\|X^{t,(m)}R^{t,(m)}-X^{*}\right\|\left\|Y^{t,(m)}R^{t,(m)}\right\|_{2,\infty}.
\end{align*}
Since Lemma \ref{lem:ncv3} holds for the $t$-th iteration, we have
\begin{align*}
  \left\|Y^{t,(m)}R^{t,(m)}\right\|_{2,\infty}\leq \left\|Y^{t,(m)}R^{t,(m)}-Y^*\right\|_{2,\infty}  + \|Y^*\|_{2,\infty}\leq 2\|Y^*\|_{2,\infty},
\end{align*}
as long as $\|Y^{t,(m)}R^{t,(m)}-Y^*\|_{2,\infty}\ll \|Y^*\|_{2,\infty}$. 
By Lemma \ref{ar:lem2}, we have
\begin{align*}
\left\|F^{t,(m)}R^{t,(m)}-F^{t}R^t\right\|_F\leq 5\kappa    \left\|F^{t,(m)}O^{t,(m)}-F^{t}R^t\right\|_F,
\end{align*}
which implies
\begin{align*}
   \left\|X^{t,(m)}R^{t,(m)}-X^{*}\right\|&\leq \left\|F^{t,(m)}R^{t,(m)}-F^{*}\right\|\\
  &\leq  \left\|F^{t,(m)}R^{t,(m)}-F^{t}R^t\right\|_F+ \left\|F^{t}R^t-F^{*}\right\|\\
   &\leq  5\kappa\left\|F^{t,(m)}O^{t,(m)}-F^{t}R^t\right\|_F+ \left\|F^{t}R^t-F^{*}\right\|\\
  &\leq 2\left\|F^{t}R^t-F^{*}\right\|
\end{align*}
as long as $\kappa\left\|F^{t,(m)}O^{t,(m)}-F^{t}R^t\right\|_F\ll \|F^{t}R^t-F^{*}\|$.
% Here the last inequality holds since $\left\|F^{t,(m)}O^{t,(m)}-F^{t}R^t\right\|_F=O(1)$ by Lemma \ref{lem:ncv2} and $\|F^{t}R^t-F^{*}\|=O(\sqrt{n})$ by Lemma \ref{lem:ncv1}.


Consequently, we have
\begin{align}\label{ineq2:lem_ncv3}
 &\left|\frac{1}{n^{3/2}}\sum_{i\neq m}\frac{e^{c_i}}{(1+e^{c_i})^2}\left(X^{t,(m)}R^{t,(m)}-X^{*}\right)_{i,\cdot}^{\top}\left(Y^{t,(m)}R^{t,(m)}\right)_{m,\cdot}\right|\leq\frac{4}{n}\left\|F^{t}R^t-F^{*}\right\|\|Y^*\|_{2,\infty}. 
\end{align}
Similarly, we have
\begin{align}\label{ineq13:lem_ncv3}
\left| \frac{1}{n^{3/2}}\sum_{i\neq m}\frac{e^{c_i}}{(1+e^{c_i})^2}\left(Y^{t,(m)}R^{t,(m)}-Y^{*}\right)_{i,\cdot}^{\top}\left(X^{t,(m)}R^{t,(m)}\right)_{m,\cdot}\right|\leq\frac{4}{n}\left\|F^{t}R^t-F^{*}\right\|\|X^*\|_{2,\infty}. 
\end{align}

\end{enumerate}

Combine \eqref{ineq1:lem_ncv3}, \eqref{ineq12:lem_ncv3}, \eqref{ineq2:lem_ncv3} and \eqref{ineq13:lem_ncv3}, we have
\begin{align*}
&\left|r_1\right|\notag\\
&\lesssim \frac{\eta\sqrt{\su}}{\sqrt{n}}\left(\|\theta^t-\theta^{t,(m)}\|_2+\|H^t-H^{t,(m)}\|_F+\frac{1}{n}\|X^*\|\|F^tR^t-F^{t,(m)}O^{t,(m)}\|_F\right)\notag\\
&\quad + \frac{\eta\sqrt{\su}}{\sqrt{n}}\left(\|\theta^t-\theta^{*}\|_{2}+\|H^t-H^{*}\|_{F}+\frac{1}{n}\|X^*\|\|F^tR^t-F^*\|_F\right)+\eta\sqrt{\frac{\log n}{n}}\\
&\quad+\frac{\eta}{\sqrt{n}}\left(\|\theta^{t,(m)}-\theta^{*}\|_2+\sz\| H^{t,(m)}-H^*\|\right)+\frac{\eta}{n}\left\|F^{t}R^t-F^{*}\right\|\|F^*\|_{2,\infty}\notag\\
&\lesssim\frac{\eta\sqrt{\overline{C}}}{\sqrt{n}}c_{21}+ {\eta(\sqrt{\overline{C}}}+\sz)c_{11}+\eta\sqrt{\frac{\log n}{n}}+\eta\sqrt{\mu \sX\sY r^2 }c_{14}.
\end{align*}


Note that
\begin{align*}
\nabla_X L^{(m)}(\theta,H,X,Y)
&=\frac1n\sum_{\substack{
        i \neq j \\
        i, j \neq m
    }}\left(\frac{e^{P_{ij}}}{1+e^{P_{ij}}}-A_{ij}\right)e_ie_j^TY\\
&\quad+\frac1n\sum_{i\neq m}\left(\frac{e^{P_{im}}}{1+e^{P_{im}}}-\frac{e^{P_{im}^*}}{1+e^{P_{im}^*}}\right)e_ie_m^TY+\frac1n\sum_{i\neq m}\left(\frac{e^{P_{mi}}}{1+e^{P_{mi}}}-\frac{e^{P_{mi}^*}}{1+e^{P_{mi}^*}}\right)e_me_i^TY,
\end{align*}
where the $m$-th row of the first and second terms are all zeros. Thus, by the gradient descent update, we have
\begin{align*}
&\left(F^{t+1,(m)}R^{t+1,(m)}-F^{*}\right)_{m,\cdot}\\
&=\left(X^{t,(m)}_{m,\cdot}-\eta\left\{\frac1n\sum_{i\neq m}\left(\frac{e^{P_{mi}^{t,(m)}}}{1+e^{P_{mi}^{t,(m)}}}-\frac{e^{P_{mi}^*}}{1+e^{P_{mi}^*}}\right)e_i^TY^{t,(m)}+\lambda X^{t,(m)}_{m,\cdot}\right\}\right)R^{t+1,(m)}-X^*_{m,\cdot}\\
&=\left\{X^{t,(m)}_{m,\cdot}R^{t,(m)}-X^*_{m,\cdot}-\eta\left(\frac1n\sum_{i\neq m}\left(\frac{e^{P_{mi}^{t,(m)}}}{1+e^{P_{mi}^{t,(m)}}}-\frac{e^{P_{mi}^*}}{1+e^{P_{mi}^*}}\right)e_i^TY^{t,(m)}+\lambda X^{t,(m)}_{m,\cdot}\right)R^{t,(m)}\right\}\\
&+\left\{X^{t,(m)}_{m,\cdot}R^{t,(m)}-\eta\left(\frac1n\sum_{i\neq m}\left(\frac{e^{P_{mi}^{t,(m)}}}{1+e^{P_{mi}^{t,(m)}}}-\frac{e^{P_{mi}^*}}{1+e^{P_{mi}^*}}\right)e_i^TY^{t,(m)}+\lambda X^{t,(m)}_{m,\cdot}\right)R^{t,(m)}\right\}\left(\left(R^{t,(m)}\right)^{-1}R^{t+1,(m)}-I_r\right)
\end{align*}
By the mean value theorem, we have for some $\{c_i\}$ that
\begin{align*}
& \sum_{i\neq m}\left(\frac{e^{P^{t,(m)}_{mi}}}{1+e^{P^{t,(m)}_{mi}}}-\frac{e^{P^{*}_{mi}}}{1+e^{P^{*}_{mi}}}\right)e_i^TY^{t,(m)}\\
&= \sum_{i\neq m}\frac{e^{c_i}}{(1+e^{c_i})^2}\left(P^{t,(m)}_{mi}-P^{*}_{mi}\right)e_i^TY^{t,(m)}\\
& = \sum_{i\neq m}\frac{e^{c_i}}{(1+e^{c_i})^2}\left(\frac{1}{\sqrt{n}}\left(\theta^{t,(m)}_i-\theta^{*}_i+\theta^{t,(m)}_m-\theta^{*}_m\right)+\langle H^{t,(m)}-H^*,z_mz_i^T\rangle\right)e_i^TY^{t,(m)}\\
& \quad +\frac1n\sum_{i\neq m}\frac{e^{c_i}}{(1+e^{c_i})^2}\left(X^{t,(m)}(Y^{t,(m)})^T-X^{*}Y^{*T}\right)_{mi}e_i^TY^{t,(m)}.
\end{align*}
Note that
\begin{align*}
&X^{t,(m)}(Y^{t,(m)})^T-X^{*}Y^{*T}\\
&=\left(X^{t,(m)}R^{t,(m)}-X^*\right)\left(Y^{*}\right)^T+(X^{t,(m)}R^{t,(m)})\left(Y^{t,(m)}R^{t,(m)}-Y^*\right)^T.
\end{align*}
Thus, we further have
\begin{align*}
& \sum_{i\neq m}\left(\frac{e^{P^{t,(m)}_{mi}}}{1+e^{P^{t,(m)}_{mi}}}-\frac{e^{P^{*}_{mi}}}{1+e^{P^{*}_{mi}}}\right)e_i^TY^{t,(m)}\\
&= \sum_{i\neq m}\frac{e^{c_i}}{(1+e^{c_i})^2}\left(\frac{1}{\sqrt{n}}\left(\theta^{t,(m)}_i-\theta^{*}_i+\theta^{t,(m)}_m-\theta^{*}_m\right)+\langle H^{t,(m)}-H^*,z_mz_i^T\rangle\right)e_i^TY^{t,(m)}\\
& \quad +\left(X^{t,(m)}R^{t,(m)}-X^*\right)_{m,\cdot}^{\top}\left(\frac1n\sum_{i\neq m}\frac{e^{c_i}}{(1+e^{c_i})^2}(Y^*_{i,\cdot})e_i^TY^{t,(m)}\right)\\
& \quad +\frac1n\sum_{i\neq m}\frac{e^{c_i}}{(1+e^{c_i})^2}\left((X^{t,(m)}R^{t,(m)})\left(Y^{t,(m)}R^{t,(m)}-Y^*\right)^T\right)_{mi}e_i^TY^{t,(m)}.
\end{align*}
Consequently, we have
\begin{align}\label{eq21:lem_ncv3}
&\left(F^{t+1,(m)}R^{t+1,(m)}-F^{*}\right)_{m,\cdot}\notag\\
&=\left(I_r-\frac{\eta}{n^2}\sum_{i\neq m}\frac{e^{c_i}}{(1+e^{c_i})^2}(Y^*_{i,\cdot})e_i^TY^{t,(m)}R^{t,(m)}\right)\left(X^{t,(m)}R^{t,(m)}-X^*\right)_{m,\cdot}\notag\\
&\quad+\left(\frac{\eta}{n^{3/2}}\sum_{i\neq m}\frac{e^{c_i}}{(1+e^{c_i})^2}e_i^TY^{t,(m)}R^{t,(m)}\right)\left(\theta^{t,(m)}_m-\theta^{*}_m\right)\notag\\
&\quad -\frac{\eta}{n}\sum_{i\neq m}\frac{e^{c_i}}{(1+e^{c_i})^2}\left(\frac{1}{\sqrt{n}}\left(\theta^{t,(m)}_i-\theta^{*}_i\right)+\langle H^{t,(m)}-H^*,z_mz_i^T\rangle\right)e_i^TY^{t,(m)}R^{t,(m)}\notag\\
&\quad-\frac{\eta}{n^2}\sum_{i\neq m}\frac{e^{c_i}}{(1+e^{c_i})^2}\left((X^{t,(m)}R^{t,(m)})\left(Y^{t,(m)}R^{t,(m)}-Y^*\right)^T\right)_{mi}e_i^TY^{t,(m)}R^{t,(m)}-\eta\lambda X^{t,(m)}_{m,\cdot}R^{t,(m)}\notag\\
&+\left\{X^{t,(m)}_{m,\cdot}R^{t,(m)}-\eta\left(\frac1n\sum_{i\neq m}\left(\frac{e^{P_{mi}^{t,(m)}}}{1+e^{P_{mi}^{t,(m)}}}-\frac{e^{P_{mi}^*}}{1+e^{P_{mi}^*}}\right)e_i^TY^{t,(m)}+\lambda X^{t,(m)}_{m,\cdot}\right)R^{t,(m)}\right\}\left(\left(R^{t,(m)}\right)^{-1}R^{t+1,(m)}-I_r\right)\notag\\
&=\left(I_r-\frac{\eta}{n^2}\sum_{i\neq m}\frac{e^{c_i}}{(1+e^{c_i})^2}(Y^*_{i,\cdot})(Y^*_{i,\cdot})^{\top}\right)\left(X^{t,(m)}R^{t,(m)}-X^*\right)_{m,\cdot}\notag\\
&\quad+\left(\frac{\eta}{n^{3/2}}\sum_{i\neq m}\frac{e^{c_i}}{(1+e^{c_i})^2}(Y^*_{i,\cdot})\right)\left(\theta^{t,(m)}_m-\theta^{*}_m\right)+r_2,
\end{align}
where
\begin{align*}
r_2&=-\frac{\eta}{n^2}\underbrace{\left(\sum_{i\neq m}\frac{e^{c_i}}{(1+e^{c_i})^2}(Y^*_{i,\cdot})\left(Y^{t,(m)}R^{t,(m)}-Y^{*}\right)_{i,\cdot}^{\top}\right)\left(X^{t,(m)}R^{t,(m)}-X^*\right)_{m,\cdot}}_{(a)}\notag\\
&\quad +\frac{\eta}{n^{3/2}}\underbrace{\left(\sum_{i\neq m}\frac{e^{c_i}}{(1+e^{c_i})^2}\left(Y^{t,(m)}R^{t,(m)}-Y^*\right)_{i,\cdot}\right)\left(\theta^{t,(m)}_m-\theta^{*}_m\right)}_{(b)}\notag\\
&\quad-\frac{\eta}{n}\underbrace{\sum_{i\neq m}\frac{e^{c_i}}{(1+e^{c_i})^2}\left(\frac{1}{\sqrt{n}}\left(\theta^{t,(m)}_i-\theta^{*}_i\right)+\langle H^{t,(m)}-H^*,z_mz_i^T\rangle\right)e_i^TY^{t,(m)}R^{t,(m)}}_{(c)}\\
&\quad-\frac{\eta}{n^2}\underbrace{\sum_{i\neq m}\frac{e^{c_i}}{(1+e^{c_i})^2}\left((X^{t,(m)}R^{t,(m)})\left(Y^{t,(m)}R^{t,(m)}-Y^*\right)^T\right)_{mi}e_i^TY^{t,(m)}R^{t,(m)}}_{(d)}-\eta\lambda \underbrace{X^{t,(m)}_{m,\cdot}R^{t,(m)}}_{(e)}\\
&+\underbrace{\left\{X^{t,(m)}_{m,\cdot}R^{t,(m)}-\eta\left(\frac1n\sum_{i\neq m}\left(\frac{e^{P_{mi}^{t,(m)}}}{1+e^{P_{mi}^{t,(m)}}}-\frac{e^{P_{mi}^*}}{1+e^{P_{mi}^*}}\right)e_i^TY^{t,(m)}+\lambda X^{t,(m)}_{m,\cdot}\right)R^{t,(m)}\right\}\left(\left(R^{t,(m)}\right)^{-1}R^{t+1,(m)}-I_r\right)}_{(f)}
\end{align*}
We bound $\|r_2\|_2$ in the following.
\begin{enumerate}
    
\item For (a), by Cahuchy-Schwarz, we have
\begin{align*}
\| (a)   \|_2\leq \left\|\left(X^{t,(m)}R^{t,(m)}-X^*\right)_{m,\cdot}\right\|_2\|Y^{t,(m)}R^{t,(m)}-Y^*\|_F\|Y^*\|_F.
\end{align*}
Note that
\begin{align*}
&\left\|\left(X^{t,(m)}R^{t,(m)}-X^*\right)_{m,\cdot}\right\|_2\leq c_{31}\\
&\|Y^{t,(m)}R^{t,(m)}-Y^*\|_F\\
&\quad\leq \|Y^{t,(m)}R^{t,(m)}-Y^tR^t\|_F+\|Y^{t}R^{t}-Y^*\|_F\\
&\quad\leq 5\kappa\|Y^{t,(m)}O^{t,(m)}-Y^tR^t\|_F+\|Y^{t}R^{t}-Y^*\|_F\tag{by Lemma \ref{ar:lem2}}\\
&\quad\leq 5\kappa c_{21}+c_{11}\sqrt{n}\\
&\quad \lesssim c_{11}\sqrt{n}\\
&\|Y^*\|_F\leq \sqrt{\mu r\sigma_{\max}}.
\end{align*}
Thus, we have
\begin{align}\label{ineq15:lem_ncv3}
\| (a)   \|_2\lesssim c_{11}c_{31}     \sqrt{\mu r\sigma_{\max}n}.
\end{align}

\item For (b), by Cahuchy-Schwarz, we have
\begin{align}\label{ineq14:lem_ncv3}
\|(b)\|_2\leq \sqrt{n}|\theta^{t,(m)}_m-\theta^{*}_m|\|Y^{t,(m)}R^{t,(m)}-Y^tR^t\|_F\lesssim c_{11}c_{31}n.
\end{align}

\item For (c), note that
\begin{align*}
&\left\|\sum_{i\neq m}\frac{e^{c_i}}{(1+e^{c_i})^2}\left(\frac{1}{\sqrt{n}}\left(\theta^{t,(m)}_i-\theta^{*}_i\right)+\langle H^{t,(m)}-H^*,z_mz_i^T\rangle\right)e_i\right\|_2\\
&\leq \left\|\frac{1}{\sqrt{n}}\sum_{i\neq m}\frac{e^{c_i}}{(1+e^{c_i})^2}\left(\theta^{t,(m)}_i-\theta^{*}_i\right)e_i\right\|_2+ \left\|\sum_{i\neq m}\frac{e^{c_i}}{(1+e^{c_i})^2}\langle H^{t,(m)}-H^*,z_mz_i^T\rangle e_i\right\|_2\\
&\leq\frac{1}{4\sqrt{n}}\left\|\theta^{t,(m)}-\theta^{*}\right\|_2+\frac{1}{4}\sqrt{\sum_{i\neq m}\left|\langle H^{t,(m)}-H^*,z_mz_i^T\rangle\right|^2}\\
&\leq \frac{1}{4\sqrt{n}}\left\|\theta^{t,(m)}-\theta^{*}\right\|_2+\frac{1}{4}\| H^{t,(m)}-H^*\|\|z_m\|_2\sqrt{\sum_{i\neq m}\|z_i\|_2^2}\\
&\leq \frac14\left(\frac{1}{\sqrt{n}}\left\|\theta^{t,(m)}-\theta^{*}\right\|_2+\frac{\sz}{\sqrt{n}}\| H^{t,(m)}-H^*\|\right).
\end{align*}
Moreover, we have
\begin{align*}
    \|Y^{t,(m)}\|\leq  \|F^{t,(m)}O^{t,(m)}-F^tR^t\|+\|F^tR^t-F^*\|+\|F^*\|\leq 2\|F^*\|.
\end{align*}
Thus, we have
\begin{align}\label{ineq16:lem_ncv3}
\|(c)\|_2\leq \|F^*\|\left(\frac{1}{\sqrt{n}}\left\|\theta^{t,(m)}-\theta^{*}\right\|_2+\frac{\sz}{\sqrt{n}}\| H^{t,(m)}-H^*\|\right)\lesssim \sqrt{\sigma_{\max}}\sz c_{11}.
\end{align}

\item For (d), note that
\begin{align*}
&\left\|\sum_{i\neq m}\frac{e^{c_i}}{(1+e^{c_i})^2}\left((X^{t,(m)}R^{t,(m)})\left(Y^{t,(m)}R^{t,(m)}-Y^*\right)^T\right)_{mi}e_i\right\|_2\\
&\leq \frac14 \left\|\left((X^{t,(m)}R^{t,(m)})\left(Y^{t,(m)}R^{t,(m)}-Y^*\right)^T\right)_{m,\cdot}\right\|_2\\
&= \frac14 \left\|(X^{t,(m)}R^{t,(m)})^{\top}_{m,\cdot}\left(Y^{t,(m)}R^{t,(m)}-Y^*\right)^T\right\|_2\\
&\leq \frac14  \left\|(X^{t,(m)}R^{t,(m)})_{m,\cdot}\right\|_2\left\|Y^{t,(m)}R^{t,(m)}-Y^*\right\|\\
&\lesssim  \left\|F^*\right\|_{2,\infty}\left\|Y^{t,(m)}R^{t,(m)}-Y^*\right\|.
\end{align*}
Thus, we have
\begin{align}\label{ineq17:lem_ncv3}
\|(d)\|_2\lesssim \|F^*\|\left\|F^*\right\|_{2,\infty}\left\|Y^{t,(m)}R^{t,(m)}-Y^*\right\|\lesssim \sqrt{\mu\sX\sY r^2 \sigma_{\max}}c_{14}n.
\end{align}

\item For (e), we have
\begin{align}\label{ineq18:lem_ncv3}
\|(e)\|_2\leq \left\|X^{t,(m)}R^{t,(m)}\right\|_{2,\infty}\leq \left\|F^{t,(m)}R^{t,(m)}-F^*\right\|_{2,\infty}+\|F^*\|_{2,\infty}\leq2\|F^*\|_{2,\infty}\lesssim  \sqrt{\mu\sX\sY r^2 n}.
\end{align}

\item Finally, we bound (f).
We denote
\begin{align*}
(1)&:=\left\{X^{t,(m)}_{m,\cdot}R^{t,(m)}-X^*_{m,\cdot}-\eta\left(\frac1n\sum_{i\neq m}\left(\frac{e^{P_{mi}^{t,(m)}}}{1+e^{P_{mi}^{t,(m)}}}-\frac{e^{P_{mi}^*}}{1+e^{P_{mi}^*}}\right)e_i^TY^{t,(m)}+\lambda X^{t,(m)}_{m,\cdot}\right)R^{t,(m)}\right\}\\
&=\left(I_r-\frac{\eta}{n^2}\sum_{i\neq m}\frac{e^{c_i}}{(1+e^{c_i})^2}(Y^*_{i,\cdot})(Y^*_{i,\cdot})^{\top}\right)\left(X^{t,(m)}R^{t,(m)}-X^*\right)_{m,\cdot}\notag\\
&\quad+\left(\frac{\eta}{n^{3/2}}\sum_{i\neq m}\frac{e^{c_i}}{(1+e^{c_i})^2}(Y^*_{i,\cdot})\right)\left(\theta^{t,(m)}_m-\theta^{*}_m\right)-\frac{\eta}{n^2}(a)+\frac{\eta}{n^{3/2}}(b)-\frac{\eta}{n}(c)-\frac{\eta}{n^2}(d)-\eta\lambda (e).
\end{align*}
Note that, by Cauchy-Schwartz, we have
\begin{align*}
&\left\|\sum_{i\neq m}\frac{e^{c_i}}{(1+e^{c_i})^2}(Y^*_{i,\cdot})(Y^*_{i,\cdot})^{\top}\right\|\leq \|Y^*\|_F^2,\\
&\left\|\sum_{i\neq m}\frac{e^{c_i}}{(1+e^{c_i})^2}(Y^*_{i,\cdot})\right\|_2\leq \sqrt{n}\|Y^*\|_F.
\end{align*}
Thus, it can be seen that $\|(1)\|_2\leq \|F^*\|_{2,\infty}$ and we have
\begin{align*}
\|(1)+X^*_{m,\cdot}\|_2\leq \|(1)\|_2+\|X^*_{m,\cdot}\|_2\leq\|(1)\|_2+\|F^*\|_{2,\infty}\leq 2\|F^*\|_{2,\infty}.
\end{align*}
Note that
\begin{align*}
(f)=\left((1)+X^*_{m,\cdot}\right)\left(\left(R^{t,(m)}\right)^{-1}R^{t+1,(m)}-I_r\right).
\end{align*}
Regarding the term $\left(R^{t,(m)}\right)^{-1}R^{t+1,(m)}-I_r$, we have the following claim.
\begin{claim}\label{claim:rotation}
With probability at least $1-n^{-10}$, we have
\begin{align*}
\left\|\left(R^{t,(m)}\right)^{-1}R^{t+1,(m)}-I_r\right\|\lesssim \frac{\eta}{n}\left\| F^{t, (m)}R^{t, (m)}-F^*\right\|.
\end{align*}
\end{claim}
Consequently, we have
\begin{align}\label{ineq19:lem_ncv3}
\|(f)\|_2&\leq \|(1)+X^*_{m,\cdot}\|_2\left\|\left(R^{t,(m)}\right)^{-1}R^{t+1,(m)}-I_r\right\|\notag\\
&\lesssim\frac{\eta}{n}\left\| F^{t, (m)}R^{t, (m)}-F^*\right\|\|F^*\|_{2,\infty}\notag\\
&\lesssim \eta\sqrt{\mu\sX\sY r^2} c_{14}.
\end{align}












It remains to prove Claim \ref{claim:rotation}.
\begin{proof}[Proof of Claim \ref{claim:rotation}]
To facilitate analysis, we introduce an auxiliary point $\tilde{F}^{t+1,(m)}:=\begin{bmatrix}
\tilde{X}^{t+1,(m)}\\
\tilde{Y}^{t+1,(m)}
\end{bmatrix}$ where
\begin{align*}
&\tilde{X}^{t+1,(m)}\\
&={X}^{t,(m)}{R}^{t,(m)}-\eta\left[\frac1n\sum_{\substack{
        i \neq j \\
        i, j \neq m
    }}\left(\frac{e^{P_{ij}^{t,(m)}}}{1+e^{P_{ij}^{t,(m)}}}-A_{ij}\right)e_ie_j^T+\frac1n\sum_{i\neq m}\left(\frac{e^{P_{im}^{t,(m)}}}{1+e^{P_{im}^{t,(m)}}}-\frac{e^{P_{im}^{*}}}{1+e^{P_{im}^{*}}}\right)(e_ie_m^T+e_me_i^T)\right]Y^*\\
&\quad-\eta\lambda X^*-\frac{4c_{\aug}\eta}{n^2}X^*({R}^{t,(m)})^T\left(({X}^{t,(m)})^T{X}^{t,(m)}-({Y}^{t,(m)})^T{Y}^{t,(m)}\right){R}^{t,(m)},\\
&\tilde{Y}^{t+1,(m)}\\
&={Y}^{t,(m)}{R}^{t,(m)}-\eta\left[\frac1n\sum_{\substack{
        i \neq j \\
        i, j \neq m
    }}\left(\frac{e^{P_{ij}^{t,(m)}}}{1+e^{P_{ij}^{t,(m)}}}-A_{ij}\right)e_je_i^T+\frac1n\sum_{i\neq m}\left(\frac{e^{P_{im}^{t,(m)}}}{1+e^{P_{im}^{t,(m)}}}-\frac{e^{P_{im}^{*}}}{1+e^{P_{im}^{*}}}\right)(e_ie_m^T+e_me_i^T)\right]X^*\\
&\quad-\eta\lambda Y^*-\frac{4c_{\aug}\eta}{n^2}Y^*({R}^{t,(m)})^T\left(({Y}^{t,(m)})^T{Y}^{t,(m)}-({X}^{t,(m)})^T{X}^{t,(m)}\right){R}^{t,(m)}.
\end{align*}
We have the following claim.
\begin{claim}\label{claim2:rotation}
It holds that
\begin{align*}
I_r=\argmin_{R\in\cO^{r\times r}}\left\|\tilde{F}^{t+1,(m)}R-F^*\right\|_F,\text{ and } \sigma_{\min}\left(\tilde{F}^{t+1,(m)T}F^{*}\right)\geq \sigma_{\min}/2.
\end{align*}
\begin{proof}[Proof of Claim \ref{claim2:rotation}]
See Claim 4 in \cite{chen2020noisy}.
\end{proof}
\end{claim}
With this claim at hand, by Lemma \ref{ar:lem5} with $S=\tilde{F}^{t+1,(m)T}F^{*}$ and $K=\left({F}^{t+1,(m)}R^{t,(m)}-\tilde{F}^{t+1,(m)}\right)^TF^*$, we have
\begin{align}\label{ineq1:claim2_rotation}
&\left\|\left(R^{t,(m)}\right)^{-1}R^{t+1,(m)}-I_r\right\|\\
&=\left\|\text{sgn}(S+K)-\text{sgn}(S)\right\|\tag{by Claim \ref{claim2:rotation} and the definition of $R^{t+1,(m)}$}\\
&\leq \frac{1}{\sigma_{\min}\left(\tilde{F}^{t+1,(m)T}F^{*}\right)}\left\|\left({F}^{t+1,(m)}R^{t,(m)}-\tilde{F}^{t+1,(m)}\right)^TF^*\right\|\tag{by Lemma \ref{ar:lem5}}\\
&\leq \frac{2}{\sigma_{\min}}\left\|{F}^{t+1,(m)}R^{t,(m)}-\tilde{F}^{t+1,(m)}\right\|\|F^*\|\tag{by Claim \ref{claim2:rotation}}.
\end{align}
Here  \(\text{sgn}(A) = UV^\top\) for a matrix \( A \) with SVD \( U \Sigma V^\top \). Note that
\begin{align*}
    &F^{t+1, (m)} R^{t, (m)} - \tilde{F}^{t+1, (m)} \\
    &= -\eta \begin{bmatrix} B & 0 \\ 0 & B^\top \end{bmatrix} \begin{bmatrix} Y^{t, (m)}R^{t, (m)}-Y^*  \\ X^{t, (m)}R^{t, (m)}-X^* \end{bmatrix} + \frac{4c_{\aug}\eta}{n^2} \begin{bmatrix} X^\star \\ -Y^\star \end{bmatrix} R^{t, (m) \top} C R^{t, (m)} - \eta \lambda\begin{bmatrix}   X^{t, (m)}R^{t, (m)}-X^*\\ Y^{t, (m)}R^{t, (m)}-Y^* \end{bmatrix} ,
\end{align*}
where we denote
\begin{align*}
 &B := \frac1n\sum_{\substack{
        i \neq j \\
        i, j \neq m
    }}\left(\frac{e^{P_{ij}^{t,(m)}}}{1+e^{P_{ij}^{t,(m)}}}-A_{ij}\right)e_ie_j^T+\frac1n\sum_{i\neq m}\left(\frac{e^{P_{im}^{t,(m)}}}{1+e^{P_{im}^{t,(m)}}}-\frac{e^{P_{im}^{*}}}{1+e^{P_{im}^{*}}}\right)(e_ie_m^T+e_me_i^T),\\ 
 &C := X^{t, (m) \top} X^{t, (m)} - Y^{t, (m) \top} Y^{t, (m)}.
\end{align*}
This enables us to obtain
\begin{align*}
 &\left\|F^{t+1, (m)} R^{t, (m)} - \tilde{F}^{t+1, (m)}\right\| \\
& \leq \eta \left\| B \right\| \left\| F^{t, (m)}R^{t, (m)}-F^*\right\| + \frac{4c_{\aug}\eta}{n^2} \left\| F^\star \right\| \left\| C \right\|_F +\eta \lambda\left\| F^{t, (m)}R^{t, (m)}-F^*\right\|.   
\end{align*}
We then bound $\|B\|$ in the following.
Note that
\begin{align*}
B&=\frac1n\sum_{i\neq j}\left(\frac{e^{P_{ij}^{t,(m)}}}{1+e^{P_{ij}^{t,(m)}}}-\frac{e^{P_{ij}^{*}}}{1+e^{P_{ij}^{*}}}\right)e_ie_j^T +   \frac1n\sum_{\substack{
        i \neq j \\
        i, j \neq m
    }}\left(\frac{e^{P_{ij}^{*}}}{1+e^{P_{ij}^{*}}}-A_{ij}\right)e_ie_j^T.
\end{align*}
For the first term, we have
\begin{align*}
&\left\|\sum_{i\neq j}\left(\frac{e^{P_{ij}^{t,(m)}}}{1+e^{P_{ij}^{t,(m)}}}-\frac{e^{P_{ij}^{*}}}{1+e^{P_{ij}^{*}}}\right)e_ie_j^T\right\|\\
&\leq \left\|\sum_{i\neq j}\left(\frac{e^{P_{ij}^{t,(m)}}}{1+e^{P_{ij}^{t,(m)}}}-\frac{e^{P_{ij}^{*}}}{1+e^{P_{ij}^{*}}}\right)e_ie_j^T\right\|_F\\
&=\sqrt{\sum_{i\neq j}\left(\frac{e^{P_{ij}^{t,(m)}}}{1+e^{P_{ij}^{t,(m)}}}-\frac{e^{P_{ij}^{*}}}{1+e^{P_{ij}^{*}}}\right)^2}\\
&=\frac14\sqrt{\sum_{i\neq j}\left(P_{ij}^{t,(m)}-P_{ij}^{*}\right)^2}\tag{by mean value theorem}\\
&\lesssim \sqrt{\su}\left(\|\theta^{t,(m)}-\theta^{*}\|_{2}+\|H^{t,(m)}-H^{*}\|_{F}+\frac{1}{n}\|F^*\|\|F^{t,(m)}R^{t,(m)}-F^{*}\|_{F}\right).
\end{align*}
For the second term, same as bounding $\|\nabla_{\Gamma}L_c(\theta^*,H^*,\Gamma^*)\|$ in the proof of Lemma \ref{lem:gradient_norm}, we have
\begin{align*}
\left\| \frac1n\sum_{\substack{
        i \neq j \\
        i, j \neq m
    }}\left(\frac{e^{P_{ij}^{*}}}{1+e^{P_{ij}^{*}}}-A_{ij}\right)e_ie_j^T\right\|\lesssim\sqrt{\frac{\log n}{n}}.
\end{align*}
Consequently, we have
\begin{align*}
\|B\|&\lesssim \frac{\sqrt{\su}}{n}\left(\|\theta^{t,(m)}-\theta^{*}\|_{2}+\|H^{t,(m)}-H^{*}\|_{F}+\frac{1}{n}\|F^*\|\|F^{t,(m)}R^{t,(m)}-F^{*}\|_{F}\right)+\sqrt{\frac{\log n}{n}}\\
&\lesssim \sqrt{\frac{\overline{C}}{n}}c_{11}+\sqrt{\frac{\log n}{n}}.
\end{align*}
Thus, we have
\begin{align*}
 &\left\|F^{t+1, (m)} R^{t, (m)} - \tilde{F}^{t+1, (m)}\right\| \\
& \leq c\eta\sqrt{\frac{\overline{C}c^2_{11}+\log n}{n}}\left\| F^{t, (m)}R^{t, (m)}-F^*\right\| + \frac{4c_{\aug}\eta}{n^2} \left\| F^\star \right\| \left\|  X^{t, (m) \top} X^{t, (m)} - Y^{t, (m) \top} Y^{t, (m)} \right\|_F \\
&\quad +\eta \lambda\left\| F^{t, (m)}R^{t, (m)}-F^*\right\|.   
\end{align*}
By \eqref{ineq1:claim2_rotation}, we obtain
\begin{align*}
 &\left\|\left(R^{t,(m)}\right)^{-1}R^{t+1,(m)}-I_r\right\|\\
 &\leq \frac{2\|F^*\|}{\sigma_{\min}}  \Bigg(c\eta\sqrt{\frac{\overline{C}c^2_{11}+\log n}{n}}\left\| F^{t, (m)}R^{t, (m)}-F^*\right\| + \frac{4c_{\aug}\eta}{n^2} \left\| F^\star \right\| \left\|  X^{t, (m) \top} X^{t, (m)} - Y^{t, (m) \top} Y^{t, (m)} \right\|_F \\
 &\qquad\qquad\qquad+\eta \lambda\left\| F^{t, (m)}R^{t, (m)}-F^*\right\|\Bigg)\\
  &\lesssim \frac{\|F^*\|}{\sigma_{\min}} \eta \Bigg(\sqrt{\frac{\overline{C}c^2_{11}+\log n}{n}}\left\| F^{t, (m)}R^{t, (m)}-F^*\right\| + c_{\aug}c_{51}\eta\sqrt{\sigma_{\max}} +\lambda\left\| F^{t, (m)}R^{t, (m)}-F^*\right\|\Bigg)\\
&\lesssim \frac{\eta\sqrt{\sigma_{\max}}}{\sigma_{\min}}\left(\sqrt{\frac{\overline{C}c^2_{11}+\log n}{n}}+\lambda\right) \left\| F^{t, (m)}R^{t, (m)}-F^*\right\| \tag{as long as $\eta$ small enough}\\
&\lesssim \frac{\eta}{n}\left\| F^{t, (m)}R^{t, (m)}-F^*\right\|
\end{align*}
as long as $\frac{n\sqrt{\sigma_{\max}}}{\sigma_{\min}}\left(\sqrt{\frac{\overline{C}c^2_{11}+\log n}{n}}+\lambda\right)\lesssim 1$.
We then prove Claim \ref{claim:rotation}.

\end{proof}
\end{enumerate}

Combine \eqref{ineq15:lem_ncv3}, \eqref{ineq14:lem_ncv3}, \eqref{ineq16:lem_ncv3}, \eqref{ineq17:lem_ncv3}, \eqref{ineq18:lem_ncv3}, \eqref{ineq19:lem_ncv3}, we obtain
\begin{align*}
&\|r_2\|_2\\
&\lesssim \eta\left(\frac{1}{n^{3/2}} c_{11}c_{31} \sqrt{\mu r\sigma_{\max}}+\frac{1}{\sqrt{n}}c_{11}c_{31}+\frac{1}{n}\sqrt{\sigma_{\max}}\sz c_{11}+\frac{1}{n}\sqrt{\mu\sX\sY r^2 \sigma_{\max}}c_{14}+\lambda\sqrt{\mu\sX\sY r^2 n}+\sqrt{\mu\sX\sY r^2} c_{14}\right).
\end{align*}

Similarly, we have 
\begin{align}\label{eq20:lem_ncv3}
&\left(F^{t+1,(m)}R^{t+1,(m)}-F^{*}\right)_{m+n,\cdot}\notag\\
&=\left(I_r-\frac{\eta}{n^2}\sum_{i\neq m}\frac{e^{c_i}}{(1+e^{c_i})^2}(X^*_{i,\cdot})(X^*_{i,\cdot})^{\top}\right)\left(Y^{t,(m)}R^{t,(m)}-Y^*\right)_{m,\cdot}\notag\\
&\quad+\left(\frac{\eta}{n^{3/2}}\sum_{i\neq m}\frac{e^{c_i}}{(1+e^{c_i})^2}(X^*_{i,\cdot})\right)\left(\theta^{t,(m)}_m-\theta^{*}_m\right)+r_3,
\end{align}
where
\begin{align*}
&\|r_3\|_2\\
&\lesssim \eta\left(\frac{1}{n^{3/2}} c_{11}c_{31} \sqrt{\mu r\sigma_{\max}}+\frac{1}{\sqrt{n}}c_{11}c_{31}+\frac{1}{n}\sqrt{\sigma_{\max}}\sz c_{11}+\frac{1}{n}\sqrt{\mu\sX\sY r^2 \sigma_{\max}}c_{14}+\lambda\sqrt{\mu\sX\sY r^2 n}+\sqrt{\mu\sX\sY r^2} c_{14}\right).
\end{align*}

By \eqref{eq11:lem_ncv3}, \eqref{eq21:lem_ncv3} and \eqref{eq20:lem_ncv3}, we obtain
\begin{align}\label{ineq58:pf_lem_ncv3}
&\begin{bmatrix}
\theta^{t+1,(m)}_m-\theta^*_m\\
\left(F^{t+1,(m)}R^{t,(m)}-F^{*}\right)_{m,\cdot}\\
\left(F^{t+1,(m)}R^{t,(m)}-F^{*}\right)_{m+n,\cdot}
\end{bmatrix}\notag\\
&=A\begin{bmatrix}
\theta^{t,(m)}_m-\theta^*_m\\
\left(F^{t,(m)}R^{t,(m)}-F^{*}\right)_{m,\cdot}\\
\left(F^{t,(m)}R^{t,(m)}-F^{*}\right)_{m+n,\cdot}
\end{bmatrix}+
\begin{bmatrix}
r_1\\
0\\
0
\end{bmatrix}
+
\begin{bmatrix}
0\\
r_2\\
0
\end{bmatrix}
+
\begin{bmatrix}
0\\
0\\
r_3
\end{bmatrix},
\end{align}
where
\begin{align*}
A&=
\begin{bmatrix}
 1-\frac{2\eta}{n}\sum_{i\neq m}\frac{e^{c_i}}{(1+e^{c_i})^2}&-\frac{\eta}{n^{3/2}}\sum_{i\neq m}\frac{e^{c_i}}{(1+e^{c_i})^2}\left(Y^{*}_{i,\cdot}\right)^T &-\frac{\eta}{n^{3/2}}\sum_{i\neq m}\frac{e^{c_i}}{(1+e^{c_i})^2}(X^*_{i,\cdot})^{\top} \\
 \frac{\eta}{n^{3/2}}\sum_{i\neq m}\frac{e^{c_i}}{(1+e^{c_i})^2}(Y^*_{i,\cdot}) & I_r-\frac{\eta}{n^2}\sum_{i\neq m}\frac{e^{c_i}}{(1+e^{c_i})^2}(Y^*_{i,\cdot})(Y^*_{i,\cdot})^{\top} & 0 \\
\frac{\eta}{n^{3/2}}\sum_{i\neq m}\frac{e^{c_i}}{(1+e^{c_i})^2}(X^*_{i,\cdot})& 0 & I_r-\frac{\eta}{n^2}\sum_{i\neq m}\frac{e^{c_i}}{(1+e^{c_i})^2}(X^*_{i,\cdot})(X^*_{i,\cdot})^{\top}\\
\end{bmatrix}\\
&=I_{2r+1}-\eta\sum_{i\neq m}\frac{e^{c_i}}{(1+e^{c_i})^2}
\begin{bmatrix}
\frac{1}{\sqrt{n}}\\
\frac{1}{n}Y^*_{i,\cdot}\\
0
\end{bmatrix}^{\otimes 2}
-\eta\sum_{i\neq m}\frac{e^{c_i}}{(1+e^{c_i})^2}
\begin{bmatrix}
\frac{1}{\sqrt{n}}\\
0\\
\frac{1}{n}X^*_{i,\cdot}
\end{bmatrix}^{\otimes 2}\\
&=I_{2r+1}-\eta\sum_{i\neq m}\frac{e^{c_i}}{(1+e^{c_i})^2}
\begin{bmatrix}
\frac{1}{\sqrt{n}}\\
\frac{1}{n}e_i^{\top}Y^*\\
0
\end{bmatrix}^{\otimes 2}
-\eta\sum_{i\neq m}\frac{e^{c_i}}{(1+e^{c_i})^2}
\begin{bmatrix}
\frac{1}{\sqrt{n}}\\
0\\
\frac{1}{n}e_i^{\top}X^*
\end{bmatrix}^{\otimes 2}\\
&=I_{2r+1}-\eta\sum_{i\neq m}\frac{e^{c_i}}{(1+e^{c_i})^2}
\left(
\begin{bmatrix}
\frac{1}{\sqrt{n}}\\
\frac{1}{n}e_i^{\top}Y^*\\
0
\end{bmatrix}^{\otimes 2}
+
\begin{bmatrix}
\frac{1}{\sqrt{n}}\\
0\\
\frac{1}{n}e_i^{\top}X^*
\end{bmatrix}^{\otimes 2}
\right).
\end{align*}

Notice that $|P^{t,(m)}_{im}|\leq 2|P^{*}_{im}|$. Thus, by Assumption \ref{assumption:scales}, we have $|c_i|\leq 2|P^{*}_{im}|\leq 2c_P$, which implies
\begin{align*}
\frac{e^{2c_P}}{(1+e^{2c_P})^2}\leq\frac{e^{c_i}}{(1+e^{c_i})^2}\leq \frac14.
\end{align*}
Denote 
\begin{align*}
B:=\sum_{i\neq m}\frac{e^{c_i}}{(1+e^{c_i})^2}
\left(
\begin{bmatrix}
\frac{1}{\sqrt{n}}\\
\frac{1}{n}e_i^{\top}Y^*\\
0
\end{bmatrix}^{\otimes 2}
+
\begin{bmatrix}
\frac{1}{\sqrt{n}}\\
0\\
\frac{1}{n}e_i^{\top}X^*
\end{bmatrix}^{\otimes 2}
\right).
\end{align*}
We then have
\begin{align}\label{ineq56:pf_lem_ncv3}
&\left\|
A\begin{bmatrix}
\theta^{t,(m)}_m-\theta^*_m\\
\left(F^{t,(m)}R^{t,(m)}-F^{*}\right)_{m,\cdot}\\
\left(F^{t,(m)}R^{t,(m)}-F^{*}\right)_{m+n,\cdot}
\end{bmatrix}
\right\|^2_2\notag\\
&=\begin{bmatrix}
\theta^{t,(m)}_m-\theta^*_m\\
\left(F^{t,(m)}R^{t,(m)}-F^{*}\right)_{m,\cdot}\\
\left(F^{t,(m)}R^{t,(m)}-F^{*}\right)_{m+n,\cdot}
\end{bmatrix}^{\top}(I-2\eta B+\eta^2 B^2)
\begin{bmatrix}
\theta^{t,(m)}_m-\theta^*_m\\
\left(F^{t,(m)}R^{t,(m)}-F^{*}\right)_{m,\cdot}\\
\left(F^{t,(m)}R^{t,(m)}-F^{*}\right)_{m+n,\cdot}
\end{bmatrix}\notag\\
&=\left\|
\begin{bmatrix}
\theta^{t,(m)}_m-\theta^*_m\\
\left(F^{t,(m)}R^{t,(m)}-F^{*}\right)_{m,\cdot}\\
\left(F^{t,(m)}R^{t,(m)}-F^{*}\right)_{m+n,\cdot}
\end{bmatrix}
\right\|^2_2
-2\eta \begin{bmatrix}
\theta^{t,(m)}_m-\theta^*_m\\
\left(F^{t,(m)}R^{t,(m)}-F^{*}\right)_{m,\cdot}\\
\left(F^{t,(m)}R^{t,(m)}-F^{*}\right)_{m+n,\cdot}
\end{bmatrix}^{\top}B
\begin{bmatrix}
\theta^{t,(m)}_m-\theta^*_m\\
\left(F^{t,(m)}R^{t,(m)}-F^{*}\right)_{m,\cdot}\\
\left(F^{t,(m)}R^{t,(m)}-F^{*}\right)_{m+n,\cdot}
\end{bmatrix}\notag\\
&\quad +
\eta^2\begin{bmatrix}
\theta^{t,(m)}_m-\theta^*_m\\
\left(F^{t,(m)}R^{t,(m)}-F^{*}\right)_{m,\cdot}\\
\left(F^{t,(m)}R^{t,(m)}-F^{*}\right)_{m+n,\cdot}
\end{bmatrix}^{\top}B^2
\begin{bmatrix}
\theta^{t,(m)}_m-\theta^*_m\\
\left(F^{t,(m)}R^{t,(m)}-F^{*}\right)_{m,\cdot}\\
\left(F^{t,(m)}R^{t,(m)}-F^{*}\right)_{m+n,\cdot}
\end{bmatrix}.
\end{align}

Denote by $L = \text{diag}((1 - 2/n)I_n, I_{r})$ and 
\begin{align*}
B_1:=\sum_{i\neq m}\frac{e^{c_i}}{(1+e^{c_i})^2}
\begin{bmatrix}
\frac{1}{\sqrt{n}}\\
\frac{1}{n}e_i^{\top}Y^*
\end{bmatrix}^{\otimes 2}
,\quad  B_2:=\sum_{i\neq m}\frac{e^{c_i}}{(1+e^{c_i})^2}
\begin{bmatrix}
\frac{1}{\sqrt{n}}\\
\frac{1}{n}e_i^{\top}X^*
\end{bmatrix}^{\otimes 2}.
\end{align*}
Note that $LB_kL$ is a submatrix of $\cP D^*\cP$ ($k=1,2$), so its spectral norm can be controlled as
\begin{align*}
    \left\|LB_k L\right\| \leq \frac{(1+e^{c_P})^2}{4 e^{c_P}}\left\|\cP D^*\cP\right\|\leq \frac{(1+e^{c_P})^2}{4 e^{c_P}}\suD. 
\end{align*}
On the other hand, since $L\succcurlyeq (1-2/n)I_{n+r}$, as long as $n\geq 7$, we have
\begin{align*}
    \left\|B_k\right\|\leq \frac{n^2}{(n-2)^2}\cdot \frac{(1+e^{c_P})^2}{4 e^{c_P}}\suD\leq  \frac{(1+e^{c_P})^2}{2 e^{c_P}}\suD.
\end{align*}
Thus, $\|B\|\leq \|B_1\| + \|B_2\|\leq \frac{(1+e^{c_P})^2}{ e^{c_P}}\suD$. On the other hand we want to lower bound the smallest eigenvalue of $B$. For any $\begin{bmatrix}
\theta\\
\bx\\
\by
\end{bmatrix}$, where $\theta\in \bbR$, $\bx,\by\in\bbR^{r}$, we have
\begin{align}
\begin{bmatrix}
\theta\\
\bx\\
\by
\end{bmatrix}^{\top}B
\begin{bmatrix}
\theta\\
\bx\\
\by
\end{bmatrix}&=
\begin{bmatrix}
\theta\\
\bx
\end{bmatrix}^{\top}
\left(\sum_{i\neq m}
\frac{e^{c_i}}{(1+e^{c_i})^2}
\begin{bmatrix}
\frac{1}{\sqrt{n}}\\
\frac{1}{n}e_i^{\top}Y^*
\end{bmatrix}^{\otimes 2}\right)
\begin{bmatrix}
\theta\\
\bx
\end{bmatrix}
+
\begin{bmatrix}
\theta\\
\by
\end{bmatrix}^{\top}
\left(\sum_{i\neq m}
\frac{e^{c_i}}{(1+e^{c_i})^2}
\begin{bmatrix}
\frac{1}{\sqrt{n}}\\
\frac{1}{n}e_i^{\top}X^*
\end{bmatrix}^{\otimes 2}
\right)
\begin{bmatrix}
\theta\\
\by
\end{bmatrix} \notag \\
&=\begin{bmatrix}
\theta\\
\bx
\end{bmatrix}^{\top}
B_1
\begin{bmatrix}
\theta\\
\bx
\end{bmatrix}
+
\begin{bmatrix}
\theta\\
\by
\end{bmatrix}^{\top}
B_2
\begin{bmatrix}
\theta\\
\by
\end{bmatrix}.\label{pf:lem_ncv3eq3}
\end{align}
Taking advantage of the idea that $LB_1L$ is a submatrix of $\cP D^*\cP$, we denote by $v\in \mathbb{R}^{n(2r+1)+p^2}$ such that 
\begin{align*}
    v_k =
    \begin{cases}
      \theta & \text{if } k=m\\
      x_j & \text{if } k = n+p^2+(m-1)r+j \text{ for some } j\in [r]\\
      0 & \text{otherwise}
    \end{cases}.
\end{align*}
Then we know that 
\begin{align}
    \begin{bmatrix}
\theta\\
\bx
\end{bmatrix}^{\top}
B_1
\begin{bmatrix}
\theta\\
\bx
\end{bmatrix}\geq \begin{bmatrix}
\theta\\
\bx
\end{bmatrix}^{\top}
LB_1L
\begin{bmatrix}
\theta\\
\bx
\end{bmatrix} \geq \frac{4 e^{2 c_P}}{(1+e^{2 c_P})^2} v^\top \cP D^*\cP v. \label{pf:lem_ncv3eq1}
\end{align}
Denote by $Q:=(\cP D^*\cP)^{\dagger}\cP D^*\cP$, then Assumption \ref{assumption:D_eigen} implies
\begin{align}
    v^\top \cP D^*\cP v\geq \slD \left\|Q v\right\|_2^2.\label{pf:lem_ncv3eq2}
\end{align}
On the other hand, we have
\begin{align*}
    \left\|Q v\right\|_2^2&\geq (Q v)_m^2 +\sum_{j=1}^r (Qv)_{n+p^2+(m-1)r+j}^2 \\
    &=\left(v_m - ((I-Q)v)_m\right)^2 +\sum_{j=1}^r \left(v_{n+p^2+(m-1)r+j} - ((I-Q)v)_{n+p^2+(m-1)r+j}\right)^2 \\
    &\geq v_m^2+\sum_{j=1}^r v_{n+p^2+(m-1)r+j}^2 - 2\left(|v_m|+ \sum_{j=1}^r \left| v_{n+p^2+(m-1)r+j}\right|\right)\left\|(I-Q)v\right\|_\infty \\
    &\geq \left\|v\right\|_2^2 - 2\sqrt{r+1}\left\|v\right\|_2\left\|I-Q\right\|_{2,\infty}\left\|v\right\|_2 \geq  \left(1-2c_{2,\infty}\sqrt{\frac{(r+1)(r^2+1)}{n}}\right)\left\|v\right\|_2^2
\end{align*}
according to Assumption \ref{assumption:2_infty}. Therefore, as long as $n\geq 16(r+1)(r^2+1)c_{2,\infty}^2$, we have $\left\|Q v\right\|_2^2\geq \left\|v\right\|_2^2 / 2$. Combine this with \eqref{pf:lem_ncv3eq1} and \eqref{pf:lem_ncv3eq2} we get 
\begin{align*}
    \begin{bmatrix}
\theta\\
\bx
\end{bmatrix}^{\top}
B_1
\begin{bmatrix}
\theta\\
\bx
\end{bmatrix}\geq \frac{4 e^{2 c_P}}{(1+e^{2 c_P})^2}\cdot \frac{\slD}{2}\left\|v\right\|_2^2 = \frac{2 \slD e^{2 c_P}}{(1+e^{2 c_P})^2}\left(\theta^2 +\left\|\bx\right\|_2^2\right). 
\end{align*}
Similarly, we have 
\begin{align*}
    \begin{bmatrix}
\theta\\
\by
\end{bmatrix}^{\top}
B_2
\begin{bmatrix}
\theta\\
\by
\end{bmatrix}\geq\frac{2 \slD e^{2 c_P}}{(1+e^{2 c_P})^2}\left(\theta^2 +\left\|\by\right\|_2^2\right). 
\end{align*}
Plugging these in \eqref{pf:lem_ncv3eq3} we know that 
\begin{align*}
    \begin{bmatrix}
\theta\\
\bx\\
\by
\end{bmatrix}^{\top}B
\begin{bmatrix}
\theta\\
\bx\\
\by
\end{bmatrix}\geq \frac{2 \slD e^{2 c_P}}{(1+e^{2 c_P})^2}\left(\theta^2 +\left\|\bx\right\|_2^2\right)+\frac{2 \slD e^{2 c_P}}{(1+e^{2 c_P})^2}\left(\theta^2 +\left\|\by\right\|_2^2\right)\geq \frac{2 \slD e^{2 c_P}}{(1+e^{2 c_P})^2}\left\|
\begin{bmatrix}
\theta\\
\bx\\
\by
\end{bmatrix}
\right\|^2_2.
\end{align*}
Since this holds for all $\theta\in \bbR$, $\bx,\by\in\bbR^{r}$, we know that 
\begin{align*}
    B\succcurlyeq\frac{2 \slD e^{2 c_P}}{(1+e^{2 c_P})^2} I_{2r+1}.
\end{align*}
To sum up, as long as $n\geq \max\{16(r+1)(r^2+1)c_{2,\infty}^2, 7\}$, we have 
\begin{align*}
   \frac{2 \slD e^{2 c_P}}{(1+e^{2 c_P})^2}  I_{2r+1}\preccurlyeq B\preccurlyeq \frac{(1+e^{c_P})^2}{ e^{c_P}}\suD I_{2r+1}.
\end{align*}






% \newpage
% Denote $X^{*}_i,Y^{*}_i\in\bbR^{r}$ the $i$-th row of $X^*, Y^*$, respectively. We have
% \begin{align}\label{ineq50:pf_lem_ncv3}
% &\sum_{i\neq m}X^{*}_i X^{*\top}_i\preccurlyeq X^{*\top} X^{*}\preccurlyeq \sigma_{\max}I_r
% \end{align}
% and
% \begin{align}\label{ineq51:pf_lem_ncv3}
% \sum_{i\neq m}X^{*}_i X^{*\top}_i
% &=X^{*\top} X^{*}-X^{*}_m X^{*\top}_m\notag\\
% &\succcurlyeq X^{*\top} X^{*}-\|X^*\|_{2,\infty}^2 I_r\notag\\
% &\succcurlyeq \left(\sigma_{\min}-\|X^*\|_{2,\infty}^2\right) I_r\notag\\
% &\succcurlyeq\frac{\sigma_{\min}}{2} I_r.
% \end{align}
% Moreover, we have
% \begin{align}\label{ineq52:pf_lem_ncv3}
% \left\|\sum_{i\neq m}X^{*}_i\right\|_2 \leq n \|X^*\|_{2,\infty}.
% \end{align}
% Similar properties also hold for $Y^{*}_i$.




% For any $\begin{bmatrix}
% \theta\\
% \bx\\
% \by
% \end{bmatrix}$, where $\theta\in \bbR$, $\bx,\by\in\bbR^{r}$, we have
% \begin{align*}
%  &\begin{bmatrix}
% \theta\\
% \bx\\
% \by
% \end{bmatrix}^{\top}B
% \begin{bmatrix}
% \theta\\
% \bx\\
% \by
% \end{bmatrix}\notag\\
% &\leq \frac14\begin{bmatrix}
% \theta\\
% \bx\\
% \by
% \end{bmatrix}^{\top}
% \left(\sum_{i\neq m}
% \begin{bmatrix}
% \frac{1}{\sqrt{n}}\\
% \frac{1}{n}e_i^{\top}Y^*\\
% 0
% \end{bmatrix}^{\otimes 2}
% +
% \begin{bmatrix}
% \frac{1}{\sqrt{n}}\\
% 0\\
% \frac{1}{n}e_i^{\top}X^*
% \end{bmatrix}^{\otimes 2}
% \right)
% \begin{bmatrix}
% \theta\\
% \bx\\
% \by
% \end{bmatrix}\notag\\
% &=\frac14
% \left(
% \begin{bmatrix}
% \theta\\
% \bx
% \end{bmatrix}^{\top}
% \left(\sum_{i\neq m}
% \begin{bmatrix}
% \frac{1}{\sqrt{n}}\\
% \frac{1}{n}e_i^{\top}Y^*
% \end{bmatrix}^{\otimes 2}\right)
% \begin{bmatrix}
% \theta\\
% \bx
% \end{bmatrix}
% +
% \begin{bmatrix}
% \theta\\
% \by
% \end{bmatrix}^{\top}
% \left(\sum_{i\neq m}
% \begin{bmatrix}
% \frac{1}{\sqrt{n}}\\
% \frac{1}{n}e_i^{\top}X^*
% \end{bmatrix}^{\otimes 2}
% \right)
% \begin{bmatrix}
% \theta\\
% \by
% \end{bmatrix}
% \right)\notag\\
% &=\frac14
% \left(
% \begin{bmatrix}
% \theta\\
% \bx
% \end{bmatrix}^{\top}
% \begin{bmatrix}
% \frac{n-1}{n} & \frac{1}{n^{3/2}} \sum_{i\neq m} Y^{*\top}_i\\
% \frac{1}{n^{3/2}} \sum_{i\neq m} Y^{*}_i & \frac{1}{n^2} \sum_{i\neq m} Y^{*}_i Y^{*\top}_i
% \end{bmatrix}
% \begin{bmatrix}
% \theta\\
% \bx
% \end{bmatrix}
% +
% \begin{bmatrix}
% \theta\\
% \by
% \end{bmatrix}^{\top}
% \begin{bmatrix}
% \frac{n-1}{n} & \frac{1}{n^{3/2}} \sum_{i\neq m} X^{*\top}_i\\
% \frac{1}{n^{3/2}} \sum_{i\neq m} X^{*}_i & \frac{1}{n^2} \sum_{i\neq m} X^{*}_i X^{*\top}_i
% \end{bmatrix}
% \begin{bmatrix}
% \theta\\
% \by
% \end{bmatrix}
% \right)\notag\\
% &=\frac14
% \Bigg(
% \frac{2(n-1)}{n}\theta^2+\frac{2\theta}{n^{3/2}}\bx^{\top}\left(\sum_{i\neq m}Y^*_{i}\right)+\frac{1}{n^2}\bx^{\top}\left(\sum_{i\neq m} Y^{*}_i Y^{*\top}_i\right)\bx\notag\\
% &\qquad\qquad\qquad\qquad+\frac{2\theta}{n^{3/2}}\by^{\top}\left(\sum_{i\neq m}X^*_{i}\right)+\frac{1}{n^2}\by^{\top}\left(\sum_{i\neq m} X^{*}_i X^{*\top}_i\right)\by
% \Bigg)\notag\\
% & \leq \frac14
% \left(
% \frac{2(n-1)}{n}\theta^2
% +\frac{2\|X^*\|_{2,\infty}}{\sqrt{n}}|\theta|\|\bx\|_2+\frac{2\|Y^*\|_{2,\infty}}{\sqrt{n}}|\theta|\|\by\|_2+\frac{\sigma_{\max}}{n^2}(\|\bx\|_2^2+\|\by\|_2^2)
% \right)\tag{by \eqref{ineq50:pf_lem_ncv3}, \eqref{ineq52:pf_lem_ncv3}}\\
% & \leq \frac14
% \left(
% \frac{2(n-1)}{n}\theta^2
% +\frac{\|X^*\|_{2,\infty}}{\sqrt{n}}(\theta^2+\|\bx\|_2^2)+\frac{\|Y^*\|_{2,\infty}}{\sqrt{n}}(\theta^2+\|\by\|_2^2)+\frac{\sigma_{\max}}{n^2}(\|\bx\|_2^2+\|\by\|_2^2)
% \right)\notag\\
% &\leq \frac14
% \left(
% \frac{2(n-1)}{n}\theta^2
% +\sqrt{\frac{\mu r \sigma_{\max}}{n^2}}(2\theta^2+\|\bx\|_2^2+\|\by\|_2^2)+\frac{\sigma_{\max}}{n^2}(\|\bx\|_2^2+\|\by\|_2^2)
% \right)\notag\\
% &\leq \left(1+\sqrt{\frac{\mu r \sigma_{\max}}{n^2}}+\frac{\sigma_{\max}}{n^2}\right)
% \left\|
% \begin{bmatrix}
% \theta\\
% \bx\\
% \by
% \end{bmatrix}
% \right\|^2_2,
% \end{align*}
% which implies
% \begin{align}\label{ineq54:pf_lem_ncv3}
%   \|B\|\leq   1+\sqrt{\frac{\mu r \sigma_{\max}}{n^2}}+\frac{\sigma_{\max}}{n^2}.
% \end{align}
% Similarly, we have
% \begin{align}
% &\begin{bmatrix}
% \theta\\
% \bx\\
% \by
% \end{bmatrix}^{\top}B
% \begin{bmatrix}
% \theta\\
% \bx\\
% \by
% \end{bmatrix}\notag\\
% &\geq\frac{e^{2c_P}}{(1+e^{2c_P})^2}
% \left(
% \begin{bmatrix}
% \theta\\
% \bx
% \end{bmatrix}^{\top}
% \begin{bmatrix}
% \frac{n-1}{n} & \frac{1}{n^{3/2}} \sum_{i\neq m} Y^{*\top}_i\\
% \frac{1}{n^{3/2}} \sum_{i\neq m} Y^{*}_i & \frac{1}{n^2} \sum_{i\neq m} Y^{*}_i Y^{*\top}_i
% \end{bmatrix}
% \begin{bmatrix}
% \theta\\
% \bx
% \end{bmatrix}
% +
% \begin{bmatrix}
% \theta\\
% \by
% \end{bmatrix}^{\top}
% \begin{bmatrix}
% \frac{n-1}{n} & \frac{1}{n^{3/2}} \sum_{i\neq m} X^{*\top}_i\\
% \frac{1}{n^{3/2}} \sum_{i\neq m} X^{*}_i & \frac{1}{n^2} \sum_{i\neq m} X^{*}_i X^{*\top}_i
% \end{bmatrix}
% \begin{bmatrix}
% \theta\\
% \by
% \end{bmatrix}
% \right)\notag\\
% &\geq \frac{e^{2c_P}}{(1+e^{2c_P})^2}\left(
% \frac{2(n-1)}{n}\theta^2
% -\frac{\|X^*\|_{2,\infty}}{\sqrt{n}}(\theta^2+\|\bx\|_2^2)-\frac{\|Y^*\|_{2,\infty}}{\sqrt{n}}(\theta^2+\|\bx\|_2^2)+\frac{\sigma_{\min}}{2n^2}(\|\bx\|_2^2+\|\by\|_2^2)
% \right)\tag{by \eqref{ineq51:pf_lem_ncv3}, \eqref{ineq52:pf_lem_ncv3}}\\
% &\geq  \frac{e^{2c_P}}{(1+e^{2c_P})^2} 
% \left(
% \frac{2(n-1)}{n}\theta^2
% -\sqrt{\frac{\mu r \sigma_{\max}}{n^2}}(2\theta^2+\|\bx\|_2^2+\|\by\|_2^2)+\frac{\sigma_{\min}}{2n^2}(\|\bx\|_2^2+\|\by\|_2^2)
% \right)\notag\\
% &=  \frac{2e^{2c_P}}{(1+e^{2c_P})^2} \left(1-\frac{1}{n}-\sqrt{\frac{\mu r \sigma_{\max}}{n^2}}\right)\theta^2+ \frac{e^{2c_P}}{(1+e^{2c_P})^2}\left(\frac{\sigma_{\min}}{2n^2}-\sqrt{\frac{\mu r \sigma_{\max}}{n^2}}\right)(\|\bx\|_2^2+\|\by\|_2^2)\notag\\\label{ineq55:pf_lem_ncv3}
% &\geq \textcolor{red}{???}\left\|
% \begin{bmatrix}
% \theta\\
% \bx\\
% \by
% \end{bmatrix}
% \right\|^2_2.
% \end{align}
% Combine \eqref{ineq56:pf_lem_ncv3}, \eqref{ineq54:pf_lem_ncv3} and \eqref{ineq55:pf_lem_ncv3}, we have

By \eqref{ineq56:pf_lem_ncv3}, we then have
\begin{align*}
&\left\|A
\begin{bmatrix}
\theta^{t+1,(m)}_m-\theta^*_m\\
\left(F^{t+1,(m)}R^{t,(m)}-F^{*}\right)_{m,\cdot}\\
\left(F^{t+1,(m)}R^{t,(m)}-F^{*}\right)_{m+n,\cdot}
\end{bmatrix}
\right\|_2^2\notag\\
&\leq \left(1- \frac{4 \slD e^{2 c_P}}{(1+e^{2 c_P})^2}\eta +\frac{(1+e^{c_P})^4}{ e^{2 c_P}}\suD^2 \eta^2 \right)
\left\|
\begin{bmatrix}
\theta^{t+1,(m)}_m-\theta^*_m\\
\left(F^{t+1,(m)}R^{t,(m)}-F^{*}\right)_{m,\cdot}\\
\left(F^{t+1,(m)}R^{t,(m)}-F^{*}\right)_{m+n,\cdot}
\end{bmatrix}
\right\|_2^2\notag\\
&\leq \left(1-\frac{2 \slD e^{2 c_P}}{(1+e^{2 c_P})^2}\eta\right)\left\|
\begin{bmatrix}
\theta^{t+1,(m)}_m-\theta^*_m\\
\left(F^{t+1,(m)}R^{t,(m)}-F^{*}\right)_{m,\cdot}\\
\left(F^{t+1,(m)}R^{t,(m)}-F^{*}\right)_{m+n,\cdot}
\end{bmatrix}
\right\|_2^2
\end{align*}
as long as $\eta\leq \frac{2e^{4c_{P}}\slD}{(1+e^{2c_P})^6\suD^2}$.
Recall equation \eqref{ineq58:pf_lem_ncv3}. Consequently, we have
\begin{align*}
&\left\|
\begin{bmatrix}
\theta^{t+1,(m)}_m-\theta^*_m\\
\left(F^{t+1,(m)}R^{t,(m)}-F^{*}\right)_{m,\cdot}\\
\left(F^{t+1,(m)}R^{t,(m)}-F^{*}\right)_{m+n,\cdot}
\end{bmatrix}
\right\|_2\\
&\leq
\left\|A
\begin{bmatrix}
\theta^{t,(m)}_m-\theta^*_m\\
\left(F^{t,(m)}R^{t,(m)}-F^{*}\right)_{m,\cdot}\\
\left(F^{t,(m)}R^{t,(m)}-F^{*}\right)_{m+n,\cdot}
\end{bmatrix}
\right\|_2+|r_1|+\|r_2\|_2+\|r_3\|_2\\
&\leq \left(1-\frac{ \slD e^{2 c_P}}{(1+e^{2 c_P})^2}\eta\right)c_{31}+c\frac{\eta\sqrt{\overline{C}}}{\sqrt{n}}c_{21}+ c{\eta(\sqrt{\overline{C}}}+\sz)c_{11}+c\eta\sqrt{\frac{\log n}{n}}+c\eta\sqrt{\mu \sX\sY r^2 }c_{14}\\
&\quad +c\eta\left(\frac{1}{n^{3/2}} c_{11}c_{31} \sqrt{\mu r\sigma_{\max}}+\frac{1}{\sqrt{n}}c_{11}c_{31}+\frac{1}{n}\sqrt{\sigma_{\max}}\sz c_{11}+\frac{1}{n}\sqrt{\mu\sX\sY r^2 \sigma_{\max}}c_{14}+\lambda\sqrt{\mu\sX\sY r^2 n}\right)\\
&\leq c_{31}
\end{align*}
as long as $\max\{\sqrt{\overline{C}}\sz c_{11},\sqrt{\mu\sX\sY r^2 \overline{C}}c_{14}, \lambda\sqrt{\mu\sX\sY r^2 n}\}\lesssim \frac{ \slD e^{2 c_P}}{(1+e^{2 c_P})^2} c_{31}$.


\subsection{Proofs of Lemma \ref{lem:ncv4}}\label{pf:lem_ncv4}
Suppose Lemma \ref{lem:ncv1}-Lemma \ref{lem:ncv5} hold for the $t$-th iteration. In the following, we prove Lemma \ref{lem:ncv4} for the $(t+1)$-th iteration.
Since Lemma \ref{lem:ncv1}-Lemma \ref{lem:ncv5} hold for the $t$-th, we know Lemma \ref{lem:ncv1} holds for the $t+1$-th iteration, which implies $\|H^{t+1}-H^*\|_F\leq c_{11}\sqrt{n}$. For any fixed $m$, we have
\begin{align*}
|\theta^{t+1}_m-\theta^{*}_m|
&\leq |\theta^{t+1,(m)}_m-\theta^{*}_m|+|\theta^{t+1}_m-\theta^{t+1,(m)}_m|\\
&\leq |\theta^{t+1,(m)}_m-\theta^{*}_m|+\|\theta^{t+1}-\theta^{t+1,(m)}\|_2.
\end{align*}
It then holds that
\begin{align*}
\|\theta^{t+1}-\theta^*\|_{\infty}
&=\max_{1\leq m\leq n}|\theta^{t+1}_m-\theta^{*}_m|\\
&\leq \max_{1\leq m\leq n}|\theta^{t+1,(m)}_m-\theta^{*}_m|+\max_{1\leq m\leq n}\|\theta^{t+1}-\theta^{t+1,(m)}\|_2\\
&\leq c_{21}+c_{31}=c_{41},
\end{align*}
where the last inequality holds since Lemma \ref{lem:ncv2} and \ref{lem:ncv3} hold for the $(t+1)$-th iteration.

For $1\leq m\leq n$, we have
\begin{align*}
\left\|\left(F^{t+1}R^{t+1}-F^*\right)_{m,\cdot}\right\|_2
&\leq \left\|\left(F^{t+1,(m)}R^{t+1,(m)}-F^*\right)_{m,\cdot}\right\|_2+ \left\|\left(F^{t+1,(m)}R^{t+1,(m)}-F^{t+1}R^{t+1}\right)_{m,\cdot}\right\|_2\\
&\leq \left\|\left(F^{t+1,(m)}R^{t+1,(m)}-F^*\right)_{m,\cdot}\right\|_2+ \left\|F^{t+1,(m)}R^{t+1,(m)}-F^{t+1}R^{t+1}\right\|_F\\
&\leq \left\|\left(F^{t+1,(m)}R^{t+1,(m)}-F^*\right)_{m,\cdot}\right\|_2+ 5\kappa\left\|F^{t+1,(m)}O^{t+1,(m)}-F^{t+1}R^{t+1}\right\|_F,
\end{align*}
and 
\begin{align*}
\left\|\left(F^{t+1}R^{t+1}-F^*\right)_{m+n,\cdot}\right\|_2
&\leq \left\|\left(F^{t+1,(m)}R^{t+1,(m)}-F^*\right)_{m+n,\cdot}\right\|_2+ \left\|\left(F^{t+1,(m)}R^{t+1,(m)}-F^{t+1}R^{t+1}\right)_{m+n,\cdot}\right\|_2\\
&\leq \left\|\left(F^{t+1,(m)}R^{t+1,(m)}-F^*\right)_{m+n,\cdot}\right\|_2+ \left\|F^{t+1,(m)}R^{t+1,(m)}-F^{t+1}R^{t+1}\right\|_F\\
&\leq \left\|\left(F^{t+1,(m)}R^{t+1,(m)}-F^*\right)_{m+n,\cdot}\right\|_2+ 5\kappa\left\|F^{t+1,(m)}O^{t+1,(m)}-F^{t+1}R^{t+1}\right\|_F,
\end{align*}
where the last inequalities follow from Lemma \ref{ar:lem2}.
It then holds that
\begin{align*}
&\max_{1\leq m\leq n}\left\|\left(F^{t+1}R^{t+1}-F^*\right)_{m,\cdot}\right\|_2\\
&\leq \max_{1\leq m\leq n} \left\|\left(F^{t+1,(m)}R^{t+1,(m)}-F^*\right)_{m,\cdot}\right\|_2+5\kappa\max_{1\leq m\leq n}\left\|F^{t+1,(m)}O^{t+1,(m)}-F^{t+1}R^{t+1}\right\|_F\\
&\leq c_{31}+5\kappa c_{21}=c_{43},\\
&\max_{1\leq m\leq n}\left\|\left(F^{t+1}R^{t+1}-F^*\right)_{m+n,\cdot}\right\|_2\\
&\leq \max_{1\leq m\leq n} \left\|\left(F^{t+1,(m)}R^{t+1,(m)}-F^*\right)_{m+n,\cdot}\right\|_2+5\kappa\max_{1\leq m\leq n}\left\|F^{t+1,(m)}O^{t+1,(m)}-F^{t+1}R^{t+1}\right\|_F\\
&\leq c_{31}+5\kappa c_{21}=c_{43},\\
\end{align*}
where the last inequalities hold since Lemma \ref{lem:ncv2} and \ref{lem:ncv3} hold for the $(t+1)$-th iteration. 
We then finish the proof.











\subsection{Proofs of Lemma \ref{lem:ncv5}}\label{pf:lem_ncv5}
Suppose Lemma \ref{lem:ncv1}-Lemma \ref{lem:ncv5} hold for the $t$-th iteration. In the following, we prove Lemma \ref{lem:ncv5} for the $(t+1)$-th iteration.

First of all, we show that $X^{t+1}(Y^{t+1})^T=Y^{t+1}(X^{t+1})^T$. By the gradient decent update, we have
\begin{align*}
X^{t+1}=X^t-\eta\nabla_X f(M^t,F^t),\quad Y^{t+1}=Y^t-\eta\nabla_Y f(M^t,F^t).
\end{align*}
As a result, we have
\begin{align*}
X^{t+1}(Y^{t+1})^T
&=\left(X^t-\eta\nabla_X f(M^t,F^t)\right)\left(Y^t-\eta\nabla_Y f(M^t,F^t)\right)^T\\
&=X^{t}(Y^{t})^T-\eta X^t\nabla_Y f(M^t,F^t)^T-\eta\nabla_X f(M^t,F^t)(Y^{t})^T+\eta^2\nabla_X f(M^t,F^t)\nabla_Y f(M^t,F^t)^T\\
&=Y^{t}(X^{t})^T-\eta Y^{t}\nabla_X f(M^t,F^t)^T-\eta \nabla_Y f(M^t,F^t)^T (X^t)^T+\eta^2\nabla_Y f(M^t,F^t)\nabla_X f(M^t,F^t)^T\\
&=\left(Y^t-\eta\nabla_Y f(M^t,F^t)\right)\left(X^t-\eta\nabla_X f(M^t,F^t)\right)^T\\
&=Y^{t+1}(X^{t+1})^T,
\end{align*}
where the third equation holds since $X^{t}(Y^{t})^T=Y^{t}(X^{t})^T$. Similarly, we can show $X^{t+1,(m)}(Y^{t+1,(m)})^T=Y^{t+1,(m)}(X^{t+1,(m)})^T$.


Then, we show $\|(X^{t+1})^TX^{t+1}-(Y^{t+1})^TY^{t+1}\|_F\leq c_{51}\eta n^2$. We denote 
\begin{align*}
&A^t=(X^{t})^TX^{t}-(Y^{t})^TY^{t},\ A^{t+1}=(X^{t+1})^TX^{t+1}-(Y^{t+1})^TY^{t+1},\\
&D^t=\frac1n\sum_{i\neq j}\left(\frac{e^{P_{ij}^t}}{1+e^{P_{ij}^t}}-A_{ij}\right)e_i e_j^T.
\end{align*}
Same as Lemma 15 in \cite{chen2020noisy}, it can be seen that
\begin{align}\label{ineq1:lem_ncv5}
\|A^{t+1}\|_F\leq (1-\lambda\eta)\|A^{t}\|_F+\eta^2\|Y^{tT}D^{tT}D^{t}Y^{t}-X^{tT}D^{tT}D^{t}X^{t}\|_F.
\end{align}
Note that
\begin{align*}
\|Y^{tT}D^{tT}D^{t}Y^{t}-X^{tT}D^{tT}D^{t}X^{t}\|_F
&\leq     \|Y^{tT}D^{tT}D^{t}Y^{t}\|_F+\|X^{tT}D^{tT}D^{t}X^{t}\|_F\\
&\leq \|Y^t\|\|D^t\|^2\|Y^t\|_F+\|X^t\|\|D^t\|^2\|X^t\|_F.
\end{align*}
Moreover, by Lemma \ref{lem:ncv1} for the $t$-th iteration, we have
\begin{align*}
&\|X^t\|\leq \|X^tR^t-X^*\|+\|X^*\|\leq 2\|X^*\|,\quad  \|X^t\|_F\leq \|X^tR^t-X^*\|_F+\|X^*\|_F\leq 2\|X^*\|_F,\\
&\|Y^t\|\leq 2\|Y^*\|,\ \|Y^t\|_F\leq 2\|Y^*\|_F.
\end{align*}
Thus, we have
\begin{align*}
 \|Y^{tT}D^{tT}D^{t}Y^{t}-X^{tT}D^{tT}D^{t}X^{t}\|_F
 &\leq 4\|Y^*\|\|Y^*\|_F\|D^t\|^2+4\|X^*\|\|X^*\|_F  \|D^t\|^2
 &\lesssim \sqrt{\mu r}\sigma_{\max}\|D^t\|^2.
\end{align*}
By Lemma \ref{lem:gradient_spectral}, we have
\begin{align*}
 \|D^t\|&\lesssim \sqrt{\frac{c_{11}^2\overline{C}+\log n}{n}}.
\end{align*}
This implies
\begin{align}\label{ineq2:lem_ncv5}
 \|Y^{tT}D^{tT}D^{t}Y^{t}-X^{tT}D^{tT}D^{t}X^{t}\|_F   \lesssim \sqrt{\mu r}\sigma_{\max}\|D^t\|^2\lesssim \frac{\sqrt{\mu r}\sigma_{\max}(c_{11}^2\overline{C}+\log n)}{n}.
\end{align}
Combine \eqref{ineq1:lem_ncv5} and \eqref{ineq2:lem_ncv5}, we have
\begin{align*}
\|A^{t+1}\|_F
&\leq (1-\lambda\eta)\|A^{t}\|_F+C\eta^2\frac{\sqrt{\mu r}\sigma_{\max}(c_{11}^2\overline{C}+\log n)}{n}\\
&\leq (1-\lambda\eta)c_{51}\eta n^2+C\eta^2\frac{\sqrt{\mu r}\sigma_{\max}(c_{11}^2\overline{C}+\log n)}{n}\\
&\leq c_{51}\eta n^2
\end{align*}
as long as $\lambda\eta<1$ and $c_{51}\lambda n^3\gtrsim \sqrt{\mu r}\sigma_{\max} (c_{11}^2\overline{C}+\log n)$.
The upper bound on the leave-one-out sequences can be derived similarly.

Finally, we prove \eqref{ineq:gradient} in the following.
By the gradient descent update, we have
\begin{align*}
&f(M^{t+1},F^{t+1})\\
&=f(M^{t+1},F^{t+1}R^t)\\
&=f\left(M^t-\eta\nabla_{M}f(M^t,F^t)+\eta
\begin{bmatrix}
\mean\left(\nabla_{\theta}f(M^t,F^t)\right)\cdot\mathbf{1}\\
0
\end{bmatrix}, \left(F^t-\eta\nabla_F f(M^t,F^t)\right)R^t\right)\\
&=f(M^t,F^tR^t)-\eta\left\langle\nabla_M f(M^t,F^tR^t),\nabla_{M}f(M^t,F^t)-
\begin{bmatrix}
\mean\left(\nabla_{\theta}f(M^t,F^t)\right)\cdot\mathbf{1}\\
0
\end{bmatrix} \right\rangle\\
&\quad -\eta\left\langle\nabla_F f(M^t,F^tR^t),\nabla_F f(M^t,F^tR^t)\right\rangle\\
&\quad +\frac{\eta^2}{2}
\vec\begin{bmatrix}
\nabla_{M}f(M^t,F^t)-
\begin{bmatrix}
\mean\left(\nabla_{\theta}f(M^t,F^t)\right)\cdot\mathbf{1}\\
0
\end{bmatrix}\\
\nabla_F f(M^t,F^tR^t)
\end{bmatrix}^T \nabla^2 f(\tilde{M},\tilde{F})
\vec\begin{bmatrix}
\nabla_{M}f(M^t,F^t)-
\begin{bmatrix}
\mean\left(\nabla_{\theta}f(M^t,F^t)\right)\cdot\mathbf{1}\\
0
\end{bmatrix}\\
\nabla_F f(M^t,F^tR^t)
\end{bmatrix}\\
&=f(M^t,F^tR^t)-\eta\left\|\nabla_{M}f(M^t,F^t)-
\begin{bmatrix}
\mean\left(\nabla_{\theta}f(M^t,F^t)\right)\cdot\mathbf{1}\\
0
\end{bmatrix} \right\|_F^2 -\eta\left\|\nabla_F f(M^t,F^tR^t)\right\|^2_{F}\\
&\quad +\frac{\eta^2}{2}
\vec\begin{bmatrix}
\nabla_{M}f(M^t,F^t)-
\begin{bmatrix}
\mean\left(\nabla_{\theta}f(M^t,F^t)\right)\cdot\mathbf{1}\\
0
\end{bmatrix}\\
\nabla_F f(M^t,F^tR^t)
\end{bmatrix}^T \nabla^2 f(\tilde{M},\tilde{F})
\vec\begin{bmatrix}
\nabla_{M}f(M^t,F^t)-
\begin{bmatrix}
\mean\left(\nabla_{\theta}f(M^t,F^t)\right)\cdot\mathbf{1}\\
0
\end{bmatrix}\\
\nabla_F f(M^t,F^tR^t)
\end{bmatrix},
\end{align*}
where the last equation follows from the fact that
\begin{align*}
 \left\langle\begin{bmatrix}
\mean\left(\nabla_{\theta}f(M^t,F^t)\right)\cdot\mathbf{1}\\
0
\end{bmatrix},\nabla_{M}f(M^t,F^t)-
\begin{bmatrix}
\mean\left(\nabla_{\theta}f(M^t,F^t)\right)\cdot\mathbf{1}\\
0
\end{bmatrix} \right\rangle   =0.
\end{align*}
By Lemma \ref{lem:convexity}, we have 
\begin{align*}
& \vec\begin{bmatrix}
\nabla_{M}f(M^t,F^t)-
\begin{bmatrix}
\mean\left(\nabla_{\theta}f(M^t,F^t)\right)\cdot\mathbf{1}\\
0
\end{bmatrix}\\
\nabla_F f(M^t,F^tR^t)
\end{bmatrix}^T \nabla^2 f(\tilde{M},\tilde{F})
\vec\begin{bmatrix}
\nabla_{M}f(M^t,F^t)-
\begin{bmatrix}
\mean\left(\nabla_{\theta}f(M^t,F^t)\right)\cdot\mathbf{1}\\
0
\end{bmatrix}\\
\nabla_F f(M^t,F^tR^t)
\end{bmatrix}\\
&\leq \overline{C}\left( \left\|\nabla_{M}f(M^t,F^t)-
\begin{bmatrix}
\mean\left(\nabla_{\theta}f(M^t,F^t)\right)\cdot\mathbf{1}\\
0
\end{bmatrix}\right\|_F^2
+\left\|\nabla_F f(M^t,F^tR^t)\right\|_F^2\right).
\end{align*}
Thus, it holds that
\begin{align*}
&f(M^{t+1},F^{t+1})\\
&\leq f(M^t,F^tR^t)-\left(\eta-\frac{\overline{C}}{2}\eta^2\right)\left(\left\|\nabla_{M}f(M^t,F^t)-
\begin{bmatrix}
\mean\left(\nabla_{\theta}f(M^t,F^t)\right)\cdot\mathbf{1}\\
0
\end{bmatrix} \right\|_F^2+\left\|\nabla_F f(M^t,F^tR^t)\right\|^2_{F}\right) \\
&\leq f(M^t,F^tR^t)-\frac{\eta}{2}\left(\left\|\nabla_{M}f(M^t,F^t)-
\begin{bmatrix}
\mean\left(\nabla_{\theta}f(M^t,F^t)\right)\cdot\mathbf{1}\\
0
\end{bmatrix} \right\|_F^2+\left\|\nabla_F f(M^t,F^tR^t)\right\|^2_{F}\right)\\
&= f(M^t,F^t)-\frac{\eta}{2}
\left\|
\nabla f(M^t,F^t)
-
\begin{bmatrix}
\mean\left(\nabla_{\theta}f(M^t,F^t)\right)\cdot\mathbf{1}\\
0
\end{bmatrix} 
\right\|_F^2
\end{align*}
as long as $\overline{{C}}\eta\leq 1$. We then finish the proofs.











\subsection{Proofs of Lemma \ref{lem:ncv6}}\label{pf:lem_ncv6}
\begin{proof}
Summing \eqref{ineq:gradient} from $t=1$ to $t=t_0$ leads to 
\begin{align*}
&f(M^{t_0},F^{t_0})\leq f(M^{0},F^{0})-\frac{\eta}{2}\sum^{t_0-1}_{t=0}\left\|
\nabla f(M^t,F^t)
-
\begin{bmatrix}
\mean\left(\nabla_{\theta}f(M^t,F^t)\right)\cdot\mathbf{1}\\
0
\end{bmatrix} 
\right\|_F^2.
\end{align*}
Thus, we have
\begin{align}\label{ineq2:lem_ncv6}
&\min_{0\leq t<t_0}\left\|
\nabla f(M^t,F^t)
-
\begin{bmatrix}
\mean\left(\nabla_{\theta}f(M^t,F^t)\right)\cdot\mathbf{1}\\
0
\end{bmatrix} 
\right\|_F\notag\\
&\leq \left(\frac{1}{t_0}\sum^{t_0-1}_{t=0}\left\|
\nabla f(M^t,F^t)
-
\begin{bmatrix}
\mean\left(\nabla_{\theta}f(M^t,F^t)\right)\cdot\mathbf{1}\\
0
\end{bmatrix} 
\right\|_F^2\right)^{1/2}\notag\\
&\leq \left(\frac{2}{\eta t_0}\left(f(M^*,F^*)-f(M^{t_0},F^{t_0})\right)\right)^{1/2},
\end{align}
where we use the fact that $(M^0,F^0)=(M^*,F^*)$. 
Thus, it remains to control $f(M^*,F^*)-f(M^{t_0},F^{t_0})$. Note that
\begin{align*}
 f(M^{t_0},F^{t_0})
 &=f(M^{t_0},F^{t_0}R^{t_0})\\
 &=f(M^*,F^*)+\left\langle\nabla f(M^*,F^*),
 \begin{bmatrix}
M^{t_0}-M^*\\
F^{t_0}R^{t_0}-F^*
 \end{bmatrix}
 \right\rangle\\
 &\quad+\frac12\vec\left(
 \begin{bmatrix}
M^{t_0}-M^*\\
F^{t_0}R^{t_0}-F^*
 \end{bmatrix}
 \right)^T \nabla^2 f(\tilde{M},\tilde{F})
 \vec\left(
 \begin{bmatrix}
M^{t_0}-M^*\\
F^{t_0}R^{t_0}-F^*
 \end{bmatrix}
 \right),
\end{align*}
where $(\tilde{M},\tilde{F})$ lies in the line segment connecting $(M^*,F^*)$ and $(M^{t_0},F^{t_0}R^{t_0})$. By triangle inequality, we have
\begin{align}\label{ineq1:lem_ncv6}
 &f(M^*,F^*)- f(M^{t_0},F^{t_0})\notag\\
 &\leq \|\nabla_{\theta} f(M^*,F^*)\|_2\|\theta^{t_0}-\theta^*\|_2+\|\nabla_{H} f(M^*,F^*)\|_F\|H^{t_0}-H^*\|_F+\|\nabla_{F} f(M^*,F^*)\|_F\|F^{t_0}R^{t_0}-F^*\|_F\notag\\
 &\quad+\frac12\left|\vec\left(
 \begin{bmatrix}
M^{t_0}-M^*\\
F^{t_0}R^{t_0}-F^*
 \end{bmatrix}
 \right)^T \nabla^2 f(\tilde{M},\tilde{F})
 \vec\left(
 \begin{bmatrix}
M^{t_0}-M^*\\
F^{t_0}R^{t_0}-F^*
 \end{bmatrix}
 \right)\right|.
\end{align}
By the gradient decent updating rule, we have $\mathbf{1}^T{\theta^{t_0}}=0$ and thus $\mathbf{1}^T\tilde{\theta}=0$.
Moreover, by Lemma \ref{lem:ncv4}, it holds that
\begin{align*}
&\|\tilde{\theta}-\theta^*\|_{\infty}\leq \|{\theta}^{t_0}-\theta^*\|_{\infty}\leq c_{41}\leq c_1,\\
&\|\tilde{H}-H^*\|_{F}\leq \|{H}^{t_0}-H^*\|_{F}\leq c_{11}\sqrt{n}\leq c_2\sqrt{n},\\
&\|\tilde{F}-F^*\|_{2,\infty}\leq \|{F}^{t_0}{R}^{t_0}-F^*\|_{\infty}\leq c_{43}\leq c_3.
\end{align*}
Thus, by Lemma \ref{lem:convexity}, we have
\begin{align*}
&\frac{1}{2}\left|\vec\left(
 \begin{bmatrix}
M^{t_0}-M^*\\
F^{t_0}R^{t_0}-F^*
 \end{bmatrix}
 \right)^T \nabla^2 f(\tilde{M},\tilde{F})
 \vec\left(
 \begin{bmatrix}
M^{t_0}-M^*\\
F^{t_0}R^{t_0}-F^*
 \end{bmatrix}
 \right)\right|\\
 &\leq \frac{\overline{C}}{2}\left\|
  \begin{bmatrix}
M^{t_0}-M^*\\
F^{t_0}R^{t_0}-F^*
 \end{bmatrix}
 \right\|_F^2\\
 & \leq \frac{\overline{C} c_{11}^2 n}{2},
\end{align*}
where the last inequality follows from Lemma \ref{lem:ncv1}.


Consequently, by \eqref{ineq1:lem_ncv6} and Lemma \ref{lem:gradient_norm}, we have shown that
\begin{align*}
&f(M^*,F^*)- f(M^{t_0},F^{t_0})\\
&\lesssim \sqrt{n\log n}\|\theta^{t_0}-\theta^*\|_2+\sz\sqrt{p\log n}\|H^{t_0}-H^*\|_F+\lambda \sqrt{\mu r\sigma_{\max}}\|F^{t_0}R^{t_0}-F^*\|_F+\overline{C} c_{11}^2 n,
\end{align*}
where we use the fact that $\|X^*\|_F\leq \sqrt{\mu r \sigma_{\max}}$ by Assumption \ref{assumption:incoherent}.
By Lemma \ref{lem:ncv1}, this further implies that
\begin{align*}
&f(M^*,F^*)- f(M^{t_0},F^{t_0})\\
&\lesssim (\sqrt{n\log n}+\sz\sqrt{p\log n}+\lambda \sqrt{\mu r\sigma_{\max}})\cdot c_{11}\sqrt{n}+\overline{C} c_{11}^2 n\\
&= \left(\sqrt{n\log n}+\sz\sqrt{p\log n}+c_{\lambda}\sqrt{\frac{\mu r\sigma_{\max}\log n}{n}}\right)\cdot c_{11}\sqrt{n}+\overline{C} c_{11}^2 n\\
&\lesssim n^2
\end{align*}
as long as $c_{11}\left(\sqrt{\log n}+\sz\sqrt{\log n}+c_{\lambda}\sqrt{\frac{\mu r\sigma_{\max}\log n}{n^2}}+\overline{C}c_{11}\right)\lesssim n$.
Thus, we have
\begin{align*}
\frac{2}{\eta t_0}\left(f(M^*,F^*)-f(M^{t_0},F^{t_0})\right)\lesssim\frac{n^2}{\eta t_0}\leq n^{-10}
\end{align*}
as long as $\eta t_0\geq n^{12}$ (which holds as long as $t_0$ large enough). Together with \eqref{ineq2:lem_ncv6}, we finish the proofs.

\end{proof}

==> proof_Lem3.3_v1.tex <==
\subsection{Proofs of Lemma \ref{lem:ncv3}}\label{pf:lem_ncv3}
Suppose Lemma \ref{lem:ncv1}-Lemma \ref{lem:ncv5} hold for the $t$-th iteration. In the following, we prove Lemma \ref{lem:ncv3} for the $(t+1)$-th iteration. 













First of all, for any fixed $m$, we will show that $|\theta^{t+1,(m)}_m-\theta^*_m|\leq c_{31}$.
Note that by the gradient descent update, we have
\begin{align*}
&\theta^{t+1,(m)}_m-\theta^*_m\\
&=\theta^{t,(m)}_m-\theta^*_m
-\frac{2\eta}{\sqrt{n}}\sum_{i\neq m}\left(\frac{e^{P^{t,(m)}_{im}}}{1+e^{P^{t,(m)}_{im}}}-\frac{e^{P^{*}_{im}}}{1+e^{P^{*}_{im}}}\right)+\eta\cdot\mean\left(\nabla_{\theta}L^{(m)}(M^{t,(m)}, F^{t,(m)})\right),
\end{align*}
where we use the symmetry of $X^{t,(m)}(Y^{t,(m)})^T$ obtained via Lemma \ref{lem:ncv5}.
By the mean value theorem, we have for some $\{c_i\}$ that
\begin{align*}
& \sum_{i\neq m}\left(\frac{e^{P^{t,(m)}_{im}}}{1+e^{P^{t,(m)}_{im}}}-\frac{e^{P^{*}_{im}}}{1+e^{P^{*}_{im}}}\right)\\
&= \sum_{i\neq m}\frac{e^{c_i}}{(1+e^{c_i})^2}\left(P^{t,(m)}_{im}-P^{*}_{im}\right)\\
& = \sum_{i\neq m}\frac{e^{c_i}}{(1+e^{c_i})^2}\left(\frac{1}{\sqrt{n}}\left(\theta^{t,(m)}_i-\theta^{*}_i+\theta^{t,(m)}_m-\theta^{*}_m\right)+\langle H^{t,(m)}-H^*,z_iz_m^T\rangle+\frac1n \left(X^{t,(m)}(Y^{t,(m)})^T-X^{*}Y^{*T}\right)_{im}\right)\\
& = \left(\frac{1}{\sqrt{n}}\sum_{i\neq m}\frac{e^{c_i}}{(1+e^{c_i})^2}\right)\left(\theta^{t,(m)}_m-\theta^{*}_m\right)\\
&\quad+\sum_{i\neq m}\frac{e^{c_i}}{(1+e^{c_i})^2}\left(\frac{1}{\sqrt{n}}\left(\theta^{t,(m)}_i-\theta^{*}_i\right)+\langle H^{t,(m)}-H^*,z_iz_m^T\rangle+\frac1n \left(X^{t,(m)}(Y^{t,(m)})^T-X^{*}Y^{*T}\right)_{im}\right).
\end{align*}
Thus, it holds that
\begin{align}\label{eq1:lem_ncv3}
 &\theta^{t+1,(m)}_m-\theta^*_m\notag\\
 &=\left(1-\frac{2\eta}{n}\sum_{i\neq m}\frac{e^{c_i}}{(1+e^{c_i})^2}\right)\left(\theta^{t,(m)}_m-\theta^*_m\right)
+\eta\cdot\mean\left(\nabla_{\theta}L^{(m)}(M^{t,(m)}, F^{t,(m)})\right)\notag\\
&\quad -\frac{2\eta}{\sqrt{n}}\sum_{i\neq m}\frac{e^{c_i}}{(1+e^{c_i})^2}\left(\frac{1}{\sqrt{n}}\left(\theta^{t,(m)}_i-\theta^{*}_i\right)+\langle H^{t,(m)}-H^*,z_iz_m^T\rangle+\frac1n \left(X^{t,(m)}(Y^{t,(m)})^T-X^{*}Y^{*T}\right)_{im}\right)
\end{align}
In the following, we bound the second and third terms, respectively.
\begin{enumerate}
\item  For the second term, note that
\begin{align*}
&\left|\mean\left(\nabla_{\theta}L^{(m)}(M^{t,(m)}, F^{t,(m)})\right)\right|\\
&=\left|\mean\left(\nabla_{\theta}L^{(m)}(M^{t,(m)}, F^{t,(m)}O^{t,(m)})\right)\right|\\
&\leq \left|\mean\left(\nabla_{\theta}L^{(m)}(M^{t,(m)}, F^{t,(m)}O^{t,(m)})-\nabla_{\theta}L(M^{t}, F^{t}R^{t})\right)\right|+ \left|\mean\left(\nabla_{\theta}L(M^{t}, F^{t}R^{t})\right)\right|.
\end{align*}
For the first part, we have the following claim.
\begin{claim}\label{claim1:gradient_mean}
It holds that
\begin{align*}
 & \left|\mean\left(\nabla_{\theta}L^{(m)}(M^{t,(m)}, F^{t,(m)}O^{t,(m)})-\nabla_{\theta}L(M^{t}, F^{t}R^{t})\right)\right|\\
 & \lesssim   \sqrt{\frac{\su}{n}}\left(\|\theta^t-\theta^{t,(m)}\|_2+\|H^t-H^{t,(m)}\|_F+\frac{1}{n}\|X^*\|\|F^tR^t-F^{t,(m)}O^{t,(m)}\|_F\right)+\sqrt{\frac{\log n}{n}}.
\end{align*}
\end{claim}
\begin{proof}[Proof of Claim \ref{claim1:gradient_mean}]
 Note that
\begin{align*}
&\left|\mean\left(\nabla_{\theta}L(M^t,F^tR^t)-\nabla_{\theta}L^{(m)}(M^{t,(m)},F^{t,(m)}O^{t,(m)})\right)\right|\\
&\leq\left|\mean\left(\nabla_{\theta}L(M^t,F^tR^t)-\nabla_{\theta}L(M^{t,(m)},F^{t,(m)}O^{t,(m)})\right)\right|\\
&\quad+\left|\mean\left(\nabla_{\theta}L(M^{t,(m)},F^{t,(m)}O^{t,(m)})-\nabla_{\theta}L^{(m)}(M^{t,(m)},F^{t,(m)}O^{t,(m)})\right)\right|\\
\end{align*}
For the first term, we have
\begin{align*}
&\mean\left(\nabla_{\theta}L(M^t,F^tR^t)-\nabla_{\theta}L(M^{t,(m)},F^{t,(m)}O^{t,(m)})\right)\\
&=\frac{2}{n^{3/2}}\sum_{i\neq j}\left(\frac{e^{P_{ij}^{t}}}{1+e^{P_{ij}^{t}}}-\frac{e^{P_{ij}^{t,(m)}}}{1+e^{P_{ij}^{t,(m)}}}\right)\\
&\leq \frac{1}{2n^{3/2}}\sum_{i\neq j}\left|P^t_{ij}-P^{t,(m)}_{ij}\right| \tag{by mean-value theorem}\\
&\leq \frac{1}{2\sqrt{n}}\sqrt{\sum_{i\neq j}\left|P^t_{ij}-P^{t,(m)}_{ij}\right|^2}. \tag{by Cauchy-Schwarz}
\end{align*}

Note that
\begin{align*}
&\sum_{i\neq j}(P_{ij}^{t}-P_{ij}^{t,(m)})^2\\
&=\sum_{i\neq j}\left(\frac{1}{\sqrt{n}}\langle\theta^{t}-\theta^{t,(m)},e_i+e_j\rangle+\langle H^{t}-H^{t,(m)},z_iz_j^T\rangle+\frac1n\langle X^{t}Y^{tT}-X^{t,(m)}Y^{t,(m) T},e_i e_j^T\rangle\right)^2\\
&=
\begin{bmatrix}
  \vec(\theta^{t}-\theta^{t,(m)})\\
  \vec(H^{t}-H^{t,(m)})\\
  \frac1n\vec(X^{t}Y^{tT}-X^{t,(m)}Y^{t,(m) T})
\end{bmatrix}^T
\left(\sum_{i\neq j}
  \begin{bmatrix}
  \frac{1}{\sqrt{n}}\vec(e_i+e_j)\\
  \vec(z_iz_j^T)\\
  \vec(e_ie_j^T)
  \end{bmatrix}
   \begin{bmatrix}
  \frac{1}{\sqrt{n}}\vec(e_i+e_j)\\
  \vec(z_iz_j^T)\\
  \vec(e_ie_j^T)
  \end{bmatrix}^T
\right)
\begin{bmatrix}
  \vec(\theta^{t}-\theta^{t,(m)})\\
  \vec(H^{t}-H^{t,(m)})\\
  \frac1n\vec(X^{t}Y^{tT}-X^{t,(m)}Y^{t,(m) T})
\end{bmatrix}\\
&\leq \su \left\|\begin{bmatrix}
  \vec(\theta^{t}-\theta^{t,(m)})\\
  \vec(H^{t}-H^{t,(m)})\\
  \frac1n\vec(X^{t}Y^{tT}-X^{t,(m)}Y^{t,(m) T})
\end{bmatrix}\right\|^2 \tag{by Assumption \ref{assumption:eigenvalues} and $\mathbf{1}^T(\theta^t-\theta^{t,(m)})=0$}\\
& =\su\left(\|\theta^t-\theta^{t,(m)}\|^2_{2}+\|H^t-H^{t,(m)}\|^2_{F}+\frac{1}{n^2}\|X^tY^{tT}-X^{t,(m)}Y^{t,(m) T}\|^2_{F}\right).
\end{align*}
As a result, we have
\begin{align*}
&\left|\mean\left(\nabla_{\theta}L(M^t,F^tR^t)-\nabla_{\theta}L(M^{t,(m)},F^{t,(m)}O^{t,(m)})\right)\right|\\
&\lesssim \sqrt{\frac{\su}{n}}\left(\|\theta^t-\theta^{t,(m)}\|_{2}+\|H^t-H^{t,(m)}\|_{F}+\frac{1}{n}\|X^tY^{tT}-X^{t,(m)}Y^{t,(m) T}\|_{F}\right)\\
&\lesssim \sqrt{\frac{\su}{n}}\left(\|\theta^t-\theta^{t,(m)}\|_2+\|H^t-H^{t,(m)}\|_F+\frac{1}{n}\|X^*\|\|F^tR^t-F^{t,(m)}O^{t,(m)}\|_F\right).
\end{align*}

For the second term, note that
\begin{align*}
 &\nabla_{\theta}L(M^{t,(m)},F^{t,(m)}O^{t,(m)})-\nabla_{\theta}L^{(m)}(M^{t,(m)},F^{t,(m)}O^{t,(m)})\\
 &=\frac{2}{\sqrt{n}}\sum_{i\neq m}\left(\frac{e^{P_{im}^*}}{1+e^{P_{im}^*}}-A_{im}\right)(e_i+e_m).
\end{align*}
Thus, we have
\begin{align*}
&\left|\mean\left(\nabla_{\theta}L(M^{t,(m)},F^{t,(m)}O^{t,(m)})-\nabla_{\theta}L^{(m)}(M^{t,(m)},F^{t,(m)}O^{t,(m)})\right)\right|\\
&\leq \frac1n \left\|\frac{2}{\sqrt{n}}\sum_{i\neq m}\left(\frac{e^{P_{im}^*}}{1+e^{P_{im}^*}}-A_{im}\right)(e_i+e_m)\right\|_1\\
&\leq \frac{1}{\sqrt{n}}\left\|\frac{2}{\sqrt{n}}\sum_{i\neq m}\left(\frac{e^{P_{im}^*}}{1+e^{P_{im}^*}}-A_{im}\right)(e_i+e_m)\right\|_2\\
&\lesssim \sqrt{\frac{\log n}{n}} \tag{by \eqref{ineq1:lem_ncv2}}.
\end{align*}
Combining the above two terms, we then finish the proof.  
\end{proof}

For the second part, we have the following claim.
\begin{claim}\label{claim2:gradient_mean}
It holds that
\begin{align*}
 & \left|\mean\left(\nabla_{\theta}L(M^{t}, F^{t}R^{t})\right)\right|\\
 & \lesssim  \sqrt{\frac{\su}{n}}\left(\|\theta^t-\theta^{*}\|_{2}+\|H^t-H^{*}\|_{F}+\frac{1}{n}\|X^*\|\|F^tR^t-F^{*}\|_{F}\right)+\sqrt{\frac{\log n}{n}}.
\end{align*}
\end{claim}
\begin{proof}[Proof of Claim \ref{claim2:gradient_mean}]
Note that
\begin{align*}
\nabla_{\theta}L(M^t,F^tR^t)=\nabla_{\theta}L(M^*,F^*)+\nabla_{\theta}L(M^t,F^tR^t)-\nabla_{\theta}L(M^*,F^*).
\end{align*}
For the first term, by Lemma \ref{lem:gradient_norm}, we have
\begin{align*}
\left| \mean\left(\nabla_{\theta}L(M^*,F^*)\right)\right|\leq \frac{1}{\sqrt{n}}\left\|\nabla_{\theta}L(M^*,F^*)\right\|_2\lesssim \sqrt{\frac{\log n}{n}}.
\end{align*}
For the rest of the terms, same as the proof of Claim \ref{claim1:gradient_mean}, we have
\begin{align*}
\left|\mean\left(\nabla_{\theta}L(M^t,F^tR^t)-\nabla_{\theta}L(M^*,F^*)\right)\right|
\lesssim \sqrt{\frac{\su}{n}}\left(\|\theta^t-\theta^{*}\|_{2}+\|H^t-H^{*}\|_{F}+\frac{1}{n}\|X^*\|\|F^tR^t-F^{*}\|_{F}\right).
\end{align*}
Combining the above two terms, we then finish the proof.


% For the rest of the terms, we have 
% \begin{align*}
% &n\cdot \mean\left(\nabla_{\theta}L(M^t,F^tR^t)-\nabla_{\theta}L(M^*,F^*)\right)\\
% &=\frac{2}{\sqrt{n}}\sum_{i\neq j}\left(\frac{e^{P_{ij}^{t}}}{1+e^{P_{ij}^{t}}}-\frac{e^{P_{ij}^{*}}}{1+e^{P_{ij}^{*}}}\right)\\
% &\leq \frac{1}{2\sqrt{n}}\sum_{i\neq j}\left|P^t_{ij}-P^{*}_{ij}\right| \tag{by mean-value theorem}\\
% &\leq \frac{\sqrt{n}}{2}\sqrt{\sum_{i\neq j}\left|P^t_{ij}-P^{*}_{ij}\right|^2}. \tag{by Cauchy-Schwarz}
% \end{align*}
% Note that
% \begin{align*}
% &\sum_{i\neq j}(P_{ij}^{t}-P_{ij}^*)^2\\
% &=\sum_{i\neq j}\left(\frac{1}{\sqrt{n}}\langle\theta^{t}-\theta^*,e_i+e_j\rangle+\langle H^{t}-H^*,z_iz_j^T\rangle+\frac1n\langle X^{t}Y^{tT}-X^*Y^{*T},e_i e_j^T\rangle\right)^2\\
% &=
% \begin{bmatrix}
%   \vec(\theta^{t}-\theta^*)\\
%   \vec(H^{t}-H^*)\\
%   \frac1n\vec(X^{t}Y^{tT}-X^*Y^{*T})
% \end{bmatrix}^T
% \left(\sum_{i\neq j}
%   \begin{bmatrix}
%   \frac{1}{\sqrt{n}}\vec(e_i+e_j)\\
%   \vec(z_iz_j^T)\\
%   \vec(e_ie_j^T)
%   \end{bmatrix}
%    \begin{bmatrix}
%   \frac{1}{\sqrt{n}}\vec(e_i+e_j)\\
%   \vec(z_iz_j^T)\\
%   \vec(e_ie_j^T)
%   \end{bmatrix}^T
% \right)
% \begin{bmatrix}
%   \vec(\theta^{t}-\theta^*)\\
%   \vec(H^{t}-H^*)\\
%   \frac1n\vec(X^{t}Y^{tT}-X^*Y^{*T})
% \end{bmatrix}\\
% &\lesssim \left\|\begin{bmatrix}
%   \vec(\theta^{t}-\theta^*)\\
%   \vec(H^{t}-H^*)\\
%   \frac1n\vec(X^{t}Y^{tT}-X^*Y^{*T})
% \end{bmatrix}\right\|^2 \tag{by balanced eigenvalues assumption and $\mathbf{1}^T(\theta^t-\theta^*)=0$}\\
% & =\|\theta^t-\theta^{*}\|^2_{2}+\|H^t-H^{*}\|^2_{F}+\frac{1}{n^2}\|X^tY^{tT}-X^{*}Y^{*T}\|^2_{F}.
% \end{align*}
% As a result, we have
% \begin{align*}
% \left|\mean\left(\nabla_{\theta}L(M^t,F^tR^t)-\nabla_{\theta}L(M^*,F^*)\right)\right|
% \lesssim \frac{1}{\sqrt{{n}}}\left(\|\theta^t-\theta^{*}\|_{2}+\|H^t-H^{*}\|_{F}+\frac{1}{n}\|X^tY^{tT}-X^{*}Y^{*T}\|_{F}\right).
% \end{align*}
% Combine the above results, we show that
% \begin{align*}
%  \left|\mean\left(\nabla_{\theta}f(M^t,F^tR^t)\right)\right| 
%  \lesssim O\left(\sqrt{\frac{\log n}{n}}\right)+\frac{1}{\sqrt{{n}}}\left(\|\theta^t-\theta^{*}\|_{2}+\|H^t-H^{*}\|_{F}+\frac{1}{n}\|X^tY^{tT}-X^{*}Y^{*T}\|_{F}\right),
% \end{align*}
% which implies
% \begin{align*}
%  (4)
%  \lesssim O\left(\sqrt{\log n}\right)+\|\theta^t-\theta^{*}\|_{2}+\|H^t-H^{*}\|_{F}+\frac{1}{n}\|X^tY^{tT}-X^{*}Y^{*T}\|_{F}.
% \end{align*}
\end{proof}

By Claim \ref{claim1:gradient_mean} and \ref{claim2:gradient_mean}, we have
\begin{align}\label{ineq1:lem_ncv3}
&\left|\mean\left(\nabla_{\theta}L^{(m)}(M^{t,(m)}, F^{t,(m)})\right)\right|\notag\\
&\lesssim \sqrt{\frac{\su}{n}}\left(\|\theta^t-\theta^{t,(m)}\|_2+\|H^t-H^{t,(m)}\|_F+\frac{1}{n}\|X^*\|\|F^tR^t-F^{t,(m)}O^{t,(m)}\|_F\right)\notag\\
&\quad + \sqrt{\frac{\su}{n}}\left(\|\theta^t-\theta^{*}\|_{2}+\|H^t-H^{*}\|_{F}+\frac{1}{n}\|X^*\|\|F^tR^t-F^*\|_F\right)+O\left(\sqrt{\frac{\log n}{n}}\right).
\end{align}


\item For the third term, note that
\begin{align*}
&\left|\sum_{i\neq m}\frac{e^{c_i}}{(1+e^{c_i})^2}\left(\frac{1}{\sqrt{n}}\left(\theta^{t,(m)}_i-\theta^{*}_i\right)+\langle H^{t,(m)}-H^*,z_iz_m\rangle+\frac1n \left(X^{t,(m)}(Y^{t,(m)})^T-X^{*}Y^{*T}\right)_{im}\right)\right|\\
&\leq \frac14\sum_{i\neq m}\frac{1}{\sqrt{n}}\left|\theta^{t,(m)}_i-\theta^{*}_i\right|+\left|\langle H^{t,(m)}-H^*,z_iz_m^T\rangle\right|+\frac1n \left|\left(X^{t,(m)}(Y^{t,(m)})^T-X^{*}Y^{*T}\right)_{im}\right|\\
&\leq \|\theta^{t,(m)}-\theta^{*}\|_2+\| H^{t,(m)}-H^*\|\sum_{i\neq m}\|z_i\|\|z_m\|+\frac{1}{\sqrt{n}}\left\|\left(X^{t,(m)}(Y^{t,(m)})^T-X^{*}Y^{*T}\right)_{\cdot,m}\right\|_2\\
&\leq \|\theta^{t,(m)}-\theta^{*}\|_2+\sz\| H^{t,(m)}-H^*\|+\frac{1}{\sqrt{n}}\left\|\left(X^{t,(m)}(Y^{t,(m)})^T-X^{*}Y^{*T}\right)_{\cdot,m}\right\|_2,
\end{align*}
where the second inequality follows from the Cauchy-Schwarz inequality.
Notice that
\begin{align*}
X^{t,(m)}(Y^{t,(m)})^T-X^{*}Y^{*T}=\left(X^{t,(m)}R^{t,(m)}-X^{*}\right)\left(Y^{t,(m)}R^{t,(m)}\right)^T+X^*\left(Y^{t,(m)}R^{t,(m)}-Y^{*}\right)^T.
\end{align*}
Thus, we have
\begin{align*}
&\left(X^{t,(m)}(Y^{t,(m)})^T-X^{*}Y^{*T}\right)_{\cdot,m}\\
&=\left(X^{t,(m)}R^{t,(m)}-X^{*}\right)\left(Y^{t,(m)}R^{t,(m)}\right)_{m,\cdot}+X^*\left(Y^{t,(m)}R^{t,(m)}-Y^{*}\right)_{m,\cdot},
\end{align*}
which implies
\begin{align*}
&\left\|\left(X^{t,(m)}(Y^{t,(m)})^T-X^{*}Y^{*T}\right)_{\cdot,m}\right\|_2\\
&\leq \left\|\left(X^{t,(m)}R^{t,(m)}-X^{*}\right)\left(Y^{t,(m)}R^{t,(m)}\right)_{m,\cdot}\right\|_2+\left\|X^*\left(Y^{t,(m)}R^{t,(m)}-Y^{*}\right)_{m,\cdot}\right\|_2\\
&\leq \left\|X^{t,(m)}R^{t,(m)}-X^{*}\right\|\left\|\left(Y^{t,(m)}R^{t,(m)}\right)_{m,\cdot}\right\|_2+\left\|X^*\right\|\left\|\left(Y^{t,(m)}R^{t,(m)}-Y^{*}\right)_{m,\cdot}\right\|_2\\
&\leq  \left\|X^{t,(m)}R^{t,(m)}-X^{*}\right\|\left\|Y^{t,(m)}R^{t,(m)}\right\|_{2,\infty}+\left\|X^*\right\|\left\|\left(Y^{t,(m)}R^{t,(m)}-Y^{*}\right)_{m,\cdot}\right\|_2.
\end{align*}
Since Lemma \ref{lem:ncv3} holds for the $t$-th iteration, we have
\begin{align*}
  \left\|Y^{t,(m)}R^{t,(m)}\right\|_{2,\infty}\leq \left\|Y^{t,(m)}R^{t,(m)}-Y^*\right\|_{2,\infty}  + \|Y^*\|_{2,\infty}\leq 2\|Y^*\|_{2,\infty},
\end{align*}
as long as $\|Y^{t,(m)}R^{t,(m)}-Y^*\|_{2,\infty}\ll \|Y^*\|_{2,\infty}$. 
By Lemma \ref{ar:lem2}, we have
\begin{align*}
\left\|F^{t,(m)}R^{t,(m)}-F^{t}R^t\right\|_F\leq 5\kappa    \left\|F^{t,(m)}O^{t,(m)}-F^{t}R^t\right\|_F,
\end{align*}
which implies
\begin{align*}
   \left\|X^{t,(m)}R^{t,(m)}-X^{*}\right\|&\leq \left\|F^{t,(m)}R^{t,(m)}-F^{*}\right\|\\
  &\leq  \left\|F^{t,(m)}R^{t,(m)}-F^{t}R^t\right\|_F+ \left\|F^{t}R^t-F^{*}\right\|\\
   &\leq  5\kappa\left\|F^{t,(m)}O^{t,(m)}-F^{t}R^t\right\|_F+ \left\|F^{t}R^t-F^{*}\right\|\\
  &\leq 2\left\|F^{t}R^t-F^{*}\right\|
\end{align*}
as long as $\kappa\left\|F^{t,(m)}O^{t,(m)}-F^{t}R^t\right\|_F\ll \|F^{t}R^t-F^{*}\|$.
% Here the last inequality holds since $\left\|F^{t,(m)}O^{t,(m)}-F^{t}R^t\right\|_F=O(1)$ by Lemma \ref{lem:ncv2} and $\|F^{t}R^t-F^{*}\|=O(\sqrt{n})$ by Lemma \ref{lem:ncv1}.


Consequently, we have
\begin{align}\label{ineq2:lem_ncv3}
 &\left|\sum_{i\neq m}\frac{e^{c_i}}{(1+e^{c_i})^2}\left(\frac{1}{\sqrt{n}}\left(\theta^{t,(m)}_i-\theta^{*}_i\right)+\langle H^{t,(m)}-H^*,z_iz_m^T\rangle+\frac1n \left(X^{t,(m)}(Y^{t,(m)})^T-X^{*}Y^{*T}\right)_{im}\right)\right|\notag\\
&\leq \|\theta^{t,(m)}-\theta^{*}\|_2+\sz\| H^{t,(m)}-H^*\|\notag\\
&\quad+\frac{1}{\sqrt{n}}\left(4\left\|F^{t}R^t-F^{*}\right\|\|Y^*\|_{2,\infty}+\left\|X^*\right\|\left\|\left(Y^{t,(m)}R^{t,(m)}-Y^{*}\right)_{m,\cdot}\right\|_2\right)   
\end{align}

\end{enumerate}

Combine \eqref{eq1:lem_ncv3}, \eqref{ineq1:lem_ncv3}, and \eqref{ineq2:lem_ncv3}, we have
\begin{align*}
&\left|\theta^{t+1,(m)}_m-\theta^*_m\right|\notag\\
&\leq\left|1-\frac{2\eta}{n}\sum_{i\neq m}\frac{e^{c_i}}{(1+e^{c_i})^2}\right|\left|\theta^{t,(m)}_m-\theta^*_m\right|\\
&\quad+ c\frac{\eta\sqrt{\su}}{\sqrt{n}}\left(\|\theta^t-\theta^{t,(m)}\|_2+\|H^t-H^{t,(m)}\|_F+\frac{1}{n}\|X^*\|\|F^tR^t-F^{t,(m)}O^{t,(m)}\|_F\right)\notag\\
&\quad + c\frac{\eta\sqrt{\su}}{\sqrt{n}}\left(\|\theta^t-\theta^{*}\|_{2}+\|H^t-H^{*}\|_{F}+\frac{1}{n}\|X^*\|\|F^tR^t-F^*\|_F\right)+c\eta\sqrt{\frac{\log n}{n}}\\
&\quad+\frac{2\eta}{\sqrt{n}}\Bigg(\|\theta^{t,(m)}-\theta^{*}\|_2+\sz\| H^{t,(m)}-H^*\|\notag\\
&\qquad\qquad\quad+\frac{1}{\sqrt{n}}\left(4\left\|F^{t}R^t-F^{*}\right\|\|Y^*\|_{2,\infty}+\left\|X^*\right\|\left\|\left(Y^{t,(m)}R^{t,(m)}-Y^{*}\right)_{m,\cdot}\right\|_2\right)\Bigg)\\
&\leq\left|1-\frac{2\eta}{n}\sum_{i\neq m}\frac{e^{c_i}}{(1+e^{c_i})^2}\right|\left|\theta^{t,(m)}_m-\theta^*_m\right|\\
&\quad+ c\frac{\eta\sqrt{\overline{C}}}{\sqrt{n}}c_{21}+ c{\eta(\sqrt{\overline{C}}}+\sz)c_{11}+c\eta\sqrt{\frac{\log n}{n}}+c\eta\sqrt{\mu \sX\sY r^2 }c_{14}\\
&\quad+\frac{2\eta}{n}\sqrt{\sigma_{\max}}\left\|\left(Y^{t,(m)}R^{t,(m)}-Y^{*}\right)_{m,\cdot}\right\|_2.
\end{align*}
Notice that $|P^{t,(m)}_{im}|\leq 2|P^{*}_{im}|$. Thus, by Assumption \ref{assumption:scales}, we have $|c_i|\leq 2|P^{*}_{im}|\leq 2c_P$, which implies
\begin{align*}
 \sum_{i\neq m}\frac{e^{c_i}}{(1+e^{c_i})^2}\geq    (n-1)\frac{e^{2c_P}}{(1+e^{2c_P})^2}.
\end{align*}
Consequently, we obtain
\begin{align*}
&\left|\theta^{t+1,(m)}_m-\theta^*_m\right|\notag\\
&\leq\left(1-{\eta}\frac{e^{2c_P}}{(1+e^{2c_P})^2}\right)\left|\theta^{t,(m)}_m-\theta^*_m\right|\\
&\quad+ c\frac{\eta\sqrt{\overline{C}}}{\sqrt{n}}c_{21}+ c{\eta(\sqrt{\overline{C}}}+\sz)c_{11}+c\eta\sqrt{\frac{\log n}{n}}+c\eta\sqrt{\mu \sX\sY r^2 }c_{14}\\
&\quad+\frac{2\eta}{n}\sqrt{\sigma_{\max}}\left\|\left(Y^{t,(m)}R^{t,(m)}-Y^{*}\right)_{m,\cdot}\right\|_2\\
&\leq\left(1-{\eta}\frac{e^{2c_P}}{(1+e^{2c_P})^2}\right)c_{31}\\
&\quad+ c\frac{\eta\sqrt{\overline{C}}}{\sqrt{n}}c_{21}+ c{\eta(\sqrt{\overline{C}}}+\sz)c_{11}+c\eta\sqrt{\frac{\log n}{n}}+c\eta\sqrt{\mu \sX\sY r^2 }c_{14}+\frac{2\eta}{n}\sqrt{\sigma_{\max}}c_{32}.
\end{align*}
Thus, as long as
\begin{align}\label{condition1}
\max\left\{\sqrt{\frac{\overline{C}}{n}}c_{21}, 
(\sqrt{\overline{C}}+\sz)c_{11},
\sqrt{\frac{\log n}{n}},
\sqrt{\mu \sX\sY r^2 }c_{14},
\frac{\sqrt{\sigma_{\max}}}{n}c_{32}
\right\}\lesssim \frac{e^{2c_P}}{(1+e^{2c_P})^2} c_{31},
\end{align}
we have
\begin{align*}
\left|\theta^{t+1,(m)}_m-\theta^*_m\right|\leq c_{31},
\end{align*}
which then finishes the proof of the first part of Lemma \ref{lem:ncv3}.

Then, for any fixed $m$, we will show that $\left\|\left(F^{t+1,(m)}R^{t+1,(m)}-F^{*}\right)_{m,\cdot}\right\|_2\leq c_{32}$ in the following (the proof for $\left\|\left(F^{t+1,(m)}R^{t+1,(m)}-F^{*}\right)_{m+n,\cdot}\right\|_2$ is the same so we omit it here). Note that
\begin{align*}
\nabla_X L^{(m)}(\theta,H,X,Y)
&=\frac1n\sum_{\substack{
        i \neq j \\
        i, j \neq m
    }}\left(\frac{e^{P_{ij}}}{1+e^{P_{ij}}}-A_{ij}\right)e_ie_j^TY\\
&\quad+\frac1n\sum_{i\neq m}\left(\frac{e^{P_{im}}}{1+e^{P_{im}}}-\frac{e^{P_{im}^*}}{1+e^{P_{im}^*}}\right)e_ie_m^TY+\frac1n\sum_{i\neq m}\left(\frac{e^{P_{mi}}}{1+e^{P_{mi}}}-\frac{e^{P_{mi}^*}}{1+e^{P_{mi}^*}}\right)e_me_i^TY,
\end{align*}
where the $m$-th row of the first and second terms are all zeros. Thus, by the gradient descent update, we have
\begin{align*}
&\left(F^{t+1,(m)}R^{t+1,(m)}-F^{*}\right)_{m,\cdot}\\
&=\left(X^{t,(m)}_{m,\cdot}-\eta\left\{\frac1n\sum_{i\neq m}\left(\frac{e^{P_{mi}^{t,(m)}}}{1+e^{P_{mi}^{t,(m)}}}-\frac{e^{P_{mi}^*}}{1+e^{P_{mi}^*}}\right)e_i^TY^{t,(m)}+\lambda X^{t,(m)}_{m,\cdot}\right\}\right)R^{t+1,(m)}-X^*_{m,\cdot}\\
&=\underbrace{\left\{X^{t,(m)}_{m,\cdot}R^{t,(m)}-X^*_{m,\cdot}-\eta\left(\frac1n\sum_{i\neq m}\left(\frac{e^{P_{mi}^{t,(m)}}}{1+e^{P_{mi}^{t,(m)}}}-\frac{e^{P_{mi}^*}}{1+e^{P_{mi}^*}}\right)e_i^TY^{t,(m)}+\lambda X^{t,(m)}_{m,\cdot}\right)R^{t,(m)}\right\}}_{(1)}\\
&+\underbrace{\left\{X^{t,(m)}_{m,\cdot}R^{t,(m)}-\eta\left(\frac1n\sum_{i\neq m}\left(\frac{e^{P_{mi}^{t,(m)}}}{1+e^{P_{mi}^{t,(m)}}}-\frac{e^{P_{mi}^*}}{1+e^{P_{mi}^*}}\right)e_i^TY^{t,(m)}+\lambda X^{t,(m)}_{m,\cdot}\right)R^{t,(m)}\right\}\left(\left(R^{t,(m)}\right)^{-1}R^{t+1,(m)}-I_r\right)}_{(2)}
\end{align*}
In the following, we bound $\|(1)\|_2$ and $\|(2)\|_2$, respectively.
\begin{enumerate}
\item We first bound (1). By the mean value theorem, we have for some $\{c_i\}$ that
\begin{align*}
& \sum_{i\neq m}\left(\frac{e^{P^{t,(m)}_{mi}}}{1+e^{P^{t,(m)}_{mi}}}-\frac{e^{P^{*}_{mi}}}{1+e^{P^{*}_{mi}}}\right)e_i^TY^{t,(m)}\\
&= \sum_{i\neq m}\frac{e^{c_i}}{(1+e^{c_i})^2}\left(P^{t,(m)}_{mi}-P^{*}_{mi}\right)e_i^TY^{t,(m)}\\
& = \sum_{i\neq m}\frac{e^{c_i}}{(1+e^{c_i})^2}\left(\frac{1}{\sqrt{n}}\left(\theta^{t,(m)}_i-\theta^{*}_i+\theta^{t,(m)}_m-\theta^{*}_m\right)+\langle H^{t,(m)}-H^*,z_mz_i^T\rangle\right)e_i^TY^{t,(m)}\\
& \quad +\frac1n\sum_{i\neq m}\frac{e^{c_i}}{(1+e^{c_i})^2}\left(X^{t,(m)}(Y^{t,(m)})^T-X^{*}Y^{*T}\right)_{mi}e_i^TY^{t,(m)}.
\end{align*}
Note that
\begin{align*}
&X^{t,(m)}(Y^{t,(m)})^T-X^{*}Y^{*T}\\
&=\left(X^{t,(m)}R^{t,(m)}-X^*\right)\left(Y^{t,(m)}R^{t,(m)}\right)^T+X^*\left(Y^{t,(m)}R^{t,(m)}-Y^*\right)^T.
\end{align*}
Thus, we further have
\begin{align*}
& \sum_{i\neq m}\left(\frac{e^{P^{t,(m)}_{mi}}}{1+e^{P^{t,(m)}_{mi}}}-\frac{e^{P^{*}_{mi}}}{1+e^{P^{*}_{mi}}}\right)e_i^TY^{t,(m)}\\
&= \sum_{i\neq m}\frac{e^{c_i}}{(1+e^{c_i})^2}\left(\frac{1}{\sqrt{n}}\left(\theta^{t,(m)}_i-\theta^{*}_i+\theta^{t,(m)}_m-\theta^{*}_m\right)+\langle H^{t,(m)}-H^*,z_mz_i^T\rangle\right)e_i^TY^{t,(m)}\\
& \quad +\frac1n\sum_{i\neq m}\frac{e^{c_i}}{(1+e^{c_i})^2}\left(X^*\left(Y^{t,(m)}R^{t,(m)}-Y^*\right)^T\right)_{mi}e_i^TY^{t,(m)}\\
& \quad +\frac1n\sum_{i\neq m}\frac{e^{c_i}}{(1+e^{c_i})^2}\left(\left(X^{t,(m)}R^{t,(m)}-X^*\right)\left(Y^{t,(m)}R^{t,(m)}\right)^T\right)_{mi}e_i^TY^{t,(m)}.
\end{align*}
Moreover, we have
\begin{align*}
  & \frac1n\sum_{i\neq m}\frac{e^{c_i}}{(1+e^{c_i})^2}\left(X^{t,(m)}R^{t,(m)}-X^*\right)_{m,\cdot}\left(Y^{t,(m)}R^{t,(m)}\right)^T_{i,\cdot}e_i^TY^{t,(m)}\\ 
  &=\frac1n\left(X^{t,(m)}R^{t,(m)}-X^*\right)_{m,\cdot}\left(\sum_{i\neq m}\frac{e^{c_i}}{(1+e^{c_i})^2}\left(Y^{t,(m)}R^{t,(m)}\right)^T_{i,\cdot}e_i^T\right)Y^{t,(m)}\\
  &=\frac1n\left(X^{t,(m)}R^{t,(m)}-X^*\right)_{m,\cdot}\left(Y^{t,(m)}R^{t,(m)}\right)^T AY^{t,(m)}\\
  &\quad-\frac1n \left(\left(X^{t,(m)}R^{t,(m)}-X^*\right)\left(Y^{t,(m)}R^{t,(m)}\right)^T\right)_{mm}e_m^TY^{t,(m)},
\end{align*}
where $A$ is a diagonal matrix with
\begin{align*}
A_{ii}=
\begin{cases} 
      \frac{e^{c_i}}{(1+e^{c_i})^2} & i\neq m\\
      1 & i=m
   \end{cases}.
\end{align*}
Thus, we obtain
\begin{align*}
& \sum_{i\neq m}\left(\frac{e^{P^{t,(m)}_{mi}}}{1+e^{P^{t,(m)}_{mi}}}-\frac{e^{P^{*}_{mi}}}{1+e^{P^{*}_{mi}}}\right)e_i^TY^{t,(m)}\\
&= \sum_{i\neq m}\frac{e^{c_i}}{(1+e^{c_i})^2}\left(\frac{1}{\sqrt{n}}\left(\theta^{t,(m)}_i-\theta^{*}_i+\theta^{t,(m)}_m-\theta^{*}_m\right)+\langle H^{t,(m)}-H^*,z_mz_i^T\rangle\right)e_i^TY^{t,(m)}\\
& \quad +\frac1n\sum_{i\neq m}\frac{e^{c_i}}{(1+e^{c_i})^2}\left(X^*\left(Y^{t,(m)}R^{t,(m)}-Y^*\right)^T\right)_{mi}e_i^TY^{t,(m)}\\
&\quad +\frac1n\left(X^{t,(m)}R^{t,(m)}-X^*\right)_{m,\cdot}\left(Y^{t,(m)}R^{t,(m)}\right)^T AY^{t,(m)}\\
  &\quad-\frac1n \left(\left(X^{t,(m)}R^{t,(m)}-X^*\right)\left(Y^{t,(m)}R^{t,(m)}\right)^T\right)_{mm}e_m^TY^{t,(m)}.
\end{align*}
Consequently, we have
\begin{align*}
(1)
&=\underbrace{\left(X^{t,(m)}R^{t,(m)}-X^*\right)_{m,\cdot}\left(I_r-\frac{\eta}{n^2}\left(Y^{t,(m)}R^{t,(m)}\right)^T AY^{t,(m)}R^{t,(m)}\right)}_{(a)}\\
&\quad -\frac{\eta}{n}\underbrace{\sum_{i\neq m}\frac{e^{c_i}}{(1+e^{c_i})^2}\left(\frac{1}{\sqrt{n}}\left(\theta^{t,(m)}_i-\theta^{*}_i+\theta^{t,(m)}_m-\theta^{*}_m\right)+\langle H^{t,(m)}-H^*,z_mz_i^T\rangle\right)e_i^TY^{t,(m)}R^{t,(m)}}_{(b)}\\
&\quad-\frac{\eta}{n^2}\underbrace{\sum_{i\neq m}\frac{e^{c_i}}{(1+e^{c_i})^2}\left(X^*\left(Y^{t,(m)}R^{t,(m)}-Y^*\right)^T\right)_{mi}e_i^TY^{t,(m)}R^{t,(m)}}_{(c)}\\
&\quad +\frac{\eta}{n^2}\underbrace{\left(\left(X^{t,(m)}R^{t,(m)}-X^*\right)\left(Y^{t,(m)}R^{t,(m)}\right)^T\right)_{mm}e_m^TY^{t,(m)}R^{t,(m)}}_{(d)}\\
&\quad-\eta\lambda \underbrace{X^{t,(m)}_{m,\cdot}R^{t,(m)}}_{(e)}.
\end{align*}
Thus, to upper bound $\|(1)\|_2$, we only need to bound $\|(a)\|_2$--$\|(e)\|_2$, respectively.
\begin{enumerate}
\item Bound (a).
By Lemma \ref{ar:lem4} and the definition of $A$, we have
\begin{align*}
\sigma_{\min}\left(\left(Y^{t,(m)}R^{t,(m)}\right)^T AY^{t,(m)}R^{t,(m)}\right)\geq \frac{\sigma_{\min}}{2}\min_{i\neq m}\frac{e^{c_i}}{(1+e^{c_i})^2}\geq \frac{e^{2c_P}}{2(1+e^{2c_P})^2}\sigma_{\min}.
\end{align*}
Thus, it holds that
\begin{align*}
I_r-\frac{\eta}{n^2}\left(Y^{t,(m)}R^{t,(m)}\right)^T AY^{t,(m)}R^{t,(m)}\preceq \left(1-\frac{e^{2c_P}}{2(1+e^{2c_P})^2}\cdot\frac{\eta\sigma_{\min}}{n^2}\right)I_r,
\end{align*}
which implies
\begin{align*}
\|(a)\|_2\leq \left(1-\frac{e^{2c_P}}{2(1+e^{2c_P})^2}\cdot\frac{\eta\sigma_{\min}}{n^2}\right)\left\|\left(X^{t,(m)}R^{t,(m)}-X^*\right)_{m,\cdot}\right\|_2.
\end{align*}

\item Bound (b).
Note that
\begin{align*}
&\left\|\sum_{i\neq m}\frac{e^{c_i}}{(1+e^{c_i})^2}\left(\frac{1}{\sqrt{n}}\left(\theta^{t,(m)}_i-\theta^{*}_i+\theta^{t,(m)}_m-\theta^{*}_m\right)+\langle H^{t,(m)}-H^*,z_mz_i^T\rangle\right)e_i\right\|_2\\
&\leq \left\|\frac{1}{\sqrt{n}}\left(\theta^{t,(m)}_m-\theta^{*}_m\right)\sum_{i\neq m}\frac{e^{c_i}}{(1+e^{c_i})^2}e_i\right\|_2+\left\|\frac{1}{\sqrt{n}}\sum_{i\neq m}\frac{e^{c_i}}{(1+e^{c_i})^2}\left(\theta^{t,(m)}_i-\theta^{*}_i\right)e_i\right\|_2\\
&\quad+ \left\|\sum_{i\neq m}\frac{e^{c_i}}{(1+e^{c_i})^2}\langle H^{t,(m)}-H^*,z_mz_i^T\rangle e_i\right\|_2\\
&\leq \frac14\left|\theta^{t,(m)}_m-\theta^{*}_m\right|+\frac{1}{4\sqrt{n}}\left\|\theta^{t,(m)}-\theta^{*}\right\|_2+\frac{1}{4}\sqrt{\sum_{i\neq m}\left|\langle H^{t,(m)}-H^*,z_mz_i^T\rangle\right|^2}\\
&\leq \frac14\left|\theta^{t,(m)}_m-\theta^{*}_m\right|+\frac{1}{4\sqrt{n}}\left\|\theta^{t,(m)}-\theta^{*}\right\|_2+\frac{1}{4}\| H^{t,(m)}-H^*\|\|z_m\|_2\sqrt{\sum_{i\neq m}\|z_i\|_2^2}\\
&\leq \frac14\left(\left|\theta^{t,(m)}_m-\theta^{*}_m\right|+\frac{1}{\sqrt{n}}\left\|\theta^{t,(m)}-\theta^{*}\right\|_2+\frac{\sz}{\sqrt{n}}\| H^{t,(m)}-H^*\|\right).
\end{align*}
Moreover, we have
\begin{align*}
    \|Y^{t,(m)}\|\leq  \|F^{t,(m)}O^{t,(m)}-F^tR^t\|+\|F^tR^t-F^*\|+\|F^*\|\leq 2\|F^*\|.
\end{align*}
Thus, we have
\begin{align*}
\|(b)\|_2\leq \|F^*\|\left(\left|\theta^{t,(m)}_m-\theta^{*}_m\right|+\frac{1}{\sqrt{n}}\left\|\theta^{t,(m)}-\theta^{*}\right\|_2+\frac{\sz}{\sqrt{n}}\| H^{t,(m)}-H^*\|\right).
\end{align*}






\item Bound (c).
Note that
\begin{align*}
&\left\|\sum_{i\neq m}\frac{e^{c_i}}{(1+e^{c_i})^2}\left(X^*\left(Y^{t,(m)}R^{t,(m)}-Y^*\right)^T\right)_{mi}e_i\right\|_2\\
&\leq \frac14 \left\|\left(X^*\left(Y^{t,(m)}R^{t,(m)}-Y^*\right)^T\right)_{m,\cdot}\right\|_2\\
&= \frac14 \left\|X^*_{m,\cdot}\left(Y^{t,(m)}R^{t,(m)}-Y^*\right)^T\right\|_2\\
&\leq \frac14  \left\|X^*_{m,\cdot}\right\|_2\left\|Y^{t,(m)}R^{t,(m)}-Y^*\right\|\\
&\leq \frac14  \left\|F^*\right\|_{2,\infty}\left\|Y^{t,(m)}R^{t,(m)}-Y^*\right\|.
\end{align*}
Thus, we have
\begin{align*}
\|(c)\|_2\lesssim \|F^*\|\left\|F^*\right\|_{2,\infty}\left\|Y^{t,(m)}R^{t,(m)}-Y^*\right\|.
\end{align*}







\item Bound (d).
Note that
\begin{align*}
&\left|\left(\left(X^{t,(m)}R^{t,(m)}-X^*\right)\left(Y^{t,(m)}R^{t,(m)}\right)^T\right)_{mm}\right|\\
&\leq \left\|\left(X^{t,(m)}R^{t,(m)}-X^*\right)\left(Y^{t,(m)}R^{t,(m)}\right)^T_{\cdot,m}\right\|_2\\
&\leq \left\|X^{t,(m)}R^{t,(m)}-X^*\right\|\left\|\left(Y^{t,(m)}R^{t,(m)}\right)_{m,\cdot}\right\|_2\\
&\leq \left\|X^{t,(m)}R^{t,(m)}-X^*\right\|\left\|Y^{t,(m)}R^{t,(m)}\right\|_{2,\infty}\\
&\lesssim\left\|X^{t,(m)}R^{t,(m)}-X^*\right\|\left\|F^*\right\|_{2,\infty},
\end{align*}
where the last inequality follows from 
\begin{align*}
&\left\|Y^{t,(m)}R^{t,(m)}\right\|_{2,\infty}\\
&\leq  \left\|F^{t,(m)}R^{t,(m)}-F^*\right\|_{2,\infty}+\|F^*\|_{2,\infty}\leq2\|F^*\|_{2,\infty}\tag{by Lemma \ref{lem:ncv3}}.
\end{align*}
Thus, we have
\begin{align*}
\|(d)\|_2\lesssim \|F^*\|\left\|X^{t,(m)}R^{t,(m)}-X^*\right\|\left\|F^*\right\|_{2,\infty}.
\end{align*}






\item Bound (e).
We have
\begin{align*}
\|(e)\|_2\leq \left\|X^{t,(m)}R^{t,(m)}\right\|_{2,\infty}\leq \left\|F^{t,(m)}R^{t,(m)}-F^*\right\|_{2,\infty}+\|F^*\|_{2,\infty}\leq2\|F^*\|_{2,\infty}.
\end{align*}



\end{enumerate}

Combine the above results, we have
\begin{align}\label{ineq40}
\|(1)\|_2&\leq \left(1-\frac{e^{2c_P}}{2(1+e^{2c_P})^2}\cdot\frac{\eta\sigma_{\min}}{n^2}\right)\left\|\left(X^{t,(m)}R^{t,(m)}-X^*\right)_{m,\cdot}\right\|_2\notag\\
&\quad+\frac{\eta}{n}\|F^*\|\left(\left|\theta^{t,(m)}_m-\theta^{*}_m\right|+\frac{1}{\sqrt{n}}\left\|\theta^{t,(m)}-\theta^{*}\right\|_2+\frac{\sz}{\sqrt{n}}\| H^{t,(m)}-H^*\|\right)\notag\\
&\quad+c\frac{\eta}{n^2}\|F^*\|\left\|F^*\right\|_{2,\infty}\left\|Y^{t,(m)}R^{t,(m)}-Y^*\right\|\notag\\
&\quad+c\frac{\eta}{n^2}\|F^*\|\left\|F^*\right\|_{2,\infty}\left\|X^{t,(m)}R^{t,(m)}-X^*\right\|+c\eta\lambda\left\|F^*\right\|_{2,\infty}\notag\\
&\leq \left(1-\frac{e^{2c_P}}{2(1+e^{2c_P})^2}\cdot\frac{\eta\sigma_{\min}}{n^2}\right)\left\|\left(X^{t,(m)}R^{t,(m)}-X^*\right)_{m,\cdot}\right\|_2\notag\\
&\quad+\frac{2\eta}{n}\sqrt{\sigma_{\max}}\left|\theta^{t,(m)}_m-\theta^{*}_m\right|+c \frac{\eta\sz}{n}c_{11}+c\frac{\eta}{n}\sqrt{\mu \sX\sY r^2 \sigma_{\max}}c_{14}+c\eta c_{\lambda} \sqrt{\mu \sX\sY r^2 \log n}.
\end{align}





\item We then bound (2).
Note that
\begin{align*}
(2)=\left((1)+X^*_{m,\cdot}\right)\left(\left(R^{t,(m)}\right)^{-1}R^{t+1,(m)}-I_r\right)
\end{align*}
By \eqref{ineq40}, it can be seen that $\|(1)\|_2\leq \|F^*\|_{2,\infty}$, thus we have
\begin{align*}
\|(1)+X^*_{m,\cdot}\|_2\leq \|(1)\|_2+\|X^*_{m,\cdot}\|_2\leq\|(1)\|_2+\|F^*\|_{2,\infty}\leq 2\|F^*\|_{2,\infty}.
\end{align*}
Regarding the term $\left(R^{t,(m)}\right)^{-1}R^{t+1,(m)}-I_r$, we have the following claim.
\begin{claim}\label{claim:rotation}
With probability at least $1-n^{-10}$, we have
\begin{align*}
\left\|\left(R^{t,(m)}\right)^{-1}R^{t+1,(m)}-I_r\right\|\lesssim \frac{\eta}{n}\left\| F^{t, (m)}R^{t, (m)}-F^*\right\|.
\end{align*}
\end{claim}
Consequently, we have
\begin{align*}
\|(2)\|_2&\leq \|(1)+X^*_{m,\cdot}\|_2\left\|\left(R^{t,(m)}\right)^{-1}R^{t+1,(m)}-I_r\right\|\\
&\lesssim\frac{\eta}{n}\left\| F^{t, (m)}R^{t, (m)}-F^*\right\|\|F^*\|_{2,\infty}\\
&\lesssim \eta\sqrt{\mu\sX\sY r^2} c_{14}.
\end{align*}



\end{enumerate}



To summarize, we have shown
\begin{align*}
&\left\|\left(F^{t+1,(m)}R^{t+1,(m)}-F^{*}\right)_{m,\cdot}\right\|_2\\
&\leq \left(1-\frac{e^{2c_P}}{2(1+e^{2c_P})^2}\cdot\frac{\eta\sigma_{\min}}{n^2}\right)\left\|\left(X^{t,(m)}R^{t,(m)}-X^*\right)_{m,\cdot}\right\|_2\notag\\
&\quad+\frac{2\eta}{n}\sqrt{\sigma_{\max}}\left|\theta^{t,(m)}_m-\theta^{*}_m\right|+c \frac{\eta\sz}{n}c_{11}+c\frac{\eta}{n}\sqrt{\mu \sX\sY r^2 \sigma_{\max}}c_{14}+c\eta c_{\lambda} \sqrt{\mu \sX\sY r^2 \log n}\\
&\quad+c\eta\sqrt{\mu\sX\sY r^2} c_{14}\\
&\leq \left(1-\frac{e^{2c_P}}{2(1+e^{2c_P})^2}\cdot\frac{\eta\sigma_{\min}}{n^2}\right)c_{32}\notag\\
&\quad+\frac{2\eta}{n}\sqrt{\sigma_{\max}}c_{31}+c \frac{\eta\sz}{n}c_{11}+c\frac{\eta}{n}\sqrt{\mu \sX\sY r^2 \sigma_{\max}}c_{14}+c\eta c_{\lambda} \sqrt{\mu \sX\sY r^2 \log n}\\
&\quad+c\eta\sqrt{\mu\sX\sY r^2} c_{14}.
\end{align*}
Thus, as long as
\begin{align}\label{condition2}
\max\left\{
\frac{\sqrt{\sigma_{\max}}}{n}c_{31},
\frac{\sz}{n}c_{11},
\left(\frac{\sqrt{\sigma_{\max}}}{n}+1\right)\sqrt{\mu \sX\sY r^2}c_{14},
c_{\lambda} \sqrt{\mu \sX\sY r^2 \log n}
\right\}\lesssim \frac{e^{2c_P}}{(1+e^{2c_P})^2}\cdot\frac{\sigma_{\min}}{n^2}c_{32},
\end{align}
we have
\begin{align*}
 \left\|\left(F^{t+1,(m)}R^{t+1,(m)}-F^{*}\right)_{m,\cdot}\right\|_2\leq c_{32}.   
\end{align*}
By the arbitrariness of $m$, we finish the proofs.









It remains to prove Claim \ref{claim:rotation}.
\begin{proof}[Proof of Claim \ref{claim:rotation}]
To facilitate analysis, we introduce an auxiliary point $\tilde{F}^{t+1,(m)}:=\begin{bmatrix}
\tilde{X}^{t+1,(m)}\\
\tilde{Y}^{t+1,(m)}
\end{bmatrix}$ where
\begin{align*}
&\tilde{X}^{t+1,(m)}\\
&={X}^{t,(m)}{R}^{t,(m)}-\eta\left[\frac1n\sum_{\substack{
        i \neq j \\
        i, j \neq m
    }}\left(\frac{e^{P_{ij}^{t,(m)}}}{1+e^{P_{ij}^{t,(m)}}}-A_{ij}\right)e_ie_j^T+\frac1n\sum_{i\neq m}\left(\frac{e^{P_{im}^{t,(m)}}}{1+e^{P_{im}^{t,(m)}}}-\frac{e^{P_{im}^{*}}}{1+e^{P_{im}^{*}}}\right)(e_ie_m^T+e_me_i^T)\right]Y^*\\
&\quad-\eta\lambda X^*-\frac{4c_{\aug}\eta}{n^2}X^*({R}^{t,(m)})^T\left(({X}^{t,(m)})^T{X}^{t,(m)}-({Y}^{t,(m)})^T{Y}^{t,(m)}\right){R}^{t,(m)},\\
&\tilde{Y}^{t+1,(m)}\\
&={Y}^{t,(m)}{R}^{t,(m)}-\eta\left[\frac1n\sum_{\substack{
        i \neq j \\
        i, j \neq m
    }}\left(\frac{e^{P_{ij}^{t,(m)}}}{1+e^{P_{ij}^{t,(m)}}}-A_{ij}\right)e_je_i^T+\frac1n\sum_{i\neq m}\left(\frac{e^{P_{im}^{t,(m)}}}{1+e^{P_{im}^{t,(m)}}}-\frac{e^{P_{im}^{*}}}{1+e^{P_{im}^{*}}}\right)(e_ie_m^T+e_me_i^T)\right]X^*\\
&\quad-\eta\lambda Y^*-\frac{4c_{\aug}\eta}{n^2}Y^*({R}^{t,(m)})^T\left(({Y}^{t,(m)})^T{Y}^{t,(m)}-({X}^{t,(m)})^T{X}^{t,(m)}\right){R}^{t,(m)}.
\end{align*}
We have the following claim.
\begin{claim}\label{claim2:rotation}
It holds that
\begin{align*}
I_r=\argmin_{R\in\cO^{r\times r}}\left\|\tilde{F}^{t+1,(m)}R-F^*\right\|_F,\text{ and } \sigma_{\min}\left(\tilde{F}^{t+1,(m)T}F^{*}\right)\geq \sigma_{\min}/2.
\end{align*}
\begin{proof}[Proof of Claim \ref{claim2:rotation}]
See Claim 4 in \cite{chen2020noisy}.
\end{proof}
\end{claim}
With this claim at hand, by Lemma \ref{ar:lem5} with $S=\tilde{F}^{t+1,(m)T}F^{*}$ and $K=\left({F}^{t+1,(m)}R^{t,(m)}-\tilde{F}^{t+1,(m)}\right)^TF^*$, we have
\begin{align}\label{ineq1:claim2_rotation}
&\left\|\left(R^{t,(m)}\right)^{-1}R^{t+1,(m)}-I_r\right\|\\
&=\left\|\text{sgn}(S+K)-\text{sgn}(S)\right\|\tag{by Claim \ref{claim2:rotation} and the definition of $R^{t+1,(m)}$}\\
&\leq \frac{1}{\sigma_{\min}\left(\tilde{F}^{t+1,(m)T}F^{*}\right)}\left\|\left({F}^{t+1,(m)}R^{t,(m)}-\tilde{F}^{t+1,(m)}\right)^TF^*\right\|\tag{by Lemma \ref{ar:lem5}}\\
&\leq \frac{2}{\sigma_{\min}}\left\|{F}^{t+1,(m)}R^{t,(m)}-\tilde{F}^{t+1,(m)}\right\|\|F^*\|\tag{by Claim \ref{claim2:rotation}}.
\end{align}
Here  \(\text{sgn}(A) = UV^\top\) for a matrix \( A \) with SVD \( U \Sigma V^\top \). Note that
\begin{align*}
    &F^{t+1, (m)} R^{t, (m)} - \tilde{F}^{t+1, (m)} \\
    &= -\eta \begin{bmatrix} B & 0 \\ 0 & B^\top \end{bmatrix} \begin{bmatrix} Y^{t, (m)}R^{t, (m)}-Y^*  \\ X^{t, (m)}R^{t, (m)}-X^* \end{bmatrix} + \frac{4c_{\aug}\eta}{n^2} \begin{bmatrix} X^\star \\ -Y^\star \end{bmatrix} R^{t, (m) \top} C R^{t, (m)} - \eta \lambda\begin{bmatrix}   X^{t, (m)}R^{t, (m)}-X^*\\ Y^{t, (m)}R^{t, (m)}-Y^* \end{bmatrix} ,
\end{align*}
where we denote
\begin{align*}
 &B := \frac1n\sum_{\substack{
        i \neq j \\
        i, j \neq m
    }}\left(\frac{e^{P_{ij}^{t,(m)}}}{1+e^{P_{ij}^{t,(m)}}}-A_{ij}\right)e_ie_j^T+\frac1n\sum_{i\neq m}\left(\frac{e^{P_{im}^{t,(m)}}}{1+e^{P_{im}^{t,(m)}}}-\frac{e^{P_{im}^{*}}}{1+e^{P_{im}^{*}}}\right)(e_ie_m^T+e_me_i^T),\\ 
 &C := X^{t, (m) \top} X^{t, (m)} - Y^{t, (m) \top} Y^{t, (m)}.
\end{align*}
This enables us to obtain
\begin{align*}
 &\left\|F^{t+1, (m)} R^{t, (m)} - \tilde{F}^{t+1, (m)}\right\| \\
& \leq \eta \left\| B \right\| \left\| F^{t, (m)}R^{t, (m)}-F^*\right\| + \frac{4c_{\aug}\eta}{n^2} \left\| F^\star \right\| \left\| C \right\|_F +\eta \lambda\left\| F^{t, (m)}R^{t, (m)}-F^*\right\|.   
\end{align*}
We then bound $\|B\|$ in the following.
Note that
\begin{align*}
B&=\frac1n\sum_{i\neq j}\left(\frac{e^{P_{ij}^{t,(m)}}}{1+e^{P_{ij}^{t,(m)}}}-\frac{e^{P_{ij}^{*}}}{1+e^{P_{ij}^{*}}}\right)e_ie_j^T +   \frac1n\sum_{\substack{
        i \neq j \\
        i, j \neq m
    }}\left(\frac{e^{P_{ij}^{*}}}{1+e^{P_{ij}^{*}}}-A_{ij}\right)e_ie_j^T.
\end{align*}
For the first term, we have
\begin{align*}
&\left\|\sum_{i\neq j}\left(\frac{e^{P_{ij}^{t,(m)}}}{1+e^{P_{ij}^{t,(m)}}}-\frac{e^{P_{ij}^{*}}}{1+e^{P_{ij}^{*}}}\right)e_ie_j^T\right\|\\
&\leq \left\|\sum_{i\neq j}\left(\frac{e^{P_{ij}^{t,(m)}}}{1+e^{P_{ij}^{t,(m)}}}-\frac{e^{P_{ij}^{*}}}{1+e^{P_{ij}^{*}}}\right)e_ie_j^T\right\|_F\\
&=\sqrt{\sum_{i\neq j}\left(\frac{e^{P_{ij}^{t,(m)}}}{1+e^{P_{ij}^{t,(m)}}}-\frac{e^{P_{ij}^{*}}}{1+e^{P_{ij}^{*}}}\right)^2}\\
&=\frac14\sqrt{\sum_{i\neq j}\left(P_{ij}^{t,(m)}-P_{ij}^{*}\right)^2}\tag{by mean value theorem}\\
&\lesssim \sqrt{\su}\left(\|\theta^{t,(m)}-\theta^{*}\|_{2}+\|H^{t,(m)}-H^{*}\|_{F}+\frac{1}{n}\|F^*\|\|F^{t,(m)}R^{t,(m)}-F^{*}\|_{F}\right).
\end{align*}
For the second term, same as bounding $\|\nabla_{\Gamma}L_c(\theta^*,H^*,\Gamma^*)\|$ in the proof of Lemma \ref{lem:gradient_norm}, we have
\begin{align*}
\left\| \frac1n\sum_{\substack{
        i \neq j \\
        i, j \neq m
    }}\left(\frac{e^{P_{ij}^{*}}}{1+e^{P_{ij}^{*}}}-A_{ij}\right)e_ie_j^T\right\|\lesssim\sqrt{\frac{\log n}{n}}.
\end{align*}
Consequently, we have
\begin{align*}
\|B\|&\lesssim \frac{\sqrt{\su}}{n}\left(\|\theta^{t,(m)}-\theta^{*}\|_{2}+\|H^{t,(m)}-H^{*}\|_{F}+\frac{1}{n}\|F^*\|\|F^{t,(m)}R^{t,(m)}-F^{*}\|_{F}\right)+\sqrt{\frac{\log n}{n}}\\
&\lesssim \sqrt{\frac{\overline{C}}{n}}c_{11}+\sqrt{\frac{\log n}{n}}.
\end{align*}
Thus, we have
\begin{align*}
 &\left\|F^{t+1, (m)} R^{t, (m)} - \tilde{F}^{t+1, (m)}\right\| \\
& \leq c\eta\sqrt{\frac{\overline{C}c^2_{11}+\log n}{n}}\left\| F^{t, (m)}R^{t, (m)}-F^*\right\| + \frac{4c_{\aug}\eta}{n^2} \left\| F^\star \right\| \left\|  X^{t, (m) \top} X^{t, (m)} - Y^{t, (m) \top} Y^{t, (m)} \right\|_F \\
&\quad +\eta \lambda\left\| F^{t, (m)}R^{t, (m)}-F^*\right\|.   
\end{align*}
By \eqref{ineq1:claim2_rotation}, we obtain
\begin{align*}
 &\left\|\left(R^{t,(m)}\right)^{-1}R^{t+1,(m)}-I_r\right\|\\
 &\leq \frac{2\|F^*\|}{\sigma_{\min}}  \Bigg(c\eta\sqrt{\frac{\overline{C}c^2_{11}+\log n}{n}}\left\| F^{t, (m)}R^{t, (m)}-F^*\right\| + \frac{4c_{\aug}\eta}{n^2} \left\| F^\star \right\| \left\|  X^{t, (m) \top} X^{t, (m)} - Y^{t, (m) \top} Y^{t, (m)} \right\|_F \\
 &\qquad\qquad\qquad+\eta \lambda\left\| F^{t, (m)}R^{t, (m)}-F^*\right\|\Bigg)\\
  &\lesssim \frac{\|F^*\|}{\sigma_{\min}} \eta \Bigg(\sqrt{\frac{\overline{C}c^2_{11}+\log n}{n}}\left\| F^{t, (m)}R^{t, (m)}-F^*\right\| + c_{\aug}c_{51}\eta\sqrt{\sigma_{\max}} +\lambda\left\| F^{t, (m)}R^{t, (m)}-F^*\right\|\Bigg)\\
&\lesssim \frac{\eta\sqrt{\sigma_{\max}}}{\sigma_{\min}}\left(\sqrt{\frac{\overline{C}c^2_{11}+\log n}{n}}+\lambda\right) \left\| F^{t, (m)}R^{t, (m)}-F^*\right\| \tag{as long as $\eta$ small enough}\\
&\lesssim \frac{\eta}{n}\left\| F^{t, (m)}R^{t, (m)}-F^*\right\|
\end{align*}
as long as $\frac{n\sqrt{\sigma_{\max}}}{\sigma_{\min}}\left(\sqrt{\frac{\overline{C}c^2_{11}+\log n}{n}}+\lambda\right)\lesssim 1$.
We then prove Claim \ref{claim:rotation}.

\end{proof}




\textcolor{red}{
Question: \eqref{condition1} and \eqref{condition2} cannot hold simultaneously (see $c_{31}$ and $c_{32}$) !!!
}


==> proof_convexity.tex <==
\section{Proofs of Lemma \ref{lem:convexity}}\label{proof_convexity}

\paragraph{Observations}
Based on the constraints on $(\theta,H,X,Y)$, it can be seen that: 
\begin{align*}
 &\|\theta-\theta^{*}\|_{2}\leq c_1 \sqrt{n}, \\
 &\|XR-X^*\|\leq \|XR-X^*\|_{F}\leq \sqrt{n}\|XR-X^*\|_{2,\infty}\leq c_3 \sqrt{n}\\
 &\|YR-Y^*\|\leq \|YR-Y^*\|_{F}\leq \sqrt{n}\|YR-Y^*\|_{2,\infty}\leq c_3 \sqrt{n}.
\end{align*}
This further implies that
\begin{align*}
&\|XY^T-X^*Y^{*T}\|_{F}\\
&=\|(XR-X^*)(YR)^T+X^{*}(YR-Y^*)^T\|_F\\
&\leq \|XR-X^*\|_F\|YR\|+\|X^{*}\|\|YR-Y^*\|_F\\
&\leq \|XR-X^*\|_F\|YR-Y^*\|+\|XR-X^*\|_F\|Y^*\|+\|X^{*}\|\|YR-Y^*\|_F\\
&\leq 3 c_3\sqrt{\sigma_{\max}n},
\end{align*}
where we use the fact that $\|X^*\|=\|Y^*\|=\sqrt{\sigma_{\max}}\geq c_3\sqrt{n}$. Moreover, we have
\begin{align*}
&\|XY^T-X^*Y^{*T}\|_{\infty}\\
&=\|(XR-X^*)(YR)^T+X^{*}(YR-Y^*)^T\|_{\infty}\\
&\leq \|XR-X^*\|_{2,\infty}\|YR\|_{2,\infty}+\|X^{*}\|_{2,\infty}\|YR-Y^*\|_{2,\infty} \tag{Cauchy}\\
&\leq \|XR-X^*\|_{2,\infty}\|YR-Y^*\|_{2,\infty}+ \|XR-X^*\|_{2,\infty}\|Y^*\|_{2,\infty}+\|X^{*}\|_{2,\infty}\|YR-Y^*\|_{2,\infty} \\
&\leq 3c_3 \sqrt{\frac{\mu r \sigma_{\max}}{n}},
\end{align*}
where we use the fact that $c_3, \|X^*\|_{2,\infty}, \|Y^*\|_{2,\infty}\leq \sqrt{\frac{\mu r \sigma_{\max}}{n}}$. Thus, we obtain
\begin{align*}
|P_{ij}|&\leq |P^*_{ij}|+|P_{ij}-P^*_{ij}|\\
&\leq |P^*_{ij}|+\frac{2}{\sqrt{n}}\|\theta-\theta^*\|_{\infty}+\|H-H^*\|\|z_i\|\|z_j\|+\frac1n \|XY^T-X^*Y^{*T}\|_{\infty}\\
&\leq |P^*_{ij}|+\frac{2}{\sqrt{n}}\|\theta-\theta^*\|_{\infty}+\frac{\sz}{n}\|H-H^*\|+\frac1n \|XY^T-X^*Y^{*T}\|_{\infty}\\
&\leq |P^*_{ij}|+\frac{1}{\sqrt{n}}\left(2c_1+\sz c_2+\frac{3c_3 \sqrt{\mu r \sigma_{\max}}}{n}\right).
\end{align*}
Based on Assumption \ref{assumption:scales}, we know $|P^*_{ij}|\leq 2\stheta+\sz\sH+\sX\sY r=c_P$ and this leads to the fact that $|P_{ij}|\leq 2c_P$ as long as
\begin{align*}
\frac{1}{\sqrt{n}}\left(2c_1+\sz c_2+3c_3 r \sqrt{\sX\sY\mu  }\right)\leq 2\stheta+\sz\sH+\sX\sY r,
\end{align*}
where we use the fact that $\sigma_{\max}\leq \sX\sY rn^2$.
We will use the above observations in the following proofs.


\begin{proof}
By the form of $\nabla^2 L(\theta,H,X,Y)$, we have
\begin{align*}
\vec(\Delta)^T\nabla^2 L(\theta,H,X,Y)\vec(\Delta)
&=\sum_{i\neq j}\frac{e^{P_{ij}}}{(1+e^{P_{ij}})^2}\left(\frac{1}{\sqrt{n}}\langle\Delta_{\theta},e_i+e_j\rangle+\langle\Delta_{H},z_iz_j^T\rangle+\frac1n\langle\Delta_{X}Y^T+X\Delta_{Y}^T,e_i e_j^T\rangle\right)^2\\
&\quad +\frac2n\sum_{i\neq j}\left(\frac{e^{P_{ij}}}{1+e^{P_{ij}}}-A_{ij}\right)\langle\Delta_X,e_ie_j^T\Delta_Y\rangle.
\end{align*}
Thus, it holds that
\begin{align}\label{eq:convexity}
&\vec(\Delta)^T\nabla^2 f_{\aug}(\theta,H,X,Y)\vec(\Delta)\notag\\
&=\vec(\Delta)^T\nabla^2 L(\theta,H,X,Y)\vec(\Delta)
+\lambda\|\Delta_X\|_F^2+\lambda\|\Delta_Y\|_F^2+\frac{2c_{\aug}}{n^2}\|\Delta_X^T X+X^T\Delta_X-\Delta_Y^T Y-Y^T\Delta_Y\|_F^2\notag\\
&=\sum_{i\neq j}\frac{e^{P_{ij}}}{(1+e^{P_{ij}})^2}\left(\frac{1}{\sqrt{n}}\langle\Delta_{\theta},e_i+e_j\rangle+\langle\Delta_{H},z_iz_j^T\rangle+\frac1n\langle\Delta_{X}Y^T+X\Delta_{Y}^T,e_i e_j^T\rangle\right)^2\notag\\
&\quad+\lambda\|\Delta_X\|_F^2+\lambda\|\Delta_Y\|_F^2+\frac{2c_{\aug}}{n^2}\|\Delta_X^T X+X^T\Delta_X-\Delta_Y^T Y-Y^T\Delta_Y\|_F^2\notag\\
&\quad +\frac2n\sum_{i\neq j}\left(\frac{e^{P_{ij}}}{1+e^{P_{ij}}}-A_{ij}\right)\langle\Delta_X,e_ie_j^T\Delta_Y\rangle.   
\end{align}
We first deal with the last term, which is the only term that contains $A_{ij}$ thus has randomness. Note that
\begin{align*}
& \frac2n\sum_{i\neq j}\left(\frac{e^{P_{ij}}}{1+e^{P_{ij}}}-A_{ij}\right)\langle\Delta_X,e_ie_j^T\Delta_Y\rangle\\
& =\frac2n\sum_{i\neq j}\left(\frac{e^{P_{ij}}}{1+e^{P_{ij}}}-\frac{e^{P^{*}_{ij}}}{1+e^{P^{*}_{ij}}}\right)\langle\Delta_X,e_ie_j^T\Delta_Y\rangle+\frac2n\sum_{i\neq j}\left(\frac{e^{P^{*}_{ij}}}{1+e^{P^{*}_{ij}}}-A_{ij}\right)\langle\Delta_X,e_ie_j^T\Delta_Y\rangle.  
\end{align*}
For the first term, we have
\begin{align*}
&\left|\frac2n\sum_{i\neq j}\left(\frac{e^{P_{ij}}}{1+e^{P_{ij}}}-\frac{e^{P^{*}_{ij}}}{1+e^{P^{*}_{ij}}}\right)\langle\Delta_X,e_ie_j^T\Delta_Y\rangle\right|\\
&=\left|\frac2n\sum_{i\neq j}\left(\frac{e^{P_{ij}}}{1+e^{P_{ij}}}-\frac{e^{P^{*}_{ij}}}{1+e^{P^{*}_{ij}}}\right)(\Delta_X\Delta_Y^T)_{ij}\right|\\
&\leq \frac{1}{n}\sum_{i\neq j}|P_{ij}-P_{ij}^*||(\Delta_X\Delta_Y^T)_{ij}|\tag{\text{mean-value theorem}}\\
&\leq \frac{1}{n}\|\Delta_X\Delta_Y^T\|_F\cdot\sqrt{\sum_{i\neq j}(P_{ij}-P_{ij}^*)^2}\tag{\text{Cauchy}}.
\end{align*}
Note that
\begin{align*}
&\sum_{i\neq j}(P_{ij}-P_{ij}^*)^2\\
&=\sum_{i\neq j}\left(\frac{1}{\sqrt{n}}\langle\theta-\theta^*,e_i+e_j\rangle+\langle H-H^*,z_iz_j^T\rangle+\frac1n\langle XY^T-X^*Y^{*T},e_i e_j^T\rangle\right)^2\\
&=
\begin{bmatrix}
  \vec(\theta-\theta^*)\\
  \vec(H-H^*)\\
  \frac1n\vec(XY^T-X^*Y^{*T})
\end{bmatrix}^T
\left(\sum_{i\neq j}
  \begin{bmatrix}
  \frac{1}{\sqrt{n}}\vec(e_i+e_j)\\
  \vec(z_iz_j^T)\\
  \vec(e_ie_j^T)
  \end{bmatrix}
   \begin{bmatrix}
  \frac{1}{\sqrt{n}}\vec(e_i+e_j)\\
  \vec(z_iz_j^T)\\
  \vec(e_ie_j^T)
  \end{bmatrix}^T
\right)
\begin{bmatrix}
  \vec(\theta-\theta^*)\\
  \vec(H-H^*)\\
  \frac1n\vec(XY^T-X^*Y^{*T})
\end{bmatrix}\\
&\leq \su \left\|\begin{bmatrix}
  \vec(\theta-\theta^*)\\
  \vec(H-H^*)\\
  \frac1n\vec(XY^T-X^*Y^{*T})
\end{bmatrix}\right\|^2 \tag{By Assumption \ref{assumption:eigenvalues} and $\mathbf{1}^T(\theta-\theta^*)=0$}\\
& =\su\|\theta-\theta^{*}\|^2_{2}+\su\|H-H^{*}\|^2_{F}+\frac{\su}{n^2}\|XY^T-X^{*}Y^{*T}\|^2_{F}.
\end{align*}
Thus, we have
\begin{align*}
 &\left|\frac2n\sum_{i\neq j}\left(\frac{e^{P_{ij}}}{1+e^{P_{ij}}}-\frac{e^{P^{*}_{ij}}}{1+e^{P^{*}_{ij}}}\right)\langle\Delta_X,e_ie_j^T\Delta_Y\rangle\right|\\
 &\leq   \frac{\sqrt{\su}}{n}\|\Delta_X\Delta_Y^T\|_F\cdot\left(\|\theta-\theta^{*}\|_{2}+\|H-H^{*}\|_{F}+\frac{1}{n}\|XY^T-X^{*}Y^{*T}\|_{F}\right)\\
 &\leq   \sqrt{\frac{\su}{n}}\|\Delta_X\Delta_Y^T\|_F\cdot\left(c_1+c_2+\frac{3c_3\sqrt{\sigma_{\max}}}{n}\right)\tag{By the observations}\\
 &\leq c\frac{\sigma_{\min}}{n^{5/2}}\|\Delta_X\Delta_Y^T\|_F\tag{as long as $\sqrt{\su}\left(c_1+c_2+\frac{3c_3\sqrt{\sigma_{\max}}}{n}\right)\leq c\frac{\sigma_{\min}}{n^2}$ for some $c$}\\
 &\leq c\frac{\sigma_{\min}}{n^{5/2}}\left(\|\Delta_X\|_F^2+\|\Delta_Y\|_F^2\right)\tag{$ab\leq a^2+b^2$}
\end{align*}
For the second term, note that $(\frac{e^{P^{*}_{ij}}}{1+e^{P^{*}_{ij}}}-A_{ij})(\Delta_X\Delta_Y^T)_{ij}$ is mean-zero $|(\Delta_X\Delta_Y^T)_{ij}|^2$-subgaussian variable. By the independency, it holds that
\begin{align*}
\sum_{i\neq j}\left(\frac{e^{P^{*}_{ij}}}{1+e^{P^{*}_{ij}}}-A_{ij}\right)(\Delta_X\Delta_Y^T)_{ij}
\end{align*}
is mean-zero $\|\Delta_X\Delta_Y^T\|^2_F$-subgaussian variable. Thus, with probability at least $1-n^{-10}$, we have
\begin{align*}
  \left|\sum_{i\neq j}\left(\frac{e^{P^{*}_{ij}}}{1+e^{P^{*}_{ij}}}-A_{ij}\right)(\Delta_X\Delta_Y^T)_{ij}  \right|\lesssim \|\Delta_X\Delta_Y^T\|_F\sqrt{\log n}.
\end{align*}
As a result, with probability at least $1-n^{-10}$, we have
\begin{align*}
&\left|\frac2n\sum_{i\neq j}\left(\frac{e^{P^{*}_{ij}}}{1+e^{P^{*}_{ij}}}-A_{ij}\right)\langle\Delta_X,e_ie_j^T\Delta_Y\rangle\right|\\
&\lesssim \frac{\sqrt{\log n}}{n}\|\Delta_X\Delta_Y^T\|_F\\
 &\leq \frac{\sigma_{\min}}{n^{5/2}}\|\Delta_X\Delta_Y^T\|_F\tag{as long as $\sqrt{\frac{\log n}{n}}\ll \frac{\sigma_{\min}}{n^2}$ }\\
 &\leq \frac{\sigma_{\min}}{n^{5/2}}\left(\|\Delta_X\|_F^2+\|\Delta_Y\|_F^2\right)\tag{$ab\leq a^2+b^2$}.
\end{align*}
To summarize, we show that with probability at least $1-n^{-10}$,
\begin{align*}
    \left|\frac2n\sum_{i\neq j}\left(\frac{e^{P_{ij}}}{1+e^{P_{ij}}}-A_{ij}\right)\langle\Delta_X,e_ie_j^T\Delta_Y\rangle\right|\leq c\frac{\sigma_{\min}}{n^{5/2}}\left(\|\Delta_X\|_F^2+\|\Delta_Y\|_F^2\right).
\end{align*}

For the rest of the terms, note that
\begin{align}\label{ineq:convexity_upper}
&\sum_{i\neq j}\frac{e^{P_{ij}}}{(1+e^{P_{ij}})^2}\left(\frac{1}{\sqrt{n}}\langle\Delta_{\theta},e_i+e_j\rangle+\langle\Delta_{H},z_iz_j^T\rangle+\frac1n\langle\Delta_{X}Y^T+X\Delta_{Y}^T,e_i e_j^T\rangle\right)^2\notag\\
&\quad+\frac{2c_{\aug}}{n^2}\|\Delta_X^T X+X^T\Delta_X-\Delta_Y^T Y-Y^T\Delta_Y\|_F^2   \notag \\
&\leq \frac14
\begin{bmatrix}
  \vec(\Delta_{\theta})\\
  \vec(\Delta_{H})\\
  \frac1n\vec(\Delta_{X}Y^T+X\Delta_{Y}^T)
\end{bmatrix}^T
\left(\sum_{i\neq j}
  \begin{bmatrix}
  \frac{1}{\sqrt{n}}\vec(e_i+e_j)\\
  \vec(z_iz_j^T)\\
  \vec(e_ie_j^T)
  \end{bmatrix}
   \begin{bmatrix}
  \frac{1}{\sqrt{n}}\vec(e_i+e_j)\\
  \vec(z_iz_j^T)\\
  \vec(e_ie_j^T)
  \end{bmatrix}^T
\right)
\begin{bmatrix}
  \vec(\Delta_{\theta})\\
  \vec(\Delta_{H})\\
  \frac1n\vec(\Delta_{X}Y^T+X\Delta_{Y}^T)
\end{bmatrix}\notag\\
&\quad+\frac{2c_{\aug}}{n^2}\|\Delta_X^T X+X^T\Delta_X-\Delta_Y^T Y-Y^T\Delta_Y\|_F^2    \notag\\
&\leq \su\|\Delta_{\theta}\|^2_F+\su\|\Delta_{H}\|^2_F+\frac{\su}{n^2} \|\Delta_{X}Y^T+X\Delta_{Y}^T\|^2_F+\frac{2c_{\aug}}{n^2}\|\Delta_X^T X+X^T\Delta_X-\Delta_Y^T Y-Y^T\Delta_Y\|_F^2\notag\\
&\leq \su\|\Delta_{\theta}\|^2_F+\su\|\Delta_{H}\|^2_F+\frac{\su}{n^2} \|\Delta_{X}Y^T+X\Delta_{Y}^T\|^2_F+\frac{\su}{4n^2}\|\Delta_X^T X+X^T\Delta_X-\Delta_Y^T Y-Y^T\Delta_Y\|_F^2 ,
\end{align}
where the second inequality follows from Assumption \ref{assumption:eigenvalues} and the condition that $\mathbf{1}^T\Delta_{\theta}=0$, and the third inequality follows from the fact that $8c_{\aug}\leq \su$.
Moreover, we have
\begin{align*}
&\sum_{i\neq j}\frac{e^{P_{ij}}}{(1+e^{P_{ij}})^2}\left(\frac{1}{\sqrt{n}}\langle\Delta_{\theta},e_i+e_j\rangle+\langle\Delta_{H},z_iz_j^T\rangle+\frac1n\langle\Delta_{X}Y^T+X\Delta_{Y}^T,e_i e_j^T\rangle\right)^2\\
&\quad+\frac{2c_{\aug}}{n^2}\|\Delta_X^T X+X^T\Delta_X-\Delta_Y^T Y-Y^T\Delta_Y\|_F^2    \\
&\geq \frac{e^{2c_P}}{(1+e^{2c_P})^2}
\begin{bmatrix}
  \vec(\Delta_{\theta})\\
  \vec(\Delta_{H})\\
  \frac1n\vec(\Delta_{X}Y^T+X\Delta_{Y}^T)
\end{bmatrix}^T
\left(\sum_{i\neq j}
  \begin{bmatrix}
  \frac{1}{\sqrt{n}}\vec(e_i+e_j)\\
  \vec(z_iz_j^T)\\
  \vec(e_ie_j^T)
  \end{bmatrix}
   \begin{bmatrix}
  \frac{1}{\sqrt{n}}\vec(e_i+e_j)\\
  \vec(z_iz_j^T)\\
  \vec(e_ie_j^T)
  \end{bmatrix}^T
\right)
\begin{bmatrix}
  \vec(\Delta_{\theta})\\
  \vec(\Delta_{H})\\
  \frac1n\vec(\Delta_{X}Y^T+X\Delta_{Y}^T)
\end{bmatrix}\\
&\quad+\frac{2c_{\aug}}{n^2}\|\Delta_X^T X+X^T\Delta_X-\Delta_Y^T Y-Y^T\Delta_Y\|_F^2  
\end{align*}
since by observations, we know $|P_{ij}|\leq 2c_P$. Then, similarly, by Assumption \ref{assumption:eigenvalues} and the condition that $\mathbf{1}^T\Delta_{\theta}=0$, we have
\begin{align}\label{ineq:convexity_lower}
&\sum_{i\neq j}\frac{e^{P_{ij}}}{(1+e^{P_{ij}})^2}\left(\frac{1}{\sqrt{n}}\langle\Delta_{\theta},e_i+e_j\rangle+\langle\Delta_{H},z_iz_j^T\rangle+\frac1n\langle\Delta_{X}Y^T+X\Delta_{Y}^T,e_i e_j^T\rangle\right)^2\notag\\
&\quad+\frac{2c_{\aug}}{n^2}\|\Delta_X^T X+X^T\Delta_X-\Delta_Y^T Y-Y^T\Delta_Y\|_F^2   \notag \\
&\geq \sl\frac{e^{2c_P}}{(1+e^{2c_P})^2}\left(\|\Delta_{\theta}\|^2_F+\|\Delta_{H}\|^2_F+\frac{1}{n^2} \|\Delta_{X}Y^T+X\Delta_{Y}^T\|^2_F\right)+\frac{2c_{\aug}}{n^2}\|\Delta_X^T X+X^T\Delta_X-\Delta_Y^T Y-Y^T\Delta_Y\|_F^2\notag\\
&= \sl\frac{e^{2c_P}}{(1+e^{2c_P})^2}\left(\|\Delta_{\theta}\|^2_F+\|\Delta_{H}\|^2_F+\frac{1}{n^2} \|\Delta_{X}Y^T+X\Delta_{Y}^T\|^2_F\right)\notag\\
&\quad +\frac{\sl e^{2c_P}}{4(1+e^{2c_P})^2n^2}\|\Delta_X^T X+X^T\Delta_X-\Delta_Y^T Y-Y^T\Delta_Y\|_F^2
\end{align}
By \eqref{eq:convexity}, \eqref{ineq:convexity_upper} and \eqref{ineq:convexity_lower}, to obtain the local geometry results, we only need to bound:
\begin{align}\label{term1:lem_convexity}
\|\Delta_{X}Y^T+X\Delta_{Y}^T\|^2_F+\frac{1}{4}\|\Delta_X^T X+X^T\Delta_X-\Delta_Y^T Y-Y^T\Delta_Y\|_F^2 .  
\end{align}
For the upper bound of \eqref{term1:lem_convexity}, note that 
\begin{align*}
&\|\Delta_{X}Y^T+X\Delta_{Y}^T\|^2_F\leq \left(\|Y\|\|\Delta_X\|_F+\|X\|\|\Delta_Y\|_F\right)^2   \leq \left(\|X\|^2+\|Y\|^2\right)\left(\|\Delta_X\|_F^2+\|\Delta_Y\|_F^2\right),\\
 &\|\Delta_X^T X+X^T\Delta_X-\Delta_Y^T Y-Y^T\Delta_Y\|_F^2\leq 4\left(\|X\|^2+\|Y\|^2\right)\left(\|\Delta_X\|_F^2+\|\Delta_Y\|_F^2\right).
\end{align*}
Thus, it holds that
\begin{align*}
&\|\Delta_{X}Y^T+X\Delta_{Y}^T\|^2_F+\frac{1}{4}\|\Delta_X^T X+X^T\Delta_X-\Delta_Y^T Y-Y^T\Delta_Y\|_F^2\\
&\leq
2\left(\|X\|^2+\|Y\|^2\right)\left(\|\Delta_X\|_F^2+\|\Delta_Y\|_F^2\right).
\end{align*}
By Weyl's inequality, we have
\begin{align*}
|\sigma_{\max}(X)-\sigma_{\max}(X^{*})|\leq \|XR-X^{*}\|\leq c_3 \sqrt{n},\  |\sigma_{\max}(Y)-\sigma_{\max}(Y^{*})|\leq \|YR-Y^{*}\|\leq c_3 \sqrt{n}.
\end{align*}
As long as $c_3\sqrt{n}\ll \sqrt{\sigma_{\max}}$, we have 
\begin{align*}
\sigma_{\max}(X)\leq 2\sqrt{\sigma_{\max}},\ 
\sigma_{\max}(Y)\leq 2\sqrt{\sigma_{\max}},
\end{align*}
which implies
\begin{align*}
\|\Delta_{X}Y^T+X\Delta_{Y}^T\|^2_F+\frac{1}{4}\|\Delta_X^T X+X^T\Delta_X-\Delta_Y^T Y-Y^T\Delta_Y\|_F^2  \leq 16 \sigma_{\max} \left(\|\Delta_X\|_F^2+\|\Delta_Y\|_F^2\right).
\end{align*}

For the lower bound of \eqref{term1:lem_convexity}, note that 
\begin{align*}
&\left\| \Delta_X Y^{T} + X \Delta_Y^{T} \right\|_F^2 + \frac{1}{4} \left\| \Delta_X^{T} X + X^{T} \Delta_X -\Delta_Y^T Y-Y^T\Delta_Y\right\|_F^2 \\
&= \left\| \Delta_X Y^{T} \right\|_F^2 + \left\| X \Delta_Y^{T} \right\|_F^2 + \frac12\left\| \Delta_X^{T} X \right\|_F^2 + \frac{1}{2} \left\| \Delta_Y^{T} Y \right\|_F^2 - \left\langle \Delta_X^{T} X, \Delta_Y^{T} Y \right\rangle  \\
&\quad+\frac{1}{2} \left\langle X^{T} \Delta_X, \Delta_X^{T} X \right\rangle+ \frac{1}{2} \left\langle Y^{T} \Delta_Y, \Delta_Y^{T} Y \right\rangle+ \left\langle \Delta_X^T X, Y^{T} \Delta_Y \right\rangle \\
&= \left\| \Delta_X Y^{T} \right\|_F^2 + \left\| X \Delta_Y^{T} \right\|_F^2 + \frac12\left\| \Delta_X^{T} X - \Delta_Y^{T} Y \right\|_F^2 + \frac{1}{2} \left\langle X^{T} \Delta_X + Y^T\Delta_Y, \Delta_X^{T} X + \Delta_Y^{T} Y \right\rangle \\
&= \left\| \Delta_X Y^{T} \right\|_F^2 + \left\| X \Delta_Y^{T} \right\|_F^2 + \frac12\left\| \Delta_X^{T} X - \Delta_Y^{T} Y \right\|_F^2 \\
&\quad+ \frac{1}{2} \left\langle (XR)^{T} (\Delta_X R)+(YR)^T(\Delta_Y R), (\Delta_X R)^{T} (XR) + (\Delta_YR)^{T} (YR) \right\rangle \\
&= \left\| \Delta_X Y^{T} \right\|_F^2 + \left\| X \Delta_Y^{T} \right\|_F^2 + \frac12\left\| \Delta_X^{T} X - \Delta_Y^{T} Y \right\|_F^2 \\
&\quad+ \frac{1}{2} \left\langle X_2^{T} (\Delta_X R)+Y_2^T(\Delta_Y R), (\Delta_X R)^TX_2 + (\Delta_Y R)^T Y_2 \right\rangle + \mathcal{E}_1 \\
&=  \left\| \Delta_X Y^{T} \right\|_F^2 + \left\| X \Delta_Y^{T} \right\|_F^2 + \frac12\left\| \Delta_X^{T} X - \Delta_Y^{T} Y \right\|_F^2  + \frac12\left\| X_2^{T} \Delta_X +Y_2^T\Delta_Y  \right\|_F^2 + \mathcal{E}_1,
\end{align*}
where 
\begin{align*}
% \mathcal{E}_1 &:= \frac{1}{2} \left\langle (X - X_2)^{T} \Delta_X + (Y - Y_2)^{T} \Delta_Y, \Delta_X^{T} X_2 + \Delta_Y^{T} Y_2 \right\rangle \\
% & \quad+ \frac{1}{2} \left\langle X_2^{T} \Delta_X + Y_2^{T} \Delta_Y, \Delta_X^{T} (X - X_2) + \Delta_Y^{T} (Y - Y_2) \right\rangle \\
% & \quad+ \frac{1}{2} \left\langle (X - X_2)^{T} \Delta_X + (Y - Y_2)^{T} \Delta_Y, \Delta_X^{T} (X - X_2) + \Delta_Y^{T} (Y - Y_2) \right\rangle\\
\mathcal{E}_1 &:=  \left\langle (XR - X_2)^{T} \Delta_X R + (YR - Y_2)^{T} \Delta_Y R, (\Delta_X R)^{T} X_2 + (\Delta_Y R)^{T} Y_2 \right\rangle \\
& \quad+ \frac{1}{2} \left\langle (X R- X_2)^{T} \Delta_X R + (YR - Y_2)^{T} \Delta_Y R, (\Delta_X R)^{T} (XR - X_2) + (\Delta_Y R)^{T} (YR - Y_2) \right\rangle.
\end{align*}
Based on the fact that $|\langle A,B\rangle|\leq\|A\|_F\|B\|_F$ and $\|AB\|_F\leq \|A\|\|B\|_F$, we have
\begin{align*}
|\mathcal{E}_1|\leq 
\left((\|XR-X_2\|+\|YR-Y_2\|)(\|X_2\|+\|Y_2\|)+\frac12 (\|XR-X_2\|+\|YR-Y_2\|)^2\right)\left(\|\Delta_X\|^2_F+\|\Delta_Y\|^2_F\right).
\end{align*}
By the definition of $X_2,Y_2$, as long as $c_4\sqrt{n}\ll \sqrt{\sigma_{\max}}$, we have 
\begin{align*}
\|X_2\|\leq \|X_2-X^*\|+\|X^*\|\leq 2 \sqrt{\sigma_{\max}},\ \|Y_2\|\leq \|Y_2-X^*\|+\|Y^*\|\leq 2 \sqrt{\sigma_{\max}}.
\end{align*}
Moreover, by the observations, we have
\begin{align*}
&\|XR-X_2\|\leq \|XR-X^*\|+\|X_2-X^*\|\leq (c_3+c_4)\sqrt{n},\notag\\
&\|YR-Y_2\|\leq \|YR-Y^*\|+\|Y_2-Y^*\|\leq (c_3+c_4) \sqrt{n}.
\end{align*}
Thus, we have
\begin{align*}
 |\mathcal{E}_1|\leq 10(c_3+c_4) \sqrt{n\sigma_{\max}}  \left(\|\Delta_X\|^2_F+\|\Delta_Y\|^2_F\right).
\end{align*}
As a result, we have
\begin{align*}
 &\left\| \Delta_X Y^{T} + X \Delta_Y^{T} \right\|_F^2 + \frac{1}{4} \left\| \Delta_X^{T} X + X^{T} \Delta_X -\Delta_Y^T Y-Y^T\Delta_Y\right\|_F^2 \\
 &\geq  \left\| \Delta_X Y^{T} \right\|_F^2 + \left\| X \Delta_Y^{T} \right\|_F^2  - |\mathcal{E}_1|\\
 &\geq \frac{\sigma_{\min}}{4}\left(\left\| \Delta_X \right\|_F^2 + \left\|  \Delta_Y \right\|_F^2 \right)- |\mathcal{E}_1|\\
 &\geq \left(\frac{\sigma_{\min}}{4}-10(c_3+c_4) \sqrt{n\sigma_{\max}}  \right)\left(\left\| \Delta_X \right\|_F^2 + \left\|  \Delta_Y \right\|_F^2 \right).
\end{align*}
% and 
% \begin{align*}
%  &\left\| \Delta_X Y^{T} + X \Delta_Y^{T} \right\|_F^2 + \frac{1}{4} \left\| \Delta_X^{T} X + X^{T} \Delta_X -\Delta_Y^T Y-Y^T\Delta_Y\right\|_F^2 \\
%  &\lesssim \left(\|X\|^2+\|Y\|^2+\|X_2\|^2+\|Y_2\|^2\right) \left(\left\| \Delta_X \right\|_F^2 + \left\|  \Delta_Y \right\|_F^2 \right)  +|\mathcal{E}_1|\\
%  &\lesssim\sigma_{\max}\left(\left\| \Delta_X \right\|_F^2 + \left\|  \Delta_Y \right\|_F^2 \right)+ |\mathcal{E}_1|\\
%  &\lesssim (\sigma_{\max}+\lambda n^2)\left(\left\| \Delta_X \right\|_F^2 + \left\|  \Delta_Y \right\|_F^2 \right).
% \end{align*}
Here we use Weyl's inequality to obtain that
\begin{align*}
|\sigma_{\min}(X)-\sigma_{\min}(X^{*})|\leq \|XR-X^{*}\|\leq c_3 \sqrt{n},\  |\sigma_{\min}(Y)-\sigma_{\min}(Y^{*})|\leq \|YR-Y^{*}\|\leq c_3 \sqrt{n}.
\end{align*}
As long as $c_3\sqrt{n}\ll \sqrt{\sigma_{\min}}$, we have
\begin{align*}
  \sigma_{\min}(X)\geq \frac12\sqrt{\sigma_{\min}}, \ \sigma_{\min}(Y)\geq\frac12\sqrt{\sigma_{\min}}.
\end{align*}

Combine the upper and lower bound for \eqref{term1:lem_convexity} with \eqref{ineq:convexity_upper} and \eqref{ineq:convexity_lower}, we obtain that
\begin{align*}
&\sum_{i\neq j}\frac{e^{P_{ij}}}{(1+e^{P_{ij}})^2}\left(\frac{1}{\sqrt{n}}\langle\Delta_{\theta},e_i+e_j\rangle+\langle\Delta_{H},z_iz_j^T\rangle+\frac1n\langle\Delta_{X}Y^T+X\Delta_{Y}^T,e_i e_j^T\rangle\right)^2\notag\\
&\quad+\frac{2c_{\aug}}{n^2}\|\Delta_X^T X+X^T\Delta_X-\Delta_Y^T Y-Y^T\Delta_Y\|_F^2   \notag \\
&\leq\su\|\Delta_{\theta}\|^2_F+\su\|\Delta_{H}\|^2_F+ \frac{16\su\sigma_{\max}}{n^2}\left(\left\| \Delta_X \right\|_F^2 + \left\|  \Delta_Y \right\|_F^2 \right),
\end{align*}
and 
\begin{align*}
&\sum_{i\neq j}\frac{e^{P_{ij}}}{(1+e^{P_{ij}})^2}\left(\frac{1}{\sqrt{n}}\langle\Delta_{\theta},e_i+e_j\rangle+\langle\Delta_{H},z_iz_j^T\rangle+\frac1n\langle\Delta_{X}Y^T+X\Delta_{Y}^T,e_i e_j^T\rangle\right)^2\notag\\
&\quad+\frac{2c_{\aug}}{n^2}\|\Delta_X^T X+X^T\Delta_X-\Delta_Y^T Y-Y^T\Delta_Y\|_F^2   \notag \\
&\geq \sl\frac{e^{2c_P}}{(1+e^{2c_P})^2}\left(\|\Delta_{\theta}\|^2_F+\|\Delta_{H}\|^2_F+ \frac{1}{n^2}\left(\frac{\sigma_{\min}}{4}-10(c_3+c_4) \sqrt{n\sigma_{\max}}  \right)\left(\left\| \Delta_X \right\|_F^2 + \left\|  \Delta_Y \right\|_F^2 \right)\right).
\end{align*}

Combine the above results with \eqref{eq:convexity}, we final obtain that with probability at least $1-n^{-10}$, we have
\begin{align*}
 &\vec(\Delta)^T\nabla^2 f_{\aug}(\theta,H,X,Y)\vec(\Delta)\notag\\  
 &\leq \su\|\Delta_{\theta}\|^2_F+\su\|\Delta_{H}\|^2_F+ \left(\frac{16\su\sigma_{\max}}{n^2}+\lambda +c\frac{\sigma_{\min}}{n^{5/2}}\right)\left(\left\| \Delta_X \right\|_F^2 + \left\|  \Delta_Y \right\|_F^2 \right)\\
 &\leq \su|\Delta_{\theta}\|^2_F+\su\|\Delta_{H}\|^2_F+\frac{20\su\sigma_{\max}}{n^2}\left(\left\| \Delta_X \right\|_F^2 + \left\|  \Delta_Y \right\|_F^2 \right)
\end{align*}
as long as $\lambda, c\frac{\sigma_{\min}}{n^{5/2}}\ll \frac{\su\sigma_{\max}}{n^2}$,
and 
\begin{align*}
 &\vec(\Delta)^T\nabla^2 f_{\aug}(\theta,H,X,Y)\vec(\Delta)\notag\\  
 &\geq \sl\frac{e^{2c_P}}{(1+e^{2c_P})^2}\left(\|\Delta_{\theta}\|^2_F+\|\Delta_{H}\|^2_F\right)\notag\\
 &\quad+ \left(\sl\frac{e^{2c_P}}{(1+e^{2c_P})^2}\frac{1}{n^2}\left(\frac{\sigma_{\min}}{4}-10(c_3+c_4) \sqrt{n\sigma_{\max}}  \right)+\lambda -c\frac{\sigma_{\min}}{n^{5/2}}\right)\left(\left\| \Delta_X \right\|_F^2 + \left\|  \Delta_Y \right\|_F^2 \right)\\
 &\geq  \sl\frac{e^{2c_P}}{(1+e^{2c_P})^2}\left(  \|\Delta_{\theta}\|^2_F+\|\Delta_{H}\|^2_F+ \frac{\sigma_{\min}}{8n^2}\left(\left\| \Delta_X \right\|_F^2 + \left\|  \Delta_Y \right\|_F^2 \right)\right)
\end{align*}
as long as $\sigma_{\min}\gg 40(c_3+c_4)\sqrt{n\sigma_{\max}}$, $n\gg c^2$.
This further implies that 
\begin{align*}
\left\|\nabla^2f_{\aug}(\theta,H,X,Y)\right\|\leq \max\left\{\su,\frac{20\su\sigma_{\max}}{n^2}\right\}.
\end{align*}
We then finish the proofs.
\end{proof}

==> proof_convexity_v1.tex <==
\section{Proofs of Lemma \ref{lem:convexity}}\label{proof_convexity}

\paragraph{Observations}
Based on the constraints on $(\theta,H,X,Y)$, it can be seen that: 
\begin{align*}
 &\|\theta-\theta^{*}\|_{2}\lesssim \sqrt{n}, \\
 &\|XR-X^*\|\leq \|XR-X^*\|_{F}\leq \sqrt{n}\|XR-X^*\|_{2,\infty}\lesssim \sqrt{n}\\
 &\|YR-Y^*\|\leq \|YR-Y^*\|_{F}\leq \sqrt{n}\|YR-Y^*\|_{2,\infty}\lesssim \sqrt{n}.
\end{align*}
This further implies that
\begin{align*}
&\|XY^T-X^*Y^{*T}\|_{F}\\
&=\|(XR-X^*)(YR)^T+X^{*}(YR-Y^*)^T\|_F\\
&\leq \|XR-X^*\|_F\|YR\|+\|X^{*}\|\|(YR-Y^*)^T\|_F\\
&\lesssim n^{3/2},
\end{align*}
where we use the fact that $\|X^*\|=\|Y^*\|=\sqrt{\sigma_{\max}}=O(n)$. Moreover, we have
\begin{align*}
&\|XY^T-X^*Y^{*T}\|_{\infty}\\
&=\|(XR-X^*)(YR)^T+X^{*}(YR-Y^*)^T\|_{\infty}\\
&\leq \|XR-X^*\|_{2,\infty}\|YR\|_{2,\infty}+\|X^{*}\|_{2,\infty}\|(YR-Y^*)^T\|_{2,\infty} \tag{Cauchy}\\
&\lesssim \sqrt{n},
\end{align*}
where we use the fact that $\|X^*\|_{2,\infty}, \|Y^*\|_{2,\infty}=O(\sqrt{n})$. Thus, we obtain
\begin{align*}
|P_{ij}|&\leq |P^*_{ij}|+|P_{ij}-P^*_{ij}|\\
&\leq |P^*_{ij}|+\frac{2}{\sqrt{n}}\|\theta-\theta^*\|_{\infty}+\|H-H^*\|\|z_i\|\|z_j\|+\frac1n \|XY^T-X^*Y^{*T}\|_{\infty}\\
&\leq |P^*_{ij}|+\frac{1}{\sqrt{n}},
\end{align*}
where we use the fact that $\|z_i\|=O(\frac{1}{\sqrt{n}})$. Based on our scales assumptions, we know $|P^*_{ij}|$ is constant order and this leads to the fact that $|P_{ij}|\leq C$ for some constant $C$. We will use the above observations in the following proofs.


\begin{proof}
By the form of $\nabla^2 L(\theta,H,X,Y)$, we have
\begin{align*}
\vec(\Delta)^T\nabla^2 L(\theta,H,X,Y)\vec(\Delta)
&=\sum_{i\neq j}\frac{e^{P_{ij}}}{(1+e^{P_{ij}})^2}\left(\frac{1}{\sqrt{n}}\langle\Delta_{\theta},e_i+e_j\rangle+\langle\Delta_{H},z_iz_j^T\rangle+\frac1n\langle\Delta_{X}Y^T+X\Delta_{Y}^T,e_i e_j^T\rangle\right)^2\\
&\quad +\frac2n\sum_{i\neq j}\left(\frac{e^{P_{ij}}}{1+e^{P_{ij}}}-A_{ij}\right)\langle\Delta_X,e_ie_j^T\Delta_Y\rangle.
\end{align*}
Thus, it holds that
\begin{align}\label{eq:convexity}
&\vec(\Delta)^T\nabla^2 f_{\aug}(\theta,H,X,Y)\vec(\Delta)\notag\\
&=\vec(\Delta)^T\nabla^2 L(\theta,H,X,Y)\vec(\Delta)
+\lambda\|\Delta_X\|_F^2+\lambda\|\Delta_Y\|_F^2+\frac{1}{4n^2}\|\Delta_X^T X+X^T\Delta_X-\Delta_Y^T Y-Y^T\Delta_Y\|_F^2\notag\\
&=\sum_{i\neq j}\frac{e^{P_{ij}}}{(1+e^{P_{ij}})^2}\left(\frac{1}{\sqrt{n}}\langle\Delta_{\theta},e_i+e_j\rangle+\langle\Delta_{H},z_iz_j^T\rangle+\frac1n\langle\Delta_{X}Y^T+X\Delta_{Y}^T,e_i e_j^T\rangle\right)^2\notag\\
&\quad+\lambda\|\Delta_X\|_F^2+\lambda\|\Delta_Y\|_F^2+\frac{1}{4n^2}\|\Delta_X^T X+X^T\Delta_X-\Delta_Y^T Y-Y^T\Delta_Y\|_F^2\notag\\
&\quad +\frac2n\sum_{i\neq j}\left(\frac{e^{P_{ij}}}{1+e^{P_{ij}}}-A_{ij}\right)\langle\Delta_X,e_ie_j^T\Delta_Y\rangle.   
\end{align}
We first deal with the last term, which is the only term that contains $A_{ij}$ thus has randomness. Note that
\begin{align*}
& \frac2n\sum_{i\neq j}\left(\frac{e^{P_{ij}}}{1+e^{P_{ij}}}-A_{ij}\right)\langle\Delta_X,e_ie_j^T\Delta_Y\rangle\\
& =\frac2n\sum_{i\neq j}\left(\frac{e^{P_{ij}}}{1+e^{P_{ij}}}-\frac{e^{P^{*}_{ij}}}{1+e^{P^{*}_{ij}}}\right)\langle\Delta_X,e_ie_j^T\Delta_Y\rangle+\frac2n\sum_{i\neq j}\left(\frac{e^{P^{*}_{ij}}}{1+e^{P^{*}_{ij}}}-A_{ij}\right)\langle\Delta_X,e_ie_j^T\Delta_Y\rangle.  
\end{align*}
For the first term, we have
\begin{align*}
&\left|\frac2n\sum_{i\neq j}\left(\frac{e^{P_{ij}}}{1+e^{P_{ij}}}-\frac{e^{P^{*}_{ij}}}{1+e^{P^{*}_{ij}}}\right)\langle\Delta_X,e_ie_j^T\Delta_Y\rangle\right|\\
&=\left|\frac2n\sum_{i\neq j}\left(\frac{e^{P_{ij}}}{1+e^{P_{ij}}}-\frac{e^{P^{*}_{ij}}}{1+e^{P^{*}_{ij}}}\right)(\Delta_X\Delta_Y^T)_{ij}\right|\\
&\lesssim \frac{1}{n}\sum_{i\neq j}|P_{ij}-P_{ij}^*||(\Delta_X\Delta_Y^T)_{ij}|\tag{\text{mean-value theorem}}\\
&\leq \frac{1}{n}\|\Delta_X\Delta_Y^T\|_F\cdot\sqrt{\sum_{i\neq j}(P_{ij}-P_{ij}^*)^2}\tag{\text{Cauchy}}.
\end{align*}
Note that
\begin{align*}
&\sum_{i\neq j}(P_{ij}-P_{ij}^*)^2\\
&=\sum_{i\neq j}\left(\frac{1}{\sqrt{n}}\langle\theta-\theta^*,e_i+e_j\rangle+\langle H-H^*,z_iz_j^T\rangle+\frac1n\langle XY^T-X^*Y^{*T},e_i e_j^T\rangle\right)^2\\
&=
\begin{bmatrix}
  \vec(\theta-\theta^*)\\
  \vec(H-H^*)\\
  \frac1n\vec(XY^T-X^*Y^{*T})
\end{bmatrix}^T
\left(\sum_{i\neq j}
  \begin{bmatrix}
  \frac{1}{\sqrt{n}}\vec(e_i+e_j)\\
  \vec(z_iz_j^T)\\
  \vec(e_ie_j^T)
  \end{bmatrix}
   \begin{bmatrix}
  \frac{1}{\sqrt{n}}\vec(e_i+e_j)\\
  \vec(z_iz_j^T)\\
  \vec(e_ie_j^T)
  \end{bmatrix}^T
\right)
\begin{bmatrix}
  \vec(\theta-\theta^*)\\
  \vec(H-H^*)\\
  \frac1n\vec(XY^T-X^*Y^{*T})
\end{bmatrix}\\
&\lesssim \left\|\begin{bmatrix}
  \vec(\theta-\theta^*)\\
  \vec(H-H^*)\\
  \frac1n\vec(XY^T-X^*Y^{*T})
\end{bmatrix}\right\|^2 \tag{By the balanced eigenvalues assumption and $\mathbf{1}^T(\theta-\theta^*)=0$}\\
& =\|\theta-\theta^{*}\|^2_{2}+\|H-H^{*}\|^2_{F}+\frac{1}{n^2}\|XY^T-X^{*}Y^{*T}\|^2_{F}.
\end{align*}
Thus, we have
\begin{align*}
 &\left|\frac2n\sum_{i\neq j}\left(\frac{e^{P_{ij}}}{1+e^{P_{ij}}}-\frac{e^{P^{*}_{ij}}}{1+e^{P^{*}_{ij}}}\right)\langle\Delta_X,e_ie_j^T\Delta_Y\rangle\right|\\
 &\lesssim   \frac{1}{n}\|\Delta_X\Delta_Y^T\|_F\cdot\left(\|\theta-\theta^{*}\|_{2}+\|H-H^{*}\|_{F}+\frac{1}{n}\|XY^T-X^{*}Y^{*T}\|_{F}\right)\\
 &\lesssim   \frac{1}{n}\|\Delta_X\Delta_Y^T\|_F\cdot\sqrt{n}\tag{By the observations}\\
 &\lesssim \frac{\sigma_{\min}}{n^{5/2}}\|\Delta_X\Delta_Y^T\|_F\tag{since $\sigma_{\min}\sim n^2$}\\
 &\leq \frac{\sigma_{\min}}{n^{5/2}}\left(\|\Delta_X\|_F^2+\|\Delta_Y\|_F^2\right)\tag{$ab\leq a^2+b^2$}
\end{align*}
For the second term, note that $(\frac{e^{P^{*}_{ij}}}{1+e^{P^{*}_{ij}}}-A_{ij})(\Delta_X\Delta_Y^T)_{ij}$ is mean-zero $|(\Delta_X\Delta_Y^T)_{ij}|^2$-subgaussian variable. By the independency, it holds that
\begin{align*}
\sum_{i\neq j}\left(\frac{e^{P^{*}_{ij}}}{1+e^{P^{*}_{ij}}}-A_{ij}\right)(\Delta_X\Delta_Y^T)_{ij}
\end{align*}
is mean-zero $\|\Delta_X\Delta_Y^T\|^2_F$-subgaussian variable. Thus, with probability at least $1-n^{-10}$, we have
\begin{align*}
  \left|\sum_{i\neq j}\left(\frac{e^{P^{*}_{ij}}}{1+e^{P^{*}_{ij}}}-A_{ij}\right)(\Delta_X\Delta_Y^T)_{ij}  \right|\lesssim \|\Delta_X\Delta_Y^T\|_F\sqrt{\log n}.
\end{align*}
As a result, with probability at least $1-n^{-10}$, we have
\begin{align*}
&\left|\frac2n\sum_{i\neq j}\left(\frac{e^{P^{*}_{ij}}}{1+e^{P^{*}_{ij}}}-A_{ij}\right)\langle\Delta_X,e_ie_j^T\Delta_Y\rangle\right|\\
&\lesssim \frac{\sqrt{\log n}}{n}\|\Delta_X\Delta_Y^T\|_F\\
 &\lesssim \frac{\sigma_{\min}}{n^{5/2}}\|\Delta_X\Delta_Y^T\|_F\tag{since $\sigma_{\min}\sim n^2$}\\
 &\leq \frac{\sigma_{\min}}{n^{5/2}}\left(\|\Delta_X\|_F^2+\|\Delta_Y\|_F^2\right)\tag{$ab\leq a^2+b^2$}.
\end{align*}
To summarize, we show that with probability at least $1-n^{-10}$,
\begin{align*}
    \left|\frac2n\sum_{i\neq j}\left(\frac{e^{P_{ij}}}{1+e^{P_{ij}}}-A_{ij}\right)\langle\Delta_X,e_ie_j^T\Delta_Y\rangle\right|\lesssim \frac{\sigma_{\min}}{n^{5/2}}\left(\|\Delta_X\|_F^2+\|\Delta_Y\|_F^2\right).
\end{align*}

For the rest of the terms, note that
\begin{align}\label{ineq:convexity_upper}
&\sum_{i\neq j}\frac{e^{P_{ij}}}{(1+e^{P_{ij}})^2}\left(\frac{1}{\sqrt{n}}\langle\Delta_{\theta},e_i+e_j\rangle+\langle\Delta_{H},z_iz_j^T\rangle+\frac1n\langle\Delta_{X}Y^T+X\Delta_{Y}^T,e_i e_j^T\rangle\right)^2\notag\\
&\quad+\frac{1}{4n^2}\|\Delta_X^T X+X^T\Delta_X-\Delta_Y^T Y-Y^T\Delta_Y\|_F^2   \notag \\
&\leq \frac14
\begin{bmatrix}
  \vec(\Delta_{\theta})\\
  \vec(\Delta_{H})\\
  \frac1n\vec(\Delta_{X}Y^T+X\Delta_{Y}^T)
\end{bmatrix}^T
\left(\sum_{i\neq j}
  \begin{bmatrix}
  \frac{1}{\sqrt{n}}\vec(e_i+e_j)\\
  \vec(z_iz_j^T)\\
  \vec(e_ie_j^T)
  \end{bmatrix}
   \begin{bmatrix}
  \frac{1}{\sqrt{n}}\vec(e_i+e_j)\\
  \vec(z_iz_j^T)\\
  \vec(e_ie_j^T)
  \end{bmatrix}^T
\right)
\begin{bmatrix}
  \vec(\Delta_{\theta})\\
  \vec(\Delta_{H})\\
  \frac1n\vec(\Delta_{X}Y^T+X\Delta_{Y}^T)
\end{bmatrix}\notag\\
&\quad+\frac{1}{4n^2}\|\Delta_X^T X+X^T\Delta_X-\Delta_Y^T Y-Y^T\Delta_Y\|_F^2    \notag\\
&\lesssim \|\Delta_{\theta}\|^2_F+\|\Delta_{H}\|^2_F+\frac{1}{n^2} \|\Delta_{X}Y^T+X\Delta_{Y}^T\|^2_F+\frac{1}{4n^2}\|\Delta_X^T X+X^T\Delta_X-\Delta_Y^T Y-Y^T\Delta_Y\|_F^2 ,
\end{align}
where the last inequality follows from the balanced eigenvalues assumption and the condition that $\mathbf{1}^T\Delta_{\theta}=0$.
Moreover, we have
\begin{align*}
&\sum_{i\neq j}\frac{e^{P_{ij}}}{(1+e^{P_{ij}})^2}\left(\frac{1}{\sqrt{n}}\langle\Delta_{\theta},e_i+e_j\rangle+\langle\Delta_{H},z_iz_j^T\rangle+\frac1n\langle\Delta_{X}Y^T+X\Delta_{Y}^T,e_i e_j^T\rangle\right)^2\\
&\quad+\frac{1}{4n^2}\|\Delta_X^T X+X^T\Delta_X-\Delta_Y^T Y-Y^T\Delta_Y\|_F^2    \\
&\gtrsim
\begin{bmatrix}
  \vec(\Delta_{\theta})\\
  \vec(\Delta_{H})\\
  \frac1n\vec(\Delta_{X}Y^T+X\Delta_{Y}^T)
\end{bmatrix}^T
\left(\sum_{i\neq j}
  \begin{bmatrix}
  \frac{1}{\sqrt{n}}\vec(e_i+e_j)\\
  \vec(z_iz_j^T)\\
  \vec(e_ie_j^T)
  \end{bmatrix}
   \begin{bmatrix}
  \frac{1}{\sqrt{n}}\vec(e_i+e_j)\\
  \vec(z_iz_j^T)\\
  \vec(e_ie_j^T)
  \end{bmatrix}^T
\right)
\begin{bmatrix}
  \vec(\Delta_{\theta})\\
  \vec(\Delta_{H})\\
  \frac1n\vec(\Delta_{X}Y^T+X\Delta_{Y}^T)
\end{bmatrix}\\
&\quad+\frac{1}{4n^2}\|\Delta_X^T X+X^T\Delta_X-\Delta_Y^T Y-Y^T\Delta_Y\|_F^2  
\end{align*}
since by observations, we know $|P_{ij}|\leq C$ for some constant $C$. Then, similarly, by the balanced eigenvalues assumption and the condition that $\mathbf{1}^T\Delta_{\theta}=0$, we have
\begin{align}\label{ineq:convexity_lower}
&\sum_{i\neq j}\frac{e^{P_{ij}}}{(1+e^{P_{ij}})^2}\left(\frac{1}{\sqrt{n}}\langle\Delta_{\theta},e_i+e_j\rangle+\langle\Delta_{H},z_iz_j^T\rangle+\frac1n\langle\Delta_{X}Y^T+X\Delta_{Y}^T,e_i e_j^T\rangle\right)^2\notag\\
&\quad+\frac{1}{4n^2}\|\Delta_X^T X+X^T\Delta_X-\Delta_Y^T Y-Y^T\Delta_Y\|_F^2   \notag \\
&\gtrsim\|\Delta_{\theta}\|^2_F+\|\Delta_{H}\|^2_F+\frac{1}{n^2} \|\Delta_{X}Y^T+X\Delta_{Y}^T\|^2_F+\frac{1}{4n^2}\|\Delta_X^T X+X^T\Delta_X-\Delta_Y^T Y-Y^T\Delta_Y\|_F^2.
\end{align}
By \eqref{eq:convexity}, \eqref{ineq:convexity_upper} and \eqref{ineq:convexity_lower}, to obtain the local geometry results, we only need to bound:
\begin{align*}
\|\Delta_{X}Y^T+X\Delta_{Y}^T\|^2_F+\frac{1}{4}\|\Delta_X^T X+X^T\Delta_X-\Delta_Y^T Y-Y^T\Delta_Y\|_F^2 .  
\end{align*}
Note that 
\begin{align*}
&\left\| \Delta_X Y^{T} + X \Delta_Y^{T} \right\|_F^2 + \frac{1}{4} \left\| \Delta_X^{T} X + X^{T} \Delta_X -\Delta_Y^T Y-Y^T\Delta_Y\right\|_F^2 \\
&= \left\| \Delta_X Y^{T} \right\|_F^2 + \left\| X \Delta_Y^{T} \right\|_F^2 + \frac12\left\| \Delta_X^{T} X \right\|_F^2 + \frac{1}{2} \left\| \Delta_Y^{T} Y \right\|_F^2 - \left\langle \Delta_X^{T} X, \Delta_Y^{T} Y \right\rangle  \\
&\quad+\frac{1}{2} \left\langle X^{T} \Delta_X, \Delta_X^{T} X \right\rangle+ \frac{1}{2} \left\langle Y^{T} \Delta_Y, \Delta_Y^{T} Y \right\rangle+ \left\langle \Delta_X^T X, Y^{T} \Delta_Y \right\rangle \\
&= \left\| \Delta_X Y^{T} \right\|_F^2 + \left\| X \Delta_Y^{T} \right\|_F^2 + \frac12\left\| \Delta_X^{T} X - \Delta_Y^{T} Y \right\|_F^2 + \frac{1}{2} \left\langle X^{T} \Delta_X + Y^T\Delta_Y, \Delta_X^{T} X + \Delta_Y^{T} Y \right\rangle \\
&= \left\| \Delta_X Y^{T} \right\|_F^2 + \left\| X \Delta_Y^{T} \right\|_F^2 + \frac12\left\| \Delta_X^{T} X - \Delta_Y^{T} Y \right\|_F^2 \\
&\quad+ \frac{1}{2} \left\langle (XR)^{T} (\Delta_X R)+(YR)^T(\Delta_Y R), (\Delta_X R)^{T} (XR) + (\Delta_YR)^{T} (YR) \right\rangle \\
&= \left\| \Delta_X Y^{T} \right\|_F^2 + \left\| X \Delta_Y^{T} \right\|_F^2 + \frac12\left\| \Delta_X^{T} X - \Delta_Y^{T} Y \right\|_F^2 \\
&\quad+ \frac{1}{2} \left\langle X_2^{T} (\Delta_X R)+Y_2^T(\Delta_Y R), (\Delta_X R)^TX_2 + (\Delta_Y R)^T Y_2 \right\rangle + \mathcal{E}_1 \\
&=  \left\| \Delta_X Y^{T} \right\|_F^2 + \left\| X \Delta_Y^{T} \right\|_F^2 + \frac12\left\| \Delta_X^{T} X - \Delta_Y^{T} Y \right\|_F^2  + \frac12\left\| X_2^{T} \Delta_X +Y_2^T\Delta_Y  \right\|_F^2 + \mathcal{E}_1,
\end{align*}
where 
\begin{align*}
% \mathcal{E}_1 &:= \frac{1}{2} \left\langle (X - X_2)^{T} \Delta_X + (Y - Y_2)^{T} \Delta_Y, \Delta_X^{T} X_2 + \Delta_Y^{T} Y_2 \right\rangle \\
% & \quad+ \frac{1}{2} \left\langle X_2^{T} \Delta_X + Y_2^{T} \Delta_Y, \Delta_X^{T} (X - X_2) + \Delta_Y^{T} (Y - Y_2) \right\rangle \\
% & \quad+ \frac{1}{2} \left\langle (X - X_2)^{T} \Delta_X + (Y - Y_2)^{T} \Delta_Y, \Delta_X^{T} (X - X_2) + \Delta_Y^{T} (Y - Y_2) \right\rangle\\
\mathcal{E}_1 &:=  \left\langle (XR - X_2)^{T} \Delta_X R + (YR - Y_2)^{T} \Delta_Y R, (\Delta_X R)^{T} X_2 + (\Delta_Y R)^{T} Y_2 \right\rangle \\
& \quad+ \frac{1}{2} \left\langle (X R- X_2)^{T} \Delta_X R + (YR - Y_2)^{T} \Delta_Y R, (\Delta_X R)^{T} (XR - X_2) + (\Delta_Y R)^{T} (YR - Y_2) \right\rangle.
\end{align*}
Based on the fact that $|\langle A,B\rangle|\leq\|A\|_F\|B\|_F$ and $\|AB\|_F\leq \|A\|\|B\|_F$, we have
\begin{align*}
|\mathcal{E}_1|\leq 
\left((\|XR-X_2\|+\|YR-Y_2\|)(\|X_2\|+\|Y_2\|)+\frac12 (\|XR-X_2\|+\|YR-Y_2\|)^2\right)\left(\|\Delta_X\|^2_F+\|\Delta_Y\|^2_F\right).
\end{align*}
By the definition of $X_2,Y_2$, we have 
\begin{align*}
\|X_2\|\leq \|X_2-X^*\|+\|X^*\|\lesssim n,\ \|Y_2\|\leq \|Y_2-X^*\|+\|Y^*\|\lesssim n,
\end{align*}
where we use the fact that $\|X^*\|,\|Y^*\|=O(n)$. Moreover, by the observations, we have
\begin{align*}
\|XR-X_2\|\leq \|XR-X^*\|+\|X_2-X^*\|\lesssim \sqrt{n},\ \|YR-Y_2\|\leq \|YR-Y^*\|+\|Y_2-Y^*\|\lesssim \sqrt{n}.
\end{align*}
Thus, we have
\begin{align*}
 |\mathcal{E}_1|\lesssim n^{3/2}   \left(\|\Delta_X\|^2_F+\|\Delta_Y\|^2_F\right)\lesssim \lambda n^2\left(\|\Delta_X\|^2_F+\|\Delta_Y\|^2_F\right),
\end{align*}
where we use the fact that $\lambda=O(\frac{1}{\sqrt{n}})$.
As a result, we have
\begin{align*}
 &\left\| \Delta_X Y^{T} + X \Delta_Y^{T} \right\|_F^2 + \frac{1}{4} \left\| \Delta_X^{T} X + X^{T} \Delta_X -\Delta_Y^T Y-Y^T\Delta_Y\right\|_F^2 \\
 &\geq  \left\| \Delta_X Y^{T} \right\|_F^2 + \left\| X \Delta_Y^{T} \right\|_F^2  - |\mathcal{E}_1|\\
 &\gtrsim \sigma_{\min}\left(\left\| \Delta_X \right\|_F^2 + \left\|  \Delta_Y \right\|_F^2 \right)- |\mathcal{E}_1|\\
 &\gtrsim (\sigma_{\min}-\lambda n^2)\left(\left\| \Delta_X \right\|_F^2 + \left\|  \Delta_Y \right\|_F^2 \right),
\end{align*}
and 
\begin{align*}
 &\left\| \Delta_X Y^{T} + X \Delta_Y^{T} \right\|_F^2 + \frac{1}{4} \left\| \Delta_X^{T} X + X^{T} \Delta_X -\Delta_Y^T Y-Y^T\Delta_Y\right\|_F^2 \\
 &\lesssim \left(\|X\|^2+\|Y\|^2+\|X_2\|^2+\|Y_2\|^2\right) \left(\left\| \Delta_X \right\|_F^2 + \left\|  \Delta_Y \right\|_F^2 \right)  +|\mathcal{E}_1|\\
 &\lesssim\sigma_{\max}\left(\left\| \Delta_X \right\|_F^2 + \left\|  \Delta_Y \right\|_F^2 \right)+ |\mathcal{E}_1|\\
 &\lesssim (\sigma_{\max}+\lambda n^2)\left(\left\| \Delta_X \right\|_F^2 + \left\|  \Delta_Y \right\|_F^2 \right).
\end{align*}
Here we use Weyl's inequality to obtain that
\begin{align*}
|\sigma_i(X)-\sigma_i(X^{*})|\leq \|XR-Y^{*}\|\lesssim \sqrt{n},\  |\sigma_i(Y)-\sigma_i(Y^{*})|\leq \|YR-Y^{*}\|\lesssim \sqrt{n}.
\end{align*}
Since $\sigma_{\max}(X^{*}), \sigma_{\min}(X^{*}), \sigma_{\max}(Y^{*}), \sigma_{\min}(Y^{*}) = O(n)$, we have
\begin{align*}
&\sigma_{\max}(X)\lesssim\sigma_{\max}(X^{*})=\sqrt{\sigma_{\max}},\  \sigma_{\min}(X)\gtrsim\sigma_{\min}(X^{*})=\sqrt{\sigma_{\min}}, \\
&\sigma_{\max}(Y)\lesssim\sigma_{\max}(Y^{*})=\sqrt{\sigma_{\max}},\  \sigma_{\min}(Y)\gtrsim\sigma_{\min}(Y^{*})=\sqrt{\sigma_{\min}}.
\end{align*}

By \eqref{ineq:convexity_upper} and \eqref{ineq:convexity_lower}, we obtain that
\begin{align*}
&\sum_{i\neq j}\frac{e^{P_{ij}}}{(1+e^{P_{ij}})^2}\left(\frac{1}{\sqrt{n}}\langle\Delta_{\theta},e_i+e_j\rangle+\langle\Delta_{H},z_iz_j^T\rangle+\frac1n\langle\Delta_{X}Y^T+X\Delta_{Y}^T,e_i e_j^T\rangle\right)^2\notag\\
&\quad+\frac{1}{4n^2}\|\Delta_X^T X+X^T\Delta_X-\Delta_Y^T Y-Y^T\Delta_Y\|_F^2   \notag \\
&\lesssim\|\Delta_{\theta}\|^2_F+\|\Delta_{H}\|^2_F+ \left(\frac{\sigma_{\max}}{n^2}+\lambda \right)\left(\left\| \Delta_X \right\|_F^2 + \left\|  \Delta_Y \right\|_F^2 \right),
\end{align*}
and 
\begin{align*}
&\sum_{i\neq j}\frac{e^{P_{ij}}}{(1+e^{P_{ij}})^2}\left(\frac{1}{\sqrt{n}}\langle\Delta_{\theta},e_i+e_j\rangle+\langle\Delta_{H},z_iz_j^T\rangle+\frac1n\langle\Delta_{X}Y^T+X\Delta_{Y}^T,e_i e_j^T\rangle\right)^2\notag\\
&\quad+\frac{1}{4n^2}\|\Delta_X^T X+X^T\Delta_X-\Delta_Y^T Y-Y^T\Delta_Y\|_F^2   \notag \\
&\gtrsim\|\Delta_{\theta}\|^2_F+\|\Delta_{H}\|^2_F+ \left(\frac{\sigma_{\min}}{n^2}-\lambda \right)\left(\left\| \Delta_X \right\|_F^2 + \left\|  \Delta_Y \right\|_F^2 \right).
\end{align*}

Combine the above results with \eqref{eq:convexity}, we final obtain that with probability at least $1-n^{-10}$, we have
\begin{align*}
 &\vec(\Delta)^T\nabla^2 f_{\aug}(\theta,H,X,Y)\vec(\Delta)\notag\\  
 &\lesssim \|\Delta_{\theta}\|^2_F+\|\Delta_{H}\|^2_F+ \left(c\frac{\sigma_{\max}}{n^2}+c\lambda+\lambda +c\frac{\sigma_{\min}}{n^{5/2}}\right)\left(\left\| \Delta_X \right\|_F^2 + \left\|  \Delta_Y \right\|_F^2 \right)\\
 &\lesssim \|\Delta_{\theta}\|^2_F+\|\Delta_{H}\|^2_F+ \left(\frac{\sigma_{\max}}{n^2}+\lambda \right)\left(\left\| \Delta_X \right\|_F^2 + \left\|  \Delta_Y \right\|_F^2 \right),
\end{align*}
and 
\begin{align*}
 &\vec(\Delta)^T\nabla^2 f_{\aug}(\theta,H,X,Y)\vec(\Delta)\notag\\  
 &\gtrsim \|\Delta_{\theta}\|^2_F+\|\Delta_{H}\|^2_F+ \left(c\frac{\sigma_{\min}}{n^2}-c\lambda +\lambda -c\frac{\sigma_{\min}}{n^{5/2}}\right)\left(\left\| \Delta_X \right\|_F^2 + \left\|  \Delta_Y \right\|_F^2 \right)\\
 &\gtrsim  \|\Delta_{\theta}\|^2_F+\|\Delta_{H}\|^2_F+ \left(\frac{\sigma_{\min}}{n^2}+\lambda \right)\left(\left\| \Delta_X \right\|_F^2 + \left\|  \Delta_Y \right\|_F^2 \right).
\end{align*}
We then finish the proofs.
\end{proof}

==> proof_cv_ncv.tex <==
\section{Proofs for Section \ref{sec:cv_ncv}}\label{pf:cv_ncv}


\subsection{Proofs of Proposition \ref{prop:assumption_example}}\label{pf:prop_assumption_example}
In this example, we have
\begin{align*}
\Gamma^*=
\begin{bmatrix}
p\mathbf{1}\mathbf{1}^T & q\mathbf{1}\mathbf{1}^T\\
q\mathbf{1}\mathbf{1}^T & p\mathbf{1}\mathbf{1}^T\\
\end{bmatrix}
=\Pi
\begin{bmatrix}
p & q\\
q & p\\
\end{bmatrix}
\Pi^{T}
=\Pi
\begin{bmatrix}
1 & 1\\
1 & -1\\
\end{bmatrix}
\begin{bmatrix}
\frac{p+q}{2} & 0\\
0 & \frac{p-q}{2}\\
\end{bmatrix}
\begin{bmatrix}
1 & 1\\
1 & -1\\
\end{bmatrix}
\Pi^{T},
\end{align*}
where $\Pi\in\bbR^{n\times 2}$ with the first $n/2$ rows being $[1,0]$ and the last $n/2$ rows being $[0,1]$. It then holds that
\begin{align}\label{eq3:pf_example}
X^{*}=Y^{*}
=\Pi
\begin{bmatrix}
1 & 1\\
1 & -1\\
\end{bmatrix}
\begin{bmatrix}
\sqrt{\frac{p+q}{2}} & 0\\
0 & \sqrt{\frac{p-q}{2}}\\
\end{bmatrix}
=\begin{bmatrix}
\sqrt{\frac{p+q}{2}}\mathbf{1} & \sqrt{\frac{p-q}{2}} \mathbf{1}\\
\sqrt{\frac{p+q}{2}}\mathbf{1} & -\sqrt{\frac{p-q}{2}} \mathbf{1}
\end{bmatrix},
\end{align}
where $\mathbf{1}\in\bbR^{\frac{n}{2}\times 1}$.
We denote
\begin{align*}
&\cA_1:=\{(i,j)\mid 1\leq i,j\leq n/2, i\neq j\},\\
&\cA_2:=\{(i,j)\mid 1\leq i\leq n/2,n/2< j\leq n, i\neq j\},\\
&\cA_3:=\{(i,j)\mid n/2< i\leq n,1\leq j\leq n/2,i\neq j\},\\
&\cA_4:=\{(i,j)\mid n/2< i,j\leq n, i\neq j\}.
\end{align*}
Since $\theta^*=0, H^*=0$, we then have
\begin{align*}
D^{*}
&=
\sum_{(i,j)\in\cA_1}\frac{e^{\frac{p}{n}}}{(1+e^{\frac{p}{n}})^2}
\begin{bmatrix}
\frac1n e_i \left[\sqrt{\frac{p+q}{2}}, \sqrt{\frac{p-q}{2}}\right]\\[10pt]
\frac1n e_j \left[\sqrt{\frac{p+q}{2}}, \sqrt{\frac{p-q}{2}}\right]
\end{bmatrix}^{\otimes 2}
+\sum_{(i,j)\in\cA_2}\frac{e^{\frac{q}{n}}}{(1+e^{\frac{q}{n}})^2}
\begin{bmatrix}
\frac1n e_i \left[\sqrt{\frac{p+q}{2}}, -\sqrt{\frac{p-q}{2}}\right]\\[10pt]
\frac1n e_j \left[\sqrt{\frac{p+q}{2}}, \sqrt{\frac{p-q}{2}}\right]
\end{bmatrix}^{\otimes 2}\\
&\quad +\sum_{(i,j)\in\cA_3}\frac{e^{\frac{q}{n}}}{(1+e^{\frac{q}{n}})^2}
\begin{bmatrix}
\frac1n e_i \left[\sqrt{\frac{p+q}{2}}, \sqrt{\frac{p-q}{2}}\right]\\[10pt]
\frac1n e_j \left[\sqrt{\frac{p+q}{2}}, -\sqrt{\frac{p-q}{2}}\right]
\end{bmatrix}^{\otimes 2}
+\sum_{(i,j)\in\cA_4}\frac{e^{\frac{p}{n}}}{(1+e^{\frac{p}{n}})^2}
\begin{bmatrix}
\frac1n e_i \left[\sqrt{\frac{p+q}{2}}, -\sqrt{\frac{p-q}{2}}\right]\\[10pt]
\frac1n e_j \left[\sqrt{\frac{p+q}{2}}, -\sqrt{\frac{p-q}{2}}\right]
\end{bmatrix}^{\otimes 2}.
\end{align*}
In what follows, we view $D^*$ as a $4n\times 4n$ matrix and denote
\begin{align*}
D^*=
\begin{bmatrix}
D_{11}^* & D_{12}^* & D_{13}^* & D_{14}^*\\
D_{21}^* & D_{22}^* & D_{23}^* & D_{24}^*\\
D_{31}^* & D_{32}^* & D_{33}^* & D_{34}^*\\
D_{41}^* & D_{42}^* & D_{43}^* & D_{44}^*
\end{bmatrix},
\end{align*}
where $D_{ij}^*\in\bbR^{n\times n}$.
Recall that we have
\begin{align*}
D^*
\begin{bmatrix}
\Delta_X\\
\Delta_Y
\end{bmatrix}
=
\begin{bmatrix}
X^*\\
Y^*
\end{bmatrix},
\end{align*}
where we view $\Delta_X,\Delta_Y,X^*,Y^*$ as $2n\times 1$ vectors. Thus, we have
\begin{align}\label{eq1:pf_example}
\begin{bmatrix}
D_{11}^* & D_{12}^* \\
D_{21}^* & D_{22}^*    
\end{bmatrix}\Delta_X
+\begin{bmatrix}
D_{13}^* & D_{14}^*\\
D_{23}^* & D_{24}^*\\  
\end{bmatrix}\Delta_Y
=X^*.
\end{align}
Based on the specific form of $X^*$ and $Y^*$, it can be seen that the solutions must have the following form:\textcolor{red}{Why???}
\begin{align}\label{eq2:pf_example}
\Delta_X=\Delta_Y
=\vec 
\begin{bmatrix}
a & b\\
\vdots & \vdots\\
a & b\\
c & d\\
\vdots & \vdots\\
c & d\\
\end{bmatrix}.
\end{align}
The matrix on the RHS has its first $n$ rows being $[a,b]$ and last $n$ rows being $[c,d]$ for some $a,b,c,d$.
By \eqref{eq1:pf_example}, we have
\begin{align}\label{eq4:pf_example}
\begin{bmatrix}
D_{11}^* + D_{13}^* & D_{12}^* + D_{14}^* \\
D_{21}^* + D_{23}^* & D_{22}^* + D_{24}^*  
\end{bmatrix}\Delta_X
=X^*.
\end{align}
With a little abuse of notion, we denote $e_i,e_j\in\bbR^{\frac{n}{2}\times 1}$ the one-hot vector in the following. And we denote $s=\sqrt{\frac{p+q}{2}}, t=\sqrt{\frac{p-q}{2}}$. It then holds that
\begin{align}\label{eq5:pf_example}
&D_{11}^* + D_{13}^*
=\frac{1}{n^2}\sum_{\substack{
        i \neq j \\
        1\leq i, j \leq \frac{n}{2}
    }}\frac{e^{\frac{p}{n}}}{(1+e^{\frac{p}{n}})^2}
\begin{bmatrix}
e_i [s, t]
\end{bmatrix}^{\otimes 2}
+\frac{1}{n^2}\sum_{\substack{
        i \neq j \\
        1\leq i, j \leq \frac{n}{2}
    }}\frac{e^{\frac{p}{n}}}{(1+e^{\frac{p}{n}})^2}
\begin{bmatrix}
e_i [s, t]
\end{bmatrix}^{\otimes}
\begin{bmatrix}
e_j [s, t]
\end{bmatrix}\notag\\
&\qquad\qquad\qquad +
\frac{1}{n^2}\sum_{
        1\leq i, j \leq \frac{n}{2}}\frac{e^{\frac{q}{n}}}{(1+e^{\frac{q}{n}})^2}
\begin{bmatrix}
e_i [s, -t]
\end{bmatrix}^{\otimes 2}\notag\\
&D_{12}^* + D_{14}^*
=
\frac{1}{n^2}\sum_{
        1\leq i, j \leq \frac{n}{2}}\frac{e^{\frac{q}{n}}}{(1+e^{\frac{q}{n}})^2}
\begin{bmatrix}
e_i [s, -t]
\end{bmatrix}^{\otimes}
\begin{bmatrix}
e_j [s, t]
\end{bmatrix}\notag\\
&D_{21}^* + D_{23}^*
=
\frac{1}{n^2}\sum_{
        1\leq i, j \leq \frac{n}{2}}\frac{e^{\frac{q}{n}}}{(1+e^{\frac{q}{n}})^2}
\begin{bmatrix}
e_i [s, t]
\end{bmatrix}^{\otimes}
\begin{bmatrix}
e_j [s, -t]
\end{bmatrix}\notag\\
&D_{22}^* + D_{24}^*
=\frac{1}{n^2}\sum_{\substack{
        i \neq j \\
        1\leq i, j \leq \frac{n}{2}
    }}\frac{e^{\frac{p}{n}}}{(1+e^{\frac{p}{n}})^2}
\begin{bmatrix}
e_i [s, -t]
\end{bmatrix}^{\otimes 2}
+\frac{1}{n^2}\sum_{\substack{
        i \neq j \\
        1\leq i, j \leq \frac{n}{2}
    }}\frac{e^{\frac{p}{n}}}{(1+e^{\frac{p}{n}})^2}
\begin{bmatrix}
e_i [s, -t]
\end{bmatrix}^{\otimes}
\begin{bmatrix}
e_j [s, -t]
\end{bmatrix}\notag\\
&\qquad\qquad\qquad +
\frac{1}{n^2}\sum_{
        1\leq i, j \leq \frac{n}{2}}\frac{e^{\frac{q}{n}}}{(1+e^{\frac{q}{n}})^2}
\begin{bmatrix}
e_i [s, t]
\end{bmatrix}^{\otimes 2}.
\end{align}
Combine \eqref{eq3:pf_example}, \eqref{eq2:pf_example}, \eqref{eq4:pf_example}, \eqref{eq5:pf_example}, we have
\begin{align*}
&\mathbf{1}_{\frac{n}{2}}\cdot[s,t]
=(n-2)\frac{as+bt}{n^2}\frac{e^{\frac{p}{n}}}{(1+e^{\frac{p}{n}})^2}\cdot (\mathbf{1}_{\frac{n}{2}}\cdot[s,t])
+\frac{n}{2}\frac{as-bt}{n^2}\frac{e^{\frac{q}{n}}}{(1+e^{\frac{q}{n}})^2}\cdot (\mathbf{1}_{\frac{n}{2}}\cdot[s,-t])\\
&\qquad\qquad\qquad +\frac{n}{2}\frac{cs+dt}{n^2}\frac{e^{\frac{q}{n}}}{(1+e^{\frac{q}{n}})^2}\cdot (\mathbf{1}_{\frac{n}{2}}\cdot[s,-t])\\
&\mathbf{1}_{\frac{n}{2}}\cdot[s,-t]
=(n-2)\frac{cs-dt}{n^2}\frac{e^{\frac{p}{n}}}{(1+e^{\frac{p}{n}})^2}\cdot (\mathbf{1}_{\frac{n}{2}}\cdot[s,-t])
+\frac{n}{2}\frac{cs+dt}{n^2}\frac{e^{\frac{q}{n}}}{(1+e^{\frac{q}{n}})^2}\cdot (\mathbf{1}_{\frac{n}{2}}\cdot[s,t])\\
&\qquad\qquad\qquad +\frac{n}{2}\frac{as-bt}{n^2}\frac{e^{\frac{q}{n}}}{(1+e^{\frac{q}{n}})^2}\cdot (\mathbf{1}_{\frac{n}{2}}\cdot[s,t]),
\end{align*}
which implies
\begin{align*}
\begin{cases}
as-bt=-(cs+dt)\\
(n-2)\frac{as+bt}{n^2}\frac{e^{\frac{p}{n}}}{(1+e^{\frac{p}{n}})^2}=1\\
(n-2)\frac{cs-dt}{n^2}\frac{e^{\frac{p}{n}}}{(1+e^{\frac{p}{n}})^2}=1
\end{cases}.
\end{align*}
We denote
\begin{align*}
N:=\frac{n^2}{n-2}\frac{(1+e^{\frac{p}{n}})^2}{e^{\frac{p}{n}}}.
\end{align*}
It then holds that
\begin{align*}
a=c=\frac{N}{2s}, \quad b=-d=\frac{N}{2t}
\end{align*}
and 
\begin{align}\label{eq6:pf_example}
\Delta_X
=\begin{bmatrix}
\frac{N}{2s}\mathbf{1} & \frac{N}{2t}\mathbf{1}\\[10pt]
\frac{N}{2s}\mathbf{1} & -\frac{N}{2t}\mathbf{1}
\end{bmatrix}.
\end{align}
Combine with \eqref{eq3:pf_example}, we have
\begin{align*}
\Delta_X Y^{*\top}+X^{*}\Delta^{\top}_Y=\Delta_X X^{*\top}+X^{*}\Delta^{\top}_X
=\begin{bmatrix}
2N\mathbf{1}\mathbf{1}^{\top} & 0\\
0 & 2N\mathbf{1}\mathbf{1}^{\top}
\end{bmatrix}\in\bbR^{n\times n}.
\end{align*}
By the definition of $M^*$, we have
\begin{align*}
M^*=
\begin{bmatrix}
\frac{e^{\frac{p}{n}}}{(1+e^{\frac{p}{n}})^2}\mathbf{1}\mathbf{1}^{\top} & \frac{e^{\frac{q}{n}}}{(1+e^{\frac{q}{n}})^2}\mathbf{1}\mathbf{1}^{\top}\\
\frac{e^{\frac{q}{n}}}{(1+e^{\frac{q}{n}})^2}\mathbf{1}\mathbf{1}^{\top} & \frac{e^{\frac{p}{n}}}{(1+e^{\frac{p}{n}})^2}\mathbf{1}\mathbf{1}^{\top}
\end{bmatrix}
-
\begin{bmatrix}
\frac{e^{\frac{p}{n}}}{(1+e^{\frac{p}{n}})^2} & & \\
 & \ddots & \\
 & & \frac{e^{\frac{p}{n}}}{(1+e^{\frac{p}{n}})^2}
\end{bmatrix}.
\end{align*}
Thus, we have
\begin{align*}
\frac1n M^*\odot \left(\frac1n(\Delta_X Y^{*\top}+X^{*}\Delta^{\top}_Y) \right)
&=\begin{bmatrix}
\frac{2}{n-2}\mathbf{1}\mathbf{1}^{\top} & 0\\
0 & \frac{2}{n-2}\mathbf{1}\mathbf{1}^{\top}
\end{bmatrix}
-
\begin{bmatrix}
\frac{2}{n-2} & & \\
 & \ddots & \\
 & & \frac{2}{n-2}
\end{bmatrix}\\
&=\frac{2}{n-2}
\begin{bmatrix}
\mathbf{1}\mathbf{1}^{\top}-I_{\frac{n}{2}} & 0\\
0 & \mathbf{1}\mathbf{1}^{\top}-I_{\frac{n}{2}} 
\end{bmatrix}.
\end{align*}
Note that
\begin{align*}
  \begin{bmatrix}
\mathbf{1}\mathbf{1}^{\top}-I_{\frac{n}{2}} & 0\\
0 & \mathbf{1}\mathbf{1}^{\top}-I_{\frac{n}{2}} 
\end{bmatrix}  
\end{align*}
has $2$ singular values equal to $\frac{n}{2}-1$ and $n-2$ singular values equal to $1$. And in this example, we have $r=2$. Thus we verify
\begin{align*}
\sigma_{3}\left(\frac1n M^*\odot \left(\frac1n(\Delta_X Y^{*\top}+X^{*}\Delta^{\top}_Y) \right)\right)=\frac{2}{n-2}<\frac12.
\end{align*}
That is to say Assumption \ref{assumption:r+1} holds with $\eps = 1/2$. Thus, we finish the proofs.

























\subsection{Proofs of Theorem \ref{thm:cv_ncv}}\label{pf:thm_cv_ncv}
For notation simplicity, we denote the solution given by gradient descent as $(\theta,H,X,Y)$ instead of $(\hat{\theta},\hat{H},\hat{X},\hat{Y})$. First of all, we have the following claim.
\begin{claim}\label{claim1:pf_cv_ncv}
Let $U\Sigma V^T$ be the SVD of $XY^T$. There exists an invertible matrix $Q\in\bbR^{r\times r}$ such that $X=U\Sigma^{1/2}Q$, $Y=V\Sigma^{1/2}Q^{-T}$ and
\begin{align}\label{ineq1:pf_cv_ncv}
\left\|\Sigma_Q-\Sigma_Q^{-1}\right\|_F\leq\frac{8 \sqrt{\kappa} }{\lambda \sqrt{\sigma_{\min}}} \|\cP(\nabla f(\theta,H,X,Y))\|_F.
\end{align}
Here $U_Q\Sigma_Q V_Q^T$ is the SVD of Q. 
% and $\cP$ is the projection onto the space where $\mathbf{1}^T\nabla_{\theta} f(\theta, H, X, Y)=0$.
\end{claim}
\begin{proof}[Proof of Claim \ref{claim1:pf_cv_ncv}]
Let
\begin{align*}
B_1:=\nabla_{\Gamma}L_c(\theta,H,XY^{\top})Y + \lambda X \quad \text{and} \quad B_2:=\nabla_{\Gamma}L_c(\theta,H,XY^{\top})X + \lambda Y.
\end{align*}
By the definition of $\nabla_X f(\theta,H,X,Y)$ and $\nabla_Y f(\theta,H,X,Y)$, we have
\begin{align*}
    \max\{\|{B}_1\|_F, \|{B}_2\|_F\} 
   & =\max\{\|\nabla_X f(\theta,H,X,Y)\|_F, \|\nabla_Y f(\theta,H,X,Y)\|_F\}\\
&\leq \|\cP(\nabla f(\theta,H,X,Y))\|_F.
\end{align*}
In addition, the definition of $B_1$ and $B_2$ allow us to obtain
\begin{align*}
    \|X^\top X - Y^\top Y\|_F &= \frac{1}{\lambda} \|X^\top ({B}_1 - \nabla_{\Gamma}L_c(\theta,H,XY^{\top}) Y) - ({B}_2 - \nabla_{\Gamma}L_c(\theta,H,XY^{\top})X)^{\top}Y\|_F \\
    &= \frac{1}{\lambda} \|X^\top {B}_1 - {B}_2^\top Y\|_F \\
    &\leq \frac{1}{\lambda} \|X\| \|{B}_1\|_F + \frac{1}{\lambda} \|{B}_2\|_F \|Y\| \\
    &\leq \frac{4}{\lambda} \sqrt{ \sigma_{\max}} \|\cP(\nabla f(\theta,H,X,Y))\|_F.
\end{align*}
Here, the last inequality follows from the fact that $\|X\|, \|Y\| \leq 2\sqrt{\sigma_{\max}}$. In view of Lemma \ref{ar:lem6}, one can find an invertible ${Q}$ such that $X = U \Sigma^{1/2} {Q}$, $Y = V \Sigma^{1/2} {Q}^{-T}$ and
\begin{align*}
    \|\Sigma_{Q} - \Sigma_{Q}^{-1}\|_F &\leq \frac{1}{\sigma_{\min} (\Sigma)} \|X^\top X - Y^\top Y\|_F \\
    &\leq \frac{2}{\sigma_{\min}} \cdot \frac{4}{\lambda} \sqrt{ \sigma_{\max}} \|\cP(\nabla f(\theta,H,X,Y))\|_F\\
    &= \frac{8 \sqrt{\kappa} }{\lambda \sqrt{\sigma_{\min}}} \|\cP(\nabla f(\theta,H,X,Y))\|_F,
\end{align*}
where $\Sigma_Q$ is a diagonal matrix consisting of all singular values of ${Q}$. Here the second inequality follows from 
\begin{align*}
\left|\sigma_{\min}(XY^{\top})-\sigma_{\min}(X^* Y^{*\top})\right|\leq \left\|XY^{\top}-X^* Y^{*\top}\right\|\lesssim \sqrt{\sigma_{\max}}\|X-X^*\|\lesssim c_{14}\sqrt{\sigma_{\max} n},
\end{align*}
which implies $\sigma_{\min}(XY^{\top})\geq \sigma_{\min}/2$ as long as $c_{14}\sqrt{\sigma_{\max} n}\ll \sigma_{\min}$.
This completes the proof.   
\end{proof}

With Claim \ref{claim1:pf_cv_ncv} in hand, we are ready to establish the following claim.
\begin{claim}\label{claim2:pf_cv_ncv}
Suppose that Assumption \ref{assumption:r+1} holds. Under the same notations in Claim \ref{claim1:pf_cv_ncv}, let $\nabla_{\Gamma}L_c(\theta, H, XY^{\top})=-\lambda UV^{\top}+R$.
% \begin{align*}
% \nabla_{\Gamma}L_c(\theta, H, XY^{\top})=-\lambda UV^{\top}+R,
% \end{align*}
Then $R$ satisfies:
\begin{align*}
\|\cP_{\cT}(R)\|_F\leq \frac{ 72 \kappa}{\sqrt{\sigma_{\min}}} \|\cP(\nabla f(\theta,H,X,Y))\|_F\quad\text{and}\quad \|\cP_{\cT^{\perp}}(R)\|<\left(1-\frac{\eps}{4}\right)\lambda
\end{align*}
for $\eps>0$ specified in Assumption \ref{assumption:r+1}. Here $\cT$ is the tangent space for $U\Sigma V^{\top}$ defined as 
\begin{align*}
\cT:=\{UA^{\top}+BV^{\top}\mid A,B\in\bbR^{n\times r}\},
\end{align*}
$\cT^{\perp}$ is the orthogonal complement of $\cT$, and $\cP_{\cT}$, $\cP_{\cT^{\perp}}$ are the orthogonal projection onto the subspace $\cT$, $\cT^{\perp}$, respectively.
\end{claim}
\begin{proof}[Proof of Claim \ref{claim2:pf_cv_ncv}]
Recall the notations in the proof of Claim \ref{claim1:pf_cv_ncv}, we have
\begin{align}\label{eq:B}
B_1=\nabla_{\Gamma}L_c(\theta,H,XY^{\top})Y + \lambda X \quad \text{and} \quad B_2=\nabla_{\Gamma}L_c(\theta,H,XY^{\top})X + \lambda Y.
\end{align}
By the definition of $R$, we have
\begin{align}\label{eq:R}
\nabla_{\Gamma}L_c(\theta, H, XY^{\top})=R-\lambda UV^{\top}.
\end{align}
From the definition of $\mathcal{P}_{\cT}$, we have
\begin{align}\label{eq4:pf_cv_ncv}
    \|\mathcal{P}_{\cT}({R})\|_F &= \|UU^\top {R} (I - VV^\top) + RVV^\top\|_F \notag\\
    &\leq \|U^\top {R} (I - VV^\top)\|_F + \|RVV^\top\|_F \notag\\
    &\leq \|U^\top {R}\|_F + \|RV\|_F.
\end{align}
In addition, by Claim \ref{claim1:pf_cv_ncv}, we have
\begin{align}\label{eq2:pf_cv_ncv}
    X &= U \Sigma^{1/2} {Q} \quad \text{and} \quad Y = V \Sigma^{1/2} {Q}^{-T} 
\end{align}
for some invertible matrix ${Q} \in \mathbb{R}^{r \times r}$, whose SVD $U_Q \Sigma_Q V_Q^\top$ obeys \eqref{ineq1:pf_cv_ncv}. Combine \eqref{eq:B} and \eqref{eq:R}, we have
\begin{align*}
    -\lambda UV^\top Y + RY &= -\lambda X + {B}_1,
\end{align*}
which together with \eqref{eq2:pf_cv_ncv} yields
\begin{align*}
    RV &= \lambda U \Sigma^{1/2} (I_r - {Q} {Q}^\top) \Sigma^{-1/2} + {B}_1 {Q}^\top \Sigma^{-1/2}.
\end{align*}
Apply the triangle inequality to get
\begin{align}\label{eq3:pf_cv_ncv}
    \|RV\|_F &\leq \|\lambda U \Sigma^{1/2} (I_r - {Q} {Q}^\top) \Sigma^{-1/2}\|_F + \|{B}_1 {Q}^\top \Sigma^{-1/2}\|_F \notag\\
    &\leq \lambda \|\Sigma^{1/2}\| \|\Sigma^{-1/2}\| \| {Q} {Q}^\top - I_r \|_F + \|{Q}\| \|\Sigma^{-1/2}\| \|{B}_1\|_F.
\end{align}
In order to further upper bound \eqref{eq3:pf_cv_ncv}, we first recognize the fact that as long as $c_{14}\sqrt{\sigma_{\max} n}\ll \sigma_{\min}$,
\begin{align*}
    \|\Sigma^{1/2}\| &\leq \sqrt{2 \sigma_{\max}}, \quad \text{and} \quad \|\Sigma^{-1/2}\| = 1 / \sqrt{\sigma_{\min} (\Sigma)} \leq \sqrt{2 / \sigma_{\min}},
\end{align*}
which holds since
\begin{align*}
\left|\sigma_{i}(XY^{\top})-\sigma_{i}(X^* Y^{*\top})\right|\leq \left\|XY^{\top}-X^* Y^{*\top}\right\|\lesssim \sqrt{\sigma_{\max}}\|X-X^*\|\lesssim c_{14}\sqrt{\sigma_{\max} n}.
\end{align*}
Second, Claim \ref{claim1:pf_cv_ncv} and \eqref{ncv:grad} yields
\begin{align*}
    \|\Sigma_{Q} - \Sigma_{Q}^{-1}\|_F &\leq \frac{8 \sqrt{\kappa} }{\lambda \sqrt{\sigma_{\min}}} \|\cP(\nabla f(\theta,H,X,Y))\|_F \ll 1 .
\end{align*}
This in turn implies that $\|{Q}\| = \|\Sigma_Q\| \leq 2$. Putting the above bounds together yields
\begin{align*}
    \|RV\|_F &\leq \lambda \sqrt{2 \sigma_{\max}} \sqrt{\frac{2}{\sigma_{\min}}} \|\Sigma_Q^2 - I_r\|_F + 2 \sqrt{\frac{2}{\sigma_{\min}}} \|\cP(\nabla f(\theta,H,X,Y))\|_F \\
    &\leq \lambda \sqrt{2 \sigma_{\max}} \sqrt{\frac{2}{\sigma_{\min}}} \|\Sigma_Q \| \|\Sigma_Q - \Sigma_Q^{-1}\|_F + 2 \sqrt{\frac{2}{\sigma_{\min}}}\|\cP(\nabla f(\theta,H,X,Y))\|_F \\
    &\leq 2 \lambda \sqrt{2 \sigma_{\max}} \sqrt{\frac{2}{\sigma_{\min}}}\frac{8 \sqrt{\kappa} }{\lambda \sqrt{\sigma_{\min}}} \|\cP(\nabla f(\theta,H,X,Y))\|_F + 2 \sqrt{\frac{2}{\sigma_{\min}}} \|\cP(\nabla f(\theta,H,X,Y))\|_F  \\
    &\leq \frac{ 36 \kappa}{\sqrt{\sigma_{\min}}} \|\cP(\nabla f(\theta,H,X,Y))\|_F .
\end{align*}
Similarly, we can show that
\begin{align*}
    \|U^\top {R}\|_F &\leq \frac{ 36 \kappa}{\sqrt{\sigma_{\min}}} \|\cP(\nabla f(\theta,H,X,Y))\|_F.
\end{align*}
These bounds together with \eqref{eq4:pf_cv_ncv} result in
\begin{align}\label{eq6:pf_cv_ncv}
    \|\mathcal{P}_{\cT}({R})\|_F &\leq \frac{ 72 \kappa}{\sqrt{\sigma_{\min}}} \|\cP(\nabla f(\theta,H,X,Y))\|_F.
\end{align}


In the following, we establish the bound for $\|\cP_{\cT^{\perp}}(R)\|$. Note that
\begin{align*}
\nabla_{\Gamma}L_c(\theta,H,XY^{\top})=-\lambda UV^{\top}+R=-\lambda UV^{\top}+\mathcal{P}_{\cT}({R})+\mathcal{P}_{\cT^{\perp}}({R}).
\end{align*}
Suppose for the moment that
\begin{align}\label{eq5:pf_cv_ncv}
  \|\mathcal{P}_{\cT}({R})\|_F \leq\frac{\eps}{4}\lambda \quad\text{and} \quad \sigma_{r+1}\left(\nabla_{\Gamma}L_c(\theta,H,XY^{\top})\right)<\left(1-\frac{\eps}{2}\right)\lambda.
\end{align}
Then, by Weyl's inequality, we have
\begin{align*}
\sigma_{r+1}\left(-\lambda UV^{\top}+\mathcal{P}_{\cT^{\perp}}({R})\right)
&\leq\sigma_{r+1}\left( -\lambda UV^{\top}+\mathcal{P}_{\cT}({R})+\mathcal{P}_{\cT^{\perp}}({R})\right)+\|\mathcal{P}_{\cT}({R})\|_F\\
&=\sigma_{r+1}\left(\nabla_{\Gamma}L_c(\theta,H,XY^{\top})\right)+\|\mathcal{P}_{\cT}({R})\|_F\\
&< \left(1-\frac{\eps}{2}\right)\lambda+\frac{\eps}{4}\lambda\\
&=\left(1-\frac{\eps}{4}\right)\lambda.
\end{align*}
Since $-\lambda UV^T\in\cT$ with $r$ singular values of $\lambda$, we conclude that 
\begin{align*}
\|\cP_{\cT^{\perp}}(R)\|<\left(1-\frac{\eps}{4}\right)\lambda.
\end{align*}
Thus, it remains to verify the two conditions listed in \eqref{eq5:pf_cv_ncv}. For the first condition, by \eqref{eq6:pf_cv_ncv}, we have
\begin{align*}
\|\mathcal{P}_{\cT}({R})\|_F \leq\frac{\eps}{4}\lambda\quad\text{as long as} \quad 
\|\cP(\nabla f(\theta,H,X,Y))\|_F\leq \frac{\eps\lambda}{288\kappa}\sqrt{\sigma_{\min}},
\end{align*}
which is guaranteed by \eqref{ncv:grad}. 
We then verify the second condition in the following. For notation simplicity, we denote
\begin{align*}
\ell_{ij}(x):=\log (1+e^x)-A_{ij}x.
\end{align*}
Then we have
\begin{align*}
&\left(\nabla_{\Gamma} L_c(\theta,H,XY^{\top})-\nabla_{\Gamma} L_c(\theta^{*},H^{*},{\Gamma}^{{*}})\right)_{ij}\\
&=
\begin{cases}
\int^1_{0}\ell''_{ij}\left(P^{*}_{ij}+\tau(P_{ij}-P^{*}_{ij})\right)d\tau\cdot \frac{P_{ij}-P^{*}_{ij}}{n} & i\neq j\\
0 & i=j
\end{cases}.
\end{align*}
We define a matrix $H\in\bbR^{n\times n}$ such that
\begin{align*}
H_{ij}=
\begin{cases}
\int^1_{0}\ell''_{ij}\left(P^{*}_{ij}+\tau(P_{ij}-P^{*}_{ij})\right)d\tau & i\neq j\\
0 & i=j
\end{cases}.
\end{align*}
It then holds that
\begin{align}\label{eq14:pr_cv_ncv}
&\nabla_{\Gamma} L_c(\theta,H,XY^{\top})\notag\\
&=\nabla_{\Gamma} L_c(\theta^{*},H^{*},{\Gamma}^{{*}})+\frac1n H\odot(P-P^*)\notag\\
&=\nabla_{\Gamma} L_c(\theta^{*},H^{*},{\Gamma}^{{*}})+\frac1n (H-M^*)\odot(P-P^*)+\frac1n M^*\odot(P-P^*).
\end{align}
Recall the definition of $M^*$ where 
\begin{align*}
M^{*}_{ij}=
\begin{cases}
    \frac{e^{P_{ij}^*}}{(1+e^{P_{ij}^*})^2} & i\neq j\\
    0 & i=j
\end{cases}
=\begin{cases}
    \ell''_{ij}(P^{*}_{ij}) & i\neq j\\
    0 & i=j
\end{cases}.
\end{align*}
We then have for $i\neq j$:
\begin{align*}
|M^{*}_{ij}-H_{ij}|\leq \int^1_{0}\left|\ell''_{ij}\left(P^{*}_{ij}+\tau(P_{ij}-P^{*}_{ij})\right)- \ell''_{ij}(P^{*}_{ij})\right|d\tau\leq \frac14 |P_{ij}-P^{*}_{ij}|,
\end{align*}
where the last inequality follows from the mean-value theorem and the fact that $|\ell'''_{ij}(x)|\leq \ell''_{ij}(x)\leq 1/4$ for any $x$.
This further implies that
\begin{align*}
&\left\|\frac1n (H-M^*)\odot(P-P^*)\right\|\notag\\
&\leq\left\|\frac1n (H-M^*)\odot(P-P^*)\right\|_F\notag\\
&\leq \frac1n \cdot n\|P-P^{*}\|_{\infty}^2\notag\\
&\leq \left(\frac{2}{\sqrt{n}}\|\theta-\theta^*\|_{\infty}+\frac{\sz}{n}\|H-H^*\|_F+\frac1n \|XY^{\top}-\Gamma^{*}\|_{\infty}\right)^2\\
&\lesssim \left(\frac{1}{\sqrt{n}}\|\theta-\theta^*\|_{\infty}+\frac{\sz}{n}\|H-H^*\|_F+\frac1n\|F^*\|_{2,\infty} \|F-F^*\|_{2,\infty}\right)^2\\
&\lesssim \frac1n \left(c_{41}^2+\sz^2 c_{11}^2+ \mu\sX\sY r^2 c_{43}^2\right),
\end{align*}
where the last inequality follows from \eqref{ncv:est} and Assumption \ref{assumption:incoherent}.
Thus, as long as $n$ large enough, we have
\begin{align}\label{eq12:pf_cv_ncv}
\left\|\frac1n (H-M^*)\odot(P-P^*)\right\|
\lesssim \frac1n \left(c_{41}^2+\sz^2 c_{11}^2+ \mu\sX\sY r^2 c_{43}^2\right)<\frac{\eps\lambda}{10}.
\end{align}
Moreover, as shown in the proofs of Lemma \ref{lem:gradient_norm}, we have
\begin{align}\label{eq13:pf_cv_ncv}
\left\|\nabla_{\Gamma}L_c(\theta^*,H^*,\Gamma^*)\right\|
\lesssim\sqrt{\frac{\log n}{n}}<\frac{\eps\lambda}{10}
\end{align}
as long as $\eps c_{\lambda}\gg 1$.
Thus, it remains to deal with $\frac1n M^*\odot(P-P^*)$.
Note that
\begin{align}\label{eq18:pf_cv_ncv}
\frac1n M^*\odot(P-P^*)=
\underbrace{\frac1n M^*\odot(\hat{P}^d-\bar{P})}_{(1)}
+\underbrace{\frac1n M^*\odot(\bar{P}-P^*)}_{(2)}
+\underbrace{\frac1n M^*\odot(P-\hat{P}^d)}_{(3)}.
\end{align}
In what follows, we will deal with (1),(2) and (3), respectively.
\begin{enumerate}
\item For (1), note that
\begin{align*}
\|(1)\|
&\leq \left\|\frac1n M^*\odot(\hat{P}^d-\bar{P})\right\|_F\\
&\leq \frac{1}{4n}\sqrt{\sum_{i\neq j}(\hat{P}^d_{ij}-\bar{P}_{ij})^2}\\
&\lesssim \frac{\sqrt{\su}}{n}\left(\|\hat{\theta}^d-\bar{\theta}\|_{2}+\|\hat{H}^d-\bar{H}\|_{F}+\frac{1}{n}\|\hat{X}^d\hat{Y}^{d\top}-\bar{X}\bar{Y}^{\top}\|_{F}\right),
\end{align*}
where the last inequality follows the same trick we used before and we omit the details here. By Theorem \ref{thm:ncv_debias}, we obtain
\begin{align}\label{eq14:pf_cv_ncv}
\|(1)\|\lesssim \frac{\sqrt{\su}c_d}{n^{3/4}}<\frac{\eps\lambda}{10}
\end{align}
as long as $n$ is large enough. 

\item 
For (2), note that
\begin{align*}
\|(2)\|
&\leq \left\|\frac1n M^*\odot(\bar{P}-P^*)\right\|_F\\
&\leq \frac{1}{4n}\sqrt{\sum_{i\neq j}(\bar{P}_{ij}-P^*_{ij})^2}\\
&\lesssim \frac{\sqrt{\su}}{n}\left(\|\bar{\theta}-\theta^*\|_{2}+\|\bar{H}-H^*\|_{F}+\frac{1}{n}\|\bar{X}\bar{Y}^{\top}-X^{*}Y^{*\top}\|_{F}\right).
\end{align*}
By Proposition \ref{prop:bar_dist}, we have
\begin{align}\label{eq15:pf_cv_ncv}
\|(2)\|\lesssim c'_a\sqrt{\frac{\su}{n}}<\frac{\eps\lambda}{10}
\end{align}
as long as $\eps c_{\lambda}\gg \sqrt{\su\mu\sX\sY r^2}/\slD$.

\item 
We denote $\hat\Delta$ such that
\begin{align*}
\begin{bmatrix}
\hat{\Delta}_{\theta}\\
\hat{\Delta}_{H}\\
\hat{\Delta}_{X}\\
\hat{\Delta}_{Y}
\end{bmatrix}
=
\begin{bmatrix}
\hat{\theta}^d-\theta\\
\hat{H}^d-H\\
\hat{X}^d-X\\
\hat{Y}^d-Y
\end{bmatrix}.
\end{align*}
With a little abuse of notation, we denote $(\Delta_{\theta}, \Delta_{H}, \Delta_{X}, \Delta_{Y})$ such that
\begin{align*}
\begin{bmatrix}
\Delta_{\theta}\\
\Delta_{H}\\
\Delta_{X}\\
\Delta_{Y}
\end{bmatrix} =-(\cP D^*\cP)^{\dagger}\begin{bmatrix}
0\\
0\\
-\lambda X^{*}\\
-\lambda Y^{*}
\end{bmatrix},
\end{align*}
% \begin{align*}
% \begin{cases}
% \begin{bmatrix}
% 0\\
% 0\\
% -\lambda X^{*}\\
% -\lambda Y^{*}
% \end{bmatrix}
% +\cP D^*\cP
%  \begin{bmatrix}
% \Delta_{\theta}\\
% \Delta_{H}\\
% \Delta_{X}\\
% \Delta_{Y}
% \end{bmatrix}
% =0\\
% \cP_{\theta}(\Delta_{\theta})=\Delta_{\theta}
% \end{cases}.
% \end{align*}
Then by Assumption \ref{assumption:r+1}, we have
\begin{align*}
    \sigma_{r+1}\left(\frac{1}{n}{M}^* \odot \left(\frac{(\Delta_{\theta})_i+(\Delta_{\theta})_j}{\sqrt{n}}+{z}_i^T\Delta_{H}{z}_j+\frac{(\Delta_{X}{Y}^{*T}+{X}^*{\Delta^T_{Y}})_{ij}}{n}\right)_{ij}\right) <(1-\epsilon)\lambda
\end{align*}
for some $\eps>0$.
We further have the following claim.
\begin{claim}\label{claim1:delta_diff}
It holds that
\begin{align*}
 \left\|\begin{bmatrix}
\hat{\Delta}_{\theta}-{\Delta}_{\theta}\\
\hat{\Delta}_{H}-{\Delta}_{H}\\
\hat{\Delta}_{X}-{\Delta}_{X}\\
\hat{\Delta}_{Y}-{\Delta}_{Y}
\end{bmatrix}
\right\|_F   \leq c_{\text{diff}},
\end{align*}
where 
\begin{align}
c_{\text{diff}}\asymp \frac{\hat{c}\sqrt{\mu\sX\sY r^2 }+c_{11}\slD}{\slD^2} c_{\lambda}\sqrt{\log n}.
\end{align}
\end{claim}
\begin{proof}[Proof of Claim \ref{claim1:delta_diff}]
By the definition of $(\Delta_{\theta}, \Delta_{H}, \Delta_{X}, \Delta_{Y})$, we have
\begin{align*}
\begin{bmatrix}
\Delta_{\theta}\\
\Delta_{H}\\
\Delta_{X}\\
\Delta_{Y}
\end{bmatrix} =-(\cP D^*\cP)^{\dagger}\begin{bmatrix}
0\\
0\\
-\lambda X^{*}\\
-\lambda Y^{*}
\end{bmatrix},
\end{align*}
where $(\cP D^*\cP)^{\dagger}$ represents the pseudo-inverse of $\cP D^*\cP$.
By the definition of the debiased estimator, we have
\begin{align*}
\begin{bmatrix}
\hat{\Delta}_{\theta}\\
\hat{\Delta}_{H}\\
\hat{\Delta}_{X}\\
\hat{\Delta}_{Y}
\end{bmatrix} 
=-(\cP\hat{D}\cP)^{\dagger}\left(\cP\nabla L(\hat{\theta},\hat{H},\hat{X},\hat{Y})\right),
\end{align*}
where $(\cP \hat{D}\cP)^{\dagger}$ represents the pseudo-inverse of $\cP \hat{D}\cP$.
For notation simplicity, we denote
\begin{align*}
& A_1:=(\cP D^*\cP)^{\dagger},\ 
b_1:=\begin{bmatrix}
0\\
0\\
-\lambda X^{*}\\
-\lambda Y^{*}
\end{bmatrix}\\
\text{and }
& A_2:=(\cP\hat{D}\cP)^{\dagger},\ 
b_2:=\cP\nabla L(\hat{\theta},\hat{H},\hat{X},\hat{Y}).
\end{align*}
It then holds that
\begin{align}\label{eq8:delta_diff}
\left\|\begin{bmatrix}
\hat{\Delta}_{\theta}-{\Delta}_{\theta}\\
\hat{\Delta}_{H}-{\Delta}_{H}\\
\hat{\Delta}_{X}-{\Delta}_{X}\\
\hat{\Delta}_{Y}-{\Delta}_{Y}
\end{bmatrix}
\right\|_F
&=\|A_1b_1-A_2b_2\|_2\notag\\
&\leq \|A_1-A_2\|\|b_2\|_2+\|A_1\|\|b_1-b_2\|_2.
\end{align}
In the following, we control $ \|A_1-A_2\|$, $\|b_1-b_2\|_2$, $\|A_1\|$, and $\|b_2\|_2$, respectively.
\begin{enumerate}
    
\item For $ \|A_1-A_2\|$, by Theorem 3.3 in \cite{stewart1977perturbation}, we have
\begin{align}\label{eq4:delta_diff}
\|A_1-A_2\|
&\leq \frac{1+\sqrt{5}}{2}\max\{\|(\cP\hat{D}\cP)^{\dagger}\|^2, \|(\cP D^*\cP)^{\dagger}\|^2\}\cdot \|\cP\hat{D}\cP-\cP D^*\cP\|.
\end{align}
By Lemma \ref{lem:D}, we have
\begin{align*}
\max\{\|(\cP\hat{D}\cP)^{\dagger}\|^2, \|(\cP D^*\cP)^{\dagger}\|^2\}\lesssim \frac{1}{\slD^2}, \quad
\|\cP\hat{D}\cP-\cP D^*\cP\|\lesssim  \frac{\hat{c}}{\sqrt{n}}.
\end{align*}
Finally, by \eqref{eq4:delta_diff}, we obtain
\begin{align}\label{eqA:delta_diff}
\|A_1-A_2\|\lesssim \frac{\hat{c}}{\slD^2\sqrt{n}}.
\end{align}

\item For $\|b_1-b_2\|_2$, we have
\begin{align}\label{eq5:delta_diff}
\|b_1-b_2\|_2
&=\left\|\begin{bmatrix}
0\\
0\\
-\lambda X^{*}\\
-\lambda Y^{*}
\end{bmatrix}-\cP\nabla L(\hat{\theta},\hat{H},\hat{X},\hat{Y})\right\|_2\notag\\
&\leq \left\|\begin{bmatrix}
0\\
0\\
\lambda X^{*}\\
\lambda Y^{*}
\end{bmatrix}-
\begin{bmatrix}
0\\
0\\
\lambda \hat{X}\\
\lambda \hat{Y}
\end{bmatrix}\right\|_2
+\left\|\cP\nabla L(\hat{\theta},\hat{H},\hat{X},\hat{Y})-\begin{bmatrix}
0\\
0\\
-\lambda \hat{X}\\
-\lambda \hat{Y}
\end{bmatrix}\right\|_2
\end{align}
For the first term, we have
\begin{align}\label{eq6:delta_diff}
 \left\|\begin{bmatrix}
0\\
0\\
\lambda X^{*}\\
\lambda Y^{*}
\end{bmatrix}-
\begin{bmatrix}
0\\
0\\
\lambda \hat{X}\\
\lambda \hat{Y}
\end{bmatrix}\right\|_2
\leq \lambda (\|X^*-\hat{X}\|_F+(\|Y^*-\hat{Y}\|_F)\leq 2 \lambda c_{11}\sqrt{n},
\end{align}
where the last inequality follows from Lemma \ref{lem:ncv1}.
For the second term, follow the same argument as in Appendix \ref{pf:prop_debias_dist}, we have
\begin{align}\label{eq7:delta_diff}
\left\|\cP\nabla L(\hat{\theta},\hat{H},\hat{X},\hat{Y})-\begin{bmatrix}
0\\
0\\
-\lambda \hat{X}\\
-\lambda \hat{Y}
\end{bmatrix}\right\|_2   \lesssim n^{-5}.
\end{align}
Combine \eqref{eq5:delta_diff}, \eqref{eq6:delta_diff} and \eqref{eq7:delta_diff}, we have
\begin{align*}
\|b_1-b_2\|_2\lesssim \lambda c_{11}\sqrt{n}.
\end{align*}

\item For $\|A_1\|$, by Lemma \ref{lem:D}, we have $\|A_1\|\leq 1/\slD$.


\item For $\|b_2\|_2$, we have
\begin{align*}
\|b_2\|_2
&\leq \|b_1-b_2\|_2+\|b_1\|_2\\
&\leq \|b_1-b_2\|_2+\lambda(\|X^*\|_F+\|Y^*\|_F)\\
&\lesssim \lambda \sqrt{\mu r\sigma_{\max}}
\end{align*}
as long as $ \sqrt{\mu r\sigma_{\max}}\gg c_{11}\sqrt{n}$.




\end{enumerate}

Combine the above results with \eqref{eq8:delta_diff}, we have
\begin{align*}
\left\|\begin{bmatrix}
\hat{\Delta}_{\theta}-{\Delta}_{\theta}\\
\hat{\Delta}_{H}-{\Delta}_{H}\\
\hat{\Delta}_{X}-{\Delta}_{X}\\
\hat{\Delta}_{Y}-{\Delta}_{Y}
\end{bmatrix}
\right\|_2 
&\lesssim \frac{\hat{c}}{\slD^2\sqrt{n}}\cdot \lambda \sqrt{\mu r\sigma_{\max}}+\frac{1}{\slD}\cdot\lambda c_{11}\sqrt{n}\\
&\leq \frac{\hat{c}}{\slD^2}\cdot \lambda \sqrt{\mu\sX\sY r^2 n}+\frac{1}{\slD}\cdot\lambda c_{11}\sqrt{n}\\
&=\frac{\hat{c}\sqrt{\mu\sX\sY r^2 }+c_{11}\slD}{\slD^2} c_{\lambda}\sqrt{\log n}.
\end{align*}
We then finish the proofs.

\end{proof}








By Weyl's inequality, we have
\begin{align*}
&\sigma_{r+1}\left(\frac{1}{n}{M}^* \odot \left((\hat{P}^d-P)-\frac1n(\hat{X}^d-X)(\hat{Y}^d-Y)^{\top}\right)\right)\\
&=\sigma_{r+1}\left(\frac{1}{n}{M}^* \odot \left(\frac{(\hat{\Delta}_{\theta})_i+(\hat{\Delta}_{\theta})_j}{\sqrt{n}}+{z}_i^T\hat{\Delta}_{H}{z}_j+\frac{(\hat{\Delta}_{X}{Y}^{T}+{X}{\hat{\Delta}^T_{Y}})_{ij}}{n}\right)_{ij}\right)\\
&\leq \sigma_{r+1}\left(\frac{1}{n}{M}^* \odot \left(\frac{(\Delta_{\theta})_i+(\Delta_{\theta})_j}{\sqrt{n}}+{z}_i^T\Delta_{H}{z}_j+\frac{(\Delta_{X}{Y}^{*T}+{X}^*{\Delta^T_{Y}})_{ij}}{n}\right)_{ij}\right)\\
&\quad +\frac1n \left\|{M}^* \odot\left(\frac{(\hat{\Delta}_{\theta}-{\Delta}_{\theta})_i+(\hat{\Delta}_{\theta}-{\Delta}_{\theta})_j}{\sqrt{n}}\right)_{ij} \right\|_F+\frac1n \left\|{M}^* \odot\left({z}_i^T(\hat{\Delta}_{H}-{\Delta}_{H}){z}_j\right)_{ij} \right\|_F\\
&\quad + \frac{1}{n^2} \left\|{M}^* \odot \left((\hat{\Delta}_{X}{Y}^{T}+{X}{\hat{\Delta}^T_{Y}})-(\Delta_{X}{Y}^{*T}+{X}^*{\Delta^T_{Y}})\right) \right\|_F\\
&\leq \sigma_{r+1}\left(\frac{1}{n}{M}^* \odot \left(\frac{(\Delta_{\theta})_i+(\Delta_{\theta})_j}{\sqrt{n}}+{z}_i^T\Delta_{H}{z}_j+\frac{(\Delta_{X}{Y}^{*T}+{X}^*{\Delta^T_{Y}})_{ij}}{n}\right)_{ij}\right)\\
&\quad +\frac{1}{4n} \left\|\left(\frac{(\hat{\Delta}_{\theta}-{\Delta}_{\theta})_i+(\hat{\Delta}_{\theta}-{\Delta}_{\theta})_j}{\sqrt{n}}\right)_{ij} \right\|_F+\frac{1}{4n}\left\|\left({z}_i^T(\hat{\Delta}_{H}-{\Delta}_{H}){z}_j\right)_{ij} \right\|_F\\
&\quad + \frac{1}{4n^2} \left\|(\hat{\Delta}_{X}{Y}^{T}+{X}{\hat{\Delta}^T_{Y}})-(\Delta_{X}{Y}^{*T}+{X}^*{\Delta^T_{Y}})\right\|_F.
\end{align*}
By Claim \ref{claim1:delta_diff}, we can bound the Frobenius norms on the RHS respectively.
\begin{enumerate}
    \item For the first Frobenius norm, we have
    \begin{align*}
      \left\|\left(\frac{(\hat{\Delta}_{\theta}-{\Delta}_{\theta})_i+(\hat{\Delta}_{\theta}-{\Delta}_{\theta})_j}{\sqrt{n}}\right)_{ij} \right\|_F  \leq 2 \|\hat{\Delta}_{\theta}-{\Delta}_{\theta}\|_2\lesssim c_{\text{diff}}.
    \end{align*}


    
      \item For the second Frobenius norm, we have
      \begin{align*}
      \left\|\left({z}_i^T(\hat{\Delta}_{H}-{\Delta}_{H}){z}_j\right)_{ij} \right\|_F
      &=\sqrt{\sum_{i,j}\left({z}_i^T(\hat{\Delta}_{H}-{\Delta}_{H}){z}_j\right)^2}    \\
      &\leq \|\hat{\Delta}_{H}-{\Delta}_{H}\|\sqrt{\sum_{i,j}\|z_i\|_2^2\|z_j\|_2^2} \\
      &\leq \sz \|\hat{\Delta}_{H}-{\Delta}_{H}\| \\
      &\leq \sz c_{\text{diff}}.
      \end{align*}


      \item For the third Frobenius norm, we have
      \begin{align*}
        &\left\|(\hat{\Delta}_{X}{Y}^{T}+{X}{\hat{\Delta}^T_{Y}})-(\Delta_{X}{Y}^{*T}+{X}^*{\Delta^T_{Y}})\right\|_F\\
        &\leq \|\hat{\Delta}_{X}{Y}^{T}-\Delta_{X}{Y}^{*T}\|_F
        + \|{X}{\hat{\Delta}^T_{Y}}-{X}^*{\Delta^T_{Y}}\|_F\\
        &\leq \|\hat{\Delta}_{X}\|_F \|Y-Y^*\|_F+ \|Y^*\|_F \|\hat{\Delta}_{X}-{\Delta}_{X}\|_F+\|\hat{\Delta}_{Y}\|_F \|X-X^*\|_F+ \|X^*\|_F \|\hat{\Delta}_{Y}-{\Delta}_{Y}\|_F\\
        &\lesssim c_a c_{11} n+\sqrt{\mu r \sigma_{\max}}c_{\text{diff}}\\
        &\lesssim ( c_a c_{11}+\sqrt{\mu\sX\sY r^2}c_{\text{diff}})n,
      \end{align*}
where the last inequality follows from Lemma \ref{lem:ncv1}, Proposition \ref{prop:debias_dist}, Claim \ref{claim1:delta_diff}, and Assumption \ref{assumption:incoherent}.


\end{enumerate}

Combine the above bounds, we have
\begin{align*}
&\sigma_{r+1}\left(\frac{1}{n}{M}^* \odot \left((\hat{P}^d-P)-\frac1n(\hat{X}^d-X)(\hat{Y}^d-Y)^{\top}\right)\right)\\
&\leq \sigma_{r+1}\left(\frac{1}{n}{M}^* \odot \left(\frac{(\Delta_{\theta})_i+(\Delta_{\theta})_j}{\sqrt{n}}+{z}_i^T\Delta_{H}{z}_j+\frac{(\Delta_{X}{Y}^{*T}+{X}^*{\Delta^T_{Y}})_{ij}}{n}\right)_{ij}\right)\\
&\quad+\frac{c}{n}( c_a c_{11}+\sqrt{\mu\sX\sY r^2}c_{\text{diff}})\\
&< (1-\eps)\lambda +\frac{\eps\lambda}{20}\\
&=\left(1-\frac{19\eps}{20}\right)\lambda
\end{align*}
as long as $ c_a c_{11}+\sqrt{\mu\sX\sY r^2}c_{\text{diff}}\ll \eps\lambda n$ ($n$ is large enough).
By Weyl's inequality, we have
\begin{align}
&\sigma_{r+1}\left(\frac{1}{n}{M}^* \odot (\hat{P}^d-P)\right)\notag\\
&\leq \sigma_{r+1}\left(\frac{1}{n}{M}^* \odot \left((\hat{P}^d-P)-\frac1n(\hat{X}^d-X)(\hat{Y}^d-Y)^{\top}\right)\right)+\frac{1}{n^2}\left\|{M}^* \odot(\hat{X}^d-X)(\hat{Y}^d-Y)^{\top}\right\|_F\notag\\
&\leq \sigma_{r+1}\left(\frac{1}{n}{M}^* \odot \left((\hat{P}^d-P)-\frac1n(\hat{X}^d-X)(\hat{Y}^d-Y)^{\top}\right)\right)+\frac{1}{4n^2}\|\hat{X}^d-X\|_F\|\hat{Y}^d-Y\|_F\notag\\
&\leq \sigma_{r+1}\left(\frac{1}{n}{M}^* \odot \left((\hat{P}^d-P)-\frac1n(\hat{X}^d-X)(\hat{Y}^d-Y)^{\top}\right)\right)+\frac{c_a^2}{4n}\tag{by Proposition \ref{prop:debias_dist}}\\
&<\left(1-\frac{19\eps}{20}\right)\lambda+\frac{\eps\lambda}{20}\notag\\\label{eq16:pf_cv_ncv}
&=\left(1-\frac{9\eps}{10}\right)\lambda
\end{align}
as long as $c_a^2\ll \eps\lambda n$ ($n$ is large enough).
\end{enumerate}

Combine \eqref{eq18:pf_cv_ncv}, \eqref{eq14:pf_cv_ncv}, \eqref{eq15:pf_cv_ncv}, \eqref{eq16:pf_cv_ncv} and apply Weyl's inequality, we have
\begin{align}\label{eq19:pf_cv_ncv}
\sigma_{r+1}\left(\frac{1}{n}{M}^* \odot (P-P^*)\right)
&\leq \sigma_{r+1}\left(\frac{1}{n}{M}^* \odot (P-\hat{P}^d)\right)+\|(1)\|+\|(2)\|\notag\\    
&<\left(1-\frac{9\eps}{10}\right)\lambda+\frac{\eps\lambda}{10}+\frac{\eps\lambda}{10}\notag\\
&=\left(1-\frac{7\eps}{10}\right)\lambda.
\end{align}

Finally, combine \eqref{eq14:pr_cv_ncv}, \eqref{eq12:pf_cv_ncv}, \eqref{eq13:pf_cv_ncv}, \eqref{eq19:pf_cv_ncv} and apply Weyl's inequality, we have
\begin{align*}
&\sigma_{r+1}\left(\nabla_{\Gamma} L_c(\theta,H,XY^{\top})\right)\notag\\
&\leq \sigma_{r+1}\left(\frac{1}{n}{M}^* \odot (P-P^*)\right)+\left\|\frac1n (H-M^*)\odot(P-P^*)\right\|+\left\|\nabla_{\Gamma}L_c(\theta^*,H^*,\Gamma^*)\right\|\notag\\
&<\left(1-\frac{7\eps}{10}\right)\lambda+\frac{\eps\lambda}{10}+\frac{\eps\lambda}{10}\notag\\
&=\left(1-\frac{\eps}{2}\right)\lambda.
\end{align*}
Thus, we finish the proof of Claim \ref{claim2:pf_cv_ncv}.



\end{proof}

The following claim shows that $\|\hat{\theta}_c-\theta^*\|_{\infty}$, $\|\hat{H}_c-H^*\|_F$, $\|\hat{\Gamma}_c-\Gamma^*\|_{\infty}$ is bounded even though the convex optimization problem is not constrained to do so.
\begin{claim}\label{claim:MLE_bound}
We have
\begin{align*}
\|\hat{\theta}_c-\theta^*\|_{\infty}\leq c_P \sqrt{n}, \ 
\|\hat{H}_c-H^*\|_{F}\leq c_P n, \ \|\hat{\Gamma}_c-\Gamma^*\|_{\infty}\leq c_P n.
\end{align*}
\end{claim}
\begin{proof}[Proof of Claim \ref{claim:MLE_bound}]
In the following, we fix a constant $c=c_P$. We define a constraint convex optimization problem as
\begin{align}\label{obj:con}
(\hat{\theta}^{con}, \hat{H}^{con}, \hat{\Gamma}^{con}) 
:=\argmin_{\substack{\mathbf{1}^{\top}\theta=0,\|{\theta}-\theta^*\|_{\infty}\leq c\sqrt{n},\\
\|{H}-H^*\|_{F}\leq c n, \ \|{\Gamma}-\Gamma^*\|_{\infty}\leq c n}} f_c(\theta,H,\Gamma),
\end{align}
where $f_c$ is the convex objective defined in \eqref{obj:cv}.
By \eqref{ncv:est}, $(\theta,H, \Gamma)$ is feasible for the constraint of \eqref{obj:con}. We then have
\begin{align}\label{eq7:MLE_bound}
L_c(\hat{\theta}^{con}, \hat{H}^{con}, \hat{\Gamma}^{con}) +\lambda\|\hat{\Gamma}^{con}\|_{*}\leq L_c({\theta}, {H}, {\Gamma})+\lambda\|\Gamma\|_{*}.
\end{align}
We denote 
\begin{align*}
\Delta_{\theta}^{con}:=\hat{\theta}^{con}-\theta,\ 
\Delta_{H}^{con}:=\hat{H}^{con}-H,\ 
\Delta_{\Gamma}^{con}:=\hat{\Gamma}^{con}-\Gamma.
\end{align*}
By Taylor expansion, we have
\begin{align}\label{eq30:MLE_bound}
&L_c(\hat{\theta}^{con}, \hat{H}^{con}, \hat{\Gamma}^{con}) -L_c({\theta}, {H}, {\Gamma})\notag\\
&=\nabla L_c({\theta}, {H}, {\Gamma})^{\top}
\begin{bmatrix}
\Delta_{\theta}^{con}\\
\Delta_{H}^{con}\\
\Delta_{\Gamma}^{con}
\end{bmatrix}
+\frac12 
\begin{bmatrix}
\Delta_{\theta}^{con}\\
\Delta_{H}^{con}\\
\Delta_{\Gamma}^{con}
\end{bmatrix}^{\top}
\nabla^2 L_c(\tilde{\theta}, \tilde{H}, \tilde{\Gamma})
\begin{bmatrix}
\Delta_{\theta}^{con}\\
\Delta_{H}^{con}\\
\Delta_{\Gamma}^{con}
\end{bmatrix}\notag\\
&=\nabla L_c({\theta}, {H}, {\Gamma})^{\top}
\begin{bmatrix}
\Delta_{\theta}^{con}\\
\Delta_{H}^{con}\\
\Delta_{\Gamma}^{con}
\end{bmatrix}
+\frac12 
\begin{bmatrix}
\Delta_{\theta}^{con}\\
\Delta_{H}^{con}\\
\Delta_{\Gamma}^{con}
\end{bmatrix}^{\top}
\left(\sum_{i\neq j}\frac{e^{ \tilde{P}_{ij}}}{(1+e^{ \tilde{P}_{ij}})^2} 
\begin{bmatrix}
\frac{{e}_i+{e}_j}{\sqrt{n}}\\
{z}_i{z}_j^T\\
\frac{{e}_i{e}_j^T}{n}
\end{bmatrix}^{\otimes 2}\right)
\begin{bmatrix}
\Delta_{\theta}^{con}\\
\Delta_{H}^{con}\\
\Delta_{\Gamma}^{con}
\end{bmatrix}.
\end{align}
Note that for some constant $c'$
\begin{align}\label{ineq30:MLE_bound}
 &\begin{bmatrix}
\Delta_{\theta}^{con}\\
\Delta_{H}^{con}\\
\Delta_{\Gamma}^{con}
\end{bmatrix}^{\top}
\left(\sum_{i\neq j}\frac{e^{ \tilde{P}_{ij}}}{(1+e^{ \tilde{P}_{ij}})^2} 
\begin{bmatrix}
\frac{{e}_i+{e}_j}{\sqrt{n}}\\
{z}_i{z}_j^T\\
\frac{{e}_i{e}_j^T}{n}
\end{bmatrix}^{\otimes 2}\right)
\begin{bmatrix}
\Delta_{\theta}^{con}\\
\Delta_{H}^{con}\\
\Delta_{\Gamma}^{con}
\end{bmatrix}\notag\\
&\geq_{(1)}  \frac{e^{c' c_P}}{(1+e^{c' c_P})^2}
\begin{bmatrix}
\Delta_{\theta}^{con}\\
\Delta_{H}^{con}\\
\Delta_{\Gamma}^{con}
\end{bmatrix}^{\top}
\left(\sum_{i\neq j}
\begin{bmatrix}
\frac{{e}_i+{e}_j}{\sqrt{n}}\\
{z}_i{z}_j^T\\
\frac{{e}_i{e}_j^T}{n}
\end{bmatrix}^{\otimes 2}\right)
\begin{bmatrix}
\Delta_{\theta}^{con}\\
\Delta_{H}^{con}\\
\Delta_{\Gamma}^{con}
\end{bmatrix}\notag\\
&=\frac{e^{c' c_P}}{(1+e^{c' c_P})^2}\begin{bmatrix}
\Delta_{\theta}^{con}\\
\Delta_{H}^{con}\\
\frac1n \Delta_{\Gamma}^{con}
\end{bmatrix}^{\top}
\left(\sum_{i\neq j}
\begin{bmatrix}
\frac{{e}_i+{e}_j}{\sqrt{n}}\\
{z}_i{z}_j^T\\
{{e}_i{e}_j^T}
\end{bmatrix}^{\otimes 2}\right)
\begin{bmatrix}
\Delta_{\theta}^{con}\\
\Delta_{H}^{con}\\
\frac1n \Delta_{\Gamma}^{con}
\end{bmatrix}\notag\\
&\geq \frac{\sl e^{c' c_P}}{(1+e^{c' c_P})^2} \left(\|\Delta_{\theta}^{con}\|_2^2+\|\Delta_{H}^{con}\|_F^2+\frac{1}{n^2}\|\Delta_{\Gamma}^{con}\|_F^2\right),
\end{align}
where the last inequality follows from Assumption \ref{assumption:eigenvalues}.
Here (1) follows from the following argument: note that
\begin{align*}
|P_{ij}|
&:=\left|\frac{\theta_i+\theta_j}{\sqrt{n}}+{z}_i^\top{H}{z}_j + \frac{(XY^{\top})_{ij}}{n}\right|\\
&\leq |P_{ij}^{*}|+\frac{2}{\sqrt{n}}\|\theta-\theta^*\|_{\infty}+\frac{\sz}{n}\|H-H^*\|_2+\frac{1}{n}\|XY^{\top}-\Gamma^*\|_{\infty}.
\end{align*}
Further, by \eqref{ncv:est}, we have
\begin{align*}
&\|XY^T-\Gamma^*\|_{\infty}\\
&=\|(X-X^*)Y^T+X^{*}(Y-Y^*)^T\|_{\infty}\\
&\leq \|X-X^*\|_{2,\infty}\|Y\|_{2,\infty}+\|X^{*}\|_{2,\infty}\|Y-Y^*\|_{2,\infty} \tag{Cauchy}\\
&\lesssim c_{43}\sqrt{\mu \sX\sY r^2 n}.
\end{align*}
Thus, by \eqref{ncv:est} and Assumption \ref{assumption:scales}, we have $|P_{ij}|\leq 2c_P$.
Similarly, we have
\begin{align*}
|(\hat{P}^{con})_{ij}|
&:=\left|\frac{(\hat{\theta}^{con})_i+(\hat{\theta}^{con})_j}{\sqrt{n}}+{z}_i^\top{\hat{H}^{con}}{z}_j + \frac{(\hat{\Gamma}^{con})_{ij}}{n}\right|\\
&\leq |P_{ij}^{*}|+\frac{2}{\sqrt{n}}\|\hat{\theta}^{con}-\theta^*\|_{\infty}+\frac{\sz}{n}\|\hat{H}^{con}-H^*\|_2+\frac{1}{n}\|\hat{\Gamma}^{con}-\Gamma^*\|_{\infty}\\
&\leq |P_{ij}^{*}|+\frac{2}{\sqrt{n}}\|\hat{\theta}^{con}-\theta^*\|_{\infty}+\frac{\sz}{n}\|\hat{H}^{con}-H^*\|_F+\frac{1}{n}\|\hat{\Gamma}^{con}-\Gamma^*\|_{\infty}.
\end{align*}
Further, by the constraints, we have $|(\hat{P}^{con})_{ij}|\lesssim c_P$. Since $\tilde{P}_{ij}$ lies between $P_{ij}$ and $(\hat{P}^{con})_{ij}$, we conclude that $|\tilde{P}_{ij}|\lesssim c_P$. Consequently, we have $\frac{e^{ \tilde{P}_{ij}}}{(1+e^{ \tilde{P}_{ij}})^2} \geq \frac{e^{c' c_P}}{(1+e^{c' c_P})^2}$ for some constant $c'$, which implies (1).

Combine \eqref{eq30:MLE_bound} and \eqref{ineq30:MLE_bound}, we have
\begin{align}\label{eq8:MLE_bound}
L_c(\hat{\theta}^{con}, \hat{H}^{con}, \hat{\Gamma}^{con}) -L_c({\theta}, {H}, {\Gamma})
\geq \nabla L_c({\theta}, {H}, {\Gamma})^{\top}
\begin{bmatrix}
\Delta_{\theta}^{con}\\
\Delta_{H}^{con}\\
\Delta_{\Gamma}^{con}
\end{bmatrix}
+C\left(\|\Delta_{\theta}^{con}\|_2^2+\|\Delta_{H}^{con}\|_F^2+\frac{1}{n^2}\|\Delta_{\Gamma}^{con}\|_F^2\right)
\end{align}
for $C:=\frac{\sl e^{c' c_P}}{2(1+e^{c' c_P})^2} $. By \eqref{eq7:MLE_bound} and \eqref{eq8:MLE_bound}, we obtain
\begin{align}\label{eq9:MLE_bound}
 C\left(\|\Delta_{\theta}^{con}\|_2^2+\|\Delta_{H}^{con}\|_F^2+\frac{1}{n^2}\|\Delta_{\Gamma}^{con}\|_F^2\right)
 \leq -\nabla L_c({\theta}, {H}, {\Gamma})^{\top}
\begin{bmatrix}
\Delta_{\theta}^{con}\\
\Delta_{H}^{con}\\
\Delta_{\Gamma}^{con}
\end{bmatrix}+\lambda\|\Gamma\|_{*}-\lambda\|\hat{\Gamma}^{con}\|_{*}.
\end{align}
In addition, by the convexity of $\|\cdot\|_{*}$, we have
\begin{align*}
\|\hat{\Gamma}^{con}\|_{*}-\|\Gamma\|_{*}=\|\Gamma+\Delta_{\Gamma}^{con}\|_{*}-\|\Gamma\|_{*}\geq \langle UV^{\top}+W,\Delta_{\Gamma}^{con}\rangle
\end{align*}
for any $W\in\cT^{\perp}$ obeying $\|W\|\leq 1$. In the following, we pick $W$ such that $\langle W, \Delta_{\Gamma}^{con}\rangle=\|\cP_{\cT^{\perp}}(\Delta_{\Gamma}^{con})\|_{*}$. We then obtain $\|\hat{\Gamma}^{con}\|_{*}-\|\Gamma\|_{*}\geq  \langle UV^{\top},\Delta_{\Gamma}^{con}\rangle+\|\cP_{\cT^{\perp}}(\Delta_{\Gamma}^{con})\|_{*}$, and consequently, by \eqref{eq9:MLE_bound}, we have
\begin{align*}
C\left(\|\Delta_{\theta}^{con}\|_2^2+\|\Delta_{H}^{con}\|_F^2+\frac{1}{n^2}\|\Delta_{\Gamma}^{con}\|_F^2\right)
 \leq -\nabla L_c({\theta}, {H}, {\Gamma})^{\top}
\begin{bmatrix}
\Delta_{\theta}^{con}\\
\Delta_{H}^{con}\\
\Delta_{\Gamma}^{con}
\end{bmatrix}-\lambda\langle UV^{\top},\Delta_{\Gamma}^{con}\rangle-\lambda\|\cP_{\cT^{\perp}}(\Delta_{\Gamma}^{con})\|_{*}.
\end{align*}
Recall the definition of $R$ in \eqref{eq:R}, we further have
\begin{align}\label{eq10:MLE_bound}
&C\left(\|\Delta_{\theta}^{con}\|_2^2+\|\Delta_{H}^{con}\|_F^2+\frac{1}{n^2}\|\Delta_{\Gamma}^{con}\|_F^2\right)\notag\\
& \leq  -\nabla_{\theta} L_c({\theta}, {H}, {\Gamma})^{\top} \Delta_{\theta}^{con} -\nabla_{H} L_c({\theta}, {H}, {\Gamma})^{\top} \Delta_{H}^{con}-\langle R,\Delta_{\Gamma}^{con}\rangle-\lambda\|\cP_{\cT^{\perp}}(\Delta_{\Gamma}^{con})\|_{*}\notag\\
&=  -\nabla_{\theta} L_c({\theta}, {H}, {\Gamma})^{\top} \Delta_{\theta}^{con} -\nabla_{H} L_c({\theta}, {H}, {\Gamma})^{\top} \Delta_{H}^{con}-\langle \cP_{\cT}(R),\Delta_{\Gamma}^{con}\rangle-\langle \cP_{\cT^{\perp}}(R),\Delta_{\Gamma}^{con}\rangle-\lambda\|\cP_{\cT^{\perp}}(\Delta_{\Gamma}^{con})\|_{*}\notag\\
&\leq  -\nabla_{\theta} L_c({\theta}, {H}, {\Gamma})^{\top} \Delta_{\theta}^{con} -\nabla_{H} L_c({\theta}, {H}, {\Gamma})^{\top} \Delta_{H}^{con}\notag\\
&\quad +\|\cP_{\cT}(R)\|_F\|\cP_{\cT}(\Delta_{\Gamma}^{con})\|_F-\langle \cP_{\cT^{\perp}}(R),\Delta_{\Gamma}^{con}\rangle-\lambda\|\cP_{\cT^{\perp}}(\Delta_{\Gamma}^{con})\|_{*}.
\end{align}
By Claim \ref{claim2:pf_cv_ncv}, we have
\begin{align}\label{eq11:MLE_bound}
 -\langle \cP_{\cT^{\perp}}(R),\Delta_{\Gamma}^{con}\rangle
 \leq  \| \cP_{\cT^{\perp}}(R)\|\|\cP_{\cT^{\perp}}(\Delta_{\Gamma}^{con})\|_{*}
 \leq\left(1-\frac{\eps}{4}\right)\lambda\cdot\|\cP_{\cT^{\perp}}(\Delta_{\Gamma}^{con})\|_{*}.
\end{align}
Combine \eqref{eq10:MLE_bound} and \eqref{eq11:MLE_bound}, we obtain
\begin{align*}
 &C\left(\|\Delta_{\theta}^{con}\|_2^2+\|\Delta_{H}^{con}\|_F^2+\frac{1}{n^2}\|\Delta_{\Gamma}^{con}\|_F^2\right)\notag\\ &\leq  -\nabla_{\theta} L_c({\theta}, {H}, {\Gamma})^{\top} \Delta_{\theta}^{con} -\nabla_{H} L_c({\theta}, {H}, {\Gamma})^{\top} \Delta_{H}^{con} +\|\cP_{\cT}(R)\|_F\|\cP_{\cT}(\Delta_{\Gamma}^{con})\|_F-\frac{\eps}{4}\lambda\|\cP_{\cT^{\perp}}(\Delta_{\Gamma}^{con})\|_{*}\notag\\
 &\leq  -\nabla_{\theta} L_c({\theta}, {H}, {\Gamma})^{\top} \Delta_{\theta}^{con} -\nabla_{H} L_c({\theta}, {H}, {\Gamma})^{\top} \Delta_{H}^{con} +\|\cP_{\cT}(R)\|_F\|\cP_{\cT}(\Delta_{\Gamma}^{con})\|_F\notag\\
  &\leq  -\nabla_{\theta} L_c({\theta}, {H}, {\Gamma})^{\top} \Delta_{\theta}^{con} -\nabla_{H} L_c({\theta}, {H}, {\Gamma})^{\top} \Delta_{H}^{con} +\frac{ 72 \kappa}{\sqrt{\sigma_{\min}}} \|\cP(\nabla f(\theta,H,X,Y))\|_F\|\Delta_{\Gamma}^{con}\|_F\tag{by Claim \ref{claim2:pf_cv_ncv}}\\
&= -\left(\nabla_{\theta} L_c({\theta}, {H}, {\Gamma})-\mean(\nabla_{\theta} L_c({\theta}, {H}, {\Gamma}))\cdot\mathbf{1}\right)^{\top} \Delta_{\theta}^{con} -\nabla_{H} L_c({\theta}, {H}, {\Gamma})^{\top} \Delta_{H}^{con} \notag\\
&\quad+\frac{ 72 \kappa}{\sqrt{\sigma_{\min}}} \|\cP(\nabla f(\theta,H,X,Y))\|_F\|\Delta_{\Gamma}^{con}\|_F\tag{since $\mathbf{1}^T\Delta_{\theta}^{con}=0$}\\
&\leq \|\cP(\nabla f(\theta,H,X,Y))\|_F\|\Delta_{\theta}^{con}\|_F+\|\cP(\nabla f(\theta,H,X,Y))\|_F\|\Delta_{H}^{con}\|_F\notag\\
&\quad+\frac{ 72 \kappa}{\sqrt{\sigma_{\min}}} \|\cP(\nabla f(\theta,H,X,Y))\|_F\|\Delta_{\Gamma}^{con}\|_F\notag\\
&\leq \left(1+\frac{ 72 \kappa n}{\sqrt{\sigma_{\min}}}\right)\|\cP(\nabla f(\theta,H,X,Y))\|_F\cdot\left(\|\Delta_{\theta}^{con}\|_2+\|\Delta_{H}^{con}\|_F+\frac{1}{n}\|\Delta_{\Gamma}^{con}\|_F\right).
\end{align*}
Note that
\begin{align*}
\|\Delta_{\theta}^{con}\|_2^2+\|\Delta_{H}^{con}\|_F^2+\frac{1}{n^2}\|\Delta_{\Gamma}^{con}\|_F^2\geq \frac13 \left(\|\Delta_{\theta}^{con}\|_2+\|\Delta_{H}^{con}\|_F+\frac{1}{n}\|\Delta_{\Gamma}^{con}\|_F\right)^2.
\end{align*}
Thus, we have
\begin{align*}
&\frac{C}{3}\left(\|\Delta_{\theta}^{con}\|_2+\|\Delta_{H}^{con}\|_F+\frac{1}{n}\|\Delta_{\Gamma}^{con}\|_F\right)^2\\
&\leq \left(1+\frac{ 72 \kappa n}{\sqrt{\sigma_{\min}}}\right)\|\cP(\nabla f(\theta,H,X,Y))\|_F\cdot\left(\|\Delta_{\theta}^{con}\|_2+\|\Delta_{H}^{con}\|_F+\frac{1}{n}\|\Delta_{\Gamma}^{con}\|_F\right),
\end{align*}
which implies
\begin{align*}
\|\Delta_{\theta}^{con}\|_2+\|\Delta_{H}^{con}\|_F+\frac{1}{n}\|\Delta_{\Gamma}^{con}\|_F   
\leq \frac{3}{C}\left(1+\frac{ 72 \kappa n}{\sqrt{\sigma_{\min}}}\right)\|\cP(\nabla f(\theta,H,X,Y))\|_F.
\end{align*}
Further by \eqref{ncv:grad}, we obtain
\begin{align*}
\|\Delta_{\theta}^{con}\|_2\lesssim n^{-5},\quad
\|\Delta_{H}^{con}\|_F \lesssim n^{-5},\quad
\|\Delta_{\Gamma}^{con}\|_F\lesssim n^{-4}.
\end{align*}
Consequently, we show that
\begin{align*}
&\|\hat{\theta}^{con}-\theta^*\|_{\infty}\leq \|\Delta_{\theta}^{con}\|_2+\|\theta-\theta^*\|_{\infty}\lesssim c_{41}<c\sqrt{n},\\
&\|\hat{H}^{con}-H^*\|_F\leq \|\Delta_{H}^{con}\|_F+\|H-H^*\|_F\lesssim c_{11}\sqrt{n}<cn,\\
&\|\hat{\Gamma}^{con}-\Gamma^*\|_{\infty}\leq \|\Delta_{\Gamma}^{con}\|_F+\|\Gamma-\Gamma^*\|_{\infty}\lesssim c_{43}\sqrt{\mu\sX\sY r^2 n}<cn
\end{align*}
as long as $n$ is large enough.
In other words, the minimizer of \eqref{obj:con} is in the interior of the constraint. By the convexity of \eqref{obj:con}, we have $(\hat{\theta}^{con}, \hat{H}^{con}, \hat{\Gamma}^{con}) =(\hat{\theta}_c, \hat{H}_c, \hat{\Gamma}_c)$. By the constraints, we finish the proofs.
\end{proof}


With Claim \ref{claim2:pf_cv_ncv} and Claim \ref{claim:MLE_bound} in hand, we are ready to prove Theorem \ref{thm:cv_ncv} in the following.

\begin{proof}[Proof of Theorem \ref{thm:cv_ncv}]
We denote 
\begin{align*}
\Delta_{\theta}:=\hat{\theta}_c-\theta,\ 
\Delta_{H}:=\hat{H}_c-H,\ 
\Delta_{\Gamma}:=\hat{\Gamma}_c-XY^{\top}.
\end{align*}
By the optimality of $(\hat{\theta}_c, \hat{H}_c, \hat{\Gamma}_c)$, we have
\begin{align}\label{eq7:pf_cv_ncv}
L_c(\hat{\theta}_c, \hat{H}_c, \hat{\Gamma}_c)+\lambda\|\hat{\Gamma}_c\|_{*}\leq L_c({\theta}, {H}, {\Gamma})+\lambda\|\Gamma\|_{*}.
\end{align}
By Taylor expansion, we have
\begin{align}\label{eq30:pf_cv_ncv}
&L_c(\hat{\theta}_c, \hat{H}_c, \hat{\Gamma}_c)-L_c({\theta}, {H}, {\Gamma})\notag\\
&=\nabla L_c({\theta}, {H}, {\Gamma})^{\top}
\begin{bmatrix}
\Delta_{\theta}\\
\Delta_{H}\\
\Delta_{\Gamma}
\end{bmatrix}
+\frac12 
\begin{bmatrix}
\Delta_{\theta}\\
\Delta_{H}\\
\Delta_{\Gamma}
\end{bmatrix}^{\top}
\nabla^2 L_c(\tilde{\theta}, \tilde{H}, \tilde{\Gamma})
\begin{bmatrix}
\Delta_{\theta}\\
\Delta_{H}\\
\Delta_{\Gamma}
\end{bmatrix}\notag\\
&=\nabla L_c({\theta}, {H}, {\Gamma})^{\top}
\begin{bmatrix}
\Delta_{\theta}\\
\Delta_{H}\\
\Delta_{\Gamma}
\end{bmatrix}
+\frac12 
\begin{bmatrix}
\Delta_{\theta}\\
\Delta_{H}\\
\Delta_{\Gamma}
\end{bmatrix}^{\top}
\left(\sum_{i\neq j}\frac{e^{ \tilde{P}_{ij}}}{(1+e^{ \tilde{P}_{ij}})^2} 
\begin{bmatrix}
\frac{{e}_i+{e}_j}{\sqrt{n}}\\
{z}_i{z}_j^T\\
\frac{{e}_i{e}_j^T}{n}
\end{bmatrix}^{\otimes 2}\right)
\begin{bmatrix}
\Delta_{\theta}\\
\Delta_{H}\\
\Delta_{\Gamma}
\end{bmatrix}.
\end{align}
Note that for some constant $c''$
\begin{align}\label{ineq30:pf_cv_ncv}
 &\begin{bmatrix}
\Delta_{\theta}\\
\Delta_{H}\\
\Delta_{\Gamma}
\end{bmatrix}^{\top}
\left(\sum_{i\neq j}\frac{e^{ \tilde{P}_{ij}}}{(1+e^{ \tilde{P}_{ij}})^2} 
\begin{bmatrix}
\frac{{e}_i+{e}_j}{\sqrt{n}}\\
{z}_i{z}_j^T\\
\frac{{e}_i{e}_j^T}{n}
\end{bmatrix}^{\otimes 2}\right)
\begin{bmatrix}
\Delta_{\theta}\\
\Delta_{H}\\
\Delta_{\Gamma}
\end{bmatrix}\notag\\
&\geq_{(1)}
 \frac{e^{c'' c_P}}{(1+e^{c'' c_P})^2}
\begin{bmatrix}
\Delta_{\theta}\\
\Delta_{H}\\
\Delta_{\Gamma}
\end{bmatrix}^{\top}
\left(\sum_{i\neq j}
\begin{bmatrix}
\frac{{e}_i+{e}_j}{\sqrt{n}}\\
{z}_i{z}_j^T\\
\frac{{e}_i{e}_j^T}{n}
\end{bmatrix}^{\otimes 2}\right)
\begin{bmatrix}
\Delta_{\theta}\\
\Delta_{H}\\
\Delta_{\Gamma}
\end{bmatrix}\notag\\
&= \frac{e^{c'' c_P}}{(1+e^{c'' c_P})^2}\begin{bmatrix}
\Delta_{\theta}\\
\Delta_{H}\\
\frac1n \Delta_{\Gamma}
\end{bmatrix}^{\top}
\left(\sum_{i\neq j}
\begin{bmatrix}
\frac{{e}_i+{e}_j}{\sqrt{n}}\\
{z}_i{z}_j^T\\
{{e}_i{e}_j^T}
\end{bmatrix}^{\otimes 2}\right)
\begin{bmatrix}
\Delta_{\theta}\\
\Delta_{H}\\
\frac1n \Delta_{\Gamma}
\end{bmatrix}\notag\\
&\geq  \frac{\sl e^{c'' c_P}}{(1+e^{c'' c_P})^2}\left( \|\Delta_{\theta}\|_2^2+\|\Delta_{H}\|_F^2+\frac{1}{n^2}\|\Delta_{\Gamma}\|_F^2\right),
\end{align}
where the last inequality follows Assumption \ref{assumption:eigenvalues}.
Here (1) follows from the following argument: note that
\begin{align*}
|P_{ij}|
&:=\left|\frac{\theta_i+\theta_j}{\sqrt{n}}+{z}_i^\top{H}{z}_j + \frac{(XY^{\top})_{ij}}{n}\right|\\
&\leq |P_{ij}^{*}|+\frac{2}{\sqrt{n}}\|\theta-\theta^*\|_{\infty}+\frac{\sz}{n}\|H-H^*\|_2+\frac{1}{n}\|XY^{\top}-\Gamma^*\|_{\infty}.
\end{align*}
Further, by \eqref{ncv:est}, we have
\begin{align*}
&\|XY^T-\Gamma^*\|_{\infty}\\
&=\|(X-X^*)Y^T+X^{*}(Y-Y^*)^T\|_{\infty}\\
&\leq \|X-X^*\|_{2,\infty}\|Y\|_{2,\infty}+\|X^{*}\|_{2,\infty}\|Y-Y^*\|_{2,\infty} \tag{Cauchy}\\
&\lesssim c_{43}\sqrt{\mu \sX\sY r^2 n}.
\end{align*}
Thus, by \eqref{ncv:est} and Assumption \ref{assumption:scales}, as long as $n$ is large enough, we have $|P_{ij}|\leq 2c_P$.
Similarly, we have
\begin{align*}
|(\hat{P}_c)_{ij}|
&:=\left|\frac{(\hat{\theta}_c)_i+(\hat{\theta}_c)_j}{\sqrt{n}}+{z}_i^\top{\hat{H}_c}{z}_j + \frac{(\hat{\Gamma}_c)_{ij}}{n}\right|\\
&\leq |P_{ij}^{*}|+\frac{2}{\sqrt{n}}\|\hat{\theta}_c-\theta^*\|_{\infty}+\frac{\sz}{n}\|\hat{H}_c-H^*\|_2+\frac{1}{n}\|\hat{\Gamma}_c-\Gamma^*\|_{\infty}\\
&\leq |P_{ij}^{*}|+\frac{2}{\sqrt{n}}\|\hat{\theta}_c-\theta^*\|_{\infty}+\frac{\sz}{n}\|\hat{H}_c-H^*\|_F+\frac{1}{n}\|\hat{\Gamma}_c-\Gamma^*\|_{\infty}.
\end{align*}
Further by Claim \ref{claim:MLE_bound}, we have $|(\hat{P}_c)_{ij}|\lesssim c_P$.
Since $\tilde{P}_{ij}$ lies between $P_{ij}$ and $(\hat{P}_c)_{ij}$, we conclude that $|\tilde{P}_{ij}|\lesssim c_P$. Consequently, we have $\frac{e^{ \tilde{P}_{ij}}}{(1+e^{ \tilde{P}_{ij}})^2} \geq  \frac{e^{c'' c_P}}{(1+e^{c'' c_P})^2}$ for some constant $c''$, which implies (1).

Combine \eqref{eq30:pf_cv_ncv} and \eqref{ineq30:pf_cv_ncv}, we have
\begin{align}\label{eq8:pf_cv_ncv}
L_c(\hat{\theta}_c, \hat{H}_c, \hat{\Gamma}_c)-L_c({\theta}, {H}, {\Gamma})
\geq \nabla L_c({\theta}, {H}, {\Gamma})^{\top}
\begin{bmatrix}
\Delta_{\theta}\\
\Delta_{H}\\
\Delta_{\Gamma}
\end{bmatrix}
+C'\left(\|\Delta_{\theta}\|_2^2+\|\Delta_{H}\|_F^2+\frac{1}{n^2}\|\Delta_{\Gamma}\|_F^2\right)
\end{align}
for $C':= \frac{\sl e^{c'' c_P}}{2(1+e^{c'' c_P})^2}$. By \eqref{eq7:pf_cv_ncv} and \eqref{eq8:pf_cv_ncv}, we obtain
\begin{align}\label{eq9:pf_cv_ncv}
 C'\left(\|\Delta_{\theta}\|_2^2+\|\Delta_{H}\|_F^2+\frac{1}{n^2}\|\Delta_{\Gamma}\|_F^2\right)
 \leq -\nabla L_c({\theta}, {H}, {\Gamma})^{\top}
\begin{bmatrix}
\Delta_{\theta}\\
\Delta_{H}\\
\Delta_{\Gamma}
\end{bmatrix}+\lambda\|\Gamma\|_{*}-\lambda\|\hat{\Gamma}_c\|_{*}.
\end{align}
In addition, by the convexity of $\|\cdot\|_{*}$, we have
\begin{align*}
\|\hat{\Gamma}_c\|_{*}-\|\Gamma\|_{*}=\|\Gamma+\Delta_{\Gamma}\|_{*}-\|\Gamma\|_{*}\geq \langle UV^{\top}+W,\Delta_{\Gamma}\rangle
\end{align*}
for any $W\in\cT^{\perp}$ obeying $\|W\|\leq 1$. In the following, we pick $W$ such that $\langle W, \Delta_{\Gamma}\rangle=\|\cP_{\cT^{\perp}}(\Delta_{\Gamma})\|_{*}$. We then obtain $\|\hat{\Gamma}_c\|_{*}-\|\Gamma\|_{*}\geq  \langle UV^{\top},\Delta_{\Gamma}\rangle+\|\cP_{\cT^{\perp}}(\Delta_{\Gamma})\|_{*}$, and consequently, by \eqref{eq9:pf_cv_ncv}, we have
\begin{align*}
C'\left(\|\Delta_{\theta}\|_2^2+\|\Delta_{H}\|_F^2+\frac{1}{n^2}\|\Delta_{\Gamma}\|_F^2\right)
 \leq -\nabla L_c({\theta}, {H}, {\Gamma})^{\top}
\begin{bmatrix}
\Delta_{\theta}\\
\Delta_{H}\\
\Delta_{\Gamma}
\end{bmatrix}-\lambda\langle UV^{\top},\Delta_{\Gamma}\rangle-\lambda\|\cP_{\cT^{\perp}}(\Delta_{\Gamma})\|_{*}.
\end{align*}
Recall the definition of $R$ in \eqref{eq:R}, we further have
\begin{align}\label{eq10:pf_cv_ncv}
&C'\left(\|\Delta_{\theta}\|_2^2+\|\Delta_{H}\|_F^2+\frac{1}{n^2}\|\Delta_{\Gamma}\|_F^2\right)\notag\\
& \leq  -\nabla_{\theta} L_c({\theta}, {H}, {\Gamma})^{\top} \Delta_{\theta} -\nabla_{H} L_c({\theta}, {H}, {\Gamma})^{\top} \Delta_{H}-\langle R,\Delta_{\Gamma}\rangle-\lambda\|\cP_{\cT^{\perp}}(\Delta_{\Gamma})\|_{*}\notag\\
&=  -\nabla_{\theta} L_c({\theta}, {H}, {\Gamma})^{\top} \Delta_{\theta} -\nabla_{H} L_c({\theta}, {H}, {\Gamma})^{\top} \Delta_{H}-\langle \cP_{\cT}(R),\Delta_{\Gamma}\rangle-\langle \cP_{\cT^{\perp}}(R),\Delta_{\Gamma}\rangle-\lambda\|\cP_{\cT^{\perp}}(\Delta_{\Gamma})\|_{*}\notag\\
&\leq  -\nabla_{\theta} L_c({\theta}, {H}, {\Gamma})^{\top} \Delta_{\theta} -\nabla_{H} L_c({\theta}, {H}, {\Gamma})^{\top} \Delta_{H}\notag\\
&\quad +\|\cP_{\cT}(R)\|_F\|\cP_{\cT}(\Delta_{\Gamma})\|_F-\langle \cP_{\cT^{\perp}}(R),\Delta_{\Gamma}\rangle-\lambda\|\cP_{\cT^{\perp}}(\Delta_{\Gamma})\|_{*}.
\end{align}
By Claim \ref{claim2:pf_cv_ncv}, we have
\begin{align}\label{eq11:pf_cv_ncv}
 -\langle \cP_{\cT^{\perp}}(R),\Delta_{\Gamma}\rangle
 \leq  \| \cP_{\cT^{\perp}}(R)\|\|\cP_{\cT^{\perp}}(\Delta_{\Gamma})\|_{*}
 \leq\left(1-\frac{\eps}{4}\right)\lambda\cdot\|\cP_{\cT^{\perp}}(\Delta_{\Gamma})\|_{*}
\end{align}
Combine \eqref{eq10:pf_cv_ncv} and \eqref{eq11:pf_cv_ncv}, we obtain
\begin{align*}
 &C'\left(\|\Delta_{\theta}\|_2^2+\|\Delta_{H}\|_F^2+\frac{1}{n^2}\|\Delta_{\Gamma}\|_F^2\right)\notag\\ &\leq  -\nabla_{\theta} L_c({\theta}, {H}, {\Gamma})^{\top} \Delta_{\theta} -\nabla_{H} L_c({\theta}, {H}, {\Gamma})^{\top} \Delta_{H} +\|\cP_{\cT}(R)\|_F\|\cP_{\cT}(\Delta_{\Gamma})\|_F-\frac{\eps}{4}\lambda\|\cP_{\cT^{\perp}}(\Delta_{\Gamma})\|_{*}\notag\\
 &\leq  -\nabla_{\theta} L_c({\theta}, {H}, {\Gamma})^{\top} \Delta_{\theta} -\nabla_{H} L_c({\theta}, {H}, {\Gamma})^{\top} \Delta_{H} +\|\cP_{\cT}(R)\|_F\|\cP_{\cT}(\Delta_{\Gamma})\|_F\notag\\
  &\leq  -\nabla_{\theta} L_c({\theta}, {H}, {\Gamma})^{\top} \Delta_{\theta} -\nabla_{H} L_c({\theta}, {H}, {\Gamma})^{\top} \Delta_{H} +\frac{ 72 \kappa}{\sqrt{\sigma_{\min}}} \|\cP(\nabla f(\theta,H,X,Y))\|_F\|\Delta_{\Gamma}\|_F\tag{by Claim \ref{claim2:pf_cv_ncv}}\\
&= -\left(\nabla_{\theta} L_c({\theta}, {H}, {\Gamma})-\mean(\nabla_{\theta} L_c({\theta}, {H}, {\Gamma}))\cdot\mathbf{1}\right)^{\top} \Delta_{\theta} -\nabla_{H} L_c({\theta}, {H}, {\Gamma})^{\top} \Delta_{H} \notag\\
&\quad+\frac{ 72 \kappa}{\sqrt{\sigma_{\min}}} \|\cP(\nabla f(\theta,H,X,Y))\|_F\|\Delta_{\Gamma}\|_F\tag{since $\mathbf{1}^T\Delta_{\theta}=0$}\\
&\leq \|\cP(\nabla f(\theta,H,X,Y))\|_F\|\Delta_{\theta}\|_F+\|\cP(\nabla f(\theta,H,X,Y))\|_F\|\Delta_{H}\|_F\notag\\
&\quad+\frac{ 72 \kappa}{\sqrt{\sigma_{\min}}} \|\cP(\nabla f(\theta,H,X,Y))\|_F\|\Delta_{\Gamma}\|_F\notag\\
&\leq \left(1+\frac{ 72 \kappa n}{\sqrt{\sigma_{\min}}}\right)\|\cP(\nabla f(\theta,H,X,Y))\|_F\cdot\left(\|\Delta_{\theta}\|_2+\|\Delta_{H}\|_F+\frac{1}{n}\|\Delta_{\Gamma}\|_F\right).
\end{align*}
Note that
\begin{align*}
\|\Delta_{\theta}\|_2^2+\|\Delta_{H}\|_F^2+\frac{1}{n^2}\|\Delta_{\Gamma}\|_F^2\geq \frac13 \left(\|\Delta_{\theta}\|_2+\|\Delta_{H}\|_F+\frac{1}{n}\|\Delta_{\Gamma}\|_F\right)^2.
\end{align*}
Thus, we have
\begin{align*}
&\frac{C'}{3}\left(\|\Delta_{\theta}\|_2+\|\Delta_{H}\|_F+\frac{1}{n}\|\Delta_{\Gamma}\|_F\right)^2\\
&\leq \left(1+\frac{ 72 \kappa n}{\sqrt{\sigma_{\min}}}\right)\|\cP(\nabla f(\theta,H,X,Y))\|_F\cdot\left(\|\Delta_{\theta}\|_2+\|\Delta_{H}\|_F+\frac{1}{n}\|\Delta_{\Gamma}\|_F\right),
\end{align*}
which implies
\begin{align*}
\|\Delta_{\theta}\|_2+\|\Delta_{H}\|_F+\frac{1}{n}\|\Delta_{\Gamma}\|_F   
\leq \frac{3}{C'}\left(1+\frac{ 72 \kappa n}{\sqrt{\sigma_{\min}}}\right)\|\cP(\nabla f(\theta,H,X,Y))\|_F.
\end{align*}


\end{proof}









\subsection{Proofs of Corollary \ref{cor:cv_ncv}}\label{pf:cor_cv_ncv}
Note that by Lemma \ref{lem:ncv1}, we have
\begin{align*}
\|\hat{X}\hat{Y}^{\top}-\Gamma^{*}\|\leq 
\|\hat{X}-{X}^{*}\|\|\hat{Y}\|+\|\hat{Y}-{Y}^{*}\|\|{X}^{*}\|
\lesssim \sqrt{\sigma_{\max}n}c_{14}.
\end{align*}
and
\begin{align*}
\|\hat{X}\hat{Y}^{\top}-\Gamma^{*}\|_F\leq 
\|\hat{X}-{X}^{*}\|_F\|\hat{Y}\|+\|\hat{Y}-{Y}^{*}\|_F\|{X}^{*}\|
\lesssim \sqrt{\sigma_{\max}n}c_{11}.
\end{align*}
By Lemma \ref{lem:ncv4}, we have
\begin{align*}
\|\hat{X}\hat{Y}^{\top}-\Gamma^{*}\|_{\infty}\leq 
\|\hat{X}-{X}^{*}\|_{2,\infty}\|\hat{Y}\|_{2,\infty}+\|\hat{Y}-{Y}^{*}\|_{2,\infty}\|{X}^{*}\|_{2,\infty}
\lesssim \sqrt{\mu\sX\sY r^2 n}c_{43}.
\end{align*}
Further by Theorem \ref{thm:cv_ncv}, we have
\begin{align*}
&\|\hat{\Gamma}_c-\Gamma^{*}\|\lesssim \sqrt{\sigma_{\max}n}c_{14}\\
&\|\hat{\Gamma}_c-\Gamma^{*}\|_{F}\lesssim \sqrt{\sigma_{\max}n}c_{11}\\
&\|\hat{\Gamma}_c-\Gamma^{*}\|_{\infty}\lesssim \sqrt{\mu\sX\sY r^2 n}c_{43}.
\end{align*}

































==> proof_mem_est.tex <==
\section{Proofs for Section \ref{sec:mem_est}}
\subsection{Proofs of Theorem \ref{thm:mem_est}}\label{pf:thm_mem_est}

We first prove the following lemma.
\begin{lemma}\label{lem:U_2inf}
It holds that
\begin{align*}
    \min_{R\in\cO^{r\times r}}
    \|\hat{U}_c R-U^*\|_{2,\infty}\lesssim\frac{1}{\sqrt{\sigma_{\min}}}c_{43}+\frac{\sqrt{\kappa\mu\sX\sY r^2 }}{\sigma_{\min}}c_{14}n.
\end{align*}
\end{lemma}
\begin{proof}[Proof of Lemma \ref{lem:U_2inf}]
Let $\hat{U}\hat{\Sigma}\hat{V}^{\top}$ be the SVD of $\hat{X}\hat{Y}^{\top}$, where $\hat{X},\hat{Y}$ are the nonconvex estimators given in Section \ref{sec:ncv_debias}.
By Weyl’s inequality and Corollary \ref{cor:cv_ncv}, we have
\begin{align*}
|\sigma_{\min}(\hat{\Gamma})-\sigma_{\min}|\leq \|\hat{\Gamma}-{\Gamma}^*\|\lesssim \sqrt{\sigma_{\max}n}c_{14},
\end{align*}
which implies $\sigma_{\min}(\hat{\Gamma})\geq \sigma_{\min}/2$. By Davis-Kahan Theorem, we have
\begin{align*}
\min_{R\in\cO^{r\times r}}\|\hat{U}_c R-\hat{U}\|
&\leq \frac{2}{\sigma_{\min}(\hat{\Gamma})}\|\hat{\Gamma}_c -\hat{\Gamma}\|\\
&\leq \frac{4}{\sigma_{\min}}\|\hat{\Gamma}_c -\hat{\Gamma}\|_F\\
&\lesssim_{(1)}\frac{1}{\sigma_{\min}}\frac{(1+e^{c c_P})^2}{\sl e^{c c_P}}\left(1+\frac{ 72 \kappa n}{\sqrt{\sigma_{\min}}}\right)n^{-4}\\
&\lesssim n^{-5},
\end{align*}
where (1) follows from Theorem \ref{thm:cv_ncv} and \eqref{ncv:grad}.
We denote $\hat{R}_c:=\hat{O}_c\hat{R}$, where
\begin{align*}
\hat{O}_c:=\argmin_{R\in\cO^{r\times r}}\|\hat{U}_c R-\hat{U}\|,\quad
\hat{R}:=\argmin_{R\in\cO^{r\times r}}\|\hat{U} R-{U}^*\|.
\end{align*}
It then holds that
\begin{align}\label{ineq1:pf_mem}
&\min_{R\in\cO^{r\times r}}
\|\hat{U}_c R-U^*\|_{2,\infty}\notag\\
&\leq 
\|\hat{U}_c \hat{R}_c-U^*\|_{2,\infty}\notag\\
&\leq 
\|\hat{U}_c \hat{R}_c-\hat{U}\hat{R}\|_{2,\infty}+
\|\hat{U}\hat{R}-U^*\|_{2,\infty}\notag\\
&\leq \|\hat{U}_c \hat{O}_c\hat{R}-\hat{U}\hat{R}\|+
\|\hat{U}\hat{R}-U^*\|_{2,\infty}\notag\\
&\leq n^{-5}+\|\hat{U}\hat{R}-U^*\|_{2,\infty}.
\end{align}
Thus, it remains to bound $\|\hat{U}\hat{R}-U^*\|_{2,\infty}$ in the following.
By Claim \ref{claim1:pf_cv_ncv}, there exists an invertible matrix $Q$ such that $\hat{X}=\hat{U}\hat{\Sigma}^{\frac{1}{2}}Q$ and \eqref{ineq1:pf_cv_ncv} holds. By the definition of $X^{*}$, we have $X^*=U^*\Sigma^{* \frac{1}{2}}$. Thus, we have
\begin{align}\label{eq1:pf_mem}
&\hat{U}=  \hat{X}(\hat{\Sigma}^{\frac{1}{2}}Q)^{-1},\quad \hat{U}^{\top}\hat{X}=\hat{\Sigma}^{\frac{1}{2}}Q\notag\\
& U^*=X^*(\Sigma^{* \frac{1}{2}})^{-1},\quad U^{*\top}X^*=\Sigma^{* \frac{1}{2}}.
\end{align}
It then holds that
\begin{align}\label{ineq2:pf_mem}
&\|\hat{U}\hat{R}-U^*\|_{2,\infty}\notag\\
&=\|\hat{X}(\hat{\Sigma}^{\frac{1}{2}}Q)^{-1}\hat{R}-X^*(\Sigma^{* \frac{1}{2}})^{-1}\|_{2,\infty}\notag\\
&\leq \|(\hat{X}-X^*)(\Sigma^{* \frac{1}{2}})^{-1}\|_{2,\infty}+\|\hat{X}(Q^{-1}\hat{\Sigma}^{-\frac{1}{2}}\hat{R}-\Sigma^{* -\frac{1}{2}})\|_{2,\infty}\notag\\
&\leq \|\Sigma^{* -\frac{1}{2}}\|\|\hat{X}-X^*\|_{2,\infty}+\|Q^{-1}\hat{\Sigma}^{-\frac{1}{2}}\hat{R}-\Sigma^{* -\frac{1}{2}}\|\|\hat{X}\|_{2,\infty}\notag\\
&\leq \frac{1}{\sqrt{\sigma_{\min}}}c_{43}+2\|Q^{-1}\hat{\Sigma}^{-\frac{1}{2}}\hat{R}-\Sigma^{* -\frac{1}{2}}\|\sqrt{\mu\sX\sY r^2 n},
\end{align}
where the last inequality follows from \eqref{ncv:est} and the fact that
\begin{align*}
\|\hat{X}\|_{2,\infty}\leq \|\hat{X}-X^*\|_{2,\infty}+\|{X}^*\|_{2,\infty} \leq 2   \|{X}^*\|_{2,\infty}
\leq 2\sqrt{\mu\sX\sY r^2 n}.
\end{align*}
Note that
\begin{align*}
&\|Q^{-1}\hat{\Sigma}^{-\frac{1}{2}}\hat{R}-\Sigma^{* -\frac{1}{2}}\|\\
&=\|\Sigma^{* -\frac{1}{2}}(\hat{R}^{\top} \hat{\Sigma}^{\frac{1}{2}}Q-\Sigma^{* \frac{1}{2}})Q^{-1}\hat{\Sigma}^{-\frac{1}{2}}\hat{R}\|\\
&\leq \|\Sigma^{* -\frac{1}{2}}\| \|\hat{R}^{\top} \hat{\Sigma}^{\frac{1}{2}}Q-\Sigma^{* \frac{1}{2}}\| \|Q^{-1}\hat{\Sigma}^{-\frac{1}{2}}\hat{R}\|\\
&\leq \|\Sigma^{* -\frac{1}{2}}\| \|\hat{\Sigma}^{ -\frac{1}{2}}\|\|Q^{-1}\|\|\hat{R}^{\top} \hat{\Sigma}^{\frac{1}{2}}Q-\Sigma^{* \frac{1}{2}}\|.
\end{align*}
Since $Q$ satisfies \eqref{ineq1:pf_cv_ncv}, we have $\|Q^{-1}\|\leq 2$. Moreover, we have show that $\|\hat{\Sigma}^{-\frac{1}{2}}\|=\sqrt{1/\sigma_{\min}(\hat{\Gamma})}\leq \sqrt{2/\sigma_{\min}}$.
Thus, we obtain
\begin{align}\label{ineq3:pf_mem}
\|Q^{-1}\hat{\Sigma}^{-\frac{1}{2}}\hat{R}-\Sigma^{* -\frac{1}{2}}\|\leq \frac{4}{\sigma_{\min}}\|\hat{R}^{\top} \hat{\Sigma}^{\frac{1}{2}}Q-\Sigma^{* \frac{1}{2}}\|.
\end{align}
By \eqref{eq1:pf_mem}, we have
\begin{align*}
&\|\hat{R}^{\top} \hat{\Sigma}^{\frac{1}{2}}Q-\Sigma^{* \frac{1}{2}}\|\\
&=\|\hat{R}^{\top}\hat{U}^{\top}\hat{X}-{U}^{* \top}{X}^{*}\|\\
&\leq \|(\hat{R}^{\top}\hat{U}^{\top}-{U}^{* \top})\hat{X}\|+\|{U}^{* \top}(\hat{X}-{X}^{*})\|\\
&\leq \|\hat{X}\|\|\hat{U}\hat{R}-U^{*}\|+\|\hat{X}-{X}^{*}\|\\
&\leq 2\sqrt{\sigma_{\max}}\|\hat{U}\hat{R}-U^{*}\|+c_{14}\sqrt{n},
\end{align*}
where the last inequality follows from Lemma \ref{lem:ncv1} and the fact that
\begin{align*}
\|\hat{X}\|\leq \|\hat{X}-X^*\|+\|{X}^*\|\leq 2\|{X}^*\|=2\sqrt{\sigma_{\max}}.
\end{align*}
By Davis-Kahan Theorem and the definition of $\hat{R}$, we have
\begin{align*}
 \|\hat{U}\hat{R}-U^{*}\|=\min_{R\in\cO^{r\times r}}\|\hat{U}R-U^{*}\|  \leq \frac{2}{\sqrt{\sigma_{\min}} }\|\hat{X}-X^{*}\|
 \leq 2c_{14}\sqrt{\frac{n}{\sigma_{\min}}}.
\end{align*}
Thus, we have
\begin{align}\label{ineq4:pf_mem}
 \|\hat{R}^{\top} \hat{\Sigma}^{\frac{1}{2}}Q-\Sigma^{* \frac{1}{2}}\|\leq 4c_{14}\sqrt{\kappa n} +c_{14}\sqrt{n}\leq   5c_{14}\sqrt{\kappa n} .
\end{align}
Combine \eqref{ineq3:pf_mem} and \eqref{ineq4:pf_mem}, we have
\begin{align}\label{ineq5:pf_mem}
 \|Q^{-1}\hat{\Sigma}^{-\frac{1}{2}}\hat{R}-\Sigma^{* -\frac{1}{2}}\|\leq \frac{20}{\sigma_{\min}} c_{14}\sqrt{\kappa n} .  
\end{align}
Further by \eqref{ineq2:pf_mem}, we have
\begin{align*}
&\|\hat{U}\hat{R}-U^*\|_{2,\infty}\notag\\
&\leq \frac{1}{\sqrt{\sigma_{\min}}}c_{43}+\frac{40}{\sigma_{\min}}\sqrt{\kappa\mu\sX\sY r^2 }c_{14}n.
\end{align*}
Plug the above inequality into \eqref{ineq1:pf_mem}, we obtain
\begin{align*}
&\min_{R\in\cO^{r\times r}}
\|\hat{U}_c R-U^*\|_{2,\infty}\notag\\
&\leq n^{-5}+    \frac{1}{\sqrt{\sigma_{\min}}}c_{43}+\frac{40}{\sigma_{\min}}\sqrt{\kappa\mu\sX\sY r^2 }c_{14}n\notag\\
&\lesssim \frac{1}{\sqrt{\sigma_{\min}}}c_{43}+\frac{\sqrt{\kappa\mu\sX\sY r^2 }}{\sigma_{\min}}c_{14}n.
\end{align*}
We then finish the proof of Lemma \ref{lem:U_2inf}.
\end{proof}

Let
\begin{align*}
H:=\argmin_{R\in\cO^{r\times r}}\max_{1\leq i\leq n}\|R\hat{u}_i-u^{*}_i\|.
\end{align*}
By Lemma \ref{lem:U_2inf}, we have
\begin{align}\label{prop1:pf_mem}
  \max_{1\leq i\leq n}\|H\hat{u}_i-u^{*}_i\|  =\min_{R\in\cO^{r\times r}}
\|\hat{U}_c R-U^*\|_{2,\infty}\lesssim \frac{1}{\sqrt{\sigma_{\min}}}c_{43}+\frac{\sqrt{\kappa\mu\sX\sY r^2 }}{\sigma_{\min}}c_{14}n.
\end{align}
Recall the definition of efficient vertex-hunting algorithms, we have
\begin{align}\label{prop2:pf_mem}
 \max_{1\leq \ell \leq r}\|H\hat{v}_{\ell}-v_{\ell}\|\lesssim  \max_{1\leq i\leq n}\|H\hat{u}_i-u^{*}_i\| \lesssim \frac{1}{\sqrt{\sigma_{\min}}}c_{43}+\frac{\sqrt{\kappa\mu\sX\sY r^2 }}{\sigma_{\min}}c_{14}n.
\end{align}
We then prove Theorem \ref{thm:mem_est} in the following.
\begin{proof}[Proof of Theorem \ref{thm:mem_est}]
Note that
\begin{align*}
\underbrace{
\begin{bmatrix}
v_1,\ldots,v_r
\end{bmatrix}}_{=:Q}\pi^{*}_i=u^{*}_i,\quad
\underbrace{\begin{bmatrix}
H\hat{v}_1,\ldots,H\hat{v}_r
\end{bmatrix}}_{=:\hat{Q}}\hat{\pi}_i=H\hat{u}_i.
\end{align*}
We have the following claim.
\begin{claim}\label{claim1:pf_mem}
Under Assumption \ref{assumption:mem_est}, it holds that \begin{align*}
\|Q\|\lesssim \sqrt{\frac{r}{n}}\text{ and }
\|Q^{-1}\|\lesssim \sqrt{\frac{n}{r}}.
\end{align*}
\end{claim}
\begin{proof}[Proof of Claim \ref{claim1:pf_mem}]
Note that $U^*=\Pi^* B=\Pi^* Q^{\top}$. Thus, it holds that
\begin{align*}
I_r=U^{*\top}U^*=Q\Pi^{*\top}\Pi^*Q^{\top}=\frac{n}{r}QGQ^{\top}.
\end{align*}
This further implies that
\begin{align*}
Q^{\top}Q=\frac{n}{r}(Q^{\top}Q)G(Q^{\top}Q).
\end{align*}
Since $Q^{\top}Q$ is invertible, we have
\begin{align*}
Q^{\top}Q=\frac{r}{n}G^{-1}\text{ and }
Q^{-1}Q^{-\top}=(Q^{\top}Q)^{-1}=\frac{n}{r}G.
\end{align*}
By Assumption \ref{assumption:mem_est}, it then holds that
\begin{align*}
\|Q\|\leq \sqrt{\frac{r}{n}\|G^{-1}\|}\lesssim \sqrt{\frac{r}{n}}\text{ and }
\|Q^{-1}\|\leq \sqrt{\frac{n}{r}\|G\|}\lesssim \sqrt{\frac{n}{r}}.
\end{align*}
We then finish the proof of Claim \ref{claim1:pf_mem}.
\end{proof}
By Claim \ref{claim1:pf_mem}, we have $\sigma_{\min}(Q)\gtrsim \sqrt{r/n}$.
By Weyl's inequality, we have
\begin{align*}
|\sigma_{\min}(\hat{Q})-\sigma_{\min}(Q)|
&\leq \|\hat{Q}-Q\|\\
&\leq \|\hat{Q}-Q\|_F\\
&\leq \sqrt{r}\max_{1\leq \ell \leq r}\|H\hat{v}_{\ell}-v_{\ell}\|\\
&\lesssim \sqrt{r}\left(\frac{1}{\sqrt{\sigma_{\min}}}c_{43}+\frac{\sqrt{\kappa\mu\sX\sY r^2 }}{\sigma_{\min}}c_{14}n\right)\tag{by \eqref{prop2:pf_mem}}\\
&\ll \sqrt{\frac{r}{n}}.
\end{align*}
Thus, it holds that
\begin{align}\label{ineq6:pf_mem}
\|\hat{Q}^{-1}\|=\frac{1}{\sigma_{\min}(\hat{Q})}\leq \frac{2}{\sigma_{\min}({Q})}\lesssim \sqrt{\frac{n}{r}}.
\end{align}
Note that
\begin{align*}
\hat{\pi}_i-\pi^{*}_i
&=\hat{Q}^{-1}H\hat{u}_i-Q^{-1}u^{*}_i\\
&=\hat{Q}^{-1}(H\hat{u}_i-u^{*}_i)-\hat{Q}^{-1}(\hat{Q}-Q)Q^{-1}u^{*}_i\\
&=\hat{Q}^{-1}(H\hat{u}_i-u^{*}_i)-\hat{Q}^{-1}(\hat{Q}-Q)\pi^{*}_i.
\end{align*}
Consequently, we have
\begin{align*}
\|\hat{\pi}_i-\pi^{*}_i\|
&\leq \|\hat{Q}^{-1}\|\left(\|H\hat{u}_i-u^{*}_i\|+\|(\hat{Q}-Q)\pi^{*}_i\|\right)\\
&\lesssim \sqrt{\frac{n}{r}}\left(\|H\hat{u}_i-u^{*}_i\|+\|(\hat{Q}-Q)\pi^{*}_i\|\right),
\end{align*}
where the last inequality follows from \eqref{ineq6:pf_mem}.
Note that
\begin{align*}
\|(\hat{Q}-Q)\pi^{*}_i\|
&=\left\|\sum^r_{\ell=1}\pi^{*}_i(\ell)(H\hat{v}_{\ell}-v_{\ell})\right\|\\
&\leq \sum^r_{\ell=1}\pi^{*}_i(\ell)\|H\hat{v}_{\ell}-v_{\ell}\|\\
&\leq \max_{1\leq\ell r}\|H\hat{v}_{\ell}-v_{\ell}\|,
\end{align*}
where the last inequality follows from the fact that $\sum^r_{\ell=1}\pi^{*}_i(\ell)=1$. Thus, we obtain
\begin{align*}
\|\hat{\pi}_i-\pi^{*}_i\|\lesssim    \sqrt{\frac{n}{r}}\left(\|H\hat{u}_i-u^{*}_i\|+\max_{1\leq\ell r}\|H\hat{v}_{\ell}-v_{\ell}\|\right),
\end{align*}
which then gives
\begin{align*}
\max_{1\leq i\leq n}\|\hat{\pi}_i-\pi^{*}_i\|\lesssim    \sqrt{\frac{n}{r}}\left(\max_{1\leq i\leq n}\|H\hat{u}_i-u^{*}_i\|+\max_{1\leq\ell r}\|H\hat{v}_{\ell}-v_{\ell}\|\right).
\end{align*}
Further by \eqref{prop1:pf_mem} and \eqref{prop2:pf_mem}, we obtain
\begin{align*}
 \max_{1\leq i\leq n}\|\hat{\pi}_i-\pi^{*}_i\|
 &\lesssim    \sqrt{\frac{n}{r}}\left(\frac{1}{\sqrt{\sigma_{\min}}}c_{43}+\frac{\sqrt{\kappa\mu\sX\sY r^2 }}{\sigma_{\min}}c_{14}n\right) \\
 &= \sqrt{\frac{1}{nr}}\left(\frac{n}{\sqrt{\sigma_{\min}}}c_{43}+\frac{n^2}{\sigma_{\min}}\sqrt{\kappa\mu\sX\sY r^2 }c_{14}\right).
\end{align*}

\end{proof}

==> proof_ncv_debias.tex <==

\section{Proofs for Section \ref{sec:ncv_debias}}

We first prove some useful lemmas in the following.

% \begin{lemma}\label{lem:D}
% Suppose Assumption \ref{assumption:scales} and \ref{assumption:eigenvalues} holds. We have
% \begin{align*}
% \slD\leq \lambda_{\min}(\cP D^* \cP)\leq \lambda_{\max}(\cP D^* \cP)\leq \suD,
% \end{align*}
% where 
% \begin{align*}
% \slD = \frac{\sl e^{c_P}}{(1+e^{c_P})^2}\min \left\{1,\frac{\sigma_{\min}}{n^2} \right\},\quad
% \suD = \frac{\su}{4}\max \left\{1,\frac{2\sigma_{\max}}{n^2} \right\}.
% \end{align*}
% Moreover, we have
% \begin{align*}
% \|\cP\hat{D}\cP-\cP D^* \cP\|\lesssim  \frac{\hat{c}}{\sqrt{n}}
% \end{align*}
% and 
% \begin{align*}
% \frac{\slD}{2}\leq \lambda_{\min}(\cP \hat{D} \cP)\leq \lambda_{\max}(\cP  \hat{D}  \cP)\leq {2\suD}.
% \end{align*}
% Here 
% \begin{align*}
% \hat{c}=\frac{(1+e^{c_P})^2}{e^{c_P}}\left(\suD c_{41}+\sqrt{\mu \sX\sY r^2}(\suD c_{43}+c_{11})+\sz\suD c_{11}\right).
% \end{align*}
% \end{lemma}
\begin{lemma}\label{lem:D}
Under Assumption \ref{assumption:D_eigen}, we have
\begin{align*}
\|\cP\hat{D}\cP-\cP D^* \cP\|\lesssim  \frac{\hat{c}}{\sqrt{n}}
\end{align*}
and 
\begin{align*}
\frac{\slD}{2}\leq \lambda_{\min}(\cP \hat{D} \cP)\leq \lambda_{\max}(\cP  \hat{D}  \cP)\leq {2\suD}.
\end{align*}
Here 
\begin{align*}
\hat{c}=\frac{(1+e^{c_P})^2}{e^{c_P}}\left(\suD c_{41}+\sqrt{\mu \sX\sY r^2}(\suD c_{43}+c_{11})+\sz\suD c_{11}\right).
\end{align*}
\end{lemma}
\begin{proof}[Proof of Lemma \ref{lem:D}]
% Note that for any $\Delta=\begin{bmatrix}
% \Delta_{\theta}\\ \Delta_H\\ \Delta_X\\ \Delta_Y
% \end{bmatrix}$, we have
% \begin{align*}
% &\vec(\Delta)^T(\cP D^* \cP)\vec(\Delta)\\
% &=
% \begin{bmatrix}
%   \vec(\Delta_{\theta})\\
%   \vec(\Delta_{H})\\
%   \frac1n\vec(\Delta_{X}Y^{* \top}+X^{*}\Delta_{Y}^{\top})
% \end{bmatrix}^T\!\!\!\!\!
% \cP_c\!
% \left(\sum_{i\neq j}
% \frac{e^{{P}^*_{ij}}}{(1+e^{{P}^*_{ij}})^2}
%   \begin{bmatrix}
%   \frac{1}{\sqrt{n}}\vec(e_i+e_j)\\
%   \vec(z_iz_j^T)\\
%   \vec(e_ie_j^T)
%   \end{bmatrix}
%    \begin{bmatrix}
%   \frac{1}{\sqrt{n}}\vec(e_i+e_j)\\
%   \vec(z_iz_j^T)\\
%   \vec(e_ie_j^T)
%   \end{bmatrix}^T
% \right)\cP_c\!
% \begin{bmatrix}
%   \vec(\Delta_{\theta})\\
%   \vec(\Delta_{H})\\
%   \frac1n\vec(\Delta_{X}Y^{* \top}+X^{*}\Delta_{Y}^{\top})
% \end{bmatrix}\\
% &\leq \frac14
% \begin{bmatrix}
%   \vec(\Delta_{\theta})\\
%   \vec(\Delta_{H})\\
%   \frac1n\vec(\Delta_{X}Y^{* \top}+X^{*}\Delta_{Y}^{\top})
% \end{bmatrix}^T\!\!\!\!\!
% \cP_c\!
% \left(\sum_{i\neq j}
%   \begin{bmatrix}
%   \frac{1}{\sqrt{n}}\vec(e_i+e_j)\\
%   \vec(z_iz_j^T)\\
%   \vec(e_ie_j^T)
%   \end{bmatrix}
%    \begin{bmatrix}
%   \frac{1}{\sqrt{n}}\vec(e_i+e_j)\\
%   \vec(z_iz_j^T)\\
%   \vec(e_ie_j^T)
%   \end{bmatrix}^T
% \right)\cP_c\!
% \begin{bmatrix}
%   \vec(\Delta_{\theta})\\
%   \vec(\Delta_{H})\\
%   \frac1n\vec(\Delta_{X}Y^{* \top}+X^{*}\Delta_{Y}^{\top})
% \end{bmatrix}\\
% &\leq\frac{\su}{4}
% \left(
% \|\Delta_{\theta}\|_2^2+\|\Delta_{H}\|_F^2+\frac{1}{n^2}\|\Delta_{X}Y^{* \top}+X^{*}\Delta_{Y}^{\top}\|_F^2
% \right)\tag{by Assumption \ref{assumption:eigenvalues}}\\
% &\leq\frac{\su}{4}
% \left(
% \|\Delta_{\theta}\|_2^2+\|\Delta_{H}\|_F^2+\frac{1}{n^2}(\|\Delta_{X}\|_F\|Y^{*}\|+\|\Delta_{Y}\|_F\|X^{*}\|)^2
% \right)\\
% &\leq\frac{\su}{4}
% \left(
% \|\Delta_{\theta}\|_2^2+\|\Delta_{H}\|_F^2+\frac{2\sigma_{\max}}{n^2}(\|\Delta_{X}\|_F^2+\|\Delta_{Y}\|_F^2)
% \right)\\
% &\leq \frac{\su}{4}\max \left\{1,\frac{2\sigma_{\max}}{n^2} \right\}\|\vec(\Delta)\|_2^2,
% \end{align*}
% which then gives $\lambda_{\max}(\cP D^* \cP)\leq \suD$. Similarly, we have
% \begin{align*}
% &\vec(\Delta)^T(\cP D^* \cP)\vec(\Delta)\\
% &=
% \begin{bmatrix}
%   \vec(\Delta_{\theta})\\
%   \vec(\Delta_{H})\\
%   \frac1n\vec(\Delta_{X}Y^{* \top}+X^{*}\Delta_{Y}^{\top})
% \end{bmatrix}^T\!\!\!\!\!
% \cP_c\!
% \left(\sum_{i\neq j}
% \frac{e^{{P}^*_{ij}}}{(1+e^{{P}^*_{ij}})^2}
%   \begin{bmatrix}
%   \frac{1}{\sqrt{n}}\vec(e_i+e_j)\\
%   \vec(z_iz_j^T)\\
%   \vec(e_ie_j^T)
%   \end{bmatrix}
%    \begin{bmatrix}
%   \frac{1}{\sqrt{n}}\vec(e_i+e_j)\\
%   \vec(z_iz_j^T)\\
%   \vec(e_ie_j^T)
%   \end{bmatrix}^T
% \right)\cP_c\!
% \begin{bmatrix}
%   \vec(\Delta_{\theta})\\
%   \vec(\Delta_{H})\\
%   \frac1n\vec(\Delta_{X}Y^{* \top}+X^{*}\Delta_{Y}^{\top})
% \end{bmatrix}\\
% &\geq \frac{e^{c_P}}{(1+e^{c_P})^2}
% \begin{bmatrix}
%   \vec(\Delta_{\theta})\\
%   \vec(\Delta_{H})\\
%   \frac1n\vec(\Delta_{X}Y^{* \top}+X^{*}\Delta_{Y}^{\top})
% \end{bmatrix}^T\!\!\!\!\!
% \cP_c\!
% \left(\sum_{i\neq j}
%   \begin{bmatrix}
%   \frac{1}{\sqrt{n}}\vec(e_i+e_j)\\
%   \vec(z_iz_j^T)\\
%   \vec(e_ie_j^T)
%   \end{bmatrix}
%    \begin{bmatrix}
%   \frac{1}{\sqrt{n}}\vec(e_i+e_j)\\
%   \vec(z_iz_j^T)\\
%   \vec(e_ie_j^T)
%   \end{bmatrix}^T
% \right)\cP_c\!
% \begin{bmatrix}
%   \vec(\Delta_{\theta})\\
%   \vec(\Delta_{H})\\
%   \frac1n\vec(\Delta_{X}Y^{* \top}+X^{*}\Delta_{Y}^{\top})
% \end{bmatrix}\\
% &\geq\frac{\sl e^{c_P}}{(1+e^{c_P})^2}
% \left(
% \|\Delta_{\theta}\|_2^2+\|\Delta_{H}\|_F^2+\frac{1}{n^2}\|\Delta_{X}Y^{* \top}+X^{*}\Delta_{Y}^{\top}\|_F^2
% \right)\\
% &\geq_{\textcolor{red}{(1)}}\frac{\sl e^{c_P}}{(1+e^{c_P})^2}
% \left(
% \|\Delta_{\theta}\|_2^2+\|\Delta_{H}\|_F^2+\frac{\sigma_{\min}}{n^2}(\|\Delta_{X}\|_F^2+\|\Delta_{Y}\|_F^2)
% \right)\tag{\textcolor{red}{Not true!}}\\
% &\geq\frac{\sl e^{c_P}}{(1+e^{c_P})^2}\min \left\{1,\frac{\sigma_{\min}}{n^2} \right\}\|\vec(\Delta)\|_2^2,
% \end{align*}
% which then gives $\lambda_{\min}(\cP D^* \cP)\geq \slD$.

% \textcolor{red}{
% Question: 
% (1) does not hold! Similar to local convexity, we need to add another term so that this is true.
% We need to make assumption on $D^*$ instead of proving it? Is it possible that $\lambda_{\min}(\cP D^* \cP)$ can't be lower bounded by a positive constant given Assumption \ref{assumption:eigenvalues}? If we add the assumption on $\cP D^* \cP$, do we still need $f_{\aug}$ for local convexity and do we still need Assumption \ref{assumption:eigenvalues}?
% }













We first control $\|\cP\hat{D}\cP-\cP D^*\cP\|$ in the following.
Note that
\begin{align*}
&\hat{D}- D^*\notag\\
&=
\sum_{i\neq j}\left(\frac{e^{\hat{P}_{ij}}}{(1+e^{\hat{P}_{ij}})^2}-\frac{e^{P^{*}_{ij}}}{(1+e^{P^{*}_{ij}})^2}\right)\begin{bmatrix}
\frac{1}{\sqrt{n}}(e_i+e_j)\\
z_iz_j^T\\
\frac1ne_ie_j^TY^*\\
\frac1ne_je_i^TX^*
\end{bmatrix}^{\otimes 2}\notag\\
&\quad+\sum_{i\neq j}\frac{e^{\hat{P}_{ij}}}{(1+e^{\hat{P}_{ij}})^2}\left(
\begin{bmatrix}
\frac{1}{\sqrt{n}}(e_i+e_j)\\
z_iz_j^T\\
\frac1ne_ie_j^T\hat{Y}\\
\frac1ne_je_i^T\hat{X}
\end{bmatrix}^{\otimes 2}
-\begin{bmatrix}
\frac{1}{\sqrt{n}}(e_i+e_j)\\
z_iz_j^T\\
\frac1ne_ie_j^TY^*\\
\frac1ne_je_i^TX^*
\end{bmatrix}^{\otimes 2}
\right)
\end{align*}
Thus, it holds that
\begin{align}\label{eq1:delta_diff}
&\|\cP\hat{D}\cP-\cP D^*\cP\|\notag\\
&\leq 
\left\|\sum_{i\neq j}\left(\frac{e^{\hat{P}_{ij}}}{(1+e^{\hat{P}_{ij}})^2}-\frac{e^{P^{*}_{ij}}}{(1+e^{P^{*}_{ij}})^2}\right)
\cP
\begin{bmatrix}
\frac{1}{\sqrt{n}}(e_i+e_j)\\
z_iz_j^T\\
\frac1ne_ie_j^TY^*\\
\frac1ne_je_i^TX^*
\end{bmatrix}^{\otimes 2}\cP\right\|\notag\\
&\quad+\left\|\sum_{i\neq j}\frac{e^{\hat{P}_{ij}}}{(1+e^{\hat{P}_{ij}})^2}\left(
\begin{bmatrix}
\frac{1}{\sqrt{n}}(e_i+e_j)\\
z_iz_j^T\\
\frac1ne_ie_j^T\hat{Y}\\
\frac1ne_je_i^T\hat{X}
\end{bmatrix}^{\otimes 2}
-\begin{bmatrix}
\frac{1}{\sqrt{n}}(e_i+e_j)\\
z_iz_j^T\\
\frac1ne_ie_j^TY^*\\
\frac1ne_je_i^TX^*
\end{bmatrix}^{\otimes 2}
\right)\right\|
\end{align}
For the first term, we have
\begin{align*}
&\left\|\sum_{i\neq j}\left(\frac{e^{\hat{P}_{ij}}}{(1+e^{\hat{P}_{ij}})^2}-\frac{e^{P^{*}_{ij}}}{(1+e^{P^{*}_{ij}})^2}\right)\cP\begin{bmatrix}
\frac{1}{\sqrt{n}}(e_i+e_j)\\
z_iz_j^T\\
\frac1ne_ie_j^TY^*\\
\frac1ne_je_i^TX^*
\end{bmatrix}^{\otimes 2}\cP\right\|\\
&\leq \left\|\sum_{i\neq j}\left|\frac{e^{\hat{P}_{ij}}}{(1+e^{\hat{P}_{ij}})^2}-\frac{e^{P^{*}_{ij}}}{(1+e^{P^{*}_{ij}})^2}\right|\cP\begin{bmatrix}
\frac{1}{\sqrt{n}}(e_i+e_j)\\
z_iz_j^T\\
\frac1ne_ie_j^TY^*\\
\frac1ne_je_i^TX^*
\end{bmatrix}^{\otimes 2}\cP\right\|\\
&\leq\frac14 \left\|\sum_{i\neq j}\left|\hat{P}_{ij}-P^*_{ij}\right|\cP\begin{bmatrix}
\frac{1}{\sqrt{n}}(e_i+e_j)\\
z_iz_j^T\\
\frac1ne_ie_j^TY^*\\
\frac1ne_je_i^TX^*
\end{bmatrix}^{\otimes 2}\cP\right\|\tag{by mean-value theorem}\\
&\leq \frac14 \max_{i\neq j}|\hat{P}_{ij}-P^*_{ij}|
 \left\|\cP\sum_{i\neq j}\begin{bmatrix}
\frac{1}{\sqrt{n}}(e_i+e_j)\\
z_iz_j^T\\
\frac1ne_ie_j^TY^*\\
\frac1ne_je_i^TX^*
\end{bmatrix}^{\otimes 2}\cP\right\|\\
&\leq \frac{(1+e^{c_P})^2}{4e^{c_P}} \max_{i\neq j}|\hat{P}_{ij}-P^*_{ij}|
 \left\|\cP D^{*}\cP\right\|.
\end{align*}
Note that
\begin{align*}
\max_{i\neq j}|\hat{P}_{ij}-P^*_{ij}|
&\lesssim\frac{1}{\sqrt{n}}\|\hat{\theta}-\theta^*\|_{\infty}+  \frac{\sz}{n}\|\hat{H}-H^*\|_{F}+\frac1n\|F^{*}\|_{2,\infty}\|\hat{F}-F^*\|_{2,\infty},\\
&\lesssim \frac{c_{41}+\sz c_{11}+\sqrt{\mu\sX\sY r^2}c_{43}}{\sqrt{n}},
\end{align*}
where the last inequality follows from \eqref{ncv:est} and Assumption \ref{assumption:incoherent}. 
Since we have $\|\cP D^*\cP\|\leq \suD$, it then holds that
\begin{align}\label{eq2:delta_diff}
 &\left\|\sum_{i\neq j}\left(\frac{e^{\hat{P}_{ij}}}{(1+e^{\hat{P}_{ij}})^2}-\frac{e^{P^{*}_{ij}}}{(1+e^{P^{*}_{ij}})^2}\right)\cP\begin{bmatrix}
\frac{1}{\sqrt{n}}(e_i+e_j)\\
z_iz_j^T\\
\frac1ne_ie_j^TY^*\\
\frac1ne_je_i^TX^*
\end{bmatrix}^{\otimes 2}\cP\right\|\notag\\
&\lesssim \frac{(1+e^{c_P})^2}{e^{c_P}}\cdot \frac{c_{41}+\sz c_{11}+\sqrt{\mu\sX\sY r^2}c_{43}}{\sqrt{n}} \cdot \suD.   
\end{align}

For the second term, note that for any $\Delta$,
\begin{align*}
&\left|\vec(\Delta)^T\left(\sum_{i\neq j}\frac{e^{\hat{P}_{ij}}}{(1+e^{\hat{P}_{ij}})^2}\left(
\begin{bmatrix}
\frac{1}{\sqrt{n}}(e_i+e_j)\\
z_iz_j^T\\
\frac1ne_ie_j^T\hat{Y}\\
\frac1ne_je_i^T\hat{X}
\end{bmatrix}^{\otimes 2}
-\begin{bmatrix}
\frac{1}{\sqrt{n}}(e_i+e_j)\\
z_iz_j^T\\
\frac1ne_ie_j^TY^*\\
\frac1ne_je_i^TX^*
\end{bmatrix}^{\otimes 2}
\right)\right)\vec(\Delta)\right|\\
&=\Bigg|
\sum_{i\neq j}\frac{e^{\hat{P}_{ij}}}{(1+e^{\hat{P}_{ij}})^2}\cdot\\
&\qquad\Bigg(
\frac{2}{n^{3/2}}\langle\Delta_{\theta}, e_i+e_j\rangle \langle e_i^T\Delta_X, e_j^T(\hat{Y}-Y^*)\rangle+\frac{2}{n^{3/2}}\langle\Delta_{\theta}, e_i+e_j\rangle \langle e_j^T\Delta_Y, e_i^T(\hat{X}-X^*)\rangle\\
&\qquad\quad +\frac{2}{n}\langle\Delta_{H}, z_iz_j^T\rangle \langle e_i^T\Delta_X, e_j^T(\hat{Y}-Y^*)\rangle+\frac{2}{n}\langle\Delta_{H}, z_iz_j^T\rangle \langle e_j^T\Delta_Y, e_i^T(\hat{X}-X^*)\rangle\\
&\qquad\quad +\frac{2}{n^2}\langle e^T_j\Delta_Y, e^T_i\hat{X}\rangle \langle e_i^T\Delta_X, e_j^T(\hat{Y}-Y^*)\rangle+\frac{2}{n^2}\langle e^T_i\Delta_X, e^T_j Y^{*}\rangle \langle e_j^T\Delta_Y, e_i^T(\hat{X}-X^*)\rangle\\
&\qquad\quad +\frac{1}{n^2}\langle e^T_i\Delta_X, e^T_j\hat{Y}\rangle \langle e_i^T\Delta_X, e_j^T(\hat{Y}-Y^*)\rangle+\frac{1}{n^2}\langle e^T_i\Delta_X, e^T_j Y^{*}\rangle \langle e_i^T\Delta_X, e_j^T(\hat{Y}-Y^*)\rangle\\
&\qquad\quad +\frac{1}{n^2}\langle e^T_j\Delta_Y, e^T_i\hat{X}\rangle \langle e_j^T\Delta_Y, e_i^T(\hat{X}-X^*)\rangle+\frac{1}{n^2}\langle e^T_j\Delta_Y, e^T_i X^{*}\rangle \langle e_j^T\Delta_Y, e_i^T(\hat{X}-X^*)\rangle
\Bigg)
\Bigg|.
\end{align*}
Note that
\begin{align*}
&\left|\frac{2}{n^{3/2}}
\sum_{i\neq j}\frac{e^{\hat{P}_{ij}}}{(1+e^{\hat{P}_{ij}})^2}
\langle\Delta_{\theta}, e_i+e_j\rangle \langle e_i^T\Delta_X, e_j^T(\hat{Y}-Y^*)\rangle
\right|\\
&\lesssim \frac{1}{n^{3/2}}
\sqrt{\sum_{i\neq j}|\langle\Delta_{\theta}, e_i+e_j\rangle|^2}\cdot
\sqrt{\sum_{i\neq j}| \langle e_i^T\Delta_X, e_j^T(\hat{Y}-Y^*)\rangle |^2}\\
&\lesssim\frac{1}{n^{3/2}}\cdot \sqrt{n}\|\Delta_{\theta}\|_2\cdot\|\Delta_{X}\|_F\|\hat{Y}-Y^*\|_F\\
&\lesssim_{(i)} \frac{c_{11}}{\sqrt{n}}\|\Delta_{\theta}\|_2\cdot\|\Delta_{X}\|_F\\
&\lesssim \frac{c_{11}}{\sqrt{n}}(\|\Delta_{\theta}\|_2^2+\|\Delta_{X}\|_F^2),
\end{align*}
where (i) follows from Lemma \ref{lem:ncv1}.
Similar arguments hold for the other terms, for which we omit the proofs. We then have
\begin{align*}
&\left|\vec(\Delta)^T\left(\sum_{i\neq j}\frac{e^{\hat{P}_{ij}}}{(1+e^{\hat{P}_{ij}})^2}\left(
\begin{bmatrix}
\frac{1}{\sqrt{n}}(e_i+e_j)\\
z_iz_j^T\\
\frac1ne_ie_j^T\hat{Y}\\
\frac1ne_je_i^T\hat{X}
\end{bmatrix}^{\otimes 2}
-\begin{bmatrix}
\frac{1}{\sqrt{n}}(e_i+e_j)\\
z_iz_j^T\\
\frac1ne_ie_j^TY^*\\
\frac1ne_je_i^TX^*
\end{bmatrix}^{\otimes 2}
\right)\right)\vec(\Delta)\right|\\  
&\lesssim\frac{c_{11}+\sqrt{\sz}c_{11}+\sqrt{\mu r \sigma_{\max}/n^2}c_{11}}{\sqrt{n}}(\|\Delta_{\theta}\|_2^2+\|\Delta_{H}\|_F^2+\|\Delta_{X}\|_F^2+\|\Delta_{Y}\|_F^2)\\
&=\frac{c_{11}+\sqrt{\sz}c_{11}+\sqrt{\mu r \sigma_{\max}/n^2}c_{11}}{\sqrt{n}}\|\vec(\Delta)\|_2^2.
\end{align*}
Consequently, we have
\begin{align}\label{eq3:delta_diff}
&\left\|\sum_{i\neq j}\frac{e^{\hat{P}_{ij}}}{(1+e^{\hat{P}_{ij}})^2}\left(
\begin{bmatrix}
\frac{1}{\sqrt{n}}(e_i+e_j)\\
z_iz_j^T\\
\frac1ne_ie_j^T\hat{Y}\\
\frac1ne_je_i^T\hat{X}
\end{bmatrix}^{\otimes 2}
-\begin{bmatrix}
\frac{1}{\sqrt{n}}(e_i+e_j)\\
z_iz_j^T\\
\frac1ne_ie_j^TY^*\\
\frac1ne_je_i^TX^*
\end{bmatrix}^{\otimes 2}
\right)\right\| \notag\\
&\lesssim \frac{c_{11}+\sqrt{\sz}c_{11}+\sqrt{\mu r \sigma_{\max}/n^2}c_{11}}{\sqrt{n}},\notag\\
&\lesssim \frac{c_{11}+\sqrt{\sz}c_{11}+\sqrt{\mu \sX\sY r^2}c_{11}}{\sqrt{n}},
\end{align}
where the last inequality follows from $\sigma_{\max}\leq \sX\sY r n^2$. Combine \eqref{eq1:delta_diff}, \eqref{eq2:delta_diff} and \eqref{eq3:delta_diff}, we have
\begin{align*}
&\|\cP\hat{D}\cP-\cP D^*\cP\|\\
&\lesssim  \frac{(1+e^{c_P})^2}{e^{c_P}}\cdot \frac{c_{41}+\sz c_{11}+\sqrt{\mu\sX\sY r^2}c_{43}}{\sqrt{n}} \cdot \suD+\frac{c_{11}+\sqrt{\sz}c_{11}+\sqrt{\mu \sX\sY r^2}c_{11}}{\sqrt{n}}\\
&\lesssim \frac{1}{\sqrt{n}} \frac{(1+e^{c_P})^2}{e^{c_P}}\left(\suD c_{41}+\sqrt{\mu \sX\sY r^2}(\suD c_{43}+c_{11})+\sz\suD c_{11}\right)\\
&=  \frac{\hat{c}}{\sqrt{n}} .
\end{align*}
By Weyl's inequality, we have
\begin{align*}
|\lambda_i(\cP\hat{D}\cP)-\lambda_i(\cP D^*\cP)|\lesssim \|\cP \hat{D}\cP-\cP D^*\cP\|\lesssim \frac{\hat{c}}{\sqrt{n}}.
\end{align*}
Since $\slD\leq \lambda_{\min}(\cP D^* \cP)\leq \lambda_{\max}(\cP D^* \cP)\leq \suD$, we then have $\frac{\slD}{2}\leq \lambda_{\min}(\cP \hat{D} \cP)\leq \lambda_{\max}(\cP  \hat{D}  \cP)\leq {2\suD}$ as long as $n$ is large enough.

\end{proof}


\subsection{Proofs of Proposition \ref{prop:debias_dist}}\label{pf:prop_debias_dist}
By \eqref{def:debias}, we have
\begin{align*}
\left\|\begin{bmatrix}
\hat{\theta}^d-\hat{\theta}\\
\hat{H}^d-\hat{H}\\
\hat{X}^d-\hat{X}\\
\hat{Y}^d-\hat{Y}
\end{bmatrix}\right\|_F
&=\|(\cP \hat{D}\cP)^{\dagger}\cP\nabla L(\hat{\theta},\hat{H},\hat{X},\hat{Y})\|_F\\
&\leq 
\frac{1}{\lambda_{\min}(\cP \hat{D}\cP )}\|\cP\nabla L(\hat{\theta},\hat{H},\hat{X},\hat{Y})\|_F.
\end{align*}
Note that by \eqref{ncv:grad}, we have
\begin{align*}
\left\|\nabla L(\hat{\theta},\hat{H},\hat{X},\hat{Y})
-
\begin{bmatrix}
\mean(\nabla_{\theta} L(\hat{\theta},\hat{H},\hat{X},\hat{Y}))\cdot\mathbf{1}\\
0\\
-\lambda\hat{X}\\
-\lambda\hat{Y}
\end{bmatrix}\right\|_F
\lesssim n^{-5}.
\end{align*}
Thus, it holds that
\begin{align*}
\left\|\cP\nabla L(\hat{\theta},\hat{H},\hat{X},\hat{Y})
-
\begin{bmatrix}
0\\
0\\
-\lambda\hat{X}\\
-\lambda\hat{Y}
\end{bmatrix}\right\|_F
&=\left\|\cP\left(\nabla L(\hat{\theta},\hat{H},\hat{X},\hat{Y})
-
\begin{bmatrix}
\mean(\nabla_{\theta} L(\hat{\theta},\hat{H},\hat{X},\hat{Y}))\cdot\mathbf{1}\\
0\\
-\lambda\hat{X}\\
-\lambda\hat{Y}
\end{bmatrix}\right)\right\|_F\\
&\leq \left\|\nabla L(\hat{\theta},\hat{H},\hat{X},\hat{Y})
-
\begin{bmatrix}
\mean(\nabla_{\theta} L(\hat{\theta},\hat{H},\hat{X},\hat{Y}))\cdot\mathbf{1}\\
0\\
-\lambda\hat{X}\\
-\lambda\hat{Y}
\end{bmatrix}\right\|_F\\
&\lesssim n^{-5},
\end{align*}
which then gives
\begin{align*}
\|\cP \nabla L(\hat{\theta},\hat{H},\hat{X},\hat{Y})\|_F
&\leq c n^{-5}+\lambda (\|\hat{X}\|_F+\|\hat{Y}\|_F)  \\
&\leq  c n^{-5}+\lambda (\|\hat{X}-X^*\|_F+\|\hat{Y}-Y^*\|_F)+ \lambda (\|X^*\|_F+\|Y^*\|_F)\\
&\lesssim \lambda \|X^{*}\|_F\\
&\lesssim \lambda\sqrt{\mu r\sigma_{\max}}
\end{align*}
as long as $\|\hat{X}-X^*\|_F\ll \|X^*\|_F$ and $n^{-5}\ll \lambda \|X^*\|_F$.
By Lemma \ref{lem:D}, we have $\lambda_{\min}(\cP \hat{D}\cP )\geq \slD/2$.
As a result, we have
\begin{align*}
 \left\|\begin{bmatrix}
\hat{\theta}^d-\hat{\theta}\\
\hat{H}^d-\hat{H}\\
\hat{X}^d-\hat{X}\\
\hat{Y}^d-\hat{Y}
\end{bmatrix}\right\|_F
\lesssim \frac{{\lambda}\sqrt{\mu r\sigma_{\max}}}{\slD}\lesssim \frac{c_{\lambda}\sqrt{\mu \sX\sY r^2}}{\slD}\sqrt{n\log n}.
\end{align*}













\subsection{Proofs of Proposition \ref{prop:bar_dist}}\label{pf:prop_bar_dist}
By \eqref{def:bar}, we have
\begin{align*}
\left\|\begin{bmatrix}
\bar{\theta}-{\theta^{*}}\\
\bar{H}-{H^{*}}\\
\bar{X}-{X^{*}}\\
\bar{Y}-{Y^{*}}
\end{bmatrix}\right\|_F
&=\|(\cP D^* \cP)^{\dagger} \cP\nabla L({\theta^{*}},{H^{*}},{X^{*}},{Y^{*}})\|_F\\
&\leq \frac{1}{\lambda_{\min}(\cP {D^{*}}\cP )}\|\cP\nabla L({\theta^{*}},{H^{*}},{X^{*}},{Y^{*}})\|_F\\
&\leq \frac{1}{\lambda_{\min}(\cP {D^{*}}\cP )}\|\nabla L({\theta^{*}},{H^{*}},{X^{*}},{Y^{*}})\|_F.
\end{align*}
By Lemma \ref{lem:gradient_norm}, we have
% \begin{align*}
% \left\|\nabla L({\theta^{*}},{H^{*}},{X^{*}},{Y^{*}})
% -
% \begin{bmatrix}
% 0\\
% 0\\
% -\lambda{X^{*}}\\
% -\lambda{Y^{*}}
% \end{bmatrix}\right\|_F
% = \|\nabla f({\theta^{*}},{H^{*}},{X^{*}},{Y^{*}})\|_F
% \lesssim \sqrt{n\log n}+\lambda   \left(\|X^{*}\|_F+\|Y^{*}\|_F\right).
% \end{align*}
% Thus, it holds that
\begin{align*}
\|\nabla L({\theta^{*}},{H^{*}},{X^{*}},{Y^{*}})\|_F
&\lesssim \sqrt{n\log n}+\sqrt{\frac{\log n}{n}} (\|{X^{*}}\|_F+\|{Y^{*}}\|_F)  \\
&\lesssim \sqrt{\mu\sX\sY r^2}\cdot\sqrt{n\log n}.
\end{align*}
Note that $\lambda_{\min}(\cP {D^{*}}\cP )\geq \slD$.
As a result, we have
\begin{align*}
 \left\|\begin{bmatrix}
\bar{\theta}-{\theta^{*}}\\
\bar{H}-{H^{*}}\\
\bar{X}-{X^{*}}\\
\bar{Y}-{Y^{*}}
\end{bmatrix}\right\|_F
\lesssim \frac{\sqrt{\mu \sX\sY r^2}}{\slD}\sqrt{n\log n}.
\end{align*}

In order to show the second part of the result, we introduce the following lemma first.
\begin{lemma}\label{concentrationlemma}
    Consider some fixed constants $a_{ij}$ for $ i\neq j\in [n]$, and random variable 
\begin{align*}
		X = \sum_{i\neq j} a_{ij}\left(\frac{e^{P_{ij}^*}}{1+e^{P_{ij}^*}}-A_{ij}\right).
\end{align*}
Then with probability at least $1-O(n^{-11})$ we have 
\begin{align*}
    |X|\lesssim \sqrt{\frac{(1+e^{c_P})^2}{e^{c_P}}\text{Var}[X]\cdot\log n}
\end{align*}
\end{lemma}
\begin{proof}
    Denote by $X_{ij} = a_{ij}(e^{P_{ij}^*}/(1+e^{P_{ij}^*})-A_{ij})$. Then we know that $\mathbb{E} X_{ij} = 0$ and $|X_{ij}|\leq a_{ij}$. Therefore, by Hoeffding inequality, with probability at least $1-O(n^{-11})$, we have
	\begin{align}
	\left|\sum_{i\neq j}X_{ij}\right|&\lesssim \left(\log n\cdot\sum_{i\neq j}a_{ij}^2\right)^{\frac{1}{2}}.\label{concentrationlemmaeq1}
	\end{align}
 On the other hand, since $A_{ij}$ are independent random variables, we know that
	\begin{align*}
		\text{Var}[X] &= \sum_{i\neq j}\text{Var}[X_{ij}]=\sum_{i\neq j}a_{ij}^2 \frac{e^{P_{ij}^*}}{(1+e^{P_{ij}^*})^2} \geq  \frac{e^{c_P}}{(1+e^{c_P})^2}\sum_{i\neq j}a_{ij}^2.
	\end{align*}
As a result, we have $\sum_{i\neq j}a_{ij}^2\lesssim e^{-c_P}(1+e^{c_P})^2 \text{Var}[X]$. Combine this with \eqref{concentrationlemmaeq1} we get
	\begin{align*}
		|X| = \left|\sum_{i\neq j}X_{ij}\right|&\lesssim \sqrt{\frac{(1+e^{c_P})^2}{e^{c_P}}\text{Var}[X]\cdot\log n}
	\end{align*}
	with probability exceeding $1-O(n^{-11})$.
\end{proof}

Let's come back to control
\begin{align*}
 \left\|\begin{bmatrix}
\bar{\theta}-{\theta^{*}}\\
\bar{X}-{X^{*}}\\
\bar{Y}-{Y^{*}}
\end{bmatrix}\right\|_{\infty}.
\end{align*}
According to the definition of $\bar{\theta},\bar{X},\bar{Y}$ from \eqref{def:bar}, we know that each entry of $\bar{\theta}-{\theta^{*}}, \bar{X}-{X^{*}}, \bar{Y}-{Y^{*}}$ can be written as linear combinations of $e^{P_{ij}^*}/(1+e^{P_{ij}^*})-A_{ij}$, since $\nabla L(\theta^*,H^*, X^*, Y^*)$ is a linear combination of $e^{P_{ij}^*}/(1+e^{P_{ij}^*})-A_{ij}$. Then by Lemma \ref{concentrationlemma}, we know that given any index $i$ we have 
\begin{align*}
    \left|\begin{bmatrix}
\bar{\theta}-{\theta^{*}}\\
\bar{X}-{X^{*}}\\
\bar{Y}-{Y^{*}}
\end{bmatrix}_i\right|\lesssim \sqrt{\frac{(1+e^{c_P})^2}{e^{c_P}}\text{Var}\left[\begin{bmatrix}
\bar{\theta}-{\theta^{*}}\\
\bar{X}-{X^{*}}\\
\bar{Y}-{Y^{*}}
\end{bmatrix}_i\right]\cdot\log n}
\end{align*}
with probability at least $1-O(n^{-11})$. Taking a union bound for all indices $i$ we know that 
\begin{align}
 \left\|\begin{bmatrix}
\bar{\theta}-{\theta^{*}}\\
\bar{X}-{X^{*}}\\
\bar{Y}-{Y^{*}}
\end{bmatrix}\right\|_{\infty}\lesssim \sqrt{\frac{(1+e^{c_P})^2}{e^{c_P}}\max_{i}\text{Var}\left[\begin{bmatrix}
\bar{\theta}-{\theta^{*}}\\
\bar{X}-{X^{*}}\\
\bar{Y}-{Y^{*}}
\end{bmatrix}_{i}\right]\cdot\log n}\label{pf:prop:bar_disteq1}
\end{align}
with probability at least $1-O(n^{-10})$. On the other hand, from \eqref{def:bar} we know that 
\begin{align*}
\text{Var}\begin{bmatrix}
\bar{\theta}-\theta^*\\
\bar{H}-H^*\\
\bar{X}-X^*\\
\bar{Y}-Y^*
\end{bmatrix}=(\cP D^*\cP)^{\dagger}.
\end{align*}
Therefore, one can see that
\begin{align*}
    \max_{i}\text{Var}\left[\begin{bmatrix}
\bar{\theta}-{\theta^{*}}\\
\bar{X}-{X^{*}}\\
\bar{Y}-{Y^{*}}
\end{bmatrix}_{i}\right]\leq \max_{i}\text{Var}\left[\begin{bmatrix}
\bar{\theta}-{\theta^{*}}\\
\bar{H}-H^* \\
\bar{X}-{X^{*}}\\
\bar{Y}-{Y^{*}}
\end{bmatrix}_{i}\right]\leq \left\|\text{Var}\begin{bmatrix}
\bar{\theta}-{\theta^{*}}\\
\bar{H}-H^* \\
\bar{X}-{X^{*}}\\
\bar{Y}-{Y^{*}}
\end{bmatrix}\right\|=\left\|(\cP D^*\cP)^{\dagger}\right\|\leq \slD^{-1}.
\end{align*}
Plugging this in \eqref{pf:prop:bar_disteq1} we get 
\begin{align*}
 \left\|\begin{bmatrix}
\bar{\theta}-{\theta^{*}}\\
\bar{X}-{X^{*}}\\
\bar{Y}-{Y^{*}}
\end{bmatrix}\right\|_{\infty}\lesssim \sqrt{\frac{(1+e^{c_P})^2}{\slD e^{c_P}}\cdot\log n}
\end{align*}
with probability at least $1-O(n^{-10})$.







\subsection{Proofs of Theorem \ref{thm:ncv_debias}}\label{pf:ncv_debias}

We first prove the following lemma.
\begin{lemma}\label{lem:debias_bar}
Under Assumption \ref{assumption:2_infty}, we have
\begin{align*}
\|\hat{\theta}^d-\bar{\theta}\|_{\infty}\leq c_{\infty}
\text{ and }
\|\hat{F}^d-\bar{F}\|_{2, \infty}\leq c_{\infty}\sqrt{r},
\end{align*}
where 
\begin{align*}
c_{\infty}\asymp \frac{\lambda\hat{c}}{\slD^2}\sqrt{\frac{\mu r\sigma_{\max}}{n}}+ \frac{c_{11}\hat{c}}{\slD}+ c_{2,\infty}c_{11}\sqrt{r^2+1}
\end{align*}
and $\hat{c}$ is defined in Lemma \ref{lem:D}.
\end{lemma}
\begin{proof}[Proof of Lemma \ref{lem:debias_bar}]
By \eqref{def:debias} and \eqref{def:bar}, we have
\begin{align}\label{ineq1:pf_debias_bar}
\begin{bmatrix}
\hat{\theta}^d-\bar{\theta}\\
\hat{H}^d-\bar{H}\\
\hat{X}^d-\bar{X}\\
\hat{Y}^d-\bar{Y}
\end{bmatrix}
&=\begin{bmatrix}
\hat{\theta}-{\theta}^*\\
\hat{H}-{H}^*\\
\hat{X}-{X}^*\\
\hat{Y}-{Y}^*
\end{bmatrix}
+\left((\cP D^*\cP)^{\dagger}-(\cP \hat{D}\cP)^{\dagger}\right)\cP\nabla L(\hat{\theta},\hat{H},\hat{X},\hat{Y})\notag\\
&\quad+ (\cP D^*\cP)^{\dagger}\cP\left(\nabla L({\theta}^*,{H}^*,{X}^*,{Y}^*)-\nabla L(\hat{\theta},\hat{H},\hat{X},\hat{Y})\right).
\end{align}
For notation simplicity, we denote
\begin{align*}
V^*:=
\begin{bmatrix}
{\theta}^*\\
{H}^*\\
{X}^*\\
{Y}^*
\end{bmatrix} \text{ and }
\hat{V}:=
\begin{bmatrix}
\hat{\theta}\\
\hat{H}\\
\hat{X}\\
\hat{Y}
\end{bmatrix}.
\end{align*}
We can further decompose the third term on the RHS of \eqref{ineq1:pf_debias_bar} as 
\begin{align*}
 &(\cP D^*\cP)^{\dagger}\cP\left(\nabla L({\theta}^*,{H}^*,{X}^*,{Y}^*)-\nabla L(\hat{\theta},\hat{H},\hat{X},\hat{Y})\right)\\
&=(\cP D^*\cP)^{\dagger}\cP\left(\int^1_0 \left(\nabla^2 L(\hat{V}+t(V^*-\hat{V}))-\nabla^2 L(V^*)\right)dt(V^*-\hat{V})\right)\\
&\quad +(\cP D^*\cP)^{\dagger}\cP\left(\nabla^2 L(V^*)-D^*\right)(V^*-\hat{V})
+\left((\cP D^*\cP)^{\dagger}(\cP D^*\cP)-I\right)(V^*-\hat{V})+(V^*-\hat{V}).
\end{align*}
Consequently, we have
\begin{align}
&\left\|
\begin{bmatrix}
\hat{\theta}^d-\bar{\theta}\\
\hat{X}^d-\bar{X}\\
\hat{Y}^d-\bar{Y}
\end{bmatrix}
\right\|_{\infty}\notag\\
&\leq 
\underbrace{\left\|\left((\cP D^*\cP)^{\dagger}-(\cP \hat{D}\cP)^{\dagger}\right)\cP\nabla L(\hat{V})\right\|_2}_{(1)}\notag\\
&\quad +
\underbrace{\left\|(\cP D^*\cP)^{\dagger}\cP\left(\int^1_0 \left(\nabla^2 L(\hat{V}+t(V^*-\hat{V}))-\nabla^2 L(V^*)\right)dt(V^*-\hat{V})\right)\right\|_2}_{(2)}\notag\\
&\quad +
\underbrace{\left\|(\cP D^*\cP)^{\dagger}\cP\left(\nabla^2 L(V^*)-D^*\right)(V^*-\hat{V})\right\|_2}_{(3)}
+
\underbrace{\left\|\left((\cP D^*\cP)^{\dagger}(\cP D^*\cP)-I\right)(V^*-\hat{V})\right\|_{\infty}}_{(4)}.
\end{align}

In the following, we bound (1)-(4), respectively.
\begin{enumerate}
\item For (1), by Theorem 3.3 in \cite{stewart1977perturbation}, we have
\begin{align*}
\|(\cP D^*\cP)^{\dagger}-(\cP \hat{D}\cP)^{\dagger}\|
&\leq \frac{1+\sqrt{5}}{2}\max\{\|(\cP\hat{D}\cP)^{\dagger}\|^2, \|(\cP D^*\cP)^{\dagger}\|^2\}\cdot \|\cP\hat{D}\cP-\cP D^*\cP\|.
\end{align*}
By Lemma \ref{lem:D}, we have
\begin{align*}
\max\{\|(\cP\hat{D}\cP)^{\dagger}\|^2, \|(\cP D^*\cP)^{\dagger}\|^2\}\lesssim \frac{1}{\slD^2}, \quad
\|\cP\hat{D}\cP-\cP D^*\cP\|\lesssim  \frac{\hat{c}}{\sqrt{n}}.
\end{align*}
Thus, we obtain
\begin{align*}
\|(\cP D^*\cP)^{\dagger}-(\cP \hat{D}\cP)^{\dagger}\|\lesssim \frac{\hat{c}}{\slD^2\sqrt{n}}.
\end{align*}
Further, as shown in the proof of Proposition \ref{prop:debias_dist}, we have
\begin{align*}
\|\cP\nabla L(\hat{V})\|_F\lesssim\lambda\sqrt{\mu r\sigma_{\max}}.
\end{align*}
Consequently, we have
\begin{align*}
(1)\leq \|(\cP D^*\cP)^{\dagger}-(\cP \hat{D}\cP)^{\dagger}\|\|\cP\nabla L(\hat{V})\|_F\lesssim \frac{\lambda\hat{c}}{\slD^2}\sqrt{\frac{\mu r\sigma_{\max}}{n}}.
\end{align*}

\item  We then bound (2). Denote $V^t=\hat{V}+t(V^*-\hat{V})$ and define $D^t$ correspondingly. Following the same argument as in the proof of Lemma \ref{lem:D}, we have
\begin{align*}
\|\cP D^{t}\cP-\cP D^* \cP\|\lesssim  \frac{\hat{c}}{\sqrt{n}}.
\end{align*}
Further, as already being shown in the proof of Lemma \ref{lem:convexity},
we have
\begin{align*}
\|\nabla^2 L(V^t)-D^t\|\lesssim   \frac{\sqrt{\su}}{n}\cdot\left(\|\hat{\theta}-\theta^{*}\|_{2}+\|\hat{H}-H^{*}\|_{F}+\frac{1}{n}\|X^*\|\|\hat{F}-F^*\|_{F}\right)\lesssim \frac{c_{11}}{\sqrt{n}}
\end{align*}
and
\begin{align*}
 \|\nabla^2 L(V^*)-D^*\|\lesssim \frac{\sqrt{\log n}}{n}.
\end{align*}
Consequently, we have for all $t\in [0,1]$
\begin{align*}
&\left\|\cP\left(\nabla^2 L(\hat{V}+t(V^*-\hat{V}))-\nabla^2 L(V^*)\right)\cP\right\|\\
&\leq \|\nabla^2 L(V^t)-D^t\|+\|\cP D^{t}\cP-\cP D^* \cP\|+ \|\nabla^2 L(V^*)-D^*\|\lesssim \frac{\hat{c}}{\sqrt{n}}.
\end{align*}
Thus, we have
\begin{align*}
(2)\lesssim \frac{\hat{c}}{\sqrt{n}}\|(\cP D^*\cP)^{\dagger}\|\|V^*-\hat{V}\|_F\leq  \frac{c_{11}\hat{c}}{\slD} .
\end{align*}

\item For (3), we have
\begin{align*}
(3)\leq \|(\cP D^*\cP)^{\dagger}\|\|\nabla^2 L(V^*)-D^*\|\|V^*-\hat{V}\|_F \lesssim \frac{1}{\slD}\cdot \frac{\sqrt{\log n}}{n} \cdot c_{11}\sqrt{n}=\frac{c_{11}}{\slD}\sqrt{\frac{\log n}{n}}.
\end{align*}


\item Finally, for (4), we have
\begin{align*}
(4)\leq \left\|I-(\cP D^*\cP)^{\dagger}(\cP D^*\cP)\right\|_{2\infty}\|V^*-\hat{V}\|_F\leq c_{2,\infty}c_{11}\sqrt{r^2+1},
\end{align*}
where the last inequality follows from Assumption \ref{assumption:2_infty}.

\end{enumerate}

Combine the bounds for (1)-(4), we have
\begin{align*}
&\left\|
\begin{bmatrix}
\hat{\theta}^d-\bar{\theta}\\
\hat{X}^d-\bar{X}\\
\hat{Y}^d-\bar{Y}
\end{bmatrix}
\right\|_{\infty}
\lesssim
\frac{\lambda\hat{c}}{\slD^2}\sqrt{\frac{\mu r\sigma_{\max}}{n}}+ \frac{c_{11}\hat{c}}{\slD}+ c_{2,\infty}c_{11}\sqrt{r^2+1}=c_{\infty}.
\end{align*}
Consequently, it holds that
\begin{align*}
\|\hat{\theta}^d-\bar{\theta}\|_{\infty}\lesssim c_{\infty}
\text{ and }
\|\hat{F}^d-\bar{F}\|_{2,\infty}\leq \sqrt{r}\|\hat{F}^d-\bar{F}\|_{\infty}\lesssim c_{\infty} \sqrt{r}.
\end{align*}
We then finish the proofs.
\end{proof}


With Lemma \ref{lem:debias_bar} in hand, we then prove Theorem \ref{thm:ncv_debias} in the following.
\begin{proof}[Proof of Theorem \ref{thm:ncv_debias}]
    

For notation simplicity, we denote $V:=\begin{bmatrix}
\theta\\
H\\
X\\
Y
\end{bmatrix}$ and $c(V):=\begin{bmatrix}
\theta\\
H\\
XY^T
\end{bmatrix}$, which is the convex counterpart of $V$. 
We denote
\begin{align*}
&\Delta
=\begin{bmatrix}
\Delta_{\theta}\\
\Delta_{H}\\
\Delta_{\Gamma}
\end{bmatrix}
:=c(\bar{V})-c(\hat{V}^d),\ 
\begin{bmatrix}
\Delta_X\\
\Delta_Y
\end{bmatrix}
:=\begin{bmatrix}
\bar{X}-\hat{X}^d\\
\bar{Y}-\hat{Y}^d
\end{bmatrix},\\
&\Delta'
=\begin{bmatrix}
\Delta'_{\theta}\\
\Delta'_{H}\\
\Delta'_{\Gamma}
\end{bmatrix}
:=c(\hat{V}^d)-c(V^*),\ 
\begin{bmatrix}
\Delta'_X\\
\Delta'_Y
\end{bmatrix}
=\begin{bmatrix}
\hat{X}^d-X^*\\
\hat{Y}^d-Y^*
\end{bmatrix},\\
&\Delta^{''}
=\begin{bmatrix}
\Delta''_{\theta}\\
\Delta''_{H}\\
\Delta''_{\Gamma}
\end{bmatrix}
:=c(\bar{V})-c(\hat{V}),\ 
\begin{bmatrix}
\Delta''_X\\
\Delta''_Y
\end{bmatrix}
=\begin{bmatrix}
\bar{X}-\hat{X}\\
\bar{Y}-\hat{Y}
\end{bmatrix},\\
&\Delta^{'''}
=\begin{bmatrix}
\Delta^{'''}_{\theta}\\
\Delta^{'''}_{H}\\
\Delta^{'''}_{\Gamma}
\end{bmatrix}
:=c(\bar{V})-c(V^*),\ 
\begin{bmatrix}
\Delta'''_X\\
\Delta'''_Y
\end{bmatrix}
=\begin{bmatrix}
\bar{X}-X^*\\
\bar{Y}-Y^*
\end{bmatrix},\\
&\hat{\Delta}
=\begin{bmatrix}
\hat{\Delta}_{\theta}\\
\hat{\Delta}_{H}\\
\hat{\Delta}_{\Gamma}
\end{bmatrix}
:=c(\hat{V}^d)-c(\hat{V}),\ 
\begin{bmatrix}
\hat{\Delta}_X\\
\hat{\Delta}_Y
\end{bmatrix}
=\begin{bmatrix}
\hat{X}^d-\hat{X}\\
\hat{Y}^d-\hat{Y}
\end{bmatrix},
\end{align*}
which will be used in the following proofs.
By Proposition \ref{prop:debias_dist}, Proposition \ref{prop:bar_dist} and Lemma \ref{lem:ncv1}, all the \( l_2 \)-norms related to \(\theta\) (e.g., \(\|\Delta_{\theta}\|_2\)) and all the Frobenius norms related to \(H, X, Y\) (e.g., \(\|\Delta_H\|_F\), \(\|\Delta_X\|_F\), \(\|\Delta_Y\|_F\)) are bounded by $(c_a+c_{11})\sqrt{n}$. Additionally, all the Frobenius norms related to \(\Gamma\) (e.g., \(\|\Delta_{\Gamma}\|_F\)) are bounded by $(c_a+c_{11}) \sqrt{\mu r\sigma_{\max}n}$.
% We denote
% \begin{align*}
% &\Delta
% =\begin{bmatrix}
% \Delta_{\theta}\\
% \Delta_{H}\\
% \Delta_{\Gamma}
% \end{bmatrix}
% :=c(\bar{V})-c(\hat{V}^d)
% =\begin{bmatrix}
% \bar{\theta}-\hat{\theta}^d\\
% \bar{H}-\hat{H}^d\\
% \bar{X}\bar{Y}^T-\hat{X}^d(\hat{Y}^{d})^T
% \end{bmatrix},\\
% &\Delta'
% =\begin{bmatrix}
% \Delta'_{\theta}\\
% \Delta'_{H}\\
% \Delta'_{\Gamma}
% \end{bmatrix}
% :=c(\hat{V}^d)-c(V^*)
% =\begin{bmatrix}
% \hat{\theta}^d-\theta^*\\
% \hat{H}^d-H^*\\
% \hat{X}^d(\hat{Y}^{d})^T-X^*Y^{*T}
% \end{bmatrix},\\
% &\Delta^{''}
% =\begin{bmatrix}
% \Delta''_{\theta}\\
% \Delta''_{H}\\
% \Delta''_{\Gamma}
% \end{bmatrix}
% :=c(\bar{V})-c(\hat{V})
% =\begin{bmatrix}
% \bar{\theta}-\hat{\theta}\\
% \bar{H}-\hat{H}\\
% \bar{X}\bar{Y}^T-\hat{X}\hat{Y}^T
% \end{bmatrix},\\
% &\Delta^{'''}
% =\begin{bmatrix}
% \Delta^{'''}_{\theta}\\
% \Delta^{'''}_{H}\\
% \Delta^{'''}_{\Gamma}
% \end{bmatrix}
% :=c(\bar{V})-c(V^*)
% =\begin{bmatrix}
% \bar{\theta}-\theta^*\\
% \bar{H}-H^*\\
% \bar{X}\bar{Y}^T-X^*Y^{*T}
% \end{bmatrix},\\
% &\hat{\Delta}
% =\begin{bmatrix}
% \hat{\Delta}_{\theta}\\
% \hat{\Delta}_{H}\\
% \hat{\Delta}_{\Gamma}
% \end{bmatrix}
% :=c(\hat{V}^d)-c(\hat{V})
% =\begin{bmatrix}
% \hat{\theta}^d-\hat{\theta}\\
% \hat{H}^d-\hat{H}\\
% \hat{X}^d(\hat{Y}^{d})^T-\hat{X}\hat{Y}^T
% \end{bmatrix}
% \end{align*}


% By the definition of $\bar{V}$, we have
% \begin{align}\label{eq1:pf_debias}
% Q^*\left(\nabla L(V^*)+D^*\left(\bar{V}-V^*\right)\right)=0.
% \end{align}
We define the quadratic approximation of the convex loss (defined in \eqref{obj:cv_loss}) as
\begin{align*}
\bar{L}_c\left(c(V)\right)
:={L}_c\left(c(V^*)\right)+\nabla {L}_c\left(c(V^*)\right)\left(c(V)-c(V^*)\right)+\frac12 \left(c(V)-c(V^*)\right)^T\nabla^2 {L}_c\left(c(V^*)\right)\left(c(V)-c(V^*)\right),
\end{align*}
which implies for all $V$
\begin{align}\label{eq2:pf_debias}
\nabla\bar{L}_c\left(c(V)\right)=\nabla {L}_c\left(c(V^*)\right)+\nabla^2 {L}_c\left(c(V^*)\right)\left(c(V)-c(V^*)\right).
\end{align}
Note that
\begin{align*}
\nabla L_c(c(\hat{V}^d))
&=\nabla L_c(c({V}^*))+\int^1_{0}\nabla^2L_c\left(c({V}^*)+t(c(\hat{V}^d)-c({V}^*))\right)(c(\hat{V}^d)-c({V}^*)) dt\\
&=\nabla\bar{L}_c\left(c(\bar{V})\right)-\nabla^2 {L}_c\left(c(V^*)\right)\left(c(\bar{V})-c(V^*)\right)\\
&\quad+\int^1_{0}\nabla^2L_c\left(c({V}^*)+t(c(\hat{V}^d)-c({V}^*))\right)(c(\hat{V}^d)-c({V}^*)) dt,
\end{align*}
where the second equation follows from \eqref{eq2:pf_debias} with $V=\bar{V}$. Rearranging the terms gives
\begin{align*}
&\nabla^2 {L}_c\left(c(V^*)\right)\left(c(\bar{V})-c(\hat{V}^d)\right)\\
&= \int^1_{0}\left(\nabla^2L_c\left(c({V}^*)+t(c(\hat{V}^d)-c({V}^*))\right)-\nabla^2 L_c(c(V^*))\right)dt(c(\hat{V}^d)-c({V}^*)) \\
&\quad-\nabla L_c(c(\hat{V}^d))+   \nabla\bar{L}_c\left(c(\bar{V})\right).
\end{align*}
By multiplying both sides with $c(\bar{V})-c(\hat{V}^d)$, we have
\begin{align}\label{eq3:pf_debias}
 &\left(c(\bar{V})-c(\hat{V}^d)\right)^T \nabla^2{L}_c\left(c(V^*)\right)\left(c(\bar{V})-c(\hat{V}^d)\right)\notag\\
 &= \underbrace{\left(c(\bar{V})-c(\hat{V}^d)\right)^T\left(\int^1_{0}\nabla^2L_c\left(c({V}^*)+t(c(\hat{V}^d)-c({V}^*))\right)-\nabla^2 L_c(c(V^*))dt\right)(c(\hat{V}^d)-c({V}^*))}_{(1)}\notag\\
&\quad-\underbrace{\nabla L_c(c(\hat{V}^d))^T\left(c(\bar{V})-c(\hat{V}^d)\right)}_{(2)}+   \underbrace{\nabla\bar{L}_c\left(c(\bar{V})\right)^T\left(c(\bar{V})-c(\hat{V}^d)\right)}_{(3)}.   
\end{align}
For the LHS of \eqref{eq3:pf_debias}, we have
\begin{align}
 &\left(c(\bar{V})-c(\hat{V}^d)\right)^T \nabla^2{L}_c\left(c(V^*)\right)\left(c(\bar{V})-c(\hat{V}^d)\right)\notag\\
&=\sum_{i\neq j}\frac{e^{P_{ij}^*}}{(1+e^{P_{ij}^*})^2}\left(\frac{1}{\sqrt{n}}\langle\Delta_{\theta},e_i+e_j\rangle+\langle\Delta_{H},z_iz_j^T\rangle+\frac1n\langle \Delta_{\Gamma},e_i e_j^T\rangle\right)^2\notag\\
&\geq \frac{e^{c_P}}{(1+e^{c_P})^2} \sum_{i\neq j}\left(\frac{1}{\sqrt{n}}\langle\Delta_{\theta},e_i+e_j\rangle+\langle\Delta_{H},z_iz_j^T\rangle+\frac1n\langle \Delta_{\Gamma},e_i e_j^T\rangle\right)^2\notag\\
&=\frac{e^{c_P}}{(1+e^{c_P})^2} 
\begin{bmatrix}
  \vec(\Delta_{\theta})\\
  \vec(\Delta_{H})\\
  \frac1n\vec(\Delta_{\Gamma})
\end{bmatrix}^T
\left(\sum_{i\neq j}
  \begin{bmatrix}
  \frac{1}{\sqrt{n}}\vec(e_i+e_j)\\
  \vec(z_iz_j^T)\\
  \vec(e_ie_j^T)
  \end{bmatrix}
   \begin{bmatrix}
  \frac{1}{\sqrt{n}}\vec(e_i+e_j)\\
  \vec(z_iz_j^T)\\
  \vec(e_ie_j^T)
  \end{bmatrix}^T
\right)
\begin{bmatrix}
  \vec(\Delta_{\theta})\\
  \vec(\Delta_{H})\\
  \frac1n\vec(\Delta_{\Gamma})
\end{bmatrix}\notag\\
&\geq\frac{\sl e^{c_P}}{(1+e^{c_P})^2}  \left\|\begin{bmatrix}
  \vec(\Delta_{\theta})\\
  \vec(\Delta_{H})\\
  \frac1n\vec(\Delta_{\Gamma})
\end{bmatrix}\right\|^2 \tag{by Assumption \ref{assumption:eigenvalues} and $\mathbf{1}^T\Delta_{\theta}=0$}\\\label{eq26:pf_debias}
& =\frac{\sl e^{c_P}}{(1+e^{c_P})^2}  \left(\|\Delta_{\theta}\|^2_{2}+\|\Delta_{H}\|^2_{F}+\frac{1}{n^2}\|\Delta_{\Gamma}\|^2_{F}\right).
\end{align}
For the RHS, we will bound (1), (2) and (3), respectively.
\begin{enumerate}
\item We first bound (1). We denote
\begin{align*}
\begin{bmatrix}
\theta^t\\
H^t\\
\Gamma^t
\end{bmatrix}
:=c({V}^*)+t(c(\hat{V}^d)-c({V}^*)),\ 
P_{ij}^t:=\frac{\theta_i^t+\theta_j^t}{\sqrt{n}}+z_i^TH^tz_j+\frac{\Gamma^t_{ij}}{n}.
\end{align*}
It then holds that
\begin{align*}
 &\nabla^2L_c\left(c({V}^*)+t(c(\hat{V}^d)-c({V}^*))\right)-\nabla^2 L_c(c(V^*))\\
 &=\sum_{i\neq j}\left(\frac{e^{P_{ij}^t}}{(1+e^{P_{ij}^t})^2}-\frac{e^{P_{ij}^*}}{(1+e^{P_{ij}^*})^2}\right)
   \begin{bmatrix}
  \frac{1}{\sqrt{n}}\vec(e_i+e_j)\\
  \vec(z_iz_j^T)\\
  \frac1n\vec(e_ie_j^T)
  \end{bmatrix}^{\otimes 2}.
\end{align*}
Thus, we have
\begin{align*}
&\left(c(\bar{V})-c(\hat{V}^d)\right)^T\left(\nabla^2L_c\left(c({V}^*)+t(c(\hat{V}^d)-c({V}^*))\right)-\nabla^2 L_c(c(V^*))\right)(c(\hat{V}^d)-c({V}^*))\\
&=
\begin{bmatrix}
\vec(\Delta'_{\theta})\\
\vec(\Delta'_{H})\\
\vec(\frac1n \Delta'_{\Gamma})
\end{bmatrix}^T\left(\sum_{i\neq j}\left(\frac{e^{P_{ij}^t}}{(1+e^{P_{ij}^t})^2}-\frac{e^{P_{ij}^*}}{(1+e^{P_{ij}^*})^2}\right)
\cP_c
   \begin{bmatrix}
  \frac{1}{\sqrt{n}}\vec(e_i+e_j)\\
  \vec(z_iz_j^T)\\
  \vec(e_ie_j^T)
  \end{bmatrix}^{\otimes 2}\cP_c
  \right)
  \begin{bmatrix}
\vec(\Delta_{\theta})\\
\vec(\Delta_{H})\\
\vec(\frac1n \Delta_{\Gamma})
\end{bmatrix}.
\end{align*}
Note that
\begin{align*}
&\left\|\sum_{i\neq j}\left(\frac{e^{P_{ij}^t}}{(1+e^{P_{ij}^t})^2}-\frac{e^{P_{ij}^*}}{(1+e^{P_{ij}^*})^2}\right)\cP_c
   \begin{bmatrix}
  \frac{1}{\sqrt{n}}\vec(e_i+e_j)\\
  \vec(z_iz_j^T)\\
  \vec(e_ie_j^T)
  \end{bmatrix}^{\otimes 2}\cP_c\right\|\\
&\leq
\left\|\sum_{i\neq j}\left|\frac{e^{P_{ij}^t}}{(1+e^{P_{ij}^t})^2}-\frac{e^{P_{ij}^*}}{(1+e^{P_{ij}^*})^2}\right|
  \cP_c
   \begin{bmatrix}
  \frac{1}{\sqrt{n}}\vec(e_i+e_j)\\
  \vec(z_iz_j^T)\\
  \vec(e_ie_j^T)
  \end{bmatrix}^{\otimes 2}\cP_c\right\|\\
&\leq \frac14
\left\|\sum_{i\neq j}\left|P_{ij}^t-P_{ij}^*\right|
   \cP_c
   \begin{bmatrix}
  \frac{1}{\sqrt{n}}\vec(e_i+e_j)\\
  \vec(z_iz_j^T)\\
  \vec(e_ie_j^T)
  \end{bmatrix}^{\otimes 2}\cP_c\right\|\tag{mean-value theorem}\\
&\leq \max_{i\neq j}\left|P_{ij}^t-P_{ij}^*\right|\cdot \left\|\sum_{i\neq j}\cP_c
\begin{bmatrix}
  \frac{1}{\sqrt{n}}\vec(e_i+e_j)\\
  \vec(z_iz_j^T)\\
  \vec(e_ie_j^T)
  \end{bmatrix}
  \begin{bmatrix}
  \frac{1}{\sqrt{n}}\vec(e_i+e_j)\\
  \vec(z_iz_j^T)\\
  \vec(e_ie_j^T)
\end{bmatrix}^T\cP_c\right\|\\
&\leq\su\max_{i\neq j}\left|P_{ij}^t-P_{ij}^*\right|.
\end{align*}
By the definition of $P^t_{ij}$, we have
\begin{align*}
\max_{i\neq j}\left|P_{ij}^t-P_{ij}^*\right|
&\leq \frac{2}{\sqrt{n}}\|\theta^t-\theta^*\|_{\infty}+  (\max_{i\neq j}\|z_i\|\|z_j\|  )\cdot\|H^t-H^*\|_{F}+\frac1n \|\Gamma^t-\Gamma^*\|_{\infty}\\
&\leq  \frac{2}{\sqrt{n}}\|\theta^t-\theta^*\|_{\infty}+  \frac{\sz}{n}\|H^t-H^*\|_{F}+\frac1n \|\Gamma^t-\Gamma^*\|_{\infty}\\
&\leq \frac{2}{\sqrt{n}}\|\hat{\theta}^d-\theta^*\|_{\infty}+  \frac{\sz}{n}\|\hat{H}^d-H^*\|_{F}+\frac1n \|\hat{\Gamma}^d-\Gamma^*\|_{\infty},
\end{align*}
where the last inequality follows from the definition of $\theta^t,H^t,\Gamma^t$. Moreover, notice that
\begin{align*}
\|\hat{\Gamma}^d-\Gamma^*\|_{\infty}    
&=\|(\hat{X}^d-X^*)(\hat{Y}^d)^T+X^{*}(\hat{Y}^d-Y^*)^T\|_{\infty}\\
&\leq \|\hat{X}^d-X^*\|_{2,\infty}\|\hat{Y}^d\|_{2,\infty}+\|X^{*}\|_{2,\infty}\|\hat{Y}^d-Y^*\|_{2,\infty},
\end{align*}
where $\|\hat{Y}^d\|_{2,\infty}\leq \|\hat{Y}^d-\bar{Y}\|_{2,\infty}+\|\bar{Y}-{Y}^*\|_{2,\infty}+\|{Y}^*\|_{2,\infty}\leq 3\|{Y}^*\|_{2,\infty}$. Thus, we have
\begin{align*}
\|\hat{\Gamma}^d-\Gamma^*\|_{\infty} \leq 4\|F^{*}\|_{2,\infty}\|\hat{F}^d-F^*\|_{2,\infty}
\end{align*}
and 
\begin{align*}
\max_{i\neq j}\left|P_{ij}^t-P_{ij}^*\right|
&\lesssim \frac{1}{\sqrt{n}}\|\hat{\theta}^d-\theta^*\|_{\infty}+   \frac{\sz}{n}\|\hat{H}^d-H^*\|_{F}+\frac1n\|F^{*}\|_{2,\infty}\|\hat{F}^d-F^*\|_{2,\infty}\\
&\lesssim\frac{1}{\sqrt{n}}(\|\hat{\theta}^d-\bar{\theta}\|_{\infty}+\|\bar{\theta}-\theta^*\|_{\infty})+   \frac{\sz}{n}(\|\hat{H}^d-\hat{H}\|_{F}+\|\hat{H}-H^*\|_{F})\\
&\quad+\frac1n\|F^{*}\|_{2,\infty}(\|\hat{F}^d-\bar{F}\|_{2,\infty}+\|\bar{F}-F^*\|_{2,\infty})\\
% &\lesssim\frac{1}{\sqrt{n}}\|\hat{\theta}-\theta^*\|_{\infty}+   \frac{\sz}{n}\|\hat{H}-H^*\|_{F}+\frac1n\|F^{*}\|_{2,\infty}\|\hat{F}-F^*\|_{2,\infty}\tag{\ntc}\\
% &\lesssim\frac{c_{41}+\sz c_{11}+\sqrt{\mu\sX\sY r^2}c_{43}}{\sqrt{n}}\tag{by \eqref{ncv:est}, \ntc}.
&\lesssim\frac{c_{\infty}+c_b+\sz (c_{11}+c_a)+\sqrt{\mu\sX\sY r^3}(c_{\infty}+c_b)}{\sqrt{n}}\\
&\lesssim\frac{\sqrt{\mu\sX\sY r^3}(c_{\infty}+c_b)}{\sqrt{n}},
\end{align*}
where the third inequality follows from Lemma \ref{lem:debias_bar}, Proposition \ref{prop:debias_dist}, Proposition \ref{prop:bar_dist} and Lemma \ref{lem:ncv1}.
Consequently, we have
\begin{align*}
& \left\|\sum_{i\neq j}\left(\frac{e^{P_{ij}^t}}{(1+e^{P_{ij}^t})^2}-\frac{e^{P_{ij}^*}}{(1+e^{P_{ij}^*})^2}\right)
   \begin{bmatrix}
  \frac{1}{\sqrt{n}}\vec(e_i+e_j)\\
  \vec(z_iz_j^T)\\
  \vec(e_ie_j^T)
  \end{bmatrix}
  \begin{bmatrix}
  \frac{1}{\sqrt{n}}\vec(e_i+e_j)\\
  \vec(z_iz_j^T)\\
  \vec(e_ie_j^T)
  \end{bmatrix}^T\right\| \\
&\lesssim \su\cdot  \frac{\sqrt{\mu\sX\sY r^3}(c_{\infty}+c_b)}{\sqrt{n}}
\end{align*}
and for all $t\in [0,1]$
\begin{align*}
  &\left|\left(c(\bar{V})-c(\hat{V}^d)\right)^T\left(\nabla^2L_c\left(c({V}^*)+t(c(\hat{V}^d)-c({V}^*))\right)-\nabla^2 L_c(c(V^*))\right)(c(\hat{V}^d)-c({V}^*))\right|\\
  &\lesssim\su\cdot  \frac{\sqrt{\mu\sX\sY r^3}(c_{\infty}+c_b)}{\sqrt{n}}\sqrt{\|\Delta_{\theta}\|^2_2+\|\Delta_{H}\|^2_F+\frac{1}{n^2}\|\Delta_{\Gamma}\|^2_F}  \cdot\sqrt{\|\Delta'_{\theta}\|^2_2+\|\Delta'_{H}\|^2_F+\frac{1}{n^2}\|\Delta'_{\Gamma}\|^2_F}  .
\end{align*}
As a result, we obtain
\begin{align*}
|(1)|\lesssim\frac{C_1}{\sqrt{n}}\sqrt{\|\Delta_{\theta}\|^2_2+\|\Delta_{H}\|^2_F+\frac{1}{n^2}\|\Delta_{\Gamma}\|^2_F}  \cdot\sqrt{\|\Delta'_{\theta}\|^2_2+\|\Delta'_{H}\|^2_F+\frac{1}{n^2}\|\Delta'_{\Gamma}\|^2_F} ,
\end{align*}
where $C_1:= \su\sqrt{\mu\sX\sY r^3}(c_{\infty}+c_b)$.



\item We then bound (2).
Note that
\begin{align}\label{eq4:pf_debias}
&\nabla L_c(c(\hat{V}^d))^T\left(c(\bar{V})-c(\hat{V}^d)\right)\notag\\
&=\nabla L_c(c(\hat{V}))^T \left(c(\bar{V})-c(\hat{V}^d)\right)\notag\\
&\quad+\left(c(\bar{V})-c(\hat{V}^d)\right)^T\int^1_0\nabla^2 L_c\left(c(\hat{V})+t(c(\hat{V}^d)-c(\hat{V}))\right)dt \left(c(\hat{V}^d)-c(\hat{V})\right).
\end{align}
For the first term, recall the definition of $\Delta''$, we have
\begin{align*}
&\nabla L_c(c(\hat{V}))^T \left(c(\bar{V})-c(\hat{V})\right)\\
&=\sum_{i\neq j}\left(\frac{e^{\hat{P}_{ij}}}{1+e^{\hat{P}_{ij}}}-A_{ij}\right)\left(\frac{1}{\sqrt{n}}\langle\Delta''_{\theta},e_i+e_j\rangle+\langle\Delta''_{H},z_iz_j^T\rangle+\frac1n\langle \bar{X}\bar{Y}^T-\hat{X}\hat{Y}^T,e_i e_j^T\rangle\right).
\end{align*}
Note that
\begin{align*}
\langle \bar{X}\bar{Y}^T-\hat{X}\hat{Y}^T,e_i e_j^T\rangle=\langle \Delta''_X\hat{Y}^T+\hat{X}\Delta^{''T}_Y,e_i e_j^T\rangle+\langle \Delta''_X\Delta^{''T}_Y,e_i e_j^T\rangle.
\end{align*}
Thus we have
\begin{align}\label{eq6:pf_debias}
 &L_c(c(\hat{V}))^T \left(c(\bar{V})-c(\hat{V})\right)   \notag\\
 &=\sum_{i\neq j}\left(\frac{e^{\hat{P}_{ij}}}{1+e^{\hat{P}_{ij}}}-A_{ij}\right)\left(\frac{1}{\sqrt{n}}\langle\Delta''_{\theta},e_i+e_j\rangle+\langle\Delta''_{H},z_iz_j^T\rangle+\frac1n\langle \Delta''_X,e_i e_j^T\hat{Y}\rangle+\frac1n\langle \Delta^{''}_Y,e_j e_i^T\hat{X}\rangle\right) \notag\\
 &\quad + \frac1n\sum_{i\neq j}\left(\frac{e^{\hat{P}_{ij}}}{1+e^{\hat{P}_{ij}}}-A_{ij}\right)\langle \Delta''_X\Delta^{''T}_Y,e_i e_j^T\rangle \notag\\
 &=\nabla L(\hat{V})^T(\bar{V}-\hat{V}) + \frac1n\sum_{i\neq j}\left(\frac{e^{\hat{P}_{ij}}}{1+e^{\hat{P}_{ij}}}-A_{ij}\right)\langle \Delta''_X\Delta^{''T}_Y,e_i e_j^T\rangle.
\end{align}
By \eqref{property:debias}, we have 
\begin{align*}
\cP \nabla L(\hat{V})=-\cP \left(\sum_{i\neq j}\frac{e^{\hat{P}_{ij}}}{(1+e^{\hat{P}_{ij}})^2}
\begin{bmatrix}
\frac{1}{\sqrt{n}}(e_i+e_j)\\
z_iz_j^T\\
\frac1ne_ie_j^T\hat{Y}\\
\frac1ne_je_i^T\hat{X}
\end{bmatrix}^{\otimes 2}\right)(\hat{V}^d-\hat{V}).
\end{align*}
Moreover, note that $\cP(\bar{V})=\bar{V}, \cP(\hat{V})=\hat{V}, \cP(\hat{V}^d)=\hat{V}^d$.
Thus, it holds that
\begin{align*}
&\nabla L(\hat{V})^T(\bar{V}-\hat{V})\\
& = \left(\cP\nabla L(\hat{V}) \right)^T(\bar{V}-\hat{V})\\
&=-(\bar{V}-\hat{V})^T\left(\sum_{i\neq j}\frac{e^{\hat{P}_{ij}}}{(1+e^{\hat{P}_{ij}})^2}
\begin{bmatrix}
\frac{1}{\sqrt{n}}(e_i+e_j)\\
z_iz_j^T\\
\frac1ne_ie_j^T\hat{Y}\\
\frac1ne_je_i^T\hat{X}
\end{bmatrix}^{\otimes 2}\right)(\hat{V}^d-\hat{V})\\
&=-\sum_{i\neq j}\frac{e^{\hat{P}_{ij}}}{(1+e^{\hat{P}_{ij}})^2}\cdot\left(\frac{1}{\sqrt{n}}\langle\Delta''_{\theta},e_i+e_j\rangle+\langle\Delta''_{H},z_iz_j^T\rangle+\frac1n\langle \Delta''_X\hat{Y}^T+\hat{X}\Delta^{''T}_Y,e_i e_j^T\rangle\right)\\
&\qquad\qquad\cdot \left(\frac{1}{\sqrt{n}}\langle\hat{\Delta}_{\theta},e_i+e_j\rangle+\langle\hat{\Delta}_{H},z_iz_j^T\rangle+\frac1n\langle \hat{\Delta}_X\hat{Y}^T+\hat{X}\hat{\Delta}^{T}_Y,e_i e_j^T\rangle\right)\\
&=-\sum_{i\neq j}\frac{e^{\hat{P}_{ij}}}{(1+e^{\hat{P}_{ij}})^2}\cdot\left(\frac{1}{\sqrt{n}}\langle\Delta''_{\theta},e_i+e_j\rangle+\langle\Delta''_{H},z_iz_j^T\rangle+\frac1n\langle\bar{X}\bar{Y}^T-\hat{X}\hat{Y}^T,e_i e_j^T\rangle-\frac1n \langle \Delta''_X\Delta^{''T}_Y,e_i e_j^T\rangle\right)\\
&\qquad\qquad\cdot \left(\frac{1}{\sqrt{n}}\langle\hat{\Delta}_{\theta},e_i+e_j\rangle+\langle\hat{\Delta}_{H},z_iz_j^T\rangle+\frac1n\langle\hat{X}^d\hat{Y}^{dT}-\hat{X}\hat{Y}^T,e_i e_j^T\rangle-\frac1n \langle \hat{\Delta}_X\hat{\Delta}^{T}_Y,e_i e_j^T\rangle\right)\\
&=-\sum_{i\neq j}\frac{e^{\hat{P}_{ij}}}{(1+e^{\hat{P}_{ij}})^2}\cdot\left(\frac{1}{\sqrt{n}}\langle\Delta''_{\theta},e_i+e_j\rangle+\langle\Delta''_{H},z_iz_j^T\rangle+\frac1n\langle\bar{X}\bar{Y}^T-\hat{X}\hat{Y}^T,e_i e_j^T\rangle\right)\\
&\qquad\qquad\cdot \left(\frac{1}{\sqrt{n}}\langle\hat{\Delta}_{\theta},e_i+e_j\rangle+\langle\hat{\Delta}_{H},z_iz_j^T\rangle+\frac1n\langle\hat{X}^d\hat{Y}^{dT}-\hat{X}\hat{Y}^T,e_i e_j^T\rangle\right)\\
&\quad+\frac1n\sum_{i\neq j}\frac{e^{\hat{P}_{ij}}}{(1+e^{\hat{P}_{ij}})^2}\cdot\left(\frac{1}{\sqrt{n}}\langle\Delta''_{\theta},e_i+e_j\rangle+\langle\Delta''_{H},z_iz_j^T\rangle+\frac1n\langle\bar{X}\bar{Y}^T-\hat{X}\hat{Y}^T,e_i e_j^T\rangle\right)\langle \hat{\Delta}_X\hat{\Delta}^{T}_Y,e_i e_j^T\rangle\\
&\quad+\frac1n\sum_{i\neq j}\frac{e^{\hat{P}_{ij}}}{(1+e^{\hat{P}_{ij}})^2}\cdot\left(\frac{1}{\sqrt{n}}\langle\hat{\Delta}_{\theta},e_i+e_j\rangle+\langle\hat{\Delta}_{H},z_iz_j^T\rangle+\frac1n\langle\hat{X}^d\hat{Y}^{dT}-\hat{X}\hat{Y}^T,e_i e_j^T\rangle\right)\langle \Delta''_X\Delta^{''T}_Y,e_i e_j^T\rangle\\
&\quad -\frac{1}{n^2}\sum_{i\neq j}\frac{e^{\hat{P}_{ij}}}{(1+e^{\hat{P}_{ij}})^2}\langle \hat{\Delta}_X\hat{\Delta}^{T}_Y,e_i e_j^T\rangle \langle \Delta''_X\Delta^{''T}_Y,e_i e_j^T\rangle\\
&=-\left(c(\bar{V})-c(\hat{V})\right)^T\nabla^2L_c(c(\hat{V})) \left(c(\hat{V}^d)-c(\hat{V})\right)\\
&\quad+\frac1n\sum_{i\neq j}\frac{e^{\hat{P}_{ij}}}{(1+e^{\hat{P}_{ij}})^2}\cdot\left(\frac{1}{\sqrt{n}}\langle\Delta''_{\theta},e_i+e_j\rangle+\langle\Delta''_{H},z_iz_j^T\rangle+\frac1n\langle\bar{X}\bar{Y}^T-\hat{X}\hat{Y}^T,e_i e_j^T\rangle\right)\langle \hat{\Delta}_X\hat{\Delta}^{T}_Y,e_i e_j^T\rangle\\
&\quad+\frac1n\sum_{i\neq j}\frac{e^{\hat{P}_{ij}}}{(1+e^{\hat{P}_{ij}})^2}\cdot\left(\frac{1}{\sqrt{n}}\langle\hat{\Delta}_{\theta},e_i+e_j\rangle+\langle\hat{\Delta}_{H},z_iz_j^T\rangle+\frac1n\langle\hat{X}^d\hat{Y}^{dT}-\hat{X}\hat{Y}^T,e_i e_j^T\rangle\right)\langle \Delta''_X\Delta^{''T}_Y,e_i e_j^T\rangle\\
&\quad -\frac{1}{n^2}\sum_{i\neq j}\frac{e^{\hat{P}_{ij}}}{(1+e^{\hat{P}_{ij}})^2}\langle \hat{\Delta}_X\hat{\Delta}^{T}_Y,e_i e_j^T\rangle \langle \Delta''_X\Delta^{''T}_Y,e_i e_j^T\rangle
\end{align*}
Combine the above result with \eqref{eq6:pf_debias}, we have
\begin{align}\label{eq7:pf_debias}
 &L_c(c(\hat{V}))^T \left(c(\bar{V})-c(\hat{V})\right)   \notag\\ 
 &=-\left(c(\bar{V})-c(\hat{V})\right)^T\nabla^2L_c(c(\hat{V})) \left(c(\hat{V}^d)-c(\hat{V})\right)\notag\\
&\quad+\frac1n\sum_{i\neq j}\frac{e^{\hat{P}_{ij}}}{(1+e^{\hat{P}_{ij}})^2}\cdot\left(\frac{1}{\sqrt{n}}\langle\Delta''_{\theta},e_i+e_j\rangle+\langle\Delta''_{H},z_iz_j^T\rangle+\frac1n\langle\bar{X}\bar{Y}^T-\hat{X}\hat{Y}^T,e_i e_j^T\rangle\right)\langle \hat{\Delta}_X\hat{\Delta}^{T}_Y,e_i e_j^T\rangle\notag\\
&\quad+\frac1n\sum_{i\neq j}\frac{e^{\hat{P}_{ij}}}{(1+e^{\hat{P}_{ij}})^2}\cdot\left(\frac{1}{\sqrt{n}}\langle\hat{\Delta}_{\theta},e_i+e_j\rangle+\langle\hat{\Delta}_{H},z_iz_j^T\rangle+\frac1n\langle\hat{X}^d\hat{Y}^{dT}-\hat{X}\hat{Y}^T,e_i e_j^T\rangle\right)\langle \Delta''_X\Delta^{''T}_Y,e_i e_j^T\rangle\notag\\
&\quad -\frac{1}{n^2}\sum_{i\neq j}\frac{e^{\hat{P}_{ij}}}{(1+e^{\hat{P}_{ij}})^2}\langle \hat{\Delta}_X\hat{\Delta}^{T}_Y,e_i e_j^T\rangle \langle \Delta''_X\Delta^{''T}_Y,e_i e_j^T\rangle\notag\\
&\quad +\frac1n\sum_{i\neq j}\left(\frac{e^{\hat{P}_{ij}}}{1+e^{\hat{P}_{ij}}}-A_{ij}\right)\langle \Delta''_X\Delta^{''T}_Y,e_i e_j^T\rangle.
\end{align}
Similarly, we have
\begin{align}\label{eq8:pf_debias}
 &L_c(c(\hat{V}))^T \left(c(\hat{V}^d)-c(\hat{V})\right)   \notag\\ 
 &=-\left(c(\hat{V}^d)-c(\hat{V})\right)^T\nabla^2L_c(c(\hat{V})) \left(c(\hat{V}^d)-c(\hat{V})\right)\notag\\
&\quad+\frac2n\sum_{i\neq j}\frac{e^{\hat{P}_{ij}}}{(1+e^{\hat{P}_{ij}})^2}\cdot\left(\frac{1}{\sqrt{n}}\langle\hat{\Delta}_{\theta},e_i+e_j\rangle+\langle\hat{\Delta}_{H},z_iz_j^T\rangle+\frac1n\langle\hat{X}^d\hat{Y}^{dT}-\hat{X}\hat{Y}^T,e_i e_j^T\rangle\right)\langle \hat{\Delta}_X\hat{\Delta}^{T}_Y,e_i e_j^T\rangle\notag\\
&\quad -\frac{1}{n^2}\sum_{i\neq j}\frac{e^{\hat{P}_{ij}}}{(1+e^{\hat{P}_{ij}})^2}|\langle \hat{\Delta}_X\hat{\Delta}^{T}_Y,e_i e_j^T\rangle|^2 \notag\\
&\quad +\frac1n\sum_{i\neq j}\left(\frac{e^{\hat{P}_{ij}}}{1+e^{\hat{P}_{ij}}}-A_{ij}\right)\langle \hat{\Delta}_X\hat{\Delta}^{T}_Y,e_i e_j^T\rangle.
\end{align}
Combine \eqref{eq7:pf_debias} and \eqref{eq8:pf_debias}, we obtain
\begin{align}\label{eq9:pf_debias}
   L_c(c(\hat{V}))^T \left(c(\bar{V})-c(\hat{V}^d)\right)  =-\left(c(\bar{V})-c(\hat{V}^d)\right)^T\nabla^2L_c(c(\hat{V})) \left(c(\hat{V}^d)-c(\hat{V})\right)+(r),
\end{align}
where 
\begin{align*}
(r)
&=\frac1n\sum_{i\neq j}\frac{e^{\hat{P}_{ij}}}{(1+e^{\hat{P}_{ij}})^2}\cdot\left(\frac{1}{\sqrt{n}}\langle\Delta''_{\theta},e_i+e_j\rangle+\langle\Delta''_{H},z_iz_j^T\rangle+\frac1n\langle\bar{X}\bar{Y}^T-\hat{X}\hat{Y}^T,e_i e_j^T\rangle\right)\langle \hat{\Delta}_X\hat{\Delta}^{T}_Y,e_i e_j^T\rangle\notag\\
&\quad+\frac1n\sum_{i\neq j}\frac{e^{\hat{P}_{ij}}}{(1+e^{\hat{P}_{ij}})^2}\cdot\left(\frac{1}{\sqrt{n}}\langle\hat{\Delta}_{\theta},e_i+e_j\rangle+\langle\hat{\Delta}_{H},z_iz_j^T\rangle+\frac1n\langle\hat{X}^d\hat{Y}^{dT}-\hat{X}\hat{Y}^T,e_i e_j^T\rangle\right)\langle \Delta''_X\Delta^{''T}_Y,e_i e_j^T\rangle\notag\\
&\quad-\frac2n\sum_{i\neq j}\frac{e^{\hat{P}_{ij}}}{(1+e^{\hat{P}_{ij}})^2}\cdot\left(\frac{1}{\sqrt{n}}\langle\hat{\Delta}_{\theta},e_i+e_j\rangle+\langle\hat{\Delta}_{H},z_iz_j^T\rangle+\frac1n\langle\hat{X}^d\hat{Y}^{dT}-\hat{X}\hat{Y}^T,e_i e_j^T\rangle\right)\langle \hat{\Delta}_X\hat{\Delta}^{T}_Y,e_i e_j^T\rangle\notag\\
&\quad -\frac{1}{n^2}\sum_{i\neq j}\frac{e^{\hat{P}_{ij}}}{(1+e^{\hat{P}_{ij}})^2}\langle \hat{\Delta}_X\hat{\Delta}^{T}_Y,e_i e_j^T\rangle \langle \Delta''_X\Delta^{''T}_Y,e_i e_j^T\rangle+\frac{1}{n^2}\sum_{i\neq j}\frac{e^{\hat{P}_{ij}}}{(1+e^{\hat{P}_{ij}})^2}|\langle \hat{\Delta}_X\hat{\Delta}^{T}_Y,e_i e_j^T\rangle|^2 \notag\\
&\quad +\frac1n\sum_{i\neq j}\left(\frac{e^{\hat{P}_{ij}}}{1+e^{\hat{P}_{ij}}}-A_{ij}\right)\langle \Delta''_X\Delta^{''T}_Y,e_i e_j^T\rangle-\frac1n\sum_{i\neq j}\left(\frac{e^{\hat{P}_{ij}}}{1+e^{\hat{P}_{ij}}}-A_{ij}\right)\langle \hat{\Delta}_X\hat{\Delta}^{T}_Y,e_i e_j^T\rangle.
\end{align*}
By \eqref{eq4:pf_debias} and \eqref{eq9:pf_debias}, we have
\begin{align}\label{eq10:pf_debias}
&\nabla L_c(c(\hat{V}^d))^T\left(c(\bar{V})-c(\hat{V}^d)\right)\notag\\
&=\left(c(\bar{V})-c(\hat{V}^d)\right)^T\left(\int^1_0\nabla^2 L_c\left(c(\hat{V})+t(c(\hat{V}^d)-c(\hat{V}))\right)-\nabla^2L_c(c(\hat{V})) dt\right)\left(c(\hat{V}^d)-c(\hat{V})\right)+(r).
\end{align}
As bounding (1), we have
\begin{align}\label{eq11:pf_debias}
&\left|\left(c(\bar{V})-c(\hat{V}^d)\right)^T\left(\int^1_0\nabla^2 L_c\left(c(\hat{V})+t(c(\hat{V}^d)-c(\hat{V}))\right)-\nabla^2L_c(c(\hat{V})) dt\right)\left(c(\hat{V}^d)-c(\hat{V})\right)\right|\notag\\
&\lesssim\frac{C_2}{\sqrt{n}}\sqrt{\|\Delta_{\theta}\|^2_2+\|\Delta_{H}\|^2_F+\frac{1}{n^2}\|\Delta_{\Gamma}\|^2_F}  \cdot\sqrt{\|\hat{\Delta}_{\theta}\|^2_2+\|\hat{\Delta}_{H}\|^2_F+\frac{1}{n^2}\|\hat{\Delta}_{\Gamma}\|^2_F}
\end{align}
for $C_2= \su\sqrt{\mu\sX\sY r^2}(\sqrt{r}(c_{\infty}+c_b)+c_{43})$.
It remains to bound (r).
Note that
\begin{align*}
&\left|\frac1n\sum_{i\neq j}\frac{e^{\hat{P}_{ij}}}{(1+e^{\hat{P}_{ij}})^2}\cdot\left(\frac{1}{\sqrt{n}}\langle\Delta''_{\theta},e_i+e_j\rangle+\langle\Delta''_{H},z_iz_j^T\rangle+\frac1n\langle\bar{X}\bar{Y}^T-\hat{X}\hat{Y}^T,e_i e_j^T\rangle\right)\langle \hat{\Delta}_X\hat{\Delta}^{T}_Y,e_i e_j^T\rangle\right|\notag\\
&\lesssim \frac1n \|\hat{\Delta}_X\hat{\Delta}^{T}_Y\|_F\sqrt{\sum_{i\neq j}\left(\frac{1}{\sqrt{n}}\langle\Delta''_{\theta},e_i+e_j\rangle+\langle\Delta''_{H},z_iz_j^T\rangle+\frac1n\langle\bar{X}\bar{Y}^T-\hat{X}\hat{Y}^T,e_i e_j^T\rangle\right)^2}\tag{Cauchy-Schwarz}\\
&\lesssim  \frac{\sqrt{\su}}{n} \left(\|\hat{\Delta}_X\|_F^2+\|\hat{\Delta}_Y\|_F^2\right)\sqrt{\|\Delta''_{\theta}\|^2_2+\|\Delta''_{H}\|^2_F+\frac{1}{n^2}\|\Delta''_{\Gamma}\|^2_F} \tag{by Assumption \ref{assumption:eigenvalues}}.
\end{align*}
Similarly, we have
\begin{align*}
&\left|\frac1n\sum_{i\neq j}\frac{e^{\hat{P}_{ij}}}{(1+e^{\hat{P}_{ij}})^2}\cdot\left(\frac{1}{\sqrt{n}}\langle\hat{\Delta}_{\theta},e_i+e_j\rangle+\langle\hat{\Delta}_{H},z_iz_j^T\rangle+\frac1n\langle\hat{X}^d\hat{Y}^{dT}-\hat{X}\hat{Y}^T,e_i e_j^T\rangle\right)\langle \Delta''_X\Delta^{''T}_Y,e_i e_j^T\rangle\right|\\
&\lesssim  \frac{\sqrt{\su}}{n} \left(\|\Delta''_X\|_F^2+\|\Delta''_Y\|_F^2\right)\sqrt{\|\hat{\Delta}_{\theta}\|^2_2+\|\hat{\Delta}_{H}\|^2_F+\frac{1}{n^2}\|\hat{\Delta}_{\Gamma}\|^2_F}
\end{align*}
and 
\begin{align*}
&\left|\frac2n\sum_{i\neq j}\frac{e^{\hat{P}_{ij}}}{(1+e^{\hat{P}_{ij}})^2}\cdot\left(\frac{1}{\sqrt{n}}\langle\hat{\Delta}_{\theta},e_i+e_j\rangle+\langle\hat{\Delta}_{H},z_iz_j^T\rangle+\frac1n\langle\hat{X}^d\hat{Y}^{dT}-\hat{X}\hat{Y}^T,e_i e_j^T\rangle\right)\langle \hat{\Delta}_X\hat{\Delta}^{T}_Y,e_i e_j^T\rangle\right|\\
&\lesssim  \frac{\sqrt{\su}}{n}\left(\|\hat{\Delta}_X\|_F^2+\|\hat{\Delta}_Y\|_F^2\right)\sqrt{\|\hat{\Delta}_{\theta}\|^2_2+\|\hat{\Delta}_{H}\|^2_F+\frac{1}{n^2}\|\hat{\Delta}_{\Gamma}\|^2_F}.
\end{align*}
Also, we have
\begin{align*}
&\left|\frac{1}{n^2}\sum_{i\neq j}\frac{e^{\hat{P}_{ij}}}{(1+e^{\hat{P}_{ij}})^2}\langle \hat{\Delta}_X\hat{\Delta}^{T}_Y,e_i e_j^T\rangle \langle \Delta''_X\Delta^{''T}_Y,e_i e_j^T\rangle\right|\\
&\lesssim\frac{1}{n^2}\|\Delta''_X\Delta^{''T}_Y\|_F\|\hat{\Delta}_X\hat{\Delta}^{T}_Y\|_F\tag{Cauchy-Schwarz}\\
&\leq \frac{1}{n^2}\left(\|\Delta''_X\|_F^2+\|\Delta''_Y\|_F^2\right)\left(\|\hat{\Delta}_X\|_F^2+\|\hat{\Delta}_Y\|_F^2\right)
\end{align*}
and 
\begin{align*}
&\left|\frac{1}{n^2}\sum_{i\neq j}\frac{e^{\hat{P}_{ij}}}{(1+e^{\hat{P}_{ij}})^2}|\langle \hat{\Delta}_X\hat{\Delta}^{T}_Y,e_i e_j^T\rangle|^2\right|\leq\frac{1}{n^2}\|\hat{\Delta}_X\hat{\Delta}^{T}_Y\|_F^2\leq \frac{1}{n^2}\left(\|\hat{\Delta}_X\|_F^2+\|\hat{\Delta}_Y\|_F^2\right)^2.
\end{align*}
Follow the proofs in Appendix \ref{proof_convexity}, we have
\begin{align*}
&\left|\frac1n\sum_{i\neq j}\left(\frac{e^{\hat{P}_{ij}}}{1+e^{\hat{P}_{ij}}}-A_{ij}\right)\langle \Delta''_X\Delta^{''T}_Y,e_i e_j^T\rangle\right|\\
&\lesssim\frac{\sqrt{\su}}{n}\left(\|\Delta''_X\|_F^2+\|\Delta''_Y\|_F^2\right)\left(\|\hat{\theta}-\theta^{*}\|_{2}+\|\hat{H}-H^{*}\|_{F}+\frac{1}{n}\|X^{*}\|\|\hat{F}-F^{*}\|_{F}+{\sqrt{\log n}}\right)
\end{align*}
and 
\begin{align*}
&\left|\frac1n\sum_{i\neq j}\left(\frac{e^{\hat{P}_{ij}}}{1+e^{\hat{P}_{ij}}}-A_{ij}\right)\langle \hat{\Delta}_X\hat{\Delta}^{T}_Y,e_i e_j^T\rangle\right|\\
&\lesssim\frac{\sqrt{\su}}{n}\left(\|\hat{\Delta}_X\|_F^2+\|\hat{\Delta}_Y\|_F^2\right)\left(\|\hat{\theta}-\theta^{*}\|_{2}+\|\hat{H}-H^{*}\|_{F}+\frac{1}{n}\|X^{*}\|\|\hat{F}-F^{*}\|_{F}+{\sqrt{\log n}}\right).
\end{align*}
As a result, we obtain
\begin{align*}
&|(r)|\\
&\lesssim  \frac{\sqrt{\su}}{n}\left(\|\hat{\Delta}_X\|_F^2+\|\hat{\Delta}_Y\|_F^2+\|\Delta''_X\|_F^2+\|\Delta''_Y\|_F^2\right)\\
&\quad\cdot\sqrt{\|\hat{\Delta}_{\theta}\|^2_2+\|\hat{\Delta}_{H}\|^2_F+\frac{1}{n^2}\|\hat{\Delta}_{\Gamma}\|^2_F+\|\Delta''_{\theta}\|^2_2+\|\Delta''_{H}\|^2_F+\frac{1}{n^2}\|\Delta''_{\Gamma}\|^2_F}\\
&\quad+\frac{1}{n^2}\left(\|\hat{\Delta}_X\|_F^2+\|\hat{\Delta}_Y\|_F^2+\|\Delta''_X\|_F^2+\|\Delta''_Y\|_F^2\right)\left(\|\hat{\Delta}_X\|_F^2+\|\hat{\Delta}_Y\|_F^2\right)\\
&\quad +\frac{\sqrt{\su}}{n}\left(\|\hat{\Delta}_X\|_F^2+\|\hat{\Delta}_Y\|_F^2+\|\Delta''_X\|_F^2+\|\Delta''_Y\|_F^2\right)\left(\|\hat{\theta}-\theta^{*}\|_{2}+\|\hat{H}-H^{*}\|_{F}+\frac{1}{n}\|X^{*}\|\|\hat{F}-F^{*}\|_{F}+{\sqrt{\log n}}\right)\\
&\lesssim \sqrt{\frac{\su \mu r\sigma_{\max}}{n^2}}(c_a+c_{11})^3 \sqrt{n}\\
&\lesssim \sqrt{\su \mu\sX\sY r^2}(c_a+c_{11})^3 \sqrt{n}.
\end{align*}
Combine this with \eqref{eq10:pf_debias} and \eqref{eq11:pf_debias}, we show that
\begin{align*}
|(2)|&=\left|L_c(c(\hat{V}^d))^T\left(c(\bar{V})-c(\hat{V}^d)\right)\right|\\
&\lesssim \frac{C_2}{\sqrt{n}}\sqrt{\|\Delta_{\theta}\|^2_2+\|\Delta_{H}\|^2_F+\frac{1}{n^2}\|\Delta_{\Gamma}\|^2_F}  \cdot\sqrt{\|\hat{\Delta}_{\theta}\|^2_2+\|\hat{\Delta}_{H}\|^2_F+\frac{1}{n^2}\|\hat{\Delta}_{\Gamma}\|^2_F}+\sqrt{\su \mu\sX\sY r^2}(c_a+c_{11})^3 \sqrt{n}. 
\end{align*}


\item We finally bound (3). By \eqref{eq2:pf_debias} with $V=\bar{V}$, we have
\begin{align*}
\nabla\bar{L}_c\left(c(\bar{V})\right)=\nabla {L}_c\left(c(V^*)\right)+\nabla^2 {L}_c\left(c(V^*)\right)\left(c(\bar{V})-c(V^*)\right),
\end{align*}
which then implies 
\begin{align}\label{eq24:pf_debias}
&\nabla\bar{L}_c\left(c(\bar{V})\right)^T\left(c(\bar{V})-c(\hat{V}^d)\right)\notag\\
&=\nabla {L}_c\left(c(V^*)\right)^T\left(c(\bar{V})-c(\hat{V}^d)\right)+\left(c(\bar{V})-c(\hat{V}^d)\right)^T\nabla^2 {L}_c\left(c(V^*)\right)\left(c(\bar{V})-c(V^*)\right).
\end{align}
We will deal with the first term in the following. Recall the definition of $\Delta'''$, follow the same argument as in \eqref{eq6:pf_debias}, we have
\begin{align}\label{eq20:pf_debias}
 &L_c(c(V^*))^T \left(c(\bar{V})-c(V^*)\right)   \notag\\
 &=\nabla L(V^*)^T(\bar{V}-V^*) + \frac1n\sum_{i\neq j}\left(\frac{e^{{P}^*_{ij}}}{1+e^{{P}^*_{ij}}}-A_{ij}\right)\langle \Delta'''_X\Delta^{'''T}_Y,e_i e_j^T\rangle.
\end{align}
By \eqref{property:bar}, we have $\cP\nabla L(V^*)=-\cP D^*\left(\bar{V}-V^*\right)$. Moreover, note that $\cP(\bar{V})=\bar{V}, \cP(V^*)=V^*$. Thus, we have
\begin{align*}
&\nabla L(V^*)^T(\bar{V}-V^*) \\
&=\left(\cP\nabla L(V^*)\right)^T(\bar{V}-V^*) \\
&=-\left(\bar{V}-V^*\right)^T\left(\sum_{i\neq j}\frac{e^{\hat{P}_{ij}}}{(1+e^{\hat{P}_{ij}})^2}
\begin{bmatrix}
\frac{1}{\sqrt{n}}(e_i+e_j)\\
z_iz_j^T\\
\frac1ne_ie_j^T{Y^*}\\
\frac1ne_je_i^T{X^*}
\end{bmatrix}^{\otimes 2}\right)(\bar{V}-V^*)\\
&=-\left(c(\bar{V})-c({V}^*)\right)^T\nabla^2L_c(c({V^*})) \left(c(\bar{V})-c({V}^*)\right)\\
&\quad+\frac2n\sum_{i\neq j}\frac{e^{{P}^*_{ij}}}{(1+e^{{P}^*_{ij}})^2}\cdot\left(\frac{1}{\sqrt{n}}\langle\Delta'''_{\theta},e_i+e_j\rangle+\langle\Delta'''_{H},z_iz_j^T\rangle+\frac1n\langle\bar{X}\bar{Y}^T-X^*Y^{*T},e_i e_j^T\rangle\right)\langle \Delta'''_X\Delta^{'''T}_Y,e_i e_j^T\rangle\\
&\quad -\frac{1}{n^2}\sum_{i\neq j}\frac{e^{{P}^*_{ij}}}{(1+e^{{P}^*_{ij}})^2}\left|\langle \Delta'''_X\Delta^{'''T}_Y,e_i e_j^T\rangle\right|^2,
\end{align*}
where the last equation follows the same argument as that in bounding (2). Plug this into \eqref{eq20:pf_debias}, we have
\begin{align}\label{eq21:pf_debias}
  &L_c(c(V^*))^T \left(c(\bar{V})-c(V^*)\right)   \notag\\
  &=-\left(c(\bar{V})-c({V}^*)\right)^T\nabla^2L_c(c({V^*})) \left(c(\bar{V})-c({V}^*)\right)\notag\\
&\quad+\frac2n\sum_{i\neq j}\frac{e^{{P}^*_{ij}}}{(1+e^{{P}^*_{ij}})^2}\cdot\left(\frac{1}{\sqrt{n}}\langle\Delta'''_{\theta},e_i+e_j\rangle+\langle\Delta'''_{H},z_iz_j^T\rangle+\frac1n\langle\bar{X}\bar{Y}^T-X^*Y^{*T},e_i e_j^T\rangle\right)\langle \Delta'''_X\Delta^{'''T}_Y,e_i e_j^T\rangle\notag\\
&\quad -\frac{1}{n^2}\sum_{i\neq j}\frac{e^{{P}^*_{ij}}}{(1+e^{{P}^*_{ij}})^2}\left|\langle \Delta'''_X\Delta^{'''T}_Y,e_i e_j^T\rangle\right|^2+ \frac1n\sum_{i\neq j}\left(\frac{e^{{P}^*_{ij}}}{1+e^{{P}^*_{ij}}}-A_{ij}\right)\langle \Delta'''_X\Delta^{'''T}_Y,e_i e_j^T\rangle.
\end{align}
Similarly, recall the definition of $\Delta'$, we have
\begin{align}\label{eq22:pf_debias}
  &L_c(c(V^*))^T \left(c(\hat{V}^d)-c(V^*)\right)   \notag\\
  &=-\left(c(\hat{V}^d)-c({V}^*)\right)^T\nabla^2L_c(c({V^*})) \left(c(\bar{V})-c({V}^*)\right)\notag\\
&\quad+\frac1n\sum_{i\neq j}\frac{e^{{P}^*_{ij}}}{(1+e^{{P}^*_{ij}})^2}\cdot\left(\frac{1}{\sqrt{n}}\langle\Delta'_{\theta},e_i+e_j\rangle+\langle\Delta'_{H},z_iz_j^T\rangle+\frac1n\langle\hat{X}^d\hat{Y}^{dT}-X^*Y^{*T},e_i e_j^T\rangle\right)\langle \Delta'''_X\Delta^{'''T}_Y,e_i e_j^T\rangle\notag\\
&\quad+\frac1n\sum_{i\neq j}\frac{e^{{P}^*_{ij}}}{(1+e^{{P}^*_{ij}})^2}\cdot\left(\frac{1}{\sqrt{n}}\langle\Delta'''_{\theta},e_i+e_j\rangle+\langle\Delta'''_{H},z_iz_j^T\rangle+\frac1n\langle\bar{X}\bar{Y}^T-X^*Y^{*T},e_i e_j^T\rangle\right)\langle \Delta'_X\Delta^{'T}_Y,e_i e_j^T\rangle\notag\\
&\quad -\frac{1}{n^2}\sum_{i\neq j}\frac{e^{{P}^*_{ij}}}{(1+e^{{P}^*_{ij}})^2}\langle \Delta'_X\Delta^{'T}_Y,e_i e_j^T\rangle\langle \Delta'''_X\Delta^{'''T}_Y,e_i e_j^T\rangle+ \frac1n\sum_{i\neq j}\left(\frac{e^{{P}^*_{ij}}}{1+e^{{P}^*_{ij}}}-A_{ij}\right)\langle \Delta'_X\Delta^{'T}_Y,e_i e_j^T\rangle.
\end{align}
Combine \eqref{eq21:pf_debias} and \eqref{eq22:pf_debias}, we then have
\begin{align}\label{eq23:pf_debias}
&\nabla {L}_c\left(c(V^*)\right)^T\left(c(\bar{V})-c(\hat{V}^d)\right) \notag\\
&=-\left(c(\bar{V})-c(\hat{V}^d)\right)^T\nabla^2 {L}_c\left(c(V^*)\right)\left(c(\bar{V})-c(V^*)\right)+(r),
\end{align}
where 
\begin{align*}
&(r)\\
&=\frac2n\sum_{i\neq j}\frac{e^{{P}^*_{ij}}}{(1+e^{{P}^*_{ij}})^2}\cdot\left(\frac{1}{\sqrt{n}}\langle\Delta'''_{\theta},e_i+e_j\rangle+\langle\Delta'''_{H},z_iz_j^T\rangle+\frac1n\langle\bar{X}\bar{Y}^T-X^*Y^{*T},e_i e_j^T\rangle\right)\langle \Delta'''_X\Delta^{'''T}_Y,e_i e_j^T\rangle\notag\\
&\quad -\frac{1}{n^2}\sum_{i\neq j}\frac{e^{{P}^*_{ij}}}{(1+e^{{P}^*_{ij}})^2}\left|\langle \Delta'''_X\Delta^{'''T}_Y,e_i e_j^T\rangle\right|^2+ \frac1n\sum_{i\neq j}\left(\frac{e^{{P}^*_{ij}}}{1+e^{{P}^*_{ij}}}-A_{ij}\right)\langle \Delta'''_X\Delta^{'''T}_Y,e_i e_j^T\rangle\\
&\quad-\frac1n\sum_{i\neq j}\frac{e^{{P}^*_{ij}}}{(1+e^{{P}^*_{ij}})^2}\cdot\left(\frac{1}{\sqrt{n}}\langle\Delta'_{\theta},e_i+e_j\rangle+\langle\Delta'_{H},z_iz_j^T\rangle+\frac1n\langle\hat{X}^d\hat{Y}^{dT}-X^*Y^{*T},e_i e_j^T\rangle\right)\langle \Delta'''_X\Delta^{'''T}_Y,e_i e_j^T\rangle\notag\\
&\quad-\frac1n\sum_{i\neq j}\frac{e^{{P}^*_{ij}}}{(1+e^{{P}^*_{ij}})^2}\cdot\left(\frac{1}{\sqrt{n}}\langle\Delta'''_{\theta},e_i+e_j\rangle+\langle\Delta'''_{H},z_iz_j^T\rangle+\frac1n\langle\bar{X}\bar{Y}^T-X^*Y^{*T},e_i e_j^T\rangle\right)\langle \Delta'_X\Delta^{'T}_Y,e_i e_j^T\rangle\notag\\
&\quad +\frac{1}{n^2}\sum_{i\neq j}\frac{e^{{P}^*_{ij}}}{(1+e^{{P}^*_{ij}})^2}\langle \Delta'_X\Delta^{'T}_Y,e_i e_j^T\rangle\langle \Delta'''_X\Delta^{'''T}_Y,e_i e_j^T\rangle- \frac1n\sum_{i\neq j}\left(\frac{e^{{P}^*_{ij}}}{1+e^{{P}^*_{ij}}}-A_{ij}\right)\langle \Delta'_X\Delta^{'T}_Y,e_i e_j^T\rangle.
\end{align*}
By \eqref{eq24:pf_debias} and \eqref{eq23:pf_debias}, we have
\begin{align*}
    \nabla\bar{L}_c\left(c(\bar{V})\right)^T\left(c(\bar{V})-c(\hat{V}^d)\right)=(r).
\end{align*}
Following the same argument as in bounding (2), we have
\begin{align*}
|(3)|&=|(r)|\\
&\lesssim  \frac{\sqrt{\su}}{n}\left(\|\Delta'_X\|_F^2+\|\Delta'_Y\|_F^2+\|\Delta'''_X\|_F^2+\|\Delta'''_Y\|_F^2\right)\\
&\quad\cdot\sqrt{\|\Delta'_{\theta}\|^2_2+\|\Delta'_{H}\|^2_F+\frac{1}{n^2}\|\Delta'_{\Gamma}\|^2_F+\|\Delta'''_{\theta}\|^2_2+\|\Delta'''_{H}\|^2_F+\frac{1}{n^2}\|\Delta'''_{\Gamma}\|^2_F}\\
&\quad+\frac{1}{n^2}\left(\|\Delta'_X\|_F^2+\|\Delta'_Y\|_F^2+\|\Delta'''_X\|_F^2+\|\Delta'''_Y\|_F^2\right)\left(\|\Delta'''_X\|_F^2+\|\Delta'''_Y\|_F^2\right)\\
&\quad +\frac{\sqrt{\log n}}n \left(\|\Delta'_X\|_F^2+\|\Delta'_Y\|_F^2+\|\Delta'''_X\|_F^2+\|\Delta'''_Y\|_F^2\right)\\
&\lesssim \sqrt{\su \mu\sX\sY r^2}(c_a+c_{11})^3 \sqrt{n}.
\end{align*}



\end{enumerate}

Combine the results for (1)-(3), by \eqref{eq3:pf_debias}, we have
\begin{align*}
&\left|\left(c(\bar{V})-c(\hat{V}^d)\right)^T \nabla^2{L}_c\left(c(V^*)\right)\left(c(\bar{V})-c(\hat{V}^d)\right)\right|\notag\\
&\lesssim \frac{C_1}{\sqrt{n}}\sqrt{\|\Delta_{\theta}\|^2_2+\|\Delta_{H}\|^2_F+\frac{1}{n^2}\|\Delta_{\Gamma}\|^2_F}  \cdot\sqrt{\|\Delta'_{\theta}\|^2_2+\|\Delta'_{H}\|^2_F+\frac{1}{n^2}\|\Delta'_{\Gamma}\|^2_F}\\
&\quad+\frac{C_2}{\sqrt{n}}\sqrt{\|\Delta_{\theta}\|^2_2+\|\Delta_{H}\|^2_F+\frac{1}{n^2}\|\Delta_{\Gamma}\|^2_F}  \cdot\sqrt{\|\hat{\Delta}_{\theta}\|^2_2+\|\hat{\Delta}_{H}\|^2_F+\frac{1}{n^2}\|\hat{\Delta}_{\Gamma}\|^2_F}+\sqrt{\su \mu\sX\sY r^2}(c_a+c_{11})^3 \sqrt{n}\\
&\lesssim C_2(c_a+c_{11})\sqrt{\mu \sX\sY r^2}\sqrt{\|\Delta_{\theta}\|^2_2+\|\Delta_{H}\|^2_F+\frac{1}{n^2}\|\Delta_{\Gamma}\|^2_F} +\sqrt{\su \mu\sX\sY r^2}(c_a+c_{11})^3 \sqrt{n}.
\end{align*}
Further combine with \eqref{eq26:pf_debias}, we have
\begin{align*}
&\frac{\sl e^{c_P}}{(1+e^{c_P})^2} \left(\|\Delta_{\theta}\|^2_2+\|\Delta_{H}\|^2_F+\frac{1}{n^2}\|\Delta_{\Gamma}\|^2_F\right)\\
 &\lesssim   C_2(c_a+c_{11})\sqrt{\mu \sX\sY r^2}\sqrt{\|\Delta_{\theta}\|^2_2+\|\Delta_{H}\|^2_F+\frac{1}{n^2}\|\Delta_{\Gamma}\|^2_F} +\sqrt{\su \mu\sX\sY r^2}(c_a+c_{11})^3 \sqrt{n},
\end{align*}
which implies
\begin{align*}
\sqrt{\|\Delta_{\theta}\|^2_2+\|\Delta_{H}\|^2_F+\frac{1}{n^2}\|\Delta_{\Gamma}\|^2_F}\lesssim \sqrt{\frac{(1+e^{c_P})^2}{\sl e^{c_P}}}(\su \mu\sX\sY r^2)^{1/4}(c_a+c_{11})^{3/2}\cdot n^{1/4}.
\end{align*}
Thus, we finish the proofs.
\end{proof}
% \subsection{Proofs of Theorem \ref{thm:distribution}}\label{pf:distribution}
% Recall that
% \begin{align*}
% \begin{bmatrix}
% \bar{\theta}-\theta^*\\
% \bar{H}-H^*\\
% \bar{X}-X^*\\
% \bar{Y}-Y^*
% \end{bmatrix}
% =-(\cP D^*\cP)^{\dagger}\cP
% \nabla L(\theta^*,H^*,X^*,Y^*),
% \end{align*}
% where
% \begin{align*}
% \nabla L(\theta^*,H^*,X^*,Y^*)= 
% \sum_{i\neq j}\left(\frac{e^{P_{ij}^*}}{1+e^{P_{ij}^*}}-A_{ij}\right)
% \begin{bmatrix}
% \frac{1}{\sqrt{n}}(e_i+e_j)\\
% z_i^T z_j\\
% \frac1n e_ie_j^T Y^*\\
% \frac1n e_j e_i^TX^*
% \end{bmatrix}.
% \end{align*}
% Thus, for example, $\bar{\theta}_i$ has the following form:
% \begin{align*}
% \bar{\theta}_i=\theta^*_i+\sum_{i\neq j}\alpha_{ij}A_{ij}
% \end{align*}
% for some $\{\alpha_{ij}\}$.
% We know $\sum_{i\neq j}\alpha_{ij}A_{ij}$ is asymptomatically Gaussian.
% And the cdf difference between $\sum_{i\neq j}\alpha_{ij}A_{ij}$ and Gaussian can be captured by Berry–Esseen theorem for low dimensional problems and \cite{chernozhuokov2022improved} for high dimensional problems.

==> proof_ncv_induction.tex <==
\section{Proofs for Section \ref{sec:ncv_induction}}
We define
\begin{align*}
f_{\diff}(X,Y):=\frac{c_{\aug}}{n^2}\|X^TX-Y^TY\|^2_{F}.
\end{align*}
Thus, we have $f_{\aug}(\theta,H,X,Y)=f(\theta,H,X,Y)+f_{\diff}(X,Y)$.
Note that for any $M$, $F$, and $R\in\cO^{r\times r}$, we have
\begin{align*}
f(M,FR)=f(M,F),\ \nabla_M f(M,FR)=\nabla_M f(M,F), \ \nabla_M f(M,F)R=\nabla_M f(M,FR), 
\end{align*}
which will be used in the following proofs.
We first present the following lemmas, which will be constantly used in the proofs.
\begin{lemma}\label{lem:gradient_norm}
Let $M^*, F^*$ be the ground truth parameters and $\lambda\gtrsim\sqrt{\frac{\log n}{n}}$. Under Assumption \ref{assumption:scales}, it holds with probability at least $1-n^{-10}$ that
\begin{align*}
&\|\nabla_{\theta} f(M^*,F^*)\|_2\lesssim\sqrt{n\log n},\quad
\|\nabla_{H} f(M^*,F^*)\|_F\lesssim\sz\sqrt{p\log n},\\
&\|\nabla_{F} f(M^*,F^*)\|_F\lesssim \lambda   \left(\|X^{*}\|_F+\|Y^{*}\|_F\right).
\end{align*}
\end{lemma}
\begin{proof}[Proof of Lemma \ref{lem:gradient_norm}]
In the following, we will bound $\|\nabla_{\theta} f(M^*,F^*)\|_2$, $\|\nabla_{H} f(M^*,F^*)\|_F$ and $\|\nabla_{F} f(M^*,F^*)\|_F$, respectively.
Note that
\begin{align*}
\nabla_{\theta} f(M^*,F^*)
&=\nabla_{\theta} L(M^*,F^*)\\
&= \frac{1}{\sqrt{n}}\sum_{i\neq j}\left(\frac{e^{P_{ij}^*}}{1+e^{P_{ij}^*}}-A_{ij}\right)(e_i+e_j)\\
&=\frac{2}{\sqrt{n}}\sum_{i\neq j}\left(\frac{e^{P_{ij}^*}}{1+e^{P_{ij}^*}}-A_{ij}\right)e_i\\
&=\frac{2}{\sqrt{n}}\sum_{i=1}^n\left(\sum_{j\neq i}\left(\frac{e^{P_{ij}^*}}{1+e^{P_{ij}^*}}-A_{ij}\right)\right)e_i.
\end{align*}
For any fixed $i$, we have
\begin{align*}
\sum_{j\neq i}\left(\frac{e^{P_{ij}^*}}{1+e^{P_{ij}^*}}-A_{ij}\right)  
\end{align*}
is the sum of $n-1$ independent $1$-subgaussian random variables. Thus, with probability at least $1-n^{-11}$, it holds that
\begin{align*}
    \left|\sum_{j\neq i}\left(\frac{e^{P_{ij}^*}}{1+e^{P_{ij}^*}}-A_{ij}\right) \right|\lesssim \sqrt{n\log n}.
\end{align*}
Take union bound, we have with probability at least $1-n^{-10}$, for all $i\in [n]$, it holds that 
\begin{align*}
    \left|\sum_{j\neq i}\left(\frac{e^{P_{ij}^*}}{1+e^{P_{ij}^*}}-A_{ij}\right) \right|\lesssim \sqrt{n\log n},
\end{align*}
which implies $\|\nabla_{\theta} f(M^*,F^*)\|_2\lesssim \sqrt{n\log n}$.

To bound $\|\nabla_{H} f(M^*,F^*)\|_F$, note that
\begin{align*}
 \nabla_{H} f(M^*,F^*)
=\nabla_{H} L(M^*,F^*)
=\sum_{i\neq j}\left(\frac{e^{P_{ij}^*}}{1+e^{P_{ij}^*}}-A_{ij}\right)z_iz_j^T.
\end{align*}
By Assumption \ref{assumption:scales}, we have
\begin{align*}
\left\|\sum_{i\neq j}\bbE\left[\left(\frac{e^{P_{ij}^*}}{1+e^{P_{ij}^*}}-A_{ij}\right)^2z_iz_j^Tz_jz_i^T\right]\right\|\lesssim \sum_{i\neq j}\|z_i\|_2^2\|z_j\|_2^2
\asymp \sz^2.
\end{align*}
Thus, by matrix Bernstein inequality, with probability at least $1-n^{-10}$, we have
\begin{align*}
    \left\|\sum_{i\neq j}\left(\frac{e^{P_{ij}^*}}{1+e^{P_{ij}^*}}-A_{ij}\right)z_iz_j^T\right\|\lesssim \sz\sqrt{\log n},
\end{align*}
which implies that $\|\nabla_{H} f(M^*,F^*)\|_F\leq \sqrt{p}\|\nabla_{H} f(M^*,F^*)\|\lesssim \sz\sqrt{p\log n}$.


Finally, we bound $\|\nabla_{F} f(M^*,F^*)\|_F$. Note that
\begin{align*}
\|\nabla_{F} f(M^*,F^*)\|_F&\leq \|\nabla_{X} f(M^*,F^*)\|_F+\|\nabla_{Y} f(M^*,F^*)\|_F\\
&\leq \|\nabla_{X} L(M^*,F^*)\|_F+\|\nabla_{Y} L(M^*,F^*)\|_F+\lambda\left(\|X^{*}\|_F+\|Y^{*}\|_F\right)\\
&\leq \|\nabla_{\Gamma}L_c(\theta^*,H^*,\Gamma^*)\|\left(\|X^{*}\|_F+\|Y^{*}\|_F\right)+\lambda\left(\|X^{*}\|_F+\|Y^{*}\|_F\right),
\end{align*}
where the last inequality follows from the fact that $\|AB\|_F\leq \|A\|\|B\|_F$. Here 
\begin{align*}
\nabla_{\Gamma}L_c(\theta^*,H^*,\Gamma^*)=\frac{1}{n}\sum_{i\neq j}\left(\frac{e^{P_{ij}^*}}{1+e^{P_{ij}^*}}-A_{ij}\right)e_ie_j^T.
\end{align*}
Note that
\begin{align*}
\left\|\sum_{i\neq j}\bbE\left[\left(\frac{e^{P_{ij}^*}}{1+e^{P_{ij}^*}}-A_{ij}\right)^2e_ie_j^Te_je_i^T\right]\right\|\lesssim n\left\|\sum^n_{i=1}e_ie_i^T\right\|=n.
\end{align*}
Thus, by matrix Bernstein inequality, with probability at least $1-n^{-10}$, we have $\|\nabla_{\Gamma}L_c(\theta^*,H^*,\Gamma^*)\|\lesssim\sqrt{\frac{\log n}{n}}\lesssim\lambda$. Consequently, it holds that
\begin{align*}
 \|\nabla_{F} f(M^*,F^*)\|_F\lesssim \lambda   \left(\|X^{*}\|_F+\|Y^{*}\|_F\right).
\end{align*}
\end{proof}


\begin{lemma}\label{lem:gradient_spectral}
Suppose Lemma \ref{lem:ncv1} holds for the $t$-th iteration. Under Assumption \ref{assumption:eigenvalues
}, we have
\begin{align*}
&\left\|\frac1n\sum_{i\neq j}\left(\frac{e^{P_{ij}^t}}{1+e^{P_{ij}^t}}-A_{ij}\right)e_i e_j^T\right\|\\
&\lesssim   \frac{\sqrt{\su}}{n}\left(\|\theta^t-\theta^{*}\|_{2}+\|H^t-H^{*}\|_{F}+\frac{1}{n}\|X^*\|\|F^tR^t-F^{*}\|_{F}\right)+\sqrt{\frac{\log n}{n}}\\
&\lesssim \sqrt{\frac{c_{11}^2\overline{C}+\log n}{n}}.
\end{align*}
\end{lemma}
\begin{proof}[Proof of Lemma \ref{lem:gradient_spectral}]
We denote 
\begin{align*}
D^t:=\frac1n\sum_{i\neq j}\left(\frac{e^{P_{ij}^t}}{1+e^{P_{ij}^t}}-A_{ij}\right)e_i e_j^T.
\end{align*}   
Note that
\begin{align*}
\|D^t\|\leq \left\|\frac1n\sum_{i\neq j}\left(\frac{e^{P_{ij}^t}}{1+e^{P_{ij}^t}}-\frac{e^{P_{ij}^*}}{1+e^{P_{ij}^*}}\right)e_i e_j^T\right\|
+\left\|\frac1n\sum_{i\neq j}\left(\frac{e^{P_{ij}^*}}{1+e^{P_{ij}^*}}-A_{ij}\right)e_i e_j^T\right\|.
\end{align*}
For the first term, we have
\begin{align*}
&\left\|\frac1n\sum_{i\neq j}\left(\frac{e^{P_{ij}^t}}{1+e^{P_{ij}^t}}-\frac{e^{P_{ij}^*}}{1+e^{P_{ij}^*}}\right)e_i e_j^T\right\|\\
&\leq  \frac1n\left\|\sum_{i\neq j}\left(\frac{e^{P_{ij}^t}}{1+e^{P_{ij}^t}}-\frac{e^{P_{ij}^*}}{1+e^{P_{ij}^*}}\right)e_i e_j^T\right\|_F\\
&=\frac1n\sqrt{\sum_{i\neq j}\left(\frac{e^{P_{ij}^t}}{1+e^{P_{ij}^t}}-\frac{e^{P_{ij}^*}}{1+e^{P_{ij}^*}}\right)^2}\\
&\leq \frac{1}{4n}\sqrt{\sum_{i\neq j}\left(P^t_{ij}-P^*_{ij}\right)^2}\tag{by mean value theorem}\\
&\lesssim \frac{\sqrt{\su}}{n}\left(\|\theta^t-\theta^{*}\|_{2}+\|H^t-H^{*}\|_{F}+\frac{1}{n}\|X^*\|\|F^tR^t-F^{*}\|_{F}\right),
\end{align*}
where the last inequality follows from
\begin{align*}
&\sum_{i\neq j}(P_{ij}^{t}-P_{ij}^*)^2\\
&=\sum_{i\neq j}\left(\frac{1}{\sqrt{n}}\langle\theta^{t}-\theta^*,e_i+e_j\rangle+\langle H^{t}-H^*,z_iz_j^T\rangle+\frac1n\langle X^{t}Y^{tT}-X^*Y^{*T},e_i e_j^T\rangle\right)^2\\
&=
\begin{bmatrix}
  \vec(\theta^{t}-\theta^*)\\
  \vec(H^{t}-H^*)\\
  \frac1n\vec(X^{t}Y^{tT}-X^*Y^{*T})
\end{bmatrix}^T
\left(\sum_{i\neq j}
  \begin{bmatrix}
  \frac{1}{\sqrt{n}}\vec(e_i+e_j)\\
  \vec(z_iz_j^T)\\
  \vec(e_ie_j^T)
  \end{bmatrix}
   \begin{bmatrix}
  \frac{1}{\sqrt{n}}\vec(e_i+e_j)\\
  \vec(z_iz_j^T)\\
  \vec(e_ie_j^T)
  \end{bmatrix}^T
\right)
\begin{bmatrix}
  \vec(\theta^{t}-\theta^*)\\
  \vec(H^{t}-H^*)\\
  \frac1n\vec(X^{t}Y^{tT}-X^*Y^{*T})
\end{bmatrix}\\
&\leq\su \left\|\begin{bmatrix}
  \vec(\theta^{t}-\theta^*)\\
  \vec(H^{t}-H^*)\\
  \frac1n\vec(X^{t}Y^{tT}-X^*Y^{*T})
\end{bmatrix}\right\|^2 \tag{by Assumption \ref{assumption:eigenvalues} and $\mathbf{1}^T(\theta^t-\theta^*)=0$}\\
& =\su\left(\|\theta^t-\theta^{*}\|^2_{2}+\|H^t-H^{*}\|^2_{F}+\frac{1}{n^2}\|X^tY^{tT}-X^{*}Y^{*T}\|^2_{F}\right)
\end{align*} 
and 
\begin{align*}
&\|X^tY^{tT}-X^{*}Y^{*T}\|_{F}\\
&=\|(X^tR^t-X^*)(Y^tR^t)^T+X^{*}(Y^tR^t-Y^*)^T\|_F\\
&\leq \|X^tR^t-X^*\|_F\|Y^tR^t\|+\|X^{*}\|\|Y^tR^t-Y^*\|_F\\
&\leq \|X^tR^t-X^*\|_F\|Y^tR^t-Y^*\|+\|X^tR^t-X^*\|_F\|Y^*\|+\|X^{*}\|\|Y^tR^t-Y^*\|_F\\
&\leq 3 \|X^{*}\|\|F^tR^t-Y^*\|_F.
\end{align*}
For the second term, as bound $\|\nabla_{\Gamma}L_c(\theta^*,H^*,\Gamma^*)\|$ in the proof of Lemma \ref{lem:gradient_norm}, we have with probability at least $1-n^{-10}$ that
\begin{align*}
 \left\|\frac1n\sum_{i\neq j}\left(\frac{e^{P_{ij}^*}}{1+e^{P_{ij}^*}}-A_{ij}\right)e_i e_j^T\right\|\lesssim \sqrt{\frac{\log n}{n}}   .
\end{align*}
As a result, we have
\begin{align*}
 \|D^t\|
 &\lesssim   \frac{\sqrt{\su}}{n}\left(\|\theta^t-\theta^{*}\|_{2}+\|H^t-H^{*}\|_{F}+\frac{1}{n}\|X^*\|\|F^tR^t-F^{*}\|_{F}\right)+\sqrt{\frac{\log n}{n}}\\
 &\lesssim c_{11}\sqrt{\frac{\overline{C}}{n}}+\sqrt{\frac{\log n}{n}} \tag{recall the definition of $\overline{C}$}\\
 &\lesssim \sqrt{\frac{c_{11}^2\overline{C}+\log n}{n}}.
\end{align*}
We then finish the proof.
\end{proof}





\subsection{Proofs of Lemma \ref{lem:ncv1}}\label{pf:lem_ncv1}
Suppose Lemma \ref{lem:ncv1}-Lemma \ref{lem:ncv5} hold for the $t$-th iteration. In the following, we prove Lemma \ref{lem:ncv1} for the $(t+1)$-th iteration. 
By the gradient decent update, we have
\begin{align*}
M^{t+1}=M^t-\eta\cP\left(\nabla_{M}f(M^t,F^t)\right)=\cP\left(M^t-\eta\nabla_{M}f(M^t,F^t)\right).
\end{align*}
Thus, it holds that
\begin{align*}
\|M^{t+1}-M^*\|_F
=\left\|\cP\left(M^t-\eta\nabla_{M}f(M^t,F^t)-M^*\right)\right\|_F
\leq \left\|M^t-\eta\nabla_{M}f(M^t,F^t)-M^*\right\|_F,
\end{align*}
which then gives
\begin{align}\label{ineq30:pf_lem_ncv1}
\left\|\begin{bmatrix}
M^{t+1}-M^{*}\\
F^{t+1}R^t-F^{*}
\end{bmatrix}\right\|_F
\leq 
\left\|\begin{bmatrix}
M^t-\eta\nabla_{M}f(M^t,F^t)-M^*\\
F^{t+1}R^t-F^{*}
\end{bmatrix}\right\|_F.
\end{align}
Consequently, we only need to bound the RHS of \eqref{ineq30:pf_lem_ncv1}. Note that
\begin{align*}
&\begin{bmatrix}
M^t-\eta\nabla_{M}f(M^t,F^t)-M^*\\
F^{t+1}R^t-F^{*}
\end{bmatrix}\\
&=
\begin{bmatrix}
M^t-\eta\nabla_{M}f(M^t,F^t)-M^*\\
\left(F^t-\eta\nabla_F f(M^t,F^t)\right)R^t-F^*
\end{bmatrix}\\
&=\begin{bmatrix}
M^t-\eta\nabla_{M}f(M^t,F^tR^t)
-M^*\\
F^tR^t-\eta\nabla_F f(M^t,F^tR^t)-F^*
\end{bmatrix}\\
&=\begin{bmatrix}
M^t-M^{*}\\
F^tR^t-F^*
\end{bmatrix}-\eta\nabla f(M^t,F^tR^t)\\
&=\begin{bmatrix}
M^t-M^{*}\\
F^tR^t-F^*
\end{bmatrix}-\eta\left(\nabla f_{\aug}(M^t,F^tR^t)-\nabla f_{\aug}(M^*,F^*)\right)+\eta\nabla f_{\diff}(F^tR^t)-\eta\nabla f_{\aug}(M^*,F^*).
\end{align*}
% \begin{align*}
% &\begin{bmatrix}
% M^{t+1}-M^{*}\\
% F^{t+1}R^t-F^{*}
% \end{bmatrix}\\
% &=
% \begin{bmatrix}
% M^t-\eta\nabla_{M}f(M^t,F^t)+\eta
% \begin{bmatrix}
% \mean\left(\nabla_{\theta}f(M^t,F^t)\right)\cdot\mathbf{1}\\
% 0
% \end{bmatrix}-M^*\\
% \left(F^t-\eta\nabla_F f(M^t,F^t)\right)R^t-F^*
% \end{bmatrix}\\
% &=\begin{bmatrix}
% M^t-\eta\nabla_{M}f(M^t,F^tR^t)+\eta
% \begin{bmatrix}
% \mean\left(\nabla_{\theta}f(M^t,F^tR^t)\right)\cdot\mathbf{1}\\
% 0
% \end{bmatrix}-M^*\\
% F^tR^t-\eta\nabla_F f(M^t,F^tR^t)-F^*
% \end{bmatrix}\\
% &=\begin{bmatrix}
% M^t-M^{*}\\
% F^tR^t-F^*
% \end{bmatrix}-\eta\nabla f(M^t,F^tR^t)+\eta\begin{bmatrix}
% \mean\left(\nabla_{\theta}f(M^t,F^tR^t)\right)\cdot\mathbf{1}\\
% 0
% \end{bmatrix}\\
% &=\begin{bmatrix}
% M^t-M^{*}\\
% F^tR^t-F^*
% \end{bmatrix}-\eta\left(\nabla f_{\aug}(M^t,F^tR^t)-\nabla f_{\aug}(M^*,F^*)\right)+\eta\nabla f_{\diff}(F^tR^t)-\eta\nabla f_{\aug}(M^*,F^*)\\
% &\quad+\eta\begin{bmatrix}
% \mean\left(\nabla_{\theta}f(M^t,F^tR^t)\right)\cdot\mathbf{1}\\
% 0
% \end{bmatrix}.
% \end{align*}
Also, it holds that
\begin{align*}
\nabla f_{\aug}(M^t,F^tR^t)-\nabla f_{\aug}(M^*,F^*)=\int^1_0\nabla^2 f_{\aug}\left((M^*,F^*)+\tau(M^t-M^*,F^tR^t-F^*)\right)d \tau\cdot \begin{bmatrix}
M^t-M^{*}\\
F^tR^t-F^*
\end{bmatrix}.
\end{align*}
Thus, we have
\begin{align*}
&\begin{bmatrix}
M^t-\eta\nabla_{M}f(M^t,F^t)-M^*\\
F^{t+1}R^t-F^{*}
\end{bmatrix}\\
&=\left(I-\eta\int^1_0\nabla^2 f_{\aug}\left((M^*,F^*)+\tau(M^t-M^*,F^tR^t-F^*)\right)d \tau\right)\cdot \begin{bmatrix}
M^t-M^{*}\\
F^tR^t-F^*
\end{bmatrix}\\
&\quad +\eta\nabla f_{\diff}(F^tR^t)-\eta\nabla f_{\aug}(M^*,F^*).
\end{align*}
For notation simplicity, we denote 
\begin{align*}
A:=\int^1_0\nabla^2 f_{\aug}\left((M^*,F^*)+\tau(M^t-M^*,F^tR^t-F^*)\right)d \tau.
\end{align*}
Since Lemma \ref{lem:ncv4} holds for the $t$-th iteration, we know $A$ satisfies the local geometry properties as outlined in Lemma \ref{lem:convexity} as long as $c_{41}\leq c_1$, $c_{11}\leq c_2$, $c_{43}\leq c_3$.
By triangle inequality, we have
\begin{align*}
&\left\|\begin{bmatrix}
M^t-\eta\nabla_{M}f(M^t,F^t)-M^*\\
F^{t+1}R^t-F^{*}
\end{bmatrix}\right\|_F\\
&\leq \underbrace{\left\|(I-\eta A)\begin{bmatrix}
M^t-M^{*}\\
F^tR^t-F^*
\end{bmatrix}\right\|_F}_{(1)}+\eta\underbrace{\|\nabla f_{\diff}(F^tR^t)\|_F}_{(2)}+\eta\underbrace{\|\nabla f_{\aug}(M^*,F^*)\|_F}_{(3)}.
% +\eta\cdot\underbrace{\sqrt{n}\left|\mean\left(\nabla_{\theta}f(M^t,F^tR^t)\right)\right|}_{(4)}.
\end{align*}
In the following, we bound (1)-(3), respectively.
\begin{enumerate}
\item We first bound (1).
Note that
\begin{align*}
(1)^2&=\vec
\begin{bmatrix}
M^t-M^{*}\\
F^tR^t-F^{*}
\end{bmatrix}^T
(I-2\eta A+\eta^2 A^2)
\vec
\begin{bmatrix}
M^t-M^{*}\\
F^tR^t-F^{*}
\end{bmatrix}\\
&=\left\|
\begin{bmatrix}
M^t-M^{*}\\
F^tR^t-F^{*}
\end{bmatrix}
\right\|_F^2-2\eta\vec
\begin{bmatrix}
M^t-M^{*}\\
F^tR^t-F^{*}
\end{bmatrix}^T A \ 
\vec
\begin{bmatrix}
M^t-M^{*}\\
F^tR^t-F^{*}
\end{bmatrix}\\
&\quad+\eta^2\vec
\begin{bmatrix}
M^t-M^{*}\\
F^tR^t-F^{*}
\end{bmatrix}^TA^2\ \vec
\begin{bmatrix}
M^t-M^{*}\\
F^tR^t-F^{*}
\end{bmatrix}.
\end{align*}
By Lemma \ref{lem:convexity}, we have
\begin{align*}
% & \vec
% \begin{bmatrix}
% M^t-M^{*}\\
% F^tR^t-F^{*}
% \end{bmatrix}^T A \ 
% \vec
% \begin{bmatrix}
% M^t-M^{*}\\
% F^tR^t-F^{*}
% \end{bmatrix}\geq \underline{C}\left( \|\theta^t-\theta^{*}\|^2_2+\|H^t-H^{*}\|^2_F+\frac{\sigma_{\min}}{8n^2}\|F^tR^t-F^*\|_F^2\right),\\
& \vec
\begin{bmatrix}
M^t-M^{*}\\
F^tR^t-F^{*}
\end{bmatrix}^T A \ 
\vec
\begin{bmatrix}
M^t-M^{*}\\
F^tR^t-F^{*}
\end{bmatrix}\geq \underline{C}\left\|
\begin{bmatrix}
M^t-M^{*}\\
F^tR^t-F^{*}
\end{bmatrix}
\right\|_F^2,\\
&\vec
\begin{bmatrix}
M^t-M^{*}\\
F^tR^t-F^{*}
\end{bmatrix}^TA^2\ \vec
\begin{bmatrix}
M^t-M^{*}\\
F^tR^t-F^{*}
\end{bmatrix}\leq \overline{C}^2\left\|
\begin{bmatrix}
M^t-M^{*}\\
F^tR^t-F^{*}
\end{bmatrix}
\right\|_F^2,
\end{align*}
where the second inequality holds since by Lemma \ref{lem:convexity}, we know $\|A\|\leq  \overline{C}$. As a result, we have
% \begin{align*}
% (1)^2&\leq \left(1+\eta^2\left(\frac{20\su\sigma_{\max}}{n^2}\right)^2-2\underline{C}\eta\right)\left(\|\theta^t-\theta^{*}\|^2_2+\|H^t-H^{*}\|^2_F\right)\\
% &\quad +\left(1+\eta^2\left(\frac{20\su\sigma_{\max}}{n^2}\right)^2-\underline{C}\eta\frac{\sigma_{\min}}{4n^2}\right)\|F^tR^t-F^*\|_F^2\\
% &\leq  \left(1-\underline{C}\eta\right)\left(\|\theta^t-\theta^{*}\|^2_2+\|H^t-H^{*}\|^2_F\right)+\left(1-\frac{\underline{C}\sigma_{\min}}{8n^2}\eta\right)\|F^tR^t-F^*\|_F^2,
% \end{align*}
\begin{align*}
(1)^2&\leq \left(1+\eta^2\overline{C}^2-2\underline{C}\eta\right)
\left\|
\begin{bmatrix}
M^t-M^{*}\\
F^tR^t-F^{*}
\end{bmatrix}
\right\|_F^2\\
&\leq  \left(1-\underline{C}\eta\right)
\left\|
\begin{bmatrix}
M^t-M^{*}\\
F^tR^t-F^{*}
\end{bmatrix}
\right\|_F^2,
\end{align*}
where the second inequality holds as long as $\eta\overline{C}^2\leq \underline{C}$.
This implies 
\begin{align*}
(1)&\leq \left(1-\frac{\underline{C}}{2}\eta\right)
\left\|
\begin{bmatrix}
M^t-M^{*}\\
F^tR^t-F^{*}
\end{bmatrix}
\right\|_F,
\end{align*}
% \begin{align*}
% (1)&\leq \left(1-\frac{\underline{C}}{2}\eta\right)\left(\|\theta^t-\theta^{*}\|_2+\|H^t-H^{*}\|_F\right)+\left(1-\frac{\underline{C}\sigma_{\min}}{16n^2}\eta\right)\|F^tR^t-F^*\|_F,
% \end{align*}
which follows from the fact that $\sqrt{1-x}\leq 1-\frac{x}{2}$.



\item We then bound (2). Note that
\begin{align*}
&\nabla_X f_{\diff}(F^tR^t)=\frac{4c_{\aug}}{n^2}X^t(X^{tT}X^t-Y^{tT}Y^t)R^t,\\
&\nabla_Y f_{\diff}(F^tR^t)=\frac{4c_{\aug}}{n^2}Y^t(Y^{tT}Y^t-X^{tT}X^t)R^t.
\end{align*}
Thus, we have
\begin{align*}
\|\nabla f_{\diff}(F^tR^t)\|_F&\leq \frac{4c_{\aug}}{n^2}\left(\|X^t(X^{tT}X^t-Y^{tT}Y^t)R^t\|_F+\|Y^t(Y^{tT}Y^t-X^{tT}X^t)R^t\|_F\right)\\
&\leq \frac{4c_{\aug}}{n^2}\left(\|X^t\|+\|Y^t\|\right)\|X^{tT}X^t-Y^{tT}Y^t\|_F.
\end{align*}
Since Lemma \ref{lem:ncv1} holds for the $t$-th iteration, we have
\begin{align*}
\|F^t\|=\|F^tR^t\|\leq \|F^tR^t-F^*\|+\|F^*\|\leq 2\|F^*\|,
\end{align*}
where the last inequality holds because by Lemma \ref{lem:ncv1}, we have $\|F^tR^t-F^*\|\ll \|F^*\|$.
Consequently, we have
\begin{align*}
 (2)=\|\nabla f_{\diff}(F^tR^t)\|_F\leq \frac{16c_{\aug}}{n^2} \|F^*\|  \|X^{tT}X^t-Y^{tT}Y^t\|_F.
\end{align*}


\item We then bound (3).
Note that $X^{*T}X^{*}=Y^{*T}Y^{*}$. Thus, we have $\nabla f_{\diff}(F^*)=0$, which implies $\nabla f_{\aug}(M^*,F^*)=\nabla f(M^*,F^*)$.
By Lemma \ref{lem:gradient_norm}, we have 
\begin{align*}
(3)=\|\nabla f(M^*,F^*)\|_F\lesssim \sqrt{n \log n}+c_z\sqrt{p\log n}+c_{\lambda}\sqrt{\frac{\log n}{n}}\cdot \sqrt{\mu r \sigma_{\max}}\lesssim \frac{c_{\lambda}\sqrt{\mu r\sigma_{\max}}}{n}\sqrt{n \log n}
\end{align*}
as long as $\sz^2 p\lesssim n$ and $1\lesssim \frac{c_{\lambda}\sqrt{\mu r\sigma_{\max}}}{n}$.


% \item Finally, we bound (4).
% \textcolor{red}{
% Here 
% \begin{align*}
% (4):= \sqrt{n}\left|\mean\left(\nabla_{\theta}f(M^t,F^tR^t)\right)\right|.
% \end{align*}
% At the beginning of the proof, we already removed this term by considering the projection. Thus, the bound on this term is no longer needed. But we still keep it here in case other parts need this proof.
% }



% Note that
% \begin{align*}
% \nabla_{\theta}f(M^t,F^tR^t)
% &=\nabla_{\theta}L(M^t,F^tR^t)\\
% &=\nabla_{\theta}L(M^*,F^*)+\nabla_{\theta}L(M^t,F^tR^t)-\nabla_{\theta}L(M^*,F^*).
% \end{align*}
% For the first term, we have
% \begin{align*}
% n\cdot \mean\left(\nabla_{\theta}L(M^*,F^*)\right)&=\nabla_{\theta}L(M^*,F^*)^T\cdot\mathbf{1}\\
% &=\frac{2}{\sqrt{n}}\sum_{i\neq j}\left(\frac{e^{P_{ij}^{*}}}{1+e^{P_{ij}^{*}}}-A_{ij}\right)\\
% &=\frac{4}{\sqrt{n}}\sum_{i< j}\left(\frac{e^{P_{ij}^{*}}}{1+e^{P_{ij}^{*}}}-A_{ij}\right)
% \end{align*}
% Since $\sum_{i< j}\left(\frac{e^{P_{ij}^{*}}}{1+e^{P_{ij}^{*}}}-A_{ij}\right)$ is the sum of $n(n-1)/2$ i.i.d mean zero $1$-subgaussian random variables, we have with probability at least $1-n^{-10}$ that
% \begin{align*}
% \left| \sum_{i\neq j}\left(\frac{e^{P_{ij}^{*}}}{1+e^{P_{ij}^{*}}}-A_{ij}\right)\right|\lesssim n\sqrt{\log n},
% \end{align*}
% which implies that
% \begin{align*}
% \left|\mean\left(\nabla_{\theta}L(M^*,F^*)\right)\right|=O\left(\sqrt{\frac{\log n}{n}}\right).    
% \end{align*}
% For the rest of the terms, we have 
% \begin{align*}
% &n\cdot \mean\left(\nabla_{\theta}L(M^t,F^tR^t)-\nabla_{\theta}L(M^*,F^*)\right)\\
% &=\frac{2}{\sqrt{n}}\sum_{i\neq j}\left(\frac{e^{P_{ij}^{t}}}{1+e^{P_{ij}^{t}}}-\frac{e^{P_{ij}^{*}}}{1+e^{P_{ij}^{*}}}\right)\\
% &\leq \frac{1}{2\sqrt{n}}\sum_{i\neq j}\left|P^t_{ij}-P^{*}_{ij}\right| \tag{by mean-value theorem}\\
% &\leq \frac{\sqrt{n}}{2}\sqrt{\sum_{i\neq j}\left|P^t_{ij}-P^{*}_{ij}\right|^2}. \tag{by Cauchy-Schwarz}
% \end{align*}

% Note that
% \begin{align*}
% &\sum_{i\neq j}(P_{ij}^{t}-P_{ij}^*)^2\\
% &=\sum_{i\neq j}\left(\frac{1}{\sqrt{n}}\langle\theta^{t}-\theta^*,e_i+e_j\rangle+\langle H^{t}-H^*,z_iz_j^T\rangle+\frac1n\langle X^{t}Y^{tT}-X^*Y^{*T},e_i e_j^T\rangle\right)^2\\
% &=
% \begin{bmatrix}
%   \vec(\theta^{t}-\theta^*)\\
%   \vec(H^{t}-H^*)\\
%   \frac1n\vec(X^{t}Y^{tT}-X^*Y^{*T})
% \end{bmatrix}^T
% \left(\sum_{i\neq j}
%   \begin{bmatrix}
%   \frac{1}{\sqrt{n}}\vec(e_i+e_j)\\
%   \vec(z_iz_j^T)\\
%   \vec(e_ie_j^T)
%   \end{bmatrix}
%    \begin{bmatrix}
%   \frac{1}{\sqrt{n}}\vec(e_i+e_j)\\
%   \vec(z_iz_j^T)\\
%   \vec(e_ie_j^T)
%   \end{bmatrix}^T
% \right)
% \begin{bmatrix}
%   \vec(\theta^{t}-\theta^*)\\
%   \vec(H^{t}-H^*)\\
%   \frac1n\vec(X^{t}Y^{tT}-X^*Y^{*T})
% \end{bmatrix}\\
% &\lesssim \left\|\begin{bmatrix}
%   \vec(\theta^{t}-\theta^*)\\
%   \vec(H^{t}-H^*)\\
%   \frac1n\vec(X^{t}Y^{tT}-X^*Y^{*T})
% \end{bmatrix}\right\|^2 \tag{by balanced eigenvalues assumption and $\mathbf{1}^T(\theta^t-\theta^*)=0$}\\
% & =\|\theta^t-\theta^{*}\|^2_{2}+\|H^t-H^{*}\|^2_{F}+\frac{1}{n^2}\|X^tY^{tT}-X^{*}Y^{*T}\|^2_{F}.
% \end{align*}
% As a result, we have
% \begin{align*}
% \left|\mean\left(\nabla_{\theta}L(M^t,F^tR^t)-\nabla_{\theta}L(M^*,F^*)\right)\right|
% \lesssim \frac{1}{\sqrt{{n}}}\left(\|\theta^t-\theta^{*}\|_{2}+\|H^t-H^{*}\|_{F}+\frac{1}{n}\|X^tY^{tT}-X^{*}Y^{*T}\|_{F}\right).
% \end{align*}
% Combine the above results, we show that
% \begin{align*}
%  \left|\mean\left(\nabla_{\theta}f(M^t,F^tR^t)\right)\right| 
%  \lesssim O\left(\sqrt{\frac{\log n}{n}}\right)+\frac{1}{\sqrt{{n}}}\left(\|\theta^t-\theta^{*}\|_{2}+\|H^t-H^{*}\|_{F}+\frac{1}{n}\|X^tY^{tT}-X^{*}Y^{*T}\|_{F}\right),
% \end{align*}
% which implies
% \begin{align*}
%  (4)
%  \lesssim O\left(\sqrt{\log n}\right)+\|\theta^t-\theta^{*}\|_{2}+\|H^t-H^{*}\|_{F}+\frac{1}{n}\|X^tY^{tT}-X^{*}Y^{*T}\|_{F}.
% \end{align*}

\end{enumerate}




Consequently, we conclude that
\begin{align*}
&\left\|\begin{bmatrix}
M^t-\eta\nabla_{M}f(M^t,F^t)-M^*\\
F^{t+1}R^t-F^{*}
\end{bmatrix}\right\|_F\\
&\leq\left(1-\frac{\underline{C}}{2}\eta\right)
\left\|
\begin{bmatrix}
M^t-M^{*}\\
F^tR^t-F^{*}
\end{bmatrix}
\right\|_F+\frac{16 \eta c_{\aug}}{n^2} \|F^*\|  \|X^{tT}X^t-Y^{tT}Y^t\|_F+\frac{c_{\lambda}\eta \sqrt{\mu r\sigma_{\max}}}{n}\sqrt{n \log n}.
% &\quad +\eta\left(\|\theta^t-\theta^{*}\|_{2}+\|H^t-H^{*}\|_{F}+\frac{1}{n}\|X^tY^{tT}-X^{*}Y^{*T}\|_{F}\right).
\end{align*}
Recall \eqref{ineq30:pf_lem_ncv1}, we then have
\begin{align*}
 &\left\|\begin{bmatrix}
M^{t+1}-M^{*}\\
F^{t+1}R^t-F^{*}
\end{bmatrix}\right\|_F\\  
&\leq\left(1-\frac{\underline{C}}{2}\eta\right)
\left\|
\begin{bmatrix}
M^t-M^{*}\\
F^tR^t-F^{*}
\end{bmatrix}
\right\|_F+\frac{16 \eta c_{\aug}}{n^2} \|F^*\|  \|X^{tT}X^t-Y^{tT}Y^t\|_F+\frac{c_{\lambda}\eta \sqrt{\mu r\sigma_{\max}}}{n}\sqrt{n \log n}.
\end{align*}
By Lemma \ref{ar:lem1}, we know $\|F^*\|\leq 2\sqrt{\sigma_{\max}}$. By Lemma \ref{lem:ncv5}, we have $\|X^{tT}X^t-Y^{tT}Y^t\|_F\leq c_{51}\eta n^2$. 
We then obtain that
\begin{align*}
 &\left\|\begin{bmatrix}
M^{t+1}-M^{*}\\
F^{t+1}R^t-F^{*}
\end{bmatrix}\right\|_F\\   
&\leq\left(1-\frac{\underline{C}}{2}\eta\right)
\left\|
\begin{bmatrix}
M^t-M^{*}\\
F^tR^t-F^{*}
\end{bmatrix}
\right\|_F
+{32 c_{\aug}c_{51}\sqrt{\sigma_{\max}}\eta^2}+\frac{c_{\lambda}\eta \sqrt{\mu r\sigma_{\max}}}{n}\sqrt{n \log n}.
\end{align*}
Since Lemma \ref{lem:ncv1} holds for the $t$-th iteration, we have
\begin{align*}
 &\left\|\begin{bmatrix}
M^{t+1}-M^{*}\\
F^{t+1}R^t-F^{*}
\end{bmatrix}\right\|_F\\   
&\leq\left(1-\frac{\underline{C}}{2}\eta\right)c_{11}\sqrt{n}+{32 c_{\aug}c_{51}\sqrt{\sigma_{\max}}\eta^2}+\frac{c_{\lambda}\eta \sqrt{\mu r\sigma_{\max}}}{n}\sqrt{n \log n}\\
&\leq c_{11}\sqrt{n}
\end{align*}
as long as $\frac{8 c_{\lambda} \sqrt{\mu r\sigma_{\max}}}{n}\sqrt{ \log n}\leq c_{11} \underline{C} $ and $\frac{256 c_{\aug}c_{51}\sqrt{\sigma_{\max}}\eta}{\sqrt{n}}\leq c_{11} \underline{C} $.
Finally, by the definition of $R^{t+1}$, we have
\begin{align*}
 \|F^{t+1}R^{t+1}-F^{*}\|_F\leq  \|F^{t+1}R^{t}-F^{*}\|_F.   
\end{align*}
Consequently, we have
\begin{align*}
&\left\|\begin{bmatrix}
M^{t+1}-M^{*}\\
F^{t+1}R^{t+1}-F^{*}
\end{bmatrix}\right\|_F  \leq c_{11}\sqrt{n}.
\end{align*}



It remains to show that $\|F^{t+1}R^{t+1}-F^{*}\|\leq c_{14}\sqrt{n}$.
To facilitate analysis, we introduce an auxiliary point $\tilde{F}^{t+1}:=\begin{bmatrix}
\tilde{X}^{t+1}\\
\tilde{Y}^{t+1}
\end{bmatrix}$ where
\begin{align*}
&\tilde{X}^{t+1}={X}^{t}{R}^{t}-\frac{\eta}{n}\sum_{i\neq j}\left(\frac{e^{P_{ij}^{t}}}{1+e^{P_{ij}^{t}}}-A_{ij}\right)e_ie_j^TY^*-\eta\lambda X^*-\frac{4c_{\aug}\eta}{n^2}X^*{R}^{tT}\left({X}^{tT}{X}^{t}-{Y}^{tT}{Y}^{t}\right){R}^{t},\\
&\tilde{Y}^{t+1}={Y}^{t}{R}^{t}-\frac{\eta}{n}\sum_{i\neq j}\left(\frac{e^{P_{ij}^{t}}}{1+e^{P_{ij}^{t}}}-A_{ij}\right)e_je_i^TX^*-\eta\lambda Y^*-\frac{4c_{\aug}\eta}{n^2}Y^*{R}^{tT}\left({Y}^{tT}{Y}^{t}-{X}^{tT}{X}^{t}\right){R}^{t}.
\end{align*}
We then have
\begin{align*}
\|F^{t+1}R^{t+1}-F^{*}\|\leq \underbrace{\|\tilde{F}^{t+1}-F^{*}\|}_{(1)} + \underbrace{\|F^{t+1}R^{t+1}-\tilde{F}^{t+1}\|}_{(2)}.
\end{align*}
In the following, we bound (1) and (2), respectively.
\begin{enumerate}
\item We first bound (1).
Note that
\begin{align*}
&\left\|\tilde{F}^{t+1}-F^{*}\right\|\\
&\leq \left\| 
\begin{bmatrix}
X^t R^t - \frac{8c_{\aug}\eta}{n^2} \left[ (X^t Y^{t T} - \Gamma^{*}) Y^* + \frac{1}{2} X^* R^t (X^t X^t - Y^{t T} Y^t) R^t \right] - X^* \\
Y^t R^t -\frac{8c_{\aug}\eta}{n^2} \left[ (X^t Y^{t T} - \Gamma^{*}) X^* + \frac{1}{2} Y^* R^t (Y^{t T} Y^t - X^t X^t) R^t \right] - Y^* 
\end{bmatrix}\right\|\\
&\quad +\frac{\eta}{n} \left\| 
\begin{bmatrix}
\sum_{i\neq j}\left(\frac{e^{P_{ij}^{t}}}{1+e^{P_{ij}^{t}}}-\frac{e^{P_{ij}^{*}}}{1+e^{P_{ij}^{*}}}\right)e_ie_j^TY^*  \\
 \sum_{i\neq j}\left(\frac{e^{P_{ij}^{t}}}{1+e^{P_{ij}^{t}}}-\frac{e^{P_{ij}^{*}}}{1+e^{P_{ij}^{*}}}\right)e_je_i^TX^*
\end{bmatrix}-\frac{8c_{\aug}}{n}
\begin{bmatrix}
(X^t Y^{t T} - \Gamma^{*}) Y^{*}  \\
 (X^t Y^{t T} - \Gamma^{*}) X^* 
\end{bmatrix}\right\|\\
&\quad +\frac{\eta}{n}\left\| 
\begin{bmatrix}
\sum_{i\neq j}\left(\frac{e^{P_{ij}^{*}}}{1+e^{P_{ij}^{*}}}-A_{ij}\right)e_ie_j^TY^*  \\
 \sum_{i\neq j}\left(\frac{e^{P_{ij}^{*}}}{1+e^{P_{ij}^{*}}}-A_{ij}\right)e_je_i^TX^*
\end{bmatrix}\right\|+\eta\lambda \|F^{*}\|\\
&\leq \left\| 
\begin{bmatrix}
X^t R^t - \frac{8c_{\aug}\eta}{n^2} \left[ (X^t Y^{t T} - \Gamma^{*}) Y^* + \frac{1}{2} X^* R^t (X^t X^t - Y^{t T} Y^t) R^t \right] - X^* \\
Y^t R^t -\frac{8c_{\aug}\eta}{n^2} \left[ (X^t Y^{t T} - \Gamma^{*}) X^* + \frac{1}{2} Y^* R^t (Y^{t T} Y^t - X^t X^t) R^t \right] - Y^* 
\end{bmatrix}\right\|\\
&\quad +\frac{\eta}{n} \left\| 
\sum_{i\neq j}\left(\frac{e^{P_{ij}^{t}}}{1+e^{P_{ij}^{t}}}-\frac{e^{P_{ij}^{*}}}{1+e^{P_{ij}^{*}}}\right)e_ie_j^T- \frac{8c_{\aug}}{n}(X^t Y^{t T} - \Gamma^{*})
\right\| \|F^{*}\|\\
&\quad +\frac{\eta}{n}\left\| 
\sum_{i\neq j}\left(\frac{e^{P_{ij}^{*}}}{1+e^{P_{ij}^{*}}}-A_{ij}\right)e_ie_j^T \right\|\|F^{*}\|+\eta\lambda \|F^{*}\|.
\end{align*}
For the first term, as bounding $\beta_1$ in the proof of Lemma 11 in \cite{chen2020noisy}, we have
\begin{align*}
 &\left\| 
\begin{bmatrix}
X^t R^t - \frac{8c_{\aug}\eta}{n^2} \left[ (X^t Y^{t T} - \Gamma^{*}) Y^* + \frac{1}{2} X^* R^t (X^t X^t - Y^{t T} Y^t) R^t \right] - X^* \\
Y^t R^t -\frac{8c_{\aug}\eta}{n^2} \left[ (X^t Y^{t T} - \Gamma^{*}) X^* + \frac{1}{2} Y^* R^t (Y^{t T} Y^t - X^t X^t) R^t \right] - Y^* 
\end{bmatrix}\right\|\\
&\leq \left(1-\eta\frac{8c_{\aug}\sigma_{\min}}{n^2}\right)\|F^tR^t-F^{*}\|   + \frac{32c_{\aug}\eta}{n^2}\|F^tR^t-F^{*}\|^2\|F^*\|
\end{align*}
For the second term, we have 
\begin{align*}
&\frac{1}{n} \left\| 
\sum_{i\neq j}\left(\frac{e^{P_{ij}^{t}}}{1+e^{P_{ij}^{t}}}-\frac{e^{P_{ij}^{*}}}{1+e^{P_{ij}^{*}}}\right)e_ie_j^T- \frac{8c_{\aug}}{n}(X^t Y^{t T} - \Gamma^{*})
\right\|\\
&\leq \frac{1}{n} \left\| 
\sum_{i\neq j}\left(\frac{e^{P_{ij}^{t}}}{1+e^{P_{ij}^{t}}}-\frac{e^{P_{ij}^{*}}}{1+e^{P_{ij}^{*}}}\right)e_ie_j^T- \frac{8c_{\aug}}{n}(X^t Y^{t T} - \Gamma^{*})
\right\|_F.
\end{align*}
By the mean-value theorem, there exists $\{c_{ij}\}$ such that
\begin{align*}
\frac{e^{P_{ij}^{t}}}{1+e^{P_{ij}^{t}}}-\frac{e^{P_{ij}^{*}}}{1+e^{P_{ij}^{*}}}
=\frac{e^{c_{ij}}}{(1+e^{c_{ij}})^2}\left(P_{ij}^{t}-P_{ij}^{*}\right).
\end{align*}
Note that $\frac{e^{c_{ij}}}{(1+e^{c_{ij}})^2}\leq \frac14$ and $\left|\frac{e^{c_{ij}}}{(1+e^{c_{ij}})^2}-8c_{\aug}\right|\lesssim 1$, Thus, we have
\begin{align*}
&\left\| 
\sum_{i\neq j}\left(\frac{e^{P_{ij}^{t}}}{1+e^{P_{ij}^{t}}}-\frac{e^{P_{ij}^{*}}}{1+e^{P_{ij}^{*}}}\right)e_ie_j^T- \frac{8c_{\aug}}{n}(X^t Y^{t T} - \Gamma^{*})
\right\|_F\\
&=\left\| 
\sum_{i\neq j}\frac{e^{c_{ij}}}{(1+e^{c_{ij}})^2}\left(P_{ij}^{t}-P_{ij}^{*}\right)e_ie_j^T- \frac{8c_{\aug}}{n}(X^t Y^{t T} - \Gamma^{*})
\right\|_F\\
&\lesssim \|\theta^t-\theta^{*}\|_{2}+\|H^t-H^{*}\|_{F}+\frac{1}{n}\|X^tY^{tT}-X^{*}Y^{*T}\|_{F}\\
& \lesssim\|\theta^t-\theta^{*}\|_{2}+\|H^t-H^{*}\|_{F}+\frac{1}{n}\|X^*\|\|F^tR^t-F^{*}\|_{F}\\
& \lesssim \frac{\sqrt{\sigma_{\max}}}{n} c_{11}\sqrt{n},
\end{align*}
where the last inequality follows from Lemma \ref{lem:ncv1}.
Consequently, we obtain
\begin{align*}
\frac{1}{n} \left\| 
\sum_{i\neq j}\left(\frac{e^{P_{ij}^{t}}}{1+e^{P_{ij}^{t}}}-\frac{e^{P_{ij}^{*}}}{1+e^{P_{ij}^{*}}}\right)e_ie_j^T- \frac{8c_{\aug}}{n}(X^t Y^{t T} - \Gamma^{*})
\right\|\lesssim \frac{\sqrt{\sigma_{\max}}}{n^{3/2}} c_{11}.
\end{align*}
For the third term, as bound $\|\nabla_{\Gamma}L_c(\theta^*,H^*,\Gamma^*)\|$ in the proof of Lemma \ref{lem:gradient_norm}, we have
\begin{align*}
 \left\|\frac1n\sum_{i\neq j}\left(\frac{e^{P_{ij}^*}}{1+e^{P_{ij}^*}}-A_{ij}\right)e_i e_j^T\right\|\lesssim \sqrt{\frac{\log n}{n}}   .
\end{align*}
Consequently, we have
\begin{align*}
&\left\|\tilde{F}^{t+1}-F^{*}\right\|\\
&\leq  \left(1-\eta\frac{8c_{\aug}\sigma_{\min}}{n^2}\right)\|F^tR^t-F^{*}\|   + \frac{32c_{\aug}\eta}{n^2}\|F^tR^t-F^{*}\|^2\|F^*\|\\
&\quad+c\eta\frac{{\sigma_{\max}}}{n^{3/2}} c_{11}+c{\eta}\|F^*\|\sqrt{\frac{\log n}{n}}+\eta\lambda \|F^{*}\| \\
&\leq  \left(1-\eta\frac{8c_{\aug}\sigma_{\min}}{n^2}\right)\|F^tR^t-F^{*}\|   + \eta\frac{64c_{\aug}\sqrt{\sigma_{\max}}}{n^2}\|F^tR^t-F^{*}\|^2\\
&\quad+c\eta\frac{{\sigma_{\max}}}{n^{3/2}} c_{11}+c{\eta}\sqrt{\frac{\sigma_{\max}\log n}{n}}+2\eta\lambda\sqrt{\sigma_{\max}} \\
&\leq  \left(1-\eta\frac{8c_{\aug}\sigma_{\min}}{n^2}\right)c_{14}\sqrt{n}  + \eta\frac{64c_{\aug}\sqrt{\sigma_{\max}}}{n}c_{14}^2\\
&\quad+c\eta\frac{{\sigma_{\max}}}{n^{3/2}} c_{11}+c{\eta}\sqrt{\frac{\sigma_{\max}\log n}{n}}+2\eta\lambda\sqrt{\sigma_{\max}} \\
&\leq \left(1-\eta\frac{c_{\aug}\sigma_{\min}}{n^2}\right)c_{14}\sqrt{n}
\end{align*}
as long as $\sigma_{\min}\gtrsim \sqrt{n\sigma_{\max}}c_{14}$ and $\lambda+\sqrt{\frac{\log n}{n}}+\frac{\sqrt{\sigma_{\max}}}{n^{3/2}}c_{11}\lesssim \frac{c_{\aug}\sigma_{\min}}{n^{3/2}\sqrt{\sigma_{\max}}}c_{14}$.

\textcolor{red}{
Question:
The above condition implies $c_{14}\gtrsim \kappa c_{11}$. However, since the spectral norm is smaller than the Frobenius norm, we need $c_{14}\leq c_{11}$.
}



\item We then bound (2).
Note that by the above arguments, we have
\begin{align*}
\|F^{* T}\tilde{F}^{t+1}-F^{* T}F^{*}\|\leq \|F^*\|\|\tilde{F}^{t+1}-F^{*}\|\leq 2c_{14}\sqrt{n\sigma_{\max}}\leq \sigma_{\min},
\end{align*}
which then implies the following claim.
\begin{claim}\label{claim1:lem_ncv1}
We have
\begin{align*}
I_r = \argmin_{R\in\cO^{r\times r}}\left\|\tilde{F}^{t+1}R-F^*\right\|_F.
\end{align*}
\end{claim}
\begin{proof}
See Claim 4 in \cite{chen2020noisy}.
\end{proof}

We intend to apply Lemma \ref{ar:lem3} with $F_0=F^*, F_1=\tilde{F}^{t+1}, F_2=F^{t+1}R^t$, for which we need to check the two conditions therein.
First, we already have
\begin{align*}
\|F_1-F_0\|\|F_0\|=\|\tilde{F}^{t+1}-F^*\|\|F^*\|\leq \sigma_{\min}=\frac12 \sigma_r^2(F_0).
\end{align*}
Second, note that $\|F_1-F_2\|\|F_0\|=\|\tilde{F}^{t+1}-F^{t+1}R^t\|\|F^*\|$, thus we control $\|\tilde{F}^{t+1}-F^{t+1}R^t\|$ in the following.
Note that
\begin{align*}
    &F^{t+1} R^{t} - \tilde{F}^{t+1} = -\eta \begin{bmatrix} B & 0 \\ 0 & B^\top \end{bmatrix} \begin{bmatrix} Y^{t}R^{t}-Y^*  \\ X^{t}R^{t}-X^* \end{bmatrix} + \frac{4c_{\aug}\eta}{n^2} \begin{bmatrix} X^\star \\ -Y^\star \end{bmatrix} R^{t \top} C R^{t} - \eta \lambda\begin{bmatrix}   X^{t}R^{t}-X^*\\ Y^{t}R^{t}-Y^* \end{bmatrix} ,
\end{align*}
where we denote
\begin{align*}
 &B := \frac1n\sum_{i\neq j}\left(\frac{e^{P_{ij}^{t}}}{1+e^{P_{ij}^{t}}}-A_{ij}\right)e_ie_j^T,\\ 
 &C := X^{t \top} X^{t} - Y^{t \top} Y^{t}.
\end{align*}
This enables us to obtain
\begin{align*}
 &\left\|F^{t+1} R^{t} - \tilde{F}^{t+1}\right\|  \leq \eta \left\| B \right\| \left\| F^{t}R^{t}-F^*\right\| + \frac{4c_{\aug}\eta}{n^2} \left\| F^* \right\| \left\| C \right\|_F +\eta \lambda\left\| F^{t}R^{t}-F^*\right\|.   
\end{align*}
By Lemma \ref{lem:gradient_spectral}, we have
\begin{align*}
\|B\|\lesssim \sqrt{\frac{c_{11}^2\overline{C}+\log n}{n}},
\end{align*}
which implies 
\begin{align*}
 &\left\|F^{t+1} R^{t} - \tilde{F}^{t+1}\right\|    \\
 &\leq c{\eta}\left\| F^{t}R^{t}-F^*\right\|\sqrt{\frac{c_{11}^2\overline{C}+\log n}{n}}+ \frac{4c_{\aug}\eta}{n^2} \left\| F^* \right\| \left\|X^{t \top} X^{t} - Y^{t \top} Y^{t}\right\|_F +\eta \lambda\left\| F^{t}R^{t}-F^*\right\|\\
 &\lesssim \eta\left(c_{14}\sqrt{c_{11}^2\overline{C}+\log n}+c_{\aug}c_{51}\eta\sqrt{\sigma_{\max}}+\lambda c_{14}\sqrt{n}\right).
\end{align*}
An immediate consequence is that
\begin{align*}
 \|F_1-F_2\|\|F_0\|=\|\tilde{F}^{t+1}-F^{t+1}R^t\|\|F^*\|\leq    \frac{\sigma_{\min}}{2}=\frac14 \sigma_r^2(F_0)
\end{align*}
as long as $\eta\ll \frac{\sigma_{\min}}{\sqrt{n\sigma_{\max}}}$.

Since the two conditions in Lemma \ref{ar:lem3} holds with $F_0=F^*, F_1=\tilde{F}^{t+1}, F_2=F^{t+1}R^t$, we have
\begin{align*}
(2)&=\left\|\tilde{F}^{t+1}-F^{t+1}R^{t+1}\right\|\\
&\leq 5\kappa\left\|\tilde{F}^{t+1}-F^{t+1}R^{t}\right\|\\
& \lesssim \eta\kappa\left(c_{14}\sqrt{c_{11}^2\overline{C}+\log n}+c_{\aug}c_{51}\eta\sqrt{\sigma_{\max}}+\lambda c_{14}\sqrt{n}\right).
\end{align*}

\end{enumerate}

Combine the results for (1) and (2), we have
\begin{align*}
&\|F^{t+1}R^{t+1}-F^{*}\|\\
&\leq \left(1-\eta\frac{c_{\aug}\sigma_{\min}}{n^2}\right)c_{14}\sqrt{n}+c\eta\kappa\left(c_{14}\sqrt{c_{11}^2\overline{C}+\log n}+c_{\aug}c_{51}\eta\sqrt{\sigma_{\max}}+\lambda c_{14}\sqrt{n}\right)\\
&\leq c_{14}\sqrt{n}
\end{align*}
as long as $n$ large enough.
We then finish the proofs.



\subsection{Proofs of Lemma \ref{lem:ncv2}}\label{pf:lem_ncv2}
Suppose Lemma \ref{lem:ncv1}-Lemma \ref{lem:ncv5} hold for the $t$-th iteration. In the following, we prove Lemma \ref{lem:ncv2} for the $(t+1)$-th iteration.
More specifically, we fix $m$ and aim to bound
\begin{align*}
\left\|
\begin{bmatrix}
M^{t+1,(m)}-M^{t+1}\\
F^{t+1,(m)}O^{t+1,(m)}-F^{t+1}R^{t+1}
\end{bmatrix}
\right\|_F.
\end{align*}
\begin{claim}\label{claim:lem_ncv2}
It holds that
\begin{align*}
\|F^{t+1}R^{t+1}-F^{t+1,(m)}O^{t+1,(m)}\|_F\leq \|F^{t+1}R^{t}-F^{t+1,(m)}O^{t,(m)}\|_F.
\end{align*}
\end{claim}
\begin{proof}[Proof of Claim]
By the definition of $O^{t+1,(m)}$, for any $O\in\cO^{r\times r}$, we have
\begin{align*}
\|F^{t+1}R^{t+1}-F^{t+1,(m)}O^{t+1,(m)}\|_F\leq \|F^{t+1}R^{t+1}-F^{t+1,(m)}O\|_F.
\end{align*}
Choosing $O=O^{t,(m)}(R^t)^{-1}R^{t+1}$, we then have
\begin{align*}
\|F^{t+1}R^{t+1}-F^{t+1,(m)}O\|_F&=\|F^{t+1}R^{t+1}-F^{t+1,(m)}O^{t,(m)}(R^t)^{-1}R^{t+1}\|_F\\
&=\|F^{t+1}-F^{t+1,(m)}O^{t,(m)}(R^t)^{-1}\|_F\\
&=\|F^{t+1}R^t-F^{t+1,(m)}O^{t,(m)}\|_F,
\end{align*}
which then finishes the proofs.
\end{proof}

By Claim \ref{claim:lem_ncv2}, we only need to bound $\|F^{t+1}R^{t}-F^{t+1,(m)}O^{t,(m)}\|_F$.

Moreover, by the gradient decent update and the fact that $\nabla_M f(M,F)=\nabla_M f_{\aug}(M,F)$, we have
\begin{align*}
&M^{t+1}
=M^t-\eta\cP\left(\nabla_{M}f_{\aug}(M^t,F^t)\right)
=\cP\left(M^t-\eta\nabla_{M}f_{\aug}(M^t,F^t)\right)\\
&M^{t+1,(m)}
=M^{t,(m)}-\eta\cP\left(\nabla_{M}f^{(m)}_{\aug}(M^{t,(m)},F^{t,(m)})\right)
=\cP\left(M^{t,(m)}-\eta\nabla_{M}f^{(m)}_{\aug}(M^{t,(m)},F^{t,(m)})\right).
\end{align*}
It then holds that
\begin{align}\label{ineq30:pr_lem_ncv2}
&\left\|M^{t+1}-M^{t+1,(m)}\right\|_F\notag\\
&\leq \left\|\left(M^t-\eta\nabla_{M}f_{\aug}(M^t,F^t)\right)-\left(M^{t,(m)}-\eta\nabla_{M}f^{(m)}_{\aug}(M^{t,(m)},F^{t,(m)})\right)\right\|_F.
\end{align}
Thus, we only need to control the RHS of \eqref{ineq30:pr_lem_ncv2}.


Note that
\begin{align*}
&M^t-\eta\nabla_{M}f_{\aug}(M^t,F^t)
-
\left(
M^{t,(m)}-\eta\nabla_{M}f^{(m)}_{\aug}(M^{t,(m)},F^{t,(m)})
\right)\\
&=M^t-M^{t,(m)}-\eta\left(\nabla_{M}f_{\aug}(M^t,F^t)-\nabla_{M}f_{\aug}(M^{t,(m)},F^{t,(m)})\right)\\
&\quad +\eta\left(\nabla_{M}f^{(m)}_{\aug}(M^{t,(m)},F^{t,(m)})-\nabla_{M}f_{\aug}(M^{t,(m)},F^{t,(m)})\right)\\
&=M^t-M^{t,(m)}-\eta\left(\nabla_{M}f_{\aug}(M^t,F^tR^t)-\nabla_{M}f_{\aug}(M^{t,(m)},F^{t,(m)}O^{t,(m)})\right)\\
&\quad +\eta\left(\nabla_{M}f^{(m)}(M^{t,(m)},F^{t,(m)}O^{t,(m)})-\nabla_{M}f(M^{t,(m)},F^{t,(m)}O^{t,(m)})\right),
\end{align*}
% \begin{align*}
% &M^{t+1}-M^{t+1,(m)}\\
% &=M^t-\eta\nabla_{M}f_{\aug}(M^t,F^t)+\eta
% \begin{bmatrix}
% \mean\left(\nabla_{\theta}f(M^t,F^t)\right)\cdot\mathbf{1}\\
% 0
% \end{bmatrix}\\
% &\quad-
% \left(
% M^{t,(m)}-\eta\nabla_{M}f^{(m)}_{\aug}(M^{t,(m)},F^{t,(m)})+\eta
% \begin{bmatrix}
% \mean\left(\nabla_{\theta}f^{(m)}(M^{t,(m)},F^{t,(m)})\right)\cdot\mathbf{1}\\
% 0
% \end{bmatrix}
% \right)\\
% &=M^t-M^{t,(m)}-\eta\left(\nabla_{M}f_{\aug}(M^t,F^t)-\nabla_{M}f_{\aug}(M^{t,(m)},F^{t,(m)})\right)\\
% &\quad +\eta\left(\nabla_{M}f^{(m)}_{\aug}(M^{t,(m)},F^{t,(m)})-\nabla_{M}f_{\aug}(M^{t,(m)},F^{t,(m)})\right)\\
% &\quad+\eta
% \begin{bmatrix}
% \mean\left(\nabla_{\theta}f(M^t,F^t)-\nabla_{\theta}f^{(m)}(M^{t,(m)},F^{t,(m)})\right)\cdot\mathbf{1}\\
% 0
% \end{bmatrix}\\
% &=M^t-M^{t,(m)}-\eta\left(\nabla_{M}f_{\aug}(M^t,F^tR^t)-\nabla_{M}f_{\aug}(M^{t,(m)},F^{t,(m)}O^{t,(m)})\right)\\
% &\quad +\eta\left(\nabla_{M}f^{(m)}(M^{t,(m)},F^{t,(m)}O^{t,(m)})-\nabla_{M}f(M^{t,(m)},F^{t,(m)}O^{t,(m)})\right)\\
% &\quad+\eta
% \begin{bmatrix}
% \mean\left(\nabla_{\theta}f(M^t,F^tR^t)-\nabla_{\theta}f^{(m)}(M^{t,(m)},F^{t,(m)}O^{t,(m)})\right)\cdot\mathbf{1}\\
% 0
% \end{bmatrix},
% \end{align*}
and 
\begin{align*}
&F^{t+1}R^t-F^{t+1,(m)}O^{t,(m)}\\
&=F^{t}R^t-F^{t,(m)}O^{t,(m)}-\eta\left(\nabla_F f_{\aug}(M^t,F^tR^t)-\nabla_F f_{\aug}(M^{t,(m)},F^{t,(m)}O^{t,(m)})\right)\\
&\quad+\eta\left(\nabla_F f^{(m)}(M^{t,(m)},F^{t,(m)}O^{t,(m)})-\nabla_F f(M^{t,(m)},F^{t,(m)}O^{t,(m)})\right)\\
&\quad+\eta\left(\nabla_F f_{\diff}(M^t,F^tR^t)-\nabla_F f_{\diff}(M^{t,(m)},F^{t,(m)}O^{t,(m)})\right).
\end{align*}
As a result, we have
\begin{align*}
&\begin{bmatrix}
M^t-\eta\nabla_{M}f_{\aug}(M^t,F^t)
-
\left(
M^{t,(m)}-\eta\nabla_{M}f^{(m)}_{\aug}(M^{t,(m)},F^{t,(m)})
\right)\\
F^{t+1}R^t-F^{t+1,(m)}O^{t,(m)}
\end{bmatrix}\\
&=\underbrace{\left(I-\eta A\right)
\begin{bmatrix}
M^{t}-M^{t,(m)}\\
F^{t}R^t-F^{t,(m)}O^{t,(m)}
\end{bmatrix}}_{(1)}\\
&\quad +\eta\underbrace{\left(\nabla f^{(m)}(M^{t,(m)},F^{t,(m)}O^{t,(m)})-\nabla f(M^{t,(m)},F^{t,(m)}O^{t,(m)})\right)}_{(2)}\\
% &\quad+\eta
% \underbrace{\begin{bmatrix}
% \mean\left(\nabla_{\theta}f(M^t,F^tR^t)-\nabla_{\theta}f^{(m)}(M^{t,(m)},F^{t,(m)}O^{t,(m)})\right)\cdot\mathbf{1}\\
% 0
% \end{bmatrix}}_{(3)}\\
&\quad+\eta\underbrace{\left(\nabla_F f_{\diff}(M^t,F^tR^t)-\nabla_F f_{\diff}(M^{t,(m)},F^{t,(m)}O^{t,(m)})\right)}_{(3)}
\end{align*}
where
\begin{align*}
A=\int^1_0\nabla^2 f_{\aug}\left((M^{t,(m)},F^{t,(m)}O^{t,(m)})+\tau (M^t-M^{t,(m)},F^tR^t-F^{t,(m)}O^{t,(m)})\right)d\tau.
\end{align*}
In the following, we bound the Frobenius norm of (1)-(3), respectively.
\begin{enumerate}
\item  We first bound (1).
Since Lemma \ref{lem:ncv2} and Lemma \ref{lem:ncv4} hold for the $t$-th iteration, we have
\begin{align*}
&\left\|\theta^{t,(m)}+\tau\left(\theta^t-\theta^{t,(m)}\right)-\theta^*\right\|_{\infty}
\leq \|\theta^t-\theta^*\|_{\infty}+(1-\tau)\|\theta^{t,(m)}-\theta^t\|_{\infty}\leq c_{41}+c_{21}\leq c_1\\
&\left\|H^{t,(m)}+\tau\left(H^t-H^{t,(m)}\right)-H^*\right\|_{F}   \leq \|H^t-H^*\|_{F}+(1-\tau)\|H^{t,(m)}-H^t\|_{F}\leq c_{11}\sqrt{n}+c_{21}\leq c_2\sqrt{n}\\
&\left\|F^{t,(m)}O^{t,(m)}+\tau\left(F^tR^t-F^{t,(m)}O^{t,(m)}\right)-F^*\right\|_{2,\infty}   \\
&\quad\leq \|F^tR^t-F^*\|_{2,\infty}+(1-\tau)\|F^{t,(m)}O^{t,(m)}-F^tR^t\|_{2,\infty}\\
&\quad\leq \|F^tR^t-F^*\|_{2,\infty}+\|F^{t,(m)}O^{t,(m)}-F^tR^t\|_{F}\leq c_{43}+c_{21}\leq c_3.
\end{align*}
Moreover, we have $\mathbf{1}^T(\theta^t-\theta^{t,(m)})=0$ by the GD update and $\|F^{t}R^t-F^*\|\leq c_{14}\sqrt{n}\leq c_4\sqrt{n}$ by Lemma \ref{lem:ncv1} for the $t$-th iteration. Thus Lemma \ref{lem:convexity} can be applied to bound the Frobenius norm of (1). Follow the same argument as bounding term (1) in Appendix \ref{pf:lem_ncv1}, we have
\begin{align*}
\|(1)\|_F\leq \left(1-\frac{\underline{C}}{2}\eta\right)
\left\|
\begin{bmatrix}
M^{t}-M^{t,(m)}\\
F^{t}R^t-F^{t,(m)}O^{t,(m)}
\end{bmatrix}
\right\|_F
\end{align*}





\item  We then bound (2).
Note that
\begin{align*}
(2)&=\nabla L^{(m)}(M^{t,(m)},F^{t,(m)}O^{t,(m)})-\nabla L(M^{t,(m)},F^{t,(m)}O^{t,(m)})\\
&=\sum_{i\neq m}\left(\frac{e^{P_{im}^*}}{1+e^{P_{im}^*}}-A_{im}\right)
\begin{bmatrix}
\frac{1}{\sqrt{n}}(e_i+e_m)\\
z_iz_m^T\\
\frac1n e_ie_m^T Y^{t,(m)}O^{t,(m)}\\
\frac1n e_me_i^T X^{t,(m)}O^{t,(m)}
\end{bmatrix}
+
\sum_{i\neq m}\left(\frac{e^{P_{mi}^*}}{1+e^{P_{mi}^*}}-A_{mi}\right)
\begin{bmatrix}
\frac{1}{\sqrt{n}}(e_i+e_m)\\
z_mz_i^T\\
\frac1n e_me_i^T Y^{t,(m)}O^{t,(m)}\\
\frac1n e_ie_m^T X^{t,(m)}O^{t,(m)}
\end{bmatrix}.
\end{align*}
Since the first and second terms are similar, we only focus on bounding the Frobenius norm of the first term in the following.
It can be seen that
\begin{align*}
\left(\frac{1}{\sqrt{n}}\sum_{i\neq m}\left(\frac{e^{P_{im}^*}}{1+e^{P_{im}^*}}-A_{im}\right)(e_i+e_m)\right)_j=
\begin{cases} 
      \frac{1}{\sqrt{n}}\left(\frac{e^{P_{jm}^*}}{1+e^{P_{jm}^*}}-A_{jm}\right) & j\neq m \\
      \frac{1}{\sqrt{n}}\sum_{i\neq m}\left(\frac{e^{P_{im}^*}}{1+e^{P_{im}^*}}-A_{im}\right) & j=m 
   \end{cases}.
\end{align*}
Since $\sum_{i\neq m}\left(\frac{e^{P_{im}^*}}{1+e^{P_{im}^*}}-A_{im}\right) $ is the sum of $n-1$ i.i.d mean zero $1$-subgaussian random variables, we have with probability at least $1-n^{-10}$ that $|\sum_{i\neq m}\left(\frac{e^{P_{im}^*}}{1+e^{P_{im}^*}}-A_{im}\right)|\lesssim \sqrt{n\log n}$. This implies with probability at least $1-n^{-10}$ that
\begin{align}\label{ineq1:lem_ncv2}
\left\|\frac{1}{\sqrt{n}}\sum_{i\neq m}\left(\frac{e^{P_{im}^*}}{1+e^{P_{im}^*}}-A_{im}\right)(e_i+e_m)\right\|_2\lesssim \sqrt{\frac{n-1}{n}+\log n}\lesssim\sqrt{\log n}.
\end{align}
In the following, we apply matrix Berstein's inequality to bound the Frobenius norms of the rest of the terms.
Notice that
\begin{align*}
    &\max\Bigg\{\left\|\sum_{i\neq m}\bbE\left[\left(\frac{e^{P_{im}^*}}{1+e^{P_{im}^*}}-A_{im}\right)^2\vec(z_iz_m^T)\vec(z_iz_m^T)^T\right]\right\|,\\
    &\qquad\qquad\left\|\sum_{i\neq m}\bbE\left[\left(\frac{e^{P_{im}^*}}{1+e^{P_{im}^*}}-A_{im}\right)^2\vec(z_iz_m^T)^T\vec(z_iz_m^T)\right]\right\|\Bigg\}\\
    &\quad\leq \sum_{i\neq m}\|\vec(z_iz_m^T)\|_2^2=\sum_{i\neq m}\|z_iz_m^T\|_F^2=\sum_{i\neq m}\|z_i\|^2_2\|z_m\|_2^2\lesssim \frac{\sz^2}{n}.
\end{align*}
Thus by matrix Berstein's inequality, we have with probability at least $1-n^{-10}$ that
\begin{align}\label{ineq2:lem_ncv2}
  \left\|\sum_{i\neq m}\left(\frac{e^{P_{im}^*}}{1+e^{P_{im}^*}}-A_{im}\right)z_iz_m^T\right\|_F=\left\|\sum_{i\neq m}\left(\frac{e^{P_{im}^*}}{1+e^{P_{im}^*}}-A_{im}\right)\vec(z_iz_m^T)\right\|_2 \lesssim \sz\sqrt{\frac{\log n}{n}}.
\end{align}
Notice that
\begin{align*}
    &\max\Bigg\{\left\|\sum_{i\neq m}\bbE\left[\left(\frac{e^{P_{im}^*}}{1+e^{P_{im}^*}}-A_{im}\right)^2\vec(e_me_i^T Y^{t,(m)}O^{t,(m)})\vec(e_me_i^T Y^{t,(m)}O^{t,(m)})^T\right]\right\|,\\
    &\qquad\qquad\left\|\sum_{i\neq m}\bbE\left[\left(\frac{e^{P_{im}^*}}{1+e^{P_{im}^*}}-A_{im}\right)^2\vec(e_me_i^T Y^{t,(m)}O^{t,(m)})^T\vec(e_me_i^T Y^{t,(m)}O^{t,(m)})\right]\right\|\Bigg\}\\
    &\quad\leq \sum_{i\neq m}\|\vec(e_me_i^T Y^{t,(m)}O^{t,(m)})\|_2^2\\
    &\quad=\sum_{i\neq m}\|e_me_i^T Y^{t,(m)}O^{t,(m)}\|_F^2\\
    &\quad=\sum_{i\neq m}\Tr\left(e_me_i^T Y^{t,(m)}(Y^{t,(m)})^{T}e_i e_m^T\right)\\
    &\quad = \sum_{i\neq m}\left( Y^{t,(m)}(Y^{t,(m)})^{T}\right)_{ii}\\
    &\quad \leq \|Y^{t,(m)}\|_F^2\\
    &\quad\leq (\|Y^{t,(m)}O^{t,(m)}-Y^{t}R^t\|_F+\|Y^{t}R^t-Y^*\|_F+\|Y^*\|_F)^2\lesssim \mu r\sigma_{\max},
\end{align*}
where the last equation follows from Assumption \ref{assumption:incoherent} and the fact that Lemma \ref{lem:ncv1} and Lemma \ref{lem:ncv2} hold for the $t$-th iteration.
Thus by matrix Berstein's inequality, we have with probability at least $1-n^{-10}$ that
\begin{align}\label{ineq3:lem_ncv2}
  \left\|\frac1n\sum_{i\neq m}\left(\frac{e^{P_{im}^*}}{1+e^{P_{im}^*}}-A_{im}\right)e_me_i^T Y^{t,(m)}O^{t,(m)}\right\|_F&=\left\|\frac1n\sum_{i\neq m}\left(\frac{e^{P_{im}^*}}{1+e^{P_{im}^*}}-A_{im}\right)\vec(e_me_i^T Y^{t,(m)}O^{t,(m)})\right\|_2  \notag\\
  &\lesssim \frac{\sqrt{\mu r \sigma_{\max}\log n}}{n}.
\end{align}
Similarly, we have with probability at least $1-n^{-10}$ that
\begin{align}\label{ineq4:lem_ncv2}
  \left\|\frac1n\sum_{i\neq m}\left(\frac{e^{P_{im}^*}}{1+e^{P_{im}^*}}-A_{im}\right)e_ie_m^T X^{t,(m)}O^{t,(m)}\right\|_F\lesssim \frac{\sqrt{\mu r \sigma_{\max}\log n}}{n}.
\end{align}
Combine \eqref{ineq1:lem_ncv2}, \eqref{ineq2:lem_ncv2}, \eqref{ineq3:lem_ncv2} and \eqref{ineq4:lem_ncv2}, we conclude that $ \|(2)\|_F\lesssim \frac{\sqrt{\mu r \sigma_{\max}\log n}}{n}$.
% \begin{align*}
%     \|(2)\|_F\leq O(\sqrt{\log n}).
% \end{align*}
\item  We then bound (3). 
Notice that
\begin{align*}
\|F^{t,(m)}\|=\|F^{t,(m)}O^{t,(m)}\|\leq \|F^{t,(m)}O^{t,(m)}-F^tR^t\|+\|F^tR^t-F^*\|+\|F^*\|\leq 2\|F^*\|.
\end{align*}
Then following the same argument as bounding term (2) in Appendix \ref{pf:lem_ncv1}, we have
\begin{align*}
&\|\nabla_F f_{\diff}(M^t,F^tR^t)\|_F\lesssim\frac{c_{\aug}}{n^2}\|F^*\|\|X^{tT}X^t-Y^{tT}Y^t\|_F,\\
&\|\nabla_F f_{\diff}(M^{t,(m)},F^{t,(m)}O^{t,(m)})\|_F\lesssim\frac{c_{\aug}}{n^2}\|F^*\|\|X^{t,(m)T}X^{t,(m)}-Y^{t,(m)T}Y^{t,(m)}\|_F.
\end{align*}
Thus, it holds that
\begin{align*}
\|(3)\|_F&\lesssim \frac{c_{\aug}}{n^2}\|F^*\|\left(\|X^{tT}X^t-Y^{tT}Y^t\|_F+\|X^{t,(m)T}X^{t,(m)}-Y^{t,(m)T}Y^{t,(m)}\|_F\right)\\
&\lesssim \eta c_{51} c_{\aug}\sqrt{\sigma_{\max}}.
\end{align*}

% \item  Finally, we bound (4).
% \textcolor{red}{
% Here 
% \begin{align*}
% (4):= 
% \begin{bmatrix}
% \mean\left(\nabla_{\theta}f(M^t,F^tR^t)-\nabla_{\theta}f^{(m)}(M^{t,(m)},F^{t,(m)}O^{t,(m)})\right)\cdot\mathbf{1}\\
% 0
% \end{bmatrix}.
% \end{align*}
% At the beginning of the proof, we already removed this term by considering the projection. Thus, the bound on this term is no longer needed. But we still keep it here in case other parts need this proof.
% }

% Note that
% \begin{align*}
% \|(4)\|_F
% &=\sqrt{n}\left|\mean\left(\nabla_{\theta}f(M^t,F^tR^t)-\nabla_{\theta}f^{(m)}(M^{t,(m)},F^{t,(m)}O^{t,(m)})\right)\right|\\
% &=\sqrt{n}\left|\mean\left(\nabla_{\theta}L(M^t,F^tR^t)-\nabla_{\theta}L^{(m)}(M^{t,(m)},F^{t,(m)}O^{t,(m)})\right)\right|\\
% &\leq \sqrt{n}\left|\mean\left(\nabla_{\theta}L(M^t,F^tR^t)-\nabla_{\theta}L(M^{t,(m)},F^{t,(m)}O^{t,(m)})\right)\right|\\
% &\quad+\sqrt{n}\left|\mean\left(\nabla_{\theta}L(M^{t,(m)},F^{t,(m)}O^{t,(m)})-\nabla_{\theta}L^{(m)}(M^{t,(m)},F^{t,(m)}O^{t,(m)})\right)\right|\\
% \end{align*}
% For the first term, follow the same argument as bounding term (4) in Appendix \ref{pf:lem_ncv1}, we have
% \begin{align*}
% & \sqrt{n}\left|\mean\left(\nabla_{\theta}L(M^t,F^tR^t)-\nabla_{\theta}L(M^{t,(m)},F^{t,(m)}O^{t,(m)})\right)\right|\\
% &\lesssim \|\theta^t-\theta^{t,(m)}\|_2+\|H^t-H^{t,(m)}\|_F+\frac{1}{n}\|X^*\|\|F^tR^t-F^{t,(m)}O^{t,(m)}\|_F.
% \end{align*}
% For the second term, note that
% \begin{align*}
%  &\nabla_{\theta}L(M^{t,(m)},F^{t,(m)}O^{t,(m)})-\nabla_{\theta}L^{(m)}(M^{t,(m)},F^{t,(m)}O^{t,(m)})\\
%  &=\frac{2}{\sqrt{n}}\sum_{i\neq m}\left(\frac{e^{P_{im}^*}}{1+e^{P_{im}^*}}-A_{im}\right)(e_i+e_m).
% \end{align*}
% Using the argument as bounding term (2) in this proof, we have
% \begin{align*}
% &\sqrt{n}\left|\mean\left(\nabla_{\theta}L(M^{t,(m)},F^{t,(m)}O^{t,(m)})-\nabla_{\theta}L^{(m)}(M^{t,(m)},F^{t,(m)}O^{t,(m)})\right)\right|\\
% &\lesssim \frac{1}{\sqrt{n}}\left(\frac{n-1}{\sqrt{n}}+\sqrt{\log n}\right)=O(1).
% \end{align*}
% As a result, we conclude that 
% \begin{align*}
% \|(4)\|_F\lesssim \|\theta^t-\theta^{t,(m)}\|_2+\|H^t-H^{t,(m)}\|_F+\frac{1}{n}\|X^*\|\|F^tR^t-F^{t,(m)}O^{t,(m)}\|_F+O(1).
% \end{align*}
\end{enumerate}

Combine the bounds of Frobenius norm of (1)-(3), we conclude that
\begin{align*}
&\left\|\begin{bmatrix}
M^t-\eta\nabla_{M}f_{\aug}(M^t,F^t)
-
\left(
M^{t,(m)}-\eta\nabla_{M}f^{(m)}_{\aug}(M^{t,(m)},F^{t,(m)})
\right)\\
F^{t+1}R^t-F^{t+1,(m)}O^{t,(m)}
\end{bmatrix}\right\|_F\\
&\leq \left(1-\frac{\underline{C}}{2}\eta\right)
\left\|
\begin{bmatrix}
M^{t}-M^{t,(m)}\\
F^{t}R^t-F^{t,(m)}O^{t,(m)}
\end{bmatrix}
\right\|_F
+c\eta\frac{\sqrt{\mu r \sigma_{\max}\log n}}{n}+c\eta^2 c_{51} c_{\aug}\sqrt{\sigma_{\max}}\\
&\leq \left(1-\frac{\underline{C}}{2}\eta\right)
c_{21}
+c\eta\frac{\sqrt{\mu r \sigma_{\max}\log n}}{n}+c\eta^2 c_{51} c_{\aug}\sqrt{\sigma_{\max}}\\
&\leq c_{21}
\end{align*}
as long as $\frac{\sqrt{\mu r \sigma_{\max}\log n}}{\underline{C}n}\lesssim c_{21}$ and $\eta\ll \frac{\underline{C}c_{21}}{c_{51} c_{\aug}\sqrt{\sigma_{\max}}}$.
By \eqref{ineq30:pr_lem_ncv2} and Claim \ref{claim:lem_ncv2}, we further have
\begin{align*}
\left\|
\begin{bmatrix}
M^{t+1}-M^{t+1,(m)}\\
F^{t+1}R^{t+1}-F^{t+1,(m)}O^{t+1,(m)}
\end{bmatrix}
\right\|_F \leq c_{21}.
\end{align*}
Finally, by the arbitrariness of $m$, we finish the proofs.









\subsection{Proofs of Lemma \ref{lem:ncv3}}\label{pf:lem_ncv3}
Suppose Lemma \ref{lem:ncv1}-Lemma \ref{lem:ncv5} hold for the $t$-th iteration. In the following, we prove Lemma \ref{lem:ncv3} for the $(t+1)$-th iteration. 
Note that by the gradient descent update, we have
\begin{align*}
&\theta^{t+1,(m)}_m-\theta^*_m\\
&=\theta^{t,(m)}_m-\theta^*_m
-\frac{2\eta}{\sqrt{n}}\sum_{i\neq m}\left(\frac{e^{P^{t,(m)}_{im}}}{1+e^{P^{t,(m)}_{im}}}-\frac{e^{P^{*}_{im}}}{1+e^{P^{*}_{im}}}\right)+\eta\cdot\mean\left(\nabla_{\theta}L^{(m)}(M^{t,(m)}, F^{t,(m)})\right),
\end{align*}
where we use the symmetry of $X^{t,(m)}(Y^{t,(m)})^T$ obtained via Lemma \ref{lem:ncv5}.
By the mean value theorem, we have for some $\{c_i\}$ that
\begin{align*}
& \sum_{i\neq m}\left(\frac{e^{P^{t,(m)}_{im}}}{1+e^{P^{t,(m)}_{im}}}-\frac{e^{P^{*}_{im}}}{1+e^{P^{*}_{im}}}\right)\\
&= \sum_{i\neq m}\frac{e^{c_i}}{(1+e^{c_i})^2}\left(P^{t,(m)}_{im}-P^{*}_{im}\right)\\
& = \sum_{i\neq m}\frac{e^{c_i}}{(1+e^{c_i})^2}\left(\frac{1}{\sqrt{n}}\left(\theta^{t,(m)}_i-\theta^{*}_i+\theta^{t,(m)}_m-\theta^{*}_m\right)+\langle H^{t,(m)}-H^*,z_iz_m^T\rangle+\frac1n \left(X^{t,(m)}(Y^{t,(m)})^T-X^{*}Y^{*T}\right)_{im}\right)\\
& = \left(\frac{1}{\sqrt{n}}\sum_{i\neq m}\frac{e^{c_i}}{(1+e^{c_i})^2}\right)\left(\theta^{t,(m)}_m-\theta^{*}_m\right)\\
&\quad+\sum_{i\neq m}\frac{e^{c_i}}{(1+e^{c_i})^2}\left(\frac{1}{\sqrt{n}}\left(\theta^{t,(m)}_i-\theta^{*}_i\right)+\langle H^{t,(m)}-H^*,z_iz_m^T\rangle+\frac1n \left(X^{t,(m)}(Y^{t,(m)})^T-X^{*}Y^{*T}\right)_{im}\right).
\end{align*}
Thus, it holds that
\begin{align}\label{eq1:lem_ncv3}
 &\theta^{t+1,(m)}_m-\theta^*_m\notag\\
 &=\left(1-\frac{2\eta}{n}\sum_{i\neq m}\frac{e^{c_i}}{(1+e^{c_i})^2}\right)\left(\theta^{t,(m)}_m-\theta^*_m\right)
+\eta\cdot\mean\left(\nabla_{\theta}L^{(m)}(M^{t,(m)}, F^{t,(m)})\right)\notag\\
&\quad -\frac{2\eta}{\sqrt{n}}\sum_{i\neq m}\frac{e^{c_i}}{(1+e^{c_i})^2}\left(\frac{1}{\sqrt{n}}\left(\theta^{t,(m)}_i-\theta^{*}_i\right)+\langle H^{t,(m)}-H^*,z_iz_m^T\rangle+\frac1n \left(X^{t,(m)}(Y^{t,(m)})^T-X^{*}Y^{*T}\right)_{im}\right)\notag\\
&=\left(1-\frac{2\eta}{n}\sum_{i\neq m}\frac{e^{c_i}}{(1+e^{c_i})^2}\right)\left(\theta^{t,(m)}_m-\theta^*_m\right)
+\eta\cdot\mean\left(\nabla_{\theta}L^{(m)}(M^{t,(m)}, F^{t,(m)})\right)\notag\\
&\quad -\frac{2\eta}{\sqrt{n}}\sum_{i\neq m}\frac{e^{c_i}}{(1+e^{c_i})^2}\left(\frac{1}{\sqrt{n}}\left(\theta^{t,(m)}_i-\theta^{*}_i\right)+\langle H^{t,(m)}-H^*,z_iz_m^T\rangle\right)\notag\\
&\quad -\frac{\eta}{n^{3/2}}\sum_{i\neq m}\frac{e^{c_i}}{(1+e^{c_i})^2}\left(X^{t,(m)}(Y^{t,(m)})^T-X^{*}Y^{*T}\right)_{im}\notag\\
&\quad -\frac{\eta}{n^{3/2}}\sum_{i\neq m}\frac{e^{c_i}}{(1+e^{c_i})^2}\left(X^{t,(m)}(Y^{t,(m)})^T-X^{*}Y^{*T}\right)_{mi},
\end{align}
where the last equation follows from the symmetry property.
Notice that
\begin{align*}
& X^{t,(m)}(Y^{t,(m)})^T-X^{*}Y^{*T}\notag\\
&=\left(X^{t,(m)}R^{t,(m)}-X^{*}\right)\left(Y^{t,(m)}R^{t,(m)}\right)^T+X^*\left(Y^{t,(m)}R^{t,(m)}-Y^{*}\right)^T\notag\\
&=\left(X^{t,(m)}R^{t,(m)}\right)\left(Y^{t,(m)}R^{t,(m)}-Y^{*}\right)^T+\left(X^{t,(m)}R^{t,(m)}-X^{*}\right)\left(Y^{*}\right)^T.
\end{align*}
Thus, we have
\begin{align*}
&\left(X^{t,(m)}(Y^{t,(m)})^T-X^{*}Y^{*T}\right)_{im}\\
&=\left(X^{t,(m)}R^{t,(m)}-X^{*}\right)_{i,\cdot}^{\top}\left(Y^{t,(m)}R^{t,(m)}\right)_{m,\cdot}+(X^*_{i,\cdot})^{\top}\left(Y^{t,(m)}R^{t,(m)}-Y^{*}\right)_{m,\cdot},
\end{align*}
and
\begin{align*}
&\left(X^{t,(m)}(Y^{t,(m)})^T-X^{*}Y^{*T}\right)_{mi}\\
&=\left(Y^{t,(m)}R^{t,(m)}-Y^{*}\right)_{i,\cdot}^{\top}\left(X^{t,(m)}R^{t,(m)}\right)_{m,\cdot}+\left(Y^{*}_{i,\cdot}\right)^T\left(X^{t,(m)}R^{t,(m)}-X^{*}\right)_{m,\cdot}.
\end{align*}
By \eqref{eq1:lem_ncv3}, we obtain
\begin{align}\label{eq11:lem_ncv3}
 &\theta^{t+1,(m)}_m-\theta^*_m\notag\\
&=\left(1-\frac{2\eta}{n}\sum_{i\neq m}\frac{e^{c_i}}{(1+e^{c_i})^2}\right)\left(\theta^{t,(m)}_m-\theta^*_m\right)\notag\\
&
-\frac{\eta}{n^{3/2}}\sum_{i\neq m}\frac{e^{c_i}}{(1+e^{c_i})^2}\left(Y^{*}_{i,\cdot}\right)^T\left(X^{t,(m)}R^{t,(m)}-X^{*}\right)_{m,\cdot}
-\frac{\eta}{n^{3/2}}\sum_{i\neq m}\frac{e^{c_i}}{(1+e^{c_i})^2}(X^*_{i,\cdot})^{\top}\left(Y^{t,(m)}R^{t,(m)}-Y^{*}\right)_{m,\cdot}\notag\\
&\quad+\eta\cdot\mean\left(\nabla_{\theta}L^{(m)}(M^{t,(m)}, F^{t,(m)})\right)-\frac{2\eta}{\sqrt{n}}\sum_{i\neq m}\frac{e^{c_i}}{(1+e^{c_i})^2}\left(\frac{1}{\sqrt{n}}\left(\theta^{t,(m)}_i-\theta^{*}_i\right)+\langle H^{t,(m)}-H^*,z_iz_m^T\rangle\right)\notag\\
&\quad -\frac{\eta}{n^{3/2}}\sum_{i\neq m}\frac{e^{c_i}}{(1+e^{c_i})^2}\left(X^{t,(m)}R^{t,(m)}-X^{*}\right)_{i,\cdot}^{\top}\left(Y^{t,(m)}R^{t,(m)}\right)_{m,\cdot}
\notag\\
&\quad -\frac{\eta}{n^{3/2}}\sum_{i\neq m}\frac{e^{c_i}}{(1+e^{c_i})^2}\left(Y^{t,(m)}R^{t,(m)}-Y^{*}\right)_{i,\cdot}^{\top}\left(X^{t,(m)}R^{t,(m)}\right)_{m,\cdot}\notag\\
&=\left(1-\frac{2\eta}{n}\sum_{i\neq m}\frac{e^{c_i}}{(1+e^{c_i})^2}\right)\left(\theta^{t,(m)}_m-\theta^*_m\right)
-\frac{\eta}{n^{3/2}}\sum_{i\neq m}\frac{e^{c_i}}{(1+e^{c_i})^2}\left(Y^{*}_{i,\cdot}\right)^T\left(X^{t,(m)}R^{t,(m)}-X^{*}\right)_{m,\cdot}\notag\\
&\quad-\frac{\eta}{n^{3/2}}\sum_{i\neq m}\frac{e^{c_i}}{(1+e^{c_i})^2}(X^*_{i,\cdot})^{\top}\left(Y^{t,(m)}R^{t,(m)}-Y^{*}\right)_{m,\cdot}+r_1,
\end{align}
where 
\begin{align*}
r_1&:=\eta\cdot\mean\left(\nabla_{\theta}L^{(m)}(M^{t,(m)}, F^{t,(m)})\right)-\frac{2\eta}{\sqrt{n}}\sum_{i\neq m}\frac{e^{c_i}}{(1+e^{c_i})^2}\left(\frac{1}{\sqrt{n}}\left(\theta^{t,(m)}_i-\theta^{*}_i\right)+\langle H^{t,(m)}-H^*,z_iz_m^T\rangle\right)\notag\\
&\quad -\frac{\eta}{n^{3/2}}\sum_{i\neq m}\frac{e^{c_i}}{(1+e^{c_i})^2}\left(X^{t,(m)}R^{t,(m)}-X^{*}\right)_{i,\cdot}^{\top}\left(Y^{t,(m)}R^{t,(m)}\right)_{m,\cdot}
\notag\\
&\quad -\frac{\eta}{n^{3/2}}\sum_{i\neq m}\frac{e^{c_i}}{(1+e^{c_i})^2}\left(Y^{t,(m)}R^{t,(m)}-Y^{*}\right)_{i,\cdot}^{\top}\left(X^{t,(m)}R^{t,(m)}\right)_{m,\cdot}
\end{align*}
In the following, we bound $|r_1|$.
\begin{enumerate}
\item  For the first term, note that
\begin{align*}
&\left|\mean\left(\nabla_{\theta}L^{(m)}(M^{t,(m)}, F^{t,(m)})\right)\right|\\
&=\left|\mean\left(\nabla_{\theta}L^{(m)}(M^{t,(m)}, F^{t,(m)}O^{t,(m)})\right)\right|\\
&\leq \left|\mean\left(\nabla_{\theta}L^{(m)}(M^{t,(m)}, F^{t,(m)}O^{t,(m)})-\nabla_{\theta}L(M^{t}, F^{t}R^{t})\right)\right|+ \left|\mean\left(\nabla_{\theta}L(M^{t}, F^{t}R^{t})\right)\right|.
\end{align*}
For the first part, we have the following claim.
\begin{claim}\label{claim1:gradient_mean}
It holds that
\begin{align*}
 & \left|\mean\left(\nabla_{\theta}L^{(m)}(M^{t,(m)}, F^{t,(m)}O^{t,(m)})-\nabla_{\theta}L(M^{t}, F^{t}R^{t})\right)\right|\\
 & \lesssim   \sqrt{\frac{\su}{n}}\left(\|\theta^t-\theta^{t,(m)}\|_2+\|H^t-H^{t,(m)}\|_F+\frac{1}{n}\|X^*\|\|F^tR^t-F^{t,(m)}O^{t,(m)}\|_F\right)+\sqrt{\frac{\log n}{n}}.
\end{align*}
\end{claim}
\begin{proof}[Proof of Claim \ref{claim1:gradient_mean}]
 Note that
\begin{align*}
&\left|\mean\left(\nabla_{\theta}L(M^t,F^tR^t)-\nabla_{\theta}L^{(m)}(M^{t,(m)},F^{t,(m)}O^{t,(m)})\right)\right|\\
&\leq\left|\mean\left(\nabla_{\theta}L(M^t,F^tR^t)-\nabla_{\theta}L(M^{t,(m)},F^{t,(m)}O^{t,(m)})\right)\right|\\
&\quad+\left|\mean\left(\nabla_{\theta}L(M^{t,(m)},F^{t,(m)}O^{t,(m)})-\nabla_{\theta}L^{(m)}(M^{t,(m)},F^{t,(m)}O^{t,(m)})\right)\right|\\
\end{align*}
For the first term, we have
\begin{align*}
&\mean\left(\nabla_{\theta}L(M^t,F^tR^t)-\nabla_{\theta}L(M^{t,(m)},F^{t,(m)}O^{t,(m)})\right)\\
&=\frac{2}{n^{3/2}}\sum_{i\neq j}\left(\frac{e^{P_{ij}^{t}}}{1+e^{P_{ij}^{t}}}-\frac{e^{P_{ij}^{t,(m)}}}{1+e^{P_{ij}^{t,(m)}}}\right)\\
&\leq \frac{1}{2n^{3/2}}\sum_{i\neq j}\left|P^t_{ij}-P^{t,(m)}_{ij}\right| \tag{by mean-value theorem}\\
&\leq \frac{1}{2\sqrt{n}}\sqrt{\sum_{i\neq j}\left|P^t_{ij}-P^{t,(m)}_{ij}\right|^2}. \tag{by Cauchy-Schwarz}
\end{align*}

Note that
\begin{align*}
&\sum_{i\neq j}(P_{ij}^{t}-P_{ij}^{t,(m)})^2\\
&=\sum_{i\neq j}\left(\frac{1}{\sqrt{n}}\langle\theta^{t}-\theta^{t,(m)},e_i+e_j\rangle+\langle H^{t}-H^{t,(m)},z_iz_j^T\rangle+\frac1n\langle X^{t}Y^{tT}-X^{t,(m)}Y^{t,(m) T},e_i e_j^T\rangle\right)^2\\
&=
\begin{bmatrix}
  \vec(\theta^{t}-\theta^{t,(m)})\\
  \vec(H^{t}-H^{t,(m)})\\
  \frac1n\vec(X^{t}Y^{tT}-X^{t,(m)}Y^{t,(m) T})
\end{bmatrix}^T
\left(\sum_{i\neq j}
  \begin{bmatrix}
  \frac{1}{\sqrt{n}}\vec(e_i+e_j)\\
  \vec(z_iz_j^T)\\
  \vec(e_ie_j^T)
  \end{bmatrix}
   \begin{bmatrix}
  \frac{1}{\sqrt{n}}\vec(e_i+e_j)\\
  \vec(z_iz_j^T)\\
  \vec(e_ie_j^T)
  \end{bmatrix}^T
\right)
\begin{bmatrix}
  \vec(\theta^{t}-\theta^{t,(m)})\\
  \vec(H^{t}-H^{t,(m)})\\
  \frac1n\vec(X^{t}Y^{tT}-X^{t,(m)}Y^{t,(m) T})
\end{bmatrix}\\
&\leq \su \left\|\begin{bmatrix}
  \vec(\theta^{t}-\theta^{t,(m)})\\
  \vec(H^{t}-H^{t,(m)})\\
  \frac1n\vec(X^{t}Y^{tT}-X^{t,(m)}Y^{t,(m) T})
\end{bmatrix}\right\|^2 \tag{by Assumption \ref{assumption:eigenvalues} and $\mathbf{1}^T(\theta^t-\theta^{t,(m)})=0$}\\
& =\su\left(\|\theta^t-\theta^{t,(m)}\|^2_{2}+\|H^t-H^{t,(m)}\|^2_{F}+\frac{1}{n^2}\|X^tY^{tT}-X^{t,(m)}Y^{t,(m) T}\|^2_{F}\right).
\end{align*}
As a result, we have
\begin{align*}
&\left|\mean\left(\nabla_{\theta}L(M^t,F^tR^t)-\nabla_{\theta}L(M^{t,(m)},F^{t,(m)}O^{t,(m)})\right)\right|\\
&\lesssim \sqrt{\frac{\su}{n}}\left(\|\theta^t-\theta^{t,(m)}\|_{2}+\|H^t-H^{t,(m)}\|_{F}+\frac{1}{n}\|X^tY^{tT}-X^{t,(m)}Y^{t,(m) T}\|_{F}\right)\\
&\lesssim \sqrt{\frac{\su}{n}}\left(\|\theta^t-\theta^{t,(m)}\|_2+\|H^t-H^{t,(m)}\|_F+\frac{1}{n}\|X^*\|\|F^tR^t-F^{t,(m)}O^{t,(m)}\|_F\right).
\end{align*}

For the second term, note that
\begin{align*}
 &\nabla_{\theta}L(M^{t,(m)},F^{t,(m)}O^{t,(m)})-\nabla_{\theta}L^{(m)}(M^{t,(m)},F^{t,(m)}O^{t,(m)})\\
 &=\frac{2}{\sqrt{n}}\sum_{i\neq m}\left(\frac{e^{P_{im}^*}}{1+e^{P_{im}^*}}-A_{im}\right)(e_i+e_m).
\end{align*}
Thus, we have
\begin{align*}
&\left|\mean\left(\nabla_{\theta}L(M^{t,(m)},F^{t,(m)}O^{t,(m)})-\nabla_{\theta}L^{(m)}(M^{t,(m)},F^{t,(m)}O^{t,(m)})\right)\right|\\
&\leq \frac1n \left\|\frac{2}{\sqrt{n}}\sum_{i\neq m}\left(\frac{e^{P_{im}^*}}{1+e^{P_{im}^*}}-A_{im}\right)(e_i+e_m)\right\|_1\\
&\leq \frac{1}{\sqrt{n}}\left\|\frac{2}{\sqrt{n}}\sum_{i\neq m}\left(\frac{e^{P_{im}^*}}{1+e^{P_{im}^*}}-A_{im}\right)(e_i+e_m)\right\|_2\\
&\lesssim \sqrt{\frac{\log n}{n}} \tag{by \eqref{ineq1:lem_ncv2}}.
\end{align*}
Combining the above two terms, we then finish the proof.  
\end{proof}

For the second part, we have the following claim.
\begin{claim}\label{claim2:gradient_mean}
It holds that
\begin{align*}
 & \left|\mean\left(\nabla_{\theta}L(M^{t}, F^{t}R^{t})\right)\right|\\
 & \lesssim  \sqrt{\frac{\su}{n}}\left(\|\theta^t-\theta^{*}\|_{2}+\|H^t-H^{*}\|_{F}+\frac{1}{n}\|X^*\|\|F^tR^t-F^{*}\|_{F}\right)+\sqrt{\frac{\log n}{n}}.
\end{align*}
\end{claim}
\begin{proof}[Proof of Claim \ref{claim2:gradient_mean}]
Note that
\begin{align*}
\nabla_{\theta}L(M^t,F^tR^t)=\nabla_{\theta}L(M^*,F^*)+\nabla_{\theta}L(M^t,F^tR^t)-\nabla_{\theta}L(M^*,F^*).
\end{align*}
For the first term, by Lemma \ref{lem:gradient_norm}, we have
\begin{align*}
\left| \mean\left(\nabla_{\theta}L(M^*,F^*)\right)\right|\leq \frac{1}{\sqrt{n}}\left\|\nabla_{\theta}L(M^*,F^*)\right\|_2\lesssim \sqrt{\frac{\log n}{n}}.
\end{align*}
For the rest of the terms, same as the proof of Claim \ref{claim1:gradient_mean}, we have
\begin{align*}
\left|\mean\left(\nabla_{\theta}L(M^t,F^tR^t)-\nabla_{\theta}L(M^*,F^*)\right)\right|
\lesssim \sqrt{\frac{\su}{n}}\left(\|\theta^t-\theta^{*}\|_{2}+\|H^t-H^{*}\|_{F}+\frac{1}{n}\|X^*\|\|F^tR^t-F^{*}\|_{F}\right).
\end{align*}
Combining the above two terms, we then finish the proof.


% For the rest of the terms, we have 
% \begin{align*}
% &n\cdot \mean\left(\nabla_{\theta}L(M^t,F^tR^t)-\nabla_{\theta}L(M^*,F^*)\right)\\
% &=\frac{2}{\sqrt{n}}\sum_{i\neq j}\left(\frac{e^{P_{ij}^{t}}}{1+e^{P_{ij}^{t}}}-\frac{e^{P_{ij}^{*}}}{1+e^{P_{ij}^{*}}}\right)\\
% &\leq \frac{1}{2\sqrt{n}}\sum_{i\neq j}\left|P^t_{ij}-P^{*}_{ij}\right| \tag{by mean-value theorem}\\
% &\leq \frac{\sqrt{n}}{2}\sqrt{\sum_{i\neq j}\left|P^t_{ij}-P^{*}_{ij}\right|^2}. \tag{by Cauchy-Schwarz}
% \end{align*}
% Note that
% \begin{align*}
% &\sum_{i\neq j}(P_{ij}^{t}-P_{ij}^*)^2\\
% &=\sum_{i\neq j}\left(\frac{1}{\sqrt{n}}\langle\theta^{t}-\theta^*,e_i+e_j\rangle+\langle H^{t}-H^*,z_iz_j^T\rangle+\frac1n\langle X^{t}Y^{tT}-X^*Y^{*T},e_i e_j^T\rangle\right)^2\\
% &=
% \begin{bmatrix}
%   \vec(\theta^{t}-\theta^*)\\
%   \vec(H^{t}-H^*)\\
%   \frac1n\vec(X^{t}Y^{tT}-X^*Y^{*T})
% \end{bmatrix}^T
% \left(\sum_{i\neq j}
%   \begin{bmatrix}
%   \frac{1}{\sqrt{n}}\vec(e_i+e_j)\\
%   \vec(z_iz_j^T)\\
%   \vec(e_ie_j^T)
%   \end{bmatrix}
%    \begin{bmatrix}
%   \frac{1}{\sqrt{n}}\vec(e_i+e_j)\\
%   \vec(z_iz_j^T)\\
%   \vec(e_ie_j^T)
%   \end{bmatrix}^T
% \right)
% \begin{bmatrix}
%   \vec(\theta^{t}-\theta^*)\\
%   \vec(H^{t}-H^*)\\
%   \frac1n\vec(X^{t}Y^{tT}-X^*Y^{*T})
% \end{bmatrix}\\
% &\lesssim \left\|\begin{bmatrix}
%   \vec(\theta^{t}-\theta^*)\\
%   \vec(H^{t}-H^*)\\
%   \frac1n\vec(X^{t}Y^{tT}-X^*Y^{*T})
% \end{bmatrix}\right\|^2 \tag{by balanced eigenvalues assumption and $\mathbf{1}^T(\theta^t-\theta^*)=0$}\\
% & =\|\theta^t-\theta^{*}\|^2_{2}+\|H^t-H^{*}\|^2_{F}+\frac{1}{n^2}\|X^tY^{tT}-X^{*}Y^{*T}\|^2_{F}.
% \end{align*}
% As a result, we have
% \begin{align*}
% \left|\mean\left(\nabla_{\theta}L(M^t,F^tR^t)-\nabla_{\theta}L(M^*,F^*)\right)\right|
% \lesssim \frac{1}{\sqrt{{n}}}\left(\|\theta^t-\theta^{*}\|_{2}+\|H^t-H^{*}\|_{F}+\frac{1}{n}\|X^tY^{tT}-X^{*}Y^{*T}\|_{F}\right).
% \end{align*}
% Combine the above results, we show that
% \begin{align*}
%  \left|\mean\left(\nabla_{\theta}f(M^t,F^tR^t)\right)\right| 
%  \lesssim O\left(\sqrt{\frac{\log n}{n}}\right)+\frac{1}{\sqrt{{n}}}\left(\|\theta^t-\theta^{*}\|_{2}+\|H^t-H^{*}\|_{F}+\frac{1}{n}\|X^tY^{tT}-X^{*}Y^{*T}\|_{F}\right),
% \end{align*}
% which implies
% \begin{align*}
%  (4)
%  \lesssim O\left(\sqrt{\log n}\right)+\|\theta^t-\theta^{*}\|_{2}+\|H^t-H^{*}\|_{F}+\frac{1}{n}\|X^tY^{tT}-X^{*}Y^{*T}\|_{F}.
% \end{align*}
\end{proof}

By Claim \ref{claim1:gradient_mean} and \ref{claim2:gradient_mean}, we have
\begin{align}\label{ineq1:lem_ncv3}
&\left|\mean\left(\nabla_{\theta}L^{(m)}(M^{t,(m)}, F^{t,(m)})\right)\right|\notag\\
&\lesssim \sqrt{\frac{\su}{n}}\left(\|\theta^t-\theta^{t,(m)}\|_2+\|H^t-H^{t,(m)}\|_F+\frac{1}{n}\|X^*\|\|F^tR^t-F^{t,(m)}O^{t,(m)}\|_F\right)\notag\\
&\quad + \sqrt{\frac{\su}{n}}\left(\|\theta^t-\theta^{*}\|_{2}+\|H^t-H^{*}\|_{F}+\frac{1}{n}\|X^*\|\|F^tR^t-F^*\|_F\right)+O\left(\sqrt{\frac{\log n}{n}}\right).
\end{align}


\item For the second term, we have
\begin{align}\label{ineq12:lem_ncv3}
&\left|\sum_{i\neq m}\frac{e^{c_i}}{(1+e^{c_i})^2}\left(\frac{1}{\sqrt{n}}\left(\theta^{t,(m)}_i-\theta^{*}_i\right)+\langle H^{t,(m)}-H^*,z_iz_m\rangle\right)\right|\notag\\
&\leq \frac14\sum_{i\neq m}\frac{1}{\sqrt{n}}\left|\theta^{t,(m)}_i-\theta^{*}_i\right|+\left|\langle H^{t,(m)}-H^*,z_iz_m^T\rangle\right|\notag\\
&\leq \|\theta^{t,(m)}-\theta^{*}\|_2+\| H^{t,(m)}-H^*\|\sum_{i\neq m}\|z_i\|\|z_m\|\notag\\
&\leq \|\theta^{t,(m)}-\theta^{*}\|_2+\sz\| H^{t,(m)}-H^*\|.
\end{align}

\item For the third and fourth terms, note that
\begin{align*}
&\left|\frac{1}{n^{3/2}}\sum_{i\neq m}\frac{e^{c_i}}{(1+e^{c_i})^2}\left(X^{t,(m)}R^{t,(m)}-X^{*}\right)_{i,\cdot}^{\top}\left(Y^{t,(m)}R^{t,(m)}\right)_{m,\cdot}\right|\notag\\
&\leq \frac{1}{n^{3/2}}\sum_{i\neq m}\left|\left(X^{t,(m)}R^{t,(m)}-X^{*}\right)_{i,\cdot}^{\top}\left(Y^{t,(m)}R^{t,(m)}\right)_{m,\cdot}\right|\notag\\
&=\frac{1}{n^{3/2}}\left\|\left(X^{t,(m)}R^{t,(m)}-X^{*}\right)\left(Y^{t,(m)}R^{t,(m)}\right)_{m,\cdot}\right\|_1\notag\\
&\leq \frac{1}{n}\left\|\left(X^{t,(m)}R^{t,(m)}-X^{*}\right)\left(Y^{t,(m)}R^{t,(m)}\right)_{m,\cdot}\right\|_2\notag\\
&\leq \frac{1}{n}\left\|X^{t,(m)}R^{t,(m)}-X^{*}\right\|\left\|Y^{t,(m)}R^{t,(m)}\right\|_{2,\infty}.
\end{align*}
Since Lemma \ref{lem:ncv3} holds for the $t$-th iteration, we have
\begin{align*}
  \left\|Y^{t,(m)}R^{t,(m)}\right\|_{2,\infty}\leq \left\|Y^{t,(m)}R^{t,(m)}-Y^*\right\|_{2,\infty}  + \|Y^*\|_{2,\infty}\leq 2\|Y^*\|_{2,\infty},
\end{align*}
as long as $\|Y^{t,(m)}R^{t,(m)}-Y^*\|_{2,\infty}\ll \|Y^*\|_{2,\infty}$. 
By Lemma \ref{ar:lem2}, we have
\begin{align*}
\left\|F^{t,(m)}R^{t,(m)}-F^{t}R^t\right\|_F\leq 5\kappa    \left\|F^{t,(m)}O^{t,(m)}-F^{t}R^t\right\|_F,
\end{align*}
which implies
\begin{align*}
   \left\|X^{t,(m)}R^{t,(m)}-X^{*}\right\|&\leq \left\|F^{t,(m)}R^{t,(m)}-F^{*}\right\|\\
  &\leq  \left\|F^{t,(m)}R^{t,(m)}-F^{t}R^t\right\|_F+ \left\|F^{t}R^t-F^{*}\right\|\\
   &\leq  5\kappa\left\|F^{t,(m)}O^{t,(m)}-F^{t}R^t\right\|_F+ \left\|F^{t}R^t-F^{*}\right\|\\
  &\leq 2\left\|F^{t}R^t-F^{*}\right\|
\end{align*}
as long as $\kappa\left\|F^{t,(m)}O^{t,(m)}-F^{t}R^t\right\|_F\ll \|F^{t}R^t-F^{*}\|$.
% Here the last inequality holds since $\left\|F^{t,(m)}O^{t,(m)}-F^{t}R^t\right\|_F=O(1)$ by Lemma \ref{lem:ncv2} and $\|F^{t}R^t-F^{*}\|=O(\sqrt{n})$ by Lemma \ref{lem:ncv1}.


Consequently, we have
\begin{align}\label{ineq2:lem_ncv3}
 &\left|\frac{1}{n^{3/2}}\sum_{i\neq m}\frac{e^{c_i}}{(1+e^{c_i})^2}\left(X^{t,(m)}R^{t,(m)}-X^{*}\right)_{i,\cdot}^{\top}\left(Y^{t,(m)}R^{t,(m)}\right)_{m,\cdot}\right|\leq\frac{4}{n}\left\|F^{t}R^t-F^{*}\right\|\|Y^*\|_{2,\infty}. 
\end{align}
Similarly, we have
\begin{align}\label{ineq13:lem_ncv3}
\left| \frac{1}{n^{3/2}}\sum_{i\neq m}\frac{e^{c_i}}{(1+e^{c_i})^2}\left(Y^{t,(m)}R^{t,(m)}-Y^{*}\right)_{i,\cdot}^{\top}\left(X^{t,(m)}R^{t,(m)}\right)_{m,\cdot}\right|\leq\frac{4}{n}\left\|F^{t}R^t-F^{*}\right\|\|X^*\|_{2,\infty}. 
\end{align}

\end{enumerate}

Combine \eqref{ineq1:lem_ncv3}, \eqref{ineq12:lem_ncv3}, \eqref{ineq2:lem_ncv3} and \eqref{ineq13:lem_ncv3}, we have
\begin{align*}
&\left|r_1\right|\notag\\
&\lesssim \frac{\eta\sqrt{\su}}{\sqrt{n}}\left(\|\theta^t-\theta^{t,(m)}\|_2+\|H^t-H^{t,(m)}\|_F+\frac{1}{n}\|X^*\|\|F^tR^t-F^{t,(m)}O^{t,(m)}\|_F\right)\notag\\
&\quad + \frac{\eta\sqrt{\su}}{\sqrt{n}}\left(\|\theta^t-\theta^{*}\|_{2}+\|H^t-H^{*}\|_{F}+\frac{1}{n}\|X^*\|\|F^tR^t-F^*\|_F\right)+\eta\sqrt{\frac{\log n}{n}}\\
&\quad+\frac{\eta}{\sqrt{n}}\left(\|\theta^{t,(m)}-\theta^{*}\|_2+\sz\| H^{t,(m)}-H^*\|\right)+\frac{\eta}{n}\left\|F^{t}R^t-F^{*}\right\|\|F^*\|_{2,\infty}\notag\\
&\lesssim\frac{\eta\sqrt{\overline{C}}}{\sqrt{n}}c_{21}+ {\eta(\sqrt{\overline{C}}}+\sz)c_{11}+\eta\sqrt{\frac{\log n}{n}}+\eta\sqrt{\mu \sX\sY r^2 }c_{14}.
\end{align*}


Note that
\begin{align*}
\nabla_X L^{(m)}(\theta,H,X,Y)
&=\frac1n\sum_{\substack{
        i \neq j \\
        i, j \neq m
    }}\left(\frac{e^{P_{ij}}}{1+e^{P_{ij}}}-A_{ij}\right)e_ie_j^TY\\
&\quad+\frac1n\sum_{i\neq m}\left(\frac{e^{P_{im}}}{1+e^{P_{im}}}-\frac{e^{P_{im}^*}}{1+e^{P_{im}^*}}\right)e_ie_m^TY+\frac1n\sum_{i\neq m}\left(\frac{e^{P_{mi}}}{1+e^{P_{mi}}}-\frac{e^{P_{mi}^*}}{1+e^{P_{mi}^*}}\right)e_me_i^TY,
\end{align*}
where the $m$-th row of the first and second terms are all zeros. Thus, by the gradient descent update, we have
\begin{align*}
&\left(F^{t+1,(m)}R^{t+1,(m)}-F^{*}\right)_{m,\cdot}\\
&=\left(X^{t,(m)}_{m,\cdot}-\eta\left\{\frac1n\sum_{i\neq m}\left(\frac{e^{P_{mi}^{t,(m)}}}{1+e^{P_{mi}^{t,(m)}}}-\frac{e^{P_{mi}^*}}{1+e^{P_{mi}^*}}\right)e_i^TY^{t,(m)}+\lambda X^{t,(m)}_{m,\cdot}\right\}\right)R^{t+1,(m)}-X^*_{m,\cdot}\\
&=\left\{X^{t,(m)}_{m,\cdot}R^{t,(m)}-X^*_{m,\cdot}-\eta\left(\frac1n\sum_{i\neq m}\left(\frac{e^{P_{mi}^{t,(m)}}}{1+e^{P_{mi}^{t,(m)}}}-\frac{e^{P_{mi}^*}}{1+e^{P_{mi}^*}}\right)e_i^TY^{t,(m)}+\lambda X^{t,(m)}_{m,\cdot}\right)R^{t,(m)}\right\}\\
&+\left\{X^{t,(m)}_{m,\cdot}R^{t,(m)}-\eta\left(\frac1n\sum_{i\neq m}\left(\frac{e^{P_{mi}^{t,(m)}}}{1+e^{P_{mi}^{t,(m)}}}-\frac{e^{P_{mi}^*}}{1+e^{P_{mi}^*}}\right)e_i^TY^{t,(m)}+\lambda X^{t,(m)}_{m,\cdot}\right)R^{t,(m)}\right\}\left(\left(R^{t,(m)}\right)^{-1}R^{t+1,(m)}-I_r\right)
\end{align*}
By the mean value theorem, we have for some $\{c_i\}$ that
\begin{align*}
& \sum_{i\neq m}\left(\frac{e^{P^{t,(m)}_{mi}}}{1+e^{P^{t,(m)}_{mi}}}-\frac{e^{P^{*}_{mi}}}{1+e^{P^{*}_{mi}}}\right)e_i^TY^{t,(m)}\\
&= \sum_{i\neq m}\frac{e^{c_i}}{(1+e^{c_i})^2}\left(P^{t,(m)}_{mi}-P^{*}_{mi}\right)e_i^TY^{t,(m)}\\
& = \sum_{i\neq m}\frac{e^{c_i}}{(1+e^{c_i})^2}\left(\frac{1}{\sqrt{n}}\left(\theta^{t,(m)}_i-\theta^{*}_i+\theta^{t,(m)}_m-\theta^{*}_m\right)+\langle H^{t,(m)}-H^*,z_mz_i^T\rangle\right)e_i^TY^{t,(m)}\\
& \quad +\frac1n\sum_{i\neq m}\frac{e^{c_i}}{(1+e^{c_i})^2}\left(X^{t,(m)}(Y^{t,(m)})^T-X^{*}Y^{*T}\right)_{mi}e_i^TY^{t,(m)}.
\end{align*}
Note that
\begin{align*}
&X^{t,(m)}(Y^{t,(m)})^T-X^{*}Y^{*T}\\
&=\left(X^{t,(m)}R^{t,(m)}-X^*\right)\left(Y^{*}\right)^T+(X^{t,(m)}R^{t,(m)})\left(Y^{t,(m)}R^{t,(m)}-Y^*\right)^T.
\end{align*}
Thus, we further have
\begin{align*}
& \sum_{i\neq m}\left(\frac{e^{P^{t,(m)}_{mi}}}{1+e^{P^{t,(m)}_{mi}}}-\frac{e^{P^{*}_{mi}}}{1+e^{P^{*}_{mi}}}\right)e_i^TY^{t,(m)}\\
&= \sum_{i\neq m}\frac{e^{c_i}}{(1+e^{c_i})^2}\left(\frac{1}{\sqrt{n}}\left(\theta^{t,(m)}_i-\theta^{*}_i+\theta^{t,(m)}_m-\theta^{*}_m\right)+\langle H^{t,(m)}-H^*,z_mz_i^T\rangle\right)e_i^TY^{t,(m)}\\
& \quad +\left(X^{t,(m)}R^{t,(m)}-X^*\right)_{m,\cdot}^{\top}\left(\frac1n\sum_{i\neq m}\frac{e^{c_i}}{(1+e^{c_i})^2}(Y^*_{i,\cdot})e_i^TY^{t,(m)}\right)\\
& \quad +\frac1n\sum_{i\neq m}\frac{e^{c_i}}{(1+e^{c_i})^2}\left((X^{t,(m)}R^{t,(m)})\left(Y^{t,(m)}R^{t,(m)}-Y^*\right)^T\right)_{mi}e_i^TY^{t,(m)}.
\end{align*}
Consequently, we have
\begin{align}\label{eq21:lem_ncv3}
&\left(F^{t+1,(m)}R^{t+1,(m)}-F^{*}\right)_{m,\cdot}\notag\\
&=\left(I_r-\frac{\eta}{n^2}\sum_{i\neq m}\frac{e^{c_i}}{(1+e^{c_i})^2}(Y^*_{i,\cdot})e_i^TY^{t,(m)}R^{t,(m)}\right)\left(X^{t,(m)}R^{t,(m)}-X^*\right)_{m,\cdot}\notag\\
&\quad+\left(\frac{\eta}{n^{3/2}}\sum_{i\neq m}\frac{e^{c_i}}{(1+e^{c_i})^2}e_i^TY^{t,(m)}R^{t,(m)}\right)\left(\theta^{t,(m)}_m-\theta^{*}_m\right)\notag\\
&\quad -\frac{\eta}{n}\sum_{i\neq m}\frac{e^{c_i}}{(1+e^{c_i})^2}\left(\frac{1}{\sqrt{n}}\left(\theta^{t,(m)}_i-\theta^{*}_i\right)+\langle H^{t,(m)}-H^*,z_mz_i^T\rangle\right)e_i^TY^{t,(m)}R^{t,(m)}\notag\\
&\quad-\frac{\eta}{n^2}\sum_{i\neq m}\frac{e^{c_i}}{(1+e^{c_i})^2}\left((X^{t,(m)}R^{t,(m)})\left(Y^{t,(m)}R^{t,(m)}-Y^*\right)^T\right)_{mi}e_i^TY^{t,(m)}R^{t,(m)}-\eta\lambda X^{t,(m)}_{m,\cdot}R^{t,(m)}\notag\\
&+\left\{X^{t,(m)}_{m,\cdot}R^{t,(m)}-\eta\left(\frac1n\sum_{i\neq m}\left(\frac{e^{P_{mi}^{t,(m)}}}{1+e^{P_{mi}^{t,(m)}}}-\frac{e^{P_{mi}^*}}{1+e^{P_{mi}^*}}\right)e_i^TY^{t,(m)}+\lambda X^{t,(m)}_{m,\cdot}\right)R^{t,(m)}\right\}\left(\left(R^{t,(m)}\right)^{-1}R^{t+1,(m)}-I_r\right)\notag\\
&=\left(I_r-\frac{\eta}{n^2}\sum_{i\neq m}\frac{e^{c_i}}{(1+e^{c_i})^2}(Y^*_{i,\cdot})(Y^*_{i,\cdot})^{\top}\right)\left(X^{t,(m)}R^{t,(m)}-X^*\right)_{m,\cdot}\notag\\
&\quad+\left(\frac{\eta}{n^{3/2}}\sum_{i\neq m}\frac{e^{c_i}}{(1+e^{c_i})^2}(Y^*_{i,\cdot})\right)\left(\theta^{t,(m)}_m-\theta^{*}_m\right)+r_2,
\end{align}
where
\begin{align*}
r_2&=-\frac{\eta}{n^2}\underbrace{\left(\sum_{i\neq m}\frac{e^{c_i}}{(1+e^{c_i})^2}(Y^*_{i,\cdot})\left(Y^{t,(m)}R^{t,(m)}-Y^{*}\right)_{i,\cdot}^{\top}\right)\left(X^{t,(m)}R^{t,(m)}-X^*\right)_{m,\cdot}}_{(a)}\notag\\
&\quad +\frac{\eta}{n^{3/2}}\underbrace{\left(\sum_{i\neq m}\frac{e^{c_i}}{(1+e^{c_i})^2}\left(Y^{t,(m)}R^{t,(m)}-Y^*\right)_{i,\cdot}\right)\left(\theta^{t,(m)}_m-\theta^{*}_m\right)}_{(b)}\notag\\
&\quad-\frac{\eta}{n}\underbrace{\sum_{i\neq m}\frac{e^{c_i}}{(1+e^{c_i})^2}\left(\frac{1}{\sqrt{n}}\left(\theta^{t,(m)}_i-\theta^{*}_i\right)+\langle H^{t,(m)}-H^*,z_mz_i^T\rangle\right)e_i^TY^{t,(m)}R^{t,(m)}}_{(c)}\\
&\quad-\frac{\eta}{n^2}\underbrace{\sum_{i\neq m}\frac{e^{c_i}}{(1+e^{c_i})^2}\left((X^{t,(m)}R^{t,(m)})\left(Y^{t,(m)}R^{t,(m)}-Y^*\right)^T\right)_{mi}e_i^TY^{t,(m)}R^{t,(m)}}_{(d)}-\eta\lambda \underbrace{X^{t,(m)}_{m,\cdot}R^{t,(m)}}_{(e)}\\
&+\underbrace{\left\{X^{t,(m)}_{m,\cdot}R^{t,(m)}-\eta\left(\frac1n\sum_{i\neq m}\left(\frac{e^{P_{mi}^{t,(m)}}}{1+e^{P_{mi}^{t,(m)}}}-\frac{e^{P_{mi}^*}}{1+e^{P_{mi}^*}}\right)e_i^TY^{t,(m)}+\lambda X^{t,(m)}_{m,\cdot}\right)R^{t,(m)}\right\}\left(\left(R^{t,(m)}\right)^{-1}R^{t+1,(m)}-I_r\right)}_{(f)}
\end{align*}
We bound $\|r_2\|_2$ in the following.
\begin{enumerate}
    
\item For (a), by Cahuchy-Schwarz, we have
\begin{align*}
\| (a)   \|_2\leq \left\|\left(X^{t,(m)}R^{t,(m)}-X^*\right)_{m,\cdot}\right\|_2\|Y^{t,(m)}R^{t,(m)}-Y^*\|_F\|Y^*\|_F.
\end{align*}
Note that
\begin{align*}
&\left\|\left(X^{t,(m)}R^{t,(m)}-X^*\right)_{m,\cdot}\right\|_2\leq c_{31}\\
&\|Y^{t,(m)}R^{t,(m)}-Y^*\|_F\\
&\quad\leq \|Y^{t,(m)}R^{t,(m)}-Y^tR^t\|_F+\|Y^{t}R^{t}-Y^*\|_F\\
&\quad\leq 5\kappa\|Y^{t,(m)}O^{t,(m)}-Y^tR^t\|_F+\|Y^{t}R^{t}-Y^*\|_F\tag{by Lemma \ref{ar:lem2}}\\
&\quad\leq 5\kappa c_{21}+c_{11}\sqrt{n}\\
&\quad \lesssim c_{11}\sqrt{n}\\
&\|Y^*\|_F\leq \sqrt{\mu r\sigma_{\max}}.
\end{align*}
Thus, we have
\begin{align}\label{ineq15:lem_ncv3}
\| (a)   \|_2\lesssim c_{11}c_{31}     \sqrt{\mu r\sigma_{\max}n}.
\end{align}

\item For (b), by Cahuchy-Schwarz, we have
\begin{align}\label{ineq14:lem_ncv3}
\|(b)\|_2\leq \sqrt{n}|\theta^{t,(m)}_m-\theta^{*}_m|\|Y^{t,(m)}R^{t,(m)}-Y^tR^t\|_F\lesssim c_{11}c_{31}n.
\end{align}

\item For (c), note that
\begin{align*}
&\left\|\sum_{i\neq m}\frac{e^{c_i}}{(1+e^{c_i})^2}\left(\frac{1}{\sqrt{n}}\left(\theta^{t,(m)}_i-\theta^{*}_i\right)+\langle H^{t,(m)}-H^*,z_mz_i^T\rangle\right)e_i\right\|_2\\
&\leq \left\|\frac{1}{\sqrt{n}}\sum_{i\neq m}\frac{e^{c_i}}{(1+e^{c_i})^2}\left(\theta^{t,(m)}_i-\theta^{*}_i\right)e_i\right\|_2+ \left\|\sum_{i\neq m}\frac{e^{c_i}}{(1+e^{c_i})^2}\langle H^{t,(m)}-H^*,z_mz_i^T\rangle e_i\right\|_2\\
&\leq\frac{1}{4\sqrt{n}}\left\|\theta^{t,(m)}-\theta^{*}\right\|_2+\frac{1}{4}\sqrt{\sum_{i\neq m}\left|\langle H^{t,(m)}-H^*,z_mz_i^T\rangle\right|^2}\\
&\leq \frac{1}{4\sqrt{n}}\left\|\theta^{t,(m)}-\theta^{*}\right\|_2+\frac{1}{4}\| H^{t,(m)}-H^*\|\|z_m\|_2\sqrt{\sum_{i\neq m}\|z_i\|_2^2}\\
&\leq \frac14\left(\frac{1}{\sqrt{n}}\left\|\theta^{t,(m)}-\theta^{*}\right\|_2+\frac{\sz}{\sqrt{n}}\| H^{t,(m)}-H^*\|\right).
\end{align*}
Moreover, we have
\begin{align*}
    \|Y^{t,(m)}\|\leq  \|F^{t,(m)}O^{t,(m)}-F^tR^t\|+\|F^tR^t-F^*\|+\|F^*\|\leq 2\|F^*\|.
\end{align*}
Thus, we have
\begin{align}\label{ineq16:lem_ncv3}
\|(c)\|_2\leq \|F^*\|\left(\frac{1}{\sqrt{n}}\left\|\theta^{t,(m)}-\theta^{*}\right\|_2+\frac{\sz}{\sqrt{n}}\| H^{t,(m)}-H^*\|\right)\lesssim \sqrt{\sigma_{\max}}\sz c_{11}.
\end{align}

\item For (d), note that
\begin{align*}
&\left\|\sum_{i\neq m}\frac{e^{c_i}}{(1+e^{c_i})^2}\left((X^{t,(m)}R^{t,(m)})\left(Y^{t,(m)}R^{t,(m)}-Y^*\right)^T\right)_{mi}e_i\right\|_2\\
&\leq \frac14 \left\|\left((X^{t,(m)}R^{t,(m)})\left(Y^{t,(m)}R^{t,(m)}-Y^*\right)^T\right)_{m,\cdot}\right\|_2\\
&= \frac14 \left\|(X^{t,(m)}R^{t,(m)})^{\top}_{m,\cdot}\left(Y^{t,(m)}R^{t,(m)}-Y^*\right)^T\right\|_2\\
&\leq \frac14  \left\|(X^{t,(m)}R^{t,(m)})_{m,\cdot}\right\|_2\left\|Y^{t,(m)}R^{t,(m)}-Y^*\right\|\\
&\lesssim  \left\|F^*\right\|_{2,\infty}\left\|Y^{t,(m)}R^{t,(m)}-Y^*\right\|.
\end{align*}
Thus, we have
\begin{align}\label{ineq17:lem_ncv3}
\|(d)\|_2\lesssim \|F^*\|\left\|F^*\right\|_{2,\infty}\left\|Y^{t,(m)}R^{t,(m)}-Y^*\right\|\lesssim \sqrt{\mu\sX\sY r^2 \sigma_{\max}}c_{14}n.
\end{align}

\item For (e), we have
\begin{align}\label{ineq18:lem_ncv3}
\|(e)\|_2\leq \left\|X^{t,(m)}R^{t,(m)}\right\|_{2,\infty}\leq \left\|F^{t,(m)}R^{t,(m)}-F^*\right\|_{2,\infty}+\|F^*\|_{2,\infty}\leq2\|F^*\|_{2,\infty}\lesssim  \sqrt{\mu\sX\sY r^2 n}.
\end{align}

\item Finally, we bound (f).
We denote
\begin{align*}
(1)&:=\left\{X^{t,(m)}_{m,\cdot}R^{t,(m)}-X^*_{m,\cdot}-\eta\left(\frac1n\sum_{i\neq m}\left(\frac{e^{P_{mi}^{t,(m)}}}{1+e^{P_{mi}^{t,(m)}}}-\frac{e^{P_{mi}^*}}{1+e^{P_{mi}^*}}\right)e_i^TY^{t,(m)}+\lambda X^{t,(m)}_{m,\cdot}\right)R^{t,(m)}\right\}\\
&=\left(I_r-\frac{\eta}{n^2}\sum_{i\neq m}\frac{e^{c_i}}{(1+e^{c_i})^2}(Y^*_{i,\cdot})(Y^*_{i,\cdot})^{\top}\right)\left(X^{t,(m)}R^{t,(m)}-X^*\right)_{m,\cdot}\notag\\
&\quad+\left(\frac{\eta}{n^{3/2}}\sum_{i\neq m}\frac{e^{c_i}}{(1+e^{c_i})^2}(Y^*_{i,\cdot})\right)\left(\theta^{t,(m)}_m-\theta^{*}_m\right)-\frac{\eta}{n^2}(a)+\frac{\eta}{n^{3/2}}(b)-\frac{\eta}{n}(c)-\frac{\eta}{n^2}(d)-\eta\lambda (e).
\end{align*}
Note that, by Cauchy-Schwartz, we have
\begin{align*}
&\left\|\sum_{i\neq m}\frac{e^{c_i}}{(1+e^{c_i})^2}(Y^*_{i,\cdot})(Y^*_{i,\cdot})^{\top}\right\|\leq \|Y^*\|_F^2,\\
&\left\|\sum_{i\neq m}\frac{e^{c_i}}{(1+e^{c_i})^2}(Y^*_{i,\cdot})\right\|_2\leq \sqrt{n}\|Y^*\|_F.
\end{align*}
Thus, it can be seen that $\|(1)\|_2\leq \|F^*\|_{2,\infty}$ and we have
\begin{align*}
\|(1)+X^*_{m,\cdot}\|_2\leq \|(1)\|_2+\|X^*_{m,\cdot}\|_2\leq\|(1)\|_2+\|F^*\|_{2,\infty}\leq 2\|F^*\|_{2,\infty}.
\end{align*}
Note that
\begin{align*}
(f)=\left((1)+X^*_{m,\cdot}\right)\left(\left(R^{t,(m)}\right)^{-1}R^{t+1,(m)}-I_r\right).
\end{align*}
Regarding the term $\left(R^{t,(m)}\right)^{-1}R^{t+1,(m)}-I_r$, we have the following claim.
\begin{claim}\label{claim:rotation}
With probability at least $1-n^{-10}$, we have
\begin{align*}
\left\|\left(R^{t,(m)}\right)^{-1}R^{t+1,(m)}-I_r\right\|\lesssim \frac{\eta}{n}\left\| F^{t, (m)}R^{t, (m)}-F^*\right\|.
\end{align*}
\end{claim}
Consequently, we have
\begin{align}\label{ineq19:lem_ncv3}
\|(f)\|_2&\leq \|(1)+X^*_{m,\cdot}\|_2\left\|\left(R^{t,(m)}\right)^{-1}R^{t+1,(m)}-I_r\right\|\notag\\
&\lesssim\frac{\eta}{n}\left\| F^{t, (m)}R^{t, (m)}-F^*\right\|\|F^*\|_{2,\infty}\notag\\
&\lesssim \eta\sqrt{\mu\sX\sY r^2} c_{14}.
\end{align}












It remains to prove Claim \ref{claim:rotation}.
\begin{proof}[Proof of Claim \ref{claim:rotation}]
To facilitate analysis, we introduce an auxiliary point $\tilde{F}^{t+1,(m)}:=\begin{bmatrix}
\tilde{X}^{t+1,(m)}\\
\tilde{Y}^{t+1,(m)}
\end{bmatrix}$ where
\begin{align*}
&\tilde{X}^{t+1,(m)}\\
&={X}^{t,(m)}{R}^{t,(m)}-\eta\left[\frac1n\sum_{\substack{
        i \neq j \\
        i, j \neq m
    }}\left(\frac{e^{P_{ij}^{t,(m)}}}{1+e^{P_{ij}^{t,(m)}}}-A_{ij}\right)e_ie_j^T+\frac1n\sum_{i\neq m}\left(\frac{e^{P_{im}^{t,(m)}}}{1+e^{P_{im}^{t,(m)}}}-\frac{e^{P_{im}^{*}}}{1+e^{P_{im}^{*}}}\right)(e_ie_m^T+e_me_i^T)\right]Y^*\\
&\quad-\eta\lambda X^*-\frac{4c_{\aug}\eta}{n^2}X^*({R}^{t,(m)})^T\left(({X}^{t,(m)})^T{X}^{t,(m)}-({Y}^{t,(m)})^T{Y}^{t,(m)}\right){R}^{t,(m)},\\
&\tilde{Y}^{t+1,(m)}\\
&={Y}^{t,(m)}{R}^{t,(m)}-\eta\left[\frac1n\sum_{\substack{
        i \neq j \\
        i, j \neq m
    }}\left(\frac{e^{P_{ij}^{t,(m)}}}{1+e^{P_{ij}^{t,(m)}}}-A_{ij}\right)e_je_i^T+\frac1n\sum_{i\neq m}\left(\frac{e^{P_{im}^{t,(m)}}}{1+e^{P_{im}^{t,(m)}}}-\frac{e^{P_{im}^{*}}}{1+e^{P_{im}^{*}}}\right)(e_ie_m^T+e_me_i^T)\right]X^*\\
&\quad-\eta\lambda Y^*-\frac{4c_{\aug}\eta}{n^2}Y^*({R}^{t,(m)})^T\left(({Y}^{t,(m)})^T{Y}^{t,(m)}-({X}^{t,(m)})^T{X}^{t,(m)}\right){R}^{t,(m)}.
\end{align*}
We have the following claim.
\begin{claim}\label{claim2:rotation}
It holds that
\begin{align*}
I_r=\argmin_{R\in\cO^{r\times r}}\left\|\tilde{F}^{t+1,(m)}R-F^*\right\|_F,\text{ and } \sigma_{\min}\left(\tilde{F}^{t+1,(m)T}F^{*}\right)\geq \sigma_{\min}/2.
\end{align*}
\begin{proof}[Proof of Claim \ref{claim2:rotation}]
See Claim 4 in \cite{chen2020noisy}.
\end{proof}
\end{claim}
With this claim at hand, by Lemma \ref{ar:lem5} with $S=\tilde{F}^{t+1,(m)T}F^{*}$ and $K=\left({F}^{t+1,(m)}R^{t,(m)}-\tilde{F}^{t+1,(m)}\right)^TF^*$, we have
\begin{align}\label{ineq1:claim2_rotation}
&\left\|\left(R^{t,(m)}\right)^{-1}R^{t+1,(m)}-I_r\right\|\\
&=\left\|\text{sgn}(S+K)-\text{sgn}(S)\right\|\tag{by Claim \ref{claim2:rotation} and the definition of $R^{t+1,(m)}$}\\
&\leq \frac{1}{\sigma_{\min}\left(\tilde{F}^{t+1,(m)T}F^{*}\right)}\left\|\left({F}^{t+1,(m)}R^{t,(m)}-\tilde{F}^{t+1,(m)}\right)^TF^*\right\|\tag{by Lemma \ref{ar:lem5}}\\
&\leq \frac{2}{\sigma_{\min}}\left\|{F}^{t+1,(m)}R^{t,(m)}-\tilde{F}^{t+1,(m)}\right\|\|F^*\|\tag{by Claim \ref{claim2:rotation}}.
\end{align}
Here  \(\text{sgn}(A) = UV^\top\) for a matrix \( A \) with SVD \( U \Sigma V^\top \). Note that
\begin{align*}
    &F^{t+1, (m)} R^{t, (m)} - \tilde{F}^{t+1, (m)} \\
    &= -\eta \begin{bmatrix} B & 0 \\ 0 & B^\top \end{bmatrix} \begin{bmatrix} Y^{t, (m)}R^{t, (m)}-Y^*  \\ X^{t, (m)}R^{t, (m)}-X^* \end{bmatrix} + \frac{4c_{\aug}\eta}{n^2} \begin{bmatrix} X^\star \\ -Y^\star \end{bmatrix} R^{t, (m) \top} C R^{t, (m)} - \eta \lambda\begin{bmatrix}   X^{t, (m)}R^{t, (m)}-X^*\\ Y^{t, (m)}R^{t, (m)}-Y^* \end{bmatrix} ,
\end{align*}
where we denote
\begin{align*}
 &B := \frac1n\sum_{\substack{
        i \neq j \\
        i, j \neq m
    }}\left(\frac{e^{P_{ij}^{t,(m)}}}{1+e^{P_{ij}^{t,(m)}}}-A_{ij}\right)e_ie_j^T+\frac1n\sum_{i\neq m}\left(\frac{e^{P_{im}^{t,(m)}}}{1+e^{P_{im}^{t,(m)}}}-\frac{e^{P_{im}^{*}}}{1+e^{P_{im}^{*}}}\right)(e_ie_m^T+e_me_i^T),\\ 
 &C := X^{t, (m) \top} X^{t, (m)} - Y^{t, (m) \top} Y^{t, (m)}.
\end{align*}
This enables us to obtain
\begin{align*}
 &\left\|F^{t+1, (m)} R^{t, (m)} - \tilde{F}^{t+1, (m)}\right\| \\
& \leq \eta \left\| B \right\| \left\| F^{t, (m)}R^{t, (m)}-F^*\right\| + \frac{4c_{\aug}\eta}{n^2} \left\| F^\star \right\| \left\| C \right\|_F +\eta \lambda\left\| F^{t, (m)}R^{t, (m)}-F^*\right\|.   
\end{align*}
We then bound $\|B\|$ in the following.
Note that
\begin{align*}
B&=\frac1n\sum_{i\neq j}\left(\frac{e^{P_{ij}^{t,(m)}}}{1+e^{P_{ij}^{t,(m)}}}-\frac{e^{P_{ij}^{*}}}{1+e^{P_{ij}^{*}}}\right)e_ie_j^T +   \frac1n\sum_{\substack{
        i \neq j \\
        i, j \neq m
    }}\left(\frac{e^{P_{ij}^{*}}}{1+e^{P_{ij}^{*}}}-A_{ij}\right)e_ie_j^T.
\end{align*}
For the first term, we have
\begin{align*}
&\left\|\sum_{i\neq j}\left(\frac{e^{P_{ij}^{t,(m)}}}{1+e^{P_{ij}^{t,(m)}}}-\frac{e^{P_{ij}^{*}}}{1+e^{P_{ij}^{*}}}\right)e_ie_j^T\right\|\\
&\leq \left\|\sum_{i\neq j}\left(\frac{e^{P_{ij}^{t,(m)}}}{1+e^{P_{ij}^{t,(m)}}}-\frac{e^{P_{ij}^{*}}}{1+e^{P_{ij}^{*}}}\right)e_ie_j^T\right\|_F\\
&=\sqrt{\sum_{i\neq j}\left(\frac{e^{P_{ij}^{t,(m)}}}{1+e^{P_{ij}^{t,(m)}}}-\frac{e^{P_{ij}^{*}}}{1+e^{P_{ij}^{*}}}\right)^2}\\
&=\frac14\sqrt{\sum_{i\neq j}\left(P_{ij}^{t,(m)}-P_{ij}^{*}\right)^2}\tag{by mean value theorem}\\
&\lesssim \sqrt{\su}\left(\|\theta^{t,(m)}-\theta^{*}\|_{2}+\|H^{t,(m)}-H^{*}\|_{F}+\frac{1}{n}\|F^*\|\|F^{t,(m)}R^{t,(m)}-F^{*}\|_{F}\right).
\end{align*}
For the second term, same as bounding $\|\nabla_{\Gamma}L_c(\theta^*,H^*,\Gamma^*)\|$ in the proof of Lemma \ref{lem:gradient_norm}, we have
\begin{align*}
\left\| \frac1n\sum_{\substack{
        i \neq j \\
        i, j \neq m
    }}\left(\frac{e^{P_{ij}^{*}}}{1+e^{P_{ij}^{*}}}-A_{ij}\right)e_ie_j^T\right\|\lesssim\sqrt{\frac{\log n}{n}}.
\end{align*}
Consequently, we have
\begin{align*}
\|B\|&\lesssim \frac{\sqrt{\su}}{n}\left(\|\theta^{t,(m)}-\theta^{*}\|_{2}+\|H^{t,(m)}-H^{*}\|_{F}+\frac{1}{n}\|F^*\|\|F^{t,(m)}R^{t,(m)}-F^{*}\|_{F}\right)+\sqrt{\frac{\log n}{n}}\\
&\lesssim \sqrt{\frac{\overline{C}}{n}}c_{11}+\sqrt{\frac{\log n}{n}}.
\end{align*}
Thus, we have
\begin{align*}
 &\left\|F^{t+1, (m)} R^{t, (m)} - \tilde{F}^{t+1, (m)}\right\| \\
& \leq c\eta\sqrt{\frac{\overline{C}c^2_{11}+\log n}{n}}\left\| F^{t, (m)}R^{t, (m)}-F^*\right\| + \frac{4c_{\aug}\eta}{n^2} \left\| F^\star \right\| \left\|  X^{t, (m) \top} X^{t, (m)} - Y^{t, (m) \top} Y^{t, (m)} \right\|_F \\
&\quad +\eta \lambda\left\| F^{t, (m)}R^{t, (m)}-F^*\right\|.   
\end{align*}
By \eqref{ineq1:claim2_rotation}, we obtain
\begin{align*}
 &\left\|\left(R^{t,(m)}\right)^{-1}R^{t+1,(m)}-I_r\right\|\\
 &\leq \frac{2\|F^*\|}{\sigma_{\min}}  \Bigg(c\eta\sqrt{\frac{\overline{C}c^2_{11}+\log n}{n}}\left\| F^{t, (m)}R^{t, (m)}-F^*\right\| + \frac{4c_{\aug}\eta}{n^2} \left\| F^\star \right\| \left\|  X^{t, (m) \top} X^{t, (m)} - Y^{t, (m) \top} Y^{t, (m)} \right\|_F \\
 &\qquad\qquad\qquad+\eta \lambda\left\| F^{t, (m)}R^{t, (m)}-F^*\right\|\Bigg)\\
  &\lesssim \frac{\|F^*\|}{\sigma_{\min}} \eta \Bigg(\sqrt{\frac{\overline{C}c^2_{11}+\log n}{n}}\left\| F^{t, (m)}R^{t, (m)}-F^*\right\| + c_{\aug}c_{51}\eta\sqrt{\sigma_{\max}} +\lambda\left\| F^{t, (m)}R^{t, (m)}-F^*\right\|\Bigg)\\
&\lesssim \frac{\eta\sqrt{\sigma_{\max}}}{\sigma_{\min}}\left(\sqrt{\frac{\overline{C}c^2_{11}+\log n}{n}}+\lambda\right) \left\| F^{t, (m)}R^{t, (m)}-F^*\right\| \tag{as long as $\eta$ small enough}\\
&\lesssim \frac{\eta}{n}\left\| F^{t, (m)}R^{t, (m)}-F^*\right\|
\end{align*}
as long as $\frac{n\sqrt{\sigma_{\max}}}{\sigma_{\min}}\left(\sqrt{\frac{\overline{C}c^2_{11}+\log n}{n}}+\lambda\right)\lesssim 1$.
We then prove Claim \ref{claim:rotation}.

\end{proof}
\end{enumerate}

Combine \eqref{ineq15:lem_ncv3}, \eqref{ineq14:lem_ncv3}, \eqref{ineq16:lem_ncv3}, \eqref{ineq17:lem_ncv3}, \eqref{ineq18:lem_ncv3}, \eqref{ineq19:lem_ncv3}, we obtain
\begin{align*}
&\|r_2\|_2\\
&\lesssim \eta\left(\frac{1}{n^{3/2}} c_{11}c_{31} \sqrt{\mu r\sigma_{\max}}+\frac{1}{\sqrt{n}}c_{11}c_{31}+\frac{1}{n}\sqrt{\sigma_{\max}}\sz c_{11}+\frac{1}{n}\sqrt{\mu\sX\sY r^2 \sigma_{\max}}c_{14}+\lambda\sqrt{\mu\sX\sY r^2 n}+\sqrt{\mu\sX\sY r^2} c_{14}\right).
\end{align*}

Similarly, we have 
\begin{align}\label{eq20:lem_ncv3}
&\left(F^{t+1,(m)}R^{t+1,(m)}-F^{*}\right)_{m+n,\cdot}\notag\\
&=\left(I_r-\frac{\eta}{n^2}\sum_{i\neq m}\frac{e^{c_i}}{(1+e^{c_i})^2}(X^*_{i,\cdot})(X^*_{i,\cdot})^{\top}\right)\left(Y^{t,(m)}R^{t,(m)}-Y^*\right)_{m,\cdot}\notag\\
&\quad+\left(\frac{\eta}{n^{3/2}}\sum_{i\neq m}\frac{e^{c_i}}{(1+e^{c_i})^2}(X^*_{i,\cdot})\right)\left(\theta^{t,(m)}_m-\theta^{*}_m\right)+r_3,
\end{align}
where
\begin{align*}
&\|r_3\|_2\\
&\lesssim \eta\left(\frac{1}{n^{3/2}} c_{11}c_{31} \sqrt{\mu r\sigma_{\max}}+\frac{1}{\sqrt{n}}c_{11}c_{31}+\frac{1}{n}\sqrt{\sigma_{\max}}\sz c_{11}+\frac{1}{n}\sqrt{\mu\sX\sY r^2 \sigma_{\max}}c_{14}+\lambda\sqrt{\mu\sX\sY r^2 n}+\sqrt{\mu\sX\sY r^2} c_{14}\right).
\end{align*}

By \eqref{eq11:lem_ncv3}, \eqref{eq21:lem_ncv3} and \eqref{eq20:lem_ncv3}, we obtain
\begin{align}\label{ineq58:pf_lem_ncv3}
&\begin{bmatrix}
\theta^{t+1,(m)}_m-\theta^*_m\\
\left(F^{t+1,(m)}R^{t,(m)}-F^{*}\right)_{m,\cdot}\\
\left(F^{t+1,(m)}R^{t,(m)}-F^{*}\right)_{m+n,\cdot}
\end{bmatrix}\notag\\
&=A\begin{bmatrix}
\theta^{t,(m)}_m-\theta^*_m\\
\left(F^{t,(m)}R^{t,(m)}-F^{*}\right)_{m,\cdot}\\
\left(F^{t,(m)}R^{t,(m)}-F^{*}\right)_{m+n,\cdot}
\end{bmatrix}+
\begin{bmatrix}
r_1\\
0\\
0
\end{bmatrix}
+
\begin{bmatrix}
0\\
r_2\\
0
\end{bmatrix}
+
\begin{bmatrix}
0\\
0\\
r_3
\end{bmatrix},
\end{align}
where
\begin{align*}
A&=
\begin{bmatrix}
 1-\frac{2\eta}{n}\sum_{i\neq m}\frac{e^{c_i}}{(1+e^{c_i})^2}&-\frac{\eta}{n^{3/2}}\sum_{i\neq m}\frac{e^{c_i}}{(1+e^{c_i})^2}\left(Y^{*}_{i,\cdot}\right)^T &-\frac{\eta}{n^{3/2}}\sum_{i\neq m}\frac{e^{c_i}}{(1+e^{c_i})^2}(X^*_{i,\cdot})^{\top} \\
 \frac{\eta}{n^{3/2}}\sum_{i\neq m}\frac{e^{c_i}}{(1+e^{c_i})^2}(Y^*_{i,\cdot}) & I_r-\frac{\eta}{n^2}\sum_{i\neq m}\frac{e^{c_i}}{(1+e^{c_i})^2}(Y^*_{i,\cdot})(Y^*_{i,\cdot})^{\top} & 0 \\
\frac{\eta}{n^{3/2}}\sum_{i\neq m}\frac{e^{c_i}}{(1+e^{c_i})^2}(X^*_{i,\cdot})& 0 & I_r-\frac{\eta}{n^2}\sum_{i\neq m}\frac{e^{c_i}}{(1+e^{c_i})^2}(X^*_{i,\cdot})(X^*_{i,\cdot})^{\top}\\
\end{bmatrix}\\
&=I_{2r+1}-\eta\sum_{i\neq m}\frac{e^{c_i}}{(1+e^{c_i})^2}
\begin{bmatrix}
\frac{1}{\sqrt{n}}\\
\frac{1}{n}Y^*_{i,\cdot}\\
0
\end{bmatrix}^{\otimes 2}
-\eta\sum_{i\neq m}\frac{e^{c_i}}{(1+e^{c_i})^2}
\begin{bmatrix}
\frac{1}{\sqrt{n}}\\
0\\
\frac{1}{n}X^*_{i,\cdot}
\end{bmatrix}^{\otimes 2}\\
&=I_{2r+1}-\eta\sum_{i\neq m}\frac{e^{c_i}}{(1+e^{c_i})^2}
\begin{bmatrix}
\frac{1}{\sqrt{n}}\\
\frac{1}{n}e_i^{\top}Y^*\\
0
\end{bmatrix}^{\otimes 2}
-\eta\sum_{i\neq m}\frac{e^{c_i}}{(1+e^{c_i})^2}
\begin{bmatrix}
\frac{1}{\sqrt{n}}\\
0\\
\frac{1}{n}e_i^{\top}X^*
\end{bmatrix}^{\otimes 2}\\
&=I_{2r+1}-\eta\sum_{i\neq m}\frac{e^{c_i}}{(1+e^{c_i})^2}
\left(
\begin{bmatrix}
\frac{1}{\sqrt{n}}\\
\frac{1}{n}e_i^{\top}Y^*\\
0
\end{bmatrix}^{\otimes 2}
+
\begin{bmatrix}
\frac{1}{\sqrt{n}}\\
0\\
\frac{1}{n}e_i^{\top}X^*
\end{bmatrix}^{\otimes 2}
\right).
\end{align*}

Notice that $|P^{t,(m)}_{im}|\leq 2|P^{*}_{im}|$. Thus, by Assumption \ref{assumption:scales}, we have $|c_i|\leq 2|P^{*}_{im}|\leq 2c_P$, which implies
\begin{align*}
\frac{e^{2c_P}}{(1+e^{2c_P})^2}\leq\frac{e^{c_i}}{(1+e^{c_i})^2}\leq \frac14.
\end{align*}
Denote 
\begin{align*}
B:=\sum_{i\neq m}\frac{e^{c_i}}{(1+e^{c_i})^2}
\left(
\begin{bmatrix}
\frac{1}{\sqrt{n}}\\
\frac{1}{n}e_i^{\top}Y^*\\
0
\end{bmatrix}^{\otimes 2}
+
\begin{bmatrix}
\frac{1}{\sqrt{n}}\\
0\\
\frac{1}{n}e_i^{\top}X^*
\end{bmatrix}^{\otimes 2}
\right).
\end{align*}
We then have
\begin{align}\label{ineq56:pf_lem_ncv3}
&\left\|
A\begin{bmatrix}
\theta^{t,(m)}_m-\theta^*_m\\
\left(F^{t,(m)}R^{t,(m)}-F^{*}\right)_{m,\cdot}\\
\left(F^{t,(m)}R^{t,(m)}-F^{*}\right)_{m+n,\cdot}
\end{bmatrix}
\right\|^2_2\notag\\
&=\begin{bmatrix}
\theta^{t,(m)}_m-\theta^*_m\\
\left(F^{t,(m)}R^{t,(m)}-F^{*}\right)_{m,\cdot}\\
\left(F^{t,(m)}R^{t,(m)}-F^{*}\right)_{m+n,\cdot}
\end{bmatrix}^{\top}(I-2\eta B+\eta^2 B^2)
\begin{bmatrix}
\theta^{t,(m)}_m-\theta^*_m\\
\left(F^{t,(m)}R^{t,(m)}-F^{*}\right)_{m,\cdot}\\
\left(F^{t,(m)}R^{t,(m)}-F^{*}\right)_{m+n,\cdot}
\end{bmatrix}\notag\\
&=\left\|
\begin{bmatrix}
\theta^{t,(m)}_m-\theta^*_m\\
\left(F^{t,(m)}R^{t,(m)}-F^{*}\right)_{m,\cdot}\\
\left(F^{t,(m)}R^{t,(m)}-F^{*}\right)_{m+n,\cdot}
\end{bmatrix}
\right\|^2_2
-2\eta \begin{bmatrix}
\theta^{t,(m)}_m-\theta^*_m\\
\left(F^{t,(m)}R^{t,(m)}-F^{*}\right)_{m,\cdot}\\
\left(F^{t,(m)}R^{t,(m)}-F^{*}\right)_{m+n,\cdot}
\end{bmatrix}^{\top}B
\begin{bmatrix}
\theta^{t,(m)}_m-\theta^*_m\\
\left(F^{t,(m)}R^{t,(m)}-F^{*}\right)_{m,\cdot}\\
\left(F^{t,(m)}R^{t,(m)}-F^{*}\right)_{m+n,\cdot}
\end{bmatrix}\notag\\
&\quad +
\eta^2\begin{bmatrix}
\theta^{t,(m)}_m-\theta^*_m\\
\left(F^{t,(m)}R^{t,(m)}-F^{*}\right)_{m,\cdot}\\
\left(F^{t,(m)}R^{t,(m)}-F^{*}\right)_{m+n,\cdot}
\end{bmatrix}^{\top}B^2
\begin{bmatrix}
\theta^{t,(m)}_m-\theta^*_m\\
\left(F^{t,(m)}R^{t,(m)}-F^{*}\right)_{m,\cdot}\\
\left(F^{t,(m)}R^{t,(m)}-F^{*}\right)_{m+n,\cdot}
\end{bmatrix}.
\end{align}

Denote by $L = \text{diag}((1 - 2/n)I_n, I_{r})$ and 
\begin{align*}
B_1:=\sum_{i\neq m}\frac{e^{c_i}}{(1+e^{c_i})^2}
\begin{bmatrix}
\frac{1}{\sqrt{n}}\\
\frac{1}{n}e_i^{\top}Y^*
\end{bmatrix}^{\otimes 2}
,\quad  B_2:=\sum_{i\neq m}\frac{e^{c_i}}{(1+e^{c_i})^2}
\begin{bmatrix}
\frac{1}{\sqrt{n}}\\
\frac{1}{n}e_i^{\top}X^*
\end{bmatrix}^{\otimes 2}.
\end{align*}
Note that $LB_kL$ is a submatrix of $\cP D^*\cP$ ($k=1,2$), so its spectral norm can be controlled as
\begin{align*}
    \left\|LB_k L\right\| \leq \frac{(1+e^{c_P})^2}{4 e^{c_P}}\left\|\cP D^*\cP\right\|\leq \frac{(1+e^{c_P})^2}{4 e^{c_P}}\suD. 
\end{align*}
On the other hand, since $L\succcurlyeq (1-2/n)I_{n+r}$, as long as $n\geq 7$, we have
\begin{align*}
    \left\|B_k\right\|\leq \frac{n^2}{(n-2)^2}\cdot \frac{(1+e^{c_P})^2}{4 e^{c_P}}\suD\leq  \frac{(1+e^{c_P})^2}{2 e^{c_P}}\suD.
\end{align*}
Thus, $\|B\|\leq \|B_1\| + \|B_2\|\leq \frac{(1+e^{c_P})^2}{ e^{c_P}}\suD$. On the other hand we want to lower bound the smallest eigenvalue of $B$. For any $\begin{bmatrix}
\theta\\
\bx\\
\by
\end{bmatrix}$, where $\theta\in \bbR$, $\bx,\by\in\bbR^{r}$, we have
\begin{align}
\begin{bmatrix}
\theta\\
\bx\\
\by
\end{bmatrix}^{\top}B
\begin{bmatrix}
\theta\\
\bx\\
\by
\end{bmatrix}&=
\begin{bmatrix}
\theta\\
\bx
\end{bmatrix}^{\top}
\left(\sum_{i\neq m}
\frac{e^{c_i}}{(1+e^{c_i})^2}
\begin{bmatrix}
\frac{1}{\sqrt{n}}\\
\frac{1}{n}e_i^{\top}Y^*
\end{bmatrix}^{\otimes 2}\right)
\begin{bmatrix}
\theta\\
\bx
\end{bmatrix}
+
\begin{bmatrix}
\theta\\
\by
\end{bmatrix}^{\top}
\left(\sum_{i\neq m}
\frac{e^{c_i}}{(1+e^{c_i})^2}
\begin{bmatrix}
\frac{1}{\sqrt{n}}\\
\frac{1}{n}e_i^{\top}X^*
\end{bmatrix}^{\otimes 2}
\right)
\begin{bmatrix}
\theta\\
\by
\end{bmatrix} \notag \\
&=\begin{bmatrix}
\theta\\
\bx
\end{bmatrix}^{\top}
B_1
\begin{bmatrix}
\theta\\
\bx
\end{bmatrix}
+
\begin{bmatrix}
\theta\\
\by
\end{bmatrix}^{\top}
B_2
\begin{bmatrix}
\theta\\
\by
\end{bmatrix}.\label{pf:lem_ncv3eq3}
\end{align}
Taking advantage of the idea that $LB_1L$ is a submatrix of $\cP D^*\cP$, we denote by $v\in \mathbb{R}^{n(2r+1)+p^2}$ such that 
\begin{align*}
    v_k =
    \begin{cases}
      \theta & \text{if } k=m\\
      x_j & \text{if } k = n+p^2+(m-1)r+j \text{ for some } j\in [r]\\
      0 & \text{otherwise}
    \end{cases}.
\end{align*}
Then we know that 
\begin{align}
    \begin{bmatrix}
\theta\\
\bx
\end{bmatrix}^{\top}
B_1
\begin{bmatrix}
\theta\\
\bx
\end{bmatrix}\geq \begin{bmatrix}
\theta\\
\bx
\end{bmatrix}^{\top}
LB_1L
\begin{bmatrix}
\theta\\
\bx
\end{bmatrix} \geq \frac{4 e^{2 c_P}}{(1+e^{2 c_P})^2} v^\top \cP D^*\cP v. \label{pf:lem_ncv3eq1}
\end{align}
Denote by $Q:=(\cP D^*\cP)^{\dagger}\cP D^*\cP$, then Assumption \ref{assumption:D_eigen} implies
\begin{align}
    v^\top \cP D^*\cP v\geq \slD \left\|Q v\right\|_2^2.\label{pf:lem_ncv3eq2}
\end{align}
On the other hand, we have
\begin{align*}
    \left\|Q v\right\|_2^2&\geq (Q v)_m^2 +\sum_{j=1}^r (Qv)_{n+p^2+(m-1)r+j}^2 \\
    &=\left(v_m - ((I-Q)v)_m\right)^2 +\sum_{j=1}^r \left(v_{n+p^2+(m-1)r+j} - ((I-Q)v)_{n+p^2+(m-1)r+j}\right)^2 \\
    &\geq v_m^2+\sum_{j=1}^r v_{n+p^2+(m-1)r+j}^2 - 2\left(|v_m|+ \sum_{j=1}^r \left| v_{n+p^2+(m-1)r+j}\right|\right)\left\|(I-Q)v\right\|_\infty \\
    &\geq \left\|v\right\|_2^2 - 2\sqrt{r+1}\left\|v\right\|_2\left\|I-Q\right\|_{2,\infty}\left\|v\right\|_2 \geq  \left(1-2c_{2,\infty}\sqrt{\frac{(r+1)(r^2+1)}{n}}\right)\left\|v\right\|_2^2
\end{align*}
according to Assumption \ref{assumption:2_infty}. Therefore, as long as $n\geq 16(r+1)(r^2+1)c_{2,\infty}^2$, we have $\left\|Q v\right\|_2^2\geq \left\|v\right\|_2^2 / 2$. Combine this with \eqref{pf:lem_ncv3eq1} and \eqref{pf:lem_ncv3eq2} we get 
\begin{align*}
    \begin{bmatrix}
\theta\\
\bx
\end{bmatrix}^{\top}
B_1
\begin{bmatrix}
\theta\\
\bx
\end{bmatrix}\geq \frac{4 e^{2 c_P}}{(1+e^{2 c_P})^2}\cdot \frac{\slD}{2}\left\|v\right\|_2^2 = \frac{2 \slD e^{2 c_P}}{(1+e^{2 c_P})^2}\left(\theta^2 +\left\|\bx\right\|_2^2\right). 
\end{align*}
Similarly, we have 
\begin{align*}
    \begin{bmatrix}
\theta\\
\by
\end{bmatrix}^{\top}
B_2
\begin{bmatrix}
\theta\\
\by
\end{bmatrix}\geq\frac{2 \slD e^{2 c_P}}{(1+e^{2 c_P})^2}\left(\theta^2 +\left\|\by\right\|_2^2\right). 
\end{align*}
Plugging these in \eqref{pf:lem_ncv3eq3} we know that 
\begin{align*}
    \begin{bmatrix}
\theta\\
\bx\\
\by
\end{bmatrix}^{\top}B
\begin{bmatrix}
\theta\\
\bx\\
\by
\end{bmatrix}\geq \frac{2 \slD e^{2 c_P}}{(1+e^{2 c_P})^2}\left(\theta^2 +\left\|\bx\right\|_2^2\right)+\frac{2 \slD e^{2 c_P}}{(1+e^{2 c_P})^2}\left(\theta^2 +\left\|\by\right\|_2^2\right)\geq \frac{2 \slD e^{2 c_P}}{(1+e^{2 c_P})^2}\left\|
\begin{bmatrix}
\theta\\
\bx\\
\by
\end{bmatrix}
\right\|^2_2.
\end{align*}
Since this holds for all $\theta\in \bbR$, $\bx,\by\in\bbR^{r}$, we know that 
\begin{align*}
    B\succcurlyeq\frac{2 \slD e^{2 c_P}}{(1+e^{2 c_P})^2} I_{2r+1}.
\end{align*}
To sum up, as long as $n\geq \max\{16(r+1)(r^2+1)c_{2,\infty}^2, 7\}$, we have 
\begin{align*}
   \frac{2 \slD e^{2 c_P}}{(1+e^{2 c_P})^2}  I_{2r+1}\preccurlyeq B\preccurlyeq \frac{(1+e^{c_P})^2}{ e^{c_P}}\suD I_{2r+1}.
\end{align*}






% \newpage
% Denote $X^{*}_i,Y^{*}_i\in\bbR^{r}$ the $i$-th row of $X^*, Y^*$, respectively. We have
% \begin{align}\label{ineq50:pf_lem_ncv3}
% &\sum_{i\neq m}X^{*}_i X^{*\top}_i\preccurlyeq X^{*\top} X^{*}\preccurlyeq \sigma_{\max}I_r
% \end{align}
% and
% \begin{align}\label{ineq51:pf_lem_ncv3}
% \sum_{i\neq m}X^{*}_i X^{*\top}_i
% &=X^{*\top} X^{*}-X^{*}_m X^{*\top}_m\notag\\
% &\succcurlyeq X^{*\top} X^{*}-\|X^*\|_{2,\infty}^2 I_r\notag\\
% &\succcurlyeq \left(\sigma_{\min}-\|X^*\|_{2,\infty}^2\right) I_r\notag\\
% &\succcurlyeq\frac{\sigma_{\min}}{2} I_r.
% \end{align}
% Moreover, we have
% \begin{align}\label{ineq52:pf_lem_ncv3}
% \left\|\sum_{i\neq m}X^{*}_i\right\|_2 \leq n \|X^*\|_{2,\infty}.
% \end{align}
% Similar properties also hold for $Y^{*}_i$.




% For any $\begin{bmatrix}
% \theta\\
% \bx\\
% \by
% \end{bmatrix}$, where $\theta\in \bbR$, $\bx,\by\in\bbR^{r}$, we have
% \begin{align*}
%  &\begin{bmatrix}
% \theta\\
% \bx\\
% \by
% \end{bmatrix}^{\top}B
% \begin{bmatrix}
% \theta\\
% \bx\\
% \by
% \end{bmatrix}\notag\\
% &\leq \frac14\begin{bmatrix}
% \theta\\
% \bx\\
% \by
% \end{bmatrix}^{\top}
% \left(\sum_{i\neq m}
% \begin{bmatrix}
% \frac{1}{\sqrt{n}}\\
% \frac{1}{n}e_i^{\top}Y^*\\
% 0
% \end{bmatrix}^{\otimes 2}
% +
% \begin{bmatrix}
% \frac{1}{\sqrt{n}}\\
% 0\\
% \frac{1}{n}e_i^{\top}X^*
% \end{bmatrix}^{\otimes 2}
% \right)
% \begin{bmatrix}
% \theta\\
% \bx\\
% \by
% \end{bmatrix}\notag\\
% &=\frac14
% \left(
% \begin{bmatrix}
% \theta\\
% \bx
% \end{bmatrix}^{\top}
% \left(\sum_{i\neq m}
% \begin{bmatrix}
% \frac{1}{\sqrt{n}}\\
% \frac{1}{n}e_i^{\top}Y^*
% \end{bmatrix}^{\otimes 2}\right)
% \begin{bmatrix}
% \theta\\
% \bx
% \end{bmatrix}
% +
% \begin{bmatrix}
% \theta\\
% \by
% \end{bmatrix}^{\top}
% \left(\sum_{i\neq m}
% \begin{bmatrix}
% \frac{1}{\sqrt{n}}\\
% \frac{1}{n}e_i^{\top}X^*
% \end{bmatrix}^{\otimes 2}
% \right)
% \begin{bmatrix}
% \theta\\
% \by
% \end{bmatrix}
% \right)\notag\\
% &=\frac14
% \left(
% \begin{bmatrix}
% \theta\\
% \bx
% \end{bmatrix}^{\top}
% \begin{bmatrix}
% \frac{n-1}{n} & \frac{1}{n^{3/2}} \sum_{i\neq m} Y^{*\top}_i\\
% \frac{1}{n^{3/2}} \sum_{i\neq m} Y^{*}_i & \frac{1}{n^2} \sum_{i\neq m} Y^{*}_i Y^{*\top}_i
% \end{bmatrix}
% \begin{bmatrix}
% \theta\\
% \bx
% \end{bmatrix}
% +
% \begin{bmatrix}
% \theta\\
% \by
% \end{bmatrix}^{\top}
% \begin{bmatrix}
% \frac{n-1}{n} & \frac{1}{n^{3/2}} \sum_{i\neq m} X^{*\top}_i\\
% \frac{1}{n^{3/2}} \sum_{i\neq m} X^{*}_i & \frac{1}{n^2} \sum_{i\neq m} X^{*}_i X^{*\top}_i
% \end{bmatrix}
% \begin{bmatrix}
% \theta\\
% \by
% \end{bmatrix}
% \right)\notag\\
% &=\frac14
% \Bigg(
% \frac{2(n-1)}{n}\theta^2+\frac{2\theta}{n^{3/2}}\bx^{\top}\left(\sum_{i\neq m}Y^*_{i}\right)+\frac{1}{n^2}\bx^{\top}\left(\sum_{i\neq m} Y^{*}_i Y^{*\top}_i\right)\bx\notag\\
% &\qquad\qquad\qquad\qquad+\frac{2\theta}{n^{3/2}}\by^{\top}\left(\sum_{i\neq m}X^*_{i}\right)+\frac{1}{n^2}\by^{\top}\left(\sum_{i\neq m} X^{*}_i X^{*\top}_i\right)\by
% \Bigg)\notag\\
% & \leq \frac14
% \left(
% \frac{2(n-1)}{n}\theta^2
% +\frac{2\|X^*\|_{2,\infty}}{\sqrt{n}}|\theta|\|\bx\|_2+\frac{2\|Y^*\|_{2,\infty}}{\sqrt{n}}|\theta|\|\by\|_2+\frac{\sigma_{\max}}{n^2}(\|\bx\|_2^2+\|\by\|_2^2)
% \right)\tag{by \eqref{ineq50:pf_lem_ncv3}, \eqref{ineq52:pf_lem_ncv3}}\\
% & \leq \frac14
% \left(
% \frac{2(n-1)}{n}\theta^2
% +\frac{\|X^*\|_{2,\infty}}{\sqrt{n}}(\theta^2+\|\bx\|_2^2)+\frac{\|Y^*\|_{2,\infty}}{\sqrt{n}}(\theta^2+\|\by\|_2^2)+\frac{\sigma_{\max}}{n^2}(\|\bx\|_2^2+\|\by\|_2^2)
% \right)\notag\\
% &\leq \frac14
% \left(
% \frac{2(n-1)}{n}\theta^2
% +\sqrt{\frac{\mu r \sigma_{\max}}{n^2}}(2\theta^2+\|\bx\|_2^2+\|\by\|_2^2)+\frac{\sigma_{\max}}{n^2}(\|\bx\|_2^2+\|\by\|_2^2)
% \right)\notag\\
% &\leq \left(1+\sqrt{\frac{\mu r \sigma_{\max}}{n^2}}+\frac{\sigma_{\max}}{n^2}\right)
% \left\|
% \begin{bmatrix}
% \theta\\
% \bx\\
% \by
% \end{bmatrix}
% \right\|^2_2,
% \end{align*}
% which implies
% \begin{align}\label{ineq54:pf_lem_ncv3}
%   \|B\|\leq   1+\sqrt{\frac{\mu r \sigma_{\max}}{n^2}}+\frac{\sigma_{\max}}{n^2}.
% \end{align}
% Similarly, we have
% \begin{align}
% &\begin{bmatrix}
% \theta\\
% \bx\\
% \by
% \end{bmatrix}^{\top}B
% \begin{bmatrix}
% \theta\\
% \bx\\
% \by
% \end{bmatrix}\notag\\
% &\geq\frac{e^{2c_P}}{(1+e^{2c_P})^2}
% \left(
% \begin{bmatrix}
% \theta\\
% \bx
% \end{bmatrix}^{\top}
% \begin{bmatrix}
% \frac{n-1}{n} & \frac{1}{n^{3/2}} \sum_{i\neq m} Y^{*\top}_i\\
% \frac{1}{n^{3/2}} \sum_{i\neq m} Y^{*}_i & \frac{1}{n^2} \sum_{i\neq m} Y^{*}_i Y^{*\top}_i
% \end{bmatrix}
% \begin{bmatrix}
% \theta\\
% \bx
% \end{bmatrix}
% +
% \begin{bmatrix}
% \theta\\
% \by
% \end{bmatrix}^{\top}
% \begin{bmatrix}
% \frac{n-1}{n} & \frac{1}{n^{3/2}} \sum_{i\neq m} X^{*\top}_i\\
% \frac{1}{n^{3/2}} \sum_{i\neq m} X^{*}_i & \frac{1}{n^2} \sum_{i\neq m} X^{*}_i X^{*\top}_i
% \end{bmatrix}
% \begin{bmatrix}
% \theta\\
% \by
% \end{bmatrix}
% \right)\notag\\
% &\geq \frac{e^{2c_P}}{(1+e^{2c_P})^2}\left(
% \frac{2(n-1)}{n}\theta^2
% -\frac{\|X^*\|_{2,\infty}}{\sqrt{n}}(\theta^2+\|\bx\|_2^2)-\frac{\|Y^*\|_{2,\infty}}{\sqrt{n}}(\theta^2+\|\bx\|_2^2)+\frac{\sigma_{\min}}{2n^2}(\|\bx\|_2^2+\|\by\|_2^2)
% \right)\tag{by \eqref{ineq51:pf_lem_ncv3}, \eqref{ineq52:pf_lem_ncv3}}\\
% &\geq  \frac{e^{2c_P}}{(1+e^{2c_P})^2} 
% \left(
% \frac{2(n-1)}{n}\theta^2
% -\sqrt{\frac{\mu r \sigma_{\max}}{n^2}}(2\theta^2+\|\bx\|_2^2+\|\by\|_2^2)+\frac{\sigma_{\min}}{2n^2}(\|\bx\|_2^2+\|\by\|_2^2)
% \right)\notag\\
% &=  \frac{2e^{2c_P}}{(1+e^{2c_P})^2} \left(1-\frac{1}{n}-\sqrt{\frac{\mu r \sigma_{\max}}{n^2}}\right)\theta^2+ \frac{e^{2c_P}}{(1+e^{2c_P})^2}\left(\frac{\sigma_{\min}}{2n^2}-\sqrt{\frac{\mu r \sigma_{\max}}{n^2}}\right)(\|\bx\|_2^2+\|\by\|_2^2)\notag\\\label{ineq55:pf_lem_ncv3}
% &\geq \textcolor{red}{???}\left\|
% \begin{bmatrix}
% \theta\\
% \bx\\
% \by
% \end{bmatrix}
% \right\|^2_2.
% \end{align}
% Combine \eqref{ineq56:pf_lem_ncv3}, \eqref{ineq54:pf_lem_ncv3} and \eqref{ineq55:pf_lem_ncv3}, we have

By \eqref{ineq56:pf_lem_ncv3}, we then have
\begin{align*}
&\left\|A
\begin{bmatrix}
\theta^{t+1,(m)}_m-\theta^*_m\\
\left(F^{t+1,(m)}R^{t,(m)}-F^{*}\right)_{m,\cdot}\\
\left(F^{t+1,(m)}R^{t,(m)}-F^{*}\right)_{m+n,\cdot}
\end{bmatrix}
\right\|_2^2\notag\\
&\leq \left(1- \frac{4 \slD e^{2 c_P}}{(1+e^{2 c_P})^2}\eta +\frac{(1+e^{c_P})^4}{ e^{2 c_P}}\suD^2 \eta^2 \right)
\left\|
\begin{bmatrix}
\theta^{t+1,(m)}_m-\theta^*_m\\
\left(F^{t+1,(m)}R^{t,(m)}-F^{*}\right)_{m,\cdot}\\
\left(F^{t+1,(m)}R^{t,(m)}-F^{*}\right)_{m+n,\cdot}
\end{bmatrix}
\right\|_2^2\notag\\
&\leq \left(1-\frac{2 \slD e^{2 c_P}}{(1+e^{2 c_P})^2}\eta\right)\left\|
\begin{bmatrix}
\theta^{t+1,(m)}_m-\theta^*_m\\
\left(F^{t+1,(m)}R^{t,(m)}-F^{*}\right)_{m,\cdot}\\
\left(F^{t+1,(m)}R^{t,(m)}-F^{*}\right)_{m+n,\cdot}
\end{bmatrix}
\right\|_2^2
\end{align*}
as long as $\eta\leq \frac{2e^{4c_{P}}\slD}{(1+e^{2c_P})^6\suD^2}$.
Recall equation \eqref{ineq58:pf_lem_ncv3}. Consequently, we have
\begin{align*}
&\left\|
\begin{bmatrix}
\theta^{t+1,(m)}_m-\theta^*_m\\
\left(F^{t+1,(m)}R^{t,(m)}-F^{*}\right)_{m,\cdot}\\
\left(F^{t+1,(m)}R^{t,(m)}-F^{*}\right)_{m+n,\cdot}
\end{bmatrix}
\right\|_2\\
&\leq
\left\|A
\begin{bmatrix}
\theta^{t,(m)}_m-\theta^*_m\\
\left(F^{t,(m)}R^{t,(m)}-F^{*}\right)_{m,\cdot}\\
\left(F^{t,(m)}R^{t,(m)}-F^{*}\right)_{m+n,\cdot}
\end{bmatrix}
\right\|_2+|r_1|+\|r_2\|_2+\|r_3\|_2\\
&\leq \left(1-\frac{ \slD e^{2 c_P}}{(1+e^{2 c_P})^2}\eta\right)c_{31}+c\frac{\eta\sqrt{\overline{C}}}{\sqrt{n}}c_{21}+ c{\eta(\sqrt{\overline{C}}}+\sz)c_{11}+c\eta\sqrt{\frac{\log n}{n}}+c\eta\sqrt{\mu \sX\sY r^2 }c_{14}\\
&\quad +c\eta\left(\frac{1}{n^{3/2}} c_{11}c_{31} \sqrt{\mu r\sigma_{\max}}+\frac{1}{\sqrt{n}}c_{11}c_{31}+\frac{1}{n}\sqrt{\sigma_{\max}}\sz c_{11}+\frac{1}{n}\sqrt{\mu\sX\sY r^2 \sigma_{\max}}c_{14}+\lambda\sqrt{\mu\sX\sY r^2 n}\right)\\
&\leq c_{31}
\end{align*}
as long as $\max\{\sqrt{\overline{C}}\sz c_{11},\sqrt{\mu\sX\sY r^2 \overline{C}}c_{14}, \lambda\sqrt{\mu\sX\sY r^2 n}\}\lesssim \frac{ \slD e^{2 c_P}}{(1+e^{2 c_P})^2} c_{31}$.


\subsection{Proofs of Lemma \ref{lem:ncv4}}\label{pf:lem_ncv4}
Suppose Lemma \ref{lem:ncv1}-Lemma \ref{lem:ncv5} hold for the $t$-th iteration. In the following, we prove Lemma \ref{lem:ncv4} for the $(t+1)$-th iteration.
Since Lemma \ref{lem:ncv1}-Lemma \ref{lem:ncv5} hold for the $t$-th, we know Lemma \ref{lem:ncv1} holds for the $t+1$-th iteration, which implies $\|H^{t+1}-H^*\|_F\leq c_{11}\sqrt{n}$. For any fixed $m$, we have
\begin{align*}
|\theta^{t+1}_m-\theta^{*}_m|
&\leq |\theta^{t+1,(m)}_m-\theta^{*}_m|+|\theta^{t+1}_m-\theta^{t+1,(m)}_m|\\
&\leq |\theta^{t+1,(m)}_m-\theta^{*}_m|+\|\theta^{t+1}-\theta^{t+1,(m)}\|_2.
\end{align*}
It then holds that
\begin{align*}
\|\theta^{t+1}-\theta^*\|_{\infty}
&=\max_{1\leq m\leq n}|\theta^{t+1}_m-\theta^{*}_m|\\
&\leq \max_{1\leq m\leq n}|\theta^{t+1,(m)}_m-\theta^{*}_m|+\max_{1\leq m\leq n}\|\theta^{t+1}-\theta^{t+1,(m)}\|_2\\
&\leq c_{21}+c_{31}=c_{41},
\end{align*}
where the last inequality holds since Lemma \ref{lem:ncv2} and \ref{lem:ncv3} hold for the $(t+1)$-th iteration.

For $1\leq m\leq n$, we have
\begin{align*}
\left\|\left(F^{t+1}R^{t+1}-F^*\right)_{m,\cdot}\right\|_2
&\leq \left\|\left(F^{t+1,(m)}R^{t+1,(m)}-F^*\right)_{m,\cdot}\right\|_2+ \left\|\left(F^{t+1,(m)}R^{t+1,(m)}-F^{t+1}R^{t+1}\right)_{m,\cdot}\right\|_2\\
&\leq \left\|\left(F^{t+1,(m)}R^{t+1,(m)}-F^*\right)_{m,\cdot}\right\|_2+ \left\|F^{t+1,(m)}R^{t+1,(m)}-F^{t+1}R^{t+1}\right\|_F\\
&\leq \left\|\left(F^{t+1,(m)}R^{t+1,(m)}-F^*\right)_{m,\cdot}\right\|_2+ 5\kappa\left\|F^{t+1,(m)}O^{t+1,(m)}-F^{t+1}R^{t+1}\right\|_F,
\end{align*}
and 
\begin{align*}
\left\|\left(F^{t+1}R^{t+1}-F^*\right)_{m+n,\cdot}\right\|_2
&\leq \left\|\left(F^{t+1,(m)}R^{t+1,(m)}-F^*\right)_{m+n,\cdot}\right\|_2+ \left\|\left(F^{t+1,(m)}R^{t+1,(m)}-F^{t+1}R^{t+1}\right)_{m+n,\cdot}\right\|_2\\
&\leq \left\|\left(F^{t+1,(m)}R^{t+1,(m)}-F^*\right)_{m+n,\cdot}\right\|_2+ \left\|F^{t+1,(m)}R^{t+1,(m)}-F^{t+1}R^{t+1}\right\|_F\\
&\leq \left\|\left(F^{t+1,(m)}R^{t+1,(m)}-F^*\right)_{m+n,\cdot}\right\|_2+ 5\kappa\left\|F^{t+1,(m)}O^{t+1,(m)}-F^{t+1}R^{t+1}\right\|_F,
\end{align*}
where the last inequalities follow from Lemma \ref{ar:lem2}.
It then holds that
\begin{align*}
&\max_{1\leq m\leq n}\left\|\left(F^{t+1}R^{t+1}-F^*\right)_{m,\cdot}\right\|_2\\
&\leq \max_{1\leq m\leq n} \left\|\left(F^{t+1,(m)}R^{t+1,(m)}-F^*\right)_{m,\cdot}\right\|_2+5\kappa\max_{1\leq m\leq n}\left\|F^{t+1,(m)}O^{t+1,(m)}-F^{t+1}R^{t+1}\right\|_F\\
&\leq c_{31}+5\kappa c_{21}=c_{43},\\
&\max_{1\leq m\leq n}\left\|\left(F^{t+1}R^{t+1}-F^*\right)_{m+n,\cdot}\right\|_2\\
&\leq \max_{1\leq m\leq n} \left\|\left(F^{t+1,(m)}R^{t+1,(m)}-F^*\right)_{m+n,\cdot}\right\|_2+5\kappa\max_{1\leq m\leq n}\left\|F^{t+1,(m)}O^{t+1,(m)}-F^{t+1}R^{t+1}\right\|_F\\
&\leq c_{31}+5\kappa c_{21}=c_{43},\\
\end{align*}
where the last inequalities hold since Lemma \ref{lem:ncv2} and \ref{lem:ncv3} hold for the $(t+1)$-th iteration. 
We then finish the proof.











\subsection{Proofs of Lemma \ref{lem:ncv5}}\label{pf:lem_ncv5}
Suppose Lemma \ref{lem:ncv1}-Lemma \ref{lem:ncv5} hold for the $t$-th iteration. In the following, we prove Lemma \ref{lem:ncv5} for the $(t+1)$-th iteration.

First of all, we show that $X^{t+1}(Y^{t+1})^T=Y^{t+1}(X^{t+1})^T$. By the gradient decent update, we have
\begin{align*}
X^{t+1}=X^t-\eta\nabla_X f(M^t,F^t),\quad Y^{t+1}=Y^t-\eta\nabla_Y f(M^t,F^t).
\end{align*}
As a result, we have
\begin{align*}
X^{t+1}(Y^{t+1})^T
&=\left(X^t-\eta\nabla_X f(M^t,F^t)\right)\left(Y^t-\eta\nabla_Y f(M^t,F^t)\right)^T\\
&=X^{t}(Y^{t})^T-\eta X^t\nabla_Y f(M^t,F^t)^T-\eta\nabla_X f(M^t,F^t)(Y^{t})^T+\eta^2\nabla_X f(M^t,F^t)\nabla_Y f(M^t,F^t)^T\\
&=Y^{t}(X^{t})^T-\eta Y^{t}\nabla_X f(M^t,F^t)^T-\eta \nabla_Y f(M^t,F^t)^T (X^t)^T+\eta^2\nabla_Y f(M^t,F^t)\nabla_X f(M^t,F^t)^T\\
&=\left(Y^t-\eta\nabla_Y f(M^t,F^t)\right)\left(X^t-\eta\nabla_X f(M^t,F^t)\right)^T\\
&=Y^{t+1}(X^{t+1})^T,
\end{align*}
where the third equation holds since $X^{t}(Y^{t})^T=Y^{t}(X^{t})^T$. Similarly, we can show $X^{t+1,(m)}(Y^{t+1,(m)})^T=Y^{t+1,(m)}(X^{t+1,(m)})^T$.


Then, we show $\|(X^{t+1})^TX^{t+1}-(Y^{t+1})^TY^{t+1}\|_F\leq c_{51}\eta n^2$. We denote 
\begin{align*}
&A^t=(X^{t})^TX^{t}-(Y^{t})^TY^{t},\ A^{t+1}=(X^{t+1})^TX^{t+1}-(Y^{t+1})^TY^{t+1},\\
&D^t=\frac1n\sum_{i\neq j}\left(\frac{e^{P_{ij}^t}}{1+e^{P_{ij}^t}}-A_{ij}\right)e_i e_j^T.
\end{align*}
Same as Lemma 15 in \cite{chen2020noisy}, it can be seen that
\begin{align}\label{ineq1:lem_ncv5}
\|A^{t+1}\|_F\leq (1-\lambda\eta)\|A^{t}\|_F+\eta^2\|Y^{tT}D^{tT}D^{t}Y^{t}-X^{tT}D^{tT}D^{t}X^{t}\|_F.
\end{align}
Note that
\begin{align*}
\|Y^{tT}D^{tT}D^{t}Y^{t}-X^{tT}D^{tT}D^{t}X^{t}\|_F
&\leq     \|Y^{tT}D^{tT}D^{t}Y^{t}\|_F+\|X^{tT}D^{tT}D^{t}X^{t}\|_F\\
&\leq \|Y^t\|\|D^t\|^2\|Y^t\|_F+\|X^t\|\|D^t\|^2\|X^t\|_F.
\end{align*}
Moreover, by Lemma \ref{lem:ncv1} for the $t$-th iteration, we have
\begin{align*}
&\|X^t\|\leq \|X^tR^t-X^*\|+\|X^*\|\leq 2\|X^*\|,\quad  \|X^t\|_F\leq \|X^tR^t-X^*\|_F+\|X^*\|_F\leq 2\|X^*\|_F,\\
&\|Y^t\|\leq 2\|Y^*\|,\ \|Y^t\|_F\leq 2\|Y^*\|_F.
\end{align*}
Thus, we have
\begin{align*}
 \|Y^{tT}D^{tT}D^{t}Y^{t}-X^{tT}D^{tT}D^{t}X^{t}\|_F
 &\leq 4\|Y^*\|\|Y^*\|_F\|D^t\|^2+4\|X^*\|\|X^*\|_F  \|D^t\|^2
 &\lesssim \sqrt{\mu r}\sigma_{\max}\|D^t\|^2.
\end{align*}
By Lemma \ref{lem:gradient_spectral}, we have
\begin{align*}
 \|D^t\|&\lesssim \sqrt{\frac{c_{11}^2\overline{C}+\log n}{n}}.
\end{align*}
This implies
\begin{align}\label{ineq2:lem_ncv5}
 \|Y^{tT}D^{tT}D^{t}Y^{t}-X^{tT}D^{tT}D^{t}X^{t}\|_F   \lesssim \sqrt{\mu r}\sigma_{\max}\|D^t\|^2\lesssim \frac{\sqrt{\mu r}\sigma_{\max}(c_{11}^2\overline{C}+\log n)}{n}.
\end{align}
Combine \eqref{ineq1:lem_ncv5} and \eqref{ineq2:lem_ncv5}, we have
\begin{align*}
\|A^{t+1}\|_F
&\leq (1-\lambda\eta)\|A^{t}\|_F+C\eta^2\frac{\sqrt{\mu r}\sigma_{\max}(c_{11}^2\overline{C}+\log n)}{n}\\
&\leq (1-\lambda\eta)c_{51}\eta n^2+C\eta^2\frac{\sqrt{\mu r}\sigma_{\max}(c_{11}^2\overline{C}+\log n)}{n}\\
&\leq c_{51}\eta n^2
\end{align*}
as long as $\lambda\eta<1$ and $c_{51}\lambda n^3\gtrsim \sqrt{\mu r}\sigma_{\max} (c_{11}^2\overline{C}+\log n)$.
The upper bound on the leave-one-out sequences can be derived similarly.

Finally, we prove \eqref{ineq:gradient} in the following.
By the gradient descent update, we have
\begin{align*}
&f(M^{t+1},F^{t+1})\\
&=f(M^{t+1},F^{t+1}R^t)\\
&=f\left(M^t-\eta\nabla_{M}f(M^t,F^t)+\eta
\begin{bmatrix}
\mean\left(\nabla_{\theta}f(M^t,F^t)\right)\cdot\mathbf{1}\\
0
\end{bmatrix}, \left(F^t-\eta\nabla_F f(M^t,F^t)\right)R^t\right)\\
&=f(M^t,F^tR^t)-\eta\left\langle\nabla_M f(M^t,F^tR^t),\nabla_{M}f(M^t,F^t)-
\begin{bmatrix}
\mean\left(\nabla_{\theta}f(M^t,F^t)\right)\cdot\mathbf{1}\\
0
\end{bmatrix} \right\rangle\\
&\quad -\eta\left\langle\nabla_F f(M^t,F^tR^t),\nabla_F f(M^t,F^tR^t)\right\rangle\\
&\quad +\frac{\eta^2}{2}
\vec\begin{bmatrix}
\nabla_{M}f(M^t,F^t)-
\begin{bmatrix}
\mean\left(\nabla_{\theta}f(M^t,F^t)\right)\cdot\mathbf{1}\\
0
\end{bmatrix}\\
\nabla_F f(M^t,F^tR^t)
\end{bmatrix}^T \nabla^2 f(\tilde{M},\tilde{F})
\vec\begin{bmatrix}
\nabla_{M}f(M^t,F^t)-
\begin{bmatrix}
\mean\left(\nabla_{\theta}f(M^t,F^t)\right)\cdot\mathbf{1}\\
0
\end{bmatrix}\\
\nabla_F f(M^t,F^tR^t)
\end{bmatrix}\\
&=f(M^t,F^tR^t)-\eta\left\|\nabla_{M}f(M^t,F^t)-
\begin{bmatrix}
\mean\left(\nabla_{\theta}f(M^t,F^t)\right)\cdot\mathbf{1}\\
0
\end{bmatrix} \right\|_F^2 -\eta\left\|\nabla_F f(M^t,F^tR^t)\right\|^2_{F}\\
&\quad +\frac{\eta^2}{2}
\vec\begin{bmatrix}
\nabla_{M}f(M^t,F^t)-
\begin{bmatrix}
\mean\left(\nabla_{\theta}f(M^t,F^t)\right)\cdot\mathbf{1}\\
0
\end{bmatrix}\\
\nabla_F f(M^t,F^tR^t)
\end{bmatrix}^T \nabla^2 f(\tilde{M},\tilde{F})
\vec\begin{bmatrix}
\nabla_{M}f(M^t,F^t)-
\begin{bmatrix}
\mean\left(\nabla_{\theta}f(M^t,F^t)\right)\cdot\mathbf{1}\\
0
\end{bmatrix}\\
\nabla_F f(M^t,F^tR^t)
\end{bmatrix},
\end{align*}
where the last equation follows from the fact that
\begin{align*}
 \left\langle\begin{bmatrix}
\mean\left(\nabla_{\theta}f(M^t,F^t)\right)\cdot\mathbf{1}\\
0
\end{bmatrix},\nabla_{M}f(M^t,F^t)-
\begin{bmatrix}
\mean\left(\nabla_{\theta}f(M^t,F^t)\right)\cdot\mathbf{1}\\
0
\end{bmatrix} \right\rangle   =0.
\end{align*}
By Lemma \ref{lem:convexity}, we have 
\begin{align*}
& \vec\begin{bmatrix}
\nabla_{M}f(M^t,F^t)-
\begin{bmatrix}
\mean\left(\nabla_{\theta}f(M^t,F^t)\right)\cdot\mathbf{1}\\
0
\end{bmatrix}\\
\nabla_F f(M^t,F^tR^t)
\end{bmatrix}^T \nabla^2 f(\tilde{M},\tilde{F})
\vec\begin{bmatrix}
\nabla_{M}f(M^t,F^t)-
\begin{bmatrix}
\mean\left(\nabla_{\theta}f(M^t,F^t)\right)\cdot\mathbf{1}\\
0
\end{bmatrix}\\
\nabla_F f(M^t,F^tR^t)
\end{bmatrix}\\
&\leq \overline{C}\left( \left\|\nabla_{M}f(M^t,F^t)-
\begin{bmatrix}
\mean\left(\nabla_{\theta}f(M^t,F^t)\right)\cdot\mathbf{1}\\
0
\end{bmatrix}\right\|_F^2
+\left\|\nabla_F f(M^t,F^tR^t)\right\|_F^2\right).
\end{align*}
Thus, it holds that
\begin{align*}
&f(M^{t+1},F^{t+1})\\
&\leq f(M^t,F^tR^t)-\left(\eta-\frac{\overline{C}}{2}\eta^2\right)\left(\left\|\nabla_{M}f(M^t,F^t)-
\begin{bmatrix}
\mean\left(\nabla_{\theta}f(M^t,F^t)\right)\cdot\mathbf{1}\\
0
\end{bmatrix} \right\|_F^2+\left\|\nabla_F f(M^t,F^tR^t)\right\|^2_{F}\right) \\
&\leq f(M^t,F^tR^t)-\frac{\eta}{2}\left(\left\|\nabla_{M}f(M^t,F^t)-
\begin{bmatrix}
\mean\left(\nabla_{\theta}f(M^t,F^t)\right)\cdot\mathbf{1}\\
0
\end{bmatrix} \right\|_F^2+\left\|\nabla_F f(M^t,F^tR^t)\right\|^2_{F}\right)\\
&= f(M^t,F^t)-\frac{\eta}{2}
\left\|
\nabla f(M^t,F^t)
-
\begin{bmatrix}
\mean\left(\nabla_{\theta}f(M^t,F^t)\right)\cdot\mathbf{1}\\
0
\end{bmatrix} 
\right\|_F^2
\end{align*}
as long as $\overline{{C}}\eta\leq 1$. We then finish the proofs.











\subsection{Proofs of Lemma \ref{lem:ncv6}}\label{pf:lem_ncv6}
\begin{proof}
Summing \eqref{ineq:gradient} from $t=1$ to $t=t_0$ leads to 
\begin{align*}
&f(M^{t_0},F^{t_0})\leq f(M^{0},F^{0})-\frac{\eta}{2}\sum^{t_0-1}_{t=0}\left\|
\nabla f(M^t,F^t)
-
\begin{bmatrix}
\mean\left(\nabla_{\theta}f(M^t,F^t)\right)\cdot\mathbf{1}\\
0
\end{bmatrix} 
\right\|_F^2.
\end{align*}
Thus, we have
\begin{align}\label{ineq2:lem_ncv6}
&\min_{0\leq t<t_0}\left\|
\nabla f(M^t,F^t)
-
\begin{bmatrix}
\mean\left(\nabla_{\theta}f(M^t,F^t)\right)\cdot\mathbf{1}\\
0
\end{bmatrix} 
\right\|_F\notag\\
&\leq \left(\frac{1}{t_0}\sum^{t_0-1}_{t=0}\left\|
\nabla f(M^t,F^t)
-
\begin{bmatrix}
\mean\left(\nabla_{\theta}f(M^t,F^t)\right)\cdot\mathbf{1}\\
0
\end{bmatrix} 
\right\|_F^2\right)^{1/2}\notag\\
&\leq \left(\frac{2}{\eta t_0}\left(f(M^*,F^*)-f(M^{t_0},F^{t_0})\right)\right)^{1/2},
\end{align}
where we use the fact that $(M^0,F^0)=(M^*,F^*)$. 
Thus, it remains to control $f(M^*,F^*)-f(M^{t_0},F^{t_0})$. Note that
\begin{align*}
 f(M^{t_0},F^{t_0})
 &=f(M^{t_0},F^{t_0}R^{t_0})\\
 &=f(M^*,F^*)+\left\langle\nabla f(M^*,F^*),
 \begin{bmatrix}
M^{t_0}-M^*\\
F^{t_0}R^{t_0}-F^*
 \end{bmatrix}
 \right\rangle\\
 &\quad+\frac12\vec\left(
 \begin{bmatrix}
M^{t_0}-M^*\\
F^{t_0}R^{t_0}-F^*
 \end{bmatrix}
 \right)^T \nabla^2 f(\tilde{M},\tilde{F})
 \vec\left(
 \begin{bmatrix}
M^{t_0}-M^*\\
F^{t_0}R^{t_0}-F^*
 \end{bmatrix}
 \right),
\end{align*}
where $(\tilde{M},\tilde{F})$ lies in the line segment connecting $(M^*,F^*)$ and $(M^{t_0},F^{t_0}R^{t_0})$. By triangle inequality, we have
\begin{align}\label{ineq1:lem_ncv6}
 &f(M^*,F^*)- f(M^{t_0},F^{t_0})\notag\\
 &\leq \|\nabla_{\theta} f(M^*,F^*)\|_2\|\theta^{t_0}-\theta^*\|_2+\|\nabla_{H} f(M^*,F^*)\|_F\|H^{t_0}-H^*\|_F+\|\nabla_{F} f(M^*,F^*)\|_F\|F^{t_0}R^{t_0}-F^*\|_F\notag\\
 &\quad+\frac12\left|\vec\left(
 \begin{bmatrix}
M^{t_0}-M^*\\
F^{t_0}R^{t_0}-F^*
 \end{bmatrix}
 \right)^T \nabla^2 f(\tilde{M},\tilde{F})
 \vec\left(
 \begin{bmatrix}
M^{t_0}-M^*\\
F^{t_0}R^{t_0}-F^*
 \end{bmatrix}
 \right)\right|.
\end{align}
By the gradient decent updating rule, we have $\mathbf{1}^T{\theta^{t_0}}=0$ and thus $\mathbf{1}^T\tilde{\theta}=0$.
Moreover, by Lemma \ref{lem:ncv4}, it holds that
\begin{align*}
&\|\tilde{\theta}-\theta^*\|_{\infty}\leq \|{\theta}^{t_0}-\theta^*\|_{\infty}\leq c_{41}\leq c_1,\\
&\|\tilde{H}-H^*\|_{F}\leq \|{H}^{t_0}-H^*\|_{F}\leq c_{11}\sqrt{n}\leq c_2\sqrt{n},\\
&\|\tilde{F}-F^*\|_{2,\infty}\leq \|{F}^{t_0}{R}^{t_0}-F^*\|_{\infty}\leq c_{43}\leq c_3.
\end{align*}
Thus, by Lemma \ref{lem:convexity}, we have
\begin{align*}
&\frac{1}{2}\left|\vec\left(
 \begin{bmatrix}
M^{t_0}-M^*\\
F^{t_0}R^{t_0}-F^*
 \end{bmatrix}
 \right)^T \nabla^2 f(\tilde{M},\tilde{F})
 \vec\left(
 \begin{bmatrix}
M^{t_0}-M^*\\
F^{t_0}R^{t_0}-F^*
 \end{bmatrix}
 \right)\right|\\
 &\leq \frac{\overline{C}}{2}\left\|
  \begin{bmatrix}
M^{t_0}-M^*\\
F^{t_0}R^{t_0}-F^*
 \end{bmatrix}
 \right\|_F^2\\
 & \leq \frac{\overline{C} c_{11}^2 n}{2},
\end{align*}
where the last inequality follows from Lemma \ref{lem:ncv1}.


Consequently, by \eqref{ineq1:lem_ncv6} and Lemma \ref{lem:gradient_norm}, we have shown that
\begin{align*}
&f(M^*,F^*)- f(M^{t_0},F^{t_0})\\
&\lesssim \sqrt{n\log n}\|\theta^{t_0}-\theta^*\|_2+\sz\sqrt{p\log n}\|H^{t_0}-H^*\|_F+\lambda \sqrt{\mu r\sigma_{\max}}\|F^{t_0}R^{t_0}-F^*\|_F+\overline{C} c_{11}^2 n,
\end{align*}
where we use the fact that $\|X^*\|_F\leq \sqrt{\mu r \sigma_{\max}}$ by Assumption \ref{assumption:incoherent}.
By Lemma \ref{lem:ncv1}, this further implies that
\begin{align*}
&f(M^*,F^*)- f(M^{t_0},F^{t_0})\\
&\lesssim (\sqrt{n\log n}+\sz\sqrt{p\log n}+\lambda \sqrt{\mu r\sigma_{\max}})\cdot c_{11}\sqrt{n}+\overline{C} c_{11}^2 n\\
&= \left(\sqrt{n\log n}+\sz\sqrt{p\log n}+c_{\lambda}\sqrt{\frac{\mu r\sigma_{\max}\log n}{n}}\right)\cdot c_{11}\sqrt{n}+\overline{C} c_{11}^2 n\\
&\lesssim n^2
\end{align*}
as long as $c_{11}\left(\sqrt{\log n}+\sz\sqrt{\log n}+c_{\lambda}\sqrt{\frac{\mu r\sigma_{\max}\log n}{n^2}}+\overline{C}c_{11}\right)\lesssim n$.
Thus, we have
\begin{align*}
\frac{2}{\eta t_0}\left(f(M^*,F^*)-f(M^{t_0},F^{t_0})\right)\lesssim\frac{n^2}{\eta t_0}\leq n^{-10}
\end{align*}
as long as $\eta t_0\geq n^{12}$ (which holds as long as $t_0$ large enough). Together with \eqref{ineq2:lem_ncv6}, we finish the proofs.

\end{proof}

==> proof_proposition4.1_4.2_v1.tex <==
\subsection{Proofs of Proposition \ref{prop:debias_dist}}\label{pf:prop_debias_dist}
Recall that for the debiased estimator $(\hat{\theta}^d,\hat{H}^d,\hat{X}^d,\hat{Y}^d)$, we have
\begin{align}\label{eq1:debias_dist}
\cP\left(\nabla L(\hat{\theta},\hat{H},\hat{X},\hat{Y})+\hat{D}
\begin{bmatrix}
\hat{\theta}^d-\hat{\theta}\\
\hat{H}^d-\hat{H}\\
\hat{X}^d-\hat{X}\\
\hat{Y}^d-\hat{Y}
\end{bmatrix}
\right)=0
\text{ and }
\cP_{\theta}(\hat{\theta}^d) = \hat{\theta}^d.
\end{align}
This implies
\begin{align*}
-\cP \nabla L(\hat{\theta},\hat{H},\hat{X},\hat{Y})
&=\cP \hat{D}
\begin{bmatrix}
\hat{\theta}^d-\hat{\theta}\\
\hat{H}^d-\hat{H}\\
\hat{X}^d-\hat{X}\\
\hat{Y}^d-\hat{Y}
\end{bmatrix}=\cP \hat{D}\cP \begin{bmatrix}
\hat{\theta}^d-\hat{\theta}\\
\hat{H}^d-\hat{H}\\
\hat{X}^d-\hat{X}\\
\hat{Y}^d-\hat{Y}
\end{bmatrix}.
\end{align*}
Consequently, we have
\begin{align*}
\left\|\begin{bmatrix}
\hat{\theta}^d-\hat{\theta}\\
\hat{H}^d-\hat{H}\\
\hat{X}^d-\hat{X}\\
\hat{Y}^d-\hat{Y}
\end{bmatrix}\right\|_F
\leq \frac{1}{\lambda_{\min}(\cP \hat{D}\cP )}\|\cP \nabla L(\hat{\theta},\hat{H},\hat{X},\hat{Y})\|_F.
\end{align*}
Note that by \eqref{ncv:grad}, we have
\begin{align*}
\left\|\nabla L(\hat{\theta},\hat{H},\hat{X},\hat{Y})
-
\begin{bmatrix}
\mean(\nabla_{\theta} L(\hat{\theta},\hat{H},\hat{X},\hat{Y}))\cdot\mathbf{1}\\
0\\
-\lambda\hat{X}\\
-\lambda\hat{Y}
\end{bmatrix}\right\|_F
\lesssim n^{-5}.
\end{align*}
Thus, it holds that
\begin{align*}
\left\|\cP\nabla L(\hat{\theta},\hat{H},\hat{X},\hat{Y})
-
\begin{bmatrix}
0\\
0\\
-\lambda\hat{X}\\
-\lambda\hat{Y}
\end{bmatrix}\right\|_F
&=\left\|\cP\left(\nabla L(\hat{\theta},\hat{H},\hat{X},\hat{Y})
-
\begin{bmatrix}
\mean(\nabla_{\theta} L(\hat{\theta},\hat{H},\hat{X},\hat{Y}))\cdot\mathbf{1}\\
0\\
-\lambda\hat{X}\\
-\lambda\hat{Y}
\end{bmatrix}\right)\right\|_F\\
&\leq \left\|\nabla L(\hat{\theta},\hat{H},\hat{X},\hat{Y})
-
\begin{bmatrix}
\mean(\nabla_{\theta} L(\hat{\theta},\hat{H},\hat{X},\hat{Y}))\cdot\mathbf{1}\\
0\\
-\lambda\hat{X}\\
-\lambda\hat{Y}
\end{bmatrix}\right\|_F\\
&\lesssim n^{-5},
\end{align*}
which then gives
\begin{align*}
\|\cP \nabla L(\hat{\theta},\hat{H},\hat{X},\hat{Y})\|_F
&\leq c n^{-5}+\lambda (\|\hat{X}\|_F+\|\hat{Y}\|_F)  \\
&\leq  c n^{-5}+\lambda (\|\hat{X}-X^*\|_F+\|\hat{Y}-Y^*\|_F)+ \lambda (\|X^*\|_F+\|Y^*\|_F)\\
&\lesssim \lambda \|X^{*}\|_F\\
&\lesssim \lambda\sqrt{\mu r\sigma_{\max}}
\end{align*}
as long as $\|\hat{X}-X^*\|_F\ll \|X^*\|_F$ and $n^{-5}\ll \lambda \|X^*\|_F$.
By Lemma \ref{lem:D}, we have $\lambda_{\min}(\cP \hat{D}\cP )\geq \slD/2$.
As a result, we have
\begin{align*}
 \left\|\begin{bmatrix}
\hat{\theta}^d-\hat{\theta}\\
\hat{H}^d-\hat{H}\\
\hat{X}^d-\hat{X}\\
\hat{Y}^d-\hat{Y}
\end{bmatrix}\right\|_F
\lesssim \frac{{\lambda}\sqrt{\mu r\sigma_{\max}}}{\slD}\lesssim \frac{c_{\lambda}\sqrt{\mu \sX\sY r^2}}{\slD}\sqrt{n\log n}.
\end{align*}













\subsection{Proofs of Proposition \ref{prop:bar_dist}}\label{pf:prop_bar_dist}


Recall that for $(\bar{\theta},\bar{H},\bar{X},\bar{Y})$, we have
\begin{align}\label{eq1:bar_dist}
\cP\left(\nabla L({\theta^{*}},{H^{*}},{X^{*}},{Y^{*}})+{D^{*}}
\begin{bmatrix}
\bar{\theta}-{\theta^{*}}\\
\bar{H}-{H^{*}}\\
\bar{X}-{X^{*}}\\
\bar{Y}-{Y^{*}}
\end{bmatrix}
\right)=0
\text{ and }
\cP_{\theta}(\bar{\theta}) = \bar{\theta}.
\end{align}
This implies
\begin{align*}
-\cP \nabla L({\theta^{*}},{H^{*}},{X^{*}},{Y^{*}})
&=\cP {D^{*}}
\begin{bmatrix}
\bar{\theta}-{\theta^{*}}\\
\bar{H}-{H^{*}}\\
\bar{X}-{X^{*}}\\
\bar{Y}-{Y^{*}}
\end{bmatrix}=\cP {D^{*}}\cP \begin{bmatrix}
\bar{\theta}-{\theta^{*}}\\
\bar{H}-{H^{*}}\\
\bar{X}-{X^{*}}\\
\bar{Y}-{Y^{*}}
\end{bmatrix}.
\end{align*}
Consequently, we have
\begin{align*}
\left\|\begin{bmatrix}
\bar{\theta}-{\theta^{*}}\\
\bar{H}-{H^{*}}\\
\bar{X}-{X^{*}}\\
\bar{Y}-{Y^{*}}
\end{bmatrix}\right\|_F
\leq \frac{1}{\lambda_{\min}(\cP {D^{*}}\cP )}\|\cP \nabla L({\theta^{*}},{H^{*}},{X^{*}},{Y^{*}})\|_F.
\end{align*}
By Lemma \ref{lem:gradient_norm}, we have
\begin{align*}
\left\|\nabla L({\theta^{*}},{H^{*}},{X^{*}},{Y^{*}})
-
\begin{bmatrix}
0\\
0\\
-\lambda{X^{*}}\\
-\lambda{Y^{*}}
\end{bmatrix}\right\|_F
= \|\nabla f({\theta^{*}},{H^{*}},{X^{*}},{Y^{*}})\|_F
\lesssim \sqrt{n\log n}+\lambda   \left(\|X^{*}\|_F+\|Y^{*}\|_F\right).
\end{align*}
Thus, it holds that
\begin{align*}
\left\|\cP\nabla L({\theta^{*}},{H^{*}},{X^{*}},{Y^{*}})
-
\begin{bmatrix}
0\\
0\\
-\lambda{X^{*}}\\
-\lambda{Y^{*}}
\end{bmatrix}\right\|_F
&=\left\|\cP\left(\nabla L({\theta^{*}},{H^{*}},{X^{*}},{Y^{*}})
-
\begin{bmatrix}
0\\
0\\
-\lambda{X^{*}}\\
-\lambda{Y^{*}}
\end{bmatrix}\right)\right\|_F\\
&\leq \left\|\nabla L({\theta^{*}},{H^{*}},{X^{*}},{Y^{*}})
-
\begin{bmatrix}
0\\
0\\
-\lambda{X^{*}}\\
-\lambda{Y^{*}}
\end{bmatrix}\right\|_F\\
&\lesssim\sqrt{n\log n}+\lambda   \left(\|X^{*}\|_F+\|Y^{*}\|_F\right),
\end{align*}
which then gives
\begin{align*}
\|\cP \nabla L({\theta^{*}},{H^{*}},{X^{*}},{Y^{*}})\|_F
&\lesssim \sqrt{n\log n}+\lambda (\|{X^{*}}\|_F+\|{Y^{*}}\|_F)  \\
&\lesssim c_{\lambda} \sqrt{\mu\sX\sY r^2}\cdot\sqrt{n\log n}.
\end{align*}
Note that $\lambda_{\min}(\cP {D^{*}}\cP )\geq \slD$.
As a result, we have
\begin{align*}
 \left\|\begin{bmatrix}
\bar{\theta}-{\theta^{*}}\\
\bar{H}-{H^{*}}\\
\bar{X}-{X^{*}}\\
\bar{Y}-{Y^{*}}
\end{bmatrix}\right\|_F
\lesssim \frac{c_{\lambda}\sqrt{\mu \sX\sY r^2}}{\slD}\sqrt{n\log n}.
\end{align*}




==> real_data_v1.tex <==
\section{Real Data Analysis}
In this section, we apply our model to a stock network. The dataset comprises daily closing prices of S\&P 500 stocks from November 10, 2021, to November 10, 2024, obtained via Yahoo Finance\footnote{\url{https://pypi.org/project/yfinance/}}. We compute the log returns of these prices for our analysis. To clean the data, we exclude stocks with more than one missing value. For stocks with exactly one missing value, we impute the corresponding log return as zero. Next, we construct a stock network based on the correlations of the log returns. Since it is well established that much of the variation in stock excess returns can be attributed to common factors, such as the Fama–French three factors, we first consider to remove the common factors. Specifically, we first remove the first principal component of the log-return matrix, which is largely made up of the entire market portfolio. We then construct the network using the covariance matrix of the idiosyncratic components. Let $ \Sigma $ denote the correlation matrix of the idiosyncratic components. We define an edge between nodes $ i $ and $ j $ if and only if $ \Sigma_{ij} > 0.16 $. This results in an adjacency matrix $ A $. After preprocessing, we retain $ n = 495 $ stocks.

We focus on six covariates: price-to-earnings (PE), price-to-sales (PS), price-to-book (PB), price-to-free-cash-flow (PFCF), debt-to-equity ratio (DER), and return on equity (ROE). 
To obtain these covariates for each firm, we compute the mean values of the relevant financial metrics (e.g., the mean values of price and earnings) within a defined date range, spanning from November 10, 2021, to November 10, 2024, and take the logarithm of the ratio of these means. 
During this computation, we first remove all infinite and missing values. 
Firms were excluded from the analysis if no valid data remained for certain covariates after this adjustment.
For example, firms that recently joined the S\&P 500 might lack sufficient historical data. 
Through this process, we excluded five firms: Altimeter Growth Corp (AMTM), Cboe Global Markets (CBOE), GE Vernova (GEV), Sweetgreen Inc. (SW), and Solvay (SOLV). 
For the remaining firms, if the computed mean values of both financial metrics were positive, the ratio of the means was calculated and capped at a predefined minimum value specific to each covariate. 
Otherwise, a predefined constant specific to the corresponding covariate was used.
We then took the logarithm of the obtained ratio and standardized each covariate across firms. 
This results in a $490\times 6$ covariates matrix $ Z $.
%The resulting distributions of the six covariates are presented in Figure \ref{fig:covariates_distribution}.
After these steps, we retained $ n = 490 $ stocks for our analysis.


%\begin{figure}[h]
%    \centering
%\includegraphics[width=0.8\textwidth]{Figs/covariates_distribution.png}
%    \caption{Distributions of the six standardized covariates (PE, PS, PB, PFCF, DER, and ROE).}
%    \label{fig:covariates_distribution}
%\end{figure}

\paragraph{Vertex properties.}
Using our proposed model, along with the obtained adjacency matrix $ A $ and covariate matrix $ Z $, we employ a Nesterov-accelerated gradient descent method, initialized with zero matrices, to estimate $ \hat{H} $ and $ \hat{\Gamma} $. A nuclear norm penalty is applied to $ \Gamma $ for regularization. The regularization parameter is set to be $43$ and the estimated $\hat{\Gamma}$ has a rank of $3$. The following scatter plot shows the 2-dimensional eigenratio $\hat{r}_i = [(\hat{u}_2)_i / (\hat{u}_1)_i, (\hat{u}_3)_i/(\hat{u}_1)_i]^\top$ of each stock. 

\begin{figure}[h]
    \centering
\includegraphics[width=0.8\textwidth]{Figs/eigenratioplot.png}
    \caption{Scatter plot of the eigenratios of $490$ stocks.}
    \label{fig:eigenratio}
\end{figure}

From Figure \ref{fig:eigenratio} we can see a clear triangle structure, with a few outliers around its periphery. We then remove these outliers and provide zoomed plots of the three vertices. In Figure \ref{fig:threevertices}, Vertex $1$, Vertex $2$ and Vertex $3$ represent the top left, top right and bottom corners in Figure \ref{fig:eigenratio}, and they contains $11.8\%$, $16.1\%$ and $12.7\%$ of the total nodes respectively. We observe some sector clustering effects in each zoomed plot. In the top left panel of Figure \ref{fig:threevertices}, we find that $30\%$ ($9$ out of $30$) of the real estate companies are close to Vertex $1$. As a contrast, one can only find $3$ and $2$ real estate companies in top right and bottom left panels. In the top right panel of Figure \ref{fig:threevertices}, the most noticeable clustering effects are the utilities sector and health care sector. $13$ health care companies can be found in Vertex 2, accounting for $21.31\%$ of all health care companies. As a comparison, there are $7$ and $3$ companies in Vertex $1$ and Vertex $3$ respectively. Similarly, Vertex $2$ contains $22.58\%$ ($7$ out of $31$) of the companies from the utilities sector, and it is much greater than the other vertices. When it comes to Vertex $3$, $23.81\%$ ($5$ out of $21$) communication services companies locate in this corner. For comparison, the numbers of communication services companies in Vertex $1$ and Vertex $2$ are $1$ and $3$. Besides, $19.4\%$ ($13$ out of $67$) information technology can be found in Vertex $3$. Vertex $2$ also has a considerable number ($11$) of information technology companies while Vertex $1$ only has $6$. Not surprisingly, since information technology sector of the largest sectors in the S\&P500, it can be found in different parts of Figure \ref{fig:eigenratio}. The same phenomenon is true of other two biggest sectors: financial and industrial companies are spread across the whole triangle. What's more, we also observe that two smaller sectors, consumer discretionary and consumer staples, distributed throughout the triangle. One possible explanation is that these sectors are more heterogeneous, and companies within the same sector may be doing completely different businesses. For example, big banks, transaction and payment companies (e.g., Visa, PayPal) and Berkshire Hathaway are all classified as financial sector, but their businesses are substantially different. On the contrary, sectors like utilities, real estate and communication services are more homogeneous. Also, The bottom left panel of Figure \ref{fig:threevertices} provides a zoomed-in view of a small area at the center of Figure \ref{fig:eigenratio}. We observe that $9$ out of $22$ energy companies (BKR, CTRA, FANG, EQT, KMI, MPC, OKE, SLB and VLO) are clustered here.

\begin{figure}[ht]
    \centering
\includegraphics[width=0.8\textwidth]{Figs/vertices22.png}
\caption{Zoomed-in plots of the top left, top right and bottom vertices, as well as a center area of Figure \ref{fig:eigenratio}.}
    \label{fig:threevertices}
\end{figure}


\paragraph{Check $R^2$.}
With our observations on the membership structure shown above, let's now turn to the covariates part. Under our identifiability condition $\cP_Z\Gamma = \Gamma\cP_Z = 0$, we can view $\vec(H)$ as the regression coefficients of regressing $\vec(P)$ on 
\begin{align*}
    \left[ \begin{array}{c}
   \vec(z_1z_1^\top)      \\
   \vec(z_2z_1^\top)      \\
   \vec(z_3z_1^\top)      \\
   \vdots  \\
   \vec(z_{n-1}z_n^\top)      \\
   \vec(z_nz_n^\top)      \\
\end{array}
\right]  \in \mathbb{R}^{n^2 \times p^2}
\end{align*}
with $\vec(\Gamma)$ being the residuals. Recall $P$ is defined by $P = ZHZ^\top+\Gamma$ in \eqref{prob:cv}. Therefore, the $R^2$ of the described regression represents the proportion of $P$ that can be explained by the covariates. By the definition of $R^2$, we have
\begin{align*}
    R^2 = 1 - \frac{\left\|\Gamma\right\|_F^2}{\left\|P\right\|_F^2} = 1 - \frac{\left\|\Gamma\right\|_F^2}{\left\|\Gamma\right\|_F^2 + \left\|ZHZ^\top\right\|_F^2} = \frac{\left\|ZHZ^\top\right\|_F^2}{\left\|\Gamma\right\|_F^2 + \left\|ZHZ^\top\right\|_F^2}.
\end{align*}
Plugging our estimated $\hat{H}$ and $\hat{\Gamma}$, we get $R^2 = 0.336$, which means the covariates explain a substantial part of $P$.












%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Test a Covariate-adjusted model or a Covariate-assisted model 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Build on this, we want to further test whether this dataset is suitable for a covariate-adjusted model or a covariate-assisted model.
% \paragraph{Ideas:}
% \begin{enumerate}
%     \item Apply KDE to estimate the continuous joint density $\hat{P}(A_{ij}, z_i, z_j \mid \Pi)$.
%     \item Estimate:     
%     \[
%     \hat{P}(A_{ij} \mid \Pi) = \frac{1}{n^2} \sum_{i, j=1}^n \sum_{k, l=1}^r \Pi_{ik} \Pi_{jl} \mathbf{1}[A_{ij} = A_{ij}].
%     \]

%     \item  Use KDE to estimate: $\hat{P}(z_i,z_j \mid \Pi)$.

%     \item Combine the joint and marginal estimates to compute the WMI:
% \[
% \hat{I}(A; Z \mid \Pi) = \int \sum_{A_{ij}} \hat{P}(A_{ij}, z_i,z_j \mid \Pi) \log \frac{\hat{P}(A_{ij}, z_i,z_j \mid \Pi)}{\hat{P}(A_{ij} \mid \Pi) \hat{P}(z_i,z_j \mid \Pi)} dz.
% \]

% \item
% The test statistic remains:
% \[
% T_{\text{WMI}} = \hat{I}(A; Z \mid \Pi).
% \]

% \item The null hypothesis \( H_0: A \perp Z \mid \Pi \):
% \begin{enumerate}
%     \item \textbf{Permute \( Z \):}  
%     Randomly permute the rows of \( Z \), breaking any dependency between \( A \) and \( Z \) while keeping \( A \) and \( \Pi \) fixed.

%     \item \textbf{Compute \( T_{\text{WMI}} \):}  
%     For each permutation, compute \( \hat{I}(A; Z \mid \Pi) \) to form the null distribution.

%     \item \textbf{Significance Testing:}  
%     Compute the \( p \)-value:
%     \[
%     p = \frac{\text{Number of permuted } T_{\text{WMI}} \geq \text{observed } T_{\text{WMI}}}{\text{Total permutations}}.
%     \]
% \end{enumerate}


% \end{enumerate}





==> settings.tex <==
\section{Basic settings and assumptions}
\subsection{Modeling}

We consider an undirected graph with $n$ nodes and $r$ communities. 
The edge information is incorporated into a symmetric adjacency matrix $\bA=(A_{ij})\in\{0,1\}^{n\times n}$, namely $A_{ij}=1$ if there exists an edge between nodes $i$ and $j$ and $A_{ij}=0$ otherwise. 
We assume each node $i$ is associated with a degree heterogeneity parameter $\theta_i$, a community membership probability vector $\bpi_i=(\pi_i(1),\ldots,\pi_i(r))^T\in\bbR^r$, and a covariates vector $\bz_i\in\bbR^p$. 
Conditional on $\{\bz_i\}^n_{i=1}$, the Bernoulli random variables $\{A_{ij}=A_{ji}:1\leq 1<j\leq n\}$ are assumed to be mutually independent, and for each pair $i<j$:
\begin{align}\label{model}
\bbP\left(A_{ij}=1\mid \bz_i,\bz_j\right)=\frac{e^{\frac{\theta_i+\theta_j}{\sqrt{n}}+\bz^T_i\bH \bz_j+\frac{\bGamma_{ij}}{n}}}{1+e^{\frac{\theta_i+\theta_j}{\sqrt{n}}+\bz^T_i\bH \bz_j+\frac{\bGamma_{ij}}{n}}}.
\end{align}
Here $\bGamma_{ij}$ represents the $(i,j)$ entry of $\bGamma:=\bPi \bP\bPi^{T}$, where $\bPi:=(\bpi_1,\ldots,\bpi_n)^{T}\in\bbR^{n\times r}$ represents the membership matrix, and $\bP\in\bbR^{r\times r}$ is a matrix capturing the connection probability between communities. 
We employ a symmetric matrix $\bH\in\bbR^{p\times p}$ to moderate how the covariates affect the edge formation. 
Only the adjacency matrix $\bA$ and the covariates $\{\bz_i\}^n_{i=1}$ are observed.

\textcolor{red}{Question: what if the model is given by
\begin{align*}
\bbP\left(A_{ij}=1\mid \bz_i,\bz_j\right)=\frac{e^{\frac{\theta_i+\theta_j}{\sqrt{n}}+\bz^T_i\bH \bz_j+\frac{\bGamma_{ij}}{n}-\alpha_n}}{1+e^{\frac{\theta_i+\theta_j}{\sqrt{n}}+\bz^T_i\bH \bz_j+\frac{\bGamma_{ij}}{n}-\alpha_n}}
\end{align*}
to incorporate the situation where the adjacency matrix is sparse, i.e., $\bbP(A_{ij})\rightarrow 0$ when $\alpha_n\rightarrow \infty$.
}

Let $\theta^{*}$, $H^{*}$, and $\Gamma^{*}$ be the ground truth parameters. Suppose the SVD of $\Gamma^{*}$ is given by $U^*\Sigma^*V^{*T}$. We define $X^*=U^*\Sigma^{* 1/2}\in\bbR^{n\times r}$ and $Y^*=V^*\Sigma^{* 1/2}\in \bbR^{n\times r}$, which implies $X^{*T}X^{*}=Y^{*T}Y^{*}$. Denote $\sigma_{\max}$ and $\sigma_{\min}$ the largest and smallest non-zero singular value of $\Gamma^{*}$, respectively. And we denote $\kappa=\sigma_{\max}/\sigma_{\min}$. For identifiability, we assume $\mathbf{1}^T\theta^{*}=0$.

\subsection{Convex and nonconvex problem}
We define
\begin{itemize}
    \item Nonconvex logistic loss:
    \begin{align}\label{obj:ncv_loss}
        L(\boldsymbol{\theta},\boldsymbol{H},\boldsymbol{X}, \boldsymbol{Y})= \sum_{i\neq j}\log(1+e^{P_{ij}})  - A_{ij}P_{ij} ,
        \text{where }P_{ij} = \frac{\theta_i+\theta_j}{\sqrt{n}}+\boldsymbol{z}_i^\top\boldsymbol{H}\boldsymbol{z}_j + \frac{(\boldsymbol{X}\boldsymbol{Y}^\top)_{ij}}{n}
    \end{align}
    Nonconvex objective:
    \begin{align}\label{obj:ncv}
        f(\boldsymbol{\theta},\boldsymbol{H},\boldsymbol{X}, \boldsymbol{Y}) = L(\boldsymbol{\theta},\boldsymbol{H},\boldsymbol{X}, \boldsymbol{Y})+\frac{\lambda}{2}\left\|\boldsymbol{X}\right\|_F^2 + \frac{\lambda}{2}\left\|\boldsymbol{Y}\right\|_F^2
    \end{align}
    \item Convex logistic loss:
    \begin{align}\label{obj:cv_loss}
        &L_c(\boldsymbol{\theta},\boldsymbol{H},\boldsymbol{\Gamma})= \sum_{i\neq j}\log(1+e^{P_{ij}})  - A_{ij}P_{ij}  ,
        &\text{where }P_{ij} = \frac{\theta_i+\theta_j}{\sqrt{n}}+\boldsymbol{z}_i^\top\boldsymbol{H}\boldsymbol{z}_j + \frac{\Gamma_{ij}}{n}
    \end{align}
    Convex objective:
    \begin{align}\label{obj:cv}
        f_c(\boldsymbol{\theta},\boldsymbol{H},\boldsymbol{\Gamma}) = L_c(\boldsymbol{\theta},\boldsymbol{H},\boldsymbol{\Gamma})+{\lambda}\left\|\boldsymbol{\Gamma}\right\|_{*}
    \end{align}
\end{itemize}


\subsection{Gradients}
We summarize the gradients of the loss functions in the following.

For nonconvex logistic loss, for the first derivative,  we have
\begin{align*}
& \nabla_{\theta}L(\theta,H,X,Y)=\frac{1}{\sqrt{n}}\sum_{i\neq j}\left(\frac{e^{P_{ij}}}{1+e^{P_{ij}}}-A_{ij}\right)(e_i+e_j)\in\bbR^n,\\   &\nabla_{H}L(\theta,H,X,Y)=\sum_{i\neq j}\left(\frac{e^{P_{ij}}}{1+e^{P_{ij}}}-A_{ij}\right)z_iz_j^T\in\bbR^{p\times p},\\
& \nabla_{X}L(\theta,H,X,Y)=\frac{1}{n}\sum_{i\neq j}\left(\frac{e^{P_{ij}}}{1+e^{P_{ij}}}-A_{ij}\right)e_ie_j^T Y\in\bbR^{n\times r},\\ 
& \nabla_{Y}L(\theta,H,X,Y)=\frac{1}{n}\sum_{i\neq j}\left(\frac{e^{P_{ij}}}{1+e^{P_{ij}}}-A_{ij}\right)e_je_i^T X\in\bbR^{n\times r}.
\end{align*}
For nonconvex logistic loss, for the second derivative,  we have
\begin{align*}
& \nabla_{\theta}^2L(\theta,H,X,Y)=\frac{1}{n}\sum_{i\neq j}\frac{e^{P_{ij}}}{(1+e^{P_{ij}})^2}(e_i+e_j)(e_i+e_j)^T,\\ 
& \nabla_{\theta,H}^2L(\theta,H,X,Y)=\frac{1}{\sqrt{n}}\sum_{i\neq j}\frac{e^{P_{ij}}}{(1+e^{P_{ij}})^2}(e_i+e_j)\otimes (z_iz_j^T),\\ 
& \nabla_{\theta,X}^2L(\theta,H,X,Y)=\frac{1}{n^{\frac32}}\sum_{i\neq j}\frac{e^{P_{ij}}}{(1+e^{P_{ij}})^2}(e_i+e_j)\otimes (e_ie_j^T Y),\\ 
& \nabla_{\theta,Y}^2L(\theta,H,X,Y)=\frac{1}{n^{\frac32}}\sum_{i\neq j}\frac{e^{P_{ij}}}{(1+e^{P_{ij}})^2}(e_i+e_j)\otimes (e_je_i^T X),\\ 
& \nabla_{H}^2L(\theta,H,X,Y)=\sum_{i\neq j}\frac{e^{P_{ij}}}{(1+e^{P_{ij}})^2}(z_iz_j^T)^{\otimes 2},\\
& \nabla_{H,X}^2L(\theta,H,X,Y)=\frac{1}{n}\sum_{i\neq j}\frac{e^{P_{ij}}}{(1+e^{P_{ij}})^2}(z_iz_j^T)\otimes (e_ie_j^T Y),\\
&\nabla_{H,Y}^2L(\theta,H,X,Y)=\frac1n\sum_{i\neq j}\frac{e^{P_{ij}}}{(1+e^{P_{ij}})^2}(z_iz_j^T)\otimes (e_je_i^T X),\\
& \nabla_{X}^2L(\theta,H,X,Y)=\frac{1}{n^2}\sum_{i\neq j}\frac{e^{P_{ij}}}{(1+e^{P_{ij}})^2}(e_ie_j^T Y)^{\otimes 2},\\
& \nabla_{X,Y}^2L(\theta,H,X,Y)=\frac{1}{n^2}\sum_{i\neq j}\frac{e^{P_{ij}}}{(1+e^{P_{ij}})^2}(e_ie_j^T Y)\otimes (e_je_i^T X)+\frac{1}{n}\sum_{i\neq j}\left(\frac{e^{P_{ij}}}{1+e^{P_{ij}}}-A_{ij}\right)e_ie_j^T\otimes I_r,\\
& \nabla_{Y}^2L(\theta,H,X,Y)=\frac{1}{n^2}\sum_{i\neq j}\frac{e^{P_{ij}}}{(1+e^{P_{ij}})^2}(e_je_i^T X)^{\otimes 2}.
\end{align*}
Here we view all the matrices as vectors and for vectors $u,v$, we define $u\otimes v = uv^T$, which is a matrix. The term $e_ie_j^T\otimes I_r$ is the Kronecker product between matrics, which results in an $nr\times nr$ matrix. The above second order derivative leads to the fact that
\begin{align*}
\nabla^2  L(\theta,H,X,Y)&= \sum_{i\neq j}\frac{e^{ P_{ij}}}{(1+e^{ P_{ij}})^2} 
\begin{bmatrix}
\frac{{e}_i+{e}_j}{\sqrt{n}}\\
{z}_i{z}_j^T\\
\frac{{e}_i{e}_j^T{Y}}{n}\\
\frac{{e}_j{e}_i^T{X}}{n}
\end{bmatrix}^{\otimes 2}\\
&\quad+\frac{1}{n}\sum_{i\neq j}\left(\frac{e^{P_{ij}}}{1+e^{P_{ij}}}-A_{ij}\right)e_ie_j^T\otimes I_r+\frac{1}{n}\sum_{i\neq j}\left(\frac{e^{P_{ij}}}{1+e^{P_{ij}}}-A_{ij}\right)e_je_i^T\otimes I_r.
\end{align*}

For convex logistic loss, for the first derivative,  we have
\begin{align*}
& \nabla_{\theta}L_c(\theta,H,\Gamma)=\frac{1}{\sqrt{n}}\sum_{i\neq j}\left(\frac{e^{P_{ij}}}{1+e^{P_{ij}}}-A_{ij}\right)(e_i+e_j)\in\bbR^n,\\   &\nabla_{H}L_c(\theta,H,\Gamma)=\sum_{i\neq j}\left(\frac{e^{P_{ij}}}{1+e^{P_{ij}}}-A_{ij}\right)z_iz_j^T\in\bbR^{p\times p},\\
& \nabla_{\Gamma}L_c(\theta,H,\Gamma)=\frac{1}{n}\sum_{i\neq j}\left(\frac{e^{P_{ij}}}{1+e^{P_{ij}}}-A_{ij}\right)e_ie_j^T \in\bbR^{n\times r}.
\end{align*}

For convex logistic loss, for the second derivative,  we have
\begin{align*}
& \nabla_{\theta}^2L_c(\theta,H,\Gamma)=\frac{1}{n}\sum_{i\neq j}\frac{e^{P_{ij}}}{(1+e^{P_{ij}})^2}(e_i+e_j)(e_i+e_j)^T,\\ 
& \nabla_{\theta,H}^2L_c(\theta,H,\Gamma)=\frac{1}{\sqrt{n}}\sum_{i\neq j}\frac{e^{P_{ij}}}{(1+e^{P_{ij}})^2}(e_i+e_j)\otimes (z_iz_j^T),\\ 
& \nabla_{\theta,\Gamma}^2L_c(\theta,H,\Gamma)=\frac{1}{n^{\frac32}}\sum_{i\neq j}\frac{e^{P_{ij}}}{(1+e^{P_{ij}})^2}(e_i+e_j)\otimes (e_ie_j^T ),\\ 
& \nabla_{H}^2L_c(\theta,H,\Gamma)=\sum_{i\neq j}\frac{e^{P_{ij}}}{(1+e^{P_{ij}})^2}(z_iz_j^T)^{\otimes 2},\\
& \nabla_{H,\Gamma}^2L_c(\theta,H,\Gamma)=\frac{1}{n}\sum_{i\neq j}\frac{e^{P_{ij}}}{(1+e^{P_{ij}})^2}(z_iz_j^T)\otimes (e_ie_j^T ),\\
& \nabla_{\Gamma}^2L_c(\theta,H,\Gamma)=\frac{1}{n^2}\sum_{i\neq j}\frac{e^{P_{ij}}}{(1+e^{P_{ij}})^2}(e_ie_j^T )^{\otimes 2},
\end{align*}
which implies 
\begin{align*}
\nabla^2  L_c(\theta,H,\Gamma)= \sum_{i\neq j}\frac{e^{ P_{ij}}}{(1+e^{ P_{ij}})^2} 
\begin{bmatrix}
\frac{{e}_i+{e}_j}{\sqrt{n}}\\
{z}_i{z}_j^T\\
\frac{{e}_i{e}_j^T}{n}
\end{bmatrix}^{\otimes 2}.
\end{align*}

\subsection{Assumptions}\label{sec:assumptions}
\begin{enumerate}
    \item  We make the following scale assumption on the ground truth parameters.
    \begin{assumption}[Scale Assumption]\label{assumption:scales}
    There are some constants $\stheta$, $\sH$, $\sX$, $\sY$, and $\sz$ such that the following holds:
    \begin{align*}
    \|\theta^*\|_{\infty}\leq \stheta \sqrt{n},\quad
    \|H^*\|_2\leq \sH n,\quad
    \|X^*\|_{\infty}\leq \sX \sqrt{n},\quad
     \|Y^*\|_{\infty}\leq \sY \sqrt{n},\quad
     \max_{1\leq i\leq n}\|z_i\|_2\leq \sqrt{\frac{c_z}{n}}.
    \end{align*}
    \end{assumption}

    \begin{remark}
    From this assumption, it can be seen that $\|\Gamma^*\|_{\infty}\leq \sX\sY rn$ and $\|\Gamma^*\|_F\leq \sX\sY rn^2$. Consequently, we have $\sigma_{\min}\leq \sX\sY \sqrt{r}n^2$ and $\sigma_{\max}\leq \sX\sY rn^2$. Moreover, we have $|P_{ij}^*|\leq 2\stheta+\sz\sH+\sX\sY r$. For notation simplicity, we denote $c_P:=2\stheta+\sz\sH+\sX\sY r$ in the following.
    \end{remark}
    \textcolor{blue}{Previous version: \textbf{Scales}: $\theta^{*}$ entry-wise $O(\sqrt{n})$, $H^{*}$ entry-wise $O(n)$, $X^{*}$ and $Y^{*}$ entry-wise $O(\sqrt{n})$, and the covariates vectors $z_i$ entry-wise $O(\frac{1}{\sqrt{n}})$. Thus, we have $\Gamma^*$ entry-wise $O(n)$ and $\sigma_{\max},\sigma_{\min}\sim O(n^2)$. We set $\lambda=O(\frac{1}{\sqrt{n}})$.}

    \item We make the following assumptions on the eigenvalues.
    \begin{assumption}[Balanced Eigenvalues]\label{assumption:eigenvalues}
    We assume there exists some constants $\su$ and $\sl$ such that
    \begin{align*}
\su&\geq
\lambda_{\max}\left(\cP_{c}\left(\sum_{i, j}
  \begin{bmatrix}
  \frac{1}{\sqrt{n}}\vec(e_i+e_j)\\
  \vec(z_iz_j^T)\\
  \vec(e_ie_j^T)
  \end{bmatrix}
   \begin{bmatrix}
  \frac{1}{\sqrt{n}}\vec(e_i+e_j)\\
  \vec(z_iz_j^T)\\
  \vec(e_ie_j^T)
  \end{bmatrix}^T
\right)\cP_{c}\right)\\
&\geq\lambda_{\min}\left(\cP_{c}\left(\sum_{i, j}
  \begin{bmatrix}
  \frac{1}{\sqrt{n}}\vec(e_i+e_j)\\
  \vec(z_iz_j^T)\\
  \vec(e_ie_j^T)
  \end{bmatrix}
   \begin{bmatrix}
  \frac{1}{\sqrt{n}}\vec(e_i+e_j)\\
  \vec(z_iz_j^T)\\
  \vec(e_ie_j^T)
  \end{bmatrix}^T
\right)\cP_{c}\right)
\geq \sl,
    \end{align*}
where $\lambda_{\max}(\cdot), \lambda_{\min}(\cdot)$ represents the largest and smallest non-zero eigenvalues of the corresponding matrix, and $e_i\in\bbR^n$ is the one-hot vector.
Here $\cP_c$ is a projection matrix defined as
\begin{align}\label{def:projection_cvx}
\cP_c:=
\begin{bmatrix}
\cP_{\theta} & \\
 & I
\end{bmatrix}
\text{ where }
\cP_{\theta}:=I_n-\frac1n \mathbf{1} \mathbf{1}^T
\text{ and }
I=
\begin{bmatrix}
I_H & \\
 & I_{\Gamma} 
\end{bmatrix}.
\end{align}  
\end{assumption}



\item We make the following incoherent assumption on the ground truth $U^*$ and $V^*$.
\begin{assumption}[Incoherent]\label{assumption:incoherent}
Let $U^*\Sigma^* V^{*\top}$ be the SVD of the ground truth rank-$r$ matrix $\Gamma^*\in\bbR^{n\times n}$. We assume $\Gamma^*$ is $\mu$-incoherent, that is to say
\begin{align*}
\|U^*\|_{2,\infty}\leq \sqrt{\frac{\mu}n}\|U^*\|_F=\sqrt{\frac{\mu r}{n}},\quad
\|V^*\|_{2,\infty}\leq \sqrt{\frac{\mu}n}\|V^*\|_F=\sqrt{\frac{\mu r}{n}}.
\end{align*}
\end{assumption}
\begin{remark}
By the above assumption, we have
\begin{align*}
&\|X^*\|_{2,\infty}=\|U^*\Sigma^{* 1/2}\|_{2,\infty}\leq \sqrt{\frac{\mu r \sigma_{\max}}{n}}\leq \sqrt{\mu \sX\sY r^2 n}\\
&\|Y^*\|_{2,\infty}=\|V^*\Sigma^{* 1/2}\|_{2,\infty}\leq \sqrt{\frac{\mu r \sigma_{\max}}{n}}\leq \sqrt{\mu \sX\sY r^2 n},
\end{align*}
which are of the order $\sqrt{n}$. Moreover, we have $\|X^*\|_F\leq \sqrt{n}\|X^*\|_{2,\infty}\leq \sqrt{\mu r\sigma_{\max}}$ and $\|Y^*\|_F\leq \sqrt{n}\|Y^*\|_{2,\infty}\leq \sqrt{\mu r\sigma_{\max}}$.
\end{remark}


\item \textbf{Choice of $\lambda$ and other conditions:}
In the following sections, we will choose the regularization parameter 
\begin{align*}
\lambda = c_{\lambda}\sqrt{\frac{\log n}{n}}
\end{align*}
for some large enough constant $c_{\lambda}>0$. We also assume the sample size obeys (\ntd).

%     \item \textbf{Balanced eigenvalues}: When constrained on the space that $\mathbf{1}^T\theta=\sum_{i=1}^{n}\theta_i=0$, we have
%     \begin{align*}
% \lambda\left(\sum_{i\neq j}
%   \begin{bmatrix}
%   \frac{1}{\sqrt{n}}\vec(e_i+e_j)\\
%   \vec(z_iz_j^T)\\
%   \vec(e_ie_j^T)
%   \end{bmatrix}
%    \begin{bmatrix}
%   \frac{1}{\sqrt{n}}\vec(e_i+e_j)\\
%   \vec(z_iz_j^T)\\
%   \vec(e_ie_j^T)
%   \end{bmatrix}^T
% \right)=O(1).
%     \end{align*}
% Here $\lambda(\cdot)$ represents the eigenvalues of the corresponding matrix and $e_i\in\bbR^n$ is the one-hot vector.
    % \item \textbf{RIP condition}:
    % For any $H\in\bbR^{p\times p}$, we have
    % \begin{align*}
    % \sum_{i\neq j}\left|\langle H, z_iz_j^T \rangle\right|^2=\Theta(\|H\|_F^2).
    % \end{align*}
\end{enumerate}



